Zodiacal Exoplanets in Time (ZEIT) V: A Uniform Search for Transiting Planets in Young Clusters Observed by K2

Detection of transiting exoplanets around young stars is more difficult than for older systems due to increased stellar variability. Nine young open cluster planets have been found in the K2 data, but no single analysis pipeline identified all planets. We have developed a transit search pipeline for young stars which uses a transit-shaped notch and quadratic continuum in a 12 or 24\,hour window to fit both the stellar variability and the presence of a transit. In addition, for the most rapid rotators (P$_\mathrm{rot}<2$\,days) we model the variability using a linear combination of observed rotations of each star. To maximally exploit our new pipeline, we update the membership for four stellar populations observed by K2 (Upper Scorpius, Pleiades, Hyades, Praesepe), and conduct a uniform search of the members. We identify all known transiting exoplanets in the clusters, 17 eclipsing binaries, one transiting planet candidate orbiting a potential Pleiades member, and three orbiting unlikely members of the young clusters. Limited injection-recovery testing on the known planet hosts indicates that for the older Praesepe systems, we are sensitive to additional exoplanets as small as 1-2\,R$_\oplus$, and for the larger Upper Scorpius planet host (K2-33) our pipeline is sensitive to $\sim$4\,R$_\oplus$ transiting planets. The lack of detected multiple systems in the young clusters is consistent with the expected frequency from the original Kepler sample, within our detection limits. With a robust pipeline that detects all known planets in the young clusters, occurrence rate testing at young ages is now possible.

==> Hy_memtable.tex <==
\begin{deluxetable}{cccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Candidate Hyades members.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} \\ } 
 \startdata 
210317378 & 03 52 34.34 & +11 15 38.8 & 12.42 & 9.01 & 179.36$\pm$1.64 & -5.5$\pm$1.64 & 29.7$\pm$4.1$^{(1)}$ & 136.6 & -1.9 & 89 &  \\ 
210359769 & 03 55 01.44 & +12 29 08.1 & 9.68 & 7.57 & 131.22$\pm$0.17 & -10.25$\pm$0.08 & 21.8$\pm$0.2$^{(0)}$ & 136.8 & -5.6 & 100 &  \\ 
210365286 & 03 58 14.38 & +12 37 40.9 & 14.87 & 10.99 & 129.36$\pm$2.16 & -12.5$\pm$2.16 & 24.9$\pm$3.4$^{(1)}$ & 132.8 & -6.3 & 99 & 0.8686\\ 
210371851 & 04 11 06.42 & +12 47 48.2 & 16.31 & 11.84 & 136.54$\pm$3.03 & -17.97$\pm$2.89 & 29.5$\pm$4.1$^{(1)}$ & 123.9 & -8.4 & 98 & 0.8968\\ 
210384590 & 03 58 35.82 & +13 06 18.1 & 8.8 & 7.38 & 81.0$\pm$0.73 & -6.65$\pm$0.55 & 16.6$\pm$0.3$^{(0)}$ & 102.0 & -5.9 & 48 &  \\ 
210392845 & 04 14 37.70 & +13 17 53.8 &   & 13.73 & 94.6$\pm$5.5 & -24.7$\pm$5.5 & 22.4$\pm$3.1$^{(4)}$ & 121.4 & -10.3 & 97 &  \\ 
210408563 & 04 17 47.69 & +13 39 42.4 & 11.6 & 8.53 & 108.21$\pm$2.37 & -18.23$\pm$2.37 & 22.2$\pm$3.1$^{(1)}$ & 119.1 & -11.7 & 99 & 8.685\\ 
210419589 & 04 00 44.96 & +13 54 22.7 & 13.1 & 9.34 & 129.0$\pm$2.41 & -14.86$\pm$2.41 & 43.0$\pm$5.9$^{(1)}$ & 131.1 & -10.2 & 49 & 2.6612\\ 
210425611 & 04 19 57.70 & +14 02 06.7 & 5.54 &   & 115.45$\pm$0.23 & -19.07$\pm$0.17 & 21.9$\pm$0.4$^{(0)}$ & 119.5 & -13.3 & 100 &  \\ 
210426073 & 04 19 57.72 & +14 02 41.2 & 12.51 & 8.99 & 126.2$\pm$4.5 & -17.4$\pm$5.3 & 38.2$\pm$5.3$^{(1)}$ & 117.6 & -13.1 & 82 &  \\ 
210432080 & 04 16 25.42 & +14 10 17.1 & 13.71 & 10.05 & 136.65$\pm$2.13 & -22.83$\pm$2.13 & 28.7$\pm$4.0$^{(1)}$ & 120.1 & -13.0 & 98 & 1.4486\\ 
210439387 & 04 19 20.17 & +14 18 59.2 & 11.82 & 8.77 & 111.2$\pm$3.8 & -14.3$\pm$3.0 & 19.5$\pm$2.7$^{(1)}$ & 118.0 & -13.8 & 100 &  \\ 
210444167 & 04 21 34.79 & +14 24 35.2 & 6.48 & 5.59 & 104.23$\pm$0.04 & -19.13$\pm$0.03 & 20.4$\pm$0.4$^{(0)}$ & 110.5 & -13.7 & 100 &  \\ 
210451321 & 04 17 55.57 & +14 32 46.5 & 13.55 & 10.02 & 101.12$\pm$2.13 & -16.89$\pm$2.13 & 24.6$\pm$3.4$^{(1)}$ & 119.1 & -14.3 & 99 & 10.1182\\ 
210455478 & 04 14 25.65 & +14 37 30.1 & 8.24 & 6.82 & 107.12$\pm$0.09 & -16.3$\pm$0.06 & 20.6$\pm$0.3$^{(0)}$ & 116.1 & -13.4 & 100 &  \\ 
210457230 & 03 55 20.15 & +14 39 29.7 &   & 12.7 & 163.5$\pm$5.6 & -29.1$\pm$5.6 & 51.5$\pm$7.1$^{(4)}$ & 134.8 & -11.5 & 11 &  \\ 
210459199 & 04 21 35.10 & +14 41 42.8 & 14.09 & 10.44 & 103.99$\pm$2.18 & -20.43$\pm$2.18 & 24.5$\pm$3.4$^{(1)}$ & 116.4 & -15.2 & 99 & 3.6375\\ 
210468157 & 04 20 56.07 & +14 51 34.0 & 14.92 & 11.06 & 115.5$\pm$18.5 & -32.5$\pm$18.5 & 22.9$\pm$3.2$^{(1)}$ & 116.9 & -15.6 & 98 & $<$2\\ 
210470484 & 04 17 28.14 & +14 54 03.6 & 13.07 & 9.62 & 105.77$\pm$2.37 & -21.52$\pm$2.37 & 24.7$\pm$3.4$^{(1)}$ & 119.4 & -15.3 & 99 & 2.3788\\ 
210485181 & 03 33 11.77 & +15 09 30.8 & 16.21 & 11.89 & 165.92$\pm$2.15 & -6.75$\pm$2.15 & 20.8$\pm$2.9$^{(1)}$ & 149.0 & -9.2 & 93 &  \\ 
210489127 & 04 17 51.62 & +15 13 37.7 & 14.02 & 10.36 & 105.32$\pm$2.11 & -23.23$\pm$2.11 & 25.4$\pm$3.5$^{(1)}$ & 119.1 & -16.3 & 99 & 3.6508\\ 
210490365 & 04 13 05.62 & +15 14 51.9 & 14.15 & 10.44 & 120.77$\pm$2.11 & -19.48$\pm$2.11 & 27.0$\pm$3.7$^{(1)}$ & 122.5 & -15.7 & 99 & 1.8884\\ 
210499243 & 04 15 46.28 & +15 24 02.5 & 6.2 & 5.33 & 115.63$\pm$0.03 & -21.52$\pm$0.03 & 21.9$\pm$0.8$^{(0)}$ & 122.4 & -16.8 & 100 & $<$2\\ 
210517342 & 04 06 16.13 & +15 41 53.2 & 7.67 & 6.45 & 118.93$\pm$0.12 & -19.62$\pm$0.07 & 21.3$\pm$0.2$^{(0)}$ & 126.2 & -15.8 & 100 &  \\ 
210517837 & 04 15 33.69 & +15 42 22.6 & 10.32 & 7.85 & 120.51$\pm$0.19 & -23.2$\pm$0.14 & 22.1$\pm$0.3$^{(0)}$ & 124.2 & -17.9 & 100 &  \\ 
210523892 & 04 04 10.74 & +15 48 21.9 &   & 11.86 & 133.0$\pm$3.0 & -20.0$\pm$3.0 & 22.4$\pm$3.1$^{(3)}$ & 128.8 & -16.0 & 99 & 0.2967\\ 
210545912 & 03 32 34.50 & +16 09 12.0 & 12.76 & 9.21 & 139.79$\pm$3.59 & -16.21$\pm$1.75 & 34.1$\pm$4.7$^{(1)}$ & 149.3 & -11.6 & 73 &  \\ 
210563410 & 03 42 04.44 & +16 25 18.3 & 14.64 & 10.74 & 154.06$\pm$2.1 & -22.94$\pm$2.1 & 27.8$\pm$3.8$^{(1)}$ & 143.4 & -14.0 & 97 &  \\ 
210579563 & 03 59 15.03 & +16 39 51.9 & 14.12 & 10.38 & 139.07$\pm$2.09 & -28.2$\pm$2.09 & 27.2$\pm$3.8$^{(1)}$ & 132.2 & -17.6 & 99 & 1.2774\\ 
210619926 & 03 50 24.97 & +17 14 47.4 & 9.13 & 7.25 & 127.1$\pm$0.09 & -22.28$\pm$0.04 & 21.0$\pm$0.5$^{(0)}$ & 134.8 & -17.2 & 99 & $<$2\\ 
210640966 & 04 25 47.02 & +17 32 40.6 &   & 10.32 & 108.6$\pm$3.3 & -32.4$\pm$3.6 & 36.1$\pm$5.0$^{(2)}$ & 113.3 & -24.3 & 91 & 2.5614\\ 
210643507 & 03 40 45.81 & +17 34 47.8 &   & 11.73 & 154.0$\pm$3.0 & -25.0$\pm$3.0 & 24.3$\pm$3.4$^{(3)}$ & 144.3 & -16.7 & 98 &  \\ 
210667985 & 04 25 25.03 & +17 54 55.2 & 10.49 & 7.98 & 110.82$\pm$0.87 & -29.8$\pm$0.87 & 20.5$\pm$2.8$^{(1)}$ & 113.6 & -25.3 & 100 &  \\ 
210674207 & 04 26 21.71 & +18 00 01.1 & 14.1 & 10.25 & 97.81$\pm$2.2 & -28.01$\pm$2.2 & 33.1$\pm$4.6$^{(1)}$ & 112.9 & -25.7 & 93 & 1.0542\\ 
210674406 & 04 24 16.94 & +18 00 10.5 & 9.57 & 7.52 & 110.88$\pm$0.12 & -30.63$\pm$0.07 & 21.8$\pm$0.4$^{(0)}$ & 115.6 & -25.7 & 100 & 11.4703\\ 
210675409 & 04 25 47.56 & +18 01 02.2 & 8.7 & 6.77 & 105.8$\pm$1.0 & -30.95$\pm$0.98 & 20.8$\pm$1.6$^{(0)}$ & 109.4 & -24.8 & 100 &  \\ 
210688161 & 04 00 48.77 & +18 11 38.4 & 5.83 &   & 129.71$\pm$0.16 & -28.02$\pm$0.1 & 23.3$\pm$0.3$^{(0)}$ & 141.9 & -23.9 & 98 & $<$2\\ 
210693497 & 04 22 39.56 & +18 16 09.6 & 11.9 & 8.73 & 123.42$\pm$1.74 & -32.92$\pm$1.74 & 22.5$\pm$3.1$^{(1)}$ & 115.6 & -25.9 & 100 &  \\ 
210700098 & 04 18 33.85 & +18 21 52.9 & 14.39 & 10.6 & 117.1$\pm$2.07 & -35.38$\pm$2.07 & 25.9$\pm$3.6$^{(1)}$ & 118.6 & -25.5 & 99 & 2.3381\\ 
210703831 & 04 21 32.27 & +18 25 03.3 & 6.67 & 5.75 & 110.61$\pm$0.04 & -31.87$\pm$0.03 & 20.5$\pm$0.8$^{(0)}$ & 110.7 & -24.9 & 100 &  \\ 
210704853 & 03 55 57.18 & +18 25 56.3 & 12.81 & 9.39 & 134.52$\pm$2.3 & -31.62$\pm$2.3 & 26.8$\pm$3.7$^{(1)}$ & 134.4 & -21.8 & 99 & 23.1244\\ 
210707811 & 04 17 50.63 & +18 28 30.7 & 12.5 & 8.99 & 111.75$\pm$2.3 & -33.36$\pm$2.3 & 38.0$\pm$5.2$^{(1)}$ & 119.1 & -25.8 & 84 &  \\ 
210709514 & 04 27 58.96 & +18 30 00.9 & 9.7 & 7.53 & 105.1$\pm$1.95 & -34.78$\pm$1.13 & 19.4$\pm$0.6$^{(0)}$ & 100.7 & -24.7 & 100 & 11.1304\\ 
210718930 & 04 23 56.68 & +18 38 20.2 & 15.25 & 11.49 & 89.64$\pm$2.21 & -28.26$\pm$2.2 & 17.4$\pm$2.4$^{(1)}$ & 114.7 & -27.2 & 99 & 2.4191\\ 
210725815 & 04 20 25.11 & +18 44 33.4 & 6.0 & 5.16 & 113.7$\pm$0.04 & -34.21$\pm$0.02 & 22.9$\pm$0.7$^{(0)}$ & 124.8 & -28.7 & 100 &  \\ 
210733938 & 04 25 51.73 & +18 51 50.6 & 7.3 & 5.89 & 107.86$\pm$0.57 & -38.17$\pm$0.28 & 22.6$\pm$0.9$^{(0)}$ & 118.8 & -29.6 & 100 &  \\ 
210736105 & 04 20 27.63 & +18 53 49.8 & 13.78 & 10.22 & 107.38$\pm$2.13 & -41.27$\pm$2.13 & 24.0$\pm$3.3$^{(1)}$ & 117.2 & -27.4 & 99 & 20.3105\\ 
210741091 & 04 25 14.56 & +18 58 24.9 & 11.76 & 8.71 & 97.06$\pm$2.46 & -28.51$\pm$2.46 & 19.9$\pm$2.8$^{(1)}$ & 113.7 & -28.4 & 99 & 10.9678\\ 
210742017 & 04 24 30.59 & +18 59 12.8 & 14.73 & 10.78 & 111.47$\pm$2.2 & -35.04$\pm$2.2 & 28.8$\pm$4.0$^{(1)}$ & 114.2 & -28.3 & 99 &  \\ 
210742592 & 04 04 12.81 & +18 59 44.6 & 14.84 & 11.06 & 109.98$\pm$2.07 & -27.08$\pm$2.07 & 21.7$\pm$3.0$^{(1)}$ & 128.8 & -24.9 & 99 & 0.8037\\ 
210743724 & 04 25 41.84 & +19 00 47.6 & 13.5 & 10.13 & 85.23$\pm$2.2 & -28.26$\pm$2.2 & 15.5$\pm$2.1$^{(1)}$ & 113.4 & -28.6 & 97 &  \\ 
210744677 & 04 06 20.65 & +19 01 39.0 & 14.29 & 10.47 & 111.31$\pm$2.07 & -31.33$\pm$2.07 & 29.1$\pm$4.0$^{(1)}$ & 127.3 & -25.3 & 97 & 0.4812\\ 
210744818 & 04 17 25.15 & +19 01 47.7 & 10.24 & 7.91 & 113.66$\pm$0.77 & -30.46$\pm$0.77 & 19.8$\pm$2.7$^{(1)}$ & 119.4 & -27.3 & 100 & 12.8433\\ 
210745602 & 04 24 57.13 & +19 02 31.2 & 5.87 &   & 105.19$\pm$0.04 & -34.49$\pm$0.02 & 20.3$\pm$0.8$^{(0)}$ & 107.3 & -26.9 & 100 & $<$2\\ 
210754620 & 04 24 20.95 & +19 10 50.7 & 14.93 & 11.13 & 107.78$\pm$2.2 & -40.06$\pm$2.2 & 20.3$\pm$2.8$^{(1)}$ & 114.4 & -28.9 & 100 &  \\ 
210758134 & 04 20 12.97 & +19 14 00.5 & 7.29 & 6.12 & 114.65$\pm$0.05 & -35.07$\pm$0.05 & 23.2$\pm$0.7$^{(0)}$ & 126.4 & -30.5 & 100 &  \\ 
210769813 & 04 00 15.59 & +19 24 36.5 & 14.47 & 10.7 & 123.09$\pm$2.06 & -36.86$\pm$2.06 & 24.8$\pm$3.4$^{(1)}$ & 131.5 & -25.3 & 99 & 1.8626\\ 
210771915 & 04 05 25.67 & +19 26 31.8 & 10.73 & 8.11 & 122.02$\pm$0.24 & -32.64$\pm$0.16 & 21.1$\pm$0.4$^{(0)}$ & 125.4 & -25.8 & 99 & 13.8499\\ 
210772796 & 04 03 39.04 & +19 27 18.0 & 9.7 & 7.6 & 122.15$\pm$0.18 & -33.42$\pm$0.12 & 20.9$\pm$0.3$^{(0)}$ & 125.1 & -25.2 & 100 & 11.6032\\ 
210786154 & 04 23 22.85 & +19 39 31.2 & 9.04 & 7.15 & 98.4$\pm$0.52 & -33.44$\pm$0.63 & 16.5$\pm$1.3$^{(0)}$ & 88.2 & -23.1 & 99 & 10.017\\ 
210815169 & 03 30 31.22 & +20 05 55.2 & 9.99 &   & 163.92$\pm$1.32 & -55.52$\pm$1.33 & 33.6$\pm$4.6$^{(1)}$ & 150.6 & -20.8 & 20 &  \\ 
210815471 & 03 30 30.43 & +20 06 11.8 & 8.07 & 6.54 & 161.69$\pm$0.13 & -57.98$\pm$0.06 & 26.8$\pm$0.2$^{(0)}$ & 187.7 & -26.0 & 100 &  \\ 
210827030 & 04 07 03.25 & +20 16 50.9 & 14.45 & 10.56 & 167.15$\pm$2.07 & -46.63$\pm$2.07 & 29.0$\pm$4.0$^{(1)}$ & 126.8 & -29.0 & 95 &  \\ 
210835395 & 04 04 27.04 & +20 24 30.4 & 14.16 & 10.32 & 118.92$\pm$2.08 & -37.12$\pm$2.07 & 31.1$\pm$4.3$^{(1)}$ & 128.6 & -28.8 & 97 &  \\ 
210839963 & 03 52 20.75 & +20 28 41.2 &   & 11.98 & 149.2$\pm$5.2 & -41.1$\pm$5.2 & 45.3$\pm$6.3$^{(4)}$ & 136.8 & -26.6 & 33 & $<$2\\ 
210865372 & 03 43 47.09 & +20 51 36.3 & 13.12 & 9.61 & 138.67$\pm$2.34 & -38.0$\pm$2.34 & 26.9$\pm$3.7$^{(1)}$ & 142.4 & -25.7 & 98 & 12.3168\\ 
210865436 & 04 10 33.75 & +20 51 39.3 & 12.2 & 9.26 & 98.4$\pm$6.3 & -21.3$\pm$6.1 & 15.5$\pm$2.1$^{(1)}$ & 124.3 & -31.3 & 95 &  \\ 
210888551 & 03 46 34.01 & +21 12 46.2 & 12.75 & 9.7 & 97.1$\pm$20.0 & -50.0$\pm$11.2 & 14.6$\pm$2.0$^{(1)}$ & 140.6 & -27.2 & 20 &  \\ 
210941195 & 03 59 14.19 & +22 02 37.9 & 11.89 & 8.7 & 149.55$\pm$2.24 & -44.09$\pm$2.24 & 24.8$\pm$3.4$^{(1)}$ & 132.2 & -32.2 & 99 & 20.7309\\ 
210942311 & 03 36 19.95 & +22 03 41.3 & 15.0 & 11.33 & 105.64$\pm$3.69 & -25.88$\pm$3.69 & 17.5$\pm$2.4$^{(1)}$ & 147.0 & -27.0 & 81 &  \\ 
210942999 & 03 34 10.58 & +22 04 21.2 & 14.37 & 10.48 & 190.68$\pm$2.13 & -43.3$\pm$2.13 & 30.9$\pm$4.3$^{(1)}$ & 148.4 & -26.5 & 77 & 1.8088\\ 
210963067 & 04 12 47.36 & +22 23 27.0 & 14.16 & 10.16 & 119.39$\pm$2.08 & -41.51$\pm$2.08 & 38.1$\pm$5.3$^{(1)}$ & 122.7 & -36.0 & 83 & 1.8443\\ 
210966863 & 04 14 30.42 & +22 27 06.7 & 6.93 & 6.01 & 92.69$\pm$0.04 & -32.49$\pm$0.02 & 15.6$\pm$0.7$^{(0)}$ & 88.3 & -26.6 & 100 &  \\ 
210976212 & 03 59 51.83 & +22 36 13.4 & 13.55 & 10.15 & 108.34$\pm$2.08 & -35.09$\pm$2.08 & 16.4$\pm$2.3$^{(1)}$ & 131.7 & -33.9 & 98 &  \\ 
211019716 & 04 18 10.79 & +23 17 04.8 & 9.06 & 6.94 & 93.58$\pm$1.07 & -38.81$\pm$0.64 & 18.7$\pm$0.2$^{(0)}$ & 103.1 & -34.4 & 99 & 1.8626\\ 
211026112 & 03 59 26.62 & +23 23 07.6 & 14.44 & 10.65 & 133.99$\pm$2.08 & -44.59$\pm$2.08 & 26.2$\pm$3.6$^{(1)}$ & 132.0 & -35.9 & 99 & 1.3183\\ 
211037886 & 04 14 32.32 & +23 34 29.8 & 7.85 & 6.52 & 119.82$\pm$0.08 & -48.3$\pm$0.05 & 22.2$\pm$0.3$^{(0)}$ & 125.2 & -41.0 & 100 &  \\ 
211041649 & 04 11 56.22 & +23 38 10.8 & 8.88 & 6.41 & 145.84$\pm$0.54 & -52.05$\pm$0.73 & 26.2$\pm$1.7$^{(0)}$ & 150.2 & -47.9 & 100 & 2.3094\\ 
211049709 & 04 08 36.21 & +23 46 07.0 & 9.12 & 7.32 & 119.8$\pm$1.11 & -43.43$\pm$0.72 & 21.2$\pm$0.3$^{(0)}$ & 124.0 & -38.5 & 100 & 9.3908\\ 
211058178 & 03 51 03.11 & +23 54 13.1 & 9.7 & 7.4 & 152.53$\pm$0.17 & -48.1$\pm$0.09 & 24.6$\pm$0.3$^{(0)}$ & 157.0 & -40.2 & 100 & 12.5745\\ 
211088189 & 04 14 50.19 & +24 22 37.5 & 15.5 & 11.59 & 106.08$\pm$2.07 & -47.48$\pm$2.07 & 18.5$\pm$2.6$^{(1)}$ & 121.3 & -42.1 & 99 &  \\ 
211137806 & 03 52 42.71 & +25 12 26.0 & 16.02 & 12.06 & 135.57$\pm$2.15 & -49.56$\pm$2.15 & 15.3$\pm$2.1$^{(1)}$ & 136.5 & -39.1 & 83 & 14.3802\\ 
211169647 & 03 52 41.02 & +25 48 16.2 & 10.46 & 7.89 & 140.71$\pm$1.12 & -51.81$\pm$0.55 & 22.4$\pm$0.3$^{(0)}$ & 141.8 & -42.2 & 99 & 14.6609\\ 
211201094 & 03 59 09.65 & +26 28 34.4 & 10.73 & 7.89 & 140.03$\pm$3.04 & -63.16$\pm$0.83 & 27.2$\pm$0.8$^{(0)}$ & 167.3 & -55.7 & 88 & 15.2565\\ 
\enddata 
 \tablecomments{stuff} 
 \label{Hymemtab} 
 \end{deluxetable} 


==> Pl_memtable.tex <==
\begin{deluxetable}{cccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Candidate Pleiades members.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} \\ } 
 \startdata 
210552485 & 03 46 38.22 & +16 15 13.1 & 15.88 & 12.23 & 19.56$\pm$2.1 & -39.51$\pm$2.1 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -43.8 & 40 & $<$2\\ 
210562819 & 03 38 10.47 & +16 24 47.9 & 16.43 & 12.73 & 25.5$\pm$2.1 & -43.88$\pm$2.1 & 6.4$\pm$0.9$^{(1)}$ & 21.0 & -43.6 & 42 &  \\ 
210673842 & 03 56 46.92 & +17 59 42.9 & 11.99 & 9.88 & 23.01$\pm$0.92 & -40.69$\pm$0.92 & 7.5$\pm$1.0$^{(1)}$ & 18.8 & -44.5 & 47 &  \\ 
210674000 & 03 33 15.93 & +17 59 51.8 & 13.16 & 10.94 & 20.8$\pm$2.21 & -45.33$\pm$2.21 & 4.9$\pm$0.7$^{(1)}$ & 21.5 & -43.9 & 29 &  \\ 
210696739 & 03 25 24.41 & +18 18 57.0 & 13.2 & 10.59 & 24.12$\pm$2.29 & -43.78$\pm$2.29 & 6.8$\pm$0.9$^{(1)}$ & 22.4 & -43.7 & 84 &  \\ 
210696763 & 03 31 20.30 & +18 18 58.4 & 15.16 & 11.72 & 13.74$\pm$2.23 & -48.38$\pm$2.23 & 7.5$\pm$1.0$^{(1)}$ & 21.7 & -43.9 & 14 &  \\ 
210704834 & 03 46 32.63 & +18 25 55.2 & 17.08 & 13.19 & 17.24$\pm$2.1 & -36.66$\pm$2.1 & 6.3$\pm$0.9$^{(1)}$ & 20.0 & -44.3 & 58 &  \\ 
210707640 & 03 59 54.67 & +18 28 21.5 & 15.57 & 12.1 & 13.61$\pm$2.06 & -41.94$\pm$2.06 & 6.4$\pm$0.9$^{(1)}$ & 18.4 & -44.7 & 76 &  \\ 
210713788 & 03 57 49.74 & +18 33 44.7 & 11.16 & 9.45 & 20.16$\pm$0.92 & -46.98$\pm$0.44 & 7.7$\pm$0.3$^{(0)}$ & 18.7 & -44.7 & 99 &  \\ 
210715961 & 03 28 38.21 & +18 35 41.8 & 17.81 & 13.53 & 27.16$\pm$2.73 & -46.88$\pm$2.73 & 8.5$\pm$1.2$^{(1)}$ & 22.0 & -43.9 & 76 &  \\ 
210720772 & 03 51 32.25 & +18 39 58.6 & 17.05 & 13.03 & 20.88$\pm$2.13 & -52.54$\pm$2.13 & 8.6$\pm$1.2$^{(1)}$ & 19.4 & -44.5 & 83 & $<$2\\ 
210724826 & 04 01 36.55 & +18 43 42.3 &   & 11.52 & 16.36$\pm$2.11 & -40.05$\pm$2.11 & 11.6$\pm$1.6$^{(4)}$ & 18.2 & -44.8 & 18 &  \\ 
210727363 & 04 19 06.21 & +18 45 57.3 & 14.59 & 11.32 & 17.09$\pm$2.07 & -45.48$\pm$2.07 & 7.2$\pm$1.0$^{(1)}$ & 16.1 & -45.2 & 12 &  \\ 
210736056 & 03 37 35.45 & +18 53 47.1 & 16.12 & 12.67 & 19.02$\pm$2.15 & -43.85$\pm$2.15 & 4.9$\pm$0.7$^{(1)}$ & 21.1 & -44.2 & 62 &  \\ 
210743589 & 03 56 57.16 & +19 00 39.1 &   & 14.09 & 34.7$\pm$5.1 & -47.4$\pm$5.1 & 9.3$\pm$1.3$^{(4)}$ & 18.8 & -44.8 & 19 &  \\ 
210754915 & 03 44 28.08 & +19 11 06.0 & 11.44 & 9.42 & 19.31$\pm$0.84 & -40.53$\pm$0.92 & 8.9$\pm$1.2$^{(1)}$ & 20.3 & -44.5 & 97 & 0.5332\\ 
210756421 & 03 43 35.52 & +19 12 25.8 & 12.71 & 10.78 & 24.46$\pm$2.1 & -45.89$\pm$2.1 & 4.5$\pm$0.6$^{(1)}$ & 20.4 & -44.4 & 13 &  \\ 
210762863 & 03 44 11.91 & +19 18 19.3 & 14.15 & 11.05 & 15.31$\pm$2.1 & -44.43$\pm$2.1 & 6.6$\pm$0.9$^{(1)}$ & 20.3 & -44.5 & 98 & 7.4885\\ 
210769047 & 03 56 23.92 & +19 23 53.8 & 16.75 & 12.89 & 16.2$\pm$2.08 & -39.09$\pm$2.08 & 8.0$\pm$1.1$^{(1)}$ & 18.9 & -44.8 & 90 & 0.6439\\ 
210769751 & 03 53 26.93 & +19 24 33.0 & 13.42 & 10.07 & 24.16$\pm$2.08 & -49.93$\pm$2.08 & 13.1$\pm$1.8$^{(1)}$ & 19.2 & -44.8 & 30 &  \\ 
210770541 & 03 53 24.07 & +19 25 17.0 & 14.89 & 11.29 & 19.41$\pm$2.08 & -50.78$\pm$2.08 & 10.5$\pm$1.4$^{(1)}$ & 19.2 & -44.8 & 88 &  \\ 
210776021 & 03 55 13.61 & +19 30 16.9 & 15.29 & 11.72 & 20.26$\pm$2.08 & -46.75$\pm$2.08 & 7.9$\pm$1.1$^{(1)}$ & 19.0 & -44.8 & 99 & 2.4272\\ 
210776486 & 03 59 28.41 & +19 30 41.4 & 16.66 & 12.6 & 22.21$\pm$2.06 & -40.51$\pm$2.06 & 10.7$\pm$1.5$^{(1)}$ & 18.5 & -44.9 & 52 &  \\ 
210779549 & 03 45 01.66 & +19 33 33.7 & 9.26 & 8.15 & 21.29$\pm$0.65 & -42.95$\pm$0.37 & 7.4$\pm$0.4$^{(0)}$ & 20.2 & -44.5 & 100 & 0.9368\\ 
210784223 & 03 55 15.74 & +19 37 46.5 & 12.53 & 9.98 & 23.42$\pm$2.3 & -54.08$\pm$2.3 & 8.9$\pm$1.2$^{(1)}$ & 19.0 & -44.9 & 73 & 0.2684\\ 
210791550 & 03 59 16.64 & +19 44 27.6 & 16.51 & 12.7 & 15.23$\pm$2.06 & -41.94$\pm$2.06 & 7.6$\pm$1.0$^{(1)}$ & 18.5 & -45.0 & 97 & 0.3727\\ 
210796589 & 03 31 52.94 & +19 49 02.8 & 12.48 & 10.31 & 26.22$\pm$2.23 & -40.39$\pm$2.23 & 6.3$\pm$0.9$^{(1)}$ & 21.7 & -44.2 & 93 &  \\ 
210802674 & 03 40 32.37 & +19 54 30.4 & 17.25 & 13.28 & 15.05$\pm$2.65 & -41.56$\pm$2.65 & 7.1$\pm$1.0$^{(1)}$ & 20.7 & -44.5 & 98 & $<$2\\ 
210803812 & 03 39 10.20 & +19 55 31.0 & 15.93 & 12.21 & 22.76$\pm$2.19 & -37.06$\pm$2.19 & 8.0$\pm$1.1$^{(1)}$ & 20.9 & -44.4 & 90 & 1.7999\\ 
210804032 & 03 44 47.29 & +19 55 41.8 & 17.88 & 13.92 & 21.59$\pm$2.66 & -43.16$\pm$2.66 & 5.8$\pm$0.8$^{(1)}$ & 20.2 & -44.6 & 99 &  \\ 
210804191 & 03 56 49.95 & +19 55 49.5 & 15.59 & 12.01 & 17.14$\pm$2.08 & -41.12$\pm$2.08 & 6.8$\pm$0.9$^{(1)}$ & 18.8 & -45.0 & 99 & 1.0307\\ 
210808112 & 04 08 40.80 & +19 59 28.6 & 14.28 & 11.06 & 21.04$\pm$2.07 & -38.09$\pm$2.07 & 8.4$\pm$1.2$^{(1)}$ & 17.4 & -45.3 & 15 &  \\ 
210811598 & 04 06 28.61 & +20 02 38.0 & 16.2 & 12.42 & 18.18$\pm$2.07 & -45.72$\pm$2.07 & 8.3$\pm$1.2$^{(1)}$ & 17.6 & -45.3 & 97 & $<$2\\ 
210813780 & 03 39 31.47 & +20 04 40.8 & 14.89 & 11.7 & 20.1$\pm$2.15 & -51.8$\pm$2.15 & 5.6$\pm$0.8$^{(1)}$ & 20.8 & -44.5 & 92 & 15.783\\ 
210815768 & 03 49 35.75 & +20 06 29.0 & 17.03 & 12.92 & 21.08$\pm$2.08 & -46.42$\pm$2.08 & 10.5$\pm$1.5$^{(1)}$ & 19.7 & -44.8 & 99 & 0.2999\\ 
210817106 & 03 43 18.74 & +20 07 44.8 & 16.13 & 12.49 & 12.51$\pm$2.1 & -44.73$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 20.4 & -44.6 & 93 &  \\ 
210818448 & 03 42 29.87 & +20 08 60.0 & 8.34 & 7.65 & 19.94$\pm$0.06 & -44.76$\pm$0.04 & 7.7$\pm$0.5$^{(0)}$ & 20.5 & -44.6 & 100 &  \\ 
210822528 & 03 42 58.59 & +20 12 45.2 & 16.96 & 12.95 & 18.47$\pm$2.59 & -41.7$\pm$2.59 & 8.6$\pm$1.2$^{(1)}$ & 20.4 & -44.6 & 99 & 0.9149\\ 
210826886 & 03 47 22.76 & +20 16 43.5 & 16.16 & 12.67 & 18.57$\pm$2.08 & -41.46$\pm$2.08 & 4.9$\pm$0.7$^{(1)}$ & 19.9 & -44.8 & 90 &  \\ 
210826887 & 03 51 54.64 & +20 16 43.5 & 14.85 & 11.31 & 3.0$\pm$9.9 & -29.4$\pm$9.6 & 9.6$\pm$1.3$^{(1)}$ & 19.4 & -44.9 & 38 &  \\ 
210829407 & 03 50 28.40 & +20 19 01.2 & 15.87 & 12.27 & 18.16$\pm$2.08 & -40.69$\pm$2.08 & 6.4$\pm$0.9$^{(1)}$ & 19.6 & -44.9 & 99 &  \\ 
210830104 & 03 50 33.85 & +20 19 38.8 & 18.44 & 14.0 & 23.32$\pm$2.55 & -50.08$\pm$2.55 & 7.2$\pm$1.0$^{(1)}$ & 19.6 & -44.9 & 100 & 1.128\\ 
210832378 & 03 42 13.89 & +20 21 44.0 & 16.62 & 12.79 & 21.64$\pm$2.1 & -48.16$\pm$2.1 & 8.4$\pm$1.2$^{(1)}$ & 20.5 & -44.6 & 100 & 0.4656\\ 
210833049 & 04 01 04.13 & +20 22 21.4 & 14.44 & 10.91 & 18.35$\pm$2.06 & -52.96$\pm$2.06 & 10.6$\pm$1.5$^{(1)}$ & 18.3 & -45.2 & 67 & 5.3682\\ 
210833622 & 03 49 56.06 & +20 22 52.8 & 16.45 & 12.63 & 21.09$\pm$2.08 & -55.71$\pm$2.08 & 9.8$\pm$1.4$^{(1)}$ & 19.6 & -44.9 & 62 & 1.0465\\ 
210833924 & 03 47 54.93 & +20 23 08.2 & 16.18 & 12.45 & 18.23$\pm$2.11 & -41.08$\pm$2.08 & 9.3$\pm$1.3$^{(1)}$ & 19.9 & -44.8 & 99 &  \\ 
210833947 & 04 08 55.39 & +20 23 09.6 & 9.23 & 8.11 & 19.01$\pm$0.1 & -50.11$\pm$0.06 & 8.0$\pm$0.4$^{(0)}$ & 17.3 & -45.4 & 90 & $<$2\\ 
210837175 & 03 43 15.80 & +20 26 10.1 & 12.86 & 10.79 & 11.6$\pm$4.5 & -36.2$\pm$5.9 & 5.1$\pm$0.7$^{(1)}$ & 20.4 & -44.7 & 33 &  \\ 
210837336 & 03 52 08.81 & +20 26 18.8 & 11.44 & 9.14 & 19.96$\pm$0.92 & -50.63$\pm$0.92 & 11.6$\pm$1.6$^{(1)}$ & 19.4 & -44.9 & 88 &  \\ 
210839388 & 04 04 08.44 & +20 28 09.6 & 14.13 & 10.86 & 14.73$\pm$2.07 & -52.23$\pm$2.07 & 8.4$\pm$1.2$^{(1)}$ & 17.9 & -45.3 & 82 & 3.4652\\ 
210840112 & 03 53 58.12 & +20 28 49.7 & 14.28 & 10.92 & 18.47$\pm$2.08 & -45.06$\pm$2.08 & 8.6$\pm$1.2$^{(1)}$ & 19.2 & -45.0 & 100 & 0.4077\\ 
210846442 & 03 56 11.34 & +20 34 30.2 & 15.39 & 11.84 & 22.39$\pm$2.08 & -49.11$\pm$2.08 & 7.8$\pm$1.1$^{(1)}$ & 18.9 & -45.1 & 100 & 1.1199\\ 
210847165 & 04 10 37.07 & +20 35 08.2 & 16.47 & 12.74 & 19.43$\pm$2.07 & -42.43$\pm$2.07 & 6.7$\pm$0.9$^{(1)}$ & 17.1 & -45.5 & 89 &  \\ 
210849741 & 03 55 26.07 & +20 37 25.9 & 11.98 & 10.24 & 25.84$\pm$2.08 & -50.7$\pm$2.08 & 4.9$\pm$0.7$^{(1)}$ & 19.0 & -45.1 & 18 &  \\ 
210854098 & 03 40 51.06 & +20 41 17.6 & 17.91 & 13.71 & 20.04$\pm$2.59 & -45.57$\pm$2.59 & 7.5$\pm$1.0$^{(1)}$ & 20.7 & -44.6 & 100 & 0.3451\\ 
210855272 & 03 50 24.95 & +20 42 18.1 & 13.85 & 10.94 & 13.7$\pm$2.08 & -44.83$\pm$2.08 & 6.1$\pm$0.8$^{(1)}$ & 19.6 & -44.9 & 99 & 17.597\\ 
210857107 & 03 55 22.37 & +20 43 57.9 & 16.89 & 12.87 & 24.91$\pm$2.08 & -43.32$\pm$2.08 & 9.2$\pm$1.3$^{(1)}$ & 19.0 & -45.1 & 96 & $<$2\\ 
210860152 & 03 48 11.41 & +20 46 42.7 & 16.15 & 12.24 & 20.03$\pm$2.08 & -47.0$\pm$2.08 & 11.5$\pm$1.6$^{(1)}$ & 19.8 & -44.9 & 98 & 0.6299\\ 
210862226 & 03 42 29.70 & +20 48 40.1 & 16.23 & 12.43 & 18.12$\pm$2.1 & -50.41$\pm$2.1 & 8.5$\pm$1.2$^{(1)}$ & 20.5 & -44.7 & 99 & 1.2913\\ 
210863662 & 04 05 50.36 & +20 49 59.4 & 17.53 & 13.48 & 27.1$\pm$2.07 & -44.64$\pm$2.07 & 7.0$\pm$1.0$^{(1)}$ & 17.7 & -45.4 & 35 &  \\ 
210863683 & 03 53 43.02 & +20 50 00.5 & 13.82 & 10.76 & 18.94$\pm$2.08 & -47.99$\pm$2.08 & 7.6$\pm$1.0$^{(1)}$ & 19.2 & -45.1 & 100 & 2.7826\\ 
210866482 & 03 52 11.21 & +20 52 33.9 & 16.44 & 12.6 & 22.84$\pm$2.08 & -48.32$\pm$2.08 & 8.5$\pm$1.2$^{(1)}$ & 19.4 & -45.0 & 100 & 0.3228\\ 
210866744 & 03 46 19.34 & +20 52 47.2 & 11.26 & 9.52 & 20.42$\pm$0.19 & -44.13$\pm$0.14 & 7.2$\pm$0.3$^{(0)}$ & 20.1 & -44.9 & 100 & 5.9344\\ 
210868554 & 03 53 28.87 & +20 54 26.6 & 11.55 & 9.51 & 19.42$\pm$0.68 & -44.62$\pm$0.36 & 7.5$\pm$0.2$^{(0)}$ & 19.2 & -45.1 & 100 & $<$2\\ 
210868642 & 03 50 50.80 & +20 54 31.7 & 15.6 & 12.2 & 24.98$\pm$2.08 & -55.83$\pm$2.08 & 5.4$\pm$0.7$^{(1)}$ & 19.5 & -45.0 & 19 &  \\ 
210870064 & 03 54 16.33 & +20 55 48.2 & 17.75 & 13.69 & 18.78$\pm$2.55 & -48.13$\pm$2.55 & 6.1$\pm$0.8$^{(1)}$ & 19.1 & -45.1 & 100 &  \\ 
210870456 & 04 06 55.64 & +20 56 10.9 & 16.44 & 12.64 & 11.6$\pm$2.07 & -39.65$\pm$2.07 & 8.1$\pm$1.1$^{(1)}$ & 17.6 & -45.5 & 42 & $<$2\\ 
210870563 & 04 08 31.73 & +20 56 17.1 & 11.02 & 9.33 & 15.18$\pm$1.83 & -40.21$\pm$1.08 & 6.3$\pm$0.3$^{(0)}$ & 17.4 & -45.5 & 65 &  \\ 
210871940 & 03 53 31.56 & +20 57 27.2 & 16.68 & 12.92 & 22.67$\pm$2.08 & -54.78$\pm$2.08 & 6.9$\pm$0.9$^{(1)}$ & 19.2 & -45.1 & 95 & 0.2773\\ 
210872505 & 03 40 35.32 & +20 57 56.8 & 14.67 & 11.3 & 20.75$\pm$2.1 & -48.06$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.7 & -44.7 & 100 & 0.534\\ 
210873256 & 03 54 13.52 & +20 58 38.7 & 17.56 & 13.56 & 13.79$\pm$2.55 & -50.99$\pm$2.55 & 6.7$\pm$0.9$^{(1)}$ & 19.1 & -45.1 & 98 & 0.3425\\ 
210876759 & 03 43 05.72 & +21 01 49.5 & 16.97 & 13.07 & 18.8$\pm$2.1 & -52.87$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 20.4 & -44.8 & 99 & 0.4336\\ 
210877263 & 03 46 29.72 & +21 02 17.1 & 16.52 & 12.55 & 22.11$\pm$2.1 & -52.8$\pm$2.1 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -44.9 & 96 & 0.3183\\ 
210878635 & 03 51 16.61 & +21 03 35.1 & 16.18 & 12.38 & 20.2$\pm$2.13 & -51.41$\pm$2.13 & 8.3$\pm$1.1$^{(1)}$ & 19.5 & -45.0 & 100 & 0.4748\\ 
210879932 & 03 55 31.94 & +21 04 46.2 & 10.84 & 9.17 & 21.55$\pm$1.08 & -50.4$\pm$0.55 & 8.2$\pm$0.3$^{(0)}$ & 19.0 & -45.2 & 99 & 5.5586\\ 
210880560 & 03 52 58.35 & +21 05 20.4 & 16.8 & 12.55 & 16.66$\pm$2.08 & -48.16$\pm$2.08 & 12.8$\pm$1.8$^{(1)}$ & 19.3 & -45.1 & 89 & 0.4317\\ 
210881103 & 03 46 09.88 & +21 05 52.8 & 15.87 & 12.25 & 18.12$\pm$2.1 & -42.92$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.1 & -44.9 & 100 & 0.4625\\ 
210882573 & 03 56 22.30 & +21 07 17.2 & 15.64 & 12.02 & 19.04$\pm$2.08 & -48.24$\pm$2.08 & 7.1$\pm$1.0$^{(1)}$ & 18.9 & -45.2 & 100 & 0.6128\\ 
210883020 & 04 01 09.04 & +21 07 40.5 & 15.22 & 11.78 & 16.29$\pm$2.06 & -37.53$\pm$2.06 & 6.0$\pm$0.8$^{(1)}$ & 18.3 & -45.4 & 81 & $<$2\\ 
210886244 & 03 55 57.53 & +21 10 39.0 & 15.38 & 11.76 & 16.69$\pm$2.14 & -46.46$\pm$2.14 & 8.5$\pm$1.2$^{(1)}$ & 18.9 & -45.2 & 100 & 0.5959\\ 
210886447 & 03 47 31.13 & +21 10 51.5 & 16.69 & 12.82 & 17.31$\pm$2.08 & -50.5$\pm$2.08 & 8.3$\pm$1.2$^{(1)}$ & 19.9 & -45.0 & 100 & 0.5596\\ 
210887995 & 03 59 42.66 & +21 12 15.4 & 17.08 & 13.03 & 17.2$\pm$2.06 & -46.25$\pm$2.06 & 8.6$\pm$1.2$^{(1)}$ & 18.5 & -45.3 & 100 & 0.547\\ 
210888723 & 03 40 49.39 & +21 12 55.7 & 16.4 & 12.49 & 19.55$\pm$2.1 & -46.77$\pm$2.1 & 8.8$\pm$1.2$^{(1)}$ & 20.7 & -44.7 & 100 & 3.7501\\ 
210890748 & 03 45 31.99 & +21 14 48.1 & 7.73 & 7.31 & 20.55$\pm$0.06 & -47.73$\pm$0.04 & 7.8$\pm$0.4$^{(0)}$ & 20.1 & -44.9 & 100 &  \\ 
210892321 & 03 59 31.45 & +21 16 18.8 & 15.35 & 11.84 & 18.83$\pm$2.05 & -48.15$\pm$2.05 & 6.7$\pm$0.9$^{(1)}$ & 18.5 & -45.3 & 100 & 0.7319\\ 
210892390 & 03 55 39.50 & +21 16 22.0 & 14.16 & 10.9 & 18.04$\pm$2.13 & -38.95$\pm$2.13 & 8.0$\pm$1.1$^{(1)}$ & 19.0 & -45.2 & 98 & 1.4066\\ 
210892842 & 03 49 26.14 & +21 16 49.4 & 13.32 & 10.36 & 20.27$\pm$2.05 & -54.55$\pm$2.05 & 8.6$\pm$1.2$^{(1)}$ & 19.7 & -45.0 & 96 &  \\ 
210894583 & 03 49 51.80 & +21 18 26.3 & 14.33 & 10.92 & 16.92$\pm$2.08 & -46.08$\pm$2.08 & 9.3$\pm$1.3$^{(1)}$ & 19.6 & -45.1 & 100 & 0.4722\\ 
210899950 & 03 54 27.83 & +21 23 23.1 & 10.71 & 9.18 & 19.2$\pm$0.22 & -47.14$\pm$0.13 & 7.4$\pm$0.3$^{(0)}$ & 19.1 & -45.2 & 100 & 4.548\\ 
210901240 & 03 50 27.31 & +21 24 35.8 & 16.83 & 12.93 & 19.32$\pm$2.51 & -33.32$\pm$2.51 & 8.0$\pm$1.1$^{(1)}$ & 19.6 & -45.1 & 51 &  \\ 
210901321 & 03 48 48.22 & +21 24 40.8 & 16.43 & 12.64 & 20.25$\pm$2.08 & -46.93$\pm$2.08 & 8.1$\pm$1.1$^{(1)}$ & 19.8 & -45.0 & 100 & 0.6231\\ 
210902186 & 03 46 25.40 & +21 25 30.5 & 12.14 & 9.78 & 18.72$\pm$2.3 & -46.88$\pm$2.3 & 9.7$\pm$1.3$^{(1)}$ & 20.0 & -45.0 & 100 &  \\ 
210904018 & 04 00 33.58 & +21 27 10.4 & 17.28 & 13.34 & 20.26$\pm$2.51 & -36.05$\pm$2.51 & 6.8$\pm$0.9$^{(1)}$ & 18.4 & -45.4 & 80 & $<$2\\ 
210904675 & 03 46 05.80 & +21 27 46.0 & 13.54 & 10.83 & 27.11$\pm$2.1 & -42.45$\pm$2.1 & 6.2$\pm$0.9$^{(1)}$ & 20.1 & -45.0 & 98 &  \\ 
210905362 & 03 42 24.00 & +21 28 24.6 & 9.66 & 8.53 & 20.99$\pm$0.15 & -47.97$\pm$0.09 & 7.8$\pm$0.2$^{(0)}$ & 20.5 & -44.8 & 100 & 2.3787\\ 
210907442 & 03 52 24.57 & +21 30 22.7 & 15.02 & 11.48 & 18.98$\pm$2.05 & -46.03$\pm$2.05 & 7.8$\pm$1.1$^{(1)}$ & 19.3 & -45.2 & 100 & 1.8182\\ 
210908248 & 03 55 03.59 & +21 31 10.1 & 17.43 & 13.46 & 25.25$\pm$2.05 & -46.51$\pm$2.05 & 7.0$\pm$1.0$^{(1)}$ & 19.0 & -45.3 & 99 &  \\ 
210909681 & 03 33 26.46 & +21 32 29.8 & 13.68 & 11.21 & 19.5$\pm$2.13 & -38.01$\pm$2.13 & 4.9$\pm$0.7$^{(1)}$ & 21.5 & -44.6 & 61 &  \\ 
210909844 & 03 58 55.69 & +21 32 38.7 & 15.22 & 11.84 & 28.91$\pm$2.05 & -52.79$\pm$2.05 & 5.9$\pm$0.8$^{(1)}$ & 18.6 & -45.4 & 11 &  \\ 
210909923 & 03 56 04.54 & +21 32 42.6 & 14.89 & 11.16 & 21.66$\pm$2.05 & -48.17$\pm$2.05 & 13.5$\pm$1.9$^{(1)}$ & 18.9 & -45.3 & 87 & 0.4704\\ 
210912544 & 04 01 26.04 & +21 35 09.0 & 15.94 & 12.26 & 21.36$\pm$2.05 & -41.59$\pm$2.05 & 7.7$\pm$1.1$^{(1)}$ & 18.3 & -45.5 & 99 & 1.1983\\ 
210913953 & 03 50 09.52 & +21 36 30.8 & 12.55 & 9.74 & 11.56$\pm$2.25 & -38.16$\pm$2.25 & 10.4$\pm$1.4$^{(1)}$ & 19.6 & -45.1 & 26 &  \\ 
210914325 & 03 58 50.05 & +21 36 53.3 & 17.52 & 13.19 & 18.14$\pm$2.51 & -46.52$\pm$2.51 & 10.5$\pm$1.4$^{(1)}$ & 18.6 & -45.4 & 99 &  \\ 
210915466 & 03 49 22.51 & +21 37 56.4 & 16.61 & 12.66 & 13.03$\pm$2.05 & -38.28$\pm$2.05 & 9.8$\pm$1.4$^{(1)}$ & 19.7 & -45.1 & 59 & 0.4171\\ 
210917578 & 03 59 29.32 & +21 39 56.4 & 17.69 & 13.61 & 19.1$\pm$2.51 & -45.06$\pm$2.51 & 6.6$\pm$0.9$^{(1)}$ & 18.5 & -45.4 & 100 &  \\ 
210917754 & 03 51 42.09 & +21 40 06.0 & 11.22 & 9.45 & 18.37$\pm$1.41 & -43.12$\pm$0.66 & 7.2$\pm$0.3$^{(0)}$ & 19.4 & -45.2 & 100 & 5.4447\\ 
210918923 & 03 46 16.07 & +21 41 10.1 & 17.66 & 13.73 & 18.07$\pm$2.6 & -47.12$\pm$2.6 & 6.3$\pm$0.9$^{(1)}$ & 20.1 & -45.0 & 100 & $<$2\\ 
210919084 & 03 52 45.66 & +21 41 19.6 & 15.54 & 11.96 & 16.56$\pm$2.05 & -46.61$\pm$2.05 & 7.2$\pm$1.0$^{(1)}$ & 19.3 & -45.2 & 100 & 1.1461\\ 
210920066 & 03 45 09.88 & +21 42 16.5 & 9.8 & 8.59 & 21.02$\pm$0.71 & -47.71$\pm$0.75 & 6.8$\pm$0.9$^{(1)}$ & 20.2 & -45.0 & 100 & 2.9317\\ 
210920246 & 03 52 48.69 & +21 42 28.1 & 13.78 & 10.66 & 16.18$\pm$2.05 & -50.79$\pm$2.05 & 8.0$\pm$1.1$^{(1)}$ & 19.3 & -45.2 & 100 & 0.553\\ 
210922592 & 03 47 34.16 & +21 44 48.5 & 11.88 & 9.9 & 17.78$\pm$1.33 & -46.55$\pm$1.33 & 6.2$\pm$0.9$^{(1)}$ & 19.9 & -45.1 & 100 & 7.5554\\ 
210922602 & 03 45 46.93 & +21 44 49.4 & 16.91 & 12.82 & 22.53$\pm$2.1 & -55.81$\pm$2.1 & 9.5$\pm$1.3$^{(1)}$ & 20.1 & -45.0 & 87 & 0.1958\\ 
210923443 & 03 52 04.37 & +21 45 39.2 & 17.38 & 13.29 & 18.3$\pm$2.51 & -42.98$\pm$2.51 & 7.7$\pm$1.1$^{(1)}$ & 19.4 & -45.2 & 100 & 0.8865\\ 
210923951 & 04 07 29.33 & +21 46 10.5 & 16.01 & 12.37 & 14.33$\pm$2.07 & -55.73$\pm$2.07 & 7.9$\pm$1.1$^{(1)}$ & 17.5 & -45.7 & 38 &  \\ 
210924735 & 03 52 53.00 & +21 46 54.8 & 11.57 & 9.35 & 15.97$\pm$0.84 & -40.05$\pm$0.84 & 10.8$\pm$1.5$^{(1)}$ & 19.3 & -45.2 & 85 & 1.7525\\ 
210926194 & 03 59 26.92 & +21 48 19.0 & 16.6 & 12.62 & 19.92$\pm$2.05 & -46.51$\pm$2.05 & 9.7$\pm$1.3$^{(1)}$ & 18.5 & -45.4 & 99 & 0.9536\\ 
210927034 & 03 47 40.94 & +21 49 05.4 & 17.85 & 13.8 & 16.22$\pm$2.55 & -50.6$\pm$2.55 & 6.7$\pm$0.9$^{(1)}$ & 19.9 & -45.1 & 100 & $<$2\\ 
210927253 & 03 51 51.55 & +21 49 17.1 & 16.12 & 12.34 & 15.3$\pm$2.05 & -52.83$\pm$2.15 & 9.1$\pm$1.3$^{(1)}$ & 19.4 & -45.2 & 95 & 0.813\\ 
210927279 & 03 31 28.34 & +21 49 18.9 & 8.74 & 7.82 & 24.12$\pm$0.1 & -47.11$\pm$0.05 & 7.8$\pm$0.3$^{(0)}$ & 21.7 & -44.5 & 100 & $<$2\\ 
210927331 & 03 51 51.89 & +21 49 22.0 & 15.65 & 12.04 & 24.03$\pm$2.09 & -42.12$\pm$2.09 & 7.6$\pm$1.1$^{(1)}$ & 19.4 & -45.2 & 100 & 1.3131\\ 
210928599 & 03 39 13.20 & +21 50 35.7 & 7.29 & 7.05 & 20.29$\pm$0.05 & -43.61$\pm$0.03 & 7.2$\pm$0.3$^{(0)}$ & 20.9 & -44.8 & 100 &  \\ 
210931244 & 03 54 34.80 & +21 53 02.1 & 14.45 & 11.18 & 17.26$\pm$2.05 & -46.12$\pm$2.05 & 7.4$\pm$1.0$^{(1)}$ & 19.1 & -45.3 & 100 & 2.7745\\ 
210932705 & 03 59 39.82 & +21 54 27.9 & 15.28 & 11.77 & 14.57$\pm$2.05 & -44.66$\pm$2.05 & 6.4$\pm$0.9$^{(1)}$ & 18.5 & -45.5 & 100 & 4.0454\\ 
210933044 & 03 49 02.96 & +21 54 47.2 & 17.33 & 13.37 & 23.55$\pm$2.08 & -55.86$\pm$2.08 & 7.3$\pm$1.0$^{(1)}$ & 19.7 & -45.1 & 95 & 0.6738\\ 
210933788 & 03 48 39.32 & +21 55 30.0 & 8.28 & 7.32 & 23.72$\pm$0.55 & -48.52$\pm$0.4 & 8.5$\pm$0.3$^{(0)}$ & 19.8 & -45.1 & 99 & $<$2\\ 
210934634 & 03 49 41.70 & +21 56 19.5 & 18.09 & 13.76 & 17.28$\pm$2.51 & -47.04$\pm$2.51 & 7.3$\pm$1.0$^{(1)}$ & 19.7 & -45.2 & 100 & 0.3971\\ 
210936682 & 03 47 04.03 & +21 58 16.7 & 11.91 & 9.88 & 19.59$\pm$0.94 & -49.99$\pm$0.92 & 6.8$\pm$0.9$^{(1)}$ & 20.0 & -45.1 & 100 &  \\ 
210936878 & 04 05 48.39 & +21 58 29.0 & 17.66 & 13.77 & 17.64$\pm$2.55 & -57.11$\pm$2.55 & 5.4$\pm$0.7$^{(1)}$ & 17.7 & -45.7 & 21 &  \\ 
210938312 & 03 40 31.76 & +21 59 52.8 & 16.59 & 12.97 & 28.63$\pm$2.12 & -40.8$\pm$2.12 & 5.0$\pm$0.7$^{(1)}$ & 20.7 & -44.9 & 31 &  \\ 
210939348 & 03 52 18.46 & +22 00 53.7 & 14.66 & 11.39 & 17.14$\pm$2.05 & -42.98$\pm$2.05 & 6.6$\pm$0.9$^{(1)}$ & 19.4 & -45.3 & 100 & 1.9941\\ 
210939705 & 03 52 06.66 & +22 01 14.7 & 16.98 & 13.12 & 21.07$\pm$2.05 & -50.14$\pm$2.05 & 7.5$\pm$1.0$^{(1)}$ & 19.4 & -45.3 & 100 & 0.4687\\ 
210940129 & 03 36 44.11 & +22 01 39.1 & 17.1 & 12.92 & 23.76$\pm$3.04 & -46.8$\pm$2.76 & 10.0$\pm$1.4$^{(1)}$ & 21.1 & -44.8 & 99 & 0.727\\ 
210940436 & 03 41 23.45 & +22 01 54.3 & 16.71 & 12.54 & 25.97$\pm$2.1 & -49.81$\pm$2.1 & 10.7$\pm$1.5$^{(1)}$ & 20.6 & -44.9 & 97 & 0.7453\\ 
210940618 & 04 06 56.03 & +22 02 04.7 & 14.05 & 10.83 & 17.18$\pm$2.06 & -47.42$\pm$2.06 & 7.8$\pm$1.1$^{(1)}$ & 17.6 & -45.7 & 99 & 1.4102\\ 
210940839 & 04 00 10.28 & +22 02 17.5 & 16.32 & 12.52 & 21.66$\pm$2.04 & -49.5$\pm$2.04 & 8.2$\pm$1.1$^{(1)}$ & 18.4 & -45.5 & 100 & 0.5797\\ 
210942652 & 03 48 17.60 & +22 04 01.3 & 16.32 & 12.61 & 22.63$\pm$2.08 & -48.03$\pm$2.08 & 7.8$\pm$1.1$^{(1)}$ & 19.8 & -45.1 & 100 & 0.7353\\ 
210942842 & 03 48 46.58 & +22 04 12.8 & 11.67 & 9.53 & 24.02$\pm$2.3 & -49.06$\pm$2.3 & 8.8$\pm$1.2$^{(1)}$ & 19.8 & -45.2 & 100 & 6.2883\\ 
210943453 & 03 34 54.95 & +22 04 46.7 & 14.89 & 11.57 & 21.74$\pm$2.08 & -44.68$\pm$2.08 & 6.9$\pm$0.9$^{(1)}$ & 21.3 & -44.7 & 100 & 0.8275\\ 
210944157 & 03 59 59.85 & +22 05 29.7 & 16.78 & 12.91 & 18.92$\pm$2.08 & -36.82$\pm$2.08 & 8.2$\pm$1.1$^{(1)}$ & 18.4 & -45.5 & 83 & 0.5733\\ 
210945519 & 03 51 23.87 & +22 06 48.1 & 12.61 & 10.2 & 16.31$\pm$2.09 & -48.33$\pm$2.09 & 7.6$\pm$1.1$^{(1)}$ & 19.5 & -45.3 & 100 & 6.4306\\ 
210946466 & 03 39 44.19 & +22 07 45.8 & 15.36 & 11.89 & 22.24$\pm$2.1 & -47.44$\pm$2.1 & 6.5$\pm$0.9$^{(1)}$ & 20.8 & -44.9 & 100 & 1.081\\ 
210946764 & 03 33 05.82 & +22 08 03.3 & 11.14 & 9.43 & 22.81$\pm$1.1 & -46.28$\pm$0.56 & 7.4$\pm$0.4$^{(0)}$ & 21.6 & -44.6 & 100 & 5.766\\ 
210947280 & 03 57 49.36 & +22 08 31.4 & 18.35 & 13.9 & 21.4$\pm$2.52 & -46.21$\pm$2.52 & 7.8$\pm$1.1$^{(1)}$ & 18.7 & -45.5 & 100 & 0.8022\\ 
210947594 & 03 50 31.94 & +22 08 47.8 & 15.81 & 12.12 & 16.66$\pm$2.04 & -42.57$\pm$2.04 & 7.7$\pm$1.1$^{(1)}$ & 19.6 & -45.2 & 100 & 1.0933\\ 
210947847 & 03 52 08.15 & +22 09 02.4 & 15.14 & 11.44 & 17.26$\pm$2.04 & -37.07$\pm$2.04 & 11.5$\pm$1.6$^{(1)}$ & 19.4 & -45.3 & 57 & 14.889\\ 
210947895 & 03 49 35.88 & +22 09 05.2 & 12.98 & 10.02 & 19.06$\pm$2.06 & -49.13$\pm$2.06 & 10.0$\pm$1.4$^{(1)}$ & 19.7 & -45.2 & 100 & 0.2471\\ 
210948982 & 04 01 49.16 & +22 10 05.5 & 15.97 & 12.24 & 21.31$\pm$2.08 & -47.69$\pm$2.08 & 8.8$\pm$1.2$^{(1)}$ & 18.2 & -45.6 & 99 & 0.5601\\ 
210949534 & 03 49 11.24 & +22 10 36.3 & 12.85 & 10.1 & 23.96$\pm$2.08 & -48.1$\pm$2.08 & 9.0$\pm$1.2$^{(1)}$ & 19.7 & -45.2 & 100 & 5.9405\\ 
210949562 & 04 01 11.35 & +22 10 38.3 & 17.1 & 13.12 & 25.86$\pm$2.08 & -47.86$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 18.3 & -45.6 & 97 & 0.2419\\ 
210949721 & 03 49 48.43 & +22 10 48.6 & 15.58 & 11.99 & 18.3$\pm$2.06 & -47.31$\pm$2.06 & 6.3$\pm$0.9$^{(1)}$ & 19.7 & -45.2 & 100 & 1.6719\\ 
210950265 & 03 50 22.91 & +22 11 18.0 & 13.57 & 10.58 & 16.63$\pm$2.04 & -48.1$\pm$2.04 & 7.6$\pm$1.0$^{(1)}$ & 19.6 & -45.2 & 100 & 1.8957\\ 
210951703 & 03 48 25.50 & +22 12 41.7 & 13.42 & 10.6 & 21.78$\pm$2.08 & -44.69$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 19.8 & -45.2 & 100 & 0.3992\\ 
210956678 & 03 37 41.34 & +22 17 19.4 & 17.21 & 13.07 & 19.58$\pm$2.59 & -48.86$\pm$2.59 & 9.8$\pm$1.4$^{(1)}$ & 21.0 & -44.8 & 100 & 0.5602\\ 
210956858 & 03 29 19.12 & +22 17 30.4 & 11.8 & 10.0 & 17.71$\pm$0.86 & -37.53$\pm$0.82 & 6.3$\pm$0.9$^{(1)}$ & 22.0 & -44.5 & 62 &  \\ 
210957162 & 03 43 06.49 & +22 17 49.5 & 17.97 & 13.79 & 23.89$\pm$2.59 & -46.78$\pm$2.59 & 6.6$\pm$0.9$^{(1)}$ & 20.4 & -45.0 & 100 & 0.1748\\ 
210957703 & 04 05 13.71 & +22 18 18.7 & 16.48 & 12.41 & 15.89$\pm$2.08 & -47.65$\pm$2.08 & 11.1$\pm$1.5$^{(1)}$ & 17.8 & -45.7 & 93 & 0.2252\\ 
210958195 & 03 49 25.54 & +22 18 44.7 & 17.36 & 13.32 & 18.96$\pm$2.06 & -41.82$\pm$2.06 & 7.8$\pm$1.1$^{(1)}$ & 19.7 & -45.2 & 100 & 0.9081\\ 
210960579 & 03 37 24.05 & +22 21 03.6 & 9.03 & 7.9 & 20.99$\pm$0.75 & -46.45$\pm$0.88 & 6.4$\pm$0.3$^{(0)}$ & 21.1 & -44.8 & 100 & 3.3876\\ 
210962804 & 04 12 47.17 & +22 23 12.6 & 12.79 & 10.16 & 12.49$\pm$2.08 & -45.5$\pm$2.08 & 8.5$\pm$1.2$^{(1)}$ & 16.9 & -46.0 & 84 & $<$2\\ 
210963935 & 03 51 03.91 & +22 24 17.1 &   & 10.73 & 15.0$\pm$2.3 & -44.5$\pm$2.5 & 9.2$\pm$1.3$^{(2)}$ & 19.5 & -45.3 & 100 & 3.4151\\ 
210964488 & 03 35 46.40 & +22 24 50.1 & 17.22 & 13.27 & 26.12$\pm$2.55 & -44.23$\pm$2.55 & 7.4$\pm$1.0$^{(1)}$ & 21.3 & -44.8 & 100 & 0.4939\\ 
210964780 & 03 53 52.82 & +22 25 06.7 & 11.57 & 9.41 & 19.32$\pm$2.24 & -47.67$\pm$2.24 & 8.6$\pm$1.2$^{(1)}$ & 19.2 & -45.4 & 100 & 6.3353\\ 
210965110 & 03 44 29.49 & +22 25 25.0 & 18.11 & 13.9 & 18.9$\pm$2.6 & -51.48$\pm$2.6 & 6.9$\pm$1.0$^{(1)}$ & 20.3 & -45.1 & 100 & $<$2\\ 
210965155 & 03 42 59.75 & +22 25 27.4 & 13.22 & 10.59 & 17.42$\pm$2.1 & -48.04$\pm$2.1 & 6.5$\pm$0.9$^{(1)}$ & 20.4 & -45.0 & 100 & 6.536\\ 
210965709 & 03 57 32.00 & +22 26 00.3 & 16.48 & 12.34 & 18.41$\pm$2.08 & -44.73$\pm$2.08 & 11.9$\pm$1.6$^{(1)}$ & 18.7 & -45.5 & 98 & 0.4095\\ 
210965731 & 03 52 56.98 & +22 26 01.4 & 15.01 & 11.57 & 18.17$\pm$2.04 & -47.24$\pm$2.04 & 7.2$\pm$1.0$^{(1)}$ & 19.3 & -45.4 & 100 & 1.29\\ 
210966253 & 03 51 46.50 & +22 26 29.8 &   & 14.61 & 23.4$\pm$5.2 & -31.7$\pm$5.2 & 13.6$\pm$1.9$^{(4)}$ & 19.4 & -45.3 & 18 &  \\ 
210966700 & 03 43 19.03 & +22 26 57.3 &   & 9.03 & 22.5$\pm$2.4 & -45.6$\pm$2.6 & 12.2$\pm$1.7$^{(2)}$ & 20.4 & -45.0 & 99 & 5.0238\\ 
210966931 & 03 35 44.26 & +22 27 10.0 & 15.52 & 12.02 & 25.08$\pm$2.08 & -47.1$\pm$2.08 & 6.7$\pm$0.9$^{(1)}$ & 21.3 & -44.8 & 100 & 1.8867\\ 
210967582 & 03 59 07.04 & +22 27 48.5 & 16.7 & 12.5 & 19.3$\pm$2.07 & -39.22$\pm$2.07 & 12.3$\pm$1.7$^{(1)}$ & 18.5 & -45.6 & 68 & 0.2592\\ 
210967607 & 03 44 25.50 & +22 27 50.1 & 18.59 & 14.24 & 20.39$\pm$2.67 & -51.48$\pm$2.67 & 6.6$\pm$0.9$^{(1)}$ & 20.3 & -45.1 & 100 &  \\ 
210967650 & 03 44 41.82 & +22 27 52.4 & 10.51 & 9.07 & 22.72$\pm$2.15 & -44.94$\pm$0.53 & 7.3$\pm$0.6$^{(0)}$ & 20.2 & -45.1 & 100 & 3.9912\\ 
210967901 & 03 50 37.41 & +22 28 08.4 & 16.16 & 12.37 & 19.17$\pm$2.05 & -48.59$\pm$2.05 & 8.5$\pm$1.2$^{(1)}$ & 19.6 & -45.3 & 100 & 1.7941\\ 
210968957 & 03 33 03.27 & +22 29 09.3 & 17.65 & 13.65 & 22.49$\pm$2.92 & -41.32$\pm$2.72 & 6.4$\pm$0.9$^{(1)}$ & 21.6 & -44.7 & 100 &  \\ 
210969800 & 03 38 22.58 & +22 29 58.9 & 9.88 & 8.7 & 21.39$\pm$0.13 & -44.82$\pm$0.08 & 7.5$\pm$0.3$^{(0)}$ & 21.0 & -44.9 & 100 & 2.1116\\ 
210969937 & 03 52 34.47 & +22 30 07.7 & 14.78 & 11.39 & 17.7$\pm$2.05 & -44.4$\pm$2.05 & 7.3$\pm$1.0$^{(1)}$ & 19.3 & -45.4 & 100 & 1.7664\\ 
210970475 & 03 53 53.32 & +22 30 37.8 & 17.74 & 13.67 & 19.15$\pm$2.51 & -48.18$\pm$2.51 & 6.2$\pm$0.9$^{(1)}$ & 19.2 & -45.4 & 100 &  \\ 
210971138 & 03 33 10.49 & +22 31 19.3 & 14.44 & 11.25 & 20.63$\pm$2.13 & -51.74$\pm$2.13 & 6.8$\pm$0.9$^{(1)}$ & 21.5 & -44.7 & 99 &  \\ 
210971340 & 03 45 26.55 & +22 31 32.2 & 15.94 & 12.25 & 20.84$\pm$2.1 & -48.22$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 20.2 & -45.1 & 100 & 1.2096\\ 
210971348 & 03 52 51.72 & +22 31 32.8 & 15.57 & 11.91 & 18.79$\pm$2.05 & -49.9$\pm$2.05 & 8.2$\pm$1.1$^{(1)}$ & 19.3 & -45.4 & 100 & 1.1077\\ 
210974237 & 03 59 22.90 & +22 34 17.0 & 13.6 & 10.56 & 17.15$\pm$2.08 & -45.89$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 18.5 & -45.6 & 100 & 1.8839\\ 
210974364 & 03 42 27.30 & +22 34 24.9 & 15.53 & 11.86 & 17.52$\pm$2.1 & -45.87$\pm$2.1 & 10.3$\pm$1.4$^{(1)}$ & 20.5 & -45.0 & 100 & 1.9793\\ 
210974893 & 03 52 05.57 & +22 34 55.4 & 14.92 & 11.48 & 19.96$\pm$2.04 & -46.54$\pm$2.04 & 7.3$\pm$1.0$^{(1)}$ & 19.4 & -45.4 & 100 & 1.9861\\ 
210977069 & 04 06 28.54 & +22 37 00.1 & 15.91 & 12.12 & 13.41$\pm$2.08 & -45.54$\pm$2.08 & 8.3$\pm$1.1$^{(1)}$ & 17.6 & -45.8 & 98 & 5.2158\\ 
210977779 & 03 43 27.43 & +22 37 41.4 & 17.16 & 13.25 & 23.43$\pm$2.1 & -55.51$\pm$2.1 & 6.9$\pm$0.9$^{(1)}$ & 20.4 & -45.1 & 98 & 0.5047\\ 
210978650 & 03 45 08.68 & +22 38 30.7 & 16.28 & 12.48 & 22.97$\pm$2.1 & -52.89$\pm$2.1 & 9.0$\pm$1.2$^{(1)}$ & 20.2 & -45.1 & 99 & 0.4623\\ 
210978953 & 03 40 07.00 & +22 38 47.7 & 16.98 & 13.05 & 21.06$\pm$2.1 & -48.45$\pm$2.1 & 8.1$\pm$1.1$^{(1)}$ & 20.8 & -45.0 & 100 & 0.482\\ 
210979439 & 03 39 44.78 & +22 39 15.6 & 16.62 & 12.73 & 18.96$\pm$2.1 & -50.81$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 20.8 & -45.0 & 100 & 0.6961\\ 
210979763 & 03 38 40.72 & +22 39 34.6 &   & 6.67 & 19.88$\pm$0.63 & -45.25$\pm$0.57 & 8.1$\pm$0.5$^{(0)}$ & 20.9 & -44.9 & 100 &  \\ 
210980418 & 03 58 34.17 & +22 40 11.5 & 17.08 & 13.0 & 23.91$\pm$2.08 & -45.34$\pm$2.08 & 7.9$\pm$1.1$^{(1)}$ & 18.6 & -45.6 & 100 & 0.6841\\ 
210982048 & 03 45 39.90 & +22 41 40.1 & 7.8 & 7.37 & 19.14$\pm$0.37 & -43.81$\pm$0.36 & 7.8$\pm$0.3$^{(0)}$ & 20.1 & -45.2 & 100 &  \\ 
210982092 & 03 53 21.87 & +22 41 42.8 & 13.56 & 11.04 & 16.37$\pm$2.04 & -35.98$\pm$2.04 & 5.5$\pm$0.8$^{(1)}$ & 19.2 & -45.4 & 68 &  \\ 
210982234 & 03 45 12.43 & +22 41 51.1 & 16.0 & 12.27 & 19.82$\pm$2.1 & -51.53$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 20.2 & -45.2 & 100 & 0.7676\\ 
210982519 & 03 37 50.93 & +22 42 06.7 & 15.9 & 12.09 & 27.52$\pm$2.1 & -36.14$\pm$2.1 & 9.8$\pm$1.4$^{(1)}$ & 21.0 & -44.9 & 19 &  \\ 
210982761 & 03 46 13.85 & +22 42 19.9 & 16.39 & 12.46 & 18.83$\pm$2.1 & -50.62$\pm$2.1 & 10.1$\pm$1.4$^{(1)}$ & 20.1 & -45.2 & 99 & 0.3079\\ 
210983092 & 03 46 09.59 & +22 42 37.5 & 15.63 & 11.9 & 19.53$\pm$2.1 & -48.71$\pm$2.1 & 10.3$\pm$1.4$^{(1)}$ & 20.1 & -45.2 & 100 & 0.8677\\ 
210984736 & 03 43 29.29 & +22 44 05.4 & 8.85 & 7.45 & 22.26$\pm$0.68 & -45.6$\pm$0.48 & 18.9$\pm$2.6$^{(1)}$ & 20.4 & -45.1 & 71 &  \\ 
210984840 & 04 06 19.95 & +22 44 10.9 &   & 9.31 & 13.3$\pm$2.0 & -49.0$\pm$1.5 & 12.4$\pm$1.7$^{(2)}$ & 17.7 & -45.8 & 50 &  \\ 
210988056 & 03 43 19.00 & +22 47 10.7 & 16.66 & 12.76 & 24.13$\pm$2.1 & -50.2$\pm$2.1 & 9.0$\pm$1.2$^{(1)}$ & 20.4 & -45.1 & 100 & 0.3057\\ 
210988354 & 03 42 29.42 & +22 47 26.1 & 14.06 & 10.92 & 18.83$\pm$2.1 & -48.36$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.5 & -45.1 & 100 & 0.325\\ 
210989020 & 03 43 04.19 & +22 48 03.5 & 14.13 & 10.78 & 20.56$\pm$2.1 & -48.72$\pm$2.1 & 9.3$\pm$1.3$^{(1)}$ & 20.4 & -45.1 & 100 & 0.3103\\ 
210989043 & 03 47 34.78 & +22 48 04.9 & 15.82 & 12.15 & 22.77$\pm$2.08 & -48.2$\pm$2.08 & 8.4$\pm$1.2$^{(1)}$ & 19.9 & -45.3 & 100 & 0.6966\\ 
210990525 & 03 35 31.69 & +22 49 24.9 & 9.69 & 8.54 & 21.48$\pm$0.15 & -45.39$\pm$0.08 & 7.7$\pm$0.2$^{(0)}$ & 21.3 & -44.8 & 100 & 2.7953\\ 
210991032 & 03 47 27.63 & +22 49 53.4 & 15.93 & 12.29 & 17.87$\pm$2.08 & -44.11$\pm$2.08 & 7.3$\pm$1.0$^{(1)}$ & 19.9 & -45.3 & 100 & $<$2\\ 
210991829 & 03 46 40.40 & +22 50 39.8 & 17.1 & 13.18 & 23.31$\pm$2.1 & -54.41$\pm$2.1 & 6.9$\pm$1.0$^{(1)}$ & 20.0 & -45.2 & 99 & 0.2955\\ 
210992480 & 03 42 56.54 & +22 51 18.2 & 17.93 & 13.78 & 19.62$\pm$2.59 & -50.13$\pm$2.59 & 6.4$\pm$0.9$^{(1)}$ & 20.4 & -45.1 & 100 & $<$2\\ 
210992697 & 03 42 04.72 & +22 51 30.8 & 9.02 & 8.0 & 21.05$\pm$0.14 & -44.65$\pm$0.07 & 7.4$\pm$0.2$^{(0)}$ & 20.5 & -45.1 & 100 & $<$2\\ 
210993561 & 03 48 22.64 & +22 52 21.7 & 14.89 & 11.48 & 23.57$\pm$2.08 & -50.84$\pm$2.08 & 7.4$\pm$1.0$^{(1)}$ & 19.8 & -45.3 & 100 & 1.1389\\ 
210994089 & 03 46 53.27 & +22 52 51.3 & 11.46 & 9.72 & 18.91$\pm$0.92 & -41.34$\pm$1.0 & 6.3$\pm$0.9$^{(1)}$ & 20.0 & -45.2 & 100 & 6.1515\\ 
210994935 & 03 42 26.29 & +22 53 40.7 & 13.56 & 10.72 & 19.87$\pm$2.09 & -48.84$\pm$2.09 & 6.8$\pm$0.9$^{(1)}$ & 20.5 & -45.1 & 100 & 4.2264\\ 
210995008 & 03 43 25.15 & +22 53 44.6 & 16.76 & 12.91 & 28.17$\pm$2.1 & -51.29$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.4 & -45.1 & 98 & 1.2523\\ 
210995339 & 03 42 59.21 & +22 54 03.2 & 11.71 & 9.71 & 20.59$\pm$1.03 & -42.04$\pm$0.96 & 7.8$\pm$1.1$^{(1)}$ & 20.4 & -45.1 & 100 & 6.6996\\ 
210996142 & 03 46 47.06 & +22 54 52.4 & 10.29 & 8.93 & 18.29$\pm$0.91 & -44.34$\pm$0.45 & 7.5$\pm$0.3$^{(0)}$ & 20.0 & -45.2 & 100 & 3.0025\\ 
210996505 & 03 46 38.39 & +22 55 11.2 & 9.27 & 8.15 & 19.32$\pm$0.74 & -43.27$\pm$0.39 & 7.3$\pm$0.3$^{(0)}$ & 20.0 & -45.2 & 100 & 6.839\\ 
210996662 & 03 47 22.90 & +22 55 19.6 & 8.12 & 7.52 & 21.62$\pm$0.05 & -47.04$\pm$0.03 & 6.6$\pm$0.7$^{(0)}$ & 19.9 & -45.3 & 100 & 1.456\\ 
210996915 & 03 57 34.60 & +22 55 32.6 & 13.25 & 10.64 & 23.72$\pm$2.08 & -40.66$\pm$2.08 & 6.7$\pm$0.9$^{(1)}$ & 18.7 & -45.6 & 99 & 8.9066\\ 
210997197 & 03 47 40.97 & +22 55 47.9 & 11.71 & 9.36 & 19.71$\pm$1.01 & -45.38$\pm$0.91 & 11.3$\pm$1.6$^{(1)}$ & 19.9 & -45.3 & 100 & 1.7668\\ 
210997261 & 03 44 44.44 & +22 55 51.7 & 16.45 & 12.55 & 11.23$\pm$2.12 & -37.42$\pm$2.1 & 8.6$\pm$1.2$^{(1)}$ & 20.2 & -45.2 & 31 & $<$2\\ 
210997742 & 03 33 49.80 & +22 56 20.1 & 17.04 & 13.29 & 23.19$\pm$2.08 & -50.61$\pm$2.08 & 5.7$\pm$0.8$^{(1)}$ & 21.5 & -44.8 & 99 & 0.3744\\ 
210998086 & 04 03 44.17 & +22 56 39.4 & 9.49 & 8.18 & 17.57$\pm$0.09 & -44.81$\pm$0.06 & 7.2$\pm$0.3$^{(0)}$ & 18.0 & -45.8 & 100 &  \\ 
210998478 & 03 41 58.65 & +22 57 02.0 & 15.43 & 11.9 & 19.85$\pm$2.1 & -51.12$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.6 & -45.1 & 100 & 6.842\\ 
211000411 & 03 49 01.00 & +22 58 49.5 & 14.34 & 11.15 & 21.03$\pm$2.08 & -52.54$\pm$2.08 & 7.1$\pm$1.0$^{(1)}$ & 19.7 & -45.3 & 100 & 8.5889\\ 
211000470 & 03 46 05.24 & +22 58 53.8 & 13.28 & 10.5 & 19.96$\pm$2.1 & -51.8$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.1 & -45.2 & 100 & 9.8931\\ 
211000740 & 03 57 35.26 & +22 59 08.2 & 15.27 & 11.65 & 19.94$\pm$2.08 & -46.28$\pm$2.08 & 7.9$\pm$1.1$^{(1)}$ & 18.7 & -45.6 & 100 & 0.9594\\ 
211001183 & 03 47 52.86 & +22 59 34.2 & 16.01 & 12.15 & 20.82$\pm$2.08 & -51.63$\pm$2.08 & 12.1$\pm$1.7$^{(1)}$ & 19.9 & -45.3 & 97 & 0.5169\\ 
211001695 & 03 48 10.17 & +23 00 04.1 & 13.77 & 11.0 & 15.74$\pm$2.08 & -41.49$\pm$2.08 & 5.9$\pm$0.8$^{(1)}$ & 19.8 & -45.3 & 100 & 6.5481\\ 
211001714 & 03 47 39.77 & +23 00 04.8 & 17.06 & 13.24 & 24.81$\pm$2.08 & -51.89$\pm$2.08 & 7.0$\pm$1.0$^{(1)}$ & 19.9 & -45.3 & 100 & 0.4571\\ 
211002011 & 03 33 13.88 & +23 00 23.1 & 11.59 & 9.67 & 23.34$\pm$1.28 & -49.11$\pm$0.68 & 7.9$\pm$0.3$^{(0)}$ & 21.5 & -44.8 & 100 & 7.6495\\ 
211002561 & 03 46 19.40 & +23 00 55.9 &   & 13.15 & 19.9$\pm$5.1 & -49.2$\pm$5.1 & 20.7$\pm$2.9$^{(4)}$ & 20.1 & -45.2 & 14 & 0.1807\\ 
211002985 & 03 41 46.65 & +23 01 19.9 & 17.11 & 13.16 & 24.76$\pm$2.59 & -54.66$\pm$2.59 & 7.3$\pm$1.0$^{(1)}$ & 20.6 & -45.1 & 99 & 0.2943\\ 
211003154 & 03 45 56.96 & +23 01 29.2 & 16.34 & 12.58 & 23.3$\pm$2.1 & -50.52$\pm$2.1 & 8.3$\pm$1.1$^{(1)}$ & 20.1 & -45.2 & 100 & 0.5743\\ 
211003258 & 03 46 31.01 & +23 01 34.9 & 17.8 & 13.7 & 17.38$\pm$2.6 & -50.46$\pm$2.6 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -45.3 & 100 & 0.7278\\ 
211003744 & 03 48 05.82 & +23 02 02.9 & 14.96 & 11.53 & 20.7$\pm$2.08 & -51.51$\pm$2.08 & 7.3$\pm$1.0$^{(1)}$ & 19.8 & -45.3 & 100 & 1.562\\ 
211004119 & 03 44 38.94 & +23 02 25.5 & 16.79 & 12.5 & 19.89$\pm$2.1 & -50.55$\pm$2.1 & 14.9$\pm$2.1$^{(1)}$ & 20.2 & -45.2 & 83 & 0.8297\\ 
211004548 & 03 49 25.60 & +23 02 50.3 & 17.14 & 13.16 & 20.46$\pm$2.08 & -53.54$\pm$2.08 & 7.4$\pm$1.0$^{(1)}$ & 19.7 & -45.4 & 100 & 0.3094\\ 
211004687 & 03 45 10.81 & +23 02 58.4 & 16.13 & 12.35 & 16.28$\pm$2.1 & -52.12$\pm$2.1 & 8.9$\pm$1.2$^{(1)}$ & 20.2 & -45.2 & 99 & 0.9335\\ 
211005117 & 03 43 44.97 & +23 03 21.2 & 15.35 & 11.7 & 20.52$\pm$2.1 & -48.91$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 20.4 & -45.2 & 100 & 2.3235\\ 
211005163 & 03 41 48.95 & +23 03 23.5 & 17.58 & 13.19 & 23.66$\pm$2.59 & -44.68$\pm$2.59 & 10.7$\pm$1.5$^{(1)}$ & 20.6 & -45.1 & 100 & 0.2391\\ 
211005706 & 03 50 27.82 & +23 03 55.3 & 16.8 & 12.94 & 25.2$\pm$2.06 & -47.67$\pm$2.06 & 7.4$\pm$1.0$^{(1)}$ & 19.6 & -45.4 & 100 & 0.5589\\ 
211005799 & 03 46 21.62 & +23 04 01.2 & 16.75 & 12.68 & 21.82$\pm$2.1 & -51.39$\pm$2.1 & 10.0$\pm$1.4$^{(1)}$ & 20.1 & -45.3 & 100 & 0.6772\\ 
211005924 & 03 46 48.78 & +23 04 07.3 & 14.86 & 11.47 & 22.55$\pm$2.1 & -48.21$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.0 & -45.3 & 100 & 0.2845\\ 
211006027 & 03 58 30.98 & +23 04 13.0 & 17.26 & 13.13 & 20.7$\pm$2.58 & -46.22$\pm$2.58 & 8.1$\pm$1.1$^{(1)}$ & 18.6 & -45.7 & 100 & 0.2924\\ 
211006108 & 03 46 36.06 & +23 04 17.4 & 15.73 & 12.07 & 21.21$\pm$2.1 & -50.38$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 20.0 & -45.3 & 100 & 0.9588\\ 
211006328 & 03 48 50.66 & +23 04 30.4 & 17.03 & 13.12 & 21.24$\pm$2.08 & -54.69$\pm$2.08 & 8.2$\pm$1.1$^{(1)}$ & 19.8 & -45.3 & 99 & 0.3617\\ 
211006594 & 03 44 08.81 & +23 04 47.7 & 14.32 & 11.13 & 21.7$\pm$2.1 & -49.85$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.3 & -45.2 & 100 & 0.5739\\ 
211007016 & 03 46 21.39 & +23 05 09.3 & 17.74 & 13.74 & 22.71$\pm$2.6 & -48.68$\pm$2.6 & 6.9$\pm$0.9$^{(1)}$ & 20.1 & -45.3 & 100 & 0.3742\\ 
211007344 & 03 56 24.98 & +23 05 26.9 & 14.2 & 11.08 & 17.9$\pm$2.08 & -45.74$\pm$2.08 & 6.8$\pm$0.9$^{(1)}$ & 18.9 & -45.6 & 100 & 14.5813\\ 
211007577 & 03 48 58.28 & +23 05 39.1 & 15.08 & 11.66 & 21.64$\pm$2.08 & -53.32$\pm$2.08 & 7.2$\pm$1.0$^{(1)}$ & 19.7 & -45.4 & 100 & 13.6986\\ 
211007717 & 03 50 21.30 & +23 05 47.0 & 11.1 & 9.39 & 20.87$\pm$2.24 & -46.43$\pm$0.51 & 7.2$\pm$0.6$^{(0)}$ & 19.6 & -45.4 & 100 & 5.3657\\ 
211007968 & 04 05 32.25 & +23 06 01.0 & 12.07 & 10.27 & 21.0$\pm$0.84 & -40.48$\pm$0.89 & 5.0$\pm$0.7$^{(1)}$ & 17.8 & -45.9 & 26 &  \\ 
211008237 & 03 42 44.36 & +23 06 16.4 & 16.89 & 12.95 & 17.2$\pm$2.1 & -51.34$\pm$2.1 & 8.4$\pm$1.2$^{(1)}$ & 20.5 & -45.1 & 100 & 0.4288\\ 
211008337 & 03 49 05.92 & +23 06 21.9 & 15.91 & 12.23 & 22.3$\pm$3.57 & -54.88$\pm$3.57 & 8.5$\pm$1.2$^{(1)}$ & 19.7 & -45.4 & 100 & 1.1187\\ 
211008438 & 03 38 23.38 & +23 06 29.0 & 14.14 & 11.04 & 23.04$\pm$2.1 & -50.42$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 21.0 & -45.0 & 100 & 3.7479\\ 
211008578 & 03 46 40.00 & +23 06 37.2 & 9.26 & 8.24 & 19.41$\pm$0.67 & -46.39$\pm$0.36 & 7.5$\pm$0.3$^{(0)}$ & 20.0 & -45.3 & 100 & 1.8161\\ 
211009416 & 03 59 27.53 & +23 07 25.6 &   & 10.13 & 14.1$\pm$1.9 & -39.2$\pm$2.1 & 8.6$\pm$1.2$^{(2)}$ & 18.5 & -45.7 & 94 & 0.4423\\ 
211010041 & 03 41 26.35 & +23 08 03.0 & 16.56 & 12.62 & 19.99$\pm$2.09 & -48.91$\pm$2.09 & 8.6$\pm$1.2$^{(1)}$ & 20.6 & -45.1 & 100 & 0.8393\\ 
211010059 & 03 44 17.15 & +23 08 03.9 & 15.88 & 12.12 & 14.75$\pm$2.13 & -40.39$\pm$2.13 & 7.9$\pm$1.1$^{(1)}$ & 20.3 & -45.2 & 99 &  \\ 
211010149 & 03 48 23.92 & +23 08 08.5 & 17.08 & 13.21 & 17.2$\pm$2.55 & -48.82$\pm$2.55 & 7.3$\pm$1.0$^{(1)}$ & 19.8 & -45.3 & 100 & 0.3215\\ 
211010517 & 04 02 34.77 & +23 08 28.7 & 16.53 & 12.78 & 15.14$\pm$2.1 & -34.79$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 18.1 & -45.8 & 27 & 0.7557\\ 
211010807 & 03 42 51.68 & +23 08 44.1 & 16.65 & 12.56 & 24.14$\pm$2.1 & -52.16$\pm$2.1 & 10.9$\pm$1.5$^{(1)}$ & 20.5 & -45.1 & 97 & 0.4038\\ 
211010818 & 03 36 38.39 & +23 08 44.5 & 17.35 & 13.27 & 20.49$\pm$2.59 & -48.29$\pm$2.59 & 7.6$\pm$1.0$^{(1)}$ & 21.2 & -44.9 & 100 & 0.304\\ 
211010854 & 03 44 09.31 & +23 08 47.1 & 16.41 & 12.51 & 22.56$\pm$2.1 & -50.7$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 20.3 & -45.2 & 100 & 0.5153\\ 
211011030 & 03 47 23.85 & +23 08 57.2 & 15.7 & 12.08 & 20.48$\pm$2.08 & -49.5$\pm$2.08 & 8.3$\pm$1.1$^{(1)}$ & 19.9 & -45.3 & 100 & 1.6638\\ 
211011793 & 03 41 32.45 & +23 09 42.1 & 12.3 & 10.12 & 19.07$\pm$2.09 & -49.02$\pm$2.09 & 6.1$\pm$0.8$^{(1)}$ & 20.6 & -45.1 & 100 &  \\ 
211011910 & 03 51 19.47 & +23 09 49.7 & 15.9 & 12.19 & 17.55$\pm$2.11 & -47.83$\pm$2.11 & 8.1$\pm$1.1$^{(1)}$ & 19.5 & -45.4 & 100 & 0.9248\\ 
211012313 & 03 45 27.71 & +23 10 13.3 & 15.24 & 11.7 & 10.48$\pm$2.1 & -41.17$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 20.2 & -45.2 & 84 &  \\ 
211012609 & 04 01 13.98 & +23 10 30.2 & 15.69 & 12.03 & 17.71$\pm$2.08 & -44.91$\pm$2.08 & 7.3$\pm$1.0$^{(1)}$ & 18.3 & -45.8 & 100 & 1.5063\\ 
211012996 & 03 44 22.13 & +23 10 55.1 & 18.0 & 13.46 & 21.97$\pm$2.6 & -50.24$\pm$2.6 & 9.9$\pm$1.4$^{(1)}$ & 20.3 & -45.2 & 100 & 0.2991\\ 
211013046 & 03 37 37.07 & +23 10 58.1 & 16.6 & 12.81 & 26.14$\pm$2.1 & -48.28$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 21.0 & -45.0 & 100 & 0.358\\ 
211013066 & 03 51 38.03 & +23 10 59.3 & 12.7 & 10.03 & 20.01$\pm$2.12 & -55.52$\pm$2.12 & 8.8$\pm$1.2$^{(1)}$ & 19.4 & -45.5 & 97 & 3.9578\\ 
211013159 & 03 37 16.52 & +23 11 04.6 & 16.34 & 12.55 & 20.28$\pm$2.1 & -55.09$\pm$2.1 & 8.3$\pm$1.1$^{(1)}$ & 21.1 & -45.0 & 96 & 0.4487\\ 
211013191 & 03 45 33.99 & +23 11 06.9 & 16.94 & 13.0 & 19.24$\pm$2.1 & -49.56$\pm$2.1 & 8.2$\pm$1.1$^{(1)}$ & 20.1 & -45.2 & 100 & 0.5883\\ 
211013627 & 03 42 15.36 & +23 11 31.2 & 16.95 & 13.06 & 21.75$\pm$2.59 & -47.19$\pm$2.59 & 8.5$\pm$1.2$^{(1)}$ & 20.5 & -45.1 & 100 & 1.0188\\ 
211014186 & 03 48 58.48 & +23 12 04.2 & 11.26 & 9.38 & 20.81$\pm$0.94 & -44.74$\pm$0.94 & 8.4$\pm$1.2$^{(1)}$ & 19.7 & -45.4 & 100 & 6.0067\\ 
211014750 & 03 43 36.56 & +23 12 34.4 & 16.25 & 12.38 & 25.9$\pm$2.1 & -52.69$\pm$2.1 & 9.9$\pm$1.4$^{(1)}$ & 20.4 & -45.2 & 97 & 0.314\\ 
211014883 & 03 43 47.48 & +23 12 42.5 & 10.27 & 8.55 & 20.49$\pm$1.33 & -41.56$\pm$1.42 & 11.0$\pm$1.5$^{(1)}$ & 20.3 & -45.2 & 99 & 5.0872\\ 
211015258 & 03 50 38.90 & +23 13 02.8 & 15.21 & 11.75 & 17.8$\pm$2.05 & -49.26$\pm$2.05 & 6.7$\pm$0.9$^{(1)}$ & 19.6 & -45.4 & 100 & 0.8891\\ 
211015308 & 03 47 48.11 & +23 13 05.1 & 10.88 & 9.32 & 20.83$\pm$0.64 & -45.99$\pm$0.32 & 7.4$\pm$0.3$^{(0)}$ & 19.9 & -45.3 & 100 & 5.1371\\ 
211015348 & 03 49 56.49 & +23 13 07.0 & 10.09 & 8.8 & 20.07$\pm$1.47 & -42.8$\pm$0.37 & 6.6$\pm$0.4$^{(0)}$ & 19.6 & -45.4 & 100 & 2.1762\\ 
211015806 & 03 59 41.19 & +23 13 31.2 & 16.53 & 12.72 & 15.39$\pm$2.08 & -35.98$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 18.5 & -45.7 & 71 & $<$2\\ 
211015853 & 03 43 24.54 & +23 13 33.4 & 10.28 & 8.65 & 20.45$\pm$0.72 & -41.71$\pm$0.38 & 7.4$\pm$0.2$^{(0)}$ & 20.4 & -45.2 & 100 & 2.7573\\ 
211015877 & 03 47 07.34 & +23 13 34.9 & 13.01 & 10.36 & 18.66$\pm$2.08 & -49.26$\pm$2.08 & 7.7$\pm$1.1$^{(1)}$ & 20.0 & -45.3 & 100 & 0.3889\\ 
211016037 & 03 49 12.30 & +23 13 42.1 & 13.5 & 10.66 & 20.79$\pm$2.08 & -52.31$\pm$2.08 & 6.9$\pm$1.0$^{(1)}$ & 19.7 & -45.4 & 100 & 5.3258\\ 
211016313 & 03 32 07.86 & +23 13 57.6 & 15.94 & 12.25 & 22.8$\pm$2.08 & -45.87$\pm$2.08 & 8.0$\pm$1.1$^{(1)}$ & 21.7 & -44.8 & 100 & 0.3193\\ 
211017407 & 03 49 41.13 & +23 14 59.6 & 17.38 & 13.06 & 20.61$\pm$2.54 & -48.63$\pm$2.54 & 10.9$\pm$1.5$^{(1)}$ & 19.7 & -45.4 & 100 & 0.1971\\ 
211017469 & 03 46 57.10 & +23 15 02.4 & 14.33 & 11.14 & 20.83$\pm$2.1 & -49.99$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.0 & -45.3 & 100 & 1.2062\\ 
211017570 & 03 49 02.33 & +23 15 08.8 & 11.4 & 9.66 & 19.44$\pm$0.85 & -47.64$\pm$0.85 & 6.8$\pm$0.9$^{(1)}$ & 19.7 & -45.4 & 100 & 6.1535\\ 
211018096 & 03 48 43.90 & +23 15 35.3 & 8.32 & 7.63 & 19.38$\pm$0.43 & -44.39$\pm$0.3 & 7.0$\pm$0.3$^{(0)}$ & 19.8 & -45.4 & 100 & 0.0356\\ 
211018106 & 03 41 25.96 & +23 15 36.1 & 16.66 & 12.82 & 26.02$\pm$2.1 & -49.28$\pm$2.1 & 8.8$\pm$1.2$^{(1)}$ & 20.6 & -45.1 & 100 & 0.5384\\ 
211018285 & 03 36 52.53 & +23 15 45.3 & 13.1 & 10.62 & 15.46$\pm$2.1 & -41.49$\pm$2.1 & 6.5$\pm$0.9$^{(1)}$ & 21.1 & -45.0 & 99 &  \\ 
211018711 & 03 44 51.24 & +23 16 08.1 & 8.86 & 7.98 & 20.52$\pm$0.09 & -44.28$\pm$0.06 & 7.7$\pm$0.3$^{(0)}$ & 20.2 & -45.2 & 100 &  \\ 
211018906 & 03 49 32.16 & +23 16 18.2 & 17.34 & 13.44 & 18.39$\pm$2.08 & -55.05$\pm$2.08 & 6.7$\pm$0.9$^{(1)}$ & 19.7 & -45.4 & 99 & 0.3855\\ 
211019565 & 03 51 15.82 & +23 16 56.2 & 13.95 & 10.85 & 21.03$\pm$2.11 & -48.64$\pm$2.11 & 7.4$\pm$1.0$^{(1)}$ & 19.5 & -45.5 & 100 & 0.4479\\ 
211020101 & 03 49 39.39 & +23 17 24.4 & 10.94 & 9.26 & 18.47$\pm$0.95 & -44.31$\pm$0.48 & 7.5$\pm$0.3$^{(0)}$ & 19.7 & -45.4 & 100 & 5.0132\\ 
211020742 & 03 48 28.03 & +23 18 02.7 & 12.12 & 9.84 & 19.19$\pm$2.3 & -51.25$\pm$2.3 & 8.7$\pm$1.2$^{(1)}$ & 19.8 & -45.4 & 100 & 0.2353\\ 
211020988 & 03 50 04.99 & +23 18 17.6 & 17.36 & 13.42 & 27.36$\pm$2.05 & -48.26$\pm$2.05 & 7.0$\pm$1.0$^{(1)}$ & 19.6 & -45.4 & 99 & 0.321\\ 
211021014 & 03 46 32.87 & +23 18 19.1 & 13.86 & 10.81 & 18.14$\pm$2.1 & -48.53$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.0 & -45.3 & 100 & 6.9448\\ 
211021827 & 03 47 55.28 & +23 19 06.0 & 15.65 & 12.14 & 20.56$\pm$2.08 & -46.69$\pm$2.08 & 6.5$\pm$0.9$^{(1)}$ & 19.9 & -45.4 & 100 & 1.3661\\ 
211022535 & 03 45 49.93 & +23 19 45.0 & 17.95 & 13.61 & 19.77$\pm$2.6 & -49.45$\pm$2.6 & 8.4$\pm$1.2$^{(1)}$ & 20.1 & -45.3 & 100 &  \\ 
211022539 & 03 50 51.44 & +23 19 45.1 & 12.08 & 10.02 & 19.51$\pm$1.12 & -47.28$\pm$0.6 & 7.1$\pm$0.3$^{(0)}$ & 19.5 & -45.5 & 100 & 8.4496\\ 
211023004 & 03 45 42.86 & +23 20 12.4 & 17.2 & 13.19 & 22.18$\pm$2.1 & -52.54$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.1 & -45.3 & 100 & $<$2\\ 
211023137 & 03 48 45.42 & +23 20 20.1 & 12.75 & 10.34 & 19.52$\pm$2.08 & -49.94$\pm$2.08 & 7.0$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 3.92\\ 
211023176 & 03 51 57.34 & +23 20 21.9 & 12.58 & 10.2 & 19.52$\pm$2.08 & -48.62$\pm$2.08 & 6.9$\pm$1.0$^{(1)}$ & 19.4 & -45.5 & 100 & 7.3022\\ 
211023213 & 03 46 10.04 & +23 20 24.0 & 9.96 & 8.66 & 21.02$\pm$1.49 & -49.87$\pm$0.66 & 8.6$\pm$0.6$^{(0)}$ & 20.1 & -45.3 & 100 & 2.8527\\ 
211023311 & 03 49 40.92 & +23 20 29.7 & 8.09 & 7.65 & 19.32$\pm$0.53 & -44.76$\pm$0.46 & 7.2$\pm$0.3$^{(0)}$ & 19.7 & -45.4 & 100 &  \\ 
211023807 & 03 51 07.10 & +23 20 57.8 & 16.62 & 12.84 & 18.51$\pm$2.05 & -46.91$\pm$2.05 & 7.2$\pm$1.0$^{(1)}$ & 19.5 & -45.5 & 100 & 0.5784\\ 
211024158 & 03 44 59.47 & +23 21 18.5 & 17.38 & 13.41 & 26.49$\pm$2.1 & -51.68$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.2 & -45.3 & 100 & 0.2388\\ 
211024494 & 03 47 22.02 & +23 21 36.7 & 16.52 & 12.73 & 25.16$\pm$2.08 & -48.06$\pm$2.08 & 8.7$\pm$1.2$^{(1)}$ & 19.9 & -45.3 & 100 & 0.3687\\ 
211024798 & 03 45 12.15 & +23 21 53.2 & 15.95 & 12.28 & 19.5$\pm$2.1 & -51.93$\pm$2.1 & 8.1$\pm$1.1$^{(1)}$ & 20.2 & -45.3 & 100 & 0.7494\\ 
211025002 & 03 51 39.07 & +23 22 04.6 & 16.93 & 13.12 & 19.05$\pm$2.12 & -56.14$\pm$2.12 & 7.1$\pm$1.0$^{(1)}$ & 19.4 & -45.5 & 97 & 0.3185\\ 
211025007 & 03 42 36.27 & +23 22 05.0 & 15.98 & 12.28 & 19.46$\pm$2.1 & -46.18$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.5 & -45.2 & 100 & 1.551\\ 
211025708 & 03 50 27.34 & +23 22 45.3 & 16.39 & 12.52 & 20.51$\pm$2.06 & -51.57$\pm$2.06 & 9.3$\pm$1.3$^{(1)}$ & 19.6 & -45.4 & 100 & 0.9801\\ 
211025716 & 03 44 11.20 & +23 22 45.6 & 11.13 & 9.41 & 22.12$\pm$0.87 & -46.98$\pm$0.5 & 8.0$\pm$0.3$^{(0)}$ & 20.3 & -45.2 & 100 & 2.5292\\ 
211025770 & 03 49 32.72 & +23 22 49.5 & 9.01 & 8.04 & 19.91$\pm$0.74 & -43.86$\pm$0.46 & 7.4$\pm$0.3$^{(0)}$ & 19.7 & -45.4 & 100 & 0.2389\\ 
211025773 & 03 49 15.61 & +23 22 49.5 & 17.5 & 13.46 & 22.1$\pm$2.55 & -54.76$\pm$2.55 & 7.3$\pm$1.0$^{(1)}$ & 19.7 & -45.4 & 100 & 0.5256\\ 
211025779 & 03 46 55.30 & +23 22 49.6 & 17.29 & 13.3 & 22.44$\pm$2.1 & -49.72$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.0 & -45.3 & 100 & 0.2824\\ 
211025925 & 03 37 56.41 & +23 22 56.9 & 15.68 & 12.07 & 27.0$\pm$2.1 & -51.57$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 21.0 & -45.0 & 99 & 0.8969\\ 
211026087 & 03 41 13.81 & +23 23 05.8 & 13.35 & 10.63 & 23.35$\pm$1.75 & -42.3$\pm$2.12 & 6.8$\pm$0.9$^{(1)}$ & 20.6 & -45.1 & 100 & 10.0234\\ 
211026321 & 03 44 58.95 & +23 23 20.2 & 13.24 & 10.49 & 18.57$\pm$2.1 & -50.42$\pm$2.1 & 7.4$\pm$1.0$^{(1)}$ & 20.2 & -45.3 & 100 & 5.8883\\ 
211027306 & 03 48 04.97 & +23 24 13.8 & 18.09 & 14.02 & 19.7$\pm$2.69 & -52.56$\pm$2.69 & 6.0$\pm$0.8$^{(1)}$ & 19.9 & -45.4 & 100 & 0.238\\ 
211027393 & 03 46 04.12 & +23 24 19.9 & 12.28 & 9.84 & 18.77$\pm$2.3 & -51.91$\pm$2.3 & 9.7$\pm$1.3$^{(1)}$ & 20.1 & -45.3 & 99 & 0.5785\\ 
211027607 & 03 44 58.01 & +23 24 31.3 & 16.15 & 12.39 & 17.68$\pm$2.1 & -50.15$\pm$2.1 & 8.5$\pm$1.2$^{(1)}$ & 20.2 & -45.3 & 100 & 0.7571\\ 
211027758 & 03 49 32.56 & +23 24 41.3 & 16.21 & 12.32 & 24.36$\pm$2.08 & -53.7$\pm$2.08 & 10.4$\pm$1.4$^{(1)}$ & 19.7 & -45.4 & 95 & 0.3933\\ 
211027775 & 03 46 35.33 & +23 24 42.2 & 13.93 & 10.74 & 19.38$\pm$2.1 & -50.93$\pm$2.1 & 8.0$\pm$1.1$^{(1)}$ & 20.0 & -45.3 & 100 & 0.7424\\ 
211027879 & 03 48 48.78 & +23 24 48.4 & 17.18 & 13.2 & 21.43$\pm$2.55 & -53.39$\pm$2.55 & 8.5$\pm$1.2$^{(1)}$ & 19.8 & -45.4 & 100 & 0.374\\ 
211028100 & 03 45 08.40 & +23 25 01.2 & 17.62 & 13.47 & 18.21$\pm$2.1 & -53.29$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.2 & -45.3 & 100 & $<$2\\ 
211028209 & 03 40 50.44 & +23 25 06.5 & 10.59 & 9.12 & 22.07$\pm$0.82 & -45.52$\pm$0.42 & 7.7$\pm$0.3$^{(0)}$ & 20.7 & -45.1 & 100 & 4.395\\ 
211028311 & 03 46 34.15 & +23 25 12.5 & 18.34 & 14.01 & 20.22$\pm$2.6 & -34.51$\pm$2.6 & 5.7$\pm$0.8$^{(1)}$ & 20.0 & -45.3 & 80 &  \\ 
211028385 & 03 48 20.82 & +23 25 16.5 &   & 5.56 & 17.99$\pm$0.39 & -46.57$\pm$0.32 & 8.4$\pm$0.4$^{(0)}$ & 19.8 & -45.4 & 100 &  \\ 
211029076 & 03 47 09.51 & +23 25 56.6 & 16.88 & 13.09 & 20.13$\pm$2.08 & -50.4$\pm$2.08 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -45.3 & 100 & 0.4739\\ 
211029135 & 03 32 37.81 & +23 25 59.3 & 17.01 & 13.06 & 20.04$\pm$2.08 & -49.74$\pm$2.08 & 7.7$\pm$1.1$^{(1)}$ & 21.6 & -44.8 & 100 & 0.286\\ 
211029232 & 03 48 34.51 & +23 26 05.2 & 10.16 & 8.87 & 20.36$\pm$0.9 & -46.76$\pm$0.87 & 6.8$\pm$0.9$^{(1)}$ & 19.8 & -45.4 & 100 & 2.885\\ 
211029245 & 03 48 15.24 & +23 26 05.7 & 16.24 & 12.55 & 15.89$\pm$2.69 & -49.66$\pm$2.69 & 7.6$\pm$1.1$^{(1)}$ & 19.8 & -45.4 & 100 & 0.6994\\ 
211029254 & 03 47 15.37 & +23 26 06.2 & 16.36 & 12.55 & 23.2$\pm$2.08 & -52.58$\pm$2.08 & 8.6$\pm$1.2$^{(1)}$ & 19.9 & -45.3 & 100 & 0.8818\\ 
211029446 & 04 00 26.14 & +23 26 17.7 & 15.87 & 11.96 & 15.54$\pm$2.08 & -48.43$\pm$2.08 & 12.7$\pm$1.8$^{(1)}$ & 18.4 & -45.8 & 90 & 0.4124\\ 
211029507 & 03 35 18.75 & +23 26 21.1 & 18.22 & 13.98 & 22.08$\pm$2.55 & -46.39$\pm$2.55 & 6.8$\pm$0.9$^{(1)}$ & 21.3 & -44.9 & 100 &  \\ 
211029542 & 04 00 16.92 & +23 26 23.1 & 15.94 & 12.32 & 15.51$\pm$2.58 & -57.33$\pm$2.58 & 6.3$\pm$0.9$^{(1)}$ & 18.4 & -45.8 & 85 &  \\ 
211029757 & 03 40 39.45 & +23 26 35.1 & 18.43 & 14.04 & 24.89$\pm$2.59 & -48.35$\pm$2.59 & 6.8$\pm$0.9$^{(1)}$ & 20.7 & -45.1 & 100 & 0.3274\\ 
211030057 & 03 47 28.10 & +23 26 53.6 & 15.54 & 11.92 & 21.64$\pm$2.08 & -50.76$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 100 & 0.5572\\ 
211030074 & 04 00 40.24 & +23 26 54.3 & 16.8 & 12.79 & 19.72$\pm$2.08 & -50.7$\pm$2.08 & 9.7$\pm$1.3$^{(1)}$ & 18.4 & -45.8 & 99 & 0.1296\\ 
211030439 & 03 43 36.60 & +23 27 14.2 & 13.69 & 10.74 & 22.03$\pm$2.1 & -46.51$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 20.4 & -45.2 & 100 & 3.0502\\ 
211030481 & 03 49 34.91 & +23 27 16.9 & 13.41 & 10.38 & 18.63$\pm$2.08 & -52.98$\pm$2.08 & 9.2$\pm$1.3$^{(1)}$ & 19.7 & -45.4 & 99 & 1.2809\\ 
211030680 & 03 41 53.65 & +23 27 28.8 & 13.27 & 10.3 & 19.11$\pm$2.1 & -50.55$\pm$2.1 & 9.0$\pm$1.2$^{(1)}$ & 20.6 & -45.2 & 100 & 7.1503\\ 
211030912 & 03 48 22.69 & +23 27 43.1 & 16.68 & 12.77 & 19.81$\pm$2.55 & -47.22$\pm$2.55 & 9.2$\pm$1.3$^{(1)}$ & 19.8 & -45.4 & 100 & 0.293\\ 
211031100 & 03 47 55.59 & +23 27 54.1 & 11.16 & 9.4 & 12.85$\pm$0.9 & -44.99$\pm$0.83 & 9.1$\pm$1.3$^{(1)}$ & 19.9 & -45.4 & 86 &  \\ 
211031105 & 03 45 52.75 & +23 27 54.3 & 16.1 & 12.31 & 21.68$\pm$2.1 & -49.56$\pm$2.1 & 8.3$\pm$1.1$^{(1)}$ & 20.1 & -45.3 & 100 & 0.6841\\ 
211031293 & 03 47 38.01 & +23 28 04.9 & 12.99 & 10.41 & 22.35$\pm$2.08 & -50.62$\pm$2.08 & 7.4$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 100 & 8.4106\\ 
211031520 & 03 45 22.19 & +23 28 18.2 & 12.08 & 9.85 & 18.88$\pm$2.3 & -49.52$\pm$2.3 & 8.9$\pm$1.2$^{(1)}$ & 20.2 & -45.3 & 100 & 8.4849\\ 
211031682 & 03 47 36.03 & +23 28 27.0 & 17.23 & 13.35 & 20.02$\pm$2.08 & -56.27$\pm$2.08 & 7.0$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 97 & 0.2819\\ 
211032220 & 04 05 09.43 & +23 28 58.8 & 12.01 & 10.35 & 12.94$\pm$2.6 & -46.32$\pm$0.38 & 5.2$\pm$0.6$^{(0)}$ & 17.8 & -45.9 & 80 &  \\ 
211032382 & 03 46 22.46 & +23 29 08.3 & 17.05 & 12.83 & 24.76$\pm$2.1 & -48.69$\pm$2.1 & 10.3$\pm$1.4$^{(1)}$ & 20.0 & -45.3 & 99 & 0.3797\\ 
211032476 & 03 41 22.97 & +23 29 13.0 & 9.04 & 8.09 & 21.51$\pm$0.11 & -45.25$\pm$0.07 & 7.8$\pm$0.2$^{(0)}$ & 20.6 & -45.1 & 100 & $<$2\\ 
211032994 & 03 47 01.42 & +23 29 42.0 & 11.21 & 9.53 & 19.68$\pm$0.89 & -45.29$\pm$0.49 & 7.5$\pm$0.3$^{(0)}$ & 20.0 & -45.4 & 100 & 5.9306\\ 
211033155 & 03 46 40.24 & +23 29 51.9 & 11.84 & 9.34 & 18.6$\pm$2.3 & -48.69$\pm$2.3 & 12.7$\pm$1.8$^{(1)}$ & 20.0 & -45.3 & 98 & 0.5243\\ 
211033487 & 03 44 36.28 & +23 30 11.1 & 15.2 & 11.68 & 19.91$\pm$2.1 & -48.84$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.3 & -45.3 & 100 & 1.6598\\ 
211033726 & 03 48 10.98 & +23 30 25.2 & 13.57 & 10.7 & 16.97$\pm$2.12 & -47.35$\pm$2.12 & 7.3$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 8.1854\\ 
211033935 & 04 02 49.96 & +23 30 38.9 & 15.6 & 12.06 & 16.16$\pm$2.1 & -45.12$\pm$2.1 & 6.5$\pm$0.9$^{(1)}$ & 18.1 & -45.9 & 100 & 1.1256\\ 
211034329 & 03 45 13.41 & +23 31 00.9 & 15.99 & 11.91 & 17.01$\pm$2.1 & -51.75$\pm$2.1 & 13.8$\pm$1.9$^{(1)}$ & 20.2 & -45.3 & 72 & 0.3403\\ 
211034343 & 03 48 20.58 & +23 31 01.7 & 17.59 & 13.53 & 16.46$\pm$2.83 & -51.3$\pm$2.64 & 7.2$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 0.2571\\ 
211034737 & 04 16 30.83 & +23 31 25.3 & 12.59 & 10.17 & 17.46$\pm$2.06 & -43.74$\pm$2.06 & 8.3$\pm$1.1$^{(1)}$ & 16.4 & -46.3 & 84 &  \\ 
211035145 & 03 34 58.66 & +23 31 48.6 & 8.76 & 7.96 & 20.87$\pm$0.58 & -42.81$\pm$0.44 & 7.4$\pm$0.4$^{(0)}$ & 21.3 & -44.9 & 100 & $<$2\\ 
211035282 & 03 46 50.08 & +23 31 56.4 & 16.11 & 12.38 & 22.28$\pm$2.1 & -51.66$\pm$2.1 & 8.6$\pm$1.2$^{(1)}$ & 20.0 & -45.3 & 100 & 2.1377\\ 
211035702 & 03 43 48.60 & +23 32 21.8 & 13.28 & 10.59 & 19.44$\pm$2.1 & -47.35$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 20.3 & -45.2 & 100 & 9.4558\\ 
211035936 & 03 47 02.34 & +23 32 36.3 & 17.72 & 13.29 & 26.79$\pm$2.6 & -50.68$\pm$2.6 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -45.4 & 98 & 2.5738\\ 
211035968 & 03 44 00.58 & +23 32 38.1 & 10.77 & 9.2 & 19.34$\pm$0.8 & -44.83$\pm$0.39 & 7.4$\pm$0.3$^{(0)}$ & 20.3 & -45.3 & 100 & 4.02\\ 
211036360 & 03 40 31.49 & +23 33 02.3 & 14.25 & 11.06 & 23.22$\pm$2.1 & -49.03$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.7 & -45.1 & 100 & 2.337\\ 
211036390 & 03 40 29.59 & +23 33 04.0 & 13.56 & 10.82 & 20.46$\pm$2.1 & -40.67$\pm$2.1 & 6.1$\pm$0.8$^{(1)}$ & 20.7 & -45.1 & 100 & 10.317\\ 
211036595 & 03 47 29.92 & +23 33 15.2 & 18.11 & 13.74 & 21.99$\pm$2.08 & -47.37$\pm$2.08 & 7.7$\pm$1.1$^{(1)}$ & 19.9 & -45.4 & 100 & 0.3079\\ 
211036655 & 04 09 17.46 & +23 33 18.0 & 12.82 & 10.48 & 10.42$\pm$2.08 & -45.05$\pm$2.08 & 7.0$\pm$1.0$^{(1)}$ & 17.3 & -46.1 & 88 &  \\ 
211036665 & 03 49 11.28 & +23 33 18.9 & 13.5 & 10.61 & 19.65$\pm$2.08 & -48.64$\pm$2.08 & 7.4$\pm$1.0$^{(1)}$ & 19.7 & -45.4 & 100 & 1.4162\\ 
211036881 & 03 51 54.51 & +23 33 31.7 & 15.63 & 11.78 & 20.25$\pm$2.08 & -53.03$\pm$2.08 & 12.4$\pm$1.7$^{(1)}$ & 19.4 & -45.5 & 90 & 0.5778\\ 
211037012 & 03 46 58.16 & +23 33 39.1 & 16.53 & 12.86 & 24.42$\pm$2.1 & -55.47$\pm$2.1 & 6.3$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 97 & 0.9133\\ 
211037018 & 03 44 20.87 & +23 33 39.3 & 15.61 & 11.99 & 19.59$\pm$2.1 & -51.16$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.3 & -45.3 & 100 & 4.4526\\ 
211037397 & 03 32 42.30 & +23 34 00.5 & 16.47 & 12.54 & 20.11$\pm$2.46 & -49.29$\pm$2.18 & 9.5$\pm$1.3$^{(1)}$ & 21.6 & -44.8 & 99 & 0.499\\ 
211037417 & 03 45 16.41 & +23 34 01.9 & 17.64 & 13.48 & 24.05$\pm$2.1 & -51.59$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.2 & -45.3 & 100 & 0.1903\\ 
211038095 & 03 44 35.89 & +23 34 42.2 & 18.44 & 13.93 & 19.46$\pm$2.6 & -47.82$\pm$2.6 & 6.9$\pm$0.9$^{(1)}$ & 20.3 & -45.3 & 100 &  \\ 
211038138 & 04 01 05.79 & +23 34 44.3 & 15.94 & 12.33 & 26.8$\pm$2.08 & -44.97$\pm$2.08 & 7.3$\pm$1.0$^{(1)}$ & 18.3 & -45.8 & 94 &  \\ 
211038211 & 03 42 48.90 & +23 34 48.8 & 16.57 & 12.76 & 23.52$\pm$2.11 & -51.61$\pm$2.1 & 7.9$\pm$1.1$^{(1)}$ & 20.5 & -45.2 & 100 & 0.6804\\ 
211038222 & 03 51 51.54 & +23 34 49.5 & 17.42 & 13.39 & 22.88$\pm$2.58 & -49.73$\pm$2.58 & 7.0$\pm$1.0$^{(1)}$ & 19.4 & -45.5 & 100 & 0.8344\\ 
211038382 & 03 51 03.27 & +23 35 00.5 & 17.36 & 13.4 & 19.0$\pm$2.51 & -47.72$\pm$2.51 & 7.3$\pm$1.0$^{(1)}$ & 19.5 & -45.5 & 100 & 1.6572\\ 
211038389 & 03 46 53.74 & +23 35 00.8 & 10.33 & 9.0 & 21.85$\pm$1.95 & -44.28$\pm$0.33 & 7.2$\pm$0.5$^{(0)}$ & 20.0 & -45.4 & 100 & 3.5941\\ 
211038588 & 03 46 12.66 & +23 35 13.9 & 16.92 & 13.01 & 23.08$\pm$2.1 & -53.9$\pm$2.1 & 8.4$\pm$1.2$^{(1)}$ & 20.1 & -45.3 & 99 & 0.5507\\ 
211038622 & 03 48 16.08 & +23 35 15.6 & 16.95 & 12.72 & 15.83$\pm$2.12 & -51.13$\pm$2.12 & 13.3$\pm$1.8$^{(1)}$ & 19.8 & -45.4 & 79 & 0.3949\\ 
211038660 & 03 42 08.84 & +23 35 17.1 & 14.62 & 11.27 & 19.63$\pm$2.1 & -48.8$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 20.5 & -45.2 & 100 & 3.0135\\ 
211038810 & 03 44 31.71 & +23 35 26.3 & 15.89 & 12.18 & 20.59$\pm$2.1 & -50.94$\pm$2.1 & 8.1$\pm$1.1$^{(1)}$ & 20.3 & -45.3 & 100 & 0.9184\\ 
211038945 & 03 46 27.77 & +23 35 33.8 & 12.43 & 9.82 & 16.1$\pm$2.3 & -49.87$\pm$2.3 & 9.9$\pm$1.4$^{(1)}$ & 20.0 & -45.3 & 99 & 5.343\\ 
211039307 & 03 40 51.27 & +23 35 54.3 & 12.33 & 10.08 & 20.32$\pm$2.1 & -47.59$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 20.7 & -45.1 & 100 & 8.3247\\ 
211039634 & 03 48 19.82 & +23 36 12.0 & 14.87 & 11.51 & 17.75$\pm$2.12 & -49.74$\pm$2.12 & 7.3$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 1.033\\ 
211039833 & 04 16 59.51 & +23 36 23.6 & 12.12 & 9.95 & 15.24$\pm$2.31 & -38.67$\pm$2.31 & 8.6$\pm$1.2$^{(1)}$ & 16.3 & -46.3 & 15 &  \\ 
211039840 & 03 44 56.68 & +23 36 23.8 & 16.01 & 12.28 & 21.72$\pm$2.1 & -51.52$\pm$2.1 & 8.1$\pm$1.1$^{(1)}$ & 20.2 & -45.3 & 100 & 0.8002\\ 
211040347 & 03 45 06.79 & +23 36 51.7 & 16.81 & 12.67 & 14.25$\pm$2.1 & -47.31$\pm$2.1 & 11.1$\pm$1.5$^{(1)}$ & 20.2 & -45.3 & 96 & 0.3337\\ 
211040850 & 03 46 43.18 & +23 37 22.2 & 17.21 & 13.11 & 18.97$\pm$2.75 & -51.03$\pm$2.75 & 8.3$\pm$1.1$^{(1)}$ & 20.0 & -45.4 & 100 & 0.5017\\ 
211040918 & 03 46 34.20 & +23 37 26.5 & 8.01 & 7.07 & 21.34$\pm$0.56 & -42.79$\pm$0.41 & 7.8$\pm$0.3$^{(0)}$ & 20.0 & -45.4 & 100 &  \\ 
211041420 & 03 45 27.51 & +23 37 57.3 & 17.13 & 13.27 & 18.22$\pm$2.1 & -52.57$\pm$2.1 & 6.5$\pm$0.9$^{(1)}$ & 20.2 & -45.3 & 100 & 0.2958\\ 
211041474 & 03 48 13.77 & +23 37 59.6 & 15.76 & 12.12 & 20.24$\pm$2.08 & -51.0$\pm$2.08 & 7.7$\pm$1.1$^{(1)}$ & 19.8 & -45.4 & 100 & 1.8306\\ 
211041526 & 03 47 26.76 & +23 38 02.7 & 16.16 & 12.28 & 22.0$\pm$2.08 & -48.55$\pm$2.08 & 10.8$\pm$1.5$^{(1)}$ & 19.9 & -45.4 & 100 & 0.4291\\ 
211041682 & 03 54 22.47 & +23 38 12.2 & 16.3 & 12.57 & 21.95$\pm$2.08 & -47.92$\pm$2.08 & 7.2$\pm$1.0$^{(1)}$ & 19.1 & -45.6 & 100 & 1.545\\ 
211041683 & 03 48 16.90 & +23 38 12.4 & 9.95 & 8.74 & 18.26$\pm$1.1 & -48.4$\pm$0.96 & 6.5$\pm$0.9$^{(1)}$ & 19.8 & -45.4 & 100 & 2.4534\\ 
211041750 & 03 49 01.14 & +23 38 15.8 & 17.65 & 13.57 & 18.27$\pm$2.55 & -50.57$\pm$2.55 & 6.7$\pm$0.9$^{(1)}$ & 19.7 & -45.4 & 100 & 0.3242\\ 
211041753 & 03 41 34.79 & +23 38 15.8 & 17.11 & 13.19 & 20.2$\pm$2.1 & -48.5$\pm$2.1 & 6.6$\pm$0.9$^{(1)}$ & 20.6 & -45.2 & 100 & 0.5168\\ 
211042045 & 03 43 37.10 & +23 38 32.3 & 15.74 & 11.88 & 18.63$\pm$2.1 & -46.65$\pm$2.1 & 11.5$\pm$1.6$^{(1)}$ & 20.4 & -45.3 & 99 & 0.366\\ 
211042246 & 03 46 52.60 & +23 38 43.4 & 16.32 & 12.21 & 17.33$\pm$2.19 & -50.23$\pm$2.19 & 12.3$\pm$1.7$^{(1)}$ & 20.0 & -45.4 & 97 & 0.0824\\ 
211042471 & 03 49 29.80 & +23 38 55.6 & 16.6 & 12.66 & 21.9$\pm$2.05 & -47.41$\pm$2.05 & 9.9$\pm$1.4$^{(1)}$ & 19.7 & -45.5 & 100 & 0.37\\ 
211042656 & 03 49 21.48 & +23 39 06.6 & 15.59 & 12.02 & 17.1$\pm$2.08 & -51.55$\pm$2.08 & 8.4$\pm$1.2$^{(1)}$ & 19.7 & -45.5 & 100 & 0.3389\\ 
211043259 & 03 48 11.19 & +23 39 44.0 & 15.51 & 11.9 & 14.64$\pm$2.08 & -42.58$\pm$2.08 & 8.9$\pm$1.2$^{(1)}$ & 19.8 & -45.4 & 100 &  \\ 
211043323 & 03 47 51.95 & +23 39 48.3 & 16.89 & 13.03 & 21.16$\pm$2.55 & -48.08$\pm$2.55 & 7.4$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 100 & 0.94\\ 
211043986 & 03 43 31.95 & +23 40 26.5 & 10.57 & 9.1 & 19.35$\pm$2.45 & -43.56$\pm$0.57 & 7.0$\pm$0.8$^{(0)}$ & 20.4 & -45.3 & 100 & 3.9906\\ 
211044267 & 03 47 26.83 & +23 40 42.0 & 7.75 & 7.34 & 22.17$\pm$0.44 & -45.04$\pm$0.34 & 7.4$\pm$0.3$^{(0)}$ & 19.9 & -45.4 & 100 & 0.0587\\ 
211044536 & 03 40 34.36 & +23 40 57.4 & 10.63 & 9.15 & 27.01$\pm$2.32 & -45.23$\pm$0.58 & 5.7$\pm$0.6$^{(0)}$ & 20.7 & -45.2 & 98 & 4.5487\\ 
211044929 & 03 49 31.21 & +23 41 19.9 & 16.63 & 12.77 & 18.57$\pm$2.08 & -48.11$\pm$2.08 & 8.5$\pm$1.2$^{(1)}$ & 19.7 & -45.5 & 100 & 0.3013\\ 
211045147 & 03 43 39.72 & +23 41 32.7 & 17.69 & 13.57 & 21.61$\pm$2.1 & -53.87$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 20.4 & -45.3 & 100 & 0.294\\ 
211045153 & 03 47 33.46 & +23 41 33.1 & 14.41 & 10.9 & 18.93$\pm$2.08 & -49.89$\pm$2.08 & 11.5$\pm$1.6$^{(1)}$ & 19.9 & -45.4 & 99 & 0.4226\\ 
211045643 & 03 47 44.65 & +23 42 03.4 & 16.48 & 12.69 & 20.46$\pm$2.08 & -51.48$\pm$2.08 & 8.6$\pm$1.2$^{(1)}$ & 19.9 & -45.4 & 100 & 0.4458\\ 
211045648 & 03 48 15.26 & +23 42 03.6 & 15.51 & 11.8 & 17.07$\pm$2.12 & -47.73$\pm$2.12 & 10.4$\pm$1.4$^{(1)}$ & 19.8 & -45.4 & 100 & 0.367\\ 
211045933 & 03 49 50.36 & +23 42 20.2 & 11.3 & 9.6 & 19.68$\pm$0.92 & -47.98$\pm$0.92 & 6.8$\pm$0.9$^{(1)}$ & 19.6 & -45.5 & 100 & 6.8472\\ 
211046046 & 03 41 58.68 & +23 42 26.4 & 13.81 & 10.84 & 18.27$\pm$2.1 & -48.1$\pm$2.1 & 6.6$\pm$0.9$^{(1)}$ & 20.6 & -45.2 & 100 & 7.7833\\ 
211046102 & 03 41 27.82 & +23 42 29.9 & 10.89 & 9.31 & 20.09$\pm$0.75 & -45.57$\pm$0.37 & 7.7$\pm$0.2$^{(0)}$ & 20.6 & -45.2 & 100 & 5.4678\\ 
211046168 & 03 49 58.34 & +23 42 34.0 & 14.98 & 11.6 & 14.08$\pm$2.06 & -55.85$\pm$2.06 & 6.6$\pm$0.9$^{(1)}$ & 19.6 & -45.5 & 77 & 1.3418\\ 
211046240 & 03 47 08.54 & +23 42 38.9 & 12.74 & 9.9 & 15.91$\pm$2.34 & -55.32$\pm$2.34 & 10.0$\pm$1.4$^{(1)}$ & 20.0 & -45.4 & 85 & 1.616\\ 
211046293 & 03 49 43.53 & +23 42 42.7 & 6.2 & 6.22 & 18.01$\pm$0.04 & -45.6$\pm$0.02 & 7.9$\pm$0.5$^{(0)}$ & 19.7 & -45.5 & 100 & 0.1765\\ 
211046315 & 03 49 28.74 & +23 42 43.9 & 11.13 & 9.43 & 19.67$\pm$0.77 & -49.13$\pm$0.77 & 7.2$\pm$1.0$^{(1)}$ & 19.7 & -45.5 & 100 & 5.7139\\ 
211046446 & 03 47 13.53 & +23 42 51.5 & 12.09 & 10.01 & 17.56$\pm$2.12 & -49.88$\pm$2.12 & 6.9$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 100 & 7.8496\\ 
211046494 & 03 47 06.78 & +23 42 54.6 & 11.89 & 9.84 & 17.81$\pm$2.34 & -55.11$\pm$2.34 & 7.5$\pm$1.0$^{(1)}$ & 20.0 & -45.4 & 99 & 8.4781\\ 
211046826 & 04 03 49.56 & +23 43 14.2 & 16.81 & 13.0 & 18.51$\pm$2.08 & -48.83$\pm$2.08 & 6.9$\pm$1.0$^{(1)}$ & 18.0 & -45.9 & 100 & 0.3081\\ 
211046948 & 03 41 02.98 & +23 43 21.7 & 15.6 & 12.0 & 20.82$\pm$2.1 & -49.02$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 20.7 & -45.2 & 100 & 1.4556\\ 
211047055 & 03 49 57.63 & +23 43 28.5 & 17.48 & 13.38 & 19.44$\pm$2.55 & -50.69$\pm$2.55 & 8.0$\pm$1.1$^{(1)}$ & 19.6 & -45.5 & 100 & 0.3019\\ 
211047412 & 03 45 37.75 & +23 43 50.3 & 18.5 & 13.72 & 10.16$\pm$2.87 & -57.52$\pm$2.98 & 8.9$\pm$1.2$^{(1)}$ & 20.1 & -45.3 & 15 &  \\ 
211047687 & 03 43 39.03 & +23 44 05.5 & 16.21 & 12.25 & 18.15$\pm$2.1 & -52.14$\pm$2.1 & 11.5$\pm$1.6$^{(1)}$ & 20.4 & -45.3 & 96 & 0.3049\\ 
211047718 & 03 47 22.68 & +23 44 07.1 & 16.17 & 12.44 & 19.48$\pm$2.12 & -49.65$\pm$2.12 & 8.7$\pm$1.2$^{(1)}$ & 19.9 & -45.4 & 100 & 0.6801\\ 
211047828 & 03 46 02.76 & +23 44 14.6 & 11.97 & 9.26 & 17.73$\pm$3.18 & -43.46$\pm$3.18 & 14.7$\pm$2.0$^{(1)}$ & 20.1 & -45.4 & 88 & 3.9585\\ 
211047980 & 03 49 05.85 & +23 44 23.3 & 14.37 & 10.76 & 18.56$\pm$2.08 & -46.41$\pm$2.08 & 13.5$\pm$1.9$^{(1)}$ & 19.7 & -45.5 & 98 & 0.8288\\ 
211047990 & 03 48 07.96 & +23 44 23.8 & 15.83 & 12.18 & 17.52$\pm$2.12 & -49.49$\pm$2.12 & 8.2$\pm$1.1$^{(1)}$ & 19.8 & -45.4 & 100 & 0.5148\\ 
211048014 & 03 47 41.18 & +23 44 25.1 & 13.21 & 10.56 & 20.4$\pm$2.12 & -49.09$\pm$2.12 & 7.0$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 100 & 0.7814\\ 
211048116 & 03 53 47.58 & +23 44 31.1 & 16.06 & 12.28 & 16.65$\pm$2.08 & -50.32$\pm$2.08 & 8.9$\pm$1.2$^{(1)}$ & 19.2 & -45.6 & 100 & 0.6775\\ 
211048126 & 03 47 09.44 & +23 44 32.0 & 14.0 & 10.69 & 20.22$\pm$2.12 & -48.44$\pm$2.12 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -45.4 & 100 & 0.8446\\ 
211048321 & 03 51 11.87 & +23 44 43.5 & 17.34 & 13.44 & 19.81$\pm$2.63 & -49.91$\pm$2.63 & 6.2$\pm$0.9$^{(1)}$ & 19.5 & -45.5 & 100 & 1.9607\\ 
211049179 & 03 47 05.78 & +23 45 35.0 & 18.29 & 14.15 & 27.34$\pm$2.83 & -50.88$\pm$2.83 & 6.8$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 100 &  \\ 
211049322 & 03 43 34.39 & +23 45 42.8 & 11.12 & 9.37 & 24.76$\pm$1.31 & -47.21$\pm$0.69 & 7.3$\pm$0.4$^{(0)}$ & 20.4 & -45.3 & 100 & 5.4442\\ 
211049396 & 03 41 39.58 & +23 45 47.1 & 13.71 & 10.87 & 22.94$\pm$2.1 & -49.49$\pm$2.1 & 6.3$\pm$0.9$^{(1)}$ & 20.6 & -45.2 & 100 & 11.0063\\ 
211049486 & 03 39 50.67 & +23 45 52.7 & 17.62 & 13.5 & 21.47$\pm$2.59 & -48.58$\pm$2.59 & 6.9$\pm$1.0$^{(1)}$ & 20.8 & -45.1 & 100 & 0.5572\\ 
211049716 & 03 37 31.07 & +23 46 07.5 & 17.44 & 13.48 & 18.9$\pm$2.65 & -49.43$\pm$2.65 & 6.2$\pm$0.9$^{(1)}$ & 21.1 & -45.1 & 100 & $<$2\\ 
211049922 & 03 55 29.01 & +23 46 20.8 & 13.36 & 10.59 & 17.11$\pm$1.25 & -45.43$\pm$1.25 & 7.0$\pm$1.0$^{(1)}$ & 19.0 & -45.7 & 100 & 3.0184\\ 
211050460 & 03 49 06.11 & +23 46 52.5 & 10.34 & 8.6 & 17.43$\pm$1.35 & -44.78$\pm$1.35 & 9.7$\pm$1.3$^{(1)}$ & 19.7 & -45.5 & 100 & 0.7768\\ 
211050553 & 03 46 40.01 & +23 46 58.7 & 15.92 & 12.03 & 22.06$\pm$2.24 & -44.5$\pm$2.24 & 10.7$\pm$1.5$^{(1)}$ & 20.0 & -45.4 & 100 & $<$2\\ 
211050613 & 03 56 26.20 & +23 47 03.6 & 11.05 & 9.39 & 22.52$\pm$1.35 & -41.65$\pm$0.55 & 6.6$\pm$0.2$^{(0)}$ & 18.9 & -45.7 & 99 &  \\ 
211050629 & 04 05 14.31 & +23 47 04.4 & 12.32 & 9.54 & 17.56$\pm$2.28 & -44.62$\pm$2.28 & 11.3$\pm$1.6$^{(1)}$ & 17.8 & -46.0 & 95 &  \\ 
211050847 & 03 46 37.67 & +23 47 15.9 & 10.0 & 8.53 & 19.65$\pm$0.73 & -47.11$\pm$0.44 & 7.7$\pm$0.2$^{(0)}$ & 20.0 & -45.4 & 100 & 6.1624\\ 
211051330 & 03 49 33.12 & +23 47 43.4 & 10.69 & 9.21 & 19.85$\pm$0.77 & -45.5$\pm$0.77 & 7.1$\pm$1.0$^{(1)}$ & 19.7 & -45.5 & 100 & 4.9432\\ 
211051561 & 03 35 16.26 & +23 47 58.2 & 17.21 & 13.18 & 27.8$\pm$2.12 & -49.0$\pm$2.12 & 8.2$\pm$1.1$^{(1)}$ & 21.3 & -45.0 & 99 & 0.4725\\ 
211051770 & 03 47 20.97 & +23 48 12.0 & 7.03 & 6.9 & 19.08$\pm$0.05 & -45.46$\pm$0.03 & 7.2$\pm$0.4$^{(0)}$ & 19.9 & -45.4 & 100 &  \\ 
211051975 & 03 36 11.06 & +23 48 23.5 & 17.07 & 13.08 & 19.69$\pm$2.55 & -51.37$\pm$2.55 & 7.9$\pm$1.1$^{(1)}$ & 21.2 & -45.0 & 100 & 0.549\\ 
211051985 & 03 48 17.36 & +23 48 23.9 & 16.57 & 12.78 & 15.75$\pm$2.62 & -48.27$\pm$2.62 & 7.3$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 0.4915\\ 
211052320 & 04 10 03.81 & +23 48 44.0 & 14.01 & 10.92 & 15.4$\pm$2.15 & -43.5$\pm$2.15 & 7.1$\pm$1.0$^{(1)}$ & 17.2 & -46.2 & 99 & 6.7602\\ 
211052343 & 03 46 27.69 & +23 48 45.7 & 16.96 & 12.63 & 20.71$\pm$2.75 & -46.14$\pm$2.75 & 10.9$\pm$1.5$^{(1)}$ & 20.0 & -45.4 & 100 & 2.3468\\ 
211052416 & 03 50 12.59 & +23 48 49.1 & 17.61 & 13.54 & 16.43$\pm$2.56 & -50.84$\pm$2.55 & 6.5$\pm$0.9$^{(1)}$ & 19.6 & -45.5 & 100 &  \\ 
211052796 & 03 53 48.05 & +23 49 09.9 & 17.83 & 13.51 & 18.48$\pm$2.58 & -51.49$\pm$2.58 & 9.0$\pm$1.3$^{(1)}$ & 19.2 & -45.6 & 100 &  \\ 
211053031 & 03 42 45.64 & +23 49 22.9 & 17.51 & 13.39 & 23.55$\pm$2.59 & -47.03$\pm$2.59 & 7.9$\pm$1.1$^{(1)}$ & 20.5 & -45.3 & 100 & 0.3519\\ 
211053255 & 03 51 16.85 & +23 49 35.7 & 11.98 & 9.96 & 20.27$\pm$0.83 & -47.4$\pm$0.45 & 7.3$\pm$0.3$^{(0)}$ & 19.5 & -45.6 & 100 & 7.9471\\ 
211053549 & 03 47 13.66 & +23 49 53.5 & 14.57 & 11.09 & 19.28$\pm$2.18 & -50.46$\pm$2.18 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -45.4 & 100 & 0.5326\\ 
211053678 & 03 43 16.59 & +23 50 01.8 & 16.22 & 12.39 & 21.55$\pm$2.1 & -52.4$\pm$2.1 & 8.9$\pm$1.2$^{(1)}$ & 20.4 & -45.3 & 100 & 0.7703\\ 
211053737 & 03 50 54.33 & +23 50 05.5 & 11.02 & 9.05 & 18.64$\pm$0.89 & -50.14$\pm$0.85 & 9.2$\pm$1.3$^{(1)}$ & 19.5 & -45.5 & 100 & 6.6498\\ 
211053776 & 03 54 27.96 & +23 50 07.3 & 12.38 & 9.66 & 17.1$\pm$2.28 & -53.27$\pm$2.28 & 10.6$\pm$1.5$^{(1)}$ & 19.1 & -45.7 & 96 & 3.0576\\ 
211053922 & 03 41 05.22 & +23 50 15.3 & 17.82 & 13.76 & 24.62$\pm$2.59 & -51.13$\pm$2.59 & 6.7$\pm$0.9$^{(1)}$ & 20.7 & -45.2 & 100 & 0.3446\\ 
211054014 & 03 49 24.05 & +23 50 21.3 & 11.05 & 9.38 & 19.21$\pm$0.77 & -46.7$\pm$0.85 & 7.2$\pm$1.0$^{(1)}$ & 19.7 & -45.5 & 100 & 5.5927\\ 
211054027 & 03 45 03.28 & +23 50 21.8 & 11.6 & 9.73 & 20.19$\pm$1.15 & -45.6$\pm$0.63 & 7.5$\pm$0.3$^{(0)}$ & 20.2 & -45.3 & 100 & 7.0949\\ 
211054508 & 03 49 57.45 & +23 50 49.5 & 10.14 & 8.5 & 22.39$\pm$1.15 & -47.59$\pm$1.15 & 11.2$\pm$1.5$^{(1)}$ & 19.6 & -45.5 & 100 &  \\ 
211054599 & 03 49 58.05 & +23 50 55.3 & 6.83 & 6.51 & 18.87$\pm$0.05 & -45.98$\pm$0.03 & 7.2$\pm$0.4$^{(0)}$ & 19.6 & -45.5 & 100 & 1.6412\\ 
211054634 & 03 39 47.96 & +23 50 57.2 & 15.54 & 11.83 & 19.61$\pm$2.15 & -48.66$\pm$2.15 & 10.9$\pm$1.5$^{(1)}$ & 20.8 & -45.1 & 99 & 0.3847\\ 
211055134 & 03 43 23.25 & +23 51 25.7 & 14.62 & 11.32 & 9.98$\pm$2.1 & -45.87$\pm$2.1 & 6.6$\pm$0.9$^{(1)}$ & 20.4 & -45.3 & 83 &  \\ 
211055359 & 03 42 26.27 & +23 51 38.7 &   & 13.45 & 14.5$\pm$3.8 & -59.7$\pm$3.8 & 5.7$\pm$0.8$^{(4)}$ & 20.5 & -45.2 & 89 & 0.4958\\ 
211055424 & 03 41 19.34 & +23 51 42.2 & 16.72 & 12.78 & 20.89$\pm$2.1 & -47.88$\pm$2.1 & 8.8$\pm$1.2$^{(1)}$ & 20.6 & -45.2 & 100 & 0.4252\\ 
211055468 & 03 50 02.17 & +23 51 44.9 & 15.54 & 12.0 & 21.13$\pm$2.08 & -50.66$\pm$2.08 & 7.2$\pm$1.0$^{(1)}$ & 19.6 & -45.5 & 100 & 0.6757\\ 
211055493 & 03 44 01.67 & +23 51 46.3 & 16.23 & 12.03 & 18.25$\pm$2.1 & -40.68$\pm$2.1 & 18.4$\pm$2.5$^{(1)}$ & 20.3 & -45.3 & 28 & 0.7814\\ 
211055718 & 03 54 23.99 & +23 51 59.2 & 17.92 & 13.83 & 17.95$\pm$2.58 & -54.84$\pm$2.58 & 7.0$\pm$1.0$^{(1)}$ & 19.1 & -45.7 & 99 &  \\ 
211056099 & 03 47 31.64 & +23 52 19.4 & 16.69 & 12.81 & 19.5$\pm$2.19 & -53.18$\pm$2.19 & 8.3$\pm$1.1$^{(1)}$ & 19.9 & -45.4 & 100 & 0.4855\\ 
211056415 & 03 44 12.13 & +23 52 37.5 & 16.36 & 12.58 & 19.64$\pm$2.1 & -50.22$\pm$2.1 & 8.4$\pm$1.2$^{(1)}$ & 20.3 & -45.3 & 100 & 0.6063\\ 
211056608 & 03 47 00.36 & +23 52 48.3 & 17.29 & 13.1 & 14.64$\pm$2.91 & -48.67$\pm$2.91 & 9.3$\pm$1.3$^{(1)}$ & 20.0 & -45.4 & 100 &  \\ 
211056628 & 03 47 29.58 & +23 52 49.7 & 18.55 & 14.01 & 12.99$\pm$2.74 & -45.1$\pm$2.74 & 7.2$\pm$1.0$^{(1)}$ & 19.9 & -45.4 & 100 & 0.2768\\ 
211056809 & 03 43 58.80 & +23 52 57.8 & 9.5 & 8.31 & 22.73$\pm$2.25 & -45.66$\pm$0.53 & 6.8$\pm$0.6$^{(0)}$ & 20.3 & -45.3 & 100 & 2.3969\\ 
211056856 & 03 45 46.90 & +23 53 00.6 & 17.85 & 13.62 & 20.3$\pm$2.75 & -51.35$\pm$2.75 & 7.7$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 &  \\ 
211056865 & 03 48 05.86 & +23 53 01.1 & 17.21 & 13.27 & 15.64$\pm$2.12 & -41.71$\pm$2.12 & 7.5$\pm$1.0$^{(1)}$ & 19.8 & -45.4 & 100 & 0.5561\\ 
211057064 & 03 49 12.19 & +23 53 12.5 & 8.11 & 7.58 & 19.4$\pm$0.44 & -44.93$\pm$0.39 & 7.8$\pm$0.3$^{(0)}$ & 19.7 & -45.5 & 100 & 0.0559\\ 
211057320 & 03 48 17.12 & +23 53 25.3 & 10.19 & 8.89 & 16.21$\pm$0.9 & -48.84$\pm$0.9 & 6.2$\pm$0.9$^{(1)}$ & 19.8 & -45.5 & 100 & 3.8184\\ 
211057388 & 03 48 18.01 & +23 53 29.3 & 13.83 & 10.96 & 12.14$\pm$2.91 & -50.69$\pm$2.86 & 6.1$\pm$0.8$^{(1)}$ & 19.8 & -45.5 & 99 & 3.8161\\ 
211057696 & 03 44 19.68 & +23 53 45.9 & 17.98 & 13.31 & 21.47$\pm$2.75 & -49.81$\pm$2.75 & 10.9$\pm$1.5$^{(1)}$ & 20.3 & -45.3 & 99 & 0.3103\\ 
211057712 & 04 03 43.83 & +23 53 47.4 & 16.35 & 12.2 & 16.46$\pm$2.09 & -46.02$\pm$2.08 & 14.3$\pm$2.0$^{(1)}$ & 18.0 & -46.0 & 74 & 0.2775\\ 
211057850 & 03 58 01.96 & +23 53 54.9 & 17.01 & 13.07 & 19.17$\pm$2.58 & -51.8$\pm$2.58 & 8.3$\pm$1.2$^{(1)}$ & 18.7 & -45.8 & 100 & 0.3022\\ 
211058381 & 03 40 18.84 & +23 54 23.7 & 16.49 & 12.77 & 18.88$\pm$2.1 & -49.11$\pm$2.1 & 6.7$\pm$0.9$^{(1)}$ & 20.7 & -45.2 & 100 & 0.6702\\ 
211058468 & 03 39 42.71 & +23 54 27.9 & 16.13 & 12.41 & 18.87$\pm$2.1 & -49.4$\pm$2.1 & 8.2$\pm$1.1$^{(1)}$ & 20.8 & -45.2 & 100 & 0.7734\\ 
211059010 & 03 41 42.40 & +23 54 57.4 & 18.4 & 13.74 & 20.74$\pm$2.74 & -54.44$\pm$2.74 & 9.4$\pm$1.3$^{(1)}$ & 20.6 & -45.2 & 99 &  \\ 
211059325 & 03 44 53.84 & +23 55 16.6 & 10.51 & 8.82 & 21.56$\pm$0.83 & -44.91$\pm$0.86 & 9.3$\pm$1.3$^{(1)}$ & 20.2 & -45.3 & 100 & 2.3386\\ 
211059650 & 03 55 48.71 & +23 55 36.4 & 14.06 & 10.44 & 16.9$\pm$4.2 & -47.4$\pm$11.4 & 15.9$\pm$2.2$^{(1)}$ & 18.9 & -45.7 & 39 & 2.9481\\ 
211059658 & 03 50 12.43 & +23 55 36.6 & 16.08 & 12.17 & 20.78$\pm$2.08 & -50.08$\pm$2.08 & 12.2$\pm$1.7$^{(1)}$ & 19.6 & -45.5 & 98 & 0.3645\\ 
211059727 & 03 46 04.29 & +23 55 40.9 & 15.54 & 11.83 & 19.06$\pm$2.79 & -47.83$\pm$2.79 & 9.1$\pm$1.3$^{(1)}$ & 20.1 & -45.4 & 100 & 0.4336\\ 
211059734 & 03 44 58.58 & +23 55 41.0 & 15.93 & 12.13 & 23.67$\pm$2.23 & -50.5$\pm$2.23 & 8.9$\pm$1.2$^{(1)}$ & 20.2 & -45.3 & 100 & 0.4849\\ 
211059754 & 03 50 25.14 & +23 55 42.0 & 16.55 & 12.8 & 19.9$\pm$2.06 & -45.97$\pm$2.06 & 7.1$\pm$1.0$^{(1)}$ & 19.6 & -45.5 & 100 & 0.6601\\ 
211059767 & 03 49 32.53 & +23 55 42.6 & 16.13 & 12.41 & 21.9$\pm$2.06 & -50.98$\pm$2.06 & 8.5$\pm$1.2$^{(1)}$ & 19.7 & -45.5 & 100 & 0.7781\\ 
211059775 & 03 50 58.16 & +23 55 42.9 & 16.55 & 12.77 & 20.33$\pm$2.05 & -46.56$\pm$2.05 & 7.4$\pm$1.0$^{(1)}$ & 19.5 & -45.6 & 100 & 0.461\\ 
211059880 & 03 41 22.88 & +23 55 48.3 & 16.08 & 12.34 & 17.29$\pm$2.13 & -48.79$\pm$2.13 & 7.7$\pm$1.1$^{(1)}$ & 20.6 & -45.2 & 100 & 0.7308\\ 
211059949 & 03 57 36.07 & +23 55 52.4 & 13.85 & 10.77 & 16.27$\pm$2.08 & -47.17$\pm$2.08 & 7.1$\pm$1.0$^{(1)}$ & 18.7 & -45.8 & 100 & 1.6758\\ 
211059981 & 03 44 56.00 & +23 55 54.0 & 15.83 & 11.91 & 27.48$\pm$2.24 & -48.97$\pm$2.23 & 13.4$\pm$1.8$^{(1)}$ & 20.2 & -45.3 & 76 & 0.3954\\ 
211060049 & 03 51 12.07 & +23 55 57.5 & 13.92 & 10.91 & 16.57$\pm$2.08 & -50.28$\pm$2.08 & 6.8$\pm$0.9$^{(1)}$ & 19.5 & -45.6 & 100 & 4.5971\\ 
211060078 & 03 50 40.07 & +23 55 59.0 & 10.11 & 8.85 & 19.43$\pm$0.77 & -45.72$\pm$0.77 & 6.5$\pm$0.9$^{(1)}$ & 19.5 & -45.5 & 100 & 2.1644\\ 
211060530 & 03 49 36.11 & +23 56 23.4 & 15.99 & 12.31 & 17.7$\pm$2.06 & -49.05$\pm$2.06 & 8.4$\pm$1.2$^{(1)}$ & 19.7 & -45.5 & 100 &  \\ 
211060621 & 03 47 52.53 & +23 56 28.5 & 9.73 & 8.57 & 20.34$\pm$0.95 & -49.34$\pm$0.95 & 6.7$\pm$0.9$^{(1)}$ & 19.9 & -45.5 & 100 & 2.8022\\ 
211060762 & 03 54 28.11 & +23 56 36.4 & 17.84 & 13.75 & 16.66$\pm$2.53 & -49.33$\pm$2.53 & 7.1$\pm$1.0$^{(1)}$ & 19.1 & -45.7 & 100 & 0.3486\\ 
211061207 & 03 45 38.98 & +23 57 01.1 & 17.26 & 13.31 & 15.91$\pm$2.79 & -50.41$\pm$2.79 & 7.6$\pm$1.0$^{(1)}$ & 20.1 & -45.4 & 100 & 0.347\\ 
211061313 & 03 45 49.42 & +23 57 05.9 & 18.0 & 13.83 & 18.6$\pm$2.75 & -47.4$\pm$2.75 & 7.7$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 &  \\ 
211061316 & 03 43 56.99 & +23 57 06.0 & 16.12 & 12.3 & 19.86$\pm$2.15 & -51.31$\pm$2.15 & 9.8$\pm$1.4$^{(1)}$ & 20.3 & -45.3 & 100 & 0.8159\\ 
211062206 & 03 56 18.59 & +23 57 51.8 & 14.56 & 11.28 & 18.9$\pm$2.1 & -53.21$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 18.9 & -45.7 & 100 & 1.1343\\ 
211062438 & 03 48 29.76 & +23 58 06.1 & 16.88 & 13.0 & 20.97$\pm$2.12 & -51.36$\pm$2.12 & 7.8$\pm$1.1$^{(1)}$ & 19.8 & -45.5 & 100 & 0.6205\\ 
211062604 & 03 42 44.46 & +23 58 15.6 & 17.21 & 13.23 & 19.38$\pm$2.64 & -50.53$\pm$2.64 & 6.9$\pm$0.9$^{(1)}$ & 20.5 & -45.3 & 100 & 0.4436\\ 
211062662 & 03 47 41.44 & +23 58 19.0 & 12.89 & 10.31 & 21.3$\pm$2.24 & -49.74$\pm$2.24 & 7.9$\pm$1.1$^{(1)}$ & 19.9 & -45.4 & 100 & 0.483\\ 
211062705 & 03 48 22.75 & +23 58 21.3 & 13.78 & 10.48 & 13.23$\pm$2.12 & -48.0$\pm$2.12 & 10.1$\pm$1.4$^{(1)}$ & 19.8 & -45.5 & 97 & 2.4666\\ 
211062846 & 03 55 34.42 & +23 58 28.6 & 17.08 & 13.26 & 14.67$\pm$2.1 & -47.76$\pm$2.1 & 6.3$\pm$0.9$^{(1)}$ & 19.0 & -45.7 & 100 & 0.5027\\ 
211063000 & 03 48 49.32 & +23 58 38.1 & 12.15 & 9.99 & 24.49$\pm$2.34 & -43.84$\pm$2.34 & 7.0$\pm$1.0$^{(1)}$ & 19.8 & -45.5 & 100 & 0.5503\\ 
211063049 & 03 48 09.21 & +23 58 40.9 & 16.35 & 12.65 & 12.33$\pm$2.19 & -47.66$\pm$2.19 & 7.7$\pm$1.1$^{(1)}$ & 19.8 & -45.5 & 99 & 0.9637\\ 
211063081 & 03 41 56.72 & +23 58 43.4 & 17.29 & 13.25 & 14.0$\pm$2.14 & -39.52$\pm$2.14 & 7.0$\pm$1.0$^{(1)}$ & 20.6 & -45.2 & 98 & 0.4007\\ 
211063098 & 03 50 50.95 & +23 58 44.3 & 16.31 & 12.34 & 14.74$\pm$2.03 & -42.02$\pm$2.03 & 11.4$\pm$1.6$^{(1)}$ & 19.5 & -45.6 & 95 &  \\ 
211063134 & 03 48 13.31 & +23 58 47.1 & 16.19 & 12.36 & 14.48$\pm$2.19 & -49.37$\pm$2.19 & 9.5$\pm$1.3$^{(1)}$ & 19.8 & -45.5 & 99 & 0.8237\\ 
211063235 & 03 39 46.34 & +23 58 53.1 & 15.35 & 11.83 & 18.73$\pm$2.2 & -50.45$\pm$2.2 & 8.2$\pm$1.1$^{(1)}$ & 20.8 & -45.2 & 100 & 1.1377\\ 
211063723 & 03 48 10.17 & +23 59 20.5 & 17.59 & 13.49 & 12.85$\pm$2.16 & -44.49$\pm$2.16 & 7.7$\pm$1.1$^{(1)}$ & 19.8 & -45.5 & 99 & 0.6734\\ 
211063744 & 03 42 40.22 & +23 59 21.7 & 14.63 & 11.15 & 16.91$\pm$2.14 & -50.28$\pm$2.14 & 9.1$\pm$1.3$^{(1)}$ & 20.5 & -45.3 & 100 & 0.2587\\ 
211063756 & 03 42 18.87 & +23 59 22.3 & 13.95 & 11.17 & 26.06$\pm$2.14 & -51.61$\pm$2.14 & 5.2$\pm$0.7$^{(1)}$ & 20.5 & -45.3 & 92 &  \\ 
211064137 & 03 46 43.60 & +23 59 42.5 & 14.9 & 11.58 & 15.02$\pm$2.24 & -52.52$\pm$2.24 & 6.3$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 99 & 2.234\\ 
211064196 & 03 50 12.25 & +23 59 45.2 & 14.38 & 10.84 & 13.86$\pm$2.06 & -46.87$\pm$2.06 & 12.2$\pm$1.7$^{(1)}$ & 19.6 & -45.5 & 92 & 1.8401\\ 
211064435 & 03 44 27.91 & +23 59 59.9 & 17.68 & 13.49 & 16.36$\pm$2.79 & -52.17$\pm$2.79 & 7.4$\pm$1.0$^{(1)}$ & 20.3 & -45.3 & 100 & 0.3044\\ 
211064526 & 03 44 35.41 & +24 00 04.8 & 13.53 & 10.65 & 18.9$\pm$2.23 & -49.64$\pm$2.23 & 6.7$\pm$0.9$^{(1)}$ & 20.3 & -45.3 & 100 & 9.0574\\ 
211064559 & 03 48 06.64 & +24 00 07.0 & 16.32 & 12.54 & 15.6$\pm$2.18 & -50.75$\pm$2.17 & 7.9$\pm$1.1$^{(1)}$ & 19.8 & -45.5 & 100 & 0.6242\\ 
211064722 & 03 42 41.85 & +24 00 15.8 & 16.42 & 12.68 & 20.5$\pm$2.14 & -51.84$\pm$2.14 & 7.1$\pm$1.0$^{(1)}$ & 20.5 & -45.3 & 100 & 0.6713\\ 
211065006 & 03 57 16.85 & +24 00 33.1 & 12.23 & 9.94 & 18.76$\pm$2.29 & -53.7$\pm$2.29 & 7.8$\pm$1.1$^{(1)}$ & 18.8 & -45.8 & 100 & 7.2904\\ 
211065077 & 03 44 47.32 & +24 00 37.9 & 15.96 & 12.33 & 21.04$\pm$2.23 & -53.21$\pm$2.23 & 7.0$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 100 & 0.7563\\ 
211065162 & 03 36 30.30 & +24 00 43.8 & 11.87 & 9.9 & 19.39$\pm$2.34 & -45.72$\pm$2.34 & 6.9$\pm$0.9$^{(1)}$ & 21.2 & -45.0 & 100 & 7.551\\ 
211065426 & 03 58 25.13 & +24 00 58.9 & 16.26 & 12.49 & 19.7$\pm$2.1 & -50.22$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 18.6 & -45.8 & 100 & 0.6209\\ 
211065494 & 03 41 26.88 & +24 01 02.6 & 15.32 & 11.47 & 17.93$\pm$2.13 & -47.26$\pm$2.13 & 13.6$\pm$1.9$^{(1)}$ & 20.6 & -45.2 & 95 & 0.3591\\ 
211066062 & 03 46 35.53 & +24 01 35.6 & 16.88 & 12.82 & 19.08$\pm$2.81 & -53.43$\pm$2.92 & 10.4$\pm$1.4$^{(1)}$ & 20.0 & -45.4 & 99 & 0.2973\\ 
211066157 & 03 46 58.26 & +24 01 41.5 & 16.98 & 13.07 & 17.51$\pm$2.91 & -49.25$\pm$2.91 & 8.2$\pm$1.1$^{(1)}$ & 20.0 & -45.4 & 100 & 0.8082\\ 
211066181 & 03 46 59.31 & +24 01 42.9 & 15.97 & 12.12 & 16.91$\pm$2.19 & -52.47$\pm$2.19 & 11.3$\pm$1.6$^{(1)}$ & 20.0 & -45.4 & 95 & 0.5265\\ 
211066186 & 03 42 41.17 & +24 01 43.0 & 17.0 & 13.08 & 21.39$\pm$2.14 & -48.31$\pm$2.14 & 7.7$\pm$1.1$^{(1)}$ & 20.5 & -45.3 & 100 & 0.5634\\ 
211066263 & 03 46 39.39 & +24 01 46.9 & 11.85 & 9.86 & 17.86$\pm$0.91 & -49.24$\pm$0.91 & 6.8$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 100 & 6.1296\\ 
211066346 & 03 46 23.46 & +24 01 51.4 & 16.73 & 12.78 & 19.12$\pm$2.75 & -48.06$\pm$2.75 & 8.3$\pm$1.1$^{(1)}$ & 20.0 & -45.4 & 100 & 0.4678\\ 
211066413 & 03 56 28.90 & +24 01 54.4 & 16.38 & 12.64 & 17.28$\pm$2.1 & -52.22$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & 18.9 & -45.8 & 100 & 0.4551\\ 
211066477 & 03 48 31.83 & +24 01 59.0 & 16.64 & 12.85 & 14.67$\pm$2.16 & -54.29$\pm$2.16 & 7.1$\pm$1.0$^{(1)}$ & 19.8 & -45.5 & 97 & 0.4896\\ 
211066484 & 03 48 33.78 & +24 01 59.2 & 16.65 & 12.94 & 16.16$\pm$2.16 & -51.96$\pm$2.16 & 6.5$\pm$0.9$^{(1)}$ & 19.8 & -45.5 & 100 & 1.3602\\ 
211066615 & 03 45 26.14 & +24 02 06.5 & 8.01 & 7.46 & 21.31$\pm$0.45 & -46.95$\pm$0.45 & 8.2$\pm$0.3$^{(0)}$ & 20.2 & -45.4 & 100 & 0.1212\\ 
211066835 & 03 45 51.63 & +24 02 20.0 & 7.84 & 7.33 & 19.72$\pm$0.5 & -44.88$\pm$0.39 & 7.4$\pm$0.2$^{(0)}$ & 20.1 & -45.4 & 100 &  \\ 
211067166 & 03 39 22.06 & +24 02 39.2 & 17.17 & 13.38 & 13.42$\pm$2.2 & -37.35$\pm$2.2 & 5.6$\pm$0.8$^{(1)}$ & 20.9 & -45.2 & 66 &  \\ 
211067419 & 03 48 26.17 & +24 02 54.1 & 9.85 & 8.66 & 18.45$\pm$0.94 & -48.9$\pm$0.94 & 6.3$\pm$0.9$^{(1)}$ & 19.8 & -45.5 & 100 & 2.491\\ 
211067634 & 03 47 09.18 & +24 03 08.0 & 15.21 & 11.72 & 19.48$\pm$2.91 & -53.8$\pm$2.91 & 7.3$\pm$1.0$^{(1)}$ & 20.0 & -45.4 & 100 & 0.2679\\ 
211067702 & 03 57 33.31 & +24 03 11.5 & 11.73 & 9.86 & 16.45$\pm$0.91 & -46.95$\pm$0.91 & 6.0$\pm$0.8$^{(1)}$ & 18.7 & -45.8 & 100 & 7.798\\ 
211067768 & 03 46 12.87 & +24 03 15.7 & 13.44 & 10.59 & 22.5$\pm$2.12 & -51.37$\pm$2.12 & 7.2$\pm$1.0$^{(1)}$ & 20.1 & -45.4 & 100 & 1.3879\\ 
211067927 & 03 41 31.19 & +24 03 25.0 & 16.97 & 13.06 & 22.91$\pm$2.14 & -53.53$\pm$2.14 & 7.4$\pm$1.0$^{(1)}$ & 20.6 & -45.2 & 100 & 0.3868\\ 
211067949 & 03 53 21.67 & +24 03 26.8 & 17.35 & 13.25 & 12.87$\pm$2.68 & -43.74$\pm$2.68 & 8.0$\pm$1.1$^{(1)}$ & 19.2 & -45.7 & 100 &  \\ 
211068230 & 03 49 52.42 & +24 03 43.3 & 18.26 & 13.93 & 22.1$\pm$2.7 & -48.6$\pm$2.7 & 6.9$\pm$1.0$^{(1)}$ & 19.6 & -45.5 & 100 &  \\ 
211068337 & 03 49 16.41 & +24 03 49.3 & 14.26 & 10.75 & 22.81$\pm$4.63 & -45.19$\pm$4.62 & 10.7$\pm$1.5$^{(1)}$ & 19.7 & -45.5 & 99 & 0.4015\\ 
211068400 & 03 53 23.71 & +24 03 54.2 & 11.15 & 9.44 & 19.79$\pm$1.04 & -45.74$\pm$0.59 & 7.3$\pm$0.3$^{(0)}$ & 19.2 & -45.7 & 100 & 4.065\\ 
211068579 & 03 44 23.06 & +24 04 05.8 & 13.01 & 10.17 & 19.19$\pm$2.23 & -52.17$\pm$2.23 & 8.7$\pm$1.2$^{(1)}$ & 20.3 & -45.3 & 100 & 0.3567\\ 
211068914 & 03 45 44.08 & +24 04 26.8 & 13.56 & 10.66 & 17.99$\pm$2.12 & -49.95$\pm$2.12 & 6.9$\pm$1.0$^{(1)}$ & 20.1 & -45.4 & 100 & 3.7965\\ 
211069011 & 03 54 21.59 & +24 04 32.5 & 9.55 & 8.42 & 19.46$\pm$0.87 & -45.69$\pm$0.45 & 7.7$\pm$0.3$^{(0)}$ & 19.1 & -45.7 & 100 & 0.8817\\ 
211069316 & 03 58 20.90 & +24 04 52.1 & 7.22 & 7.12 & 19.02$\pm$0.08 & -45.22$\pm$0.03 & 7.3$\pm$0.4$^{(0)}$ & 18.6 & -45.8 & 100 &  \\ 
211069418 & 03 42 56.54 & +24 04 58.1 & 14.78 & 11.21 & 17.46$\pm$2.14 & -53.39$\pm$2.14 & 11.3$\pm$1.6$^{(1)}$ & 20.4 & -45.3 & 89 & 0.8174\\ 
211069456 & 03 45 35.40 & +24 04 59.5 & 9.94 & 8.56 & 14.47$\pm$0.76 & -44.58$\pm$0.76 & 8.5$\pm$1.2$^{(1)}$ & 20.1 & -45.4 & 99 & 1.0199\\ 
211069510 & 03 55 09.00 & +24 05 02.3 & 15.45 & 11.89 & 18.07$\pm$2.1 & -51.16$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 19.0 & -45.7 & 100 & 1.828\\ 
211069615 & 03 42 10.92 & +24 05 08.7 & 14.59 & 11.17 & 20.13$\pm$2.14 & -50.27$\pm$2.14 & 9.2$\pm$1.3$^{(1)}$ & 20.5 & -45.3 & 100 & 0.4774\\ 
211069863 & 03 40 26.39 & +24 05 23.9 & 15.33 & 11.68 & 16.67$\pm$2.18 & -45.87$\pm$2.18 & 8.3$\pm$1.1$^{(1)}$ & 20.7 & -45.2 & 100 & 0.7654\\ 
211070495 & 03 40 25.61 & +24 06 00.3 & 16.69 & 12.83 & 20.04$\pm$2.18 & -50.43$\pm$2.18 & 7.5$\pm$1.0$^{(1)}$ & 20.7 & -45.2 & 100 & 0.606\\ 
211070577 & 03 49 55.48 & +24 06 05.2 & 16.45 & 12.62 & 19.78$\pm$2.06 & -51.91$\pm$2.06 & 8.3$\pm$1.1$^{(1)}$ & 19.6 & -45.5 & 100 & 0.5612\\ 
211070664 & 03 46 39.33 & +24 06 11.5 & 9.16 & 8.19 & 19.72$\pm$0.81 & -45.75$\pm$0.89 & 6.5$\pm$0.9$^{(1)}$ & 20.0 & -45.4 & 100 & 0.8702\\ 
211071351 & 03 43 11.64 & +24 06 52.7 & 17.28 & 13.2 & 17.18$\pm$2.65 & -43.44$\pm$2.65 & 8.5$\pm$1.2$^{(1)}$ & 20.4 & -45.3 & 100 & 0.4164\\ 
211071431 & 03 42 17.89 & +24 06 57.8 & 16.85 & 12.97 & 25.56$\pm$2.14 & -49.81$\pm$2.14 & 8.4$\pm$1.2$^{(1)}$ & 20.5 & -45.3 & 100 & 0.6026\\ 
211071504 & 03 46 31.18 & +24 07 02.5 & 13.31 & 10.46 & 15.81$\pm$1.73 & -49.28$\pm$2.21 & 7.8$\pm$1.1$^{(1)}$ & 20.0 & -45.4 & 100 & 4.8107\\ 
211071563 & 03 39 35.45 & +24 07 06.4 & 14.51 & 11.18 & 22.97$\pm$2.16 & -48.54$\pm$2.16 & 7.7$\pm$1.1$^{(1)}$ & 20.8 & -45.2 & 100 &  \\ 
211071722 & 03 45 16.14 & +24 07 16.1 & 15.01 & 11.59 & 20.82$\pm$2.79 & -48.92$\pm$2.79 & 6.9$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 100 & 2.1851\\ 
211071863 & 03 41 52.93 & +24 07 25.0 & 17.06 & 13.25 & 16.59$\pm$2.14 & -51.86$\pm$2.14 & 6.9$\pm$1.0$^{(1)}$ & 20.6 & -45.3 & 100 & 0.515\\ 
211071889 & 03 50 05.05 & +24 07 26.3 & 13.3 & 10.56 & 17.37$\pm$2.08 & -49.43$\pm$2.08 & 7.1$\pm$1.0$^{(1)}$ & 19.6 & -45.6 & 100 & 6.4254\\ 
211072160 & 03 47 16.57 & +24 07 42.1 & 8.56 & 7.49 & 17.14$\pm$0.5 & -43.36$\pm$0.57 & 9.7$\pm$1.3$^{(1)}$ & 19.9 & -45.5 & 100 & 7.5994\\ 
211072438 & 03 46 53.96 & +24 07 57.4 & 17.14 & 13.2 & 17.22$\pm$2.85 & -49.44$\pm$2.85 & 7.3$\pm$1.0$^{(1)}$ & 20.0 & -45.4 & 100 & 0.3912\\ 
211072441 & 03 44 23.55 & +24 07 57.6 & 8.93 & 7.77 & 25.62$\pm$0.79 & -45.52$\pm$0.45 & 8.1$\pm$0.3$^{(0)}$ & 20.3 & -45.4 & 99 & 0.5889\\ 
211072835 & 03 45 39.28 & +24 08 20.6 & 17.01 & 13.02 & 20.42$\pm$2.79 & -48.34$\pm$2.79 & 8.3$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 & 0.8158\\ 
211072836 & 03 47 19.35 & +24 08 20.8 & 8.24 & 7.64 & 17.88$\pm$0.76 & -43.46$\pm$0.43 & 7.6$\pm$0.3$^{(0)}$ & 19.9 & -45.5 & 100 &  \\ 
211073154 & 03 45 57.90 & +24 08 41.2 & 17.77 & 13.66 & 23.29$\pm$2.79 & -48.56$\pm$2.79 & 7.0$\pm$1.0$^{(1)}$ & 20.1 & -45.4 & 100 & 0.2184\\ 
211073598 & 03 43 28.73 & +24 09 06.4 & 17.21 & 13.26 & 18.9$\pm$2.65 & -46.28$\pm$2.65 & 7.2$\pm$1.0$^{(1)}$ & 20.4 & -45.3 & 100 &  \\ 
211073953 & 03 40 46.30 & +24 09 25.8 & 16.42 & 12.66 & 29.48$\pm$2.16 & -42.21$\pm$2.13 & 7.4$\pm$1.0$^{(1)}$ & 20.7 & -45.2 & 96 &  \\ 
211074122 & 03 47 03.58 & +24 09 34.8 & 13.67 & 10.73 & 17.01$\pm$2.19 & -51.24$\pm$2.19 & 6.9$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 0.3023\\ 
211074151 & 03 46 25.39 & +24 09 36.5 & 14.6 & 11.13 & 25.96$\pm$2.22 & -53.04$\pm$2.22 & 8.6$\pm$1.2$^{(1)}$ & 20.0 & -45.4 & 99 & 0.3224\\ 
211074500 & 03 46 04.55 & +24 09 56.1 & 17.13 & 13.15 & 20.13$\pm$2.86 & -47.55$\pm$2.86 & 6.8$\pm$0.9$^{(1)}$ & 20.1 & -45.4 & 100 & 0.728\\ 
211074799 & 03 42 00.36 & +24 10 12.9 & 18.38 & 14.03 & 23.04$\pm$2.86 & -49.34$\pm$2.86 & 6.5$\pm$0.9$^{(1)}$ & 20.6 & -45.3 & 100 & 0.2821\\ 
211074858 & 03 42 49.11 & +24 10 15.9 & 15.55 & 11.74 & 21.07$\pm$2.14 & -44.43$\pm$2.14 & 11.7$\pm$1.6$^{(1)}$ & 20.5 & -45.3 & 99 & 1.4585\\ 
211074888 & 03 44 28.01 & +24 10 17.6 & 12.74 & 10.02 & 17.1$\pm$2.23 & -49.91$\pm$2.23 & 9.0$\pm$1.2$^{(1)}$ & 20.3 & -45.4 & 100 & 3.8002\\ 
211075627 & 03 42 33.96 & +24 11 00.8 & 17.5 & 13.42 & 23.62$\pm$2.14 & -44.92$\pm$2.14 & 7.0$\pm$1.0$^{(1)}$ & 20.5 & -45.3 & 100 & 0.5641\\ 
211075637 & 03 43 13.46 & +24 11 01.2 & 17.75 & 13.6 & 15.18$\pm$2.65 & -49.21$\pm$2.65 & 6.9$\pm$0.9$^{(1)}$ & 20.4 & -45.3 & 100 & $<$2\\ 
211075777 & 03 43 21.11 & +24 11 09.2 & 17.29 & 13.3 & 19.81$\pm$2.14 & -45.23$\pm$2.14 & 7.6$\pm$1.0$^{(1)}$ & 20.4 & -45.3 & 100 &  \\ 
211075914 & 03 46 55.31 & +24 11 16.9 & 17.02 & 12.87 & 20.5$\pm$2.91 & -49.78$\pm$2.91 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -45.5 & 100 & 0.2397\\ 
211076042 & 03 46 16.00 & +24 11 23.8 & 8.22 & 7.11 & 19.9$\pm$0.7 & -43.29$\pm$0.4 & 15.1$\pm$2.1$^{(1)}$ & 20.1 & -45.4 & 93 &  \\ 
211076441 & 03 49 59.53 & +24 11 46.1 & 17.63 & 13.47 & 20.59$\pm$2.06 & -51.02$\pm$2.06 & 7.2$\pm$1.0$^{(1)}$ & 19.6 & -45.6 & 100 & 1.0385\\ 
211076650 & 03 42 41.90 & +24 11 58.1 & 13.7 & 10.47 & 20.41$\pm$2.14 & -47.52$\pm$2.14 & 10.2$\pm$1.4$^{(1)}$ & 20.5 & -45.3 & 100 & 4.8225\\ 
211076761 & 03 48 35.48 & +24 12 03.4 & 17.24 & 13.24 & 21.77$\pm$2.61 & -50.56$\pm$2.61 & 8.4$\pm$1.2$^{(1)}$ & 19.8 & -45.5 & 100 & 0.5216\\ 
211077349 & 03 42 02.87 & +24 12 36.3 & 15.1 & 11.61 & 19.16$\pm$2.18 & -49.12$\pm$2.18 & 7.2$\pm$1.0$^{(1)}$ & 20.5 & -45.3 & 100 & 0.6995\\ 
211077464 & 03 48 39.90 & +24 12 42.9 & 15.32 & 11.84 & 14.13$\pm$2.19 & -53.48$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & 19.8 & -45.5 & 98 & 0.9204\\ 
211077607 & 03 43 43.52 & +24 12 50.3 & 17.59 & 13.57 & 20.63$\pm$2.68 & -49.63$\pm$2.68 & 7.0$\pm$1.0$^{(1)}$ & 20.4 & -45.3 & 100 & 0.3123\\ 
211077649 & 03 44 47.84 & +24 12 52.8 & 16.29 & 12.43 & 17.45$\pm$2.26 & -55.84$\pm$2.33 & 9.5$\pm$1.3$^{(1)}$ & 20.2 & -45.4 & 91 & 0.8136\\ 
211077682 & 03 39 55.20 & +24 12 54.4 & 17.53 & 13.45 & 21.35$\pm$2.16 & -48.73$\pm$2.16 & 7.5$\pm$1.0$^{(1)}$ & 20.8 & -45.2 & 100 & 0.3291\\ 
211077833 & 03 40 07.10 & +24 13 03.6 & 17.52 & 13.54 & 21.03$\pm$2.64 & -48.76$\pm$2.64 & 7.3$\pm$1.0$^{(1)}$ & 20.8 & -45.2 & 100 & 0.4198\\ 
211078009 & 03 45 44.41 & +24 13 13.1 & 10.33 & 8.75 & 18.68$\pm$0.75 & -47.76$\pm$0.74 & 7.9$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 &  \\ 
211078145 & 03 43 57.27 & +24 13 20.5 & 16.17 & 12.35 & 21.01$\pm$2.24 & -50.79$\pm$2.24 & 9.6$\pm$1.3$^{(1)}$ & 20.3 & -45.4 & 100 & 0.7717\\ 
211078274 & 03 47 01.84 & +24 13 28.4 & 18.4 & 14.0 & 14.56$\pm$2.91 & -45.6$\pm$2.91 & 7.0$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 1.0167\\ 
211078393 & 03 41 00.39 & +24 13 35.3 & 16.84 & 12.94 & 17.11$\pm$2.13 & -48.87$\pm$2.13 & 7.9$\pm$1.1$^{(1)}$ & 20.7 & -45.2 & 100 & 0.5214\\ 
211078413 & 03 50 15.26 & +24 13 36.3 & 16.04 & 12.38 & 23.1$\pm$2.08 & -48.94$\pm$2.08 & 8.3$\pm$1.2$^{(1)}$ & 19.6 & -45.6 & 100 & 1.1204\\ 
211078565 & 03 42 56.56 & +24 13 45.8 & 16.92 & 12.98 & 20.09$\pm$2.64 & -49.4$\pm$2.64 & 8.6$\pm$1.2$^{(1)}$ & 20.4 & -45.3 & 100 & 0.3657\\ 
211078690 & 03 47 18.13 & +24 13 51.4 & 16.84 & 12.33 & 17.49$\pm$2.91 & -42.54$\pm$2.91 & 18.1$\pm$2.5$^{(1)}$ & 19.9 & -45.5 & 45 & 0.3239\\ 
211078698 & 03 47 11.02 & +24 13 51.7 & 17.38 & 13.4 & 18.97$\pm$2.75 & -51.29$\pm$2.75 & 7.3$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 0.4019\\ 
211078745 & 03 47 11.86 & +24 13 54.0 & 17.36 & 13.15 & 23.55$\pm$2.91 & -52.32$\pm$2.91 & 10.1$\pm$1.4$^{(1)}$ & 20.0 & -45.5 & 99 &  \\ 
211078779 & 04 12 37.63 & +24 13 56.2 & 11.6 & 9.38 & 18.33$\pm$0.92 & -51.1$\pm$0.92 & 10.2$\pm$1.4$^{(1)}$ & 16.9 & -46.3 & 81 &  \\ 
211078992 & 03 42 26.28 & +24 14 07.9 & 16.1 & 12.39 & 20.55$\pm$2.14 & -45.94$\pm$2.14 & 8.3$\pm$1.1$^{(1)}$ & 20.5 & -45.3 & 100 & 0.9519\\ 
211079106 & 03 40 26.95 & +24 14 14.5 & 16.32 & 12.52 & 19.14$\pm$2.14 & -51.12$\pm$2.14 & 7.9$\pm$1.1$^{(1)}$ & 20.7 & -45.2 & 100 & 0.8235\\ 
211079141 & 03 43 51.75 & +24 14 16.1 & 16.32 & 12.34 & 17.51$\pm$2.15 & -47.67$\pm$2.15 & 11.2$\pm$1.5$^{(1)}$ & 20.3 & -45.4 & 99 & 0.6467\\ 
211079163 & 03 44 27.49 & +24 14 17.3 & 16.62 & 12.62 & 27.9$\pm$2.23 & -53.82$\pm$2.23 & 9.9$\pm$1.4$^{(1)}$ & 20.3 & -45.4 & 88 & 0.235\\ 
211079188 & 03 47 22.37 & +24 14 18.9 & 17.43 & 13.21 & 18.57$\pm$2.81 & -45.11$\pm$2.81 & 8.9$\pm$1.2$^{(1)}$ & 19.9 & -45.5 & 100 & 0.1749\\ 
211079332 & 03 48 25.23 & +24 14 26.2 & 15.87 & 11.98 & 15.25$\pm$2.19 & -52.83$\pm$2.19 & 12.4$\pm$1.7$^{(1)}$ & 19.8 & -45.5 & 72 & 0.7114\\ 
211079794 & 03 43 50.71 & +24 14 50.9 & 11.03 & 9.34 & 21.53$\pm$0.89 & -45.15$\pm$0.49 & 8.0$\pm$0.4$^{(0)}$ & 20.3 & -45.4 & 100 & 5.3638\\ 
211079830 & 03 43 01.25 & +24 14 52.5 & 17.36 & 13.26 & 16.76$\pm$2.64 & -48.66$\pm$2.64 & 7.4$\pm$1.0$^{(1)}$ & 20.4 & -45.3 & 100 & 0.3437\\ 
211080177 & 03 44 20.65 & +24 15 11.0 & 17.63 & 13.14 & 20.61$\pm$2.23 & -55.52$\pm$2.23 & 11.8$\pm$1.6$^{(1)}$ & 20.3 & -45.4 & 77 & 0.3489\\ 
211080227 & 03 41 24.63 & +24 15 14.0 & 18.2 & 14.2 & 27.0$\pm$2.73 & -44.46$\pm$2.73 & 4.6$\pm$0.6$^{(1)}$ & 20.6 & -45.3 & 52 &  \\ 
211080295 & 03 47 25.12 & +24 15 17.4 & 16.89 & 13.02 & 18.38$\pm$2.81 & -52.25$\pm$2.92 & 7.3$\pm$1.0$^{(1)}$ & 19.9 & -45.5 & 100 & 1.1885\\ 
211080301 & 03 46 27.28 & +24 15 18.0 & 7.36 & 7.12 & 19.96$\pm$0.36 & -44.29$\pm$0.32 & 7.7$\pm$0.3$^{(0)}$ & 20.0 & -45.4 & 100 &  \\ 
211080412 & 03 45 13.14 & +24 15 23.8 & 17.04 & 13.2 & 22.14$\pm$2.86 & -54.49$\pm$2.98 & 7.3$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 100 & 2.0103\\ 
211080546 & 03 47 56.63 & +24 15 32.1 & 17.33 & 13.34 & 22.26$\pm$2.75 & -50.58$\pm$2.75 & 7.4$\pm$1.0$^{(1)}$ & 19.9 & -45.5 & 100 & 0.7302\\ 
211080604 & 03 47 09.41 & +24 15 34.9 & 17.67 & 13.62 & 13.89$\pm$2.85 & -53.37$\pm$2.85 & 7.1$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 99 &  \\ 
211080847 & 03 45 06.54 & +24 15 48.7 & 8.53 & 7.74 & 19.28$\pm$0.51 & -42.44$\pm$0.56 & 8.1$\pm$0.5$^{(0)}$ & 20.2 & -45.4 & 100 & 0.0431\\ 
211081065 & 03 39 32.31 & +24 16 01.4 & 15.96 & 12.2 & 19.05$\pm$2.16 & -51.68$\pm$2.16 & 9.5$\pm$1.3$^{(1)}$ & 20.8 & -45.2 & 99 & 0.72\\ 
211081096 & 03 48 48.96 & +24 16 02.6 & 10.64 & 8.81 & 18.26$\pm$0.84 & -48.1$\pm$0.84 & 10.4$\pm$1.4$^{(1)}$ & 19.8 & -45.5 & 100 & 5.0921\\ 
211081122 & 03 44 09.91 & +24 16 04.1 & 15.0 & 11.52 & 19.07$\pm$2.15 & -45.28$\pm$2.15 & 7.6$\pm$1.0$^{(1)}$ & 20.3 & -45.4 & 100 & 1.2348\\ 
211081593 & 03 44 04.84 & +24 16 31.9 & 11.13 & 9.39 & 18.41$\pm$0.84 & -44.68$\pm$0.84 & 6.9$\pm$1.0$^{(1)}$ & 20.3 & -45.4 & 100 & 4.6762\\ 
211081656 & 03 47 10.05 & +24 16 35.9 & 9.33 & 8.28 & 20.43$\pm$1.04 & -43.95$\pm$0.36 & 7.1$\pm$0.4$^{(0)}$ & 20.0 & -45.5 & 100 & 0.775\\ 
211081949 & 03 56 25.93 & +24 16 51.6 & 14.02 & 11.01 & 17.71$\pm$2.1 & -49.21$\pm$2.1 & 6.2$\pm$0.9$^{(1)}$ & 18.9 & -45.8 & 100 & 2.1138\\ 
211081985 & 03 48 31.05 & +24 16 53.5 & 14.77 & 11.35 & 21.98$\pm$2.08 & -51.43$\pm$2.08 & 7.5$\pm$1.0$^{(1)}$ & 19.8 & -45.5 & 100 & 0.258\\ 
211082363 & 03 46 53.62 & +24 17 15.1 & 14.79 & 11.2 & 17.33$\pm$2.24 & -53.72$\pm$2.24 & 11.5$\pm$1.6$^{(1)}$ & 20.0 & -45.5 & 90 & 0.6607\\ 
211082420 & 03 47 29.45 & +24 17 18.0 & 6.83 & 6.61 & 18.48$\pm$0.05 & -46.91$\pm$0.04 & 7.6$\pm$0.4$^{(0)}$ & 19.9 & -45.5 & 100 &  \\ 
211082429 & 03 59 12.92 & +24 17 18.7 & 16.7 & 12.84 & 17.07$\pm$2.1 & -44.46$\pm$2.1 & 7.6$\pm$1.0$^{(1)}$ & 18.5 & -45.9 & 100 & 0.5426\\ 
211082436 & 03 45 41.39 & +24 17 18.9 & 9.31 & 8.04 & 16.85$\pm$0.69 & -48.08$\pm$0.8 & 9.7$\pm$1.3$^{(1)}$ & 20.1 & -45.4 & 100 & 0.8383\\ 
211082469 & 03 45 40.24 & +24 17 20.7 & 16.62 & 12.91 & 6.36$\pm$3.04 & -51.15$\pm$3.04 & 6.8$\pm$0.9$^{(1)}$ & 20.1 & -45.4 & 50 &  \\ 
211082883 & 03 45 51.32 & +24 17 44.5 & 16.63 & 12.76 & 19.81$\pm$2.79 & -49.48$\pm$2.79 & 8.6$\pm$1.2$^{(1)}$ & 20.1 & -45.4 & 100 & 0.4114\\ 
211083317 & 03 47 40.38 & +24 18 07.0 & 13.13 & 10.33 & 21.52$\pm$2.1 & -52.32$\pm$2.1 & 8.1$\pm$1.1$^{(1)}$ & 19.9 & -45.5 & 100 & 0.3067\\ 
211083343 & 04 09 52.41 & +24 18 08.2 & 15.87 & 12.39 & 21.23$\pm$2.07 & -52.99$\pm$2.07 & 5.4$\pm$0.7$^{(1)}$ & 17.2 & -46.2 & 52 &  \\ 
211083408 & 03 45 32.95 & +24 18 11.6 & 12.9 & 10.24 & 18.38$\pm$2.23 & -54.79$\pm$2.23 & 7.9$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 99 & 0.3976\\ 
211083672 & 03 47 08.14 & +24 18 24.7 & 15.51 & 11.91 & 18.33$\pm$2.15 & -53.77$\pm$2.15 & 8.0$\pm$1.1$^{(1)}$ & 20.0 & -45.5 & 100 & 1.8237\\ 
211084069 & 03 45 30.24 & +24 18 45.5 & 14.44 & 11.14 & 16.55$\pm$2.23 & -56.2$\pm$2.23 & 7.3$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 94 & 2.1929\\ 
211084148 & 03 42 13.48 & +24 18 49.8 & 17.67 & 13.62 & 20.57$\pm$2.64 & -44.25$\pm$2.64 & 7.0$\pm$1.0$^{(1)}$ & 20.5 & -45.3 & 100 & 0.7131\\ 
211084436 & 03 48 13.56 & +24 19 06.3 & 8.19 & 7.35 & 18.64$\pm$0.53 & -43.5$\pm$0.46 & 7.1$\pm$0.4$^{(0)}$ & 19.8 & -45.5 & 100 & 1.6856\\ 
211084620 & 03 54 28.45 & +24 19 16.1 & 13.44 & 10.62 & 17.94$\pm$2.12 & -49.14$\pm$2.12 & 7.1$\pm$1.0$^{(1)}$ & 19.1 & -45.7 & 100 & 4.6203\\ 
211085091 & 03 48 57.35 & +24 19 43.9 & 14.52 & 11.05 & 21.64$\pm$2.13 & -47.63$\pm$2.13 & 9.3$\pm$1.3$^{(1)}$ & 19.7 & -45.5 & 100 & 1.706\\ 
211085419 & 03 54 08.92 & +24 20 01.3 & 12.04 & 9.72 & 15.77$\pm$0.91 & -45.37$\pm$0.91 & 9.9$\pm$1.4$^{(1)}$ & 19.1 & -45.7 & 100 & 8.1192\\ 
211085527 & 03 45 37.79 & +24 20 08.2 & 7.16 & 6.63 & 20.43$\pm$0.21 & -38.84$\pm$0.25 & 10.5$\pm$1.4$^{(1)}$ & 20.1 & -45.4 & 90 &  \\ 
211086025 & 03 46 37.28 & +24 20 36.7 &   & 9.4 & 20.9$\pm$2.1 & -42.0$\pm$1.9 & 11.2$\pm$1.5$^{(2)}$ & 20.0 & -45.5 & 99 & 4.317\\ 
211086138 & 03 48 30.10 & +24 20 43.9 & 6.95 & 6.56 & 19.96$\pm$0.04 & -44.24$\pm$0.04 & 7.9$\pm$1.3$^{(0)}$ & 19.8 & -45.5 & 100 & 0.3075\\ 
211086147 & 03 59 19.03 & +24 20 44.5 & 12.61 & 10.43 & 14.71$\pm$2.1 & -43.49$\pm$2.1 & 5.8$\pm$0.8$^{(1)}$ & 18.5 & -45.9 & 100 &  \\ 
211086163 & 03 45 24.78 & +24 20 45.5 & 16.05 & 12.25 & 16.22$\pm$2.79 & -46.26$\pm$2.79 & 9.1$\pm$1.3$^{(1)}$ & 20.2 & -45.4 & 100 & 0.941\\ 
211086170 & 03 54 15.60 & +24 20 45.8 & 17.95 & 13.71 & 13.7$\pm$2.67 & -45.7$\pm$2.67 & 6.6$\pm$0.9$^{(1)}$ & 19.1 & -45.7 & 100 & 0.1836\\ 
211086260 & 03 49 11.03 & +24 20 51.4 & 15.84 & 12.14 & 22.14$\pm$2.13 & -47.1$\pm$2.13 & 7.9$\pm$1.1$^{(1)}$ & 19.7 & -45.6 & 100 & 2.0109\\ 
211086387 & 03 46 03.45 & +24 20 57.2 & 16.4 & 12.61 & 18.81$\pm$2.79 & -44.71$\pm$2.79 & 8.0$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 & 0.3745\\ 
211086444 & 03 52 44.47 & +24 20 59.6 & 16.99 & 13.13 & 22.0$\pm$2.15 & -50.62$\pm$2.15 & 7.4$\pm$1.0$^{(1)}$ & 19.3 & -45.7 & 100 & 0.4562\\ 
211087059 & 03 54 25.24 & +24 21 36.3 & 10.76 & 9.09 & 18.03$\pm$0.23 & -45.4$\pm$0.12 & 7.5$\pm$0.2$^{(0)}$ & 19.1 & -45.7 & 100 & 0.6897\\ 
211087131 & 03 48 55.64 & +24 21 40.5 & 18.38 & 14.22 & 17.4$\pm$2.72 & -51.85$\pm$2.72 & 6.8$\pm$0.9$^{(1)}$ & 19.8 & -45.6 & 100 & 0.1267\\ 
211087357 & 03 47 40.45 & +24 21 52.4 & 10.34 & 8.95 & 17.93$\pm$0.83 & -46.52$\pm$0.77 & 6.8$\pm$0.9$^{(1)}$ & 19.9 & -45.5 & 100 & 3.252\\ 
211087739 & 03 47 30.60 & +24 22 14.0 & 14.63 & 11.36 & 14.48$\pm$2.1 & -53.34$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 19.9 & -45.5 & 98 & 2.7628\\ 
211087985 & 03 46 07.52 & +24 22 27.8 & 13.84 & 10.89 & 20.1$\pm$2.23 & -49.57$\pm$2.23 & 6.5$\pm$0.9$^{(1)}$ & 20.1 & -45.5 & 100 & 5.0781\\ 
211088007 & 03 43 43.24 & +24 22 28.5 &   & 7.56 & 18.0$\pm$1.0 & -43.9$\pm$0.9 & 9.2$\pm$1.3$^{(2)}$ & 20.4 & -45.4 & 100 &  \\ 
211088075 & 03 40 15.92 & +24 22 31.7 & 18.01 & 13.81 & 20.66$\pm$2.71 & -44.51$\pm$2.71 & 6.8$\pm$0.9$^{(1)}$ & 20.7 & -45.2 & 100 & 1.2224\\ 
211088413 & 03 49 21.75 & +24 22 51.4 & 6.64 & 6.65 & 18.76$\pm$0.04 & -45.32$\pm$0.02 & 7.2$\pm$0.5$^{(0)}$ & 19.7 & -45.6 & 100 &  \\ 
211088648 & 03 44 46.14 & +24 23 03.1 & 17.94 & 13.76 & 19.65$\pm$2.79 & -46.91$\pm$2.79 & 6.6$\pm$0.9$^{(1)}$ & 20.2 & -45.4 & 100 & 0.2858\\ 
211088777 & 03 41 38.80 & +24 23 09.5 & 17.46 & 13.43 & 23.62$\pm$2.64 & -47.35$\pm$2.64 & 7.1$\pm$1.0$^{(1)}$ & 20.6 & -45.3 & 100 & 1.5972\\ 
211089068 & 03 47 18.06 & +24 23 26.8 & 12.11 & 9.72 & 16.91$\pm$0.93 & -46.8$\pm$0.93 & 8.9$\pm$1.2$^{(1)}$ & 19.9 & -45.5 & 100 & 9.7733\\ 
211089146 & 03 47 15.45 & +24 23 31.1 & 16.82 & 12.82 & 20.56$\pm$2.85 & -46.93$\pm$2.85 & 9.6$\pm$1.3$^{(1)}$ & 19.9 & -45.5 & 100 & 0.31\\ 
211089267 & 03 47 07.88 & +24 23 37.9 & 17.01 & 13.1 & 28.21$\pm$2.15 & -48.38$\pm$2.15 & 6.8$\pm$0.9$^{(1)}$ & 20.0 & -45.5 & 99 & 3.9054\\ 
211089274 & 03 43 36.92 & +24 23 38.3 & 13.48 & 10.65 & 18.3$\pm$2.18 & -47.03$\pm$2.18 & 6.7$\pm$0.9$^{(1)}$ & 20.4 & -45.4 & 100 & 1.3696\\ 
211089323 & 03 44 25.72 & +24 23 41.0 & 8.13 & 7.47 & 21.12$\pm$0.45 & -48.82$\pm$0.4 & 8.1$\pm$0.3$^{(0)}$ & 20.3 & -45.4 & 100 &  \\ 
211089419 & 03 49 16.80 & +24 23 46.1 & 7.54 & 7.26 & 19.1$\pm$0.42 & -43.77$\pm$0.36 & 7.0$\pm$0.3$^{(0)}$ & 19.7 & -45.6 & 100 & 0.2652\\ 
211089510 & 03 41 22.44 & +24 23 51.9 & 17.39 & 13.35 & 23.01$\pm$2.13 & -52.33$\pm$2.13 & 7.3$\pm$1.0$^{(1)}$ & 20.6 & -45.3 & 100 & 0.3226\\ 
211089916 & 03 49 27.58 & +24 24 13.8 & 16.51 & 12.66 & 18.06$\pm$2.12 & -48.36$\pm$2.12 & 7.4$\pm$1.0$^{(1)}$ & 19.7 & -45.6 & 100 & 0.3888\\ 
211090094 & 03 47 37.65 & +24 24 23.4 & 16.75 & 12.76 & 20.0$\pm$2.6 & -44.57$\pm$2.6 & 9.2$\pm$1.3$^{(1)}$ & 19.9 & -45.5 & 100 & 0.7538\\ 
211090224 & 03 44 26.88 & +24 24 31.7 & 14.84 & 11.48 & 20.05$\pm$2.14 & -46.93$\pm$2.14 & 6.8$\pm$0.9$^{(1)}$ & 20.3 & -45.4 & 100 & 5.8799\\ 
211090866 & 03 45 49.37 & +24 25 07.2 & 15.32 & 11.8 & 17.84$\pm$2.3 & -45.13$\pm$2.23 & 7.0$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 2.4271\\ 
211090906 & 03 53 58.22 & +24 25 09.1 & 18.83 & 14.26 & 22.0$\pm$2.68 & -41.94$\pm$2.68 & 6.8$\pm$0.9$^{(1)}$ & 19.2 & -45.7 & 100 &  \\ 
211090925 & 03 53 40.96 & +24 25 09.8 & 14.92 & 11.58 & 17.34$\pm$2.12 & -43.61$\pm$2.12 & 6.2$\pm$0.9$^{(1)}$ & 19.2 & -45.7 & 100 & 8.5605\\ 
211091381 & 03 43 55.69 & +24 25 35.1 & 13.61 & 10.64 & 18.73$\pm$2.15 & -47.88$\pm$2.15 & 7.6$\pm$1.0$^{(1)}$ & 20.3 & -45.4 & 100 & 4.4858\\ 
211091449 & 03 44 37.77 & +24 25 38.9 & 17.61 & 13.47 & 17.29$\pm$2.23 & -43.63$\pm$2.23 & 6.7$\pm$0.9$^{(1)}$ & 20.3 & -45.4 & 100 & 0.3036\\ 
211091536 & 03 47 49.77 & +24 25 43.4 & 16.49 & 12.67 & 22.0$\pm$2.1 & -48.46$\pm$2.1 & 8.2$\pm$1.1$^{(1)}$ & 19.9 & -45.5 & 100 & 0.8216\\ 
211091768 & 03 44 56.40 & +24 25 57.4 & 10.22 & 8.87 & 18.26$\pm$0.84 & -46.68$\pm$0.84 & 7.2$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 100 & 2.7793\\ 
211091848 & 03 46 28.41 & +24 26 02.2 & 10.78 & 9.16 & 17.61$\pm$0.77 & -45.39$\pm$0.77 & 7.4$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 1.3126\\ 
211092430 & 03 43 20.57 & +24 26 35.1 & 17.16 & 13.25 & 21.24$\pm$2.71 & -47.99$\pm$2.71 & 7.4$\pm$1.0$^{(1)}$ & 20.4 & -45.4 & 100 & 0.3642\\ 
211092628 & 03 44 54.10 & +24 26 47.0 & 16.51 & 12.74 & 17.18$\pm$2.79 & -47.87$\pm$2.79 & 8.0$\pm$1.1$^{(1)}$ & 20.2 & -45.4 & 100 & 0.6325\\ 
211092630 & 03 44 17.75 & +24 26 47.0 & 15.21 & 11.66 & 18.5$\pm$2.14 & -46.62$\pm$2.14 & 7.2$\pm$1.0$^{(1)}$ & 20.3 & -45.4 & 100 & 0.2749\\ 
211093040 & 03 43 26.96 & +24 27 10.1 & 15.12 & 11.47 & 20.98$\pm$2.18 & -46.96$\pm$2.18 & 11.2$\pm$1.6$^{(1)}$ & 20.4 & -45.4 & 100 & 2.1623\\ 
211093117 & 03 46 27.01 & +24 27 14.5 & 15.7 & 12.06 & 21.09$\pm$2.19 & -45.17$\pm$2.19 & 7.6$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 0.9143\\ 
211093202 & 03 48 42.68 & +24 27 19.7 & 17.48 & 13.5 & 19.47$\pm$2.55 & -46.94$\pm$2.55 & 6.9$\pm$0.9$^{(1)}$ & 19.8 & -45.6 & 100 &  \\ 
211093203 & 03 52 17.54 & +24 27 19.7 & 16.35 & 12.47 & 19.2$\pm$2.12 & -43.87$\pm$2.12 & 9.7$\pm$1.3$^{(1)}$ & 19.4 & -45.7 & 100 & 0.5971\\ 
211093429 & 03 47 39.35 & +24 27 32.4 & 15.96 & 12.18 & 22.53$\pm$2.1 & -47.08$\pm$2.1 & 9.4$\pm$1.3$^{(1)}$ & 19.9 & -45.5 & 100 & 0.519\\ 
211093581 & 03 46 58.54 & +24 27 40.1 & 15.85 & 12.16 & 19.03$\pm$2.24 & -55.36$\pm$2.24 & 8.5$\pm$1.2$^{(1)}$ & 20.0 & -45.5 & 98 & 1.1004\\ 
211093684 & 03 49 42.28 & +24 27 46.8 & 11.8 & 9.78 & 17.16$\pm$0.84 & -49.11$\pm$0.84 & 7.6$\pm$1.1$^{(1)}$ & 19.7 & -45.6 & 100 & 7.2745\\ 
211093705 & 03 45 34.46 & +24 27 47.9 & 8.52 & 7.67 & 16.93$\pm$0.9 & -45.14$\pm$0.9 & 8.0$\pm$1.1$^{(1)}$ & 20.1 & -45.4 & 100 & 0.3279\\ 
211093906 & 03 52 43.23 & +24 27 58.7 & 16.65 & 12.93 & 19.85$\pm$2.15 & -51.84$\pm$2.15 & 7.6$\pm$1.0$^{(1)}$ & 19.3 & -45.7 & 100 & 0.6929\\ 
211093928 & 03 46 54.87 & +24 27 60.0 & 18.31 & 14.02 & 18.69$\pm$2.84 & -55.02$\pm$2.84 & 6.5$\pm$0.9$^{(1)}$ & 20.0 & -45.5 & 100 & 0.1212\\ 
211094095 & 03 45 53.78 & +24 28 08.8 & 13.97 & 10.58 & 20.12$\pm$2.12 & -51.43$\pm$2.12 & 10.5$\pm$1.5$^{(1)}$ & 20.1 & -45.5 & 99 & 19.15\\ 
211094384 & 03 45 19.96 & +24 28 24.8 & 16.35 & 12.48 & 21.68$\pm$2.79 & -46.18$\pm$2.79 & 9.4$\pm$1.3$^{(1)}$ & 20.2 & -45.4 & 100 &  \\ 
211094777 & 03 46 24.63 & +24 28 46.5 & 16.3 & 12.57 & 21.58$\pm$2.19 & -47.26$\pm$2.19 & 7.5$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 0.8915\\ 
211095218 & 03 44 26.53 & +24 29 11.6 & 16.12 & 12.1 & 22.87$\pm$2.14 & -46.54$\pm$2.14 & 13.2$\pm$1.8$^{(1)}$ & 20.3 & -45.4 & 98 & 0.347\\ 
211095259 & 03 40 30.72 & +24 29 14.0 & 11.42 & 9.56 & 23.27$\pm$1.46 & -44.39$\pm$0.75 & 7.3$\pm$0.5$^{(0)}$ & 20.7 & -45.3 & 100 & 6.8132\\ 
211095292 & 03 43 43.71 & +24 29 15.8 & 14.97 & 11.46 & 19.52$\pm$2.19 & -48.32$\pm$2.19 & 7.7$\pm$1.1$^{(1)}$ & 20.4 & -45.4 & 100 & 4.005\\ 
211095624 & 03 42 55.11 & +24 29 35.1 & 9.33 & 8.26 & 20.48$\pm$1.01 & -44.83$\pm$0.38 & 7.6$\pm$0.3$^{(0)}$ & 20.4 & -45.4 & 100 & 1.4072\\ 
211096320 & 03 46 24.11 & +24 30 13.1 & 17.94 & 13.86 & 22.11$\pm$2.75 & -47.05$\pm$2.75 & 6.0$\pm$0.8$^{(1)}$ & 20.0 & -45.5 & 100 & 0.1891\\ 
211096368 & 03 44 03.55 & +24 30 15.3 & 10.46 & 8.95 & 22.23$\pm$0.87 & -45.6$\pm$0.33 & 7.5$\pm$0.2$^{(0)}$ & 20.3 & -45.4 & 100 & 1.4758\\ 
211096385 & 03 48 17.29 & +24 30 16.0 & 13.56 & 10.67 & 19.18$\pm$2.08 & -51.02$\pm$2.08 & 7.0$\pm$1.0$^{(1)}$ & 19.8 & -45.6 & 100 & 5.4934\\ 
211096421 & 03 45 12.07 & +24 30 18.4 & 15.49 & 11.92 & 14.77$\pm$2.79 & -49.66$\pm$2.79 & 7.6$\pm$1.0$^{(1)}$ & 20.2 & -45.4 & 100 & 0.3473\\ 
211096432 & 03 47 50.95 & +24 30 18.9 & 14.83 & 11.5 & 16.04$\pm$2.1 & -50.54$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 19.9 & -45.5 & 100 & 1.4175\\ 
211097388 & 03 46 59.40 & +24 31 12.5 & 6.83 & 6.69 & 20.31$\pm$0.06 & -46.61$\pm$0.05 & 7.6$\pm$0.3$^{(0)}$ & 20.0 & -45.5 & 100 & 0.3436\\ 
211097402 & 03 46 38.89 & +24 31 13.1 & 12.74 & 10.29 & 17.17$\pm$2.1 & -47.46$\pm$2.1 & 7.5$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 7.4791\\ 
211097879 & 03 46 02.90 & +24 31 40.4 & 6.46 & 6.43 & 19.63$\pm$0.04 & -44.88$\pm$0.03 & 7.5$\pm$0.6$^{(0)}$ & 20.1 & -45.5 & 100 &  \\ 
211097941 & 03 44 39.63 & +24 31 44.2 & 15.47 & 11.88 & 21.4$\pm$2.14 & -53.08$\pm$2.14 & 8.4$\pm$1.2$^{(1)}$ & 20.2 & -45.4 & 100 & 0.6099\\ 
211098117 & 03 49 27.64 & +24 31 54.2 & 14.71 & 11.21 & 21.41$\pm$2.13 & -46.54$\pm$2.13 & 8.5$\pm$1.2$^{(1)}$ & 19.7 & -45.6 & 100 & 0.543\\ 
211098279 & 03 49 33.03 & +24 32 02.6 & 15.17 & 11.74 & 22.0$\pm$2.08 & -52.45$\pm$2.08 & 6.8$\pm$0.9$^{(1)}$ & 19.7 & -45.6 & 100 & 1.5928\\ 
211098454 & 03 42 03.31 & +24 32 13.5 & 15.07 & 11.61 & 16.99$\pm$2.14 & -46.52$\pm$2.14 & 6.8$\pm$0.9$^{(1)}$ & 20.5 & -45.3 & 100 & 2.2576\\ 
211098750 & 03 41 29.70 & +24 32 26.7 & 14.75 & 11.63 & 22.0$\pm$2.13 & -36.88$\pm$2.13 & 5.0$\pm$0.7$^{(1)}$ & 20.6 & -45.3 & 72 &  \\ 
211098921 & 03 45 21.67 & +24 32 37.4 & 16.05 & 12.36 & 15.97$\pm$2.23 & -48.97$\pm$2.23 & 7.0$\pm$1.0$^{(1)}$ & 20.2 & -45.5 & 100 & 1.1468\\ 
211099232 & 03 43 43.14 & +24 32 56.2 & 17.05 & 13.14 & 16.8$\pm$2.19 & -49.0$\pm$2.19 & 7.3$\pm$1.0$^{(1)}$ & 20.4 & -45.4 & 100 & 0.5793\\ 
211099592 & 03 45 54.48 & +24 33 16.2 & 5.82 & 5.78 & 20.02$\pm$0.05 & -45.95$\pm$0.03 & 7.9$\pm$0.9$^{(0)}$ & 20.1 & -45.5 & 100 &  \\ 
211100131 & 03 46 06.91 & +24 33 46.1 & 12.56 & 10.25 & 22.9$\pm$2.12 & -51.08$\pm$2.12 & 6.5$\pm$0.9$^{(1)}$ & 20.1 & -45.5 & 100 & 7.9101\\ 
211100238 & 03 46 21.36 & +24 33 52.6 & 17.03 & 13.15 & 16.97$\pm$2.75 & -49.11$\pm$2.75 & 7.3$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 0.4397\\ 
211100392 & 03 49 15.39 & +24 34 02.3 & 13.28 & 10.42 & 17.9$\pm$2.13 & -52.65$\pm$2.13 & 7.7$\pm$1.1$^{(1)}$ & 19.7 & -45.6 & 100 & 0.3983\\ 
211100398 & 03 46 06.50 & +24 34 02.7 & 12.3 & 10.11 & 19.35$\pm$0.93 & -47.63$\pm$0.93 & 6.7$\pm$0.9$^{(1)}$ & 20.1 & -45.5 & 100 & 7.0484\\ 
211100565 & 03 46 22.67 & +24 34 12.5 & 10.24 & 8.92 & 18.98$\pm$0.77 & -45.67$\pm$0.77 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -45.5 & 100 & 3.231\\ 
211100748 & 03 43 42.14 & +24 34 23.5 & 14.36 & 10.99 & 20.7$\pm$2.15 & -45.42$\pm$2.15 & 9.8$\pm$1.3$^{(1)}$ & 20.4 & -45.4 & 100 & 1.9343\\ 
211100894 & 03 45 16.65 & +24 34 32.5 & 14.9 & 11.45 & 19.07$\pm$2.12 & -50.24$\pm$2.12 & 8.0$\pm$1.1$^{(1)}$ & 20.2 & -45.5 & 100 & 0.8545\\ 
211100931 & 03 54 52.57 & +24 34 34.5 & 12.47 & 9.83 & 18.28$\pm$2.29 & -47.1$\pm$2.29 & 9.7$\pm$1.3$^{(1)}$ & 19.1 & -45.8 & 100 & 8.798\\ 
211101098 & 03 48 21.53 & +24 34 43.8 & 16.81 & 12.97 & 23.21$\pm$2.08 & -49.08$\pm$2.08 & 8.2$\pm$1.1$^{(1)}$ & 19.8 & -45.6 & 100 & 0.7157\\ 
211101218 & 03 54 00.37 & +24 34 50.0 & 18.25 & 13.9 & 18.21$\pm$2.67 & -46.99$\pm$2.67 & 7.7$\pm$1.1$^{(1)}$ & 19.2 & -45.8 & 100 & 0.2184\\ 
211101564 & 03 45 11.99 & +24 35 10.3 & 13.25 & 10.59 & 16.57$\pm$2.12 & -47.68$\pm$2.12 & 6.5$\pm$0.9$^{(1)}$ & 20.2 & -45.5 & 100 & 4.3894\\ 
211101696 & 03 44 19.06 & +24 35 18.5 & 16.23 & 12.44 & 17.56$\pm$2.14 & -51.15$\pm$2.14 & 8.1$\pm$1.1$^{(1)}$ & 20.3 & -45.4 & 100 & 0.6814\\ 
211101750 & 03 44 09.60 & +24 35 22.4 & 15.68 & 12.12 & 18.53$\pm$2.15 & -50.33$\pm$2.15 & 7.7$\pm$1.1$^{(1)}$ & 20.3 & -45.4 & 100 & 3.8818\\ 
211101761 & 03 44 26.28 & +24 35 23.0 & 11.16 & 9.27 & 19.43$\pm$0.84 & -47.38$\pm$0.84 & 8.4$\pm$1.2$^{(1)}$ & 20.3 & -45.4 & 100 & 0.8374\\ 
211101996 & 03 47 59.37 & +24 35 37.4 & 17.61 & 13.55 & 16.72$\pm$2.55 & -49.3$\pm$2.55 & 6.7$\pm$0.9$^{(1)}$ & 19.9 & -45.6 & 100 & 0.8448\\ 
211102156 & 04 00 25.63 & +24 35 46.6 & 12.23 & 10.4 & 23.66$\pm$2.58 & -55.53$\pm$2.58 & 5.0$\pm$0.7$^{(1)}$ & 18.4 & -46.0 & 37 &  \\ 
211102300 & 03 54 39.12 & +24 35 54.6 & 17.94 & 13.77 & 20.63$\pm$2.1 & -47.44$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 19.1 & -45.8 & 100 & 0.2253\\ 
211102389 & 03 47 38.36 & +24 35 60.0 & 17.42 & 13.47 & 9.42$\pm$2.66 & -47.48$\pm$2.66 & 7.2$\pm$1.0$^{(1)}$ & 19.9 & -45.5 & 95 &  \\ 
211102393 & 03 46 49.21 & +24 36 00.2 & 14.17 & 11.02 & 16.54$\pm$2.16 & -48.01$\pm$2.16 & 7.1$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 7.9111\\ 
211102725 & 03 46 23.03 & +24 36 18.2 & 16.48 & 12.76 & 17.35$\pm$2.16 & -50.66$\pm$2.16 & 6.6$\pm$0.9$^{(1)}$ & 20.0 & -45.5 & 100 & 1.1143\\ 
211103033 & 03 48 40.42 & +24 36 34.3 & 16.09 & 12.39 & 21.94$\pm$2.08 & -49.77$\pm$2.08 & 8.4$\pm$1.2$^{(1)}$ & 19.8 & -45.6 & 100 & 0.8848\\ 
211103222 & 03 46 05.64 & +24 36 44.6 & 14.89 & 11.49 & 26.2$\pm$6.1 & -43.6$\pm$6.1 & 7.4$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 1.1298\\ 
211103325 & 04 16 20.08 & +24 36 50.1 & 13.44 & 10.46 & 19.57$\pm$2.07 & -46.1$\pm$2.07 & 7.8$\pm$1.1$^{(1)}$ & 16.4 & -46.5 & 88 &  \\ 
211103863 & 03 46 11.75 & +24 37 20.4 & 11.32 & 9.55 & 19.3$\pm$0.77 & -46.12$\pm$0.77 & 7.0$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 5.9772\\ 
211103923 & 03 48 44.68 & +24 37 23.7 & 18.35 & 14.12 & 17.72$\pm$2.57 & -50.31$\pm$2.56 & 6.9$\pm$0.9$^{(1)}$ & 19.8 & -45.6 & 100 & 0.3484\\ 
211103969 & 03 48 45.35 & +24 37 26.5 & 17.13 & 13.17 & 18.93$\pm$2.55 & -53.21$\pm$2.55 & 7.6$\pm$1.0$^{(1)}$ & 19.8 & -45.6 & 100 & 0.1238\\ 
211104176 & 03 45 40.18 & +24 37 38.1 & 9.54 & 8.29 & 21.18$\pm$0.88 & -46.96$\pm$0.88 & 8.1$\pm$1.1$^{(1)}$ & 20.1 & -45.5 & 100 & 1.1394\\ 
211104535 & 03 47 45.91 & +24 38 01.5 & 16.52 & 12.59 & 21.49$\pm$2.1 & -53.71$\pm$2.1 & 10.1$\pm$1.4$^{(1)}$ & 19.9 & -45.6 & 98 & 0.2962\\ 
211104722 & 03 49 11.74 & +24 38 11.7 & 10.25 & 8.95 & 19.36$\pm$0.84 & -45.99$\pm$0.84 & 7.2$\pm$1.0$^{(1)}$ & 19.7 & -45.6 & 100 & 4.2628\\ 
211105653 & 03 45 36.73 & +24 39 06.7 & 15.11 & 11.4 & 21.72$\pm$2.18 & -49.82$\pm$2.18 & 13.3$\pm$1.8$^{(1)}$ & 20.1 & -45.5 & 97 & 0.3334\\ 
211105839 & 03 43 13.07 & +24 39 19.6 & 14.71 & 11.28 & 20.34$\pm$2.14 & -48.2$\pm$2.24 & 8.0$\pm$1.1$^{(1)}$ & 20.4 & -45.4 & 100 & 0.2562\\ 
211105906 & 03 43 29.88 & +24 39 23.7 & 17.38 & 13.45 & 21.32$\pm$2.71 & -50.01$\pm$2.71 & 6.9$\pm$1.0$^{(1)}$ & 20.4 & -45.4 & 100 & 0.7217\\ 
211106344 & 03 52 02.26 & +24 39 47.7 & 11.53 & 9.07 & 17.52$\pm$0.9 & -47.0$\pm$0.9 & 13.7$\pm$1.9$^{(1)}$ & 19.4 & -45.7 & 97 & 0.2931\\ 
211106429 & 03 42 21.55 & +24 39 52.8 & 13.68 & 10.71 & 20.99$\pm$2.18 & -46.45$\pm$2.18 & 7.1$\pm$1.0$^{(1)}$ & 20.5 & -45.4 & 100 & 2.9794\\ 
211106535 & 03 51 59.32 & +24 39 59.1 & 15.62 & 12.08 & 18.75$\pm$2.1 & -50.49$\pm$2.1 & 6.9$\pm$1.0$^{(1)}$ & 19.4 & -45.7 & 100 & 0.9618\\ 
211106636 & 03 51 58.82 & +24 40 04.6 & 15.43 & 11.92 & 13.42$\pm$2.1 & -46.81$\pm$2.1 & 6.7$\pm$0.9$^{(1)}$ & 19.4 & -45.7 & 100 & 0.3363\\ 
211106743 & 03 43 02.94 & +24 40 11.1 & 11.59 & 9.73 & 19.27$\pm$0.77 & -46.39$\pm$0.42 & 7.7$\pm$0.5$^{(0)}$ & 20.4 & -45.4 & 100 & 6.6874\\ 
211106969 & 03 46 09.90 & +24 40 25.1 & 14.06 & 10.62 & 17.73$\pm$2.18 & -54.12$\pm$2.18 & 11.4$\pm$1.6$^{(1)}$ & 20.1 & -45.5 & 88 & 1.9819\\ 
211107114 & 03 46 08.69 & +24 40 33.3 & 16.53 & 12.71 & 21.0$\pm$2.18 & -51.86$\pm$2.18 & 8.7$\pm$1.2$^{(1)}$ & 20.1 & -45.5 & 100 & 1.986\\ 
211107116 & 03 47 28.42 & +24 40 33.3 & 16.57 & 12.88 & 21.26$\pm$2.24 & -50.91$\pm$2.18 & 6.2$\pm$0.9$^{(1)}$ & 19.9 & -45.5 & 100 & 0.9834\\ 
211107267 & 03 45 06.55 & +24 40 43.0 & 17.45 & 13.32 & 19.79$\pm$2.12 & -50.18$\pm$2.12 & 8.4$\pm$1.2$^{(1)}$ & 20.2 & -45.5 & 100 & $<$2\\ 
211107439 & 03 44 25.59 & +24 40 52.8 & 15.26 & 11.62 & 20.55$\pm$2.14 & -51.69$\pm$2.14 & 8.8$\pm$1.2$^{(1)}$ & 20.3 & -45.4 & 100 & 1.08\\ 
211107623 & 03 47 33.68 & +24 41 03.1 & 12.44 & 10.13 & 17.99$\pm$2.16 & -48.58$\pm$2.16 & 7.8$\pm$1.1$^{(1)}$ & 19.9 & -45.6 & 100 & 8.5982\\ 
211107734 & 03 46 17.94 & +24 41 09.7 & 15.12 & 11.69 & 18.67$\pm$2.18 & -46.32$\pm$2.18 & 6.9$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 5.5174\\ 
211108136 & 03 43 09.75 & +24 41 33.1 & 14.94 & 11.42 & 20.19$\pm$2.14 & -47.37$\pm$2.14 & 9.1$\pm$1.3$^{(1)}$ & 20.4 & -45.4 & 100 & 2.0256\\ 
211108263 & 03 49 21.24 & +24 41 41.1 & 17.52 & 13.53 & 23.17$\pm$2.65 & -50.79$\pm$2.65 & 6.7$\pm$0.9$^{(1)}$ & 19.7 & -45.6 & 100 & 0.4433\\ 
211109330 & 03 54 25.03 & +24 42 43.7 & 16.97 & 12.76 & 21.03$\pm$2.67 & -47.86$\pm$2.67 & 11.2$\pm$1.5$^{(1)}$ & 19.1 & -45.8 & 99 & 0.1772\\ 
211109574 & 03 52 53.48 & +24 42 56.6 & 9.31 & 8.26 & 18.68$\pm$0.26 & -44.95$\pm$0.06 & 10.1$\pm$1.7$^{(0)}$ & 19.3 & -45.7 & 100 & $<$2\\ 
211110500 & 03 47 59.74 & +24 43 52.7 & 12.78 & 10.16 & 17.75$\pm$2.08 & -52.03$\pm$2.08 & 8.4$\pm$1.2$^{(1)}$ & 19.9 & -45.6 & 100 & 0.7364\\ 
211110672 & 04 01 55.85 & +24 44 02.6 & 16.15 & 12.35 & 17.21$\pm$2.07 & -41.41$\pm$2.07 & 9.5$\pm$1.3$^{(1)}$ & 18.2 & -46.1 & 98 & 0.5678\\ 
211111400 & 03 43 12.12 & +24 44 45.3 & 15.45 & 11.67 & 19.78$\pm$2.14 & -47.14$\pm$2.14 & 12.7$\pm$1.8$^{(1)}$ & 20.4 & -45.4 & 99 & 0.7068\\ 
211111496 & 03 46 37.77 & +24 44 51.7 & 11.49 & 9.67 & 20.26$\pm$0.84 & -49.05$\pm$0.84 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -45.5 & 100 & 7.1797\\ 
211111611 & 03 46 44.78 & +24 44 58.6 & 17.29 & 13.32 & 18.77$\pm$2.6 & -46.34$\pm$2.6 & 7.2$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 1.3443\\ 
211111670 & 04 15 44.88 & +24 45 02.5 & 12.96 & 10.19 & 17.49$\pm$2.07 & -42.78$\pm$2.07 & 8.5$\pm$1.2$^{(1)}$ & 16.5 & -46.5 & 79 &  \\ 
211112171 & 03 46 28.63 & +24 45 32.4 & 13.56 & 10.66 & 18.58$\pm$2.1 & -50.38$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.0 & -45.5 & 100 & 9.1276\\ 
211112685 & 03 44 21.90 & +24 46 06.3 & 12.44 & 10.07 & 20.22$\pm$2.14 & -51.02$\pm$2.14 & 7.6$\pm$1.1$^{(1)}$ & 20.3 & -45.4 & 100 & 0.4114\\ 
211112686 & 03 44 24.81 & +24 46 06.3 & 14.28 & 11.0 & 16.49$\pm$2.14 & -50.06$\pm$2.14 & 7.8$\pm$1.1$^{(1)}$ & 20.3 & -45.4 & 100 & 0.7643\\ 
211112974 & 03 44 20.51 & +24 46 22.3 & 10.76 & 8.87 & 20.75$\pm$0.85 & -46.15$\pm$0.84 & 9.7$\pm$1.3$^{(1)}$ & 20.3 & -45.4 & 100 & 1.1868\\ 
211113202 & 03 49 20.60 & +24 46 36.0 & 12.33 & 9.93 & 18.64$\pm$0.93 & -46.87$\pm$0.93 & 9.1$\pm$1.3$^{(1)}$ & 19.7 & -45.6 & 100 & 0.5603\\ 
211113286 & 03 45 01.13 & +24 46 41.2 & 16.37 & 12.58 & 24.09$\pm$2.12 & -51.6$\pm$2.12 & 8.9$\pm$1.2$^{(1)}$ & 20.2 & -45.5 & 100 & 0.5888\\ 
211113345 & 03 44 13.92 & +24 46 45.8 & 10.53 & 9.06 & 20.41$\pm$0.72 & -45.03$\pm$0.34 & 7.4$\pm$0.2$^{(0)}$ & 20.3 & -45.4 & 100 & 4.0255\\ 
211113696 & 03 46 20.48 & +24 47 07.8 & 13.21 & 10.5 & 18.64$\pm$2.1 & -49.43$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 20.1 & -45.5 & 100 & 6.3758\\ 
211114317 & 03 44 20.09 & +24 47 46.2 & 10.41 & 8.9 & 19.69$\pm$0.7 & -46.19$\pm$0.34 & 7.7$\pm$0.3$^{(0)}$ & 20.3 & -45.4 & 100 & 1.4729\\ 
211114329 & 03 46 54.92 & +24 47 46.9 & 10.35 & 8.98 & 17.23$\pm$1.76 & -46.6$\pm$0.31 & 8.1$\pm$0.5$^{(0)}$ & 20.0 & -45.5 & 100 & 3.3705\\ 
211115160 & 03 56 57.07 & +24 48 34.6 & 14.72 & 11.23 & 16.18$\pm$2.1 & -44.12$\pm$2.1 & 8.3$\pm$1.1$^{(1)}$ & 18.8 & -45.9 & 100 &  \\ 
211115321 & 03 44 10.95 & +24 48 46.0 & 16.86 & 12.96 & 15.0$\pm$2.14 & -46.42$\pm$2.14 & 6.6$\pm$0.9$^{(1)}$ & 20.3 & -45.4 & 100 & 0.4745\\ 
211115421 & 04 00 14.10 & +24 48 51.8 & 16.18 & 12.68 & 15.89$\pm$2.07 & -47.96$\pm$2.07 & 4.6$\pm$0.6$^{(1)}$ & 18.4 & -46.0 & 72 &  \\ 
211115457 & 03 48 22.81 & +24 48 53.6 & 15.57 & 12.03 & 20.72$\pm$2.08 & -50.89$\pm$2.08 & 6.5$\pm$0.9$^{(1)}$ & 19.8 & -45.6 & 100 & 1.7216\\ 
211115638 & 03 44 40.75 & +24 49 06.7 & 9.69 & 8.51 & 20.4$\pm$0.77 & -45.1$\pm$0.4 & 7.5$\pm$0.3$^{(0)}$ & 20.2 & -45.5 & 100 & 1.908\\ 
211115713 & 03 47 38.05 & +24 49 11.2 & 15.21 & 11.7 & 20.56$\pm$2.1 & -45.74$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 19.9 & -45.6 & 100 & 2.3229\\ 
211115721 & 03 47 03.55 & +24 49 11.7 & 8.3 & 7.33 & 21.74$\pm$0.34 & -39.65$\pm$0.34 & 10.4$\pm$1.4$^{(1)}$ & 20.0 & -45.6 & 90 & 1.228\\ 
211116507 & 03 56 23.50 & +24 49 56.7 & 13.31 & 10.55 & 17.05$\pm$2.1 & -43.99$\pm$2.1 & 7.1$\pm$1.0$^{(1)}$ & 18.9 & -45.9 & 100 & 3.3228\\ 
211116917 & 03 48 39.30 & +24 50 20.2 &   & 13.5 & 32.8$\pm$3.9 & -53.1$\pm$3.9 & 11.7$\pm$1.6$^{(4)}$ & 19.8 & -45.6 & 42 & 0.2656\\ 
211116936 & 03 45 09.74 & +24 50 21.3 & 5.71 & 5.81 & 20.4$\pm$0.05 & -45.96$\pm$0.04 & 8.0$\pm$0.4$^{(0)}$ & 20.2 & -45.5 & 100 &  \\ 
211117077 & 03 43 52.15 & +24 50 29.8 & 13.61 & 10.6 & 19.4$\pm$2.15 & -48.4$\pm$2.15 & 7.8$\pm$1.1$^{(1)}$ & 20.3 & -45.4 & 100 & 3.0034\\ 
211117230 & 03 44 27.30 & +24 50 38.3 & 13.13 & 10.02 & 19.16$\pm$2.18 & -50.98$\pm$2.18 & 10.8$\pm$1.5$^{(1)}$ & 20.3 & -45.5 & 99 & 0.3982\\ 
211117529 & 03 47 22.98 & +24 50 56.4 & 15.42 & 11.83 & 22.41$\pm$2.1 & -50.23$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 19.9 & -45.6 & 100 & 0.9252\\ 
211117626 & 03 45 23.49 & +24 51 02.9 & 14.29 & 11.04 & 19.75$\pm$2.18 & -47.69$\pm$2.18 & 7.7$\pm$1.1$^{(1)}$ & 20.2 & -45.5 & 100 & 1.2481\\ 
211118251 & 03 53 24.76 & +24 51 43.0 & 12.1 & 10.15 & 23.18$\pm$2.12 & -37.33$\pm$2.12 & 6.1$\pm$0.8$^{(1)}$ & 19.2 & -45.8 & 90 &  \\ 
211118414 & 03 44 24.73 & +24 51 53.1 & 15.73 & 11.95 & 19.95$\pm$2.18 & -51.69$\pm$2.18 & 9.6$\pm$1.3$^{(1)}$ & 20.3 & -45.5 & 100 & 0.2177\\ 
211118542 & 03 46 07.78 & +24 52 00.7 & 11.77 & 9.36 & 21.4$\pm$0.84 & -40.49$\pm$0.84 & 12.0$\pm$1.7$^{(1)}$ & 20.1 & -45.5 & 92 & 6.9551\\ 
211118985 & 03 47 35.85 & +24 52 26.9 & 16.72 & 12.8 & 21.11$\pm$2.1 & -45.05$\pm$2.1 & 8.3$\pm$1.2$^{(1)}$ & 19.9 & -45.6 & 100 & 0.2084\\ 
211119314 & 03 46 59.47 & +24 52 46.4 & 16.36 & 12.31 & 19.99$\pm$2.15 & -51.74$\pm$2.15 & 13.0$\pm$1.8$^{(1)}$ & 20.0 & -45.6 & 94 & 0.3409\\ 
211119678 & 03 45 24.13 & +24 53 09.5 & 9.52 & 8.42 & 20.06$\pm$0.55 & -45.11$\pm$0.3 & 7.6$\pm$0.3$^{(0)}$ & 20.2 & -45.5 & 100 & 1.8128\\ 
211119999 & 03 47 38.08 & +24 53 30.7 & 13.54 & 10.6 & 22.29$\pm$2.1 & -46.47$\pm$2.1 & 7.3$\pm$1.0$^{(1)}$ & 19.9 & -45.6 & 100 & 0.582\\ 
211120561 & 03 52 59.14 & +24 54 05.5 & 13.6 & 10.71 & 17.81$\pm$2.15 & -46.86$\pm$2.15 & 6.6$\pm$0.9$^{(1)}$ & 19.3 & -45.8 & 100 & 2.4861\\ 
211120664 & 03 49 00.97 & +24 54 10.4 & 15.5 & 11.88 & 24.77$\pm$2.13 & -53.33$\pm$2.13 & 9.2$\pm$1.3$^{(1)}$ & 19.7 & -45.6 & 99 & 1.4972\\ 
211120842 & 03 45 42.12 & +24 54 21.6 & 9.31 & 7.94 & 19.83$\pm$0.58 & -49.15$\pm$0.68 & 11.5$\pm$1.6$^{(1)}$ & 20.1 & -45.5 & 99 & 1.5775\\ 
211121141 & 03 44 50.18 & +24 54 40.1 & 12.85 & 10.29 & 19.49$\pm$2.12 & -50.87$\pm$2.12 & 7.8$\pm$1.1$^{(1)}$ & 20.2 & -45.5 & 100 & 5.6763\\ 
211121734 & 03 45 20.86 & +24 55 19.4 & 8.9 & 7.84 & 20.09$\pm$0.68 & -43.33$\pm$0.42 & 7.1$\pm$0.3$^{(0)}$ & 20.2 & -45.5 & 100 & 7.0681\\ 
211122237 & 03 46 40.26 & +24 55 51.9 & 13.23 & 10.34 & 17.09$\pm$2.1 & -46.05$\pm$2.1 & 8.2$\pm$1.1$^{(1)}$ & 20.0 & -45.6 & 100 & 5.1665\\ 
211123901 & 03 46 38.77 & +24 57 34.7 & 10.05 & 8.76 & 20.16$\pm$0.8 & -46.76$\pm$0.35 & 7.5$\pm$0.2$^{(0)}$ & 20.0 & -45.6 & 100 & 2.3141\\ 
211125179 & 03 47 01.00 & +24 58 57.5 & 16.25 & 12.28 & 14.61$\pm$2.15 & -47.93$\pm$2.15 & 11.8$\pm$1.6$^{(1)}$ & 20.0 & -45.6 & 95 & 0.3484\\ 
211125210 & 03 51 40.45 & +24 58 59.5 & 10.64 & 9.14 & 20.45$\pm$1.57 & -46.93$\pm$0.29 & 6.9$\pm$0.4$^{(0)}$ & 19.4 & -45.7 & 100 & 3.3701\\ 
211125236 & 03 46 19.85 & +24 59 01.6 & 16.12 & 12.01 & 22.53$\pm$2.16 & -54.83$\pm$2.16 & 16.2$\pm$2.2$^{(1)}$ & 20.1 & -45.6 & 16 & 0.6783\\ 
211125240 & 03 47 41.50 & +24 59 01.8 &   & 13.21 & 11.7$\pm$3.8 & -32.0$\pm$3.8 & 5.3$\pm$0.7$^{(4)}$ & 19.9 & -45.6 & 11 &  \\ 
211126627 & 03 48 42.15 & +25 00 28.5 & 15.29 & 11.72 & 18.3$\pm$2.08 & -49.04$\pm$2.08 & 8.4$\pm$1.2$^{(1)}$ & 19.8 & -45.6 & 100 & 0.3368\\ 
211127164 & 03 52 35.31 & +25 01 04.8 & 16.85 & 12.72 & 20.19$\pm$2.67 & -45.72$\pm$2.67 & 11.1$\pm$1.5$^{(1)}$ & 19.3 & -45.8 & 99 & 0.5157\\ 
211127297 & 03 52 03.58 & +25 01 14.0 & 16.78 & 12.97 & 19.39$\pm$2.1 & -50.41$\pm$2.1 & 7.0$\pm$1.0$^{(1)}$ & 19.4 & -45.8 & 100 & 0.6317\\ 
211127395 & 03 48 40.59 & +25 01 20.2 & 17.9 & 13.61 & 19.72$\pm$2.55 & -46.64$\pm$2.55 & 7.6$\pm$1.1$^{(1)}$ & 19.8 & -45.6 & 100 & 0.7565\\ 
211127537 & 03 52 01.64 & +25 01 29.5 & 16.34 & 12.65 & 20.02$\pm$2.1 & -50.89$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 19.4 & -45.8 & 100 & 0.7129\\ 
211127791 & 03 48 08.82 & +25 01 45.8 & 14.83 & 11.25 & 11.68$\pm$2.08 & -42.2$\pm$2.08 & 8.8$\pm$1.2$^{(1)}$ & 19.8 & -45.6 & 93 &  \\ 
211127799 & 04 00 15.85 & +25 01 46.5 & 15.28 & 11.69 & 15.2$\pm$2.07 & -42.66$\pm$2.07 & 8.2$\pm$1.1$^{(1)}$ & 18.4 & -46.1 & 100 & 2.7078\\ 
211128116 & 03 53 24.49 & +25 02 07.2 & 16.43 & 12.55 & 18.96$\pm$2.12 & -48.79$\pm$2.12 & 9.8$\pm$1.3$^{(1)}$ & 19.2 & -45.8 & 100 & 0.6341\\ 
211128863 & 03 48 17.70 & +25 02 52.3 & 10.73 & 9.16 & 17.38$\pm$0.83 & -48.02$\pm$0.83 & 7.6$\pm$1.1$^{(1)}$ & 19.8 & -45.6 & 100 & 4.5347\\ 
211128979 & 03 54 46.37 & +25 02 59.5 & 17.78 & 13.34 & 18.3$\pm$3.6 & -51.9$\pm$3.6 & 11.7$\pm$1.6$^{(1)}$ & 19.1 & -45.9 & 97 & 0.4016\\ 
211129308 & 03 51 02.31 & +25 03 19.7 & 12.75 & 10.37 & 14.65$\pm$2.06 & -38.08$\pm$2.06 & 7.5$\pm$1.0$^{(1)}$ & 19.5 & -45.7 & 96 & 5.7885\\ 
211129321 & 03 59 06.30 & +25 03 20.2 & 15.16 & 11.46 & 17.13$\pm$2.1 & -46.2$\pm$2.1 & 9.4$\pm$1.3$^{(1)}$ & 18.5 & -46.0 & 100 & 0.7786\\ 
211129400 & 03 45 42.45 & +25 03 25.5 & 12.9 & 10.5 & 12.56$\pm$2.18 & -39.62$\pm$2.18 & 6.3$\pm$0.9$^{(1)}$ & 20.1 & -45.5 & 95 & 2.8396\\ 
211129571 & 03 56 11.38 & +25 03 36.8 & 18.9 & 14.23 & 19.73$\pm$2.73 & -37.31$\pm$2.73 & 6.9$\pm$1.0$^{(1)}$ & 18.9 & -45.9 & 98 & 0.8741\\ 
211130173 & 03 53 05.12 & +25 04 15.7 &   & 13.85 & 14.7$\pm$4.7 & -38.9$\pm$4.7 & 14.6$\pm$2.0$^{(4)}$ & 19.3 & -45.8 & 49 & 0.4744\\ 
211131087 & 03 47 20.83 & +25 05 12.4 & 14.49 & 11.14 & 16.45$\pm$2.19 & -48.56$\pm$2.19 & 7.3$\pm$1.0$^{(1)}$ & 19.9 & -45.6 & 100 & 3.694\\ 
211131748 & 03 51 23.89 & +25 05 52.9 & 15.2 & 11.77 & 21.69$\pm$2.1 & -47.64$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 19.5 & -45.8 & 100 & 4.391\\ 
211132111 & 03 52 02.63 & +25 06 15.1 & 16.7 & 12.84 & 20.96$\pm$2.1 & -45.06$\pm$2.1 & 9.2$\pm$1.3$^{(1)}$ & 19.4 & -45.8 & 100 & 0.5099\\ 
211132233 & 03 48 44.04 & +25 06 22.7 & 16.44 & 12.62 & 18.75$\pm$2.12 & -49.62$\pm$2.12 & 8.7$\pm$1.2$^{(1)}$ & 19.8 & -45.7 & 100 & 0.5\\ 
211132306 & 03 58 13.92 & +25 06 27.5 & 15.0 & 11.41 & 9.36$\pm$2.1 & -52.56$\pm$2.1 & 8.7$\pm$1.2$^{(1)}$ & 18.7 & -46.0 & 26 &  \\ 
211132712 & 03 47 15.29 & +25 06 55.5 & 15.2 & 11.48 & 18.56$\pm$2.19 & -44.81$\pm$2.19 & 11.4$\pm$1.6$^{(1)}$ & 19.9 & -45.6 & 99 & 1.1254\\ 
211133821 & 03 46 27.35 & +25 08 07.9 & 10.34 & 8.99 & 21.5$\pm$0.81 & -45.65$\pm$0.44 & 7.4$\pm$0.2$^{(0)}$ & 20.0 & -45.6 & 100 & 3.4241\\ 
211134185 & 03 47 25.76 & +25 08 33.3 & 15.23 & 11.45 & 20.24$\pm$2.6 & -49.77$\pm$2.6 & 12.9$\pm$1.8$^{(1)}$ & 19.9 & -45.6 & 97 & 0.1357\\ 
211135624 & 03 56 52.31 & +25 10 05.4 & 18.25 & 13.98 & 19.01$\pm$2.71 & -46.37$\pm$2.71 & 7.7$\pm$1.1$^{(1)}$ & 18.8 & -46.0 & 100 &  \\ 
211136223 & 03 52 42.19 & +25 10 42.4 & 17.7 & 13.76 & 20.08$\pm$2.7 & -47.75$\pm$2.7 & 6.2$\pm$0.9$^{(1)}$ & 19.3 & -45.8 & 100 &  \\ 
211137863 & 03 54 47.99 & +25 12 30.5 & 14.77 & 11.76 & 24.72$\pm$2.12 & -43.71$\pm$2.12 & 4.8$\pm$0.7$^{(1)}$ & 19.1 & -45.9 & 67 &  \\ 
211138217 & 03 48 16.88 & +25 12 54.5 & 9.07 & 7.86 & 15.72$\pm$0.7 & -44.82$\pm$0.54 & 7.6$\pm$0.3$^{(0)}$ & 19.8 & -45.7 & 100 & 6.7219\\ 
211138781 & 03 47 47.85 & +25 13 34.5 & 16.1 & 12.09 & 18.29$\pm$2.12 & -48.61$\pm$2.11 & 12.9$\pm$1.8$^{(1)}$ & 19.9 & -45.6 & 97 & 0.6111\\ 
211139534 & 03 54 58.03 & +25 14 29.4 & 15.58 & 11.98 & 20.2$\pm$2.1 & -48.3$\pm$2.1 & 6.8$\pm$0.9$^{(1)}$ & 19.0 & -45.9 & 100 & 1.182\\ 
211139647 & 03 48 15.48 & +25 14 36.7 & 16.88 & 12.99 & 18.33$\pm$2.08 & -44.99$\pm$2.08 & 6.6$\pm$0.9$^{(1)}$ & 19.8 & -45.7 & 100 & 0.4809\\ 
211139723 & 03 48 26.04 & +25 14 41.0 & 14.32 & 11.09 & 19.9$\pm$2.08 & -52.46$\pm$2.08 & 7.6$\pm$1.0$^{(1)}$ & 19.8 & -45.7 & 100 & 1.634\\ 
211139797 & 03 46 54.03 & +25 14 45.0 & 14.87 & 11.49 & 18.24$\pm$2.15 & -45.78$\pm$2.15 & 6.7$\pm$0.9$^{(1)}$ & 20.0 & -45.6 & 100 & 2.6922\\ 
211140155 & 03 52 31.36 & +25 15 07.6 & 15.41 & 11.91 & 20.21$\pm$2.12 & -48.38$\pm$2.12 & 6.8$\pm$0.9$^{(1)}$ & 19.3 & -45.8 & 100 & 1.2294\\ 
211140995 & 03 57 40.66 & +25 16 04.4 & 15.28 & 11.82 & 16.23$\pm$2.1 & -43.84$\pm$2.1 & 6.3$\pm$0.9$^{(1)}$ & 18.7 & -46.0 & 100 & 1.4233\\ 
211141632 & 03 57 30.15 & +25 16 47.0 & 14.91 & 11.61 & 16.05$\pm$2.1 & -37.51$\pm$2.1 & 5.8$\pm$0.8$^{(1)}$ & 18.7 & -46.0 & 89 & 2.6829\\ 
211141637 & 03 52 45.35 & +25 16 47.5 & 13.11 & 10.52 & 18.2$\pm$2.15 & -46.03$\pm$2.15 & 7.4$\pm$1.0$^{(1)}$ & 19.3 & -45.8 & 100 & 5.0017\\ 
211142460 & 03 52 54.24 & +25 17 43.5 & 16.16 & 12.46 & 18.17$\pm$2.15 & -45.44$\pm$2.15 & 7.4$\pm$1.0$^{(1)}$ & 19.3 & -45.8 & 100 &  \\ 
211142685 & 03 55 56.40 & +25 18 00.1 & 15.33 & 11.72 & 15.99$\pm$2.62 & -40.33$\pm$2.62 & 7.8$\pm$1.1$^{(1)}$ & 18.9 & -45.9 & 99 & 2.4597\\ 
211142730 & 03 53 07.47 & +25 18 03.6 & 17.93 & 13.59 & 11.15$\pm$2.7 & -33.84$\pm$2.7 & 8.2$\pm$1.1$^{(1)}$ & 19.3 & -45.8 & 11 &  \\ 
211143325 & 03 54 11.48 & +25 18 43.0 & 16.61 & 12.72 & 20.35$\pm$2.12 & -47.48$\pm$2.12 & 8.5$\pm$1.2$^{(1)}$ & 19.1 & -45.9 & 100 & 0.4729\\ 
211143504 & 03 48 07.67 & +25 18 55.1 & 13.17 & 10.34 & 17.0$\pm$2.08 & -47.82$\pm$2.08 & 8.1$\pm$1.1$^{(1)}$ & 19.8 & -45.7 & 100 & 0.446\\ 
211143760 & 04 01 59.57 & +25 19 12.6 & 18.26 & 14.22 & 16.52$\pm$2.61 & -45.24$\pm$2.61 & 4.5$\pm$0.6$^{(1)}$ & 18.2 & -46.2 & 48 &  \\ 
211147023 & 03 50 17.67 & +25 22 46.5 & 9.48 & 8.38 & 19.4$\pm$1.01 & -45.89$\pm$0.5 & 7.4$\pm$0.3$^{(0)}$ & 19.6 & -45.8 & 100 & 1.857\\ 
211147344 & 03 57 42.97 & +25 23 07.0 & 16.36 & 12.57 & 18.18$\pm$2.1 & -47.33$\pm$2.1 & 8.2$\pm$1.1$^{(1)}$ & 18.7 & -46.0 & 100 & 0.5421\\ 
211147423 & 03 51 13.85 & +25 23 11.6 & 15.6 & 11.97 & 16.59$\pm$2.1 & -49.51$\pm$2.1 & 7.8$\pm$1.1$^{(1)}$ & 19.5 & -45.8 & 100 & 0.5336\\ 
211147822 & 03 50 39.30 & +25 23 37.5 & 11.89 & 9.43 & 21.54$\pm$2.28 & -47.7$\pm$2.28 & 10.7$\pm$1.5$^{(1)}$ & 19.6 & -45.8 & 100 & 0.5789\\ 
211149193 & 04 01 45.90 & +25 25 09.9 & 16.37 & 12.5 & 14.3$\pm$2.07 & -39.75$\pm$2.07 & 7.0$\pm$1.0$^{(1)}$ & 18.2 & -46.2 & 97 &  \\ 
211149525 & 03 50 14.75 & +25 25 30.2 & 16.76 & 12.92 & 18.86$\pm$2.06 & -52.2$\pm$2.06 & 7.8$\pm$1.1$^{(1)}$ & 19.6 & -45.8 & 100 & 0.6652\\ 
211149600 & 03 50 35.72 & +25 25 35.4 & 11.62 & 9.58 & 17.52$\pm$0.85 & -44.38$\pm$0.85 & 7.2$\pm$1.0$^{(1)}$ & 19.6 & -45.8 & 100 & 0.3144\\ 
211150258 & 03 52 58.77 & +25 26 19.4 & 17.31 & 13.33 & 18.7$\pm$2.15 & -45.89$\pm$2.15 & 7.1$\pm$1.0$^{(1)}$ & 19.3 & -45.9 & 100 & 0.1714\\ 
211151674 & 03 52 07.95 & +25 27 54.8 & 17.26 & 13.27 & 15.68$\pm$2.1 & -47.94$\pm$2.1 & 7.7$\pm$1.1$^{(1)}$ & 19.4 & -45.8 & 100 & 0.4606\\ 
211152884 & 03 56 15.79 & +25 29 15.6 & 16.86 & 12.68 & 21.21$\pm$2.1 & -50.51$\pm$2.1 & 12.3$\pm$1.7$^{(1)}$ & 18.9 & -46.0 & 96 & 0.4688\\ 
211154974 & 03 54 46.52 & +25 31 35.2 & 16.93 & 12.68 & 18.84$\pm$2.12 & -50.61$\pm$2.12 & 13.1$\pm$1.8$^{(1)}$ & 19.1 & -45.9 & 93 & 0.7217\\ 
211156183 & 03 50 08.41 & +25 32 56.1 & 16.1 & 12.38 & 18.89$\pm$2.08 & -48.66$\pm$2.08 & 8.6$\pm$1.2$^{(1)}$ & 19.6 & -45.8 & 100 & 1.7487\\ 
211158092 & 03 50 56.61 & +25 35 06.6 & 15.26 & 11.58 & 18.19$\pm$2.04 & -50.89$\pm$2.04 & 10.7$\pm$1.5$^{(1)}$ & 19.5 & -45.8 & 99 & 2.0791\\ 
211158590 & 03 51 06.34 & +25 35 40.9 & 8.98 & 8.01 & 20.23$\pm$0.92 & -45.43$\pm$0.49 & 7.4$\pm$0.2$^{(0)}$ & 19.5 & -45.8 & 100 &  \\ 
211161968 & 03 50 41.19 & +25 39 30.8 & 17.35 & 13.28 & 19.7$\pm$2.06 & -50.86$\pm$2.06 & 8.0$\pm$1.1$^{(1)}$ & 19.5 & -45.8 & 100 & 0.3277\\ 
211162249 & 03 59 55.91 & +25 39 51.1 & 15.67 & 12.07 & 21.09$\pm$2.58 & -58.42$\pm$2.58 & 8.5$\pm$1.2$^{(1)}$ & 18.4 & -46.1 & 79 &  \\ 
211163008 & 03 54 33.60 & +25 40 43.8 & 13.67 & 10.37 & 13.51$\pm$2.12 & -45.29$\pm$2.12 & 10.9$\pm$1.5$^{(1)}$ & 19.1 & -45.9 & 96 & 0.6658\\ 
211168863 & 03 53 07.28 & +25 47 21.7 & 17.4 & 13.3 & 18.3$\pm$2.7 & -49.15$\pm$2.7 & 7.7$\pm$1.1$^{(1)}$ & 19.3 & -45.9 & 100 & 0.2923\\ 
211171449 & 03 52 38.91 & +25 50 25.7 & 16.01 & 12.22 & 20.01$\pm$2.12 & -47.42$\pm$2.12 & 9.2$\pm$1.3$^{(1)}$ & 19.3 & -45.9 & 100 & 1.057\\ 
211177579 & 03 53 50.26 & +25 57 52.7 & 10.84 & 9.3 & 18.09$\pm$1.45 & -39.23$\pm$0.55 & 6.0$\pm$0.4$^{(0)}$ & 19.2 & -46.0 & 91 & 3.2972\\ 
\enddata 
 \tablecomments{stuff} 
 \label{Plmemtab} 
 \end{deluxetable} 


==> Pr_memtable.tex <==
\begin{deluxetable}{cccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Candidate Praesepe members.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} \\ } 
 \startdata 
211681193 & 08 30 17.11 & +15 39 45.0 & 17.74 & 13.91 & -31.95$\pm$2.18 & -10.07$\pm$2.18 & 5.2$\pm$0.7$^{(1)}$ & -34.6 & -10.5 & 28 & 1.63\\ 
211707676 & 08 40 54.43 & +16 01 00.8 & 18.83 & 14.32 & -27.62$\pm$3.0 & -12.64$\pm$3.0 & 5.9$\pm$0.8$^{(1)}$ & -36.6 & -10.3 & 27 & 0.31\\ 
211708110 & 08 36 37.35 & +16 01 20.5 & 17.86 & 13.88 & -34.13$\pm$2.18 & -13.81$\pm$2.18 & 5.7$\pm$0.8$^{(1)}$ & -35.8 & -10.5 & 90 &  \\ 
211709792 & 08 42 36.98 & +16 02 44.1 & 17.76 & 13.66 & -31.65$\pm$2.27 & -6.99$\pm$2.27 & 6.6$\pm$0.9$^{(1)}$ & -36.9 & -10.2 & 55 & 1.32\\ 
211711533 & 08 37 24.50 & +16 04 08.9 & 18.42 & 14.26 & -35.46$\pm$2.74 & -13.64$\pm$2.74 & 4.6$\pm$0.6$^{(1)}$ & -35.9 & -10.4 & 90 & 1.75\\ 
211716023 & 08 49 48.36 & +16 07 51.5 & 12.19 & 10.44 & -34.89$\pm$0.77 & -9.81$\pm$0.77 & 4.7$\pm$0.7$^{(1)}$ & -38.1 & -9.9 & 69 & 13.6\\ 
211725787 & 08 33 11.69 & +16 15 51.4 & 18.29 & 14.24 & -32.68$\pm$2.69 & -9.84$\pm$2.69 & 4.7$\pm$0.7$^{(1)}$ & -35.2 & -10.8 & 85 & 2.06\\ 
211727975 & 08 39 58.63 & +16 17 46.4 & 18.09 & 14.18 & -27.94$\pm$2.22 & -9.94$\pm$2.22 & 5.0$\pm$0.7$^{(1)}$ & -36.4 & -10.5 & 41 & 0.91\\ 
211729756 & 08 30 35.16 & +16 19 17.6 & 15.96 & 12.54 & -31.47$\pm$2.16 & -10.93$\pm$2.16 & 5.2$\pm$0.7$^{(1)}$ & -34.7 & -10.9 & 76 & 2.39\\ 
211734093 & 08 36 32.56 & +16 23 02.4 & 14.46 & 11.51 & -26.75$\pm$2.18 & -11.23$\pm$2.18 & 5.1$\pm$0.7$^{(1)}$ & -35.8 & -10.7 & 25 & 18.22\\ 
211737793 & 08 37 42.10 & +16 26 07.9 & 17.92 & 14.02 & -26.29$\pm$2.67 & -12.43$\pm$2.67 & 5.1$\pm$0.7$^{(1)}$ & -36.0 & -10.7 & 30 & 1.44\\ 
211746191 & 08 27 11.23 & +16 33 15.6 & 12.73 & 10.67 & -32.41$\pm$0.73 & -10.83$\pm$0.73 & 4.7$\pm$0.7$^{(1)}$ & -34.1 & -11.2 & 68 &  \\ 
211746226 & 08 27 16.76 & +16 33 17.9 & 15.97 & 12.55 & -30.22$\pm$2.16 & -13.72$\pm$2.16 & 4.6$\pm$0.6$^{(1)}$ & -34.1 & -11.2 & 20 &  \\ 
211748286 & 08 31 07.59 & +16 35 04.1 & 16.48 & 12.62 & -39.08$\pm$2.18 & -14.3$\pm$2.18 & 8.3$\pm$1.1$^{(1)}$ & -34.8 & -11.1 & 22 & 9.02\\ 
211750366 & 08 41 00.78 & +16 36 47.9 & 11.02 & 9.33 & -37.67$\pm$0.93 & -7.78$\pm$0.88 & 7.4$\pm$1.0$^{(1)}$ & -36.6 & -10.7 & 91 &  \\ 
211752612 & 08 25 33.85 & +16 38 40.8 & 17.29 & 13.58 & -33.78$\pm$2.16 & -10.14$\pm$2.16 & 4.5$\pm$0.6$^{(1)}$ & -33.8 & -11.4 & 23 & 0.59\\ 
211759361 & 08 30 04.51 & +16 44 22.2 & 12.5 & 10.69 & -26.75$\pm$2.18 & -8.48$\pm$2.18 & 4.9$\pm$0.7$^{(1)}$ & -34.6 & -11.2 & 12 &  \\ 
211760513 & 08 44 50.89 & +16 45 19.4 & 18.21 & 14.36 & -37.16$\pm$2.74 & -20.74$\pm$2.74 & 4.2$\pm$0.6$^{(1)}$ & -37.2 & -10.6 & 23 &  \\ 
211760567 & 08 35 43.43 & +16 45 21.5 & 16.94 & 13.14 & -36.91$\pm$2.19 & -10.01$\pm$2.19 & 6.1$\pm$0.8$^{(1)}$ & -35.6 & -11.0 & 99 & 13.79\\ 
211768266 & 08 26 39.37 & +16 51 52.9 & 12.68 & 10.74 & -33.01$\pm$2.21 & -10.09$\pm$2.21 & 4.6$\pm$0.6$^{(1)}$ & -34.0 & -11.5 & 54 & 12.12\\ 
211771577 & 08 48 17.26 & +16 54 47.5 & 13.03 & 10.6 & -36.46$\pm$2.08 & -9.42$\pm$2.08 & 5.7$\pm$0.8$^{(1)}$ & -37.8 & -10.5 & 98 & 11.05\\ 
211771942 & 08 26 13.41 & +16 55 05.7 & 12.82 & 10.68 & -36.14$\pm$2.21 & -9.87$\pm$2.21 & 5.0$\pm$0.7$^{(1)}$ & -33.9 & -11.5 & 57 & 12.22\\ 
211773459 & 08 48 32.71 & +16 56 23.6 & 14.71 & 11.47 & -37.29$\pm$2.08 & -8.99$\pm$2.08 & 6.5$\pm$0.9$^{(1)}$ & -37.9 & -10.5 & 97 & 5.94\\ 
211774168 & 08 41 39.14 & +16 56 57.4 & 14.94 & 12.03 & -31.6$\pm$2.24 & -3.14$\pm$2.24 & 4.1$\pm$0.6$^{(1)}$ & -36.7 & -10.9 & 11 &  \\ 
211774926 & 08 37 32.02 & +16 57 35.7 & 16.72 & 13.09 & -38.44$\pm$2.21 & -7.48$\pm$2.21 & 5.4$\pm$0.8$^{(1)}$ & -36.0 & -11.1 & 99 & 1.9\\ 
211775403 & 08 44 53.17 & +16 58 01.1 & 17.41 & 13.68 & -27.73$\pm$2.7 & -11.58$\pm$2.69 & 4.7$\pm$0.6$^{(1)}$ & -37.3 & -10.7 & 52 &  \\ 
211776073 & 08 38 24.87 & +16 58 36.3 & 15.7 & 12.35 & -36.55$\pm$2.21 & -9.73$\pm$2.21 & 4.7$\pm$0.7$^{(1)}$ & -36.1 & -11.0 & 100 & 23.12\\ 
211776951 & 08 53 30.63 & +16 59 18.7 & 9.34 & 8.5 & -37.31$\pm$1.17 & -9.16$\pm$0.79 & 5.8$\pm$0.4$^{(0)}$ & -38.7 & -10.3 & 86 &  \\ 
211781289 & 08 38 07.73 & +17 03 02.4 & 9.64 & 8.7 & -35.87$\pm$1.19 & -10.65$\pm$0.59 & 5.5$\pm$0.4$^{(0)}$ & -36.1 & -11.1 & 100 & 6.31\\ 
211781646 & 08 41 17.79 & +17 03 20.6 & 17.12 & 13.25 & -41.5$\pm$2.24 & -12.43$\pm$2.24 & 7.1$\pm$1.0$^{(1)}$ & -36.6 & -10.9 & 98 & 1.34\\ 
211787610 & 08 30 55.78 & +17 08 22.7 & 15.93 & 12.46 & -39.11$\pm$2.21 & -7.86$\pm$2.21 & 4.8$\pm$0.7$^{(1)}$ & -34.8 & -11.5 & 87 & 18.55\\ 
211788820 & 08 43 46.54 & +17 09 24.3 & 12.38 & 10.35 & -37.29$\pm$0.98 & -6.28$\pm$0.92 & 5.6$\pm$0.8$^{(1)}$ & -37.1 & -10.9 & 93 & 11.93\\ 
211789309 & 08 45 01.74 & +17 09 50.4 & 12.5 & 10.89 & -42.18$\pm$1.58 & -13.72$\pm$1.36 & 3.5$\pm$0.5$^{(1)}$ & -37.3 & -10.8 & 16 &  \\ 
211790121 & 08 39 56.63 & +17 10 33.6 & 19.27 & 14.84 & -38.42$\pm$2.91 & -9.53$\pm$2.91 & 5.0$\pm$0.7$^{(1)}$ & -36.4 & -11.1 & 100 & 0.64\\ 
211795051 & 08 42 28.05 & +17 14 48.5 & 16.65 & 13.11 & -35.8$\pm$2.24 & -10.92$\pm$2.24 & 4.3$\pm$0.6$^{(1)}$ & -36.8 & -11.0 & 100 & 14.59\\ 
211795467 & 08 38 55.66 & +17 15 09.6 & 16.22 & 12.71 & -35.74$\pm$2.19 & -11.46$\pm$2.19 & 4.3$\pm$0.6$^{(1)}$ & -36.2 & -11.2 & 100 & 15.49\\ 
211795569 & 08 38 13.64 & +17 15 15.8 & 13.84 & 11.31 & -46.59$\pm$2.21 & -16.33$\pm$2.21 & 4.2$\pm$0.6$^{(1)}$ & -36.1 & -11.2 & 23 & 24.44\\ 
211795614 & 08 37 49.11 & +17 15 18.0 & 14.34 & 11.39 & -37.29$\pm$2.21 & -15.52$\pm$2.21 & 5.1$\pm$0.7$^{(1)}$ & -36.0 & -11.2 & 100 & 15.99\\ 
211795706 & 08 38 04.53 & +17 15 23.4 & 18.76 & 14.52 & -33.68$\pm$2.75 & -8.11$\pm$2.75 & 4.3$\pm$0.6$^{(1)}$ & -36.1 & -11.2 & 98 & 1.14\\ 
211796017 & 08 26 33.30 & +17 15 39.0 & 15.68 & 12.28 & -38.45$\pm$2.21 & -8.93$\pm$2.21 & 5.1$\pm$0.7$^{(1)}$ & -34.0 & -11.8 & 52 & 32.68\\ 
211799258 & 08 32 59.08 & +17 18 23.6 & 15.7 & 12.18 & -38.97$\pm$2.21 & -14.33$\pm$2.21 & 6.7$\pm$0.9$^{(1)}$ & -35.1 & -11.5 & 98 & 24.24\\ 
211799551 & 08 38 07.11 & +17 18 38.1 & 14.92 & 11.81 & -40.34$\pm$2.21 & -12.53$\pm$2.21 & 4.9$\pm$0.7$^{(1)}$ & -36.1 & -11.3 & 100 & 18.55\\ 
211800408 & 08 27 06.78 & +17 19 21.3 & 14.29 & 11.44 & -34.83$\pm$2.21 & -8.91$\pm$2.21 & 4.6$\pm$0.6$^{(1)}$ & -34.1 & -11.8 & 74 & 16.89\\ 
211801146 & 08 37 22.85 & +17 19 59.7 & 17.65 & 13.54 & -37.02$\pm$3.44 & -8.94$\pm$2.92 & 7.2$\pm$1.0$^{(1)}$ & -35.9 & -11.3 & 99 & 0.26\\ 
211803674 & 08 40 00.06 & +17 22 06.0 & 18.02 & 14.06 & -34.02$\pm$2.64 & -9.51$\pm$2.64 & 4.8$\pm$0.7$^{(1)}$ & -36.4 & -11.2 & 100 & 1.19\\ 
211803698 & 08 43 10.43 & +17 22 07.2 & 13.43 & 10.5 & -32.55$\pm$1.03 & -13.96$\pm$1.02 & 7.6$\pm$1.1$^{(1)}$ & -37.0 & -11.1 & 87 &  \\ 
211804579 & 08 36 16.27 & +17 22 54.0 & 11.24 & 9.86 & -32.89$\pm$0.86 & -9.41$\pm$0.85 & 4.6$\pm$0.6$^{(1)}$ & -35.7 & -11.4 & 100 &  \\ 
211805435 & 08 38 32.88 & +17 23 38.0 & 17.75 & 14.02 & -37.91$\pm$2.19 & -10.84$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.1 & -11.3 & 100 & 0.68\\ 
211807213 & 08 43 50.42 & +17 25 07.8 & 17.9 & 13.92 & -36.24$\pm$2.28 & -13.13$\pm$2.28 & 5.6$\pm$0.8$^{(1)}$ & -37.1 & -11.1 & 100 & 0.61\\ 
211810140 & 08 41 14.91 & +17 27 36.6 & 17.8 & 13.95 & -36.47$\pm$2.79 & -10.97$\pm$2.79 & 4.8$\pm$0.7$^{(1)}$ & -36.6 & -11.2 & 100 & 1.42\\ 
211810283 & 08 39 16.74 & +17 27 44.7 & 11.43 & 9.97 & -33.44$\pm$1.08 & -11.69$\pm$1.08 & 4.5$\pm$0.6$^{(1)}$ & -36.3 & -11.3 & 100 &  \\ 
211810915 & 08 30 38.65 & +17 28 19.4 & 14.97 & 11.82 & -38.06$\pm$2.18 & -13.52$\pm$2.18 & 5.1$\pm$0.7$^{(1)}$ & -34.7 & -11.7 & 99 & 19.52\\ 
211812724 & 08 38 39.15 & +17 29 48.6 & 17.91 & 13.96 & -37.23$\pm$2.17 & -14.0$\pm$2.17 & 4.6$\pm$0.6$^{(1)}$ & -36.2 & -11.4 & 100 & 0.61\\ 
211815893 & 08 48 17.47 & +17 32 26.7 & 13.24 & 10.84 & -45.4$\pm$2.08 & -13.24$\pm$2.08 & 5.0$\pm$0.7$^{(1)}$ & -37.8 & -10.9 & 92 & 35.8\\ 
211815922 & 08 41 05.78 & +17 32 28.2 & 15.61 & 12.16 & -41.71$\pm$2.24 & -7.42$\pm$2.24 & 5.3$\pm$0.7$^{(1)}$ & -36.6 & -11.3 & 99 & $<$2\\ 
211817992 & 08 41 09.26 & +17 34 17.0 & 17.8 & 13.86 & -33.82$\pm$2.24 & -14.4$\pm$2.24 & 5.8$\pm$0.8$^{(1)}$ & -36.6 & -11.3 & 100 & 2.18\\ 
211820823 & 08 25 13.74 & +17 36 45.4 & 18.11 & 14.23 & -35.65$\pm$2.66 & -15.03$\pm$2.66 & 4.4$\pm$0.6$^{(1)}$ & -33.7 & -12.1 & 51 & 1.14\\ 
211822797 & 08 41 38.49 & +17 38 24.0 & 14.36 & 11.43 & -37.36$\pm$2.24 & -11.32$\pm$2.24 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -11.3 & 100 & 14.66\\ 
211822895 & 08 42 49.95 & +17 38 28.8 & 19.05 & 14.79 & -33.45$\pm$3.06 & -3.11$\pm$3.06 & 4.9$\pm$0.7$^{(1)}$ & -36.9 & -11.3 & 95 & 19.91\\ 
211823898 & 08 43 51.78 & +17 39 20.2 & 16.72 & 13.2 & -34.94$\pm$2.17 & -9.76$\pm$2.17 & 3.8$\pm$0.5$^{(1)}$ & -37.1 & -11.2 & 97 & 31.65\\ 
211826149 & 08 37 22.84 & +17 41 15.3 & 16.81 & 13.1 & -33.73$\pm$2.17 & -6.77$\pm$2.17 & 6.4$\pm$0.9$^{(1)}$ & -35.9 & -11.6 & 99 & 7.21\\ 
211827123 & 08 36 59.07 & +17 42 06.3 & 18.62 & 14.72 & -35.83$\pm$2.76 & -9.67$\pm$2.76 & 4.1$\pm$0.6$^{(1)}$ & -35.9 & -11.6 & 99 & 0.43\\ 
211827220 & 08 29 17.81 & +17 42 11.5 & 15.69 & 12.1 & -34.33$\pm$2.21 & -17.32$\pm$2.21 & 6.9$\pm$1.0$^{(1)}$ & -34.5 & -12.0 & 84 & 12.22\\ 
211827466 & 08 51 33.91 & +17 42 24.4 & 18.07 & 14.18 & -33.22$\pm$2.58 & -13.0$\pm$2.58 & 5.5$\pm$0.8$^{(1)}$ & -38.4 & -10.9 & 91 & 1.14\\ 
211827577 & 08 43 14.67 & +17 42 30.2 & 17.47 & 13.61 & -34.67$\pm$2.17 & -11.68$\pm$2.17 & 5.1$\pm$0.7$^{(1)}$ & -37.0 & -11.3 & 100 & 1.42\\ 
211827807 & 08 33 06.98 & +17 42 42.2 & 17.15 & 13.34 & -27.7$\pm$2.21 & -18.53$\pm$2.21 & 6.3$\pm$0.9$^{(1)}$ & -35.2 & -11.8 & 29 &  \\ 
211828967 & 08 48 32.00 & +17 43 41.9 & 17.15 & 13.36 & -39.03$\pm$2.09 & -7.65$\pm$2.08 & 5.3$\pm$0.7$^{(1)}$ & -37.9 & -11.0 & 99 & 1.13\\ 
211829936 & 08 53 04.39 & +17 44 31.1 & 16.64 & 12.86 & -40.07$\pm$3.74 & -6.61$\pm$3.73 & 6.2$\pm$0.9$^{(1)}$ & -38.7 & -10.8 & 82 & 24.44\\ 
211832848 & 08 38 07.16 & +17 46 56.7 & 15.51 & 12.12 & -37.27$\pm$2.17 & -11.71$\pm$2.17 & 5.5$\pm$0.8$^{(1)}$ & -36.1 & -11.6 & 100 & 0.9\\ 
211833336 & 08 39 37.04 & +17 47 19.9 & 14.58 & 11.6 & -37.21$\pm$2.17 & -9.47$\pm$2.17 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -11.5 & 100 & 16.89\\ 
211834355 & 08 41 26.15 & +17 48 12.7 & 16.37 & 12.77 & -35.35$\pm$2.24 & -12.89$\pm$2.24 & 5.3$\pm$0.7$^{(1)}$ & -36.6 & -11.5 & 100 & 21.32\\ 
211835162 & 08 41 01.76 & +17 48 51.6 & 17.36 & 13.51 & -34.93$\pm$2.24 & -20.81$\pm$2.24 & 4.5$\pm$0.6$^{(1)}$ & -36.6 & -11.5 & 83 & 1.31\\ 
211838068 & 08 39 01.85 & +17 51 20.8 & 14.89 & 11.77 & -37.59$\pm$2.17 & -13.18$\pm$2.17 & 4.9$\pm$0.7$^{(1)}$ & -36.2 & -11.6 & 100 &  \\ 
211839847 & 08 36 12.04 & +17 52 46.7 & 17.41 & 13.55 & -35.9$\pm$2.2 & -11.9$\pm$2.2 & 5.1$\pm$0.7$^{(1)}$ & -35.7 & -11.8 & 100 & 1.25\\ 
211841501 & 08 44 11.96 & +17 54 07.9 & 9.78 & 8.78 & -34.83$\pm$1.29 & -11.88$\pm$0.76 & 5.2$\pm$0.4$^{(0)}$ & -37.1 & -11.4 & 100 & 1.88\\ 
211841807 & 08 38 39.96 & +17 54 21.0 & 17.71 & 13.94 & -39.94$\pm$2.17 & -10.14$\pm$2.17 & 4.4$\pm$0.6$^{(1)}$ & -36.2 & -11.7 & 100 & 2.01\\ 
211841991 & 08 43 43.07 & +17 54 29.9 & 14.27 & 11.3 & -36.45$\pm$2.24 & -11.85$\pm$2.23 & 5.2$\pm$0.7$^{(1)}$ & -37.0 & -11.4 & 100 & 15.18\\ 
211842439 & 08 36 27.82 & +17 54 53.5 & 10.61 & 9.4 & -37.96$\pm$2.23 & -14.01$\pm$1.07 & 5.3$\pm$0.7$^{(0)}$ & -35.8 & -11.8 & 100 & 7.67\\ 
211843786 & 08 38 40.29 & +17 55 59.5 & 18.7 & 14.54 & -38.91$\pm$4.0 & -10.47$\pm$4.0 & 4.5$\pm$0.6$^{(1)}$ & -36.2 & -11.7 & 100 & 0.7\\ 
211844142 & 08 38 43.41 & +17 56 16.8 & 18.03 & 14.09 & -26.23$\pm$2.7 & -18.23$\pm$2.71 & 4.6$\pm$0.6$^{(1)}$ & -36.2 & -11.7 & 50 &  \\ 
211845034 & 08 40 36.26 & +17 57 00.4 & 16.22 & 12.58 & -36.98$\pm$2.17 & -11.2$\pm$2.17 & 6.1$\pm$0.8$^{(1)}$ & -36.5 & -11.6 & 100 & 1.33\\ 
211845069 & 08 30 02.94 & +17 57 02.1 & 17.73 & 13.72 & -26.03$\pm$2.71 & -14.55$\pm$2.71 & 6.5$\pm$0.9$^{(1)}$ & -34.6 & -12.1 & 64 & 1.33\\ 
211846954 & 08 36 00.47 & +17 58 33.3 & 15.34 & 12.0 & -36.97$\pm$2.19 & -12.25$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -35.7 & -11.8 & 100 & 0.91\\ 
211847321 & 08 39 30.66 & +17 58 51.3 & 17.28 & 13.51 & -38.06$\pm$2.17 & -13.81$\pm$2.17 & 4.7$\pm$0.6$^{(1)}$ & -36.3 & -11.7 & 100 & 0.56\\ 
211847798 & 08 42 17.54 & +17 59 14.8 & 16.47 & 12.83 & -36.84$\pm$2.19 & -9.62$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -36.8 & -11.5 & 100 & 19.02\\ 
211851325 & 08 32 44.81 & +18 02 10.1 & 15.3 & 11.75 & -42.47$\pm$2.24 & -10.48$\pm$2.24 & 7.7$\pm$1.1$^{(1)}$ & -35.1 & -12.0 & 83 & 1.17\\ 
211852745 & 08 31 47.19 & +18 03 22.5 & 17.7 & 13.85 & -42.0$\pm$2.24 & -15.66$\pm$2.24 & 3.7$\pm$0.5$^{(1)}$ & -34.9 & -12.1 & 40 &  \\ 
211880808 & 08 54 05.00 & +18 26 51.1 & 17.81 & 13.91 & -39.27$\pm$2.6 & -16.45$\pm$2.6 & 5.7$\pm$0.8$^{(1)}$ & -38.8 & -11.2 & 90 & 2.5\\ 
211884968 & 08 32 53.10 & +18 30 29.3 & 15.56 & 12.27 & -37.7$\pm$2.24 & -13.33$\pm$2.24 & 4.8$\pm$0.7$^{(1)}$ & -35.1 & -12.4 & 100 & 22.27\\ 
211885995 & 08 49 26.77 & +18 31 19.6 & 14.44 & 11.39 & -37.13$\pm$2.1 & -14.32$\pm$2.1 & 5.8$\pm$0.8$^{(1)}$ & -38.0 & -11.5 & 100 & 9.16\\ 
211886612 & 08 43 12.93 & +18 31 50.9 & 15.66 & 12.28 & -40.05$\pm$2.19 & -13.89$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -37.0 & -11.9 & 100 & 17.37\\ 
211887287 & 08 42 38.31 & +18 32 27.9 & 19.0 & 14.78 & -38.64$\pm$2.95 & -10.61$\pm$2.95 & 4.4$\pm$0.6$^{(1)}$ & -36.9 & -11.9 & 100 & 0.56\\ 
211887567 & 08 36 23.28 & +18 32 42.3 & 19.09 & 14.71 & -27.22$\pm$2.94 & -10.05$\pm$2.94 & 4.4$\pm$0.6$^{(1)}$ & -35.8 & -12.2 & 96 & 1.74\\ 
211887839 & 08 43 31.05 & +18 32 54.7 & 13.31 & 10.74 & -40.91$\pm$2.19 & -13.22$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -37.0 & -11.8 & 100 & 12.9\\ 
211888866 & 08 29 43.42 & +18 33 48.2 & 19.07 & 14.96 & -38.66$\pm$2.99 & -16.53$\pm$2.99 & 4.1$\pm$0.6$^{(1)}$ & -34.5 & -12.5 & 96 & 17.08\\ 
211889082 & 08 29 57.06 & +18 34 00.0 & 14.49 & 11.3 & -35.75$\pm$2.24 & -14.53$\pm$2.24 & 6.8$\pm$0.9$^{(1)}$ & -34.6 & -12.5 & 99 & 12.37\\ 
211889983 & 08 36 47.11 & +18 34 46.9 & 12.39 & 10.59 & -34.44$\pm$2.19 & -10.43$\pm$2.19 & 4.5$\pm$0.6$^{(1)}$ & -35.8 & -12.2 & 100 & 9.54\\ 
211890182 & 08 45 40.89 & +18 34 57.4 & 18.0 & 14.08 & -32.34$\pm$2.61 & -17.13$\pm$2.61 & 5.2$\pm$0.7$^{(1)}$ & -37.4 & -11.8 & 99 & 2.34\\ 
211890216 & 08 40 55.31 & +18 34 59.0 & 13.78 & 11.13 & -37.1$\pm$2.19 & -17.22$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.6 & -12.0 & 100 & 12.57\\ 
211890774 & 08 42 32.06 & +18 35 28.1 & 14.95 & 11.79 & -34.8$\pm$2.19 & -13.91$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -36.8 & -11.9 & 100 & 9.42\\ 
211891321 & 08 45 36.86 & +18 35 55.3 & 15.75 & 12.06 & -33.77$\pm$2.08 & -16.56$\pm$2.08 & 7.7$\pm$1.1$^{(1)}$ & -37.4 & -11.8 & 97 & 1.07\\ 
211891359 & 08 44 36.14 & +18 35 57.1 & 13.57 & 10.66 & -38.43$\pm$2.19 & -10.69$\pm$2.19 & 7.2$\pm$1.0$^{(1)}$ & -37.2 & -11.8 & 100 & 12.84\\ 
211891774 & 08 47 48.86 & +18 36 19.6 & 16.52 & 12.77 & -36.81$\pm$2.1 & -14.16$\pm$2.1 & 7.2$\pm$1.0$^{(1)}$ & -37.8 & -11.7 & 100 & 0.59\\ 
211891950 & 08 30 14.52 & +18 36 29.2 & 18.13 & 14.18 & -37.77$\pm$2.82 & -25.26$\pm$2.82 & 5.6$\pm$0.8$^{(1)}$ & -34.6 & -12.5 & 28 & $<$2\\ 
211891961 & 08 40 17.07 & +18 36 29.8 & 17.1 & 13.35 & -36.06$\pm$2.19 & -12.31$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.4 & -12.1 & 100 & 1.59\\ 
211892153 & 08 38 21.66 & +18 36 39.9 & 12.61 & 10.18 & -33.33$\pm$2.23 & -10.06$\pm$2.23 & 6.6$\pm$0.9$^{(1)}$ & -36.1 & -12.2 & 100 & 27.09\\ 
211892173 & 08 37 36.81 & +18 36 40.7 & 18.41 & 14.13 & -34.26$\pm$4.21 & -12.39$\pm$4.21 & 6.0$\pm$0.8$^{(1)}$ & -36.0 & -12.2 & 100 & 0.49\\ 
211892240 & 08 48 22.53 & +18 36 44.7 & 15.66 & 12.32 & -35.92$\pm$2.11 & -8.87$\pm$2.11 & 4.9$\pm$0.7$^{(1)}$ & -37.9 & -11.6 & 100 & 21.32\\ 
211892510 & 08 39 40.60 & +18 36 58.8 & 16.88 & 13.0 & -34.6$\pm$2.19 & -12.64$\pm$2.19 & 6.8$\pm$0.9$^{(1)}$ & -36.3 & -12.1 & 100 & 1.42\\ 
211892816 & 08 41 03.34 & +18 37 15.9 & 19.29 & 14.36 & -31.32$\pm$2.89 & -24.62$\pm$2.88 & 5.3$\pm$0.7$^{(1)}$ & -36.6 & -12.0 & 55 & 0.42\\ 
211892842 & 08 42 07.32 & +18 37 16.9 & 18.88 & 14.71 & -28.29$\pm$3.11 & -13.59$\pm$3.11 & 4.7$\pm$0.7$^{(1)}$ & -36.8 & -12.0 & 99 &  \\ 
211892898 & 08 43 34.63 & +18 37 19.9 & 11.7 & 9.6 & -36.35$\pm$2.27 & -7.27$\pm$2.27 & 7.8$\pm$1.1$^{(1)}$ & -37.0 & -11.9 & 99 & 8.51\\ 
211893704 & 08 40 19.21 & +18 38 02.5 & 18.44 & 14.3 & -37.69$\pm$2.87 & -13.3$\pm$2.87 & 6.0$\pm$0.8$^{(1)}$ & -36.5 & -12.1 & 100 & 0.78\\ 
211894087 & 08 39 19.37 & +18 38 22.4 & 18.85 & 14.53 & -36.71$\pm$2.81 & -16.46$\pm$2.81 & 4.3$\pm$0.6$^{(1)}$ & -36.3 & -12.1 & 100 & 1.16\\ 
211895099 & 08 37 33.08 & +18 39 15.5 & 10.47 & 9.28 & -37.44$\pm$2.12 & -12.23$\pm$0.99 & 5.2$\pm$0.6$^{(0)}$ & -36.0 & -12.2 & 100 & 7.31\\ 
211895966 & 08 37 03.75 & +18 40 02.5 & 13.45 & 10.89 & -36.77$\pm$2.19 & -14.73$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.9 & -12.3 & 100 & 14.73\\ 
211896120 & 08 41 32.36 & +18 40 10.8 & 16.43 & 12.92 & -33.16$\pm$2.19 & -11.41$\pm$2.19 & 4.3$\pm$0.6$^{(1)}$ & -36.7 & -12.0 & 100 &  \\ 
211896450 & 08 40 58.66 & +18 40 30.2 & 13.08 & 10.49 & -37.62$\pm$2.19 & -14.17$\pm$2.19 & 6.5$\pm$0.9$^{(1)}$ & -36.6 & -12.1 & 100 & 12.47\\ 
211896596 & 08 48 01.74 & +18 40 37.6 & 10.19 & 8.81 & -37.94$\pm$0.23 & -11.95$\pm$0.12 & 5.3$\pm$0.2$^{(0)}$ & -37.8 & -11.7 & 100 & 2.97\\ 
211896670 & 08 32 48.78 & +18 40 40.8 & 16.19 & 12.47 & -34.96$\pm$2.24 & -14.13$\pm$2.24 & 6.7$\pm$0.9$^{(1)}$ & -35.1 & -12.5 & 100 & 6.96\\ 
211896749 & 08 43 23.93 & +18 40 45.2 & 15.41 & 12.16 & -34.24$\pm$2.19 & -14.17$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -37.0 & -11.9 & 100 & 21.17\\ 
211896805 & 08 39 36.16 & +18 40 49.0 & 17.99 & 13.89 & -32.82$\pm$2.19 & -10.75$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.3 & -12.1 & 100 & 0.96\\ 
211896912 & 08 36 50.53 & +18 40 54.1 & 17.1 & 13.34 & -34.76$\pm$2.19 & -14.54$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -35.8 & -12.3 & 100 & 13.98\\ 
211896957 & 08 31 26.91 & +18 40 56.5 & 17.66 & 13.32 & -32.92$\pm$2.81 & -9.21$\pm$2.78 & 9.3$\pm$1.3$^{(1)}$ & -34.9 & -12.5 & 89 & 0.24\\ 
211896979 & 08 33 02.89 & +18 40 57.5 & 12.86 & 10.68 & -35.42$\pm$2.24 & -14.95$\pm$2.24 & 5.1$\pm$0.7$^{(1)}$ & -35.1 & -12.5 & 100 & 13.3\\ 
211897054 & 08 42 12.72 & +18 41 01.1 & 17.25 & 13.56 & -34.94$\pm$2.19 & -14.34$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.8 & -12.0 & 100 & 3.21\\ 
211897713 & 08 37 29.41 & +18 41 35.6 & 16.64 & 13.15 & -34.01$\pm$2.23 & -18.84$\pm$2.23 & 3.9$\pm$0.5$^{(1)}$ & -35.9 & -12.3 & 96 & 28.91\\ 
211897821 & 08 30 58.93 & +18 41 41.2 & 14.54 & 11.59 & -33.3$\pm$2.24 & -13.09$\pm$2.24 & 4.7$\pm$0.7$^{(1)}$ & -34.8 & -12.6 & 100 & 16.42\\ 
211897893 & 08 43 12.05 & +18 41 45.1 & 17.85 & 14.03 & -39.54$\pm$2.69 & -12.32$\pm$2.69 & 4.8$\pm$0.7$^{(1)}$ & -37.0 & -12.0 & 100 & 0.4\\ 
211897926 & 08 31 50.93 & +18 41 47.2 & 12.63 & 10.71 & -42.38$\pm$2.24 & -20.14$\pm$2.24 & 4.5$\pm$0.6$^{(1)}$ & -34.9 & -12.5 & 73 & 24.24\\ 
211898294 & 08 32 49.71 & +18 42 06.3 & 12.26 & 10.06 & -35.29$\pm$2.24 & -11.39$\pm$2.24 & 7.0$\pm$1.0$^{(1)}$ & -35.1 & -12.5 & 100 & 18.11\\ 
211898716 & 08 35 40.15 & +18 42 28.4 & 16.02 & 12.36 & -36.23$\pm$2.19 & -13.06$\pm$2.19 & 6.5$\pm$0.9$^{(1)}$ & -35.6 & -12.4 & 100 & 1.97\\ 
211899094 & 08 45 25.71 & +18 42 48.1 & 12.47 & 10.44 & -40.14$\pm$2.14 & -10.83$\pm$2.14 & 5.3$\pm$0.7$^{(1)}$ & -37.3 & -11.9 & 100 & 12.37\\ 
211899790 & 08 45 36.88 & +18 43 25.1 & 17.48 & 13.68 & -34.77$\pm$2.08 & -12.35$\pm$2.08 & 5.2$\pm$0.7$^{(1)}$ & -37.4 & -11.9 & 100 & 1.83\\ 
211899994 & 08 33 28.21 & +18 43 36.3 & 17.84 & 14.02 & -36.98$\pm$2.77 & -16.58$\pm$2.77 & 5.2$\pm$0.7$^{(1)}$ & -35.2 & -12.5 & 100 & 1.63\\ 
211900414 & 08 32 55.66 & +18 43 58.2 & 12.64 & 10.6 & -36.84$\pm$2.24 & -13.12$\pm$2.24 & 4.9$\pm$0.7$^{(1)}$ & -35.1 & -12.5 & 100 & 10.93\\ 
211900619 & 08 36 12.07 & +18 44 07.8 & 16.73 & 12.96 & -36.39$\pm$2.2 & -15.5$\pm$2.19 & 7.5$\pm$1.0$^{(1)}$ & -35.7 & -12.3 & 100 & 1.7\\ 
211900653 & 08 32 35.25 & +18 44 09.6 & 17.87 & 13.95 & -34.38$\pm$2.24 & -24.55$\pm$2.24 & 5.6$\pm$0.8$^{(1)}$ & -35.1 & -12.5 & 14 &  \\ 
211900700 & 08 44 17.07 & +18 44 11.8 & 11.98 & 10.26 & -35.93$\pm$0.9 & -12.12$\pm$0.9 & 4.9$\pm$0.7$^{(1)}$ & -37.1 & -11.9 & 100 & 11.01\\ 
211900943 & 08 32 07.96 & +18 44 26.7 & 16.08 & 12.57 & -30.04$\pm$2.24 & -12.72$\pm$2.24 & 4.6$\pm$0.6$^{(1)}$ & -35.0 & -12.5 & 99 & 27.58\\ 
211900989 & 08 50 41.62 & +18 44 29.2 &   & 14.18 & -31.0$\pm$3.0 & -14.0$\pm$3.0 & 4.6$\pm$0.6$^{(3)}$ & -38.2 & -11.6 & 91 &  \\ 
211901010 & 08 38 08.09 & +18 44 30.0 & 17.71 & 13.81 & -35.85$\pm$2.23 & -19.03$\pm$2.23 & 5.2$\pm$0.7$^{(1)}$ & -36.1 & -12.3 & 100 & 0.47\\ 
211901114 & 08 41 35.69 & +18 44 35.0 & 15.77 & 12.32 & -36.22$\pm$2.19 & -12.61$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.7 & -12.1 & 100 & 8.61\\ 
211901402 & 08 36 08.64 & +18 44 50.9 & 14.1 & 11.29 & -41.3$\pm$2.19 & -13.67$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.7 & -12.4 & 100 & 14.66\\ 
211901458 & 08 40 53.26 & +18 44 54.0 & 17.57 & 13.67 & -35.28$\pm$2.19 & -16.57$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.6 & -12.1 & 100 & 1.4\\ 
211901847 & 08 43 34.62 & +18 45 13.9 & 17.12 & 13.3 & -35.48$\pm$2.19 & -16.14$\pm$2.19 & 6.4$\pm$0.9$^{(1)}$ & -37.0 & -12.0 & 100 & 4.44\\ 
211901894 & 08 33 07.72 & +18 45 15.7 & 17.23 & 13.57 & -34.53$\pm$2.24 & -12.17$\pm$2.24 & 4.5$\pm$0.6$^{(1)}$ & -35.2 & -12.5 & 100 & 1.67\\ 
211902072 & 08 36 54.11 & +18 45 24.7 & 12.31 & 10.47 & -38.44$\pm$2.19 & -10.03$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.8 & -12.3 & 100 & 9.36\\ 
211902261 & 08 41 29.00 & +18 45 35.1 & 18.2 & 14.19 & -31.37$\pm$2.72 & -15.77$\pm$2.72 & 5.0$\pm$0.7$^{(1)}$ & -36.7 & -12.1 & 100 &  \\ 
211902283 & 08 31 54.27 & +18 45 36.2 & 17.44 & 13.76 & -36.05$\pm$2.3 & -12.42$\pm$2.3 & 4.8$\pm$0.7$^{(1)}$ & -34.9 & -12.6 & 100 & 2.18\\ 
211902344 & 08 45 14.94 & +18 45 40.0 & 17.13 & 13.41 & -36.4$\pm$2.19 & -11.71$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -37.3 & -11.9 & 100 & 5.79\\ 
211902720 & 08 42 10.29 & +18 46 00.4 & 17.59 & 13.75 & -35.59$\pm$2.19 & -16.07$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.8 & -12.1 & 100 & 1.06\\ 
211902826 & 08 42 22.04 & +18 46 05.9 & 18.0 & 14.0 & -33.46$\pm$2.19 & -16.18$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.8 & -12.1 & 100 & 2.63\\ 
211903302 & 08 38 57.77 & +18 46 30.9 & 16.37 & 12.71 & -36.44$\pm$2.19 & -13.42$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & -36.2 & -12.2 & 100 & 2.71\\ 
211903709 & 08 38 32.33 & +18 46 52.9 & 15.95 & 12.53 & -38.5$\pm$2.19 & -10.92$\pm$2.19 & 4.5$\pm$0.6$^{(1)}$ & -36.1 & -12.3 & 100 & 13.6\\ 
211905009 & 08 43 48.15 & +18 48 02.7 & 9.94 & 8.93 & -34.91$\pm$1.41 & -12.13$\pm$0.74 & 5.7$\pm$0.4$^{(0)}$ & -37.1 & -12.0 & 100 & 31.65\\ 
211905265 & 08 39 26.15 & +18 48 17.1 & 18.0 & 14.02 & -34.47$\pm$2.69 & -17.34$\pm$2.69 & 5.4$\pm$0.7$^{(1)}$ & -36.3 & -12.2 & 100 & 0.81\\ 
211905618 & 08 39 18.90 & +18 48 36.5 & 16.46 & 12.79 & -36.61$\pm$2.19 & -14.15$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -36.3 & -12.2 & 100 & 16.16\\ 
211905676 & 08 37 27.07 & +18 48 39.5 & 17.2 & 13.47 & -35.42$\pm$2.19 & -14.4$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -35.9 & -12.3 & 100 & 1.12\\ 
211906187 & 08 40 39.52 & +18 49 05.8 & 13.51 & 11.0 & -37.26$\pm$2.19 & -10.24$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.5 & -12.2 & 100 & 13.18\\ 
211906287 & 08 44 13.25 & +18 49 11.4 & 13.52 & 10.94 & -39.26$\pm$2.14 & -11.78$\pm$2.14 & 5.0$\pm$0.7$^{(1)}$ & -37.1 & -12.0 & 100 & 12.22\\ 
211906365 & 08 52 24.35 & +18 49 15.7 & 12.97 & 10.82 & -30.56$\pm$2.08 & -8.13$\pm$2.08 & 4.6$\pm$0.6$^{(1)}$ & -38.5 & -11.6 & 38 &  \\ 
211906671 & 08 45 21.06 & +18 49 32.8 & 18.24 & 14.22 & -40.03$\pm$2.72 & -13.34$\pm$2.72 & 4.2$\pm$0.6$^{(1)}$ & -37.3 & -11.9 & 100 & 0.63\\ 
211906702 & 08 40 55.72 & +18 49 34.3 & 17.14 & 13.46 & -34.75$\pm$2.19 & -15.38$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -36.6 & -12.2 & 100 & 2.1\\ 
211907026 & 08 36 58.65 & +18 49 52.2 & 17.32 & 13.26 & -37.32$\pm$2.2 & -14.78$\pm$2.19 & 8.8$\pm$1.2$^{(1)}$ & -35.9 & -12.4 & 99 & 1.0\\ 
211907530 & 08 36 51.63 & +18 50 19.3 & 17.27 & 13.48 & -35.37$\pm$2.69 & -15.51$\pm$2.69 & 6.1$\pm$0.8$^{(1)}$ & -35.8 & -12.4 & 100 & 2.06\\ 
211907679 & 08 36 21.12 & +18 50 27.7 & 18.14 & 14.31 & -34.12$\pm$2.73 & -14.55$\pm$2.73 & 4.3$\pm$0.6$^{(1)}$ & -35.7 & -12.4 & 100 & 0.51\\ 
211908029 & 08 40 58.45 & +18 50 46.3 & 16.82 & 13.13 & -36.13$\pm$2.19 & -16.06$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.6 & -12.2 & 100 & 2.9\\ 
211908085 & 08 39 40.08 & +18 50 49.2 & 18.01 & 14.02 & -35.94$\pm$2.69 & -11.67$\pm$2.69 & 5.1$\pm$0.7$^{(1)}$ & -36.3 & -12.2 & 100 & 1.62\\ 
211908380 & 08 33 02.43 & +18 51 03.9 & 17.06 & 13.51 & -34.58$\pm$2.24 & -16.16$\pm$2.24 & 3.9$\pm$0.5$^{(1)}$ & -35.1 & -12.6 & 99 &  \\ 
211908826 & 08 38 56.94 & +18 51 29.6 & 15.66 & 12.16 & -38.76$\pm$2.19 & -15.32$\pm$2.19 & 6.2$\pm$0.9$^{(1)}$ & -36.2 & -12.3 & 100 & 23.67\\ 
211908928 & 08 42 49.68 & +18 51 35.1 & 14.94 & 11.74 & -35.08$\pm$2.19 & -16.08$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.9 & -12.1 & 100 & 13.12\\ 
211909748 & 08 41 30.71 & +18 52 18.7 & 12.42 & 10.15 & -36.27$\pm$2.19 & -13.55$\pm$2.19 & 7.2$\pm$1.0$^{(1)}$ & -36.7 & -12.2 & 100 & 2.42\\ 
211909798 & 08 44 27.22 & +18 52 20.8 & 17.49 & 13.64 & -35.6$\pm$2.19 & -16.86$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -37.2 & -12.0 & 100 & 1.37\\ 
211909987 & 08 45 20.53 & +18 52 31.4 & 8.38 & 7.84 & -37.46$\pm$0.06 & -12.47$\pm$0.04 & 5.3$\pm$0.6$^{(0)}$ & -37.3 & -12.0 & 100 &  \\ 
211910082 & 08 39 35.54 & +18 52 36.8 & 10.54 & 9.33 & -35.54$\pm$2.18 & -12.91$\pm$0.97 & 6.0$\pm$0.6$^{(0)}$ & -36.3 & -12.3 & 100 & 6.69\\ 
211910450 & 08 36 48.00 & +18 52 58.1 & 8.54 & 7.94 & -35.27$\pm$0.07 & -12.63$\pm$0.04 & 4.4$\pm$0.4$^{(0)}$ & -35.8 & -12.4 & 100 & 13.07\\ 
211910532 & 08 37 32.23 & +18 53 02.2 & 15.28 & 12.04 & -36.02$\pm$2.23 & -14.47$\pm$2.23 & 4.7$\pm$0.7$^{(1)}$ & -36.0 & -12.4 & 100 & 10.36\\ 
211910548 & 08 45 21.17 & +18 53 03.5 & 17.32 & 13.63 & -35.3$\pm$2.69 & -15.04$\pm$2.69 & 4.2$\pm$0.6$^{(1)}$ & -37.3 & -12.0 & 100 & 2.13\\ 
211910977 & 08 45 18.01 & +18 53 25.3 &   & 8.6 & -36.2$\pm$1.1 & -14.3$\pm$1.1 & 5.7$\pm$0.8$^{(2)}$ & -37.3 & -12.0 & 100 & 2.29\\ 
211911179 & 08 43 54.67 & +18 53 36.9 & 12.29 & 10.41 & -36.64$\pm$2.19 & -14.59$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -37.1 & -12.1 & 100 & 10.33\\ 
211911279 & 08 36 42.70 & +18 53 42.8 & 13.33 & 10.84 & -36.9$\pm$2.19 & -11.84$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -35.8 & -12.4 & 100 & 12.84\\ 
211911467 & 08 30 51.41 & +18 53 51.5 & 17.1 & 13.39 & -36.5$\pm$2.24 & -14.24$\pm$2.24 & 4.9$\pm$0.7$^{(1)}$ & -34.7 & -12.7 & 100 & 2.18\\ 
211911846 & 08 40 47.61 & +18 54 11.9 & 11.2 & 9.69 & -39.94$\pm$2.85 & -11.01$\pm$1.3 & 5.0$\pm$0.9$^{(0)}$ & -36.5 & -12.2 & 100 & 4.3\\ 
211911911 & 08 41 36.62 & +18 54 15.5 & 15.99 & 12.44 & -36.05$\pm$2.19 & -16.24$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -36.7 & -12.2 & 100 & 1.09\\ 
211911959 & 08 39 39.20 & +18 54 17.2 & 12.77 & 11.13 & -32.11$\pm$2.19 & -10.75$\pm$2.19 & 3.2$\pm$0.4$^{(1)}$ & -36.3 & -12.3 & 23 &  \\ 
211912350 & 08 25 16.13 & +18 54 38.9 & 18.53 & 14.27 & -33.79$\pm$2.8 & -6.12$\pm$2.8 & 5.7$\pm$0.8$^{(1)}$ & -33.7 & -13.0 & 58 & 0.26\\ 
211912407 & 08 41 57.82 & +18 54 42.2 & 9.31 & 8.43 & -35.18$\pm$0.51 & -11.86$\pm$0.58 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -12.2 & 100 & 2.03\\ 
211912899 & 08 43 05.57 & +18 55 06.1 & 18.33 & 14.31 & -31.84$\pm$2.73 & -14.88$\pm$2.73 & 5.8$\pm$0.8$^{(1)}$ & -36.9 & -12.1 & 100 & 0.77\\ 
211912940 & 08 36 19.01 & +18 55 08.3 & 15.73 & 12.35 & -40.08$\pm$2.19 & -13.69$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -12.5 & 100 & 17.68\\ 
211913330 & 08 42 57.08 & +18 55 27.4 & 12.08 & 10.21 & -30.89$\pm$2.19 & -17.33$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.9 & -12.1 & 99 &  \\ 
211913532 & 08 40 19.83 & +18 55 38.3 & 14.93 & 11.54 & -36.95$\pm$2.19 & -11.17$\pm$2.19 & 7.1$\pm$1.0$^{(1)}$ & -36.5 & -12.3 & 100 & 16.33\\ 
211913669 & 08 42 34.96 & +18 55 45.8 & 16.98 & 13.32 & -34.45$\pm$2.19 & -13.57$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.9 & -12.1 & 100 & 31.32\\ 
211913733 & 08 33 05.58 & +18 55 48.7 & 15.66 & 12.19 & -35.09$\pm$2.24 & -14.47$\pm$2.24 & 5.7$\pm$0.8$^{(1)}$ & -35.2 & -12.6 & 100 & 12.63\\ 
211913859 & 08 41 03.14 & +18 55 55.1 & 16.72 & 13.1 & -35.95$\pm$2.19 & -12.08$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.6 & -12.2 & 100 & 12.37\\ 
211913907 & 08 40 03.91 & +18 55 57.5 & 18.21 & 14.17 & -36.98$\pm$2.72 & -16.2$\pm$2.72 & 5.3$\pm$0.7$^{(1)}$ & -36.4 & -12.3 & 100 & 0.42\\ 
211913977 & 08 41 22.58 & +18 56 02.0 & 12.54 & 10.54 & -36.95$\pm$2.19 & -14.1$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.6 & -12.2 & 100 & 10.62\\ 
211914072 & 08 37 34.97 & +18 56 07.8 & 16.19 & 12.85 & -41.19$\pm$2.23 & -17.16$\pm$2.23 & 4.2$\pm$0.6$^{(1)}$ & -36.0 & -12.4 & 100 &  \\ 
211914098 & 08 40 28.24 & +18 56 08.9 & 14.8 & 11.71 & -37.44$\pm$2.19 & -14.46$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.5 & -12.3 & 100 & 17.18\\ 
211914124 & 08 44 19.14 & +18 56 10.0 & 15.83 & 12.06 & -35.46$\pm$2.19 & -12.94$\pm$2.19 & 9.2$\pm$1.3$^{(1)}$ & -37.2 & -12.1 & 99 & 18.0\\ 
211914465 & 08 38 25.38 & +18 56 29.9 & 15.23 & 11.72 & -37.81$\pm$2.23 & -11.79$\pm$2.23 & 7.0$\pm$1.0$^{(1)}$ & -36.1 & -12.4 & 100 & 4.69\\ 
211914889 & 08 39 30.71 & +18 56 53.4 & 17.66 & 13.84 & -28.36$\pm$2.19 & -12.19$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.3 & -12.3 & 99 & 1.04\\ 
211914960 & 08 40 02.23 & +18 56 57.0 & 14.46 & 11.16 & -36.54$\pm$2.19 & -11.37$\pm$2.19 & 8.2$\pm$1.1$^{(1)}$ & -36.4 & -12.3 & 100 &  \\ 
211915085 & 08 48 30.07 & +18 57 03.5 &   & 14.36 & -38.0$\pm$4.0 & -8.0$\pm$4.0 & 6.1$\pm$0.8$^{(3)}$ & -37.9 & -11.9 & 100 & 0.69\\ 
211915202 & 08 40 29.22 & +18 57 09.5 & 14.01 & 10.86 & -40.24$\pm$1.75 & -19.92$\pm$1.75 & 7.6$\pm$1.1$^{(1)}$ & -36.5 & -12.3 & 88 &  \\ 
211915602 & 08 40 14.27 & +18 57 31.4 & 13.21 & 10.82 & -40.81$\pm$2.19 & -9.36$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.4 & -12.3 & 100 &  \\ 
211915709 & 08 35 44.61 & +18 57 38.3 & 17.31 & 13.55 & -39.72$\pm$2.19 & -12.73$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -35.6 & -12.5 & 100 & 1.56\\ 
211915785 & 08 41 20.34 & +18 57 43.0 & 16.91 & 13.16 & -34.35$\pm$2.19 & -16.42$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -12.2 & 100 & 3.13\\ 
211915860 & 08 36 56.25 & +18 57 47.9 & 14.07 & 10.91 & -38.41$\pm$2.19 & -13.61$\pm$2.19 & 7.7$\pm$1.1$^{(1)}$ & -35.8 & -12.5 & 100 & 4.82\\ 
211915918 & 08 44 32.90 & +18 57 50.7 & 15.98 & 12.39 & -38.59$\pm$2.2 & -16.0$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -37.2 & -12.1 & 100 & 4.67\\ 
211915935 & 08 45 32.18 & +18 57 52.1 & 16.5 & 12.92 & -35.34$\pm$2.18 & -10.63$\pm$2.18 & 4.9$\pm$0.7$^{(1)}$ & -37.4 & -12.0 & 100 & 18.22\\ 
211915940 & 08 38 00.61 & +18 57 52.9 & 16.01 & 12.34 & -36.14$\pm$2.23 & -14.61$\pm$2.23 & 7.3$\pm$1.0$^{(1)}$ & -36.0 & -12.4 & 100 & 5.91\\ 
211916015 & 08 36 29.85 & +18 57 57.1 & 9.27 & 8.3 & -35.63$\pm$0.49 & -12.56$\pm$0.57 & 6.7$\pm$0.9$^{(1)}$ & -35.8 & -12.5 & 100 & 9.27\\ 
211916232 & 08 41 13.94 & +18 58 08.9 & 15.11 & 11.76 & -37.87$\pm$2.19 & -15.18$\pm$2.19 & 6.1$\pm$0.8$^{(1)}$ & -36.6 & -12.2 & 100 & 29.77\\ 
211916235 & 08 44 27.69 & +18 58 09.6 & 16.52 & 12.87 & -37.17$\pm$2.19 & -14.2$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -37.2 & -12.1 & 100 & 16.51\\ 
211916505 & 08 37 57.56 & +18 58 23.2 & 17.98 & 13.85 & -34.44$\pm$2.76 & -11.64$\pm$2.76 & 6.4$\pm$0.9$^{(1)}$ & -36.0 & -12.4 & 100 & 0.23\\ 
211916718 & 08 39 45.73 & +18 58 34.0 & 16.08 & 12.56 & -39.61$\pm$2.19 & -12.84$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.4 & -12.3 & 100 & 15.26\\ 
211916756 & 08 37 27.06 & +18 58 36.1 & 15.9 & 12.47 & -37.27$\pm$2.19 & -15.0$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.9 & -12.4 & 100 & 23.86\\ 
211917139 & 08 40 10.85 & +18 58 57.1 & 15.6 & 12.01 & -35.66$\pm$2.19 & -13.59$\pm$2.19 & 7.6$\pm$1.1$^{(1)}$ & -36.4 & -12.3 & 100 & 1.97\\ 
211917204 & 08 44 13.28 & +18 59 00.5 & 14.19 & 11.31 & -49.59$\pm$2.7 & -16.28$\pm$2.7 & 5.2$\pm$0.7$^{(1)}$ & -37.1 & -12.1 & 91 &  \\ 
211917723 & 08 38 16.56 & +18 59 28.8 & 15.99 & 12.57 & -29.79$\pm$2.33 & -6.44$\pm$2.33 & 4.9$\pm$0.7$^{(1)}$ & -36.1 & -12.4 & 98 &  \\ 
211917847 & 08 51 43.88 & +18 59 34.7 & 18.65 & 14.34 & -48.78$\pm$2.76 & -11.92$\pm$2.76 & 5.8$\pm$0.8$^{(1)}$ & -38.4 & -11.7 & 80 &  \\ 
211918097 & 08 45 28.60 & +18 59 48.1 & 18.3 & 14.4 & -33.8$\pm$2.91 & -9.48$\pm$2.76 & 4.2$\pm$0.6$^{(1)}$ & -37.4 & -12.0 & 100 &  \\ 
211918335 & 08 40 01.70 & +18 59 59.5 & 10.02 & 8.7 & -37.38$\pm$0.69 & -12.59$\pm$0.77 & 7.6$\pm$1.1$^{(1)}$ & -36.4 & -12.3 & 100 & 0.19\\ 
211918547 & 08 45 19.18 & +19 00 10.9 & 13.3 & 10.9 & -38.78$\pm$2.19 & -10.31$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -37.3 & -12.1 & 100 & 12.84\\ 
211918605 & 08 43 35.35 & +19 00 14.2 & 15.58 & 11.79 & -29.3$\pm$2.82 & -13.73$\pm$2.82 & 12.4$\pm$1.7$^{(1)}$ & -37.0 & -12.1 & 31 & 8.21\\ 
211918998 & 08 50 59.88 & +19 00 35.6 & 17.5 & 13.65 & -38.22$\pm$2.09 & -16.59$\pm$2.09 & 5.1$\pm$0.7$^{(1)}$ & -38.3 & -11.8 & 99 & 1.56\\ 
211919747 & 08 38 37.23 & +19 01 16.1 & 13.13 & 10.61 & -37.8$\pm$2.19 & -11.93$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.1 & -12.4 & 100 & 12.9\\ 
211920022 & 08 40 05.72 & +19 01 30.7 & 12.18 & 10.01 & -36.96$\pm$2.19 & -12.44$\pm$2.19 & 7.0$\pm$1.0$^{(1)}$ & -36.4 & -12.3 & 100 & 4.67\\ 
211920429 & 08 41 10.76 & +19 01 53.9 & 16.68 & 12.84 & -34.49$\pm$2.19 & -15.06$\pm$2.19 & 8.3$\pm$1.1$^{(1)}$ & -36.6 & -12.3 & 100 &  \\ 
211920710 & 08 45 22.41 & +19 02 08.2 & 16.67 & 12.83 & -36.65$\pm$2.24 & -12.68$\pm$2.47 & 8.2$\pm$1.1$^{(1)}$ & -37.3 & -12.1 & 100 & 1.33\\ 
211920850 & 08 42 19.24 & +19 02 14.8 & 15.96 & 12.53 & -34.65$\pm$2.19 & -10.86$\pm$2.19 & 4.5$\pm$0.6$^{(1)}$ & -36.8 & -12.2 & 100 & 24.64\\ 
211921097 & 08 33 05.75 & +19 02 28.1 & 18.61 & 14.63 & -34.88$\pm$2.95 & -9.88$\pm$2.95 & 3.8$\pm$0.5$^{(1)}$ & -35.2 & -12.7 & 97 &  \\ 
211921647 & 08 45 46.53 & +19 02 58.1 & 7.99 & 7.53 & -38.86$\pm$0.06 & -12.6$\pm$0.03 & 6.4$\pm$0.4$^{(0)}$ & -37.4 & -12.1 & 100 &  \\ 
211921859 & 08 32 18.90 & +19 03 08.7 & 16.4 & 12.83 & -35.53$\pm$2.24 & -14.47$\pm$2.24 & 5.3$\pm$0.7$^{(1)}$ & -35.0 & -12.8 & 100 &  \\ 
211921927 & 08 37 19.91 & +19 03 12.1 & 15.24 & 11.83 & -36.7$\pm$2.19 & -14.84$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -35.9 & -12.5 & 100 & 2.04\\ 
211922472 & 08 52 14.53 & +19 03 39.0 & 14.11 & 11.06 & -37.34$\pm$2.08 & -11.6$\pm$2.09 & 7.0$\pm$1.0$^{(1)}$ & -38.5 & -11.7 & 98 & 34.17\\ 
211922849 & 08 43 44.73 & +19 03 58.6 & 15.03 & 11.87 & -37.72$\pm$2.19 & -14.14$\pm$2.19 & 4.7$\pm$0.6$^{(1)}$ & -37.1 & -12.2 & 100 & 19.39\\ 
211922975 & 08 43 07.05 & +19 04 06.1 & 9.4 & 8.36 & -38.09$\pm$0.89 & -11.44$\pm$0.7 & 5.0$\pm$0.4$^{(0)}$ & -36.9 & -12.2 & 100 & 4.93\\ 
211923104 & 08 55 10.46 & +19 04 11.8 & 16.29 & 12.74 & -31.79$\pm$2.09 & -13.31$\pm$2.08 & 4.6$\pm$0.6$^{(1)}$ & -39.0 & -11.6 & 30 & 17.27\\ 
211923188 & 08 41 07.36 & +19 04 16.4 & 9.98 & 8.64 & -37.59$\pm$0.59 & -12.08$\pm$0.68 & 8.1$\pm$1.1$^{(1)}$ & -36.6 & -12.3 & 100 & 7.8\\ 
211923230 & 08 36 51.07 & +19 04 18.6 & 16.73 & 13.24 & -34.72$\pm$2.19 & -11.94$\pm$2.19 & 3.7$\pm$0.5$^{(1)}$ & -35.8 & -12.5 & 99 & 32.68\\ 
211923388 & 08 36 02.42 & +19 04 26.5 & 18.12 & 14.25 & -36.06$\pm$2.71 & -9.85$\pm$2.71 & 4.8$\pm$0.7$^{(1)}$ & -35.7 & -12.6 & 100 & 0.33\\ 
211923502 & 08 43 43.56 & +19 04 33.1 & 12.93 & 10.79 & -35.69$\pm$1.61 & -11.46$\pm$1.61 & 4.8$\pm$0.7$^{(1)}$ & -37.1 & -12.2 & 100 & 12.07\\ 
211923534 & 08 36 51.64 & +19 04 35.0 & 13.21 & 10.86 & -34.84$\pm$2.19 & -14.02$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.8 & -12.5 & 100 & 12.02\\ 
211923569 & 08 33 14.40 & +19 04 36.5 & 15.28 & 12.09 & -34.2$\pm$2.24 & -13.86$\pm$2.24 & 4.6$\pm$0.6$^{(1)}$ & -35.2 & -12.7 & 100 & 15.57\\ 
211923684 & 08 53 46.09 & +19 04 43.1 & 16.62 & 13.12 & -46.0$\pm$4.0 & -20.0$\pm$4.0 & 3.9$\pm$0.5$^{(1)}$ & -38.8 & -11.6 & 32 &  \\ 
211923932 & 08 40 54.15 & +19 04 55.2 & 18.61 & 14.56 & -38.13$\pm$2.77 & -13.2$\pm$2.77 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -12.3 & 100 &  \\ 
211924229 & 08 41 15.42 & +19 05 10.4 & 15.6 & 12.25 & -34.68$\pm$2.19 & -13.88$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.3 & 100 & 21.32\\ 
211924377 & 08 41 19.10 & +19 05 18.7 & 16.94 & 12.87 & -34.12$\pm$2.19 & -20.92$\pm$2.19 & 10.9$\pm$1.5$^{(1)}$ & -36.6 & -12.3 & 13 & 5.37\\ 
211924546 & 08 36 56.80 & +19 05 28.1 & 13.87 & 10.97 & -38.3$\pm$2.19 & -12.5$\pm$2.19 & 6.3$\pm$0.9$^{(1)}$ & -35.9 & -12.5 & 100 & 14.88\\ 
211925013 & 08 41 19.69 & +19 05 54.5 & 17.95 & 14.0 & -33.74$\pm$2.19 & -16.93$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.3 & 100 & 0.86\\ 
211925093 & 08 42 42.48 & +19 05 58.9 & 11.35 & 9.88 & -36.13$\pm$0.82 & -13.53$\pm$0.83 & 4.9$\pm$0.7$^{(1)}$ & -36.9 & -12.3 & 100 & 8.69\\ 
211925319 & 08 41 06.47 & +19 06 10.7 & 18.18 & 14.17 & -37.7$\pm$2.73 & -19.49$\pm$2.72 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.3 & 100 & 27.09\\ 
211925371 & 08 37 31.05 & +19 06 14.3 & 13.23 & 10.77 & -39.09$\pm$2.23 & -13.85$\pm$2.23 & 5.5$\pm$0.8$^{(1)}$ & -36.0 & -12.5 & 100 & 13.12\\ 
211925552 & 08 37 47.39 & +19 06 24.8 & 11.92 & 10.2 & -34.94$\pm$0.92 & -13.46$\pm$1.06 & 5.4$\pm$0.7$^{(1)}$ & -36.0 & -12.5 & 100 & 9.33\\ 
211925563 & 08 41 35.99 & +19 06 25.5 & 13.49 & 10.98 & -36.45$\pm$2.19 & -14.0$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.7 & -12.3 & 100 & 13.48\\ 
211925698 & 08 43 15.87 & +19 06 33.1 & 17.07 & 13.34 & -33.21$\pm$2.23 & -13.53$\pm$2.23 & 5.2$\pm$0.7$^{(1)}$ & -37.0 & -12.2 & 100 & 6.25\\ 
211926128 & 08 31 07.18 & +19 06 56.1 & 13.44 & 11.44 & -40.08$\pm$2.24 & -12.5$\pm$2.24 & 3.3$\pm$0.5$^{(1)}$ & -34.8 & -12.9 & 16 &  \\ 
211926132 & 08 39 12.17 & +19 06 56.2 & 10.4 & 9.26 & -35.81$\pm$1.82 & -12.42$\pm$0.86 & 5.6$\pm$0.5$^{(0)}$ & -36.3 & -12.5 & 100 & 5.87\\ 
211926133 & 08 39 39.65 & +19 06 56.2 & 18.07 & 14.03 & -36.39$\pm$2.69 & -15.17$\pm$2.69 & 5.5$\pm$0.8$^{(1)}$ & -36.3 & -12.4 & 100 & 1.56\\ 
211926166 & 08 42 30.74 & +19 06 57.8 & 17.48 & 13.59 & -37.29$\pm$2.19 & -15.9$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.8 & -12.3 & 100 & 1.21\\ 
211926825 & 08 35 39.69 & +19 07 36.7 & 15.87 & 12.29 & -36.7$\pm$2.22 & -14.33$\pm$2.2 & 5.8$\pm$0.8$^{(1)}$ & -35.6 & -12.6 & 100 & 5.67\\ 
211927174 & 08 47 53.84 & +19 07 53.3 & 17.26 & 13.54 & -31.22$\pm$2.1 & -11.33$\pm$2.1 & 5.1$\pm$0.7$^{(1)}$ & -37.8 & -12.0 & 99 & 1.88\\ 
211927213 & 08 37 26.39 & +19 07 55.7 & 13.98 & 11.19 & -37.9$\pm$2.19 & -13.84$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -35.9 & -12.6 & 100 & 14.66\\ 
211927269 & 08 42 40.21 & +19 07 59.1 & 11.83 & 10.19 & -35.88$\pm$0.84 & -11.38$\pm$0.84 & 4.6$\pm$0.6$^{(1)}$ & -36.9 & -12.3 & 100 & 9.39\\ 
211927313 & 08 37 42.36 & +19 08 01.5 & 9.65 & 8.58 & -34.85$\pm$0.82 & -11.26$\pm$0.68 & 5.3$\pm$0.7$^{(1)}$ & -36.0 & -12.5 & 100 & 3.06\\ 
211927867 & 08 41 36.20 & +19 08 33.5 & 9.21 & 8.35 & -37.3$\pm$0.45 & -13.37$\pm$0.53 & 5.8$\pm$0.8$^{(1)}$ & -36.7 & -12.3 & 100 & 1.12\\ 
211928367 & 08 48 10.21 & +19 08 59.9 & 19.12 & 14.78 & -38.17$\pm$2.89 & -11.65$\pm$2.89 & 4.7$\pm$0.6$^{(1)}$ & -37.8 & -12.0 & 100 & 10.29\\ 
211928486 & 08 42 20.08 & +19 09 05.6 & 12.97 & 10.7 & -36.32$\pm$2.19 & -13.58$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.8 & -12.3 & 100 & 11.93\\ 
211928526 & 08 45 08.55 & +19 09 08.2 & 17.48 & 13.58 & -35.28$\pm$2.18 & -13.23$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -37.3 & -12.2 & 100 & 1.8\\ 
211928574 & 08 47 50.52 & +19 09 11.0 & 17.25 & 13.57 & -32.81$\pm$2.1 & -14.44$\pm$2.1 & 5.2$\pm$0.7$^{(1)}$ & -37.8 & -12.0 & 100 & 1.49\\ 
211928727 & 08 41 09.51 & +19 09 20.5 & 18.48 & 13.74 & -40.2$\pm$2.82 & -14.0$\pm$2.82 & 7.7$\pm$1.1$^{(1)}$ & -36.6 & -12.4 & 100 &  \\ 
211928930 & 08 36 08.96 & +19 09 30.9 & 15.93 & 12.38 & -38.66$\pm$2.19 & -15.48$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -35.7 & -12.6 & 100 & 8.26\\ 
211929081 & 08 48 25.45 & +19 09 39.4 &   & 13.72 & -43.0$\pm$3.0 & -7.0$\pm$3.0 & 6.5$\pm$0.9$^{(3)}$ & -37.9 & -12.0 & 99 & 21.02\\ 
211929493 & 08 49 59.38 & +19 10 01.0 & 16.67 & 13.01 & -38.33$\pm$2.12 & -16.98$\pm$2.11 & 5.5$\pm$0.8$^{(1)}$ & -38.1 & -11.9 & 100 & 14.59\\ 
211929531 & 08 43 02.42 & +19 10 03.2 & 11.81 & 10.16 & -37.27$\pm$1.01 & -12.0$\pm$0.95 & 5.1$\pm$0.7$^{(1)}$ & -36.9 & -12.3 & 100 & 9.89\\ 
211929980 & 08 40 52.31 & +19 10 28.0 & 15.81 & 12.1 & -35.78$\pm$2.19 & -12.26$\pm$2.19 & 8.6$\pm$1.2$^{(1)}$ & -36.5 & -12.4 & 100 & 1.18\\ 
211930233 & 08 37 03.46 & +19 10 41.2 & 13.03 & 10.73 & -39.18$\pm$2.19 & -12.2$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.9 & -12.6 & 100 & 19.02\\ 
211930699 & 08 36 36.43 & +19 11 06.7 & 13.93 & 11.2 & -37.74$\pm$2.19 & -12.37$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.8 & -12.6 & 100 & 6.74\\ 
211931128 & 08 36 22.69 & +19 11 29.3 & 12.02 & 10.26 & -38.84$\pm$2.19 & -12.14$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -35.7 & -12.6 & 100 & 9.79\\ 
211931309 & 08 40 32.96 & +19 11 39.6 & 8.6 & 7.96 & -36.35$\pm$0.52 & -13.68$\pm$0.3 & 5.3$\pm$0.3$^{(0)}$ & -36.5 & -12.4 & 100 & 0.11\\ 
211931411 & 08 41 49.35 & +19 11 47.0 & 13.66 & 10.83 & -36.61$\pm$2.19 & -14.44$\pm$2.19 & 6.5$\pm$0.9$^{(1)}$ & -36.7 & -12.4 & 100 & 13.66\\ 
211931651 & 08 43 22.40 & +19 12 00.8 & 16.23 & 12.65 & -36.12$\pm$2.23 & -12.87$\pm$2.23 & 5.0$\pm$0.7$^{(1)}$ & -37.0 & -12.3 & 100 & 21.94\\ 
211931736 & 08 39 58.07 & +19 12 05.9 & 9.35 & 8.48 & -35.66$\pm$0.82 & -13.17$\pm$0.43 & 5.5$\pm$0.4$^{(0)}$ & -36.4 & -12.5 & 100 & 30.07\\ 
211931872 & 08 41 10.17 & +19 12 13.3 & 18.01 & 13.9 & -33.13$\pm$2.82 & -17.95$\pm$2.81 & 5.8$\pm$0.8$^{(1)}$ & -36.6 & -12.4 & 100 & 5.14\\ 
211932539 & 08 42 12.34 & +19 12 48.6 & 13.13 & 10.83 & -35.47$\pm$2.19 & -14.5$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.8 & -12.4 & 100 & 13.48\\ 
211932810 & 08 39 46.57 & +19 13 04.0 & 14.48 & 11.51 & -36.96$\pm$2.19 & -12.64$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.4 & -12.5 & 100 & 15.9\\ 
211932923 & 08 40 26.25 & +19 13 09.9 & 12.46 & 10.46 & -38.11$\pm$2.19 & -10.12$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.5 & -12.5 & 100 & 10.69\\ 
211933215 & 08 40 41.90 & +19 13 25.5 & 10.39 & 9.06 & -35.83$\pm$0.84 & -13.31$\pm$0.84 & 6.0$\pm$0.8$^{(1)}$ & -36.5 & -12.4 & 100 & 6.11\\ 
211933524 & 08 40 39.24 & +19 13 41.9 & 7.75 & 7.23 & -35.09$\pm$0.32 & -11.59$\pm$0.36 & 4.3$\pm$0.5$^{(0)}$ & -36.5 & -12.5 & 100 & 18.9\\ 
211933636 & 08 36 08.98 & +19 13 48.1 & 15.29 & 12.04 & -36.6$\pm$2.19 & -14.72$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -35.7 & -12.7 & 100 & 18.55\\ 
211934056 & 08 37 57.03 & +19 14 10.4 & 11.56 & 10.04 & -33.78$\pm$0.84 & -12.46$\pm$0.84 & 4.8$\pm$0.7$^{(1)}$ & -36.0 & -12.6 & 100 & 9.05\\ 
211934092 & 08 45 26.64 & +19 14 12.8 & 16.9 & 13.04 & -36.15$\pm$2.14 & -15.09$\pm$2.14 & 7.6$\pm$1.1$^{(1)}$ & -37.3 & -12.2 & 100 & 1.03\\ 
211934172 & 08 40 58.91 & +19 14 16.7 &   & 13.98 & -36.0$\pm$5.0 & -23.0$\pm$5.0 & 8.6$\pm$1.2$^{(3)}$ & -36.6 & -12.4 & 96 & 0.25\\ 
211935509 & 08 36 48.97 & +19 15 26.5 & 11.07 & 9.69 & -36.32$\pm$0.64 & -11.76$\pm$0.67 & 5.0$\pm$0.7$^{(1)}$ & -35.8 & -12.7 & 100 & 7.49\\ 
211935518 & 08 41 54.36 & +19 15 26.7 & 11.16 & 9.64 & -33.62$\pm$0.76 & -12.9$\pm$0.76 & 6.3$\pm$0.9$^{(1)}$ & -36.7 & -12.4 & 100 & 4.18\\ 
211935558 & 08 38 37.48 & +19 15 28.7 & 15.99 & 12.4 & -38.51$\pm$2.19 & -12.71$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.2 & -12.6 & 100 & 0.52\\ 
211935588 & 08 28 20.20 & +19 15 30.7 & 17.01 & 13.38 & -32.68$\pm$2.22 & -12.85$\pm$2.22 & 4.1$\pm$0.6$^{(1)}$ & -34.3 & -13.1 & 97 & 25.7\\ 
211935711 & 08 39 36.43 & +19 15 37.8 & 13.65 & 11.01 & -39.01$\pm$2.19 & -13.68$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.3 & -12.5 & 100 & 17.68\\ 
211935741 & 08 41 18.40 & +19 15 39.6 & 10.07 & 7.29 & -36.1$\pm$1.67 & -11.66$\pm$0.87 & 5.0$\pm$0.7$^{(0)}$ & -36.6 & -12.4 & 100 &  \\ 
211936017 & 08 37 36.24 & +19 15 54.3 & 12.96 & 10.76 & -36.74$\pm$2.24 & -15.52$\pm$2.23 & 4.9$\pm$0.7$^{(1)}$ & -36.0 & -12.6 & 100 & 11.79\\ 
211936049 & 08 41 53.35 & +19 15 55.8 & 17.77 & 13.89 & -33.79$\pm$2.69 & -14.72$\pm$2.69 & 5.4$\pm$0.7$^{(1)}$ & -36.7 & -12.4 & 100 & 0.36\\ 
211936067 & 08 41 39.03 & +19 15 56.8 & 12.65 & 10.57 & -41.15$\pm$2.19 & -10.74$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -12.4 & 100 & 10.29\\ 
211936163 & 08 37 46.76 & +19 16 02.0 & 6.7 & 6.16 & -35.0$\pm$0.04 & -12.83$\pm$0.02 & 5.1$\pm$0.6$^{(0)}$ & -36.0 & -12.6 & 100 &  \\ 
211936168 & 08 41 45.49 & +19 16 02.2 & 10.01 & 8.93 & -37.03$\pm$1.51 & -12.96$\pm$0.78 & 5.6$\pm$0.5$^{(0)}$ & -36.7 & -12.4 & 100 & 4.9\\ 
211936199 & 08 42 12.86 & +19 16 03.8 & 12.88 & 10.48 & -34.91$\pm$2.19 & -12.8$\pm$2.19 & 5.9$\pm$0.8$^{(1)}$ & -36.8 & -12.4 & 100 & 10.77\\ 
211936457 & 08 43 56.66 & +19 16 18.1 & 18.66 & 14.61 & -30.71$\pm$2.93 & -14.8$\pm$2.93 & 4.9$\pm$0.7$^{(1)}$ & -37.1 & -12.3 & 100 & 0.35\\ 
211936622 & 08 32 09.24 & +19 16 26.7 & 13.53 & 11.32 & -35.1$\pm$2.24 & -9.2$\pm$2.24 & 3.8$\pm$0.5$^{(1)}$ & -35.0 & -12.9 & 95 &  \\ 
211936741 & 08 33 17.99 & +19 16 32.8 & 16.61 & 12.81 & -37.46$\pm$2.24 & -16.05$\pm$2.24 & 6.7$\pm$0.9$^{(1)}$ & -35.2 & -12.9 & 100 & 2.29\\ 
211936827 & 08 42 11.50 & +19 16 37.2 & 11.83 & 10.17 & -35.16$\pm$0.92 & -11.5$\pm$0.92 & 4.9$\pm$0.7$^{(1)}$ & -36.8 & -12.4 & 100 & 7.89\\ 
211936869 & 08 41 27.60 & +19 16 39.4 & 14.93 & 11.72 & -36.24$\pm$2.19 & -13.25$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.7 & -12.4 & 100 &  \\ 
211936878 & 08 40 02.49 & +19 16 39.7 & 16.8 & 13.24 & -36.24$\pm$2.19 & -13.62$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.4 & -12.5 & 100 & 17.27\\ 
211936906 & 08 40 27.44 & +19 16 40.9 & 10.96 & 9.65 & -35.48$\pm$0.84 & -12.32$\pm$0.84 & 4.8$\pm$0.7$^{(1)}$ & -36.5 & -12.5 & 100 & 8.76\\ 
211937293 & 08 38 55.27 & +19 17 01.7 & 14.9 & 11.74 & -39.53$\pm$2.19 & -13.56$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.2 & -12.6 & 100 & 18.11\\ 
211937468 & 08 39 15.28 & +19 17 11.5 & 15.44 & 12.21 & -35.08$\pm$2.19 & -12.03$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -12.6 & 100 & 17.27\\ 
211937538 & 08 56 01.73 & +19 17 15.5 & 17.61 & 13.51 & -44.29$\pm$2.66 & -13.04$\pm$2.66 & 8.2$\pm$1.1$^{(1)}$ & -39.1 & -11.7 & 24 & 0.25\\ 
211937592 & 08 44 36.40 & +19 17 17.8 & 18.65 & 14.63 & -41.04$\pm$2.92 & -13.3$\pm$2.92 & 4.6$\pm$0.6$^{(1)}$ & -37.2 & -12.3 & 100 & 0.21\\ 
211937872 & 08 42 42.08 & +19 17 32.3 & 13.89 & 11.04 & -36.49$\pm$2.19 & -11.21$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.9 & -12.4 & 100 & 13.72\\ 
211938003 & 08 38 43.92 & +19 17 38.4 & 15.49 & 11.96 & -38.34$\pm$2.19 & -13.27$\pm$2.19 & 7.0$\pm$1.0$^{(1)}$ & -36.2 & -12.6 & 100 & 0.36\\ 
211938023 & 08 45 06.78 & +19 17 39.6 & 19.51 & 15.04 & -33.43$\pm$3.04 & -14.32$\pm$3.04 & 4.4$\pm$0.6$^{(1)}$ & -37.3 & -12.3 & 100 &  \\ 
211938090 & 08 24 33.25 & +19 17 43.2 & 15.93 & 12.2 & -37.0$\pm$2.22 & -14.3$\pm$2.22 & 8.6$\pm$1.2$^{(1)}$ & -33.6 & -13.3 & 36 & 49.32\\ 
211938350 & 08 45 05.91 & +19 17 57.5 & 17.3 & 13.55 & -37.09$\pm$2.19 & -13.28$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -37.3 & -12.3 & 100 & 26.61\\ 
211938397 & 08 32 05.34 & +19 18 00.5 & 14.42 & 11.79 & -30.68$\pm$2.24 & -8.31$\pm$2.24 & 3.5$\pm$0.5$^{(1)}$ & -35.0 & -12.9 & 13 &  \\ 
211938509 & 08 41 43.89 & +19 18 08.2 & 14.57 & 11.64 & -37.11$\pm$2.19 & -11.06$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.7 & -12.4 & 100 & 16.7\\ 
211938530 & 08 41 03.15 & +19 18 09.3 & 18.16 & 14.21 & -31.48$\pm$2.72 & -15.16$\pm$2.72 & 5.7$\pm$0.8$^{(1)}$ & -36.6 & -12.5 & 100 & 27.58\\ 
211938625 & 08 53 46.68 & +19 18 14.3 & 13.98 & 11.16 & -34.88$\pm$2.08 & -10.48$\pm$2.08 & 5.6$\pm$0.8$^{(1)}$ & -38.8 & -11.8 & 97 & 13.79\\ 
211938725 & 08 39 51.36 & +19 18 20.2 & 17.07 & 13.42 & -33.92$\pm$2.59 & 0.19$\pm$2.49 & 4.6$\pm$0.6$^{(1)}$ & -36.4 & -12.5 & 12 &  \\ 
211938817 & 08 45 12.36 & +19 18 24.7 & 17.82 & 13.83 & -30.1$\pm$2.19 & -17.27$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & -37.3 & -12.3 & 94 & 0.46\\ 
211938860 & 08 40 06.36 & +19 18 26.5 & 10.73 & 9.23 & -35.84$\pm$0.84 & -12.1$\pm$0.84 & 6.2$\pm$0.9$^{(1)}$ & -36.4 & -12.5 & 100 & 7.8\\ 
211938911 & 08 39 42.56 & +19 18 28.9 & 16.48 & 12.7 & -33.69$\pm$2.19 & -16.8$\pm$2.19 & 7.3$\pm$1.0$^{(1)}$ & -36.3 & -12.6 & 100 & 1.34\\ 
211939015 & 08 40 00.71 & +19 18 34.7 & 13.65 & 10.92 & -36.57$\pm$2.19 & -12.92$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -36.4 & -12.5 & 100 & 14.24\\ 
211939094 & 08 37 33.71 & +19 18 39.6 & 15.45 & 12.02 & -38.7$\pm$2.23 & -16.48$\pm$2.23 & 5.8$\pm$0.8$^{(1)}$ & -36.0 & -12.7 & 100 & 0.95\\ 
211939206 & 08 39 52.34 & +19 18 45.5 & 10.07 & 9.01 & -36.61$\pm$0.84 & -14.1$\pm$0.84 & 5.0$\pm$0.7$^{(1)}$ & -36.4 & -12.5 & 100 & 3.14\\ 
211939350 & 08 42 13.12 & +19 18 52.9 & 18.51 & 14.31 & -24.64$\pm$2.3 & -13.27$\pm$2.3 & 4.9$\pm$0.7$^{(1)}$ & -36.8 & -12.4 & 53 & 1.76\\ 
211939364 & 08 39 40.51 & +19 18 53.9 & 16.92 & 13.23 & -40.04$\pm$2.19 & -11.16$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -36.3 & -12.6 & 100 & 29.77\\ 
211939409 & 08 51 25.85 & +19 18 56.4 &   & 12.4 & -38.0$\pm$3.0 & -13.0$\pm$3.0 & 10.8$\pm$1.5$^{(3)}$ & -38.4 & -11.9 & 55 & 9.45\\ 
211939447 & 08 43 59.26 & +19 18 58.2 & 15.56 & 12.16 & -33.1$\pm$2.19 & -15.17$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -37.1 & -12.3 & 100 & 18.33\\ 
211939462 & 08 36 48.95 & +19 18 59.3 & 15.3 & 11.95 & -37.94$\pm$2.19 & -14.8$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -35.8 & -12.7 & 100 & 1.17\\ 
211939484 & 08 45 52.80 & +19 19 00.7 & 15.39 & 12.1 & -39.24$\pm$2.09 & -14.88$\pm$2.08 & 5.1$\pm$0.7$^{(1)}$ & -37.4 & -12.2 & 100 & 24.85\\ 
211939989 & 08 39 15.38 & +19 19 28.4 & 17.88 & 13.99 & -33.94$\pm$2.75 & -12.12$\pm$2.75 & 5.2$\pm$0.7$^{(1)}$ & -36.3 & -12.6 & 100 & 0.92\\ 
211940093 & 08 39 02.28 & +19 19 34.5 & 12.02 & 10.26 & -38.75$\pm$2.19 & -10.46$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.2 & -12.6 & 100 & 4.89\\ 
211940224 & 08 37 02.68 & +19 19 42.4 & 15.59 & 12.19 & -33.12$\pm$2.19 & -11.75$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -35.9 & -12.7 & 100 & 11.6\\ 
211940389 & 08 42 29.68 & +19 19 52.6 &   & 14.05 & -31.0$\pm$3.0 & -12.0$\pm$3.0 & 6.1$\pm$0.8$^{(3)}$ & -36.8 & -12.4 & 100 & 1.18\\ 
211940576 & 08 39 15.73 & +19 20 02.5 & 18.08 & 14.18 & -33.09$\pm$2.72 & -10.01$\pm$2.72 & 5.3$\pm$0.7$^{(1)}$ & -36.3 & -12.6 & 100 & 1.85\\ 
211941071 & 08 33 27.01 & +19 20 28.8 & 14.52 & 11.35 & -37.95$\pm$2.24 & -12.19$\pm$2.24 & 6.2$\pm$0.9$^{(1)}$ & -35.2 & -12.9 & 100 & 15.74\\ 
211941583 & 08 40 20.14 & +19 20 56.4 & 6.7 & 6.05 & -36.67$\pm$0.07 & -12.2$\pm$0.04 & 4.7$\pm$0.7$^{(0)}$ & -36.5 & -12.5 & 100 & 0.14\\ 
211941765 & 08 35 57.22 & +19 21 06.4 & 18.07 & 14.15 & -35.26$\pm$2.71 & -13.97$\pm$2.7 & 4.7$\pm$0.7$^{(1)}$ & -35.7 & -12.8 & 100 & 0.6\\ 
211941802 & 08 30 51.03 & +19 21 08.9 & 13.97 & 11.19 & -38.08$\pm$2.24 & -12.76$\pm$2.24 & 5.1$\pm$0.7$^{(1)}$ & -34.7 & -13.0 & 100 & 14.11\\ 
211942008 & 08 31 16.93 & +19 21 19.1 & 15.34 & 11.89 & -30.0$\pm$3.9 & -9.1$\pm$4.3 & 6.6$\pm$0.9$^{(1)}$ & -34.8 & -13.0 & 99 &  \\ 
211942703 & 08 38 14.26 & +19 21 55.4 & 10.65 & 9.19 & -34.04$\pm$0.8 & -10.63$\pm$0.74 & 6.1$\pm$0.8$^{(1)}$ & -36.1 & -12.7 & 100 & 7.22\\ 
211942823 & 08 39 45.75 & +19 22 01.2 & 10.48 & 9.26 & -37.88$\pm$0.79 & -13.89$\pm$0.79 & 5.5$\pm$0.8$^{(1)}$ & -36.4 & -12.6 & 100 & 5.79\\ 
211943375 & 08 30 42.58 & +19 22 30.8 & 17.62 & 13.77 & -33.72$\pm$2.77 & -14.43$\pm$2.77 & 5.4$\pm$0.8$^{(1)}$ & -34.7 & -13.1 & 100 & 1.43\\ 
211943550 & 08 36 16.16 & +19 22 40.7 & 17.62 & 13.7 & -39.44$\pm$2.71 & -15.23$\pm$2.69 & 5.5$\pm$0.8$^{(1)}$ & -35.7 & -12.8 & 100 & 2.58\\ 
211943613 & 08 40 53.82 & +19 22 44.1 & 14.72 & 11.63 & -39.73$\pm$2.19 & -13.5$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -36.6 & -12.5 & 100 & 16.51\\ 
211943617 & 08 39 18.51 & +19 22 44.2 & 18.12 & 14.01 & -37.38$\pm$2.69 & -10.87$\pm$2.69 & 5.4$\pm$0.7$^{(1)}$ & -36.3 & -12.6 & 100 & 0.55\\ 
211944193 & 08 42 23.83 & +19 23 12.5 & 17.34 & 13.4 & -36.63$\pm$2.19 & -17.2$\pm$2.19 & 6.2$\pm$0.9$^{(1)}$ & -36.8 & -12.5 & 100 & 0.48\\ 
211944662 & 08 43 06.38 & +19 23 38.9 & 20.01 & 15.4 & -24.02$\pm$3.43 & -15.26$\pm$3.43 & 3.8$\pm$0.5$^{(1)}$ & -36.9 & -12.4 & 13 & 20.73\\ 
211945119 & 08 39 53.17 & +19 24 03.8 & 16.62 & 13.01 & -35.31$\pm$2.19 & -9.52$\pm$2.19 & 4.7$\pm$0.6$^{(1)}$ & -36.4 & -12.6 & 100 & 14.18\\ 
211945329 & 08 39 03.09 & +19 24 15.6 & 17.17 & 13.41 & -36.08$\pm$2.19 & -12.39$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.2 & -12.7 & 100 & 2.38\\ 
211945337 & 08 31 00.21 & +19 24 16.1 & 17.95 & 13.99 & -38.31$\pm$2.77 & -13.42$\pm$2.77 & 5.0$\pm$0.7$^{(1)}$ & -34.8 & -13.1 & 100 &  \\ 
211945362 & 08 39 31.76 & +19 24 17.6 & 16.34 & 12.72 & -34.64$\pm$2.19 & -12.5$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.3 & -12.6 & 100 & 9.16\\ 
211945445 & 08 44 44.81 & +19 24 22.2 & 15.93 & 12.34 & -35.89$\pm$2.19 & -13.99$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -37.2 & -12.4 & 100 & 20.88\\ 
211945502 & 08 43 33.75 & +19 24 24.8 & 17.18 & 13.24 & -33.8$\pm$2.19 & -13.44$\pm$2.19 & 7.6$\pm$1.1$^{(1)}$ & -37.0 & -12.4 & 100 & 0.69\\ 
211945791 & 08 42 06.50 & +19 24 40.5 & 7.92 & 7.43 & -37.04$\pm$0.39 & -12.19$\pm$0.34 & 5.4$\pm$0.4$^{(0)}$ & -36.8 & -12.5 & 100 & 0.13\\ 
211945980 & 08 40 04.16 & +19 24 50.3 & 16.63 & 12.97 & -35.3$\pm$2.19 & -14.0$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.4 & -12.6 & 100 & 2.62\\ 
211946007 & 08 42 39.44 & +19 24 52.0 & 17.22 & 13.5 & -36.59$\pm$2.19 & -12.28$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.9 & -12.5 & 100 & 2.25\\ 
211946016 & 08 43 06.15 & +19 24 52.2 & 16.44 & 12.79 & -34.79$\pm$2.19 & -13.25$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.9 & -12.4 & 100 & 8.19\\ 
211946055 & 08 37 51.81 & +19 24 53.8 & 12.52 & 10.62 & -32.05$\pm$2.23 & -8.95$\pm$2.23 & 4.7$\pm$0.6$^{(1)}$ & -36.0 & -12.7 & 100 & 17.48\\ 
211946063 & 08 38 50.73 & +19 24 54.2 & 15.77 & 12.33 & -39.03$\pm$2.19 & -12.34$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.2 & -12.7 & 100 & 22.6\\ 
211946212 & 08 37 24.20 & +19 25 01.1 & 14.78 & 11.54 & -32.98$\pm$2.19 & -12.42$\pm$2.19 & 6.5$\pm$0.9$^{(1)}$ & -35.9 & -12.7 & 100 & 16.42\\ 
211946518 & 08 38 41.46 & +19 25 18.3 & 13.85 & 11.19 & -38.89$\pm$2.19 & -10.86$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.2 & -12.7 & 100 & 14.45\\ 
211946708 & 08 45 51.40 & +19 25 27.6 & 15.56 & 12.18 & -39.36$\pm$2.08 & -16.08$\pm$2.08 & 4.9$\pm$0.7$^{(1)}$ & -37.4 & -12.3 & 100 & 21.47\\ 
211946732 & 08 36 03.33 & +19 25 28.8 & 17.4 & 13.66 & -38.51$\pm$2.2 & -12.71$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -12.8 & 100 & 1.6\\ 
211946750 & 08 36 14.29 & +19 25 30.3 & 15.45 & 11.91 & -37.42$\pm$2.19 & -15.83$\pm$2.19 & 7.7$\pm$1.1$^{(1)}$ & -35.7 & -12.8 & 100 & 1.87\\ 
211946907 & 08 56 22.77 & +19 25 38.0 & 15.46 & 12.0 & -44.29$\pm$2.13 & -13.52$\pm$2.13 & 6.4$\pm$0.9$^{(1)}$ & -39.2 & -11.7 & 65 & 18.11\\ 
211947006 & 08 50 18.54 & +19 25 42.7 & 12.38 & 10.53 & -37.2$\pm$2.09 & -13.38$\pm$2.09 & 4.6$\pm$0.6$^{(1)}$ & -38.2 & -12.1 & 100 & 8.44\\ 
211947170 & 08 33 17.62 & +19 25 50.5 & 13.22 & 10.86 & -37.77$\pm$2.24 & -12.98$\pm$2.24 & 4.9$\pm$0.7$^{(1)}$ & -35.2 & -13.0 & 100 & 11.93\\ 
211947420 & 08 28 20.47 & +19 26 04.0 & 15.59 & 12.47 & -37.31$\pm$2.22 & -7.29$\pm$2.22 & 3.8$\pm$0.5$^{(1)}$ & -34.3 & -13.2 & 22 &  \\ 
211947631 & 08 43 05.94 & +19 26 15.2 & 9.74 & 8.46 & -35.7$\pm$1.38 & -12.56$\pm$0.69 & 5.4$\pm$0.4$^{(0)}$ & -36.9 & -12.5 & 100 & 4.74\\ 
211947686 & 08 37 46.61 & +19 26 18.0 & 10.47 & 9.28 & -36.89$\pm$2.28 & -13.22$\pm$1.12 & 5.8$\pm$0.7$^{(0)}$ & -36.0 & -12.7 & 100 & 5.94\\ 
211947849 & 08 39 38.37 & +19 26 27.1 & 12.24 & 10.29 & -36.3$\pm$0.92 & -12.46$\pm$0.92 & 5.8$\pm$0.8$^{(1)}$ & -36.3 & -12.6 & 100 & 11.17\\ 
211948030 & 08 41 06.90 & +19 26 37.0 & 16.46 & 12.85 & -38.54$\pm$2.19 & -18.95$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.6 & 100 & 25.48\\ 
211948214 & 08 42 01.60 & +19 26 46.1 & 16.94 & 13.33 & -37.68$\pm$2.19 & -16.92$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.8 & -12.5 & 100 & 30.68\\ 
211948267 & 08 41 07.25 & +19 26 48.9 & 12.07 & 10.29 & -42.44$\pm$2.19 & -12.05$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.6 & -12.6 & 100 & 10.08\\ 
211948895 & 08 43 35.50 & +19 27 23.5 & 17.46 & 13.6 & -39.31$\pm$2.25 & -13.96$\pm$2.24 & 5.3$\pm$0.7$^{(1)}$ & -37.0 & -12.4 & 100 & 1.32\\ 
211949039 & 08 40 15.50 & +19 27 31.0 & 13.25 & 10.69 & -35.6$\pm$2.19 & -13.8$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.4 & -12.6 & 100 & 11.97\\ 
211949049 & 08 41 48.18 & +19 27 31.2 & 13.1 & 10.73 & -39.7$\pm$2.19 & -11.23$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.7 & -12.5 & 100 & 11.21\\ 
211949097 & 08 39 24.98 & +19 27 33.7 & 10.27 & 9.0 & -36.91$\pm$0.84 & -13.57$\pm$0.84 & 6.1$\pm$0.8$^{(1)}$ & -36.3 & -12.7 & 100 & 3.94\\ 
211949163 & 08 39 54.41 & +19 27 37.2 & 17.12 & 13.36 & -37.03$\pm$2.19 & -15.66$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -36.4 & -12.6 & 100 & 1.27\\ 
211949413 & 08 37 57.13 & +19 27 50.0 & 16.38 & 12.77 & -33.74$\pm$2.23 & -13.63$\pm$2.23 & 5.3$\pm$0.7$^{(1)}$ & -36.0 & -12.8 & 100 & 1.33\\ 
211949471 & 08 40 22.72 & +19 27 53.2 & 10.49 & 9.34 & -35.6$\pm$0.84 & -13.51$\pm$0.84 & 4.8$\pm$0.7$^{(1)}$ & -36.5 & -12.6 & 100 & 6.84\\ 
211949501 & 08 43 05.29 & +19 27 54.6 & 14.43 & 11.55 & -37.0$\pm$2.19 & -12.26$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.9 & -12.5 & 100 & 16.33\\ 
211949728 & 08 43 08.39 & +19 28 06.1 & 16.15 & 12.39 & -34.82$\pm$2.19 & -11.9$\pm$2.19 & 8.8$\pm$1.2$^{(1)}$ & -36.9 & -12.5 & 100 & 3.25\\ 
211949871 & 08 48 04.95 & +19 28 13.8 & 15.96 & 12.54 & -36.81$\pm$2.1 & -15.95$\pm$2.1 & 5.0$\pm$0.7$^{(1)}$ & -37.8 & -12.2 & 100 & 15.9\\ 
211950081 & 08 39 28.59 & +19 28 25.2 & 11.3 & 9.53 & -35.59$\pm$0.84 & -11.88$\pm$0.84 & 7.3$\pm$1.0$^{(1)}$ & -36.3 & -12.7 & 100 & 10.22\\ 
211950227 & 08 40 25.54 & +19 28 32.8 & 9.71 & 8.76 & -35.31$\pm$1.08 & -13.23$\pm$1.08 & 4.8$\pm$0.7$^{(1)}$ & -36.5 & -12.6 & 100 &  \\ 
211950505 & 08 29 13.50 & +19 28 48.0 & 11.05 & 9.65 & -30.39$\pm$2.5 & -13.97$\pm$1.43 & 5.8$\pm$0.6$^{(0)}$ & -34.4 & -13.2 & 100 & 7.99\\ 
211950696 & 08 29 58.69 & +19 28 59.1 & 18.69 & 14.61 & -36.51$\pm$2.95 & -14.32$\pm$2.95 & 4.7$\pm$0.6$^{(1)}$ & -34.6 & -13.2 & 100 & 3.25\\ 
211950703 & 08 40 52.52 & +19 28 59.6 & 10.15 & 9.05 & -35.76$\pm$0.84 & -13.85$\pm$0.84 & 5.1$\pm$0.7$^{(1)}$ & -36.5 & -12.6 & 100 & 3.82\\ 
211950716 & 08 39 41.67 & +19 29 00.5 & 18.66 & 14.17 & -43.1$\pm$2.9 & -7.33$\pm$2.9 & 7.1$\pm$1.0$^{(1)}$ & -36.3 & -12.7 & 99 & 11.01\\ 
211950844 & 08 39 36.46 & +19 29 07.9 & 14.28 & 11.39 & -35.64$\pm$2.19 & -13.29$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.3 & -12.7 & 100 & 16.16\\ 
211950886 & 08 37 54.89 & +19 29 09.8 & 16.51 & 12.9 & -34.71$\pm$2.23 & -15.98$\pm$2.23 & 5.3$\pm$0.7$^{(1)}$ & -36.0 & -12.8 & 100 & 4.54\\ 
211950897 & 08 37 16.36 & +19 29 10.4 & 13.17 & 10.47 & -34.28$\pm$2.19 & -12.06$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & -35.9 & -12.8 & 100 & 13.12\\ 
211950941 & 08 37 26.39 & +19 29 12.8 & 13.23 & 10.83 & -37.76$\pm$2.2 & -12.15$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.9 & -12.8 & 100 & 12.32\\ 
211951021 & 08 37 17.89 & +19 29 17.1 & 18.44 & 14.35 & -35.27$\pm$2.73 & -10.78$\pm$2.73 & 5.2$\pm$0.7$^{(1)}$ & -35.9 & -12.8 & 100 & 14.11\\ 
211951112 & 08 33 10.98 & +19 29 22.2 & 16.75 & 12.91 & -37.4$\pm$2.24 & -14.27$\pm$2.24 & 7.6$\pm$1.0$^{(1)}$ & -35.2 & -13.0 & 100 & 2.31\\ 
211951223 & 08 52 39.67 & +19 29 28.6 & 17.67 & 13.76 & -42.7$\pm$2.09 & -19.47$\pm$2.08 & 5.8$\pm$0.8$^{(1)}$ & -38.6 & -12.0 & 73 & 1.52\\ 
211951283 & 08 42 30.77 & +19 29 31.1 & 16.82 & 13.23 & -35.3$\pm$2.19 & -13.3$\pm$2.19 & 4.3$\pm$0.6$^{(1)}$ & -36.8 & -12.5 & 100 &  \\ 
211951438 & 08 41 50.59 & +19 29 39.6 & 18.05 & 14.12 & -35.14$\pm$2.7 & -13.87$\pm$2.7 & 4.8$\pm$0.7$^{(1)}$ & -36.7 & -12.6 & 100 & 16.07\\ 
211951824 & 08 40 41.66 & +19 30 00.8 & 17.58 & 13.54 & -35.74$\pm$2.7 & -11.13$\pm$2.69 & 7.9$\pm$1.1$^{(1)}$ & -36.5 & -12.6 & 100 & 17.79\\ 
211951863 & 08 38 46.95 & +19 30 03.3 & 8.91 & 8.22 & -34.62$\pm$0.71 & -12.88$\pm$0.45 & 5.3$\pm$0.3$^{(0)}$ & -36.2 & -12.7 & 100 & 0.59\\ 
211952098 & 08 39 12.73 & +19 30 16.9 & 18.82 & 14.34 & -29.49$\pm$3.01 & -23.16$\pm$3.01 & 5.7$\pm$0.8$^{(1)}$ & -36.3 & -12.7 & 91 & 0.13\\ 
211952381 & 08 41 10.02 & +19 30 32.1 & 9.94 & 8.91 & -34.33$\pm$0.77 & -11.1$\pm$0.77 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.6 & 100 & 3.06\\ 
211952571 & 08 25 41.63 & +19 30 42.5 & 17.99 & 14.17 & -33.22$\pm$2.25 & -12.5$\pm$2.25 & 4.0$\pm$0.6$^{(1)}$ & -33.8 & -13.4 & 85 & 0.28\\ 
211952707 & 08 37 49.83 & +19 30 50.7 & 14.85 & 11.78 & -33.34$\pm$2.23 & -10.94$\pm$2.23 & 5.1$\pm$0.7$^{(1)}$ & -36.0 & -12.8 & 100 & 15.41\\ 
211952875 & 08 43 57.94 & +19 30 59.3 & 18.52 & 14.51 & -29.85$\pm$2.78 & -19.03$\pm$2.78 & 4.7$\pm$0.7$^{(1)}$ & -37.1 & -12.5 & 98 & 0.29\\ 
211953002 & 08 37 40.71 & +19 31 06.3 & 8.21 & 7.66 & -35.52$\pm$0.06 & -12.71$\pm$0.04 & 5.4$\pm$0.4$^{(0)}$ & -36.0 & -12.8 & 100 & 0.12\\ 
211953038 & 08 43 18.44 & +19 31 07.8 & 16.16 & 12.68 & -37.28$\pm$2.23 & -9.95$\pm$2.23 & 4.6$\pm$0.6$^{(1)}$ & -37.0 & -12.5 & 100 & 22.6\\ 
211953172 & 08 41 37.41 & +19 31 13.9 & 13.03 & 10.73 & -39.28$\pm$2.19 & -12.89$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.7 & -12.6 & 100 & 13.48\\ 
211953263 & 08 37 32.43 & +19 31 17.9 & 15.06 & 11.79 & -36.63$\pm$2.23 & -17.33$\pm$2.23 & 5.2$\pm$0.7$^{(1)}$ & -36.0 & -12.8 & 100 & 1.8\\ 
211953336 & 08 39 04.11 & +19 31 21.7 & 13.2 & 10.86 & -35.54$\pm$2.19 & -11.47$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.2 & -12.7 & 100 & 12.63\\ 
211953521 & 08 35 59.87 & +19 31 31.9 & 12.72 & 10.57 & -39.93$\pm$2.19 & -14.38$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -35.7 & -12.9 & 100 & 11.83\\ 
211953567 & 08 43 10.75 & +19 31 34.6 & 11.52 & 10.01 & -33.56$\pm$0.89 & -13.21$\pm$0.9 & 4.8$\pm$0.7$^{(1)}$ & -37.0 & -12.5 & 100 & 9.11\\ 
211953774 & 08 41 11.30 & +19 31 46.6 & 15.28 & 11.94 & -35.82$\pm$2.19 & -13.12$\pm$2.19 & 6.1$\pm$0.8$^{(1)}$ & -36.6 & -12.6 & 100 & 28.91\\ 
211953905 & 08 40 18.10 & +19 31 55.2 & 7.52 & 7.16 & -36.38$\pm$0.31 & -11.6$\pm$0.28 & 5.7$\pm$0.3$^{(0)}$ & -36.4 & -12.7 & 100 & 7.85\\ 
211953944 & 08 39 02.92 & +19 31 57.3 & 15.6 & 11.96 & -35.28$\pm$2.19 & -15.33$\pm$2.19 & 8.3$\pm$1.2$^{(1)}$ & -36.2 & -12.7 & 100 & 1.96\\ 
211953966 & 08 42 40.98 & +19 31 58.5 & 17.95 & 14.09 & -28.08$\pm$2.2 & -16.25$\pm$2.2 & 4.3$\pm$0.6$^{(1)}$ & -36.9 & -12.5 & 89 & 2.07\\ 
211954140 & 08 37 03.52 & +19 32 09.5 & 15.37 & 12.1 & -35.51$\pm$2.19 & -12.7$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -35.9 & -12.8 & 100 & 21.94\\ 
211954496 & 08 39 57.77 & +19 32 29.3 & 7.49 & 7.01 & -34.82$\pm$0.32 & -13.3$\pm$0.27 & 5.6$\pm$0.4$^{(0)}$ & -36.4 & -12.7 & 100 & 8.28\\ 
211954532 & 08 36 16.39 & +19 32 31.3 & 11.23 & 9.52 & -35.92$\pm$1.23 & -16.34$\pm$0.95 & 6.8$\pm$0.9$^{(1)}$ & -35.7 & -12.9 & 100 & 9.27\\ 
211954550 & 08 41 26.98 & +19 32 32.9 & 9.68 & 8.72 & -37.67$\pm$0.81 & -12.3$\pm$0.81 & 5.4$\pm$0.7$^{(1)}$ & -36.7 & -12.6 & 100 & 3.59\\ 
211954582 & 08 41 13.19 & +19 32 34.9 &   & 10.35 & -38.8$\pm$2.8 & -6.8$\pm$2.3 & 10.7$\pm$1.5$^{(2)}$ & -36.6 & -12.6 & 77 & 3.19\\ 
211954593 & 08 42 40.72 & +19 32 35.5 & 9.64 & 8.72 & -36.41$\pm$1.15 & -12.8$\pm$0.61 & 6.1$\pm$0.4$^{(0)}$ & -36.9 & -12.6 & 100 & 0.41\\ 
211954717 & 08 42 04.48 & +19 32 42.8 & 17.77 & 13.77 & -39.68$\pm$2.19 & -10.9$\pm$2.19 & 5.9$\pm$0.8$^{(1)}$ & -36.8 & -12.6 & 100 & 0.8\\ 
211954836 & 08 32 17.87 & +19 32 49.5 & 16.68 & 13.02 & -36.59$\pm$2.24 & -14.94$\pm$2.24 & 5.5$\pm$0.8$^{(1)}$ & -35.0 & -13.1 & 100 & 24.44\\ 
211955007 & 08 41 33.55 & +19 33 00.3 & 17.5 & 13.68 & -36.31$\pm$2.19 & -14.56$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.7 & -12.6 & 100 & 47.75\\ 
211955036 & 08 39 50.83 & +19 33 02.1 & 11.54 & 10.0 & -37.0$\pm$0.92 & -12.9$\pm$0.92 & 5.1$\pm$0.7$^{(1)}$ & -36.4 & -12.7 & 100 & 0.24\\ 
211955047 & 08 37 40.61 & +19 33 03.2 & 16.4 & 12.8 & -37.89$\pm$2.56 & -15.96$\pm$2.81 & 4.8$\pm$0.7$^{(1)}$ & -36.0 & -12.8 & 100 & 29.19\\ 
211955066 & 08 26 23.29 & +19 33 03.9 & 17.54 & 13.7 & -33.85$\pm$2.22 & -20.02$\pm$2.22 & 4.6$\pm$0.6$^{(1)}$ & -33.9 & -13.4 & 83 & 1.54\\ 
211955190 & 08 39 56.50 & +19 33 10.8 & 7.31 & 6.79 & -38.97$\pm$0.23 & -11.28$\pm$0.25 & 7.3$\pm$1.0$^{(1)}$ & -36.4 & -12.7 & 100 & 33.04\\ 
211955324 & 08 44 31.86 & +19 33 17.3 & 16.67 & 12.96 & -36.32$\pm$2.19 & -14.63$\pm$2.19 & 5.9$\pm$0.8$^{(1)}$ & -37.2 & -12.5 & 100 & 5.96\\ 
211955365 & 08 30 55.47 & +19 33 19.8 & 10.61 & 9.37 & -37.73$\pm$2.27 & -12.31$\pm$1.21 & 5.5$\pm$0.5$^{(0)}$ & -34.8 & -13.2 & 100 & 6.81\\ 
211955381 & 08 45 14.46 & +19 33 20.6 & 18.01 & 13.9 & -33.84$\pm$2.69 & -13.07$\pm$2.69 & 6.7$\pm$0.9$^{(1)}$ & -37.3 & -12.4 & 100 & 0.88\\ 
211955820 & 08 37 27.94 & +19 33 45.2 & 9.56 & 8.46 & -34.79$\pm$1.2 & -13.31$\pm$0.64 & 4.5$\pm$0.6$^{(0)}$ & -35.9 & -12.8 & 100 & 3.62\\ 
211956059 & 08 40 42.48 & +19 33 57.6 & 11.13 & 9.71 & -36.01$\pm$0.83 & -13.95$\pm$0.77 & 5.3$\pm$0.7$^{(1)}$ & -36.5 & -12.7 & 100 & 8.28\\ 
211956071 & 08 26 34.82 & +19 33 58.6 & 16.11 & 12.43 & -33.14$\pm$2.22 & -15.26$\pm$2.22 & 6.6$\pm$0.9$^{(1)}$ & -34.0 & -13.4 & 98 &  \\ 
211956096 & 08 39 59.83 & +19 34 00.3 & 11.51 & 9.48 & -37.44$\pm$0.93 & -9.56$\pm$0.92 & 8.2$\pm$1.1$^{(1)}$ & -36.4 & -12.7 & 100 & 11.47\\ 
211956407 & 08 38 53.53 & +19 34 16.9 & 13.51 & 10.96 & -38.17$\pm$2.19 & -15.98$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.2 & -12.8 & 100 & 13.98\\ 
211956421 & 08 38 06.76 & +19 34 17.8 & 17.15 & 13.39 & -36.12$\pm$2.23 & -14.2$\pm$2.23 & 4.5$\pm$0.6$^{(1)}$ & -36.1 & -12.8 & 100 & 20.88\\ 
211956426 & 08 38 41.60 & +19 34 18.1 & 17.84 & 13.96 & -37.12$\pm$2.19 & -16.07$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.2 & -12.8 & 100 & 0.61\\ 
211956610 & 08 43 12.66 & +19 34 29.0 & 17.2 & 13.46 & -34.84$\pm$2.19 & -18.12$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -37.0 & -12.5 & 100 & 2.11\\ 
211956852 & 08 39 59.98 & +19 34 40.5 & 12.46 & 10.55 & -37.56$\pm$2.19 & -9.06$\pm$2.19 & 4.7$\pm$0.7$^{(1)}$ & -36.4 & -12.7 & 100 & 10.73\\ 
211956984 & 08 42 44.41 & +19 34 47.9 & 9.56 & 8.63 & -36.96$\pm$0.99 & -11.58$\pm$0.56 & 5.7$\pm$0.4$^{(0)}$ & -36.9 & -12.6 & 100 & 0.48\\ 
211957616 & 08 35 47.31 & +19 35 22.7 & 17.21 & 13.47 & -34.87$\pm$2.19 & -18.26$\pm$2.19 & 4.7$\pm$0.6$^{(1)}$ & -35.6 & -13.0 & 100 & 1.18\\ 
211957791 & 08 39 09.10 & +19 35 32.6 & 8.45 & 7.88 & -36.87$\pm$0.46 & -14.33$\pm$0.4 & 6.1$\pm$0.5$^{(0)}$ & -36.2 & -12.8 & 100 &  \\ 
211957804 & 08 36 31.22 & +19 35 33.4 & 16.64 & 13.01 & -34.84$\pm$2.19 & -14.51$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -35.8 & -12.9 & 100 & 13.12\\ 
211958252 & 08 36 55.98 & +19 35 57.1 & 15.86 & 12.43 & -34.97$\pm$2.19 & -13.32$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -35.8 & -12.9 & 100 & 11.83\\ 
211958260 & 08 37 46.41 & +19 35 57.5 & 11.99 & 10.24 & -37.0$\pm$2.23 & -11.94$\pm$2.23 & 5.3$\pm$0.7$^{(1)}$ & -36.0 & -12.9 & 100 & 9.45\\ 
211958562 & 08 42 34.03 & +19 36 12.3 & 15.62 & 12.11 & -37.32$\pm$2.19 & -13.91$\pm$2.19 & 7.1$\pm$1.0$^{(1)}$ & -36.8 & -12.6 & 100 & 1.28\\ 
211958646 & 08 37 02.03 & +19 36 17.2 & 9.03 & 8.06 & -34.73$\pm$0.83 & -14.5$\pm$0.54 & 5.8$\pm$0.5$^{(0)}$ & -35.9 & -12.9 & 100 & 4.4\\ 
211958800 & 08 32 07.34 & +19 36 24.1 & 18.4 & 14.44 & -39.01$\pm$2.38 & -7.47$\pm$2.38 & 5.1$\pm$0.7$^{(1)}$ & -35.0 & -13.2 & 99 & 25.48\\ 
211958964 & 08 26 36.83 & +19 36 32.3 & 18.38 & 14.13 & -20.6$\pm$5.2 & -17.8$\pm$5.2 & 6.9$\pm$1.0$^{(1)}$ & -34.0 & -13.4 & 21 &  \\ 
211959273 & 08 38 58.33 & +19 36 49.6 & 13.25 & 11.04 & -29.27$\pm$2.19 & -15.83$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -36.2 & -12.8 & 99 & 14.31\\ 
211959354 & 08 27 11.66 & +19 36 54.4 & 16.07 & 12.54 & -24.6$\pm$2.81 & -20.37$\pm$2.91 & 5.5$\pm$0.8$^{(1)}$ & -34.1 & -13.4 & 17 &  \\ 
211959487 & 08 41 54.77 & +19 37 01.0 & 18.66 & 14.54 & -41.0$\pm$12.0 & -15.0$\pm$12.0 & 4.4$\pm$0.6$^{(1)}$ & -36.7 & -12.6 & 99 & 24.44\\ 
211959502 & 08 36 54.04 & +19 37 01.9 & 17.64 & 13.81 & -32.78$\pm$2.19 & -16.76$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -35.8 & -12.9 & 100 & 1.9\\ 
211959522 & 08 37 27.55 & +19 37 03.1 & 11.4 & 9.81 & -34.23$\pm$0.89 & -12.69$\pm$0.9 & 5.7$\pm$0.8$^{(1)}$ & -35.9 & -12.9 & 100 & 8.86\\ 
211959779 & 08 40 09.68 & +19 37 17.1 & 11.71 & 10.13 & -35.74$\pm$0.92 & -13.05$\pm$0.92 & 5.0$\pm$0.7$^{(1)}$ & -36.4 & -12.7 & 100 & 7.97\\ 
211959781 & 08 27 05.85 & +19 37 17.2 & 17.39 & 13.41 & -36.51$\pm$2.22 & -12.0$\pm$2.22 & 7.2$\pm$1.0$^{(1)}$ & -34.1 & -13.4 & 96 & $<$2\\ 
211959786 & 08 36 14.09 & +19 37 17.4 & 12.21 & 10.36 & -33.31$\pm$0.92 & -12.07$\pm$0.91 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -12.9 & 100 & 10.93\\ 
211959857 & 08 41 20.44 & +19 37 22.5 & 14.86 & 11.79 & -37.32$\pm$2.19 & -13.46$\pm$2.19 & 4.7$\pm$0.6$^{(1)}$ & -36.6 & -12.7 & 100 & 18.11\\ 
211959869 & 08 42 43.72 & +19 37 23.4 & 11.72 & 9.8 & -34.83$\pm$0.92 & -13.33$\pm$0.92 & 6.8$\pm$0.9$^{(1)}$ & -36.9 & -12.6 & 100 & 10.58\\ 
211960587 & 08 40 33.46 & +19 38 01.0 & 11.88 & 10.17 & -39.55$\pm$2.19 & -12.01$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.5 & -12.7 & 100 & 8.97\\ 
211960649 & 08 41 19.92 & +19 38 04.7 & 13.03 & 10.76 & -37.03$\pm$2.19 & -10.55$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -12.7 & 100 & 11.74\\ 
211961037 & 08 35 45.16 & +19 38 26.1 & 12.52 & 10.54 & -38.53$\pm$2.2 & -12.52$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.6 & -13.0 & 100 & 10.97\\ 
211964245 & 08 50 13.68 & +19 41 24.1 & 18.83 & 14.51 & -37.0$\pm$2.79 & -11.96$\pm$2.8 & 3.7$\pm$0.5$^{(1)}$ & -38.2 & -12.2 & 93 & 15.41\\ 
211966140 & 08 54 19.30 & +19 43 06.6 & 12.51 & 10.45 & -36.8$\pm$2.08 & -21.1$\pm$2.08 & 5.2$\pm$0.7$^{(1)}$ & -38.9 & -12.0 & 13 &  \\ 
211966629 & 08 43 56.72 & +19 43 32.3 & 12.75 & 10.53 & -38.51$\pm$2.19 & -13.48$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -37.1 & -12.6 & 100 & 11.97\\ 
211966707 & 08 26 17.45 & +19 43 35.8 & 16.62 & 12.98 & -33.8$\pm$2.22 & -15.13$\pm$2.22 & 4.7$\pm$0.7$^{(1)}$ & -33.9 & -13.5 & 98 & 9.25\\ 
211967293 & 08 40 56.69 & +19 44 05.2 & 11.88 & 10.21 & -35.02$\pm$0.92 & -12.43$\pm$0.92 & 4.7$\pm$0.6$^{(1)}$ & -36.6 & -12.8 & 100 & 9.11\\ 
211967873 & 08 43 32.38 & +19 44 37.7 & 11.99 & 10.22 & -35.7$\pm$0.91 & -13.31$\pm$0.91 & 5.1$\pm$0.7$^{(1)}$ & -37.0 & -12.6 & 100 & 10.15\\ 
211968029 & 08 41 59.34 & +19 44 45.1 & 15.06 & 11.89 & -37.31$\pm$2.19 & -13.99$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -12.7 & 100 & 16.61\\ 
211968088 & 08 41 28.68 & +19 44 48.1 & 10.73 & 9.47 & -36.89$\pm$0.77 & -12.46$\pm$0.77 & 5.0$\pm$0.7$^{(1)}$ & -36.7 & -12.8 & 100 & 7.57\\ 
211968228 & 08 40 13.78 & +19 44 56.0 & 15.01 & 11.88 & -36.33$\pm$2.19 & -11.78$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.4 & -12.8 & 100 & 21.32\\ 
211968460 & 08 48 30.58 & +19 45 07.3 & 18.75 & 14.56 & -41.35$\pm$2.83 & -11.62$\pm$2.83 & 5.0$\pm$0.7$^{(1)}$ & -37.9 & -12.4 & 100 & 0.79\\ 
211968779 & 08 39 05.12 & +19 45 26.4 & 16.89 & 13.16 & -35.7$\pm$2.19 & -12.05$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.2 & -12.9 & 100 & 17.18\\ 
211969170 & 08 40 13.08 & +19 45 49.9 & 18.24 & 14.28 & -29.34$\pm$2.74 & -21.25$\pm$2.74 & 5.3$\pm$0.7$^{(1)}$ & -36.4 & -12.8 & 96 &  \\ 
211969273 & 08 38 27.73 & +19 45 55.6 & 15.01 & 11.76 & -35.1$\pm$2.23 & -11.78$\pm$2.23 & 5.6$\pm$0.8$^{(1)}$ & -36.1 & -12.9 & 100 & 17.27\\ 
211969494 & 08 43 20.19 & +19 46 08.5 & 10.59 & 9.36 & -35.67$\pm$0.74 & -12.68$\pm$0.75 & 5.5$\pm$0.8$^{(1)}$ & -37.0 & -12.7 & 100 & 6.38\\ 
211969550 & 08 40 56.83 & +19 46 11.9 &   & 13.99 & -34.0$\pm$5.0 & -33.0$\pm$5.0 & 8.3$\pm$1.1$^{(3)}$ & -36.6 & -12.8 & 19 &  \\ 
211969807 & 08 38 32.82 & +19 46 25.8 & 15.21 & 12.01 & -34.42$\pm$2.19 & -13.57$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.1 & -12.9 & 100 & 17.08\\ 
211970147 & 08 40 13.45 & +19 46 43.7 & 12.72 & 10.64 & -35.97$\pm$2.19 & -11.07$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.4 & -12.8 & 100 & 11.6\\ 
211970427 & 08 39 09.85 & +19 46 58.9 & 14.77 & 11.35 & -36.87$\pm$2.19 & -13.04$\pm$2.19 & 8.7$\pm$1.2$^{(1)}$ & -36.2 & -12.9 & 100 & 4.38\\ 
211970517 & 08 45 26.30 & +19 47 03.8 & 15.18 & 11.72 & -35.87$\pm$2.14 & -14.73$\pm$2.14 & 6.8$\pm$0.9$^{(1)}$ & -37.3 & -12.6 & 100 & 0.91\\ 
211970520 & 08 40 04.16 & +19 47 04.0 & 11.75 & 10.0 & -34.28$\pm$0.84 & -14.11$\pm$0.84 & 5.7$\pm$0.8$^{(1)}$ & -36.4 & -12.9 & 100 & 10.43\\ 
211970613 & 08 39 06.96 & +19 47 08.0 & 18.29 & 14.14 & -32.99$\pm$2.19 & -16.27$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.2 & -12.9 & 100 & 1.01\\ 
211970678 & 08 39 29.40 & +19 47 11.8 & 12.19 & 10.06 & -38.38$\pm$2.19 & -13.79$\pm$2.19 & 6.3$\pm$0.9$^{(1)}$ & -36.3 & -12.9 & 100 & 13.79\\ 
211970684 & 08 37 24.50 & +19 47 12.0 & 17.26 & 13.54 & -35.1$\pm$2.21 & -13.88$\pm$2.19 & 4.2$\pm$0.6$^{(1)}$ & -35.9 & -13.0 & 100 & 1.63\\ 
211970750 & 08 40 17.62 & +19 47 15.2 & 9.76 & 8.58 & -36.11$\pm$0.94 & -14.51$\pm$0.94 & 7.0$\pm$1.0$^{(1)}$ & -36.4 & -12.8 & 100 & 64.03\\ 
211970966 & 08 43 06.70 & +19 47 29.7 & 13.11 & 10.77 & -35.92$\pm$2.19 & -12.85$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.9 & -12.7 & 100 & 13.07\\ 
211970974 & 08 44 06.99 & +19 47 30.1 & 19.01 & 12.65 & -34.0$\pm$3.0 & -6.0$\pm$3.0 & 6.0$\pm$0.8$^{(1)}$ & -37.1 & -12.6 & 100 & 1.45\\ 
211971074 & 08 44 26.53 & +19 47 35.9 & 13.45 & 10.91 & -42.8$\pm$2.19 & -16.43$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -37.2 & -12.6 & 100 & 14.31\\ 
211971189 & 08 39 16.78 & +19 47 42.8 & 15.34 & 12.08 & -37.89$\pm$2.19 & -11.69$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -12.9 & 100 & 21.78\\ 
211971354 & 08 31 40.45 & +19 47 54.2 & 14.16 & 11.03 & -35.12$\pm$2.24 & -12.07$\pm$2.24 & 7.0$\pm$1.0$^{(1)}$ & -34.9 & -13.3 & 100 & 8.26\\ 
211971690 & 08 37 11.48 & +19 48 13.3 & 11.09 & 9.69 & -34.44$\pm$0.77 & -12.47$\pm$0.77 & 5.2$\pm$0.7$^{(1)}$ & -35.9 & -13.0 & 100 & 8.26\\ 
211971819 & 08 27 50.95 & +19 48 20.8 & 14.91 & 11.78 & -37.4$\pm$2.22 & -13.41$\pm$2.22 & 5.0$\pm$0.7$^{(1)}$ & -34.2 & -13.5 & 99 & 17.08\\ 
211971871 & 08 40 00.62 & +19 48 23.6 & 10.12 & 9.08 & -37.01$\pm$0.79 & -13.48$\pm$0.79 & 4.9$\pm$0.7$^{(1)}$ & -36.4 & -12.9 & 100 & 2.96\\ 
211972086 & 08 50 49.84 & +19 48 36.5 & 16.33 & 12.65 & -37.17$\pm$2.09 & -14.69$\pm$2.09 & 6.4$\pm$0.9$^{(1)}$ & -38.3 & -12.3 & 100 & 7.49\\ 
211972445 & 08 44 57.25 & +19 48 55.9 & 16.72 & 13.01 & -41.9$\pm$2.3 & -12.38$\pm$2.3 & 5.6$\pm$0.8$^{(1)}$ & -37.3 & -12.6 & 100 &  \\ 
211972472 & 08 42 15.50 & +19 48 57.6 & 16.09 & 12.62 & -37.79$\pm$2.19 & -12.58$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.8 & -12.8 & 100 & 15.33\\ 
211972478 & 08 39 37.15 & +19 48 58.0 & 14.33 & 11.39 & -36.33$\pm$2.19 & -13.95$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.3 & -12.9 & 100 & 16.07\\ 
211972627 & 08 41 10.31 & +19 49 07.0 & 11.26 & 9.75 & -35.65$\pm$0.84 & -12.8$\pm$0.84 & 5.3$\pm$0.7$^{(1)}$ & -36.6 & -12.8 & 100 & 9.05\\ 
211973202 & 08 48 01.29 & +19 49 39.2 & 17.28 & 13.51 & -36.17$\pm$2.1 & -19.19$\pm$2.1 & 5.1$\pm$0.7$^{(1)}$ & -37.8 & -12.4 & 99 & 1.63\\ 
211973205 & 08 39 47.07 & +19 49 39.5 & 12.34 & 10.44 & -38.34$\pm$2.19 & -13.83$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.4 & -12.9 & 100 & 10.54\\ 
211973218 & 08 45 22.35 & +19 49 40.1 & 16.62 & 12.5 & -42.98$\pm$2.14 & -10.74$\pm$2.14 & 13.1$\pm$1.8$^{(1)}$ & -37.3 & -12.6 & 29 & 1.74\\ 
211973228 & 08 43 27.60 & +19 49 40.6 & 16.58 & 12.92 & -36.68$\pm$2.19 & -13.44$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -37.0 & -12.7 & 100 &  \\ 
211973314 & 08 41 10.67 & +19 49 46.4 & 8.93 & 8.19 & -34.48$\pm$0.74 & -14.15$\pm$0.41 & 5.8$\pm$0.3$^{(0)}$ & -36.6 & -12.8 & 100 & 0.75\\ 
211973504 & 08 41 41.75 & +19 49 57.5 & 17.3 & 13.6 & -37.33$\pm$2.19 & -17.98$\pm$2.19 & 3.9$\pm$0.5$^{(1)}$ & -36.7 & -12.8 & 100 & 2.32\\ 
211973540 & 08 49 51.46 & +19 49 59.6 & 18.5 & 14.13 & -39.84$\pm$2.78 & -3.99$\pm$2.78 & 6.2$\pm$0.9$^{(1)}$ & -38.1 & -12.3 & 90 &  \\ 
211973658 & 08 40 23.47 & +19 50 05.9 & 7.99 & 7.59 & -36.2$\pm$0.34 & -13.11$\pm$0.33 & 6.7$\pm$0.4$^{(0)}$ & -36.5 & -12.9 & 100 & 57.87\\ 
211973710 & 08 42 13.65 & +19 50 08.6 & 15.29 & 12.05 & -40.57$\pm$2.19 & -13.98$\pm$2.19 & 4.7$\pm$0.7$^{(1)}$ & -36.8 & -12.8 & 100 & 21.94\\ 
211973760 & 08 48 23.58 & +19 50 11.8 & 16.38 & 12.84 & -39.52$\pm$2.12 & -13.5$\pm$2.11 & 4.6$\pm$0.6$^{(1)}$ & -37.9 & -12.4 & 100 & 13.18\\ 
211974178 & 08 38 55.48 & +19 50 33.5 & 17.28 & 13.58 & -35.99$\pm$2.19 & -15.23$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.2 & -13.0 & 100 & 1.7\\ 
211974283 & 08 28 20.94 & +19 50 38.6 & 10.72 & 9.43 & -29.67$\pm$2.28 & -13.52$\pm$1.3 & 4.9$\pm$0.5$^{(0)}$ & -34.3 & -13.5 & 99 &  \\ 
211974687 & 08 35 50.26 & +19 51 00.1 & 17.31 & 13.56 & -35.4$\pm$2.21 & -14.46$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -35.7 & -13.1 & 100 & 0.9\\ 
211974702 & 08 40 31.69 & +19 51 01.0 & 11.35 & 9.91 & -34.6$\pm$0.84 & -12.86$\pm$0.84 & 4.9$\pm$0.7$^{(1)}$ & -36.5 & -12.9 & 100 & 8.49\\ 
211974724 & 08 38 51.04 & +19 51 02.1 & 15.96 & 12.36 & -40.02$\pm$2.19 & -15.82$\pm$2.19 & 6.6$\pm$0.9$^{(1)}$ & -36.2 & -13.0 & 100 & 33.04\\ 
211975002 & 08 51 23.22 & +19 51 18.3 & 18.33 & 14.45 & -34.11$\pm$2.64 & -21.71$\pm$2.64 & 4.9$\pm$0.7$^{(1)}$ & -38.4 & -12.3 & 58 & 12.63\\ 
211975006 & 08 41 09.60 & +19 51 18.6 & 10.45 & 8.94 & -36.64$\pm$0.77 & -13.12$\pm$0.77 & 7.3$\pm$1.0$^{(1)}$ & -36.6 & -12.8 & 100 & 3.07\\ 
211975426 & 08 39 21.85 & +19 51 40.3 & 12.17 & 10.37 & -36.24$\pm$2.19 & -11.67$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.3 & -12.9 & 100 & 6.26\\ 
211975504 & 08 38 54.21 & +19 51 44.6 & 18.25 & 14.35 & -33.45$\pm$2.23 & -17.41$\pm$2.23 & 4.8$\pm$0.7$^{(1)}$ & -36.2 & -13.0 & 100 &  \\ 
211975510 & 08 38 29.63 & +19 51 44.9 & 13.39 & 10.93 & -39.36$\pm$2.19 & -11.39$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.1 & -13.0 & 100 & 11.83\\ 
211975634 & 08 45 40.31 & +19 51 52.1 & 19.3 & 14.67 & -47.08$\pm$2.8 & -11.08$\pm$2.8 & 5.1$\pm$0.7$^{(1)}$ & -37.4 & -12.6 & 99 &  \\ 
211975682 & 08 36 27.12 & +19 51 54.6 & 14.4 & 11.23 & -34.7$\pm$2.19 & -14.34$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & -35.8 & -13.1 & 100 & 9.22\\ 
211975860 & 08 47 50.35 & +19 52 04.3 & 18.91 & 14.64 & -37.96$\pm$4.69 & -11.09$\pm$4.69 & 4.7$\pm$0.7$^{(1)}$ & -37.8 & -12.5 & 100 & 31.99\\ 
211976081 & 08 35 46.78 & +19 52 15.3 & 13.84 & 11.06 & -40.53$\pm$2.19 & -13.28$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -35.6 & -13.1 & 100 & 14.88\\ 
211976270 & 08 41 50.08 & +19 52 27.0 & 6.58 & 4.68 & -36.79$\pm$0.04 & -13.56$\pm$0.02 & 5.6$\pm$0.3$^{(0)}$ & -36.7 & -12.8 & 100 &  \\ 
211976466 & 08 41 26.81 & +19 52 36.7 & 17.66 & 13.76 & -35.82$\pm$2.19 & -13.12$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.7 & -12.8 & 100 & 1.64\\ 
211976535 & 08 36 11.43 & +19 52 40.2 & 14.62 & 11.66 & -39.96$\pm$2.19 & -13.52$\pm$2.2 & 4.6$\pm$0.6$^{(1)}$ & -35.7 & -13.1 & 100 & 18.55\\ 
211976838 & 08 33 24.62 & +19 52 57.9 & 16.54 & 12.78 & -37.81$\pm$2.24 & -17.06$\pm$2.24 & 6.6$\pm$0.9$^{(1)}$ & -35.2 & -13.3 & 100 & 1.49\\ 
211977843 & 08 36 19.16 & +19 53 54.9 & 16.1 & 12.57 & -37.65$\pm$2.19 & -15.21$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -35.7 & -13.1 & 100 & 9.54\\ 
211977997 & 08 43 01.87 & +19 54 04.6 & 17.9 & 14.05 & -34.4$\pm$2.68 & -16.82$\pm$2.68 & 4.1$\pm$0.6$^{(1)}$ & -36.9 & -12.8 & 100 & 0.98\\ 
211978157 & 08 37 27.89 & +19 54 12.7 & 16.1 & 12.53 & -33.29$\pm$2.22 & -14.02$\pm$2.22 & 5.7$\pm$0.8$^{(1)}$ & -35.9 & -13.1 & 100 & 1.79\\ 
211978243 & 08 28 00.99 & +19 54 17.3 & 12.4 & 10.49 & -35.12$\pm$2.22 & -15.37$\pm$2.22 & 4.9$\pm$0.7$^{(1)}$ & -34.2 & -13.6 & 100 & 10.69\\ 
211978779 & 08 43 51.81 & +19 54 49.0 & 13.57 & 10.97 & -38.63$\pm$2.19 & -16.53$\pm$2.19 & 4.7$\pm$0.7$^{(1)}$ & -37.1 & -12.7 & 100 & 13.6\\ 
211978879 & 08 36 33.38 & +19 54 54.2 & 15.26 & 12.01 & -36.53$\pm$2.19 & -16.27$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -35.8 & -13.1 & 100 & 9.85\\ 
211978880 & 08 40 15.71 & +19 54 54.2 & 12.22 & 10.01 & -38.25$\pm$2.19 & -12.65$\pm$2.19 & 7.0$\pm$1.0$^{(1)}$ & -36.4 & -12.9 & 100 & 10.62\\ 
211978972 & 08 48 07.45 & +19 54 59.2 & 17.19 & 13.4 & -36.64$\pm$2.1 & -17.82$\pm$2.1 & 4.4$\pm$0.6$^{(1)}$ & -37.8 & -12.5 & 99 & 1.93\\ 
211978983 & 08 40 03.67 & +19 54 59.5 & 16.11 & 12.36 & -36.61$\pm$2.19 & -14.45$\pm$2.19 & 8.4$\pm$1.2$^{(1)}$ & -36.4 & -12.9 & 100 & 1.37\\ 
211979060 & 08 42 50.50 & +19 55 03.8 & 16.17 & 12.66 & -37.28$\pm$2.19 & -13.06$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.9 & -12.8 & 100 & 24.44\\ 
211979237 & 08 36 04.43 & +19 55 13.0 & 13.94 & 11.16 & -41.62$\pm$2.19 & -16.0$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.7 & -13.2 & 100 & 15.82\\ 
211979250 & 08 36 30.50 & +19 55 13.9 & 17.97 & 13.87 & -36.2$\pm$2.7 & -15.98$\pm$2.69 & 6.3$\pm$0.9$^{(1)}$ & -35.8 & -13.1 & 100 & 2.19\\ 
211979334 & 08 40 48.32 & +19 55 18.9 & 10.82 & 9.51 & -35.04$\pm$0.84 & -11.61$\pm$0.84 & 5.2$\pm$0.7$^{(1)}$ & -36.5 & -12.9 & 100 & 7.93\\ 
211979345 & 08 41 13.77 & +19 55 19.2 & 8.35 & 7.77 & -36.42$\pm$0.39 & -13.16$\pm$0.39 & 5.9$\pm$0.7$^{(0)}$ & -36.6 & -12.9 & 100 & 0.59\\ 
211979717 & 08 40 36.01 & +19 55 38.9 & 13.02 & 10.6 & -24.3$\pm$2.19 & -13.23$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.5 & -12.9 & 50 &  \\ 
211980019 & 08 48 34.51 & +19 55 57.4 & 15.26 & 11.89 & -39.73$\pm$2.12 & -11.6$\pm$2.11 & 6.0$\pm$0.8$^{(1)}$ & -37.9 & -12.5 & 100 & 25.7\\ 
211980039 & 08 40 30.59 & +19 55 58.9 & 15.85 & 12.39 & -38.52$\pm$2.19 & -13.17$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.5 & -12.9 & 100 & 16.61\\ 
211980142 & 08 40 56.93 & +19 56 05.5 & 8.63 & 8.05 & -34.67$\pm$0.62 & -13.59$\pm$0.39 & 5.6$\pm$0.3$^{(0)}$ & -36.6 & -12.9 & 100 &  \\ 
211980169 & 08 41 10.53 & +19 56 06.6 & 15.5 & 11.97 & -30.34$\pm$2.26 & -13.43$\pm$2.19 & 6.8$\pm$0.9$^{(1)}$ & -36.6 & -12.9 & 100 & 10.02\\ 
211980170 & 08 40 54.87 & +19 56 06.6 & 11.78 & 10.13 & -37.38$\pm$0.84 & -13.46$\pm$0.84 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -12.9 & 100 & 9.13\\ 
211980180 & 08 41 09.79 & +19 56 07.2 &   & 10.76 & -40.4$\pm$2.1 & -10.8$\pm$2.2 & 5.5$\pm$0.8$^{(2)}$ & -36.6 & -12.9 & 100 & 13.42\\ 
211980234 & 08 30 02.66 & +19 56 11.1 & 18.69 & 14.26 & -25.47$\pm$2.9 & -7.24$\pm$2.9 & 5.9$\pm$0.8$^{(1)}$ & -34.6 & -13.5 & 63 & 28.91\\ 
211980252 & 08 44 21.25 & +19 56 11.8 & 17.05 & 13.26 & -36.78$\pm$2.19 & -15.05$\pm$2.19 & 6.4$\pm$0.9$^{(1)}$ & -37.2 & -12.7 & 100 & 13.3\\ 
211980309 & 08 32 25.38 & +19 56 15.1 & 12.55 & 10.54 & -30.86$\pm$2.24 & -23.17$\pm$2.24 & 5.1$\pm$0.7$^{(1)}$ & -35.0 & -13.4 & 60 &  \\ 
211980450 & 08 40 39.38 & +19 56 23.9 & 16.48 & 12.69 & -39.67$\pm$2.19 & -12.58$\pm$2.19 & 8.0$\pm$1.1$^{(1)}$ & -36.5 & -12.9 & 100 & 1.02\\ 
211980574 & 08 40 51.86 & +19 56 30.4 & 15.78 & 12.4 & -37.54$\pm$2.19 & -13.57$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -36.5 & -12.9 & 100 & 25.92\\ 
211980688 & 08 41 25.84 & +19 56 36.8 & 10.53 & 9.33 & -35.15$\pm$0.76 & -11.22$\pm$0.76 & 4.9$\pm$0.7$^{(1)}$ & -36.6 & -12.9 & 100 & 6.78\\ 
211981232 & 08 33 34.51 & +19 57 05.9 & 18.26 & 14.32 & -42.46$\pm$2.88 & -19.22$\pm$2.88 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -13.3 & 100 & 0.8\\ 
211981509 & 08 32 39.47 & +19 57 22.3 & 11.94 & 10.37 & -33.9$\pm$0.84 & -13.46$\pm$0.84 & 4.2$\pm$0.6$^{(1)}$ & -35.1 & -13.4 & 100 & 27.84\\ 
211981575 & 08 36 08.60 & +19 57 25.4 & 17.11 & 13.2 & -36.35$\pm$2.7 & -15.74$\pm$2.69 & 6.5$\pm$0.9$^{(1)}$ & -35.7 & -13.2 & 100 & 1.02\\ 
211981687 & 08 36 01.62 & +19 57 31.4 & 18.41 & 14.32 & -38.53$\pm$2.74 & -9.71$\pm$2.73 & 5.5$\pm$0.8$^{(1)}$ & -35.7 & -13.2 & 100 & 1.85\\ 
211981916 & 08 41 43.68 & +19 57 43.7 & 12.01 & 10.26 & -35.41$\pm$0.92 & -11.94$\pm$0.92 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -12.9 & 100 & 9.42\\ 
211981954 & 08 37 49.32 & +19 57 46.4 & 18.44 & 14.22 & -39.6$\pm$2.93 & -15.83$\pm$2.92 & 5.2$\pm$0.7$^{(1)}$ & -36.0 & -13.1 & 100 & 0.28\\ 
211982230 & 08 39 30.95 & +19 58 01.9 & 16.51 & 12.69 & -37.48$\pm$2.19 & -16.02$\pm$2.19 & 8.7$\pm$1.2$^{(1)}$ & -36.3 & -13.0 & 100 & 1.18\\ 
211982334 & 08 41 33.83 & +19 58 08.7 & 11.44 & 9.93 & -35.27$\pm$0.77 & -14.33$\pm$0.77 & 4.7$\pm$0.6$^{(1)}$ & -36.7 & -12.9 & 100 & 8.97\\ 
211982469 & 08 40 11.45 & +19 58 16.1 & 6.62 & 6.53 & -35.17$\pm$0.04 & -13.57$\pm$0.02 & 4.9$\pm$0.4$^{(0)}$ & -36.4 & -13.0 & 100 & 0.24\\ 
211982727 & 08 42 29.89 & +19 58 31.7 & 17.61 & 13.73 & -38.0$\pm$2.19 & -14.06$\pm$2.19 & 4.2$\pm$0.6$^{(1)}$ & -36.8 & -12.9 & 100 & 0.59\\ 
211982734 & 08 41 28.80 & +19 58 32.1 & 15.56 & 12.1 & -38.36$\pm$2.19 & -16.24$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -36.7 & -12.9 & 100 & 1.02\\ 
211982810 & 08 32 52.24 & +19 58 35.9 &   & 10.56 & -32.2$\pm$1.7 & -12.8$\pm$2.1 & 5.7$\pm$0.8$^{(2)}$ & -35.1 & -13.4 & 100 & 11.38\\ 
211982945 & 08 38 01.14 & +19 58 43.0 & 16.7 & 12.86 & -34.75$\pm$2.23 & -13.69$\pm$2.23 & 6.8$\pm$0.9$^{(1)}$ & -36.0 & -13.1 & 100 & 0.54\\ 
211983023 & 08 32 01.89 & +19 58 47.2 & 16.91 & 13.21 & -36.38$\pm$2.24 & -15.68$\pm$2.24 & 4.9$\pm$0.7$^{(1)}$ & -35.0 & -13.4 & 100 & 22.95\\ 
211983461 & 08 37 52.09 & +19 59 13.9 & 11.04 & 9.69 & -36.12$\pm$0.77 & -13.54$\pm$0.77 & 4.8$\pm$0.7$^{(1)}$ & -36.0 & -13.1 & 100 & 7.95\\ 
211983476 & 08 41 26.03 & +19 59 15.2 & 16.66 & 13.08 & -37.54$\pm$2.19 & -16.27$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -12.9 & 100 & 4.3\\ 
211983499 & 08 38 07.58 & +19 59 16.3 & 11.74 & 9.9 & -34.53$\pm$0.93 & -14.14$\pm$0.92 & 6.2$\pm$0.8$^{(1)}$ & -36.1 & -13.1 & 100 & 8.97\\ 
211983544 & 08 42 37.62 & +19 59 19.0 & 17.17 & 13.39 & -34.3$\pm$2.57 & -13.28$\pm$2.76 & 5.6$\pm$0.8$^{(1)}$ & -36.9 & -12.9 & 100 & 1.69\\ 
211983602 & 08 38 37.86 & +19 59 23.1 & 8.12 & 7.61 & -37.05$\pm$0.29 & -13.76$\pm$0.33 & 5.1$\pm$0.7$^{(1)}$ & -36.2 & -13.1 & 100 &  \\ 
211983725 & 08 39 41.03 & +19 59 28.8 & 14.45 & 11.32 & -34.63$\pm$2.19 & -12.36$\pm$2.19 & 6.3$\pm$0.9$^{(1)}$ & -36.3 & -13.0 & 100 & 4.22\\ 
211983811 & 08 43 32.63 & +19 59 33.0 & 16.58 & 12.92 & -38.12$\pm$2.14 & -13.58$\pm$2.14 & 5.7$\pm$0.8$^{(1)}$ & -37.0 & -12.8 & 100 & 34.17\\ 
211984058 & 08 38 41.29 & +19 59 47.2 & 18.39 & 14.27 & -38.07$\pm$2.88 & -18.64$\pm$2.87 & 5.2$\pm$0.7$^{(1)}$ & -36.2 & -13.1 & 100 & 14.88\\ 
211984100 & 08 41 47.94 & +19 59 50.1 & 18.57 & 14.5 & -42.64$\pm$2.92 & -18.92$\pm$2.92 & 4.9$\pm$0.7$^{(1)}$ & -36.7 & -12.9 & 100 & 18.9\\ 
211984130 & 08 32 46.79 & +19 59 51.8 & 16.53 & 12.95 & -36.36$\pm$2.24 & -15.92$\pm$2.24 & 5.0$\pm$0.7$^{(1)}$ & -35.1 & -13.4 & 100 & 25.26\\ 
211984243 & 08 39 03.59 & +19 59 59.1 & 8.28 & 7.77 & -33.64$\pm$0.54 & -13.38$\pm$0.35 & 5.3$\pm$0.3$^{(0)}$ & -36.2 & -13.1 & 100 & 1.95\\ 
211984495 & 08 43 13.26 & +20 00 16.0 & 18.31 & 14.28 & -42.54$\pm$2.11 & -19.3$\pm$2.11 & 5.6$\pm$0.8$^{(1)}$ & -37.0 & -12.8 & 100 & 2.62\\ 
211985076 & 08 37 33.82 & +20 00 49.2 & 8.61 & 7.95 & -34.56$\pm$0.33 & -13.31$\pm$0.43 & 4.9$\pm$0.7$^{(1)}$ & -36.0 & -13.1 & 100 & 25.7\\ 
211985346 & 08 39 52.76 & +20 01 05.2 & 16.22 & 12.66 & -37.83$\pm$2.19 & -15.05$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.4 & -13.0 & 100 & 9.0\\ 
211985566 & 08 39 14.53 & +20 01 19.2 & 14.88 & 11.72 & -37.0$\pm$2.19 & -14.36$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -36.3 & -13.1 & 100 & 17.68\\ 
211985987 & 08 39 41.75 & +20 01 41.7 & 14.8 & 11.76 & -36.2$\pm$2.19 & -12.42$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.3 & -13.0 & 100 & 18.33\\ 
211986176 & 08 39 59.08 & +20 01 53.1 & 9.11 & 8.21 & -37.24$\pm$0.71 & -15.97$\pm$0.47 & 5.0$\pm$0.3$^{(0)}$ & -36.4 & -13.0 & 100 & 0.67\\ 
211986473 & 08 42 20.13 & +20 02 11.7 & 9.54 & 8.41 & -35.64$\pm$0.58 & -14.71$\pm$0.64 & 7.6$\pm$1.0$^{(1)}$ & -36.8 & -12.9 & 100 & 7.38\\ 
211986537 & 08 41 15.42 & +20 02 16.0 & 13.6 & 11.02 & -39.43$\pm$2.19 & -14.08$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.6 & -13.0 & 100 & 13.54\\ 
211986948 & 08 39 03.22 & +20 02 37.6 & 13.69 & 11.05 & -41.75$\pm$2.19 & -14.06$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.2 & -13.1 & 100 & 14.31\\ 
211987717 & 08 42 21.11 & +20 03 20.9 & 17.01 & 13.27 & -37.57$\pm$2.19 & -16.92$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -36.8 & -12.9 & 100 & 3.9\\ 
211987847 & 08 40 13.10 & +20 03 28.1 & 15.9 & 12.25 & -38.68$\pm$2.19 & -11.32$\pm$2.19 & 7.6$\pm$1.0$^{(1)}$ & -36.4 & -13.0 & 100 & 0.84\\ 
211988080 & 08 47 54.73 & +20 03 42.9 & 15.23 & 12.03 & -41.3$\pm$2.1 & -7.37$\pm$2.1 & 5.3$\pm$0.7$^{(1)}$ & -37.8 & -12.6 & 99 & 27.58\\ 
211988223 & 08 38 08.01 & +20 03 50.5 & 17.21 & 13.48 & -35.61$\pm$2.23 & -13.11$\pm$2.23 & 4.4$\pm$0.6$^{(1)}$ & -36.1 & -13.1 & 100 & 1.16\\ 
211988287 & 08 39 55.06 & +20 03 54.1 & 9.96 & 8.96 & -36.38$\pm$0.84 & -13.04$\pm$0.84 & 4.9$\pm$0.7$^{(1)}$ & -36.4 & -13.1 & 100 & 3.29\\ 
211988324 & 08 43 15.23 & +20 03 56.1 & 13.0 & 10.68 & -37.25$\pm$2.19 & -11.46$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -37.0 & -12.9 & 100 & 10.89\\ 
211988451 & 08 40 11.46 & +20 04 03.3 & 15.53 & 11.84 & -41.04$\pm$2.19 & -13.66$\pm$2.19 & 9.3$\pm$1.3$^{(1)}$ & -36.4 & -13.0 & 99 & 0.8\\ 
211988454 & 08 38 50.01 & +20 04 03.4 & 10.6 & 9.37 & -35.87$\pm$0.85 & -13.45$\pm$0.82 & 5.2$\pm$0.7$^{(1)}$ & -36.2 & -13.1 & 100 & 8.44\\ 
211988531 & 08 39 30.42 & +20 04 08.6 & 10.09 & 8.81 & -35.55$\pm$0.86 & -13.23$\pm$0.9 & 7.2$\pm$1.0$^{(1)}$ & -36.3 & -13.1 & 100 & 7.22\\ 
211988628 & 08 39 15.80 & +20 04 14.1 & 14.0 & 10.87 & -38.12$\pm$2.22 & -12.72$\pm$2.2 & 7.7$\pm$1.1$^{(1)}$ & -36.3 & -13.1 & 100 & 7.95\\ 
211988700 & 08 42 56.75 & +20 04 18.2 & 16.51 & 12.79 & -36.24$\pm$2.19 & -13.04$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.9 & -12.9 & 100 & 6.46\\ 
211988831 & 08 33 33.95 & +20 04 25.7 & 15.99 & 12.55 & -38.31$\pm$2.24 & -14.41$\pm$2.24 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -13.4 & 100 & 14.59\\ 
211988832 & 08 43 20.13 & +20 04 25.9 & 17.81 & 13.88 & -36.85$\pm$2.69 & -12.01$\pm$2.69 & 5.7$\pm$0.8$^{(1)}$ & -37.0 & -12.9 & 100 & 0.99\\ 
211988997 & 08 41 49.45 & +20 04 36.2 & 15.56 & 11.97 & -35.56$\pm$2.19 & -16.02$\pm$2.19 & 7.6$\pm$1.1$^{(1)}$ & -36.7 & -13.0 & 100 & 19.65\\ 
211989060 & 08 35 59.46 & +20 04 40.5 & 16.82 & 13.0 & -38.75$\pm$2.2 & -14.12$\pm$2.19 & 7.1$\pm$1.0$^{(1)}$ & -35.7 & -13.3 & 100 & 1.76\\ 
211989144 & 08 43 20.29 & +20 04 45.6 & 17.36 & 13.56 & -37.59$\pm$2.19 & -12.17$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -37.0 & -12.9 & 100 & 7.4\\ 
211989185 & 08 32 33.42 & +20 04 48.4 & 12.74 & 10.63 & -37.62$\pm$2.24 & -12.97$\pm$2.24 & 5.0$\pm$0.7$^{(1)}$ & -35.1 & -13.5 & 100 & 11.65\\ 
211989299 & 08 39 22.45 & +20 04 55.1 & 15.91 & 12.51 & -37.3$\pm$2.19 & -12.44$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -13.1 & 100 & 12.84\\ 
211989558 & 08 39 42.79 & +20 05 10.4 & 7.74 & 7.16 & -36.02$\pm$0.22 & -10.97$\pm$0.29 & 7.0$\pm$1.0$^{(1)}$ & -36.3 & -13.1 & 100 & 13.36\\ 
211989620 & 08 40 15.21 & +20 05 14.0 & 16.56 & 12.69 & -37.17$\pm$2.19 & -12.11$\pm$2.19 & 9.1$\pm$1.3$^{(1)}$ & -36.4 & -13.0 & 100 & 0.88\\ 
211989807 & 08 40 53.97 & +20 05 24.4 & 16.39 & 12.88 & -38.48$\pm$2.19 & -14.36$\pm$2.19 & 4.1$\pm$0.6$^{(1)}$ & -36.6 & -13.0 & 100 & 20.59\\ 
211989950 & 08 42 16.64 & +20 05 32.5 & 13.56 & 10.99 & -38.98$\pm$2.19 & -13.26$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.8 & -12.9 & 100 & 12.84\\ 
211990019 & 08 38 21.87 & +20 05 35.7 & 18.01 & 13.89 & -36.33$\pm$2.25 & -8.07$\pm$2.23 & 5.9$\pm$0.8$^{(1)}$ & -36.1 & -13.2 & 100 & 0.41\\ 
211990313 & 08 40 28.47 & +20 05 51.3 & 16.41 & 13.03 & -27.52$\pm$2.19 & -15.6$\pm$2.19 & 3.8$\pm$0.5$^{(1)}$ & -36.5 & -13.0 & 53 &  \\ 
211990578 & 08 41 32.52 & +20 06 06.9 & 17.44 & 13.72 & -35.79$\pm$2.19 & -15.34$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -36.7 & -13.0 & 100 & 1.26\\ 
211990768 & 08 28 26.94 & +20 06 17.1 & 17.1 & 13.38 & -35.81$\pm$2.22 & -13.34$\pm$2.22 & 5.2$\pm$0.7$^{(1)}$ & -34.3 & -13.7 & 100 & 1.61\\ 
211990866 & 08 38 24.30 & +20 06 21.8 & 10.36 & 9.18 & -35.62$\pm$0.76 & -12.79$\pm$0.76 & 5.6$\pm$0.8$^{(1)}$ & -36.1 & -13.2 & 100 & 4.26\\ 
211990908 & 08 40 22.31 & +20 06 24.4 & 9.92 & 8.85 & -35.27$\pm$1.37 & -13.2$\pm$0.65 & 5.6$\pm$0.4$^{(0)}$ & -36.5 & -13.1 & 100 & 2.56\\ 
211990953 & 08 41 58.84 & +20 06 27.0 & 12.74 & 10.6 & -38.66$\pm$2.19 & -14.69$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.7 & -13.0 & 100 & 11.34\\ 
211991074 & 08 37 25.26 & +20 06 35.0 & 18.82 & 14.63 & -26.53$\pm$2.35 & -22.27$\pm$2.35 & 4.8$\pm$0.7$^{(1)}$ & -35.9 & -13.2 & 17 &  \\ 
211991402 & 08 29 43.81 & +20 06 52.5 & 16.93 & 13.25 & -31.82$\pm$2.24 & -22.09$\pm$2.24 & 4.7$\pm$0.6$^{(1)}$ & -34.5 & -13.6 & 76 &  \\ 
211991549 & 08 36 20.40 & +20 07 00.4 & 16.47 & 12.9 & -40.1$\pm$2.23 & -13.43$\pm$2.2 & 4.8$\pm$0.7$^{(1)}$ & -35.7 & -13.3 & 100 & 46.28\\ 
211991571 & 08 39 05.23 & +20 07 01.8 & 9.27 & 8.41 & -35.74$\pm$0.99 & -13.04$\pm$0.51 & 5.2$\pm$0.4$^{(0)}$ & -36.2 & -13.1 & 100 & 0.79\\ 
211991662 & 08 36 22.42 & +20 07 07.0 & 17.2 & 13.45 & -35.44$\pm$2.22 & -10.66$\pm$2.21 & 4.7$\pm$0.7$^{(1)}$ & -35.7 & -13.3 & 100 & 2.32\\ 
211991772 & 08 36 15.90 & +20 07 12.9 & 14.75 & 11.75 & -41.1$\pm$2.19 & -15.56$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -13.3 & 100 & 16.51\\ 
211991806 & 08 32 59.59 & +20 07 14.9 & 17.8 & 13.9 & -38.99$\pm$2.77 & -17.41$\pm$2.77 & 5.0$\pm$0.7$^{(1)}$ & -35.1 & -13.5 & 100 & 0.36\\ 
211992034 & 08 36 45.72 & +20 07 26.2 & 11.41 & 9.94 & -33.87$\pm$0.84 & -12.93$\pm$0.84 & 4.9$\pm$0.7$^{(1)}$ & -35.8 & -13.3 & 100 & 9.02\\ 
211992053 & 08 39 45.21 & +20 07 27.5 & 16.0 & 12.3 & -35.67$\pm$2.19 & -14.33$\pm$2.19 & 8.6$\pm$1.2$^{(1)}$ & -36.4 & -13.1 & 100 & 5.08\\ 
211992423 & 08 33 07.46 & +20 07 48.2 & 13.43 & 10.93 & -35.97$\pm$2.24 & -14.01$\pm$2.24 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -13.5 & 100 & 13.07\\ 
211992451 & 08 41 24.46 & +20 07 49.5 & 15.18 & 11.64 & -37.69$\pm$2.19 & -18.09$\pm$2.19 & 7.9$\pm$1.1$^{(1)}$ & -36.6 & -13.0 & 100 & 1.4\\ 
211992683 & 08 38 12.45 & +20 08 02.6 & 17.9 & 14.02 & -38.3$\pm$2.23 & -17.4$\pm$2.23 & 4.6$\pm$0.6$^{(1)}$ & -36.1 & -13.2 & 100 & 28.91\\ 
211992776 & 08 40 01.30 & +20 08 08.3 & 9.54 & 8.62 & -34.68$\pm$1.06 & -13.62$\pm$1.08 & 5.4$\pm$0.5$^{(0)}$ & -36.4 & -13.1 & 100 & 1.18\\ 
211992843 & 08 37 54.57 & +20 08 12.3 & 14.96 & 11.82 & -37.96$\pm$2.24 & -14.84$\pm$2.23 & 5.1$\pm$0.7$^{(1)}$ & -36.0 & -13.2 & 100 & 19.27\\ 
211992880 & 08 38 21.50 & +20 08 14.6 & 17.63 & 13.54 & -37.8$\pm$2.82 & -13.74$\pm$2.82 & 6.8$\pm$0.9$^{(1)}$ & -36.1 & -13.2 & 100 & 0.24\\ 
211993172 & 08 42 37.00 & +20 08 31.8 & 13.35 & 10.87 & -42.16$\pm$2.19 & -13.73$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.9 & -13.0 & 100 & 11.97\\ 
211993420 & 08 36 45.02 & +20 08 45.9 & 17.55 & 13.78 & -34.02$\pm$2.19 & -15.02$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -35.8 & -13.3 & 100 & 2.23\\ 
211993552 & 08 50 10.26 & +20 08 55.0 & 14.13 & 11.25 & -41.52$\pm$2.11 & -15.36$\pm$2.11 & 5.3$\pm$0.7$^{(1)}$ & -38.2 & -12.5 & 100 &  \\ 
211994121 & 08 39 58.37 & +20 09 29.7 & 8.82 & 8.1 & -36.4$\pm$0.69 & -14.18$\pm$0.4 & 5.4$\pm$0.3$^{(0)}$ & -36.4 & -13.1 & 100 & 0.89\\ 
211994195 & 08 41 53.14 & +20 09 34.0 & 8.46 & 7.79 & -36.61$\pm$0.55 & -13.15$\pm$0.39 & 5.5$\pm$0.3$^{(0)}$ & -36.7 & -13.0 & 100 & 0.47\\ 
211994382 & 08 38 06.72 & +20 09 44.5 & 17.87 & 13.98 & -35.88$\pm$2.76 & -12.28$\pm$2.76 & 5.0$\pm$0.7$^{(1)}$ & -36.1 & -13.2 & 100 & 0.45\\ 
211994672 & 08 41 51.98 & +20 10 01.1 & 11.73 & 10.09 & -36.24$\pm$0.84 & -12.14$\pm$0.84 & 5.1$\pm$0.7$^{(1)}$ & -36.7 & -13.0 & 100 & 9.6\\ 
211994910 & 08 38 39.06 & +20 10 14.9 & 15.86 & 12.28 & -40.28$\pm$2.19 & -15.25$\pm$2.19 & 6.4$\pm$0.9$^{(1)}$ & -36.2 & -13.2 & 100 & 0.74\\ 
211995082 & 08 45 40.50 & +20 10 25.5 & 16.06 & 12.59 & -38.64$\pm$2.14 & -13.22$\pm$2.14 & 4.7$\pm$0.6$^{(1)}$ & -37.4 & -12.8 & 100 & 25.92\\ 
211995288 & 08 37 22.23 & +20 10 37.3 & 11.19 & 9.8 & -35.97$\pm$0.77 & -15.21$\pm$0.79 & 4.8$\pm$0.7$^{(1)}$ & -35.9 & -13.3 & 100 & 7.8\\ 
211995325 & 08 44 49.82 & +20 10 39.7 & 19.23 & 14.99 & -32.2$\pm$2.99 & -22.09$\pm$2.99 & 4.3$\pm$0.6$^{(1)}$ & -37.2 & -12.9 & 93 &  \\ 
211995540 & 08 38 57.23 & +20 10 53.6 & 13.26 & 10.72 & -41.03$\pm$2.19 & -16.65$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.2 & -13.2 & 100 & 12.02\\ 
211995547 & 08 42 21.61 & +20 10 53.9 & 9.11 & 8.28 & -37.33$\pm$0.67 & -14.58$\pm$0.45 & 5.3$\pm$0.5$^{(0)}$ & -36.8 & -13.0 & 100 & 0.59\\ 
211995573 & 08 40 26.75 & +20 10 55.2 &   & 7.43 & -33.5$\pm$1.2 & -14.0$\pm$1.1 & 9.3$\pm$1.3$^{(2)}$ & -36.5 & -13.1 & 99 & 50.14\\ 
211996051 & 08 43 35.54 & +20 11 22.5 & 9.97 & 8.92 & -37.84$\pm$1.31 & -13.36$\pm$0.65 & 5.9$\pm$0.5$^{(0)}$ & -37.0 & -12.9 & 100 & 3.65\\ 
211996186 & 08 40 18.94 & +20 11 30.6 & 12.38 & 10.04 & -36.63$\pm$2.19 & -15.76$\pm$2.32 & 7.3$\pm$1.0$^{(1)}$ & -36.5 & -13.1 & 100 & 11.97\\ 
211996321 & 08 44 40.75 & +20 11 37.1 & 13.69 & 11.07 & -36.64$\pm$2.19 & -13.53$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -37.2 & -12.9 & 100 & 14.18\\ 
211996831 & 08 40 31.85 & +20 12 06.1 & 11.3 & 9.83 & -36.83$\pm$0.82 & -13.84$\pm$0.83 & 4.9$\pm$0.7$^{(1)}$ & -36.5 & -13.1 & 100 & 4.37\\ 
211997061 & 08 36 21.82 & +20 12 19.7 & 15.53 & 12.17 & -40.75$\pm$2.19 & -15.38$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -35.7 & -13.3 & 100 & 10.15\\ 
211997350 & 08 41 37.38 & +20 12 36.9 & 16.98 & 13.33 & -38.49$\pm$2.19 & -13.81$\pm$2.19 & 4.7$\pm$0.6$^{(1)}$ & -36.7 & -13.1 & 100 & 21.63\\ 
211997380 & 08 39 15.00 & +20 12 38.8 & 11.07 & 9.65 & -36.13$\pm$2.3 & -11.82$\pm$1.14 & 5.2$\pm$0.7$^{(0)}$ & -36.3 & -13.2 & 100 & 8.12\\ 
211997576 & 08 40 58.08 & +20 12 50.4 & 18.02 & 14.01 & -39.39$\pm$2.69 & -17.06$\pm$2.69 & 5.6$\pm$0.8$^{(1)}$ & -36.6 & -13.1 & 100 & 0.94\\ 
211997741 & 08 44 11.64 & +20 13 00.1 & 16.76 & 12.86 & -34.5$\pm$2.23 & -13.9$\pm$2.23 & 7.9$\pm$1.1$^{(1)}$ & -37.1 & -12.9 & 100 & 1.38\\ 
211997840 & 08 27 30.65 & +20 13 05.8 & 13.41 & 10.9 & -37.16$\pm$2.22 & -16.45$\pm$2.22 & 5.0$\pm$0.7$^{(1)}$ & -34.1 & -13.8 & 99 & 12.95\\ 
211997857 & 08 40 08.15 & +20 13 06.6 & 18.0 & 13.81 & -39.92$\pm$2.69 & -12.35$\pm$2.69 & 7.5$\pm$1.0$^{(1)}$ & -36.4 & -13.1 & 100 & 0.83\\ 
211997888 & 08 38 55.17 & +20 13 09.0 & 16.12 & 12.54 & -40.02$\pm$2.19 & -16.93$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.2 & -13.2 & 100 & 0.97\\ 
211997901 & 08 45 59.36 & +20 13 09.8 & 18.58 & 14.45 & -21.7$\pm$4.3 & -7.9$\pm$4.3 & 4.3$\pm$0.6$^{(1)}$ & -37.4 & -12.8 & 16 &  \\ 
211998019 & 08 25 25.04 & +20 13 17.7 & 15.24 & 11.93 & -35.23$\pm$2.22 & -12.2$\pm$2.22 & 5.3$\pm$0.7$^{(1)}$ & -33.7 & -13.9 & 97 & 18.55\\ 
211998178 & 08 37 35.06 & +20 13 26.6 & 14.48 & 11.36 & -39.77$\pm$2.23 & -13.64$\pm$2.23 & 6.1$\pm$0.8$^{(1)}$ & -36.0 & -13.3 & 100 & 15.57\\ 
211998192 & 08 48 49.14 & +20 13 27.4 & 14.98 & 11.83 & -39.28$\pm$2.12 & -11.11$\pm$2.12 & 4.9$\pm$0.7$^{(1)}$ & -37.9 & -12.7 & 100 & 19.27\\ 
211998346 & 08 41 43.82 & +20 13 36.7 & 10.3 & 9.14 & -35.87$\pm$1.95 & -13.93$\pm$0.93 & 5.6$\pm$0.6$^{(0)}$ & -36.7 & -13.1 & 100 & 5.51\\ 
211998436 & 08 36 28.31 & +20 13 42.9 &   & 10.44 & -33.8$\pm$1.6 & -11.4$\pm$2.0 & 5.0$\pm$0.7$^{(2)}$ & -35.8 & -13.4 & 100 & 10.29\\ 
211998489 & 08 37 11.44 & +20 13 45.9 & 19.06 & 14.6 & -24.28$\pm$2.94 & -22.85$\pm$2.93 & 5.0$\pm$0.7$^{(1)}$ & -35.9 & -13.3 & 19 &  \\ 
211998490 & 08 48 48.34 & +20 13 46.0 & 19.14 & 14.78 & -34.8$\pm$4.85 & -0.97$\pm$4.85 & 4.3$\pm$0.6$^{(1)}$ & -37.9 & -12.7 & 74 &  \\ 
211998650 & 08 44 23.21 & +20 13 55.7 & 17.17 & 13.35 & -37.19$\pm$2.19 & -17.07$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -37.2 & -12.9 & 100 & 2.09\\ 
211998837 & 08 49 24.05 & +20 14 06.5 & 17.35 & 13.42 & -39.08$\pm$2.64 & -13.5$\pm$2.64 & 7.6$\pm$1.0$^{(1)}$ & -38.0 & -12.6 & 99 & 0.67\\ 
211999343 & 08 27 50.60 & +20 14 36.3 & 13.7 & 11.07 & -35.44$\pm$2.25 & -13.56$\pm$2.24 & 4.9$\pm$0.7$^{(1)}$ & -34.2 & -13.8 & 100 & 14.52\\ 
211999627 & 08 53 33.03 & +20 14 53.7 & 16.74 & 13.08 & -40.58$\pm$2.08 & -9.94$\pm$2.08 & 5.4$\pm$0.7$^{(1)}$ & -38.7 & -12.4 & 98 & 22.27\\ 
211999682 & 08 41 23.90 & +20 14 57.1 & 13.73 & 10.78 & -39.89$\pm$2.19 & -12.88$\pm$2.19 & 7.1$\pm$1.0$^{(1)}$ & -36.6 & -13.1 & 100 &  \\ 
211999969 & 08 40 26.57 & +20 15 13.3 & 15.47 & 12.19 & -35.78$\pm$2.19 & -15.7$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.5 & -13.2 & 100 & 24.24\\ 
212000760 & 08 35 52.07 & +20 15 58.8 & 18.66 & 13.84 & -24.81$\pm$2.78 & -7.06$\pm$2.71 & 7.1$\pm$1.0$^{(1)}$ & -35.7 & -13.4 & 45 & 0.39\\ 
212001288 & 08 36 34.91 & +20 16 30.7 & 15.54 & 12.14 & -37.26$\pm$2.19 & -14.9$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -35.8 & -13.4 & 100 & 50.99\\ 
212001425 & 08 36 41.19 & +20 16 40.0 & 16.8 & 13.16 & -37.63$\pm$2.19 & -14.89$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -35.8 & -13.4 & 100 & 8.35\\ 
212002216 & 08 44 48.71 & +20 17 26.0 & 12.48 & 10.51 & -36.86$\pm$2.19 & -12.22$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -37.2 & -12.9 & 100 & 10.93\\ 
212002298 & 08 39 19.61 & +20 17 30.6 & 17.39 & 13.16 & -25.46$\pm$2.23 & -10.38$\pm$2.19 & 9.6$\pm$1.3$^{(1)}$ & -36.3 & -13.2 & 10 & 28.91\\ 
212002525 & 08 39 42.03 & +20 17 45.1 & 16.87 & 13.14 & -37.73$\pm$2.19 & -13.34$\pm$2.19 & 5.5$\pm$0.8$^{(1)}$ & -36.3 & -13.2 & 100 & 12.63\\ 
212002808 & 08 33 23.49 & +20 18 03.3 & 18.25 & 14.13 & -33.14$\pm$2.79 & -11.62$\pm$2.79 & 6.0$\pm$0.8$^{(1)}$ & -35.2 & -13.6 & 100 & 0.33\\ 
212003318 & 08 38 16.96 & +20 18 35.3 & 17.58 & 13.24 & -34.87$\pm$3.04 & -19.97$\pm$2.93 & 10.4$\pm$1.4$^{(1)}$ & -36.1 & -13.3 & 86 & 2.78\\ 
212003469 & 08 40 28.64 & +20 18 44.9 & 11.31 & 9.46 & -37.51$\pm$0.83 & -15.54$\pm$0.88 & 7.3$\pm$1.0$^{(1)}$ & -36.5 & -13.2 & 100 & 8.14\\ 
212003893 & 08 36 56.58 & +20 19 10.1 & 14.56 & 11.23 & -39.01$\pm$2.19 & -14.54$\pm$2.19 & 8.2$\pm$1.1$^{(1)}$ & -35.9 & -13.4 & 100 & 2.13\\ 
212004774 & 08 42 50.52 & +20 20 04.0 & 18.0 & 14.07 & -37.06$\pm$2.68 & -15.85$\pm$2.68 & 5.2$\pm$0.7$^{(1)}$ & -36.9 & -13.1 & 100 &  \\ 
212004983 & 08 43 00.55 & +20 20 16.1 & 11.22 & 9.77 & -36.04$\pm$0.83 & -13.45$\pm$0.83 & 5.0$\pm$0.7$^{(1)}$ & -36.9 & -13.1 & 100 & 8.94\\ 
212005017 & 08 40 37.89 & +20 20 17.8 & 14.23 & 11.37 & -38.57$\pm$2.19 & -15.08$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.5 & -13.2 & 100 & 15.65\\ 
212005201 & 08 36 17.44 & +20 20 29.4 & 7.47 & 7.17 & -35.15$\pm$0.18 & -13.13$\pm$0.06 & 6.3$\pm$0.7$^{(0)}$ & -35.7 & -13.4 & 100 &  \\ 
212005204 & 08 44 34.50 & +20 20 29.5 & 16.86 & 13.26 & -35.3$\pm$2.19 & -13.96$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -37.2 & -13.0 & 100 & 19.91\\ 
212005503 & 08 41 51.91 & +20 20 47.8 & 15.46 & 12.19 & -38.83$\pm$2.19 & -15.07$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.7 & -13.1 & 100 & 20.73\\ 
212005504 & 08 41 20.86 & +20 20 47.9 & 15.55 & 12.27 & -34.95$\pm$2.19 & -15.82$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -36.6 & -13.2 & 100 & 21.78\\ 
212005551 & 08 40 10.61 & +20 20 50.5 & 18.79 & 14.41 & -37.4$\pm$2.77 & -14.96$\pm$2.76 & 5.5$\pm$0.8$^{(1)}$ & -36.4 & -13.2 & 100 & 0.26\\ 
212005623 & 08 39 06.87 & +20 20 54.3 & 15.11 & 11.91 & -37.68$\pm$2.19 & -15.42$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.2 & -13.3 & 100 & 8.19\\ 
212006108 & 08 38 25.37 & +20 21 21.0 & 17.9 & 14.03 & -36.5$\pm$2.23 & -19.07$\pm$2.23 & 4.6$\pm$0.6$^{(1)}$ & -36.1 & -13.3 & 100 & 3.16\\ 
212006227 & 08 45 04.22 & +20 21 27.9 & 10.22 & 9.13 & -38.26$\pm$1.55 & -16.89$\pm$1.63 & 6.1$\pm$0.6$^{(0)}$ & -37.3 & -13.0 & 100 & 3.67\\ 
212006723 & 08 43 50.85 & +20 21 56.7 & 14.6 & 11.51 & -37.42$\pm$2.19 & -10.44$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -37.1 & -13.0 & 100 & 18.79\\ 
212006725 & 08 25 22.24 & +20 21 56.8 & 18.7 & 14.33 & -35.34$\pm$2.87 & -13.96$\pm$2.87 & 6.1$\pm$0.8$^{(1)}$ & -33.7 & -14.0 & 96 & 0.2\\ 
212007145 & 08 40 01.35 & +20 22 22.6 & 18.14 & 14.21 & -30.62$\pm$2.77 & -15.95$\pm$2.74 & 5.1$\pm$0.7$^{(1)}$ & -36.4 & -13.3 & 100 & 0.87\\ 
212007343 & 08 36 39.48 & +20 22 34.0 & 16.64 & 12.75 & -35.56$\pm$2.2 & -21.09$\pm$2.19 & 9.4$\pm$1.3$^{(1)}$ & -35.8 & -13.4 & 74 & 16.98\\ 
212007419 & 08 41 11.06 & +20 22 38.5 & 14.97 & 11.82 & -35.35$\pm$2.19 & -16.46$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.6 & -13.2 & 100 & 18.55\\ 
212008129 & 08 41 47.92 & +20 23 22.6 & 18.17 & 14.23 & -38.36$\pm$2.73 & -9.87$\pm$2.73 & 5.2$\pm$0.7$^{(1)}$ & -36.7 & -13.2 & 100 & 0.33\\ 
212008490 & 08 45 07.35 & +20 23 41.9 & 11.63 & 10.05 & -37.14$\pm$0.83 & -13.6$\pm$0.83 & 4.9$\pm$0.7$^{(1)}$ & -37.3 & -13.0 & 100 & 4.57\\ 
212008515 & 08 45 28.25 & +20 23 43.4 & 8.46 & 7.86 & -37.67$\pm$0.05 & -13.51$\pm$0.04 & 6.9$\pm$0.9$^{(0)}$ & -37.4 & -13.0 & 100 &  \\ 
212008710 & 08 55 02.24 & +20 23 54.1 & 13.38 & 10.95 & -37.87$\pm$2.2 & -12.78$\pm$2.2 & 4.8$\pm$0.7$^{(1)}$ & -39.0 & -12.4 & 96 & 11.65\\ 
212008913 & 08 48 00.24 & +20 24 06.8 & 17.53 & 13.7 & -38.11$\pm$2.28 & -17.94$\pm$2.28 & 5.7$\pm$0.8$^{(1)}$ & -37.8 & -12.8 & 100 & 2.25\\ 
212009131 & 08 31 35.95 & +20 24 19.3 & 18.32 & 14.18 & -31.47$\pm$2.82 & -15.65$\pm$2.82 & 5.8$\pm$0.8$^{(1)}$ & -34.9 & -13.7 & 100 & 0.24\\ 
212009190 & 08 36 59.89 & +20 24 23.4 & 14.09 & 11.32 & -36.88$\pm$2.23 & -13.42$\pm$2.23 & 4.9$\pm$0.7$^{(1)}$ & -35.9 & -13.4 & 100 & 15.26\\ 
212009294 & 08 39 10.16 & +20 24 30.2 & 13.62 & 11.0 & -38.62$\pm$2.19 & -12.52$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -36.2 & -13.3 & 100 & 13.98\\ 
212009372 & 08 42 18.83 & +20 24 35.1 & 12.05 & 10.19 & -35.04$\pm$1.71 & -14.93$\pm$2.51 & 5.4$\pm$0.7$^{(1)}$ & -36.8 & -13.2 & 100 &  \\ 
212009427 & 08 31 29.87 & +20 24 37.5 & 13.82 & 10.77 & -34.18$\pm$2.24 & -13.6$\pm$2.24 & 7.2$\pm$1.0$^{(1)}$ & -34.9 & -13.7 & 100 & 1.56\\ 
212009464 & 08 36 41.82 & +20 24 39.9 & 12.48 & 10.52 & -36.15$\pm$2.2 & -13.02$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -35.8 & -13.5 & 100 & 11.01\\ 
212009944 & 08 40 10.02 & +20 25 08.2 & 14.49 & 11.31 & -36.26$\pm$2.19 & -14.42$\pm$2.19 & 6.7$\pm$0.9$^{(1)}$ & -36.4 & -13.3 & 100 & 19.02\\ 
212010154 & 08 45 26.00 & +20 25 22.6 & 13.99 & 11.21 & -34.7$\pm$2.19 & -13.17$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -37.3 & -13.0 & 100 & 14.38\\ 
212010383 & 08 45 25.99 & +20 25 38.6 & 13.51 & 10.88 & -39.79$\pm$2.19 & -12.43$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -37.3 & -13.0 & 100 & 14.52\\ 
212010627 & 08 39 26.68 & +20 25 52.3 & 16.21 & 12.66 & -38.5$\pm$2.19 & -10.5$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.3 & -13.3 & 100 & 4.73\\ 
212011152 & 08 38 08.09 & +20 26 22.3 & 11.46 & 9.93 & -36.35$\pm$0.76 & -14.55$\pm$0.79 & 5.1$\pm$0.7$^{(1)}$ & -36.1 & -13.4 & 100 & 9.16\\ 
212011394 & 08 48 49.98 & +20 26 36.0 & 14.97 & 11.86 & -36.14$\pm$2.28 & -13.73$\pm$2.28 & 4.6$\pm$0.6$^{(1)}$ & -37.9 & -12.8 & 100 & 19.65\\ 
212011416 & 08 33 08.45 & +20 26 37.4 & 15.59 & 11.94 & -33.96$\pm$2.24 & -14.27$\pm$2.24 & 8.4$\pm$1.2$^{(1)}$ & -35.2 & -13.7 & 99 & 5.23\\ 
212011557 & 08 38 08.17 & +20 26 46.0 & 15.29 & 12.02 & -36.34$\pm$2.3 & -12.1$\pm$2.25 & 4.8$\pm$0.7$^{(1)}$ & -36.1 & -13.4 & 100 & 21.63\\ 
212011680 & 08 38 21.39 & +20 26 53.2 & 14.43 & 11.5 & -32.9$\pm$2.23 & -13.4$\pm$2.23 & 5.0$\pm$0.7$^{(1)}$ & -36.1 & -13.4 & 100 &  \\ 
212011731 & 08 38 07.31 & +20 26 55.7 & 15.33 & 12.04 & -40.27$\pm$2.23 & -14.07$\pm$2.23 & 4.9$\pm$0.7$^{(1)}$ & -36.1 & -13.4 & 100 & 21.47\\ 
212012042 & 08 45 06.11 & +20 27 13.4 & 18.92 & 14.68 & -38.33$\pm$2.96 & -15.64$\pm$2.96 & 4.7$\pm$0.7$^{(1)}$ & -37.3 & -13.0 & 100 & 20.04\\ 
212012299 & 08 41 02.62 & +20 27 27.7 & 11.99 & 10.29 & -36.88$\pm$2.19 & -13.21$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.6 & -13.3 & 100 & 9.63\\ 
212012721 & 08 39 18.86 & +20 27 52.1 & 15.39 & 12.23 & -27.69$\pm$2.19 & -11.11$\pm$2.19 & 4.3$\pm$0.6$^{(1)}$ & -36.3 & -13.4 & 94 & 23.49\\ 
212013132 & 08 40 44.26 & +20 28 18.7 & 13.35 & 10.4 & -38.47$\pm$2.19 & -13.74$\pm$2.19 & 8.5$\pm$1.2$^{(1)}$ & -36.5 & -13.3 & 100 & 2.13\\ 
212013222 & 08 41 05.31 & +20 28 24.5 & 14.26 & 11.41 & -38.72$\pm$2.19 & -12.7$\pm$2.19 & 4.7$\pm$0.7$^{(1)}$ & -36.6 & -13.3 & 100 & 14.81\\ 
212013297 & 08 40 46.91 & +20 28 29.1 & 14.97 & 11.68 & -34.72$\pm$2.19 & -15.86$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -36.5 & -13.3 & 100 & 18.79\\ 
212013502 & 08 40 57.52 & +20 28 41.5 & 18.24 & 14.31 & -36.74$\pm$2.76 & -12.71$\pm$2.75 & 5.4$\pm$0.7$^{(1)}$ & -36.6 & -13.3 & 100 & 0.23\\ 
212013619 & 08 40 47.79 & +20 28 47.9 & 15.8 & 12.25 & -38.65$\pm$2.19 & -13.83$\pm$2.19 & 6.2$\pm$0.9$^{(1)}$ & -36.5 & -13.3 & 100 & 7.36\\ 
212013705 & 08 33 38.38 & +20 28 52.6 & 17.13 & 13.43 & -32.52$\pm$2.24 & -13.29$\pm$2.24 & 4.5$\pm$0.6$^{(1)}$ & -35.3 & -13.7 & 100 & 2.14\\ 
212014467 & 08 39 43.61 & +20 29 39.6 & 16.34 & 12.75 & -34.7$\pm$2.2 & -10.56$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.3 & -13.4 & 100 & 10.4\\ 
212014492 & 08 45 45.89 & +20 29 41.0 & 15.4 & 12.1 & -37.43$\pm$2.19 & -13.35$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -37.4 & -13.0 & 100 & 17.79\\ 
212015247 & 08 49 33.90 & +20 30 29.1 & 9.21 & 8.37 & -37.31$\pm$0.64 & -13.23$\pm$0.51 & 5.6$\pm$0.8$^{(1)}$ & -38.1 & -12.8 & 100 & 0.71\\ 
212015396 & 08 43 17.84 & +20 30 37.4 & 11.52 & 9.78 & -37.2$\pm$0.82 & -10.04$\pm$0.82 & 5.9$\pm$0.8$^{(1)}$ & -37.0 & -13.2 & 100 & 9.0\\ 
212015476 & 08 42 56.68 & +20 30 42.3 & 17.25 & 13.48 & -32.87$\pm$2.19 & -11.97$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.9 & -13.2 & 100 & 1.39\\ 
212015504 & 08 45 02.64 & +20 30 43.8 & 14.21 & 11.1 & -30.71$\pm$2.19 & -12.0$\pm$2.19 & 6.9$\pm$1.0$^{(1)}$ & -37.3 & -13.1 & 99 & 24.64\\ 
212015538 & 08 39 52.65 & +20 30 46.4 & 16.05 & 12.52 & -33.4$\pm$2.19 & -12.1$\pm$2.19 & 5.7$\pm$0.8$^{(1)}$ & -36.4 & -13.4 & 100 & 0.9\\ 
212016014 & 08 42 55.13 & +20 31 14.4 & 18.88 & 14.57 & -35.24$\pm$2.91 & -16.14$\pm$2.9 & 4.9$\pm$0.7$^{(1)}$ & -36.9 & -13.2 & 100 & 0.85\\ 
212016828 & 08 46 01.96 & +20 32 03.2 &   & 14.36 & -38.0$\pm$5.0 & -14.0$\pm$5.0 & 5.8$\pm$0.8$^{(3)}$ & -37.5 & -13.0 & 100 & 0.59\\ 
212016898 & 08 37 20.40 & +20 32 07.9 & 18.16 & 14.02 & -30.41$\pm$2.7 & -10.42$\pm$2.69 & 5.5$\pm$0.8$^{(1)}$ & -35.9 & -13.5 & 100 & 0.33\\ 
212016916 & 08 39 31.77 & +20 32 08.9 & 19.1 & 14.84 & -22.24$\pm$2.98 & -8.76$\pm$2.96 & 4.4$\pm$0.6$^{(1)}$ & -36.3 & -13.4 & 11 &  \\ 
212016988 & 08 43 36.89 & +20 32 14.0 & 15.17 & 11.94 & -39.06$\pm$2.19 & -16.83$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -37.0 & -13.2 & 100 & 19.27\\ 
212017124 & 08 39 53.36 & +20 32 21.3 & 10.3 & 9.27 & -39.38$\pm$0.6 & -18.28$\pm$0.62 & 4.0$\pm$0.6$^{(1)}$ & -36.4 & -13.4 & 95 &  \\ 
212017183 & 08 43 36.85 & +20 32 24.5 & 16.16 & 12.59 & -35.77$\pm$2.19 & -14.44$\pm$2.19 & 5.2$\pm$0.7$^{(1)}$ & -37.0 & -13.2 & 100 & 0.74\\ 
212017273 & 08 38 01.36 & +20 32 29.5 & 17.97 & 13.88 & -34.84$\pm$2.77 & -17.03$\pm$2.76 & 6.4$\pm$0.9$^{(1)}$ & -36.0 & -13.5 & 100 & 1.09\\ 
212017328 & 08 41 17.49 & +20 32 33.1 & 16.88 & 13.11 & -38.79$\pm$2.19 & -12.41$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -36.6 & -13.3 & 100 & 15.03\\ 
212017486 & 08 37 12.61 & +20 32 41.5 & 13.99 & 11.37 & -37.34$\pm$2.2 & -13.15$\pm$2.19 & 4.5$\pm$0.6$^{(1)}$ & -35.9 & -13.5 & 100 & 13.98\\ 
212017838 & 08 33 13.50 & +20 33 01.4 & 16.11 & 12.48 & -38.24$\pm$2.24 & -12.71$\pm$2.24 & 6.7$\pm$0.9$^{(1)}$ & -35.2 & -13.7 & 100 & 0.67\\ 
212018005 & 08 36 15.98 & +20 33 11.2 & 13.95 & 11.23 & -39.74$\pm$2.19 & -15.87$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -13.6 & 100 & 13.36\\ 
212018408 & 08 39 54.33 & +20 33 36.8 & 9.21 & 8.38 & -36.59$\pm$0.89 & -13.26$\pm$0.47 & 5.3$\pm$0.3$^{(0)}$ & -36.4 & -13.4 & 100 & 1.59\\ 
212018728 & 08 43 25.01 & +20 33 55.3 & 14.27 & 11.4 & -37.24$\pm$2.19 & -9.85$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -37.0 & -13.2 & 100 & 16.51\\ 
212018862 & 08 39 03.95 & +20 34 02.3 & 15.75 & 12.28 & -38.1$\pm$2.19 & -12.16$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -36.2 & -13.4 & 100 & 3.68\\ 
212018902 & 08 38 14.99 & +20 34 04.2 & 11.19 & 9.72 & -35.89$\pm$0.77 & -14.81$\pm$0.75 & 5.6$\pm$0.8$^{(1)}$ & -36.1 & -13.5 & 100 & 9.36\\ 
212018903 & 08 41 36.51 & +20 34 04.3 & 16.96 & 13.18 & -40.47$\pm$2.19 & -12.01$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.7 & -13.3 & 100 & 6.17\\ 
212018959 & 08 41 42.07 & +20 34 07.9 & 17.7 & 13.83 & -36.11$\pm$2.69 & -8.57$\pm$2.69 & 4.4$\pm$0.6$^{(1)}$ & -36.7 & -13.3 & 100 & 0.86\\ 
212019252 & 08 42 48.47 & +20 34 24.4 & 12.1 & 10.26 & -36.79$\pm$0.9 & -12.86$\pm$0.94 & 5.4$\pm$0.7$^{(1)}$ & -36.9 & -13.2 & 100 & 11.26\\ 
212019439 & 08 38 46.11 & +20 34 36.4 & 12.07 & 10.31 & -37.9$\pm$2.19 & -13.72$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -36.2 & -13.5 & 100 & 9.36\\ 
212019656 & 08 39 51.29 & +20 34 50.0 & 14.92 & 11.59 & -38.95$\pm$2.19 & -13.33$\pm$2.19 & 6.3$\pm$0.9$^{(1)}$ & -36.4 & -13.4 & 100 & 1.84\\ 
212020223 & 08 45 30.49 & +20 35 24.6 & 9.69 & 8.77 & -37.1$\pm$0.13 & -13.24$\pm$0.07 & 5.7$\pm$0.3$^{(0)}$ & -37.4 & -13.1 & 100 & 0.95\\ 
212020360 & 08 42 45.39 & +20 35 33.6 & 17.99 & 14.13 & -35.39$\pm$2.84 & -14.76$\pm$2.84 & 5.5$\pm$0.8$^{(1)}$ & -36.9 & -13.2 & 100 & 0.52\\ 
212020850 & 08 40 34.96 & +20 36 03.8 & 17.84 & 13.96 & -38.76$\pm$2.7 & -14.95$\pm$2.69 & 4.7$\pm$0.7$^{(1)}$ & -36.5 & -13.4 & 100 & 0.79\\ 
212021051 & 08 41 44.14 & +20 36 16.0 & 16.66 & 12.99 & -34.78$\pm$2.19 & -11.72$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -36.7 & -13.3 & 100 & 7.4\\ 
212021131 & 08 33 14.25 & +20 36 21.3 & 17.58 & 13.79 & -37.6$\pm$2.24 & -13.26$\pm$2.24 & 5.7$\pm$0.8$^{(1)}$ & -35.2 & -13.8 & 100 &  \\ 
212021253 & 08 37 28.46 & +20 36 28.6 & 14.57 & 11.49 & -41.18$\pm$2.25 & -13.92$\pm$2.24 & 5.6$\pm$0.8$^{(1)}$ & -35.9 & -13.6 & 100 & 7.24\\ 
212021375 & 08 36 40.03 & +20 36 35.7 & 11.59 & 10.08 & -35.88$\pm$0.79 & -14.77$\pm$0.76 & 4.8$\pm$0.7$^{(1)}$ & -35.8 & -13.6 & 100 & 8.89\\ 
212021901 & 08 35 56.51 & +20 37 07.0 & 18.08 & 14.08 & -42.28$\pm$2.77 & -12.86$\pm$2.77 & 5.0$\pm$0.7$^{(1)}$ & -35.7 & -13.6 & 100 & 1.22\\ 
212022052 & 08 41 53.65 & +20 37 15.9 & 18.0 & 14.07 & -38.24$\pm$3.43 & -16.15$\pm$2.89 & 4.5$\pm$0.6$^{(1)}$ & -36.7 & -13.3 & 100 & 0.25\\ 
212022062 & 08 38 02.48 & +20 37 16.5 & 18.04 & 14.01 & -35.35$\pm$2.77 & -15.74$\pm$2.76 & 5.6$\pm$0.8$^{(1)}$ & -36.0 & -13.5 & 100 &  \\ 
212023280 & 08 40 22.42 & +20 38 27.1 & 14.05 & 11.22 & -39.06$\pm$2.19 & -13.62$\pm$2.19 & 5.0$\pm$0.7$^{(1)}$ & -36.5 & -13.4 & 100 & 14.73\\ 
212023593 & 08 44 00.67 & +20 38 45.5 & 18.18 & 14.27 & -39.6$\pm$2.76 & -11.27$\pm$2.76 & 5.0$\pm$0.7$^{(1)}$ & -37.1 & -13.2 & 100 & 0.57\\ 
212024154 & 08 39 32.04 & +20 39 20.4 & 11.72 & 9.77 & -37.24$\pm$0.95 & -14.74$\pm$0.95 & 7.0$\pm$1.0$^{(1)}$ & -36.3 & -13.5 & 100 & 10.54\\ 
212024396 & 08 38 04.62 & +20 39 35.3 & 16.78 & 13.14 & -35.94$\pm$2.23 & -16.17$\pm$2.23 & 4.9$\pm$0.7$^{(1)}$ & -36.1 & -13.6 & 100 & 16.7\\ 
212024554 & 08 38 45.69 & +20 39 43.9 & 17.37 & 13.6 & -26.45$\pm$2.2 & -9.93$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.2 & -13.5 & 86 & 1.34\\ 
212024569 & 08 30 57.60 & +20 39 44.9 & 14.58 & 11.72 & -32.08$\pm$2.24 & -9.57$\pm$2.24 & 4.0$\pm$0.6$^{(1)}$ & -34.8 & -13.9 & 93 & 15.49\\ 
212025000 & 08 37 33.06 & +20 40 10.1 & 17.36 & 13.68 & -34.97$\pm$2.24 & -13.33$\pm$2.23 & 3.9$\pm$0.5$^{(1)}$ & -36.0 & -13.6 & 100 & 24.24\\ 
212025101 & 08 26 09.79 & +20 40 16.4 & 10.9 & 9.79 & -34.26$\pm$0.69 & -13.64$\pm$0.7 & 3.8$\pm$0.5$^{(1)}$ & -33.9 & -14.2 & 78 &  \\ 
212025163 & 08 41 40.01 & +20 40 19.9 & 9.5 & 8.59 & -35.4$\pm$0.44 & -13.62$\pm$0.53 & 5.2$\pm$0.7$^{(1)}$ & -36.7 & -13.4 & 100 & 1.06\\ 
212025207 & 08 29 44.41 & +20 40 23.2 & 11.63 & 9.81 & -36.29$\pm$0.83 & -12.59$\pm$0.79 & 6.3$\pm$0.9$^{(1)}$ & -34.5 & -14.0 & 100 & 13.85\\ 
212025597 & 08 36 19.36 & +20 40 46.7 & 18.3 & 13.89 & -30.65$\pm$2.73 & -19.99$\pm$2.73 & 7.4$\pm$1.0$^{(1)}$ & -35.7 & -13.7 & 97 &  \\ 
212025613 & 08 37 11.91 & +20 40 47.5 & 15.69 & 12.29 & -34.18$\pm$2.2 & -14.32$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -35.9 & -13.6 & 100 & 11.3\\ 
212025814 & 08 36 06.31 & +20 40 59.9 & 14.48 & 11.45 & -37.87$\pm$2.19 & -12.89$\pm$2.19 & 5.4$\pm$0.7$^{(1)}$ & -35.7 & -13.7 & 100 & 16.79\\ 
212025985 & 08 36 15.53 & +20 41 09.8 & 14.65 & 11.63 & -37.74$\pm$2.19 & -15.91$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -13.7 & 100 & 17.27\\ 
212026716 & 08 48 59.91 & +20 41 55.5 & 17.71 & 13.72 & -38.0$\pm$2.76 & -14.56$\pm$2.76 & 6.6$\pm$0.9$^{(1)}$ & -38.0 & -13.0 & 100 & 0.3\\ 
212026805 & 08 40 16.95 & +20 42 00.7 & 18.19 & 14.26 & -33.84$\pm$2.73 & -16.78$\pm$2.72 & 4.8$\pm$0.7$^{(1)}$ & -36.4 & -13.5 & 100 & 0.6\\ 
212026921 & 08 33 15.42 & +20 42 09.0 & 12.35 & 10.44 & -37.28$\pm$2.24 & -13.4$\pm$2.24 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -13.8 & 100 & 12.07\\ 
212027377 & 08 50 35.28 & +20 42 37.7 & 17.26 & 13.4 & -35.21$\pm$2.26 & -10.48$\pm$2.26 & 5.2$\pm$0.7$^{(1)}$ & -38.2 & -12.9 & 99 & 1.11\\ 
212027446 & 08 40 16.90 & +20 42 42.3 & 16.62 & 12.97 & -36.71$\pm$2.69 & -13.05$\pm$2.69 & 5.1$\pm$0.7$^{(1)}$ & -36.4 & -13.5 & 100 & 5.31\\ 
212027502 & 08 45 47.80 & +20 42 46.5 & 17.05 & 13.24 & -42.6$\pm$2.19 & -14.03$\pm$2.19 & 5.6$\pm$0.8$^{(1)}$ & -37.4 & -13.2 & 100 &  \\ 
212027544 & 08 33 13.94 & +20 42 48.3 & 18.41 & 14.4 & -34.68$\pm$2.9 & -7.04$\pm$2.9 & 4.8$\pm$0.7$^{(1)}$ & -35.2 & -13.9 & 99 & 0.46\\ 
212027750 & 08 49 14.77 & +20 43 00.9 & 13.18 & 10.82 & -44.85$\pm$2.22 & -10.97$\pm$2.22 & 5.0$\pm$0.7$^{(1)}$ & -38.0 & -13.0 & 98 & 20.31\\ 
212027753 & 08 44 12.32 & +20 43 01.0 & 17.49 & 13.54 & -39.81$\pm$2.69 & -14.04$\pm$2.69 & 5.7$\pm$0.8$^{(1)}$ & -37.1 & -13.2 & 100 & 1.0\\ 
212027816 & 08 29 18.87 & +20 43 04.8 & 15.8 & 12.4 & -35.76$\pm$2.24 & -18.51$\pm$2.24 & 4.8$\pm$0.7$^{(1)}$ & -34.5 & -14.1 & 99 &  \\ 
212027909 & 08 33 00.39 & +20 43 10.1 & 15.52 & 11.98 & -36.26$\pm$2.24 & -13.16$\pm$2.24 & 7.2$\pm$1.0$^{(1)}$ & -35.1 & -13.9 & 100 & 14.59\\ 
212028430 & 08 38 23.87 & +20 43 40.8 & 14.1 & 11.3 & -37.03$\pm$2.23 & -14.18$\pm$2.23 & 5.3$\pm$0.7$^{(1)}$ & -36.1 & -13.6 & 100 & 15.33\\ 
212028729 & 08 39 27.28 & +20 43 59.1 & 18.67 & 14.51 & -34.92$\pm$2.85 & -19.68$\pm$2.84 & 5.5$\pm$0.8$^{(1)}$ & -36.3 & -13.5 & 100 & 0.51\\ 
212029094 & 08 39 18.05 & +20 44 21.3 & 15.26 & 12.06 & -35.83$\pm$2.19 & -12.14$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -13.5 & 100 & 19.91\\ 
212029226 & 08 41 14.05 & +20 44 29.8 & 15.83 & 12.15 & -38.76$\pm$2.19 & -14.78$\pm$2.19 & 8.4$\pm$1.2$^{(1)}$ & -36.6 & -13.4 & 100 & 1.52\\ 
212030244 & 08 39 21.54 & +20 45 29.5 & 11.64 & 10.03 & -37.33$\pm$0.81 & -14.31$\pm$0.82 & 5.3$\pm$0.7$^{(1)}$ & -36.3 & -13.5 & 100 & 9.19\\ 
212031039 & 08 32 02.73 & +20 46 20.7 & 17.02 & 13.25 & -35.37$\pm$2.24 & -13.04$\pm$2.24 & 5.5$\pm$0.8$^{(1)}$ & -35.0 & -14.0 & 100 & 22.27\\ 
212031189 & 08 38 34.12 & +20 46 29.2 & 17.14 & 13.36 & -34.87$\pm$2.2 & -11.3$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.1 & -13.6 & 100 &  \\ 
212031366 & 08 41 19.22 & +20 46 39.2 & 12.93 & 10.7 & -36.97$\pm$2.19 & -14.67$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -13.5 & 100 & 12.42\\ 
212031440 & 08 37 07.15 & +20 46 43.9 & 16.47 & 12.76 & -34.79$\pm$2.2 & -10.9$\pm$2.19 & 6.1$\pm$0.8$^{(1)}$ & -35.9 & -13.7 & 100 & 16.89\\ 
212031764 & 08 33 37.97 & +20 47 03.3 & 19.2 & 14.63 & -21.95$\pm$3.07 & -13.23$\pm$3.07 & 4.6$\pm$0.6$^{(1)}$ & -35.3 & -13.9 & 31 &  \\ 
212031837 & 08 37 49.21 & +20 47 06.8 & 18.63 & 14.58 & -34.92$\pm$2.98 & -12.06$\pm$2.98 & 5.1$\pm$0.7$^{(1)}$ & -36.0 & -13.7 & 100 & 1.63\\ 
212031993 & 08 38 54.77 & +20 47 16.9 & 18.1 & 14.06 & -31.45$\pm$2.76 & -12.11$\pm$2.68 & 5.7$\pm$0.8$^{(1)}$ & -36.2 & -13.6 & 100 & 1.16\\ 
212032123 & 08 25 07.05 & +20 47 25.1 & 12.33 & 10.54 & -41.64$\pm$2.22 & -15.69$\pm$2.22 & 4.4$\pm$0.6$^{(1)}$ & -33.7 & -14.3 & 32 & 47.0\\ 
212032381 & 08 37 49.84 & +20 47 40.7 & 17.72 & 13.78 & -40.63$\pm$2.76 & -12.77$\pm$2.76 & 5.0$\pm$0.7$^{(1)}$ & -36.0 & -13.7 & 100 & 1.72\\ 
212032714 & 08 39 22.16 & +20 47 58.4 &   & 13.36 & -31.0$\pm$3.0 & -14.0$\pm$3.0 & 8.7$\pm$1.2$^{(3)}$ & -36.3 & -13.6 & 98 & 0.42\\ 
212033679 & 08 41 16.31 & +20 48 54.9 &   & 14.48 & -41.0$\pm$5.0 & -18.0$\pm$5.0 & 6.0$\pm$0.8$^{(3)}$ & -36.6 & -13.5 & 100 & 25.26\\ 
212033939 & 08 42 53.07 & +20 49 09.2 & 8.75 & 8.06 & -37.44$\pm$0.08 & -14.05$\pm$0.04 & 5.3$\pm$0.3$^{(0)}$ & -36.9 & -13.4 & 100 & 0.48\\ 
212034371 & 08 35 56.95 & +20 49 34.7 & 11.56 & 9.83 & -36.39$\pm$1.01 & -15.17$\pm$1.02 & 5.6$\pm$0.8$^{(1)}$ & -35.7 & -13.8 & 100 & 1.21\\ 
212034597 & 08 44 18.26 & +20 49 48.4 & 17.38 & 13.46 & -33.34$\pm$2.19 & -15.29$\pm$2.19 & 6.4$\pm$0.9$^{(1)}$ & -37.2 & -13.3 & 100 & $<$2\\ 
212035051 & 08 36 03.25 & +20 50 15.7 & 17.61 & 13.78 & -41.59$\pm$2.19 & -15.0$\pm$2.19 & 4.9$\pm$0.7$^{(1)}$ & -35.7 & -13.8 & 100 & 1.88\\ 
212035441 & 08 32 32.44 & +20 50 41.0 & 16.3 & 12.72 & -38.16$\pm$2.24 & -14.9$\pm$2.24 & 5.2$\pm$0.7$^{(1)}$ & -35.1 & -14.0 & 100 & 16.51\\ 
212036187 & 08 38 56.60 & +20 51 27.8 &   & 13.12 & -31.0$\pm$3.0 & -15.0$\pm$3.0 & 9.9$\pm$1.4$^{(3)}$ & -36.2 & -13.6 & 94 & 0.77\\ 
212038642 & 08 31 13.11 & +20 54 00.4 & 16.45 & 12.8 & -35.49$\pm$2.24 & -11.35$\pm$2.24 & 5.5$\pm$0.8$^{(1)}$ & -34.8 & -14.1 & 100 & 18.44\\ 
212066424 & 08 43 00.55 & +21 23 28.1 & 18.28 & 14.07 & -34.54$\pm$2.82 & -14.21$\pm$2.82 & 6.1$\pm$0.8$^{(1)}$ & -36.9 & -13.8 & 100 & 24.85\\ 
212066519 & 08 40 30.73 & +21 23 33.2 & 16.66 & 13.26 & -29.04$\pm$2.21 & -14.3$\pm$2.19 & 3.5$\pm$0.5$^{(1)}$ & -36.5 & -13.9 & 24 &  \\ 
212067464 & 08 39 09.49 & +21 24 35.9 & 10.67 & 9.34 & -27.29$\pm$1.85 & -11.16$\pm$0.94 & 5.9$\pm$0.6$^{(0)}$ & -36.2 & -14.0 & 86 &  \\ 
212068777 & 08 48 13.13 & +21 26 00.4 & 18.2 & 14.28 & -26.71$\pm$2.82 & -18.15$\pm$2.82 & 5.0$\pm$0.7$^{(1)}$ & -37.8 & -13.5 & 27 & 32.68\\ 
212068782 & 08 38 22.90 & +21 26 00.6 & 18.17 & 14.13 & -39.42$\pm$2.78 & -18.33$\pm$2.78 & 4.7$\pm$0.7$^{(1)}$ & -36.1 & -14.1 & 100 & 1.89\\ 
212069223 & 08 33 46.97 & +21 26 27.6 & 13.89 & 11.15 & -37.86$\pm$2.24 & -12.73$\pm$2.24 & 5.1$\pm$0.7$^{(1)}$ & -35.3 & -14.3 & 100 & 14.66\\ 
212069325 & 08 48 11.55 & +21 26 35.2 &   & 14.48 & -32.0$\pm$4.0 & -7.0$\pm$4.0 & 5.4$\pm$0.8$^{(3)}$ & -37.8 & -13.5 & 94 & 13.36\\ 
212069380 & 08 31 29.87 & +21 26 38.8 & 19.19 & 14.8 & -25.38$\pm$3.12 & -12.07$\pm$3.12 & 3.9$\pm$0.5$^{(1)}$ & -34.9 & -14.5 & 15 & 0.27\\ 
212070886 & 08 45 03.84 & +21 28 18.2 & 18.16 & 14.22 & -31.12$\pm$2.74 & -11.92$\pm$2.73 & 4.6$\pm$0.6$^{(1)}$ & -37.3 & -13.7 & 99 & 0.58\\ 
212072268 & 08 41 43.42 & +21 29 50.4 & 17.93 & 13.63 & -32.02$\pm$2.69 & -16.33$\pm$2.69 & 6.8$\pm$0.9$^{(1)}$ & -36.7 & -13.9 & 100 & 0.53\\ 
212074153 & 08 45 48.68 & +21 31 56.5 & 16.22 & 12.57 & -34.29$\pm$2.19 & -13.18$\pm$2.19 & 6.1$\pm$0.8$^{(1)}$ & -37.4 & -13.7 & 100 & 15.33\\ 
212074908 & 08 38 28.19 & +21 32 46.1 & 12.76 & 10.2 & -38.5$\pm$2.19 & -13.79$\pm$2.19 & 7.0$\pm$1.0$^{(1)}$ & -36.1 & -14.1 & 100 & 13.66\\ 
212075509 & 08 49 02.50 & +21 33 24.2 & 16.25 & 12.45 & -37.3$\pm$2.24 & -17.31$\pm$2.24 & 8.6$\pm$1.2$^{(1)}$ & -38.0 & -13.5 & 85 & 5.02\\ 
212075775 & 08 40 36.24 & +21 33 42.2 & 11.46 & 9.97 & -34.25$\pm$2.55 & -14.7$\pm$1.29 & 5.7$\pm$0.8$^{(0)}$ & -36.5 & -14.0 & 100 & 9.02\\ 
212075988 & 08 36 57.83 & +21 33 55.8 & 13.75 & 11.12 & -35.04$\pm$2.19 & -12.73$\pm$2.19 & 4.6$\pm$0.6$^{(1)}$ & -35.9 & -14.2 & 100 & 13.98\\ 
212076029 & 08 27 00.80 & +21 33 58.7 & 18.24 & 14.11 & -29.84$\pm$2.27 & -14.3$\pm$2.27 & 5.5$\pm$0.8$^{(1)}$ & -34.0 & -14.8 & 93 & 0.32\\ 
212076402 & 08 41 26.02 & +21 34 25.3 & 17.92 & 14.03 & -36.2$\pm$2.69 & -19.72$\pm$2.69 & 5.6$\pm$0.8$^{(1)}$ & -36.6 & -14.0 & 100 & 0.66\\ 
212077235 & 08 31 10.45 & +21 35 22.4 & 13.51 & 11.21 & -35.42$\pm$2.24 & -15.02$\pm$2.24 & 4.1$\pm$0.6$^{(1)}$ & -34.8 & -14.6 & 98 & 16.16\\ 
212077781 & 08 39 12.57 & +21 35 57.1 & 17.81 & 14.0 & -38.27$\pm$2.19 & -14.12$\pm$2.19 & 5.1$\pm$0.7$^{(1)}$ & -36.3 & -14.1 & 100 &  \\ 
212078299 & 08 46 09.20 & +21 36 28.9 & 17.06 & 13.18 & -40.78$\pm$2.19 & -16.48$\pm$2.19 & 6.0$\pm$0.8$^{(1)}$ & -37.5 & -13.7 & 100 & 1.59\\ 
212078318 & 08 36 24.30 & +21 36 29.9 & 12.43 & 10.65 & -27.73$\pm$2.19 & -8.77$\pm$2.19 & 4.4$\pm$0.6$^{(1)}$ & -35.8 & -14.3 & 53 &  \\ 
212078515 & 08 30 48.52 & +21 36 45.3 & 18.01 & 14.0 & -36.72$\pm$2.78 & -17.06$\pm$2.78 & 5.0$\pm$0.7$^{(1)}$ & -34.7 & -14.6 & 99 & 1.32\\ 
212078811 & 08 44 53.87 & +21 37 06.5 & 15.31 & 12.01 & -37.52$\pm$2.19 & -16.2$\pm$2.19 & 5.3$\pm$0.7$^{(1)}$ & -37.3 & -13.8 & 100 & 23.67\\ 
212080687 & 08 45 27.95 & +21 39 12.9 & 10.36 & 9.26 & -35.19$\pm$0.14 & -13.63$\pm$0.08 & 4.8$\pm$0.3$^{(0)}$ & -37.4 & -13.8 & 100 & 4.92\\ 
212081702 & 08 43 22.57 & +21 40 18.1 & 10.35 & 8.97 & -36.94$\pm$1.87 & -15.19$\pm$0.94 & 5.8$\pm$0.6$^{(0)}$ & -37.0 & -13.9 & 100 & 11.17\\ 
212082288 & 08 44 32.59 & +21 40 59.3 & 16.02 & 12.46 & -36.6$\pm$2.19 & -17.44$\pm$2.19 & 5.8$\pm$0.8$^{(1)}$ & -37.2 & -13.9 & 100 & 3.98\\ 
212083165 & 08 54 45.75 & +21 41 58.0 & 17.12 & 13.4 & -41.29$\pm$2.22 & -16.72$\pm$2.23 & 5.2$\pm$0.7$^{(1)}$ & -38.9 & -13.2 & 79 & 1.54\\ 
212085055 & 08 54 16.84 & +21 44 04.2 & 12.76 & 10.48 & -33.99$\pm$2.26 & -16.3$\pm$2.26 & 5.9$\pm$0.8$^{(1)}$ & -38.9 & -13.3 & 52 &  \\ 
212085291 & 08 39 35.72 & +21 44 21.4 & 18.65 & 14.66 & -37.03$\pm$2.82 & -17.17$\pm$2.81 & 4.3$\pm$0.6$^{(1)}$ & -36.3 & -14.2 & 100 & 0.69\\ 
212085300 & 08 24 33.04 & +21 44 21.9 & 9.82 & 8.86 & -32.8$\pm$1.1 & -14.63$\pm$0.67 & 5.0$\pm$0.3$^{(0)}$ & -33.6 & -15.0 & 91 & $<$2\\ 
212085656 & 08 42 20.21 & +21 44 44.0 & 18.58 & 14.49 & -35.72$\pm$2.81 & -16.54$\pm$2.81 & 4.5$\pm$0.6$^{(1)}$ & -36.8 & -14.0 & 100 & 0.18\\ 
212086091 & 08 43 02.90 & +21 45 13.7 & 17.11 & 13.07 & -40.98$\pm$2.26 & -14.66$\pm$2.26 & 9.0$\pm$1.2$^{(1)}$ & -36.9 & -14.0 & 95 & 37.13\\ 
212086391 & 08 38 47.88 & +21 45 33.4 & 17.62 & 13.53 & -41.16$\pm$2.72 & -16.56$\pm$2.72 & 7.7$\pm$1.1$^{(1)}$ & -36.2 & -14.3 & 99 & 53.73\\ 
212086697 & 08 44 40.49 & +21 45 53.8 & 15.86 & 12.34 & -37.95$\pm$2.26 & -16.13$\pm$2.26 & 5.6$\pm$0.8$^{(1)}$ & -37.2 & -13.9 & 100 & 24.44\\ 
212087322 & 08 32 33.54 & +21 46 32.9 & 18.33 & 14.08 & -40.44$\pm$2.78 & -21.31$\pm$2.78 & 5.5$\pm$0.8$^{(1)}$ & -35.1 & -14.6 & 97 &  \\ 
212087671 & 08 53 56.29 & +21 46 54.0 & 9.13 & 8.24 & -42.59$\pm$0.87 & -15.22$\pm$0.58 & 6.3$\pm$0.3$^{(0)}$ & -38.8 & -13.3 & 72 & $<$2\\ 
212088298 & 08 44 10.93 & +21 47 38.4 & 16.28 & 12.72 & -38.9$\pm$2.26 & -17.2$\pm$2.26 & 5.1$\pm$0.7$^{(1)}$ & -37.1 & -14.0 & 100 & 15.33\\ 
212088355 & 08 28 34.95 & +21 47 42.4 & 12.51 & 10.73 & -31.42$\pm$0.92 & -13.08$\pm$0.96 & 4.1$\pm$0.6$^{(1)}$ & -34.3 & -14.9 & 87 & 64.03\\ 
212088614 & 08 45 28.04 & +21 48 02.9 & 16.69 & 13.24 & -38.72$\pm$2.26 & -18.64$\pm$2.26 & 3.4$\pm$0.5$^{(1)}$ & -37.4 & -13.9 & 26 &  \\ 
212089563 & 08 54 28.82 & +21 49 06.2 & 18.02 & 14.08 & -40.84$\pm$2.85 & -16.52$\pm$2.86 & 4.9$\pm$0.7$^{(1)}$ & -38.9 & -13.3 & 78 & 0.31\\ 
212095866 & 08 38 56.16 & +21 56 27.1 & 18.23 & 14.36 & -40.85$\pm$2.34 & -16.99$\pm$2.34 & 3.8$\pm$0.5$^{(1)}$ & -36.2 & -14.4 & 95 & 0.58\\ 
212097405 & 08 32 04.07 & +21 58 15.5 &   & 10.38 & -42.5$\pm$1.6 & -19.6$\pm$1.2 & 4.6$\pm$0.6$^{(2)}$ & -35.0 & -14.8 & 45 &  \\ 
212100566 & 08 49 21.37 & +22 01 57.0 & 18.17 & 14.36 & -35.28$\pm$2.91 & -20.11$\pm$2.91 & 4.5$\pm$0.6$^{(1)}$ & -38.0 & -13.8 & 85 &  \\ 
212100611 & 08 37 22.44 & +22 02 00.4 & 15.98 & 12.25 & -38.16$\pm$2.24 & -14.97$\pm$2.24 & 8.8$\pm$1.2$^{(1)}$ & -35.9 & -14.5 & 96 & 1.34\\ 
212103507 & 08 39 21.31 & +22 05 20.7 & 16.68 & 13.06 & -36.32$\pm$2.19 & -18.18$\pm$2.19 & 4.8$\pm$0.7$^{(1)}$ & -36.3 & -14.4 & 100 & 66.88\\ 
212103723 & 08 33 21.94 & +22 05 34.5 & 18.35 & 14.4 & -28.65$\pm$2.84 & -12.4$\pm$2.84 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -14.8 & 94 & 44.23\\ 
212104191 & 08 27 58.13 & +22 06 07.5 & 9.54 & 8.63 & -34.45$\pm$0.14 & -15.2$\pm$0.07 & 6.7$\pm$0.5$^{(0)}$ & -34.2 & -15.1 & 96 & 1.13\\ 
212108286 & 08 42 07.86 & +22 11 05.2 & 16.67 & 13.02 & -38.85$\pm$2.27 & -16.59$\pm$2.27 & 5.3$\pm$0.7$^{(1)}$ & -36.8 & -14.3 & 100 & 28.1\\ 
212109351 & 08 32 58.08 & +22 12 20.4 & 16.29 & 12.87 & -39.9$\pm$2.26 & -14.04$\pm$2.26 & 4.1$\pm$0.6$^{(1)}$ & -35.1 & -14.9 & 93 & 10.51\\ 
212110857 & 08 51 16.86 & +22 14 06.7 & 17.46 & 13.53 & -40.81$\pm$2.27 & -14.38$\pm$2.28 & 5.8$\pm$0.8$^{(1)}$ & -38.3 & -13.8 & 95 & 0.92\\ 
212111862 & 08 26 01.23 & +22 15 20.0 & 16.94 & 13.17 & -33.61$\pm$2.22 & -10.55$\pm$2.22 & 5.6$\pm$0.8$^{(1)}$ & -33.9 & -15.3 & 46 & 1.62\\ 
212112321 & 08 41 11.63 & +22 15 51.8 & 15.43 & 12.1 & -34.98$\pm$2.26 & -20.4$\pm$2.26 & 5.1$\pm$0.7$^{(1)}$ & -36.6 & -14.4 & 99 & 38.07\\ 
212112522 & 08 41 28.96 & +22 16 05.5 & 9.87 & 8.7 & -35.95$\pm$1.46 & -19.53$\pm$0.76 & 4.4$\pm$0.5$^{(0)}$ & -36.7 & -14.4 & 77 &  \\ 
212112533 & 08 36 49.43 & +22 16 06.2 & 17.98 & 13.87 & -26.16$\pm$2.72 & -19.95$\pm$2.72 & 6.4$\pm$0.9$^{(1)}$ & -35.8 & -14.7 & 37 & 43.59\\ 
212112578 & 08 43 38.80 & +22 16 09.2 & 11.96 & 10.25 & -38.22$\pm$2.72 & -15.52$\pm$1.32 & 5.9$\pm$0.8$^{(0)}$ & -37.0 & -14.3 & 100 & 8.89\\ 
212112752 & 08 49 22.08 & +22 16 22.0 & 15.73 & 12.23 & -39.01$\pm$2.28 & -15.0$\pm$2.28 & 5.5$\pm$0.8$^{(1)}$ & -38.0 & -13.9 & 98 & 4.12\\ 
212119822 & 08 41 36.59 & +22 24 46.2 & 15.85 & 12.28 & -41.46$\pm$2.26 & -19.11$\pm$2.26 & 6.4$\pm$0.9$^{(1)}$ & -36.7 & -14.5 & 97 & 16.33\\ 
212120476 & 08 48 50.35 & +22 25 32.0 & 13.25 & 10.72 & -28.42$\pm$2.3 & -13.43$\pm$2.3 & 5.7$\pm$0.8$^{(1)}$ & -37.9 & -14.1 & 18 & 16.79\\ 
212123277 & 08 40 58.77 & +22 28 50.0 & 19.0 & 14.89 & -38.22$\pm$3.0 & -15.67$\pm$3.0 & 4.5$\pm$0.6$^{(1)}$ & -36.6 & -14.6 & 99 & 13.79\\ 
212127087 & 08 48 14.77 & +22 33 32.6 & 14.8 & 11.65 & -38.31$\pm$2.3 & -12.53$\pm$2.3 & 5.2$\pm$0.7$^{(1)}$ & -37.8 & -14.2 & 98 & 18.11\\ 
212129124 & 08 44 25.56 & +22 35 59.2 & 16.57 & 12.97 & -35.49$\pm$2.26 & -16.9$\pm$2.26 & 5.2$\pm$0.7$^{(1)}$ & -37.2 & -14.5 & 99 & 6.8\\ 
212129540 & 08 48 26.03 & +22 36 31.3 & 17.13 & 13.41 & -40.76$\pm$2.31 & -14.78$\pm$2.3 & 4.4$\pm$0.6$^{(1)}$ & -37.9 & -14.2 & 93 & 2.1\\ 
212129791 & 08 42 24.90 & +22 36 51.1 & 11.56 & 10.19 & -30.57$\pm$0.81 & -12.12$\pm$0.77 & 4.0$\pm$0.5$^{(1)}$ & -36.8 & -14.6 & 21 &  \\ 
212131016 & 08 28 06.88 & +22 38 20.3 & 13.3 & 10.67 & -42.1$\pm$2.22 & -20.16$\pm$2.22 & 5.8$\pm$0.8$^{(1)}$ & -34.2 & -15.5 & 14 &  \\ 
212132877 & 08 38 33.49 & +22 40 35.0 & 17.64 & 13.92 & -37.95$\pm$2.8 & -13.98$\pm$2.8 & 4.4$\pm$0.6$^{(1)}$ & -36.1 & -14.9 & 99 & 0.86\\ 
212133159 & 08 37 57.28 & +22 40 55.4 & 16.84 & 13.15 & -40.77$\pm$2.3 & -18.84$\pm$2.3 & 5.0$\pm$0.7$^{(1)}$ & -36.0 & -14.9 & 98 & 23.12\\ 
212137502 & 08 35 54.98 & +22 46 11.3 & 12.03 & 10.23 & -33.75$\pm$2.26 & -20.32$\pm$2.26 & 5.2$\pm$0.7$^{(1)}$ & -35.7 & -15.1 & 96 & 9.63\\ 
212138965 & 08 41 33.83 & +22 47 55.7 & 16.69 & 12.93 & -34.96$\pm$2.26 & -16.46$\pm$2.26 & 6.4$\pm$0.9$^{(1)}$ & -36.7 & -14.8 & 99 & 5.83\\ 
212142153 & 08 37 31.56 & +22 51 59.5 & 15.42 & 12.0 & -32.68$\pm$2.3 & -12.08$\pm$2.3 & 5.9$\pm$0.8$^{(1)}$ & -36.0 & -15.1 & 96 & 64.03\\ 
212144326 & 08 45 53.20 & +22 54 43.4 & 13.95 & 11.12 & -28.06$\pm$2.26 & -14.92$\pm$2.26 & 5.3$\pm$0.7$^{(1)}$ & -37.4 & -14.6 & 17 &  \\ 
212148248 & 08 46 10.31 & +22 59 44.8 & 19.6 & 15.09 & -33.97$\pm$3.14 & -11.83$\pm$3.13 & 4.3$\pm$0.6$^{(1)}$ & -37.5 & -14.6 & 67 & 20.17\\ 
212152808 & 08 39 35.86 & +23 05 41.2 & 17.16 & 13.3 & -43.21$\pm$2.26 & -19.94$\pm$2.26 & 6.7$\pm$0.9$^{(1)}$ & -36.3 & -15.1 & 53 & 1.73\\ 
212154066 & 08 40 57.84 & +23 07 17.0 & 18.19 & 14.17 & -36.42$\pm$2.84 & -13.87$\pm$2.83 & 4.8$\pm$0.7$^{(1)}$ & -36.6 & -15.0 & 97 & 0.67\\ 
212155860 & 08 33 15.76 & +23 09 43.4 & 17.58 & 13.72 & -33.96$\pm$2.26 & -14.04$\pm$2.26 & 5.0$\pm$0.7$^{(1)}$ & -35.2 & -15.5 & 94 & 1.08\\ 
212161536 & 08 40 03.51 & +23 17 17.4 & 17.3 & 13.41 & -36.16$\pm$2.85 & -12.64$\pm$2.84 & 6.7$\pm$0.9$^{(1)}$ & -36.4 & -15.2 & 89 & 28.36\\ 
212163442 & 08 48 56.26 & +23 19 56.6 & 13.95 & 10.86 & -40.58$\pm$2.3 & -17.2$\pm$2.3 & 7.5$\pm$1.0$^{(1)}$ & -38.0 & -14.6 & 26 & 14.81\\ 
212171351 & 08 33 26.29 & +23 31 12.3 & 15.86 & 12.37 & -33.7$\pm$2.26 & -12.25$\pm$2.26 & 5.3$\pm$0.7$^{(1)}$ & -35.2 & -15.8 & 69 & 10.69\\ 
212173061 & 08 30 08.82 & +23 33 36.5 & 11.82 & 9.74 & -37.64$\pm$2.49 & -15.01$\pm$2.49 & 7.3$\pm$1.0$^{(1)}$ & -34.6 & -16.0 & 17 & 24.05\\ 
212178022 & 08 27 25.53 & +23 41 06.1 & 14.15 & 11.34 & -34.48$\pm$2.22 & -14.67$\pm$2.22 & 5.6$\pm$0.8$^{(1)}$ & -34.1 & -16.2 & 18 &  \\ 
\enddata 
 \tablecomments{stuff} 
 \label{Prmemtab} 
 \end{deluxetable} 


==> USA_memtable.tex <==
\begin{deluxetable}{cccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Candidate Upper Scorpius members.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} \\ } 
 \startdata 
202515599 & 16 10 15.42 & -29 23 56.2 & 16.41 & 12.08 & -18.12$\pm$2.53 & -23.85$\pm$2.53 & 5.5$\pm$1.0$^{(1)}$ & -13.2 & -24.3 & 82 & 42.5\\ 
202521690 & 16 13 18.45 & -29 22 27.6 & 12.91 & 9.22 & -10.34$\pm$2.37 & -34.36$\pm$2.36 & 9.6$\pm$1.8$^{(1)}$ & -13.0 & -24.4 & 88 & 6.128\\ 
202585030 & 16 10 24.19 & -29 07 29.4 & 12.07 & 9.07 & -12.06$\pm$2.36 & -21.63$\pm$2.36 & 6.0$\pm$1.1$^{(1)}$ & -13.2 & -24.3 & 91 & 35.21\\ 
202590973 & 16 25 12.15 & -29 06 07.5 & 13.33 & 9.83 & -12.97$\pm$2.3 & -15.41$\pm$2.3 & 5.3$\pm$1.0$^{(1)}$ & -12.2 & -24.6 & 49 &  \\ 
202600756 & 16 29 50.31 & -29 03 53.4 & 9.79 & 8.64 & -8.04$\pm$1.3 & -22.43$\pm$1.07 & 6.7$\pm$0.3$^{(0)}$ & -11.8 & -24.7 & 97 & 0.927\\ 
202605327 & 16 25 37.86 & -29 02 50.2 & 13.98 & 10.52 & -13.12$\pm$2.09 & -15.3$\pm$2.09 & 4.5$\pm$0.8$^{(1)}$ & -12.1 & -24.6 & 13 &  \\ 
202615424 & 16 29 11.40 & -29 00 31.7 & 13.56 & 9.95 & -13.52$\pm$2.32 & -27.85$\pm$2.31 & 6.8$\pm$1.3$^{(1)}$ & -11.9 & -24.7 & 95 & 3.694\\ 
202621661 & 16 12 36.93 & -28 59 06.6 & 11.23 & 9.52 & -0.47$\pm$1.06 & -27.43$\pm$0.66 & 7.5$\pm$0.3$^{(0)}$ & -13.1 & -24.3 & 62 &  \\ 
202638454 & 16 30 20.09 & -28 55 18.0 & 16.32 & 11.77 & -11.53$\pm$2.15 & -36.68$\pm$2.13 & 7.1$\pm$1.3$^{(1)}$ & -11.8 & -24.7 & 86 & 17.466\\ 
202661596 & 16 24 22.06 & -28 50 04.1 & 12.45 & 9.44 & -5.9$\pm$2.31 & -13.78$\pm$2.31 & 5.2$\pm$1.0$^{(1)}$ & -12.2 & -24.6 & 19 &  \\ 
202685674 & 16 23 58.57 & -28 44 34.1 & 12.88 & 9.76 & -4.41$\pm$2.33 & -33.4$\pm$2.58 & 4.6$\pm$0.9$^{(1)}$ & -12.2 & -24.6 & 19 &  \\ 
202687442 & 16 34 58.65 & -28 44 10.1 & 15.6 & 11.59 & -10.74$\pm$2.09 & -22.76$\pm$2.09 & 4.6$\pm$0.9$^{(1)}$ & -11.5 & -24.8 & 58 & 41.941\\ 
202689729 & 16 27 54.86 & -28 43 39.3 & 12.27 & 9.02 & -13.05$\pm$2.3 & -24.83$\pm$2.3 & 6.9$\pm$1.3$^{(1)}$ & -12.0 & -24.7 & 95 & 1.541\\ 
202694812 & 16 23 05.89 & -28 42 30.2 & 11.84 & 8.97 & -5.89$\pm$2.33 & -12.4$\pm$2.33 & 6.6$\pm$1.2$^{(1)}$ & -12.3 & -24.6 & 26 & 36.663\\ 
202699293 & 16 12 30.76 & -28 41 30.0 & 12.52 & 9.39 & -10.59$\pm$2.36 & -24.66$\pm$2.36 & 5.6$\pm$1.0$^{(1)}$ & -13.0 & -24.3 & 90 & 6.822\\ 
202703609 & 16 24 55.41 & -28 40 32.5 & 11.58 & 9.36 & -13.71$\pm$1.96 & -29.97$\pm$1.53 & 4.4$\pm$0.8$^{(1)}$ & -12.2 & -24.6 & 32 &  \\ 
202704279 & 16 17 14.32 & -28 40 23.2 & 14.11 & 10.5 & -3.57$\pm$2.13 & -22.61$\pm$2.13 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -24.4 & 52 & 5.246\\ 
202709152 & 16 23 31.17 & -28 39 17.6 &   & 11.62 & -3.6$\pm$5.4 & -17.0$\pm$5.4 & 13.2$\pm$2.4$^{(4)}$ & -12.3 & -24.6 & 45 & 0.804\\ 
202709674 & 16 25 04.92 & -28 39 11.1 & 12.39 & 9.31 & -7.26$\pm$2.3 & -27.02$\pm$2.3 & 5.8$\pm$1.1$^{(1)}$ & -12.2 & -24.6 & 89 & 4.393\\ 
202709894 & 16 28 18.69 & -28 39 08.2 & 12.58 & 9.53 & -4.52$\pm$2.3 & -17.57$\pm$2.3 & 5.2$\pm$1.0$^{(1)}$ & -11.9 & -24.7 & 43 &  \\ 
202710503 & 16 08 46.76 & -28 38 59.7 & 14.14 & 10.43 & -13.63$\pm$2.14 & -24.07$\pm$2.14 & 5.6$\pm$1.0$^{(1)}$ & -13.3 & -24.2 & 91 & \\ 
202715668 & 16 29 33.84 & -28 37 51.5 & 13.36 & 9.93 & -12.04$\pm$2.3 & -15.09$\pm$2.3 & 4.6$\pm$0.9$^{(1)}$ & -11.8 & -24.7 & 19 &  \\ 
202725805 & 16 17 33.79 & -28 35 33.4 & 10.81 & 9.11 & -13.77$\pm$3.53 & -14.09$\pm$0.79 & 5.2$\pm$0.8$^{(0)}$ & -12.7 & -24.4 & 36 &  \\ 
202727642 & 16 28 39.26 & -28 35 09.4 & 13.27 & 8.99 & -7.22$\pm$2.31 & -13.05$\pm$2.3 & 10.9$\pm$2.0$^{(1)}$ & -11.9 & -24.7 & 27 &  \\ 
202743203 & 16 28 55.66 & -28 31 43.7 & 12.35 & 9.29 & -4.71$\pm$2.3 & -17.26$\pm$2.3 & 5.6$\pm$1.0$^{(1)}$ & -11.9 & -24.7 & 51 & 33.093\\ 
202758288 & 16 29 29.75 & -28 28 22.0 & 12.31 & 9.3 & -5.12$\pm$2.3 & -13.6$\pm$2.3 & 5.7$\pm$1.0$^{(1)}$ & -11.8 & -24.7 & 24 &  \\ 
202772489 & 16 23 01.19 & -28 25 11.4 & 12.98 & 9.34 & -14.49$\pm$2.33 & -21.18$\pm$2.33 & 7.2$\pm$1.3$^{(1)}$ & -12.3 & -24.5 & 93 & 17.176\\ 
202773970 & 16 29 51.68 & -28 24 52.0 & 15.35 & 11.18 & -9.84$\pm$2.12 & -18.89$\pm$2.12 & 5.0$\pm$0.9$^{(1)}$ & -11.8 & -24.7 & 61 & 3.595\\ 
202774770 & 16 25 22.91 & -28 24 41.5 & 12.85 & 9.48 & -5.44$\pm$2.3 & -11.72$\pm$2.3 & 5.6$\pm$1.0$^{(1)}$ & -12.1 & -24.6 & 11 &  \\ 
202791563 & 16 22 21.05 & -28 21 00.4 & 15.41 & 11.39 & -10.52$\pm$2.1 & -24.33$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -12.3 & -24.5 & 90 & 1.203\\ 
202795175 & 16 23 41.87 & -28 20 12.7 &   & 12.74 & -10.1$\pm$5.4 & -17.2$\pm$5.4 & 20.1$\pm$3.7$^{(4)}$ & -12.2 & -24.5 & 32 & 0.836\\ 
202800225 & 16 28 50.18 & -28 19 06.8 & 12.98 & 8.8 & -11.62$\pm$2.3 & -22.82$\pm$2.3 & 11.0$\pm$2.0$^{(1)}$ & -11.9 & -24.7 & 91 & 21.289\\ 
202800875 & 16 22 13.15 & -28 18 58.6 & 12.28 & 9.1 & -8.96$\pm$2.31 & -24.18$\pm$2.31 & 6.4$\pm$1.2$^{(1)}$ & -12.3 & -24.5 & 93 & 0.673\\ 
202805654 & 16 29 29.07 & -28 17 55.4 & 13.46 & 9.62 & -15.19$\pm$2.3 & -12.08$\pm$2.3 & 6.4$\pm$1.2$^{(1)}$ & -11.8 & -24.7 & 32 &  \\ 
202814875 & 16 28 10.75 & -28 15 53.2 & 11.92 & 8.09 & -21.5$\pm$2.45 & -21.47$\pm$2.45 & 12.2$\pm$2.3$^{(1)}$ & -11.9 & -24.6 & 59 &  \\ 
202826247 & 16 12 20.22 & -28 13 22.2 & 13.95 & 10.46 & -12.22$\pm$2.17 & -25.48$\pm$2.17 & 4.8$\pm$0.9$^{(1)}$ & -13.0 & -24.3 & 72 & 1.809\\ 
202828127 & 16 28 08.97 & -28 12 56.4 & 17.01 & 12.11 & -9.75$\pm$2.55 & -27.82$\pm$2.55 & 6.7$\pm$1.2$^{(1)}$ & -11.9 & -24.6 & 95 & 1.167\\ 
202853972 & 16 14 32.01 & -28 07 23.1 & 14.27 & 10.46 & -11.32$\pm$2.17 & -23.61$\pm$2.17 & 6.4$\pm$1.2$^{(1)}$ & -12.9 & -24.3 & 94 & 8.664\\ 
202862458 & 16 22 21.35 & -28 05 32.6 & 14.07 & 10.57 & -16.93$\pm$2.11 & -18.61$\pm$2.11 & 4.5$\pm$0.8$^{(1)}$ & -12.3 & -24.5 & 23 &  \\ 
202873945 & 16 21 39.92 & -28 03 06.6 & 16.0 & 11.24 & -4.99$\pm$2.51 & -24.17$\pm$2.51 & 8.6$\pm$1.6$^{(1)}$ & -12.4 & -24.5 & 88 & 0.625\\ 
202879519 & 16 10 44.58 & -28 01 53.9 & 14.88 & 10.77 & -17.26$\pm$2.23 & -31.88$\pm$2.3 & 7.6$\pm$1.4$^{(1)}$ & -13.1 & -24.2 & 94 &  \\ 
202880081 & 16 10 44.79 & -28 01 46.8 & 13.88 & 10.25 & -10.76$\pm$2.12 & -15.96$\pm$2.19 & 5.5$\pm$1.0$^{(1)}$ & -13.1 & -24.2 & 65 & 5.073\\ 
202888106 & 16 39 51.92 & -28 00 04.2 & 13.13 & 10.05 & -10.62$\pm$2.17 & -19.08$\pm$2.15 & 4.2$\pm$0.8$^{(1)}$ & -11.1 & -24.9 & 18 & \\ 
202891681 & 16 23 20.77 & -27 59 17.6 &   & 8.06 & -7.8$\pm$5.8 & -5.6$\pm$11.3 & 207.2$\pm$38.2$^{(4)}$ & -12.3 & -24.5 & 14 &  \\ 
202901848 & 16 40 26.53 & -27 57 08.2 & 13.5 & 9.76 & -3.2$\pm$2.33 & -26.55$\pm$2.33 & 8.4$\pm$1.5$^{(1)}$ & -11.1 & -24.9 & 88 & 2.952\\ 
202902270 & 16 31 31.86 & -27 57 02.4 & 10.25 & 8.84 & -9.22$\pm$2.02 & -13.31$\pm$2.76 & 5.0$\pm$0.7$^{(0)}$ & -11.7 & -24.7 & 19 &  \\ 
202905782 & 16 25 38.27 & -27 56 16.9 & 12.14 & 8.95 & -14.08$\pm$2.33 & -10.64$\pm$2.33 & 6.9$\pm$1.3$^{(1)}$ & -12.1 & -24.6 & 25 &  \\ 
202906224 & 16 23 17.62 & -27 56 11.0 & 16.09 & 11.69 & -12.9$\pm$2.49 & -20.24$\pm$2.49 & 5.5$\pm$1.0$^{(1)}$ & -12.3 & -24.5 & 84 & 0.715\\ 
202906766 & 16 15 13.19 & -27 56 04.1 & 14.89 & 11.07 & -16.83$\pm$2.17 & -15.46$\pm$2.31 & 4.6$\pm$0.8$^{(1)}$ & -12.8 & -24.3 & 15 & 4.343\\ 
202910245 & 16 18 09.11 & -27 55 19.6 &   & 11.4 & -5.7$\pm$4.3 & -21.1$\pm$4.3 & 17.9$\pm$3.3$^{(4)}$ & -12.6 & -24.4 & 42 & 0.588\\ 
202910382 & 16 29 02.24 & -27 55 18.1 & 10.35 & 8.8 & -29.66$\pm$2.16 & -26.8$\pm$1.42 & 9.1$\pm$0.7$^{(0)}$ & -11.9 & -24.6 & 24 &  \\ 
202911961 & 16 30 15.68 & -27 54 58.5 & 6.83 & 6.36 & -10.67$\pm$0.59 & -13.32$\pm$0.21 & 5.8$\pm$0.7$^{(0)}$ & -11.8 & -24.7 & 40 &  \\ 
202915242 & 16 10 21.55 & -27 54 17.4 & 15.35 & 11.2 & -19.4$\pm$2.42 & -18.65$\pm$2.42 & 6.0$\pm$1.1$^{(1)}$ & -13.2 & -24.2 & 75 & 1.266\\ 
202919426 & 16 21 09.02 & -27 53 24.4 & 13.51 & 9.98 & -18.8$\pm$2.34 & -15.08$\pm$2.34 & 5.2$\pm$1.0$^{(1)}$ & -12.4 & -24.5 & 27 & 16.358\\ 
202925169 & 16 07 57.86 & -27 52 11.6 &   & 8.86 & -3.6$\pm$2.8 & -20.5$\pm$2.5 & 5.0$\pm$0.9$^{(2)}$ & -13.3 & -24.2 & 36 &  \\ 
202930098 & 16 24 32.77 & -27 51 10.4 & 12.21 & 9.48 & -16.32$\pm$2.33 & -15.98$\pm$2.33 & 4.6$\pm$0.8$^{(1)}$ & -12.2 & -24.5 & 16 &  \\ 
202942404 & 16 16 11.27 & -27 48 33.9 & 11.57 & 8.34 & -6.54$\pm$2.4 & -10.96$\pm$2.4 & 8.8$\pm$1.6$^{(1)}$ & -12.8 & -24.3 & 17 & $<$2\\ 
202943412 & 16 28 20.69 & -27 48 21.3 & 10.92 & 8.61 & -14.58$\pm$0.97 & -11.71$\pm$1.05 & 6.7$\pm$1.2$^{(1)}$ & -11.9 & -24.6 & 22 &  \\ 
202949470 & 16 22 54.82 & -27 47 05.5 & 12.65 & 9.21 & -11.21$\pm$2.34 & -11.51$\pm$2.34 & 6.3$\pm$1.2$^{(1)}$ & -12.3 & -24.5 & 32 &  \\ 
202950433 & 16 27 36.91 & -27 46 54.4 & 11.77 & 8.49 & -15.64$\pm$2.33 & -9.96$\pm$2.33 & 9.3$\pm$1.7$^{(1)}$ & -11.9 & -24.6 & 13 &  \\ 
202955657 & 16 26 37.99 & -27 45 48.4 & 11.59 & 8.14 & -17.24$\pm$2.33 & -14.33$\pm$2.33 & 10.7$\pm$2.0$^{(1)}$ & -12.0 & -24.6 & 43 &  \\ 
202957308 & 16 27 48.85 & -27 45 27.2 &   & 7.16 & -11.5$\pm$7.1 & -11.2$\pm$7.1 & 396.1$\pm$73.0$^{(4)}$ & -11.9 & -24.6 & 21 &  \\ 
202959419 & 16 23 57.64 & -27 44 59.2 & 12.05 & 9.18 & -9.59$\pm$2.32 & -29.3$\pm$2.32 & 5.4$\pm$1.0$^{(1)}$ & -12.2 & -24.5 & 84 & 2.698\\ 
202960425 & 16 09 00.96 & -27 44 46.5 &   & 10.8 & -18.4$\pm$8.5 & -16.2$\pm$8.2 & 9.8$\pm$1.8$^{(4)}$ & -13.3 & -24.2 & 79 & 0.645\\ 
202963882 & 16 13 18.91 & -27 44 02.5 & 13.71 & 9.62 & -8.04$\pm$2.4 & -18.95$\pm$2.4 & 13.0$\pm$2.4$^{(1)}$ & -13.0 & -24.3 & 68 &  \\ 
202970894 & 16 29 24.64 & -27 42 33.5 & 12.88 & 9.6 & -11.27$\pm$2.34 & -13.98$\pm$2.35 & 5.3$\pm$1.0$^{(1)}$ & -11.8 & -24.6 & 37 &  \\ 
202976791 & 16 35 44.56 & -27 41 18.4 & 11.75 & 8.9 & -7.18$\pm$2.33 & -18.11$\pm$2.33 & 6.1$\pm$1.1$^{(1)}$ & -11.4 & -24.8 & 79 & 28.787\\ 
202977790 & 16 43 50.29 & -27 41 05.8 & 14.57 & 10.82 & -11.05$\pm$2.19 & -23.65$\pm$2.17 & 5.0$\pm$0.9$^{(1)}$ & -10.8 & -24.9 & 78 & 9.842\\ 
202978875 & 16 09 01.69 & -27 40 52.1 &   & 11.95 & -20.4$\pm$5.5 & -17.9$\pm$5.5 & 15.5$\pm$2.9$^{(4)}$ & -13.3 & -24.2 & 49 & \\ 
202979611 & 16 23 26.71 & -27 40 43.1 & 13.07 & 9.48 & -8.54$\pm$2.34 & -11.56$\pm$2.34 & 6.0$\pm$1.1$^{(1)}$ & -12.2 & -24.5 & 24 &  \\ 
202982521 & 16 22 51.73 & -27 40 06.6 & 11.89 & 7.8 & -2.16$\pm$2.34 & -17.32$\pm$2.34 & 17.0$\pm$3.1$^{(1)}$ & -12.3 & -24.5 & 10 &  \\ 
202988479 & 16 29 16.97 & -27 38 52.9 & 12.58 & 9.37 & -9.0$\pm$2.33 & -14.92$\pm$2.33 & 6.0$\pm$1.1$^{(1)}$ & -11.8 & -24.6 & 59 &  \\ 
203001378 & 16 21 54.81 & -27 36 10.3 & 15.67 & 11.47 & -9.29$\pm$2.49 & -19.17$\pm$2.49 & 4.8$\pm$0.9$^{(1)}$ & -12.3 & -24.5 & 55 & 2.956\\ 
203001822 & 16 41 48.59 & -27 36 04.3 & 14.64 & 10.97 & -8.01$\pm$2.11 & -21.3$\pm$2.11 & 4.4$\pm$0.8$^{(1)}$ & -11.0 & -24.9 & 32 & 1.63\\ 
203004488 & 16 18 44.32 & -27 35 30.4 & 16.79 & 12.24 & -5.22$\pm$2.61 & -27.78$\pm$2.6 & 4.7$\pm$0.9$^{(1)}$ & -12.6 & -24.4 & 42 & 1.454\\ 
203009087 & 16 26 51.61 & -27 34 31.7 & 14.04 & 9.88 & -4.87$\pm$2.33 & -10.95$\pm$2.33 & 6.7$\pm$1.2$^{(1)}$ & -12.0 & -24.6 & 12 &  \\ 
203013725 & 16 10 26.99 & -27 33 33.2 & 11.11 & 8.32 & -10.0$\pm$1.0 & -16.18$\pm$1.07 & 7.5$\pm$1.4$^{(1)}$ & -13.1 & -24.2 & 79 & \\ 
203013984 & 16 08 42.57 & -27 33 29.9 & 14.24 & 10.42 & -20.87$\pm$2.17 & -28.63$\pm$2.17 & 6.8$\pm$1.2$^{(1)}$ & -13.3 & -24.1 & 89 & 1.157\\ 
203017272 & 16 27 31.15 & -27 32 48.2 & 13.18 & 9.61 & -11.64$\pm$2.33 & -8.86$\pm$2.33 & 6.5$\pm$1.2$^{(1)}$ & -11.9 & -24.6 & 10 &  \\ 
203017692 & 16 14 45.68 & -27 32 43.1 & 13.7 & 9.98 & -9.1$\pm$2.4 & -27.13$\pm$2.4 & 6.6$\pm$1.2$^{(1)}$ & -12.8 & -24.3 & 94 & 5.116\\ 
203020085 & 16 12 32.32 & -27 32 13.3 & 11.11 & 9.05 & -12.02$\pm$1.08 & -22.08$\pm$0.7 & 5.3$\pm$0.3$^{(0)}$ & -13.0 & -24.2 & 65 & \\ 
203035025 & 16 36 20.25 & -27 29 04.5 & 8.64 & 5.88 & -9.53$\pm$0.57 & -26.21$\pm$0.64 & 23.8$\pm$4.4$^{(1)}$ & -11.3 & -24.7 & 68 &  \\ 
203036995 & 16 10 03.11 & -27 28 39.7 & 13.76 & 9.84 & -12.09$\pm$2.29 & -22.24$\pm$2.29 & 8.9$\pm$1.6$^{(1)}$ & -13.2 & -24.2 & 94 & 0.776\\ 
203046192 & 16 23 38.00 & -27 26 44.0 & 13.92 & 10.12 & -7.23$\pm$2.08 & -15.28$\pm$2.08 & 4.7$\pm$0.9$^{(1)}$ & -12.2 & -24.5 & 19 &  \\ 
203046199 & 16 28 14.12 & -27 26 43.9 & 11.41 & 9.02 & -7.84$\pm$0.98 & -20.76$\pm$1.06 & 5.3$\pm$1.0$^{(1)}$ & -11.9 & -24.6 & 79 & 1.357\\ 
203046225 & 16 41 01.32 & -27 26 43.5 & 9.59 & 4.61 & -14.52$\pm$3.61 & -12.49$\pm$3.61 & 159.0$\pm$29.3$^{(1)}$ & -11.0 & -24.8 & 22 &  \\ 
203048597 & 16 13 24.58 & -27 26 13.2 & 14.06 & 9.78 & -11.5$\pm$2.31 & -38.15$\pm$2.29 & 14.2$\pm$2.6$^{(1)}$ & -12.9 & -24.2 & 53 & 1.609\\ 
203053971 & 16 21 10.66 & -27 25 05.0 & 12.54 & 9.27 & -6.12$\pm$2.23 & -15.9$\pm$2.23 & 6.3$\pm$1.2$^{(1)}$ & -12.4 & -24.4 & 61 &  \\ 
203055760 & 16 26 19.11 & -27 24 42.1 & 13.21 & 9.62 & -5.0$\pm$2.33 & -18.5$\pm$2.33 & 5.9$\pm$1.1$^{(1)}$ & -12.0 & -24.5 & 69 & 1.761\\ 
203061783 & 16 27 02.52 & -27 23 26.3 & 13.02 & 9.3 & -15.71$\pm$2.33 & -13.02$\pm$2.33 & 6.4$\pm$1.2$^{(1)}$ & -12.0 & -24.5 & 44 & 26.684\\ 
203065665 & 16 24 26.01 & -27 22 38.6 & 11.09 & 8.73 & -12.63$\pm$0.97 & -22.33$\pm$1.08 & 6.0$\pm$1.1$^{(1)}$ & -12.2 & -24.5 & 93 & 2.461\\ 
203070560 & 16 13 51.89 & -27 21 38.0 & 13.93 & 10.26 & -9.95$\pm$2.09 & -13.92$\pm$2.09 & 4.5$\pm$0.8$^{(1)}$ & -12.9 & -24.3 & 11 & 3.697\\ 
203074940 & 16 26 25.40 & -27 20 42.7 & 15.49 & 11.18 & -8.86$\pm$2.09 & -18.57$\pm$2.09 & 5.9$\pm$1.1$^{(1)}$ & -12.0 & -24.5 & 82 & 3.349\\ 
203075534 & 16 24 58.31 & -27 20 35.3 & 13.75 & 9.61 & -4.58$\pm$2.23 & -10.74$\pm$2.23 & 7.2$\pm$1.3$^{(1)}$ & -12.1 & -24.5 & 10 &  \\ 
203082390 & 16 36 49.80 & -27 19 11.4 & 10.11 & 8.63 & -11.05$\pm$1.89 & -24.27$\pm$1.45 & 6.2$\pm$0.2$^{(0)}$ & -11.3 & -24.7 & 96 & 1.369\\ 
203082998 & 16 24 44.48 & -27 19 03.7 &   & 12.17 & -7.9$\pm$5.1 & -14.7$\pm$5.1 & 28.6$\pm$5.3$^{(4)}$ & -12.1 & -24.5 & 11 &  \\ 
203083616 & 16 14 52.53 & -27 18 55.7 & 17.73 & 12.82 & -17.85$\pm$2.59 & -21.79$\pm$2.59 & 4.8$\pm$0.9$^{(1)}$ & -12.8 & -24.3 & 53 & $<$2\\ 
203084039 & 16 27 52.93 & -27 18 50.5 & 14.13 & 10.11 & -2.87$\pm$2.13 & -17.15$\pm$2.13 & 5.2$\pm$1.0$^{(1)}$ & -11.9 & -24.6 & 27 &  \\ 
203086979 & 16 26 02.15 & -27 18 14.2 & 12.0 & 9.05 & -15.46$\pm$2.26 & -25.38$\pm$2.26 & 6.1$\pm$1.1$^{(1)}$ & -12.0 & -24.5 & 92 & 1.501\\ 
203087372 & 16 21 05.00 & -27 18 08.9 & 13.61 & 9.95 & -13.82$\pm$2.23 & -12.94$\pm$2.23 & 5.6$\pm$1.0$^{(1)}$ & -12.4 & -24.4 & 35 &  \\ 
203092153 & 16 25 57.31 & -27 17 10.5 & 12.21 & 9.19 & -10.35$\pm$2.52 & -13.0$\pm$1.94 & 5.7$\pm$1.1$^{(1)}$ & -12.0 & -24.5 & 37 &  \\ 
203092549 & 16 24 20.45 & -27 17 05.9 & 11.85 & 8.6 & -16.82$\pm$2.23 & -19.11$\pm$2.23 & 8.3$\pm$1.5$^{(1)}$ & -12.2 & -24.5 & 87 & \\ 
203092824 & 16 10 57.65 & -27 17 02.6 & 12.33 & 9.41 & -11.5$\pm$2.29 & -23.4$\pm$2.29 & 5.0$\pm$0.9$^{(1)}$ & -13.1 & -24.2 & 80 & 6.205\\ 
203097006 & 16 18 09.93 & -27 16 11.6 & 14.25 & 10.19 & -11.64$\pm$2.09 & -22.65$\pm$2.09 & 6.8$\pm$1.3$^{(1)}$ & -12.6 & -24.3 & 95 & 19.8\\ 
203098034 & 16 08 40.17 & -27 15 58.7 & 11.63 & 8.75 & -11.42$\pm$1.02 & -16.68$\pm$1.02 & 6.4$\pm$1.2$^{(1)}$ & -13.3 & -24.1 & 82 & 19.731\\ 
203102566 & 16 26 22.77 & -27 15 02.8 & 9.61 & 8.43 & -16.46$\pm$1.41 & -29.63$\pm$1.04 & 7.9$\pm$0.2$^{(0)}$ & -12.0 & -24.5 & 97 & 1.836\\ 
203106784 & 16 25 04.91 & -27 14 09.7 & 14.09 & 9.78 & -6.38$\pm$2.27 & -10.92$\pm$2.27 & 7.2$\pm$1.3$^{(1)}$ & -12.1 & -24.5 & 17 &  \\ 
203107349 & 16 25 49.17 & -27 14 02.7 & 11.88 & 8.93 & -13.26$\pm$2.26 & -10.37$\pm$2.26 & 6.3$\pm$1.2$^{(1)}$ & -12.1 & -24.5 & 19 &  \\ 
203108627 & 16 30 49.65 & -27 13 46.9 & 15.65 & 11.38 & -15.43$\pm$2.06 & -21.3$\pm$2.07 & 5.5$\pm$1.0$^{(1)}$ & -11.7 & -24.6 & 82 & 1.222\\ 
203112557 & 16 23 07.60 & -27 12 57.5 & 13.39 & 9.74 & -19.51$\pm$2.23 & -31.44$\pm$2.23 & 7.0$\pm$1.3$^{(1)}$ & -12.2 & -24.5 & 89 & 7.837\\ 
203115450 & 16 31 06.67 & -27 12 21.4 & 11.67 & 8.63 & -5.69$\pm$2.26 & -15.93$\pm$2.26 & 7.5$\pm$1.4$^{(1)}$ & -11.7 & -24.6 & 65 &  \\ 
203122134 & 16 31 18.68 & -27 10 58.7 & 15.5 & 11.35 & -14.69$\pm$2.1 & -24.31$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -11.7 & -24.6 & 84 & 0.988\\ 
203122455 & 16 30 57.54 & -27 10 54.8 & 10.19 & 8.39 & -17.47$\pm$1.95 & -20.28$\pm$1.41 & 5.5$\pm$0.6$^{(0)}$ & -11.7 & -24.6 & 63 &  \\ 
203122463 & 16 15 48.69 & -27 10 54.7 &   & 11.88 & -20.0$\pm$5.1 & -28.4$\pm$5.1 & 27.2$\pm$5.0$^{(4)}$ & -12.8 & -24.3 & 27 & 1.466\\ 
203125449 & 16 30 24.15 & -27 10 17.8 & 15.01 & 10.94 & -9.33$\pm$2.11 & -20.03$\pm$2.12 & 5.2$\pm$0.9$^{(1)}$ & -11.7 & -24.6 & 74 & 2.657\\ 
203130129 & 16 35 44.73 & -27 09 20.3 & 15.51 & 11.56 & -12.14$\pm$2.06 & -23.18$\pm$2.06 & 4.3$\pm$0.8$^{(1)}$ & -11.4 & -24.7 & 36 & 1.612\\ 
203131475 & 16 24 30.42 & -27 09 04.1 & 7.41 & 6.72 & -21.51$\pm$0.05 & -29.24$\pm$0.03 & 6.4$\pm$0.4$^{(0)}$ & -12.1 & -24.5 & 100 &  \\ 
203138121 & 16 26 42.88 & -27 07 41.8 & 15.52 & 11.2 & -13.4$\pm$2.07 & -23.06$\pm$2.07 & 5.8$\pm$1.1$^{(1)}$ & -12.0 & -24.5 & 91 & 0.827\\ 
203141803 & 16 35 40.80 & -27 06 56.7 & 12.07 & 8.86 & -10.51$\pm$2.26 & -10.38$\pm$2.26 & 7.0$\pm$1.3$^{(1)}$ & -11.4 & -24.7 & 21 & 17.176\\ 
203166243 & 16 26 49.54 & -27 01 52.9 & 14.0 & 10.44 & -14.67$\pm$2.08 & -20.79$\pm$2.08 & 4.6$\pm$0.8$^{(1)}$ & -12.0 & -24.5 & 43 & 26.756\\ 
203241615 & 15 56 42.28 & -26 46 46.8 & 17.96 & 13.09 & -8.26$\pm$2.82 & -21.7$\pm$2.82 & 5.2$\pm$1.0$^{(1)}$ & -14.1 & -23.8 & 74 &  \\ 
203274630 & 16 04 52.85 & -26 40 13.7 & 9.35 & 8.1 & -23.44$\pm$1.0 & -34.9$\pm$0.5 & 9.6$\pm$0.2$^{(0)}$ & -13.5 & -24.0 & 64 & 2.324\\ 
203279708 & 16 04 55.24 & -26 39 13.6 & 13.09 & 9.69 & -21.38$\pm$2.29 & -35.92$\pm$2.29 & 6.1$\pm$1.1$^{(1)}$ & -13.5 & -24.0 & 62 &  \\ 
203301463 & 15 59 11.89 & -26 35 00.9 & 8.07 & 6.97 & -17.66$\pm$0.29 & -20.11$\pm$0.34 & 7.9$\pm$0.5$^{(0)}$ & -13.9 & -23.8 & 96 & $<$2\\ 
203302339 & 16 17 29.70 & -26 34 51.3 & 13.52 & 9.98 & -2.51$\pm$2.29 & -15.03$\pm$2.29 & 5.5$\pm$1.0$^{(1)}$ & -12.6 & -24.3 & 18 &  \\ 
203337149 & 16 13 06.29 & -26 28 25.2 & 10.89 & 8.07 & -23.94$\pm$0.98 & -17.02$\pm$0.98 & 8.6$\pm$1.6$^{(1)}$ & -12.9 & -24.2 & 28 &  \\ 
203337814 & 16 16 47.56 & -26 28 17.9 & 15.78 & 11.68 & -20.12$\pm$2.09 & -29.53$\pm$2.09 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -24.3 & 51 &  \\ 
203338523 & 16 21 27.98 & -26 28 10.0 & 16.5 & 11.88 & -9.15$\pm$2.64 & -23.89$\pm$2.52 & 6.7$\pm$1.2$^{(1)}$ & -12.3 & -24.4 & 94 & 19.828\\ 
203343161 & 16 24 55.88 & -26 27 18.1 & 15.62 & 11.16 & -9.38$\pm$2.04 & -31.6$\pm$2.04 & 7.8$\pm$1.4$^{(1)}$ & -12.1 & -24.4 & 94 &  \\ 
203354381 & 16 26 27.87 & -26 25 15.1 & 13.89 & 9.85 & -18.44$\pm$2.27 & -36.77$\pm$2.26 & 9.3$\pm$1.7$^{(1)}$ & -12.0 & -24.5 & 83 & $<$2\\ 
203362169 & 16 23 04.38 & -26 23 43.1 & 11.1 & 7.78 & -13.55$\pm$2.23 & -19.77$\pm$2.23 & 12.4$\pm$2.3$^{(1)}$ & -12.2 & -24.4 & 82 & 3.598\\ 
203363279 & 16 00 42.65 & -26 23 29.6 & 9.1 & 7.72 & -13.0$\pm$0.79 & -17.13$\pm$0.54 & 6.4$\pm$0.3$^{(0)}$ & -13.8 & -23.9 & 94 & 1.127\\ 
203366162 & 16 23 57.72 & -26 22 55.8 & 11.6 & 8.82 & -15.52$\pm$2.3 & -11.58$\pm$2.3 & 6.2$\pm$1.1$^{(1)}$ & -12.2 & -24.4 & 28 & 3.042\\ 
203377650 & 16 16 52.25 & -26 20 38.7 &   & 12.4 & -14.8$\pm$5.1 & -37.9$\pm$5.1 & 23.1$\pm$4.3$^{(4)}$ & -12.6 & -24.2 & 22 &  \\ 
203390179 & 16 23 00.63 & -26 18 06.7 & 11.78 & 8.94 & -17.0$\pm$2.23 & -17.77$\pm$2.23 & 5.9$\pm$1.1$^{(1)}$ & -12.2 & -24.4 & 74 & 1.395\\ 
203390805 & 16 27 14.36 & -26 17 58.8 & 12.59 & 9.53 & -13.75$\pm$2.25 & -25.07$\pm$2.25 & 5.2$\pm$1.0$^{(1)}$ & -11.9 & -24.5 & 84 & 4.728\\ 
203394211 & 16 23 21.87 & -26 17 16.1 & 12.28 & 9.22 & -11.8$\pm$2.23 & -19.88$\pm$2.23 & 5.4$\pm$1.0$^{(1)}$ & -12.2 & -24.4 & 82 & 0.972\\ 
203396402 & 16 08 27.21 & -26 16 49.1 & 15.82 & 11.68 & -24.62$\pm$2.09 & -31.96$\pm$2.09 & 5.4$\pm$1.0$^{(1)}$ & -13.2 & -24.1 & 29 & 0.533\\ 
203396930 & 16 17 01.74 & -26 16 42.6 & 12.87 & 9.31 & -2.31$\pm$2.29 & -15.0$\pm$2.29 & 7.2$\pm$1.3$^{(1)}$ & -12.6 & -24.2 & 28 &  \\ 
203414491 & 16 16 30.24 & -26 13 05.8 & 12.17 & 8.53 & -14.55$\pm$2.29 & -12.01$\pm$2.29 & 10.0$\pm$1.8$^{(1)}$ & -12.7 & -24.2 & 36 & 11.275\\ 
203417323 & 16 25 16.99 & -26 12 29.8 & 15.54 & 11.41 & -12.86$\pm$2.05 & -24.23$\pm$2.05 & 4.8$\pm$0.9$^{(1)}$ & -12.1 & -24.4 & 71 & 3.434\\ 
203422687 & 16 14 23.44 & -26 11 25.8 & 11.15 & 8.19 & -13.06$\pm$2.29 & -8.68$\pm$2.29 & 9.1$\pm$1.7$^{(1)}$ & -12.8 & -24.2 & 11 &  \\ 
203425996 & 16 21 14.31 & -26 10 46.2 & 15.53 & 11.02 & -16.26$\pm$2.07 & -21.74$\pm$2.07 & 7.4$\pm$1.4$^{(1)}$ & -12.3 & -24.3 & 93 & 5.213\\ 
203429083 & 15 57 03.51 & -26 10 08.1 &   & 12.9 & -10.0$\pm$3.9 & -40.0$\pm$3.9 & 17.8$\pm$3.3$^{(4)}$ & -14.0 & -23.8 & 19 &  \\ 
203430881 & 15 58 51.61 & -26 09 47.3 & 10.66 & 9.19 & -16.54$\pm$1.54 & -29.21$\pm$0.34 & 6.4$\pm$0.4$^{(0)}$ & -13.9 & -23.8 & 94 &  \\ 
203432858 & 16 11 06.92 & -26 09 23.6 & 9.95 & 8.43 & -11.51$\pm$0.85 & -19.35$\pm$0.51 & 6.1$\pm$0.2$^{(0)}$ & -13.0 & -24.1 & 95 &  \\ 
203437558 & 16 16 22.73 & -26 08 27.1 & 12.63 & 9.5 & -1.87$\pm$2.29 & -27.72$\pm$2.29 & 5.3$\pm$1.0$^{(1)}$ & -12.7 & -24.2 & 47 &  \\ 
203437673 & 15 56 43.99 & -26 08 25.9 & 13.75 & 9.98 & -7.45$\pm$2.55 & -23.35$\pm$2.55 & 5.9$\pm$1.1$^{(1)}$ & -14.0 & -23.8 & 86 & 31.937\\ 
203452629 & 16 17 23.26 & -26 05 25.0 & 15.21 & 10.81 & -13.51$\pm$2.09 & -26.12$\pm$2.09 & 6.8$\pm$1.3$^{(1)}$ & -12.6 & -24.2 & 96 & 3.762\\ 
203456118 & 16 08 20.58 & -26 04 42.5 & 12.95 & 9.76 & -15.01$\pm$2.41 & -39.55$\pm$2.41 & 4.9$\pm$0.9$^{(1)}$ & -13.2 & -24.0 & 11 &  \\ 
203457426 & 15 55 54.89 & -26 04 26.3 & 12.64 & 9.55 & -15.64$\pm$2.29 & -23.14$\pm$2.29 & 4.8$\pm$0.9$^{(1)}$ & -14.1 & -23.7 & 72 & 1.523\\ 
203461369 & 16 13 56.41 & -26 03 38.7 & 13.64 & 9.38 & -1.89$\pm$2.29 & -29.91$\pm$2.29 & 15.4$\pm$2.8$^{(1)}$ & -12.8 & -24.2 & 25 & 3.934\\ 
203465909 & 16 27 49.04 & -26 02 43.8 & 13.77 & 9.18 & -11.18$\pm$2.26 & -29.82$\pm$2.26 & 11.3$\pm$2.1$^{(1)}$ & -11.9 & -24.5 & 91 & 3.81\\ 
203465939 & 16 17 24.55 & -26 02 43.4 & 15.54 & 11.24 & -8.5$\pm$2.09 & -15.94$\pm$2.09 & 4.5$\pm$0.8$^{(1)}$ & -12.6 & -24.2 & 17 & 17.045\\ 
203478236 & 16 20 40.41 & -26 00 18.1 & 15.92 & 11.51 & -13.92$\pm$2.13 & -19.33$\pm$2.13 & 5.8$\pm$1.1$^{(1)}$ & -12.4 & -24.3 & 87 & 1.736\\ 
203478347 & 16 26 56.48 & -26 00 16.9 & 16.61 & 12.01 & -10.34$\pm$2.5 & -15.68$\pm$2.51 & 5.0$\pm$0.9$^{(1)}$ & -11.9 & -24.4 & 45 & 2.881\\ 
203479994 & 16 16 45.10 & -25 59 57.7 & 11.94 & 8.56 & -12.05$\pm$2.29 & -24.29$\pm$2.29 & 9.6$\pm$1.8$^{(1)}$ & -12.6 & -24.2 & 95 & 0.777\\ 
203484647 & 16 23 59.24 & -25 59 01.8 & 14.32 & 10.79 & -18.71$\pm$2.05 & -31.86$\pm$2.05 & 4.6$\pm$0.8$^{(1)}$ & -12.1 & -24.4 & 19 & 3.733\\ 
203494280 & 16 17 31.71 & -25 57 04.4 & 14.43 & 10.53 & -9.31$\pm$2.09 & -15.85$\pm$2.09 & 5.3$\pm$1.0$^{(1)}$ & -12.6 & -24.2 & 54 &  \\ 
203495721 & 16 21 47.93 & -25 56 47.2 & 9.15 & 8.03 & -6.65$\pm$0.85 & -23.91$\pm$0.58 & 7.8$\pm$0.3$^{(0)}$ & -12.3 & -24.3 & 91 & $<$2\\ 
203495957 & 16 17 47.04 & -25 56 44.0 & 15.76 & 11.66 & -19.51$\pm$2.09 & -34.03$\pm$2.09 & 5.1$\pm$0.9$^{(1)}$ & -12.6 & -24.2 & 37 & 0.606\\ 
203498901 & 15 56 05.10 & -25 56 08.9 & 7.61 & 6.97 & -21.81$\pm$0.05 & -32.44$\pm$0.03 & 10.6$\pm$0.5$^{(0)}$ & -14.1 & -23.7 & 100 &  \\ 
203504633 & 16 28 44.54 & -25 54 58.9 &   & 11.6 & -24.6$\pm$3.9 & -32.8$\pm$3.9 & 6.2$\pm$1.1$^{(4)}$ & -11.8 & -24.5 & 61 & 0.62\\ 
203510168 & 16 17 53.56 & -25 53 51.3 &   & 11.81 & -10.6$\pm$2.3 & -28.4$\pm$2.5 & 6.8$\pm$1.2$^{(4)}$ & -12.6 & -24.2 & 95 &  \\ 
203517860 & 16 10 02.11 & -25 52 16.7 & 12.37 & 9.03 & -11.43$\pm$2.29 & -12.4$\pm$2.29 & 6.4$\pm$1.2$^{(1)}$ & -13.1 & -24.1 & 48 &  \\ 
203523532 & 16 21 47.40 & -25 51 07.8 & 12.59 & 8.31 & -9.8$\pm$2.23 & -11.24$\pm$2.23 & 13.0$\pm$2.4$^{(1)}$ & -12.3 & -24.3 & 13 &  \\ 
203527618 & 16 16 58.02 & -25 50 16.3 & 15.71 & 11.41 & -11.39$\pm$2.09 & -28.39$\pm$2.09 & 5.4$\pm$1.0$^{(1)}$ & -12.6 & -24.2 & 87 & 3.15\\ 
203528786 & 16 25 26.26 & -25 50 01.8 & 12.43 & 9.36 & -12.1$\pm$2.26 & -10.61$\pm$2.26 & 5.6$\pm$1.0$^{(1)}$ & -12.0 & -24.4 & 15 &  \\ 
203532363 & 16 14 29.67 & -25 49 18.5 & 15.32 & 11.09 & -11.1$\pm$2.09 & -28.32$\pm$2.09 & 5.5$\pm$1.0$^{(1)}$ & -12.8 & -24.2 & 89 & 1.498\\ 
203534383 & 16 14 02.99 & -25 48 53.1 & 16.32 & 11.71 & -11.62$\pm$2.52 & -27.45$\pm$2.52 & 6.9$\pm$1.3$^{(1)}$ & -12.8 & -24.1 & 95 & 0.278\\ 
203540227 & 16 21 10.28 & -25 47 41.0 & 14.82 & 10.8 & -10.89$\pm$2.07 & -20.56$\pm$2.07 & 5.2$\pm$1.0$^{(1)}$ & -12.3 & -24.3 & 81 & 3.788\\ 
203542353 & 16 21 15.24 & -25 47 14.0 & 14.62 & 10.01 & -17.2$\pm$2.07 & -26.16$\pm$2.07 & 13.9$\pm$2.6$^{(1)}$ & -12.3 & -24.3 & 83 & 1.88\\ 
203542463 & 16 18 08.69 & -25 47 12.6 & 17.46 & 12.14 & -13.68$\pm$2.52 & -25.61$\pm$2.52 & 8.5$\pm$1.6$^{(1)}$ & -12.5 & -24.2 & 96 &  \\ 
203544427 & 15 55 42.29 & -25 46 47.8 & 16.22 & 11.74 & -13.46$\pm$2.1 & -25.75$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -14.1 & -23.7 & 96 & 1.09\\ 
203547407 & 16 03 00.18 & -25 46 10.9 & 11.48 & 8.47 & -10.72$\pm$2.29 & -13.48$\pm$2.29 & 6.7$\pm$1.2$^{(1)}$ & -13.6 & -23.9 & 62 & 18.06\\ 
203551698 & 16 03 22.90 & -25 45 17.5 & 13.83 & 10.19 & -21.82$\pm$2.67 & -26.5$\pm$2.67 & 5.7$\pm$1.0$^{(1)}$ & -13.6 & -23.9 & 76 & $<$2\\ 
203551881 & 16 03 23.46 & -25 45 15.0 & 13.17 & 9.54 & -1.36$\pm$2.41 & -20.66$\pm$2.41 & 8.0$\pm$1.5$^{(1)}$ & -13.6 & -23.9 & 50 & $<$2\\ 
203554104 & 16 20 19.68 & -25 44 47.9 & 11.99 & 8.63 & -17.29$\pm$2.23 & -13.62$\pm$2.23 & 8.5$\pm$1.6$^{(1)}$ & -12.4 & -24.3 & 52 &  \\ 
203563208 & 16 17 38.95 & -25 42 55.4 & 14.95 & 10.55 & -12.61$\pm$2.09 & -25.71$\pm$2.09 & 8.9$\pm$1.6$^{(1)}$ & -12.6 & -24.2 & 96 & 0.576\\ 
203565563 & 16 17 33.99 & -25 42 25.9 & 14.27 & 10.42 & -17.43$\pm$2.09 & -16.19$\pm$2.09 & 5.8$\pm$1.1$^{(1)}$ & -12.6 & -24.2 & 63 & 10.227\\ 
203568037 & 16 16 24.39 & -25 41 54.1 & 15.05 & 10.38 & -12.2$\pm$2.09 & -25.78$\pm$2.09 & 12.2$\pm$2.3$^{(1)}$ & -12.7 & -24.2 & 91 & 1.199\\ 
203570322 & 15 56 59.71 & -25 41 25.4 & 10.1 & 7.93 & -18.24$\pm$1.02 & -31.12$\pm$1.23 & 8.0$\pm$1.5$^{(1)}$ & -14.0 & -23.7 & 95 & 8.64\\ 
203574463 & 15 59 49.55 & -25 40 34.3 & 15.77 & 11.55 & -11.73$\pm$2.09 & -24.22$\pm$2.09 & 5.0$\pm$0.9$^{(1)}$ & -13.8 & -23.8 & 82 & 1.009\\ 
203576244 & 16 15 06.55 & -25 40 12.2 & 11.9 & 9.28 & -19.5$\pm$2.29 & -31.73$\pm$2.29 & 4.6$\pm$0.8$^{(1)}$ & -12.7 & -24.2 & 19 & 2.913\\ 
203581504 & 16 09 26.96 & -25 39 08.2 & 15.93 & 11.7 & -14.64$\pm$2.09 & -27.3$\pm$2.09 & 5.4$\pm$1.0$^{(1)}$ & -13.1 & -24.0 & 87 & 0.592\\ 
203582679 & 15 56 59.29 & -25 38 53.5 & 13.14 & 9.53 & -28.75$\pm$2.97 & -33.31$\pm$2.97 & 8.0$\pm$1.5$^{(1)}$ & -14.0 & -23.7 & 58 & $<$2\\ 
203583386 & 16 20 15.04 & -25 38 44.4 & 8.91 & 7.67 & -10.47$\pm$0.71 & -20.96$\pm$0.49 & 6.5$\pm$0.2$^{(0)}$ & -12.4 & -24.3 & 97 & $<$2\\ 
203587408 & 16 16 42.98 & -25 37 54.8 & 14.12 & 10.05 & -9.99$\pm$2.09 & -26.27$\pm$2.09 & 7.0$\pm$1.3$^{(1)}$ & -12.6 & -24.2 & 96 & 3.139\\ 
203597399 & 16 56 02.92 & -25 35 50.4 & 11.69 & 7.93 & -10.28$\pm$2.25 & -14.34$\pm$2.25 & 11.0$\pm$2.0$^{(1)}$ & -9.9 & -24.9 & 47 &  \\ 
203604427 & 16 29 08.74 & -25 34 24.0 & 13.99 & 10.13 & -13.29$\pm$2.1 & -25.0$\pm$2.08 & 7.8$\pm$1.4$^{(1)}$ & -11.8 & -24.4 & 96 & \\ 
203625455 & 16 21 14.93 & -25 30 01.0 & 15.88 & 11.35 & -15.37$\pm$2.72 & -26.3$\pm$2.72 & 7.5$\pm$1.4$^{(1)}$ & -12.3 & -24.3 & 95 &  \\ 
203627083 & 16 16 48.74 & -25 29 40.2 &   & 11.5 & -14.0$\pm$4.0 & -31.8$\pm$4.0 & 34.4$\pm$6.3$^{(4)}$ & -12.6 & -24.2 & 30 & 1.238\\ 
203629401 & 16 02 24.40 & -25 29 12.1 & 16.78 & 12.47 & -9.59$\pm$2.51 & -22.78$\pm$2.51 & 4.2$\pm$0.8$^{(1)}$ & -13.6 & -23.9 & 23 & 0.495\\ 
203636498 & 16 21 05.10 & -25 27 42.4 & 15.22 & 10.94 & -14.83$\pm$3.27 & -26.54$\pm$3.27 & 7.9$\pm$1.5$^{(1)}$ & -12.3 & -24.3 & 95 &  \\ 
203642025 & 16 30 44.70 & -25 26 33.8 & 14.75 & 10.8 & -17.56$\pm$2.06 & -27.33$\pm$2.06 & 5.7$\pm$1.1$^{(1)}$ & -11.7 & -24.5 & 84 & 1.35\\ 
203642292 & 15 56 18.19 & -25 26 30.5 & 9.15 & 8.14 & -18.38$\pm$0.85 & -20.33$\pm$0.49 & 6.2$\pm$0.3$^{(0)}$ & -14.0 & -23.7 & 92 & 0.546\\ 
203645396 & 16 11 42.62 & -25 25 51.2 &   & 11.26 & -10.1$\pm$5.1 & -35.0$\pm$5.1 & 24.9$\pm$4.6$^{(4)}$ & -13.0 & -24.1 & 23 & 0.493\\ 
203647063 & 16 11 58.00 & -25 25 30.1 & 9.34 & 7.79 & -5.45$\pm$0.9 & -21.02$\pm$0.86 & 5.4$\pm$0.7$^{(0)}$ & -13.0 & -24.1 & 68 &$<$2\\ 
203649493 & 16 11 08.62 & -25 24 59.8 & 9.38 & 8.26 & -12.27$\pm$0.49 & -19.07$\pm$0.53 & 4.3$\pm$0.8$^{(1)}$ & -13.0 & -24.0 & 30 & \\ 
203663613 & 16 24 54.63 & -25 22 02.5 & 13.73 & 10.14 & -2.84$\pm$2.05 & -28.69$\pm$2.05 & 5.2$\pm$0.9$^{(1)}$ & -12.1 & -24.3 & 50 &  \\ 
203672170 & 16 17 13.50 & -25 20 15.1 & 11.48 & 8.42 & -17.13$\pm$2.29 & -22.26$\pm$2.29 & 8.7$\pm$1.6$^{(1)}$ & -12.6 & -24.2 & 93 &  \\ 
203674308 & 16 15 53.98 & -25 19 49.1 & 14.79 & 10.82 & -13.57$\pm$2.09 & -25.84$\pm$2.09 & 4.8$\pm$0.9$^{(1)}$ & -12.7 & -24.1 & 73 & 3.521\\ 
203679238 & 16 10 13.50 & -25 18 47.4 & 10.31 & 8.82 & -20.01$\pm$1.25 & -22.08$\pm$0.74 & 6.9$\pm$0.4$^{(0)}$ & -13.1 & -24.0 & 93 &  \\ 
203679848 & 16 16 41.37 & -25 18 39.4 & 15.56 & 11.04 & -13.01$\pm$2.09 & -25.11$\pm$2.09 & 8.0$\pm$1.5$^{(1)}$ & -12.6 & -24.2 & 96 & $<$2\\ 
203685514 & 16 16 20.74 & -25 17 30.1 & 15.36 & 11.19 & -12.72$\pm$2.1 & -21.69$\pm$2.09 & 4.9$\pm$0.9$^{(1)}$ & -12.6 & -24.2 & 73 & 1.267\\ 
203690974 & 16 12 56.48 & -25 16 21.6 & 11.8 & 9.25 & -6.58$\pm$1.03 & -17.44$\pm$1.03 & 4.7$\pm$0.9$^{(1)}$ & -12.9 & -24.1 & 30 & 1.287\\ 
203692610 & 16 10 31.63 & -25 16 01.7 & 15.57 & 11.6 & -10.26$\pm$2.09 & -25.8$\pm$2.09 & 3.9$\pm$0.7$^{(1)}$ & -13.0 & -24.0 & 10 & 1.824\\ 
203696274 & 16 17 26.58 & -25 15 16.2 & 14.84 & 10.38 & -8.99$\pm$2.09 & -24.4$\pm$2.09 & 8.7$\pm$1.6$^{(1)}$ & -12.6 & -24.2 & 95 & 0.747\\ 
203696502 & 15 57 15.57 & -25 15 13.3 & 8.38 & 7.57 & -6.54$\pm$0.36 & -15.48$\pm$0.48 & 7.8$\pm$0.8$^{(0)}$ & -14.0 & -23.7 & 58 &  \\ 
203703448 & 16 54 39.84 & -25 13 47.0 & 9.66 & 8.45 & -6.44$\pm$0.14 & -8.85$\pm$0.08 & 5.8$\pm$0.3$^{(0)}$ & -10.0 & -24.9 & 11 &  \\ 
203703588 & 16 16 44.25 & -25 13 45.3 & 8.74 & 7.72 & -11.55$\pm$0.56 & -21.4$\pm$0.51 & 7.0$\pm$0.3$^{(0)}$ & -12.6 & -24.2 & 97 & $<$2\\ 
203708909 & 16 02 06.83 & -25 12 38.5 & 16.0 & 11.87 & -9.63$\pm$2.09 & -30.67$\pm$2.09 & 4.4$\pm$0.8$^{(1)}$ & -13.6 & -23.8 & 25 & 1.128\\ 
203712588 & 16 25 15.22 & -25 11 54.1 &   & 9.64 & -17.7$\pm$5.5 & -32.5$\pm$5.5 & 86.1$\pm$15.9$^{(4)}$ & -12.0 & -24.3 & 45 & 3.307\\ 
203715134 & 15 55 54.20 & -25 11 21.7 & 11.98 & 9.16 & -22.24$\pm$2.29 & -24.44$\pm$2.29 & 5.3$\pm$1.0$^{(1)}$ & -14.1 & -23.7 & 66 & 8.586\\ 
203716389 & 16 25 17.28 & -25 11 05.8 & 14.65 & 9.91 & -13.44$\pm$2.25 & -32.06$\pm$2.25 & 8.2$\pm$1.5$^{(1)}$ & -12.0 & -24.3 & 94 & 2.388\\ 
203717757 & 16 25 18.29 & -25 10 48.8 & 13.94 & 10.3 & -9.3$\pm$2.05 & -16.29$\pm$2.05 & 4.6$\pm$0.8$^{(1)}$ & -12.0 & -24.3 & 27 & \\ 
203720901 & 16 15 21.87 & -25 10 08.4 & 11.92 & 9.09 & -16.55$\pm$2.29 & -15.29$\pm$2.29 & 5.6$\pm$1.0$^{(1)}$ & -12.7 & -24.1 & 56 &  \\ 
203725441 & 16 25 04.49 & -25 09 11.6 & 11.43 & 8.08 & -13.73$\pm$2.25 & -23.66$\pm$2.25 & 12.4$\pm$2.3$^{(1)}$ & -12.0 & -24.3 & 89 & 1.769\\ 
203726701 & 16 14 39.18 & -25 08 56.2 & 16.22 & 12.0 & -11.81$\pm$2.09 & -26.71$\pm$2.09 & 4.2$\pm$0.8$^{(1)}$ & -12.8 & -24.1 & 26 & 1.687\\ 
203731383 & 16 16 05.15 & -25 07 56.3 & 14.59 & 10.76 & -13.88$\pm$2.09 & -24.67$\pm$2.09 & 4.6$\pm$0.8$^{(1)}$ & -12.7 & -24.1 & 60 & 7.658\\ 
203737395 & 16 23 58.45 & -25 06 41.2 & 10.98 & 6.64 & -10.56$\pm$2.23 & -15.64$\pm$2.23 & 31.8$\pm$5.9$^{(1)}$ & -12.1 & -24.3 & 12 & 13.162\\ 
203747290 & 16 16 31.02 & -25 04 34.5 & 19.5 & 11.24 & -12.5$\pm$4.0 & -21.0$\pm$4.0 & 5.7$\pm$1.0$^{(1)}$ & -12.6 & -24.1 & 86 & 0.578\\ 
203750883 & 16 13 36.51 & -25 03 47.4 & 14.22 & 10.26 & -9.76$\pm$2.09 & -25.76$\pm$2.09 & 6.0$\pm$1.1$^{(1)}$ & -12.8 & -24.1 & 93 & 41.661\\ 
203753432 & 16 07 48.62 & -25 03 14.2 & 15.35 & 11.43 & -11.03$\pm$2.09 & -22.6$\pm$2.09 & 4.6$\pm$0.8$^{(1)}$ & -13.2 & -23.9 & 57 & 1.175\\ 
203758182 & 16 15 09.24 & -25 02 12.5 & 11.57 & 8.24 & -10.89$\pm$2.29 & -23.47$\pm$2.29 & 9.7$\pm$1.8$^{(1)}$ & -12.7 & -24.1 & 94 & 22.09\\ 
203759474 & 16 04 40.51 & -25 01 56.1 & 10.36 & 8.88 & -17.46$\pm$1.79 & -35.86$\pm$0.49 & 10.8$\pm$0.7$^{(0)}$ & -13.4 & -23.9 & 49 & \\ 
203759570 & 16 11 18.47 & -25 01 54.8 & 15.32 & 11.32 & -12.4$\pm$2.13 & -29.82$\pm$2.13 & 4.8$\pm$0.9$^{(1)}$ & -13.0 & -24.0 & 66 & 1.811\\ 
203763434 & 16 13 49.45 & -25 01 05.3 & 12.69 & 8.7 & -6.6$\pm$2.29 & -11.27$\pm$2.29 & 10.7$\pm$2.0$^{(1)}$ & -12.8 & -24.1 & 15 &  \\ 
203764478 & 16 02 51.95 & -25 00 51.5 & 7.13 & 6.59 & -23.84$\pm$0.06 & -23.85$\pm$0.04 & 6.9$\pm$0.7$^{(0)}$ & -13.6 & -23.8 & 82 &  \\ 
203764842 & 16 02 51.88 & -25 00 47.1 & 9.34 & 7.33 & -23.84$\pm$0.06 & -23.85$\pm$0.04 & 6.9$\pm$0.7$^{(0)}$ & -13.6 & -23.8 & 82 &  \\ 
203766590 & 16 00 32.42 & -25 00 24.6 & 14.51 & 10.79 & -22.21$\pm$2.09 & -37.23$\pm$2.09 & 5.1$\pm$0.9$^{(1)}$ & -13.7 & -23.8 & 11 & 0.942\\ 
203770078 & 16 24 49.42 & -24 59 38.9 &   & 11.03 & -8.2$\pm$4.0 & -21.1$\pm$4.0 & 51.3$\pm$9.4$^{(4)}$ & -12.0 & -24.3 & 26 & 1.899\\ 
203778209 & 16 26 04.35 & -24 57 51.8 & 11.76 & 8.3 & -7.43$\pm$2.26 & -28.18$\pm$2.26 & 10.8$\pm$2.0$^{(1)}$ & -12.0 & -24.3 & 90 & 0.712\\ 
203781238 & 16 28 11.01 & -24 57 12.9 & 14.0 & 9.67 & -5.75$\pm$2.25 & -23.04$\pm$2.25 & 9.3$\pm$1.7$^{(1)}$ & -11.8 & -24.4 & 89 & 4.808\\ 
203785951 & 16 11 19.91 & -24 56 10.8 & 10.56 & 7.39 & -24.94$\pm$0.99 & -21.2$\pm$0.98 & 12.6$\pm$2.3$^{(1)}$ & -13.0 & -24.0 & 35 &  \\ 
203786209 & 16 25 14.71 & -24 56 07.1 & 12.98 & 8.27 & -9.49$\pm$2.25 & -26.45$\pm$2.25 & 24.1$\pm$4.4$^{(1)}$ & -12.0 & -24.3 & 50 & 1.439\\ 
203786655 & 16 54 34.05 & -24 56 01.3 & 12.94 & 9.47 & -5.97$\pm$2.25 & -12.59$\pm$2.25 & 6.3$\pm$1.2$^{(1)}$ & -10.0 & -24.9 & 31 &  \\ 
203788453 & 16 17 37.23 & -24 55 36.4 & 14.17 & 10.42 & -12.26$\pm$2.09 & -21.08$\pm$2.09 & 4.7$\pm$0.9$^{(1)}$ & -12.5 & -24.2 & 60 & 4.999\\ 
203789325 & 16 17 47.68 & -24 55 25.1 & 16.26 & 11.74 & -7.75$\pm$2.52 & -20.76$\pm$2.52 & 5.6$\pm$1.0$^{(1)}$ & -12.5 & -24.2 & 83 &  \\ 
203789507 & 15 57 04.90 & -24 55 22.7 & 17.24 & 12.56 & -14.96$\pm$2.11 & -21.4$\pm$2.11 & 5.2$\pm$1.0$^{(1)}$ & -14.0 & -23.7 & 84 &  \\ 
203789628 & 16 17 46.96 & -24 55 21.1 & 14.94 & 10.47 & -11.34$\pm$2.09 & -22.92$\pm$2.09 & 9.1$\pm$1.7$^{(1)}$ & -12.5 & -24.2 & 95 & 2.02\\ 
203794605 & 16 30 23.41 & -24 54 16.1 & 14.51 & 9.29 & -9.84$\pm$2.26 & -22.94$\pm$2.26 & 17.7$\pm$3.3$^{(1)}$ & -11.7 & -24.4 & 68 & 4.497\\ 
203797224 & 16 27 22.92 & -24 53 41.3 & 13.75 & 10.26 & -20.76$\pm$2.08 & -26.48$\pm$2.07 & 4.8$\pm$0.9$^{(1)}$ & -11.9 & -24.4 & 30 &  \\ 
203799870 & 16 25 29.83 & -24 53 07.5 & 15.29 & 11.08 & -7.25$\pm$2.06 & -24.52$\pm$2.06 & 4.4$\pm$0.8$^{(1)}$ & -12.0 & -24.3 & 40 & \\ 
203800211 & 15 57 36.84 & -24 53 02.9 & 15.97 & 11.93 & -17.53$\pm$2.11 & -29.93$\pm$2.11 & 4.2$\pm$0.8$^{(1)}$ & -13.9 & -23.7 & 15 & 0.614\\ 
203801071 & 16 00 48.11 & -24 52 51.6 & 11.95 & 9.11 & -24.39$\pm$2.29 & -19.2$\pm$2.29 & 5.0$\pm$0.9$^{(1)}$ & -13.7 & -23.8 & 19 &  \\ 
203807479 & 16 16 14.88 & -24 51 27.9 & 11.61 & 8.62 & -8.31$\pm$1.03 & -28.22$\pm$1.02 & 7.4$\pm$1.4$^{(1)}$ & -12.6 & -24.1 & 95 & \\ 
203810064 & 16 22 55.45 & -24 50 53.3 & 13.07 & 9.59 & -14.57$\pm$2.23 & -40.22$\pm$2.23 & 7.3$\pm$1.3$^{(1)}$ & -12.2 & -24.3 & 68 &  \\ 
203810851 & 15 57 54.44 & -24 50 42.4 & 11.65 & 8.58 & -13.95$\pm$2.29 & -22.84$\pm$2.29 & 7.5$\pm$1.4$^{(1)}$ & -13.9 & -23.7 & 96 & 4.265\\ 
203811459 & 16 00 44.62 & -24 50 34.1 & 16.23 & 11.74 & -10.57$\pm$2.52 & -21.05$\pm$2.51 & 6.6$\pm$1.2$^{(1)}$ & -13.7 & -23.8 & 93 & 1.483\\ 
203812776 & 15 58 13.66 & -24 50 16.7 & 14.83 & 10.04 & -13.76$\pm$2.11 & -22.37$\pm$2.11 & 21.3$\pm$3.9$^{(1)}$ & -13.9 & -23.7 & 58 & \\ 
203816510 & 16 15 27.22 & -24 49 27.2 & 15.98 & 11.51 & -9.89$\pm$2.09 & -24.41$\pm$2.09 & 5.7$\pm$1.1$^{(1)}$ & -12.7 & -24.1 & 92 & 1.819\\ 
203819777 & 16 16 48.44 & -24 48 43.9 &   & 9.68 & -24.3$\pm$2.9 & -17.7$\pm$1.4 & 5.5$\pm$1.0$^{(2)}$ & -12.6 & -24.1 & 20 &  \\ 
203820892 & 16 25 51.04 & -24 48 28.4 & 16.15 & 11.57 & -10.77$\pm$2.06 & -15.49$\pm$2.06 & 4.5$\pm$0.8$^{(1)}$ & -12.0 & -24.3 & 19 &  \\ 
203823381 & 16 28 32.89 & -24 47 54.9 & 15.61 & 10.66 & -5.65$\pm$2.07 & -19.81$\pm$2.07 & 9.8$\pm$1.8$^{(1)}$ & -11.8 & -24.4 & 81 &  \\ 
203826403 & 16 26 44.42 & -24 47 13.8 &   & 10.64 & -9.8$\pm$3.9 & -24.4$\pm$3.9 & 53.9$\pm$9.9$^{(4)}$ & -11.9 & -24.3 & 38 & 3.969\\ 
203832317 & 16 21 10.22 & -24 45 53.3 & 14.44 & 10.8 & -10.04$\pm$2.07 & -21.68$\pm$2.07 & 4.1$\pm$0.8$^{(1)}$ & -12.3 & -24.2 & 19 & \\ 
203840935 & 16 28 58.37 & -24 43 54.9 & 16.63 & 11.31 & -6.35$\pm$2.08 & -10.91$\pm$2.08 & 8.0$\pm$1.5$^{(1)}$ & -11.8 & -24.4 & 18 &  \\ 
203842272 & 16 01 35.29 & -24 43 36.6 & 14.35 & 10.59 & -14.62$\pm$2.14 & -32.25$\pm$2.14 & 5.5$\pm$1.0$^{(1)}$ & -13.6 & -23.8 & 81 & 6.927\\ 
203844446 & 16 08 06.11 & -24 43 06.0 & 19.87 & 11.53 & -4.8$\pm$4.0 & -21.1$\pm$4.0 & 4.8$\pm$0.9$^{(1)}$ & -13.2 & -23.9 & 38 & 0.841\\ 
203844508 & 16 16 56.04 & -24 43 05.0 & 15.89 & 11.37 & -15.79$\pm$2.09 & -23.19$\pm$2.09 & 6.2$\pm$1.1$^{(1)}$ & -12.6 & -24.1 & 93 & 2.141\\ 
203846183 & 16 02 57.44 & -24 42 41.7 & 15.45 & 11.4 & -12.64$\pm$2.09 & -22.86$\pm$2.09 & 5.0$\pm$0.9$^{(1)}$ & -13.5 & -23.8 & 81 & 1.574\\ 
203848625 & 16 20 28.64 & -24 42 08.8 & 14.0 & 9.69 & -7.34$\pm$2.23 & -21.85$\pm$2.23 & 8.6$\pm$1.6$^{(1)}$ & -12.3 & -24.2 & 91 & 8.025\\ 
203850795 & 16 25 17.33 & -24 41 36.9 & 16.04 & 10.7 & -6.95$\pm$2.05 & -10.96$\pm$2.06 & 9.8$\pm$1.8$^{(1)}$ & -12.0 & -24.3 & 15 &  \\ 
203853503 & 15 55 45.33 & -24 40 57.3 & 9.21 & 7.94 & -20.06$\pm$0.1 & -34.65$\pm$0.05 & 9.3$\pm$0.3$^{(0)}$ & -14.0 & -23.6 & 85 & 1.955\\ 
203856109 & 16 09 51.98 & -24 40 19.7 & 16.69 & 12.13 & -14.94$\pm$2.51 & -22.9$\pm$2.51 & 5.5$\pm$1.0$^{(1)}$ & -13.1 & -24.0 & 88 & $<$2\\ 
203857254 & 16 25 22.49 & -24 40 03.9 & 16.56 & 11.76 & -8.55$\pm$2.06 & -14.49$\pm$2.06 & 4.5$\pm$0.8$^{(1)}$ & -12.0 & -24.3 & 11 & \\ 
203859264 & 16 49 34.70 & -24 39 34.6 & 8.54 & 7.43 & -1.0$\pm$0.91 & -28.37$\pm$0.59 & 8.0$\pm$0.7$^{(0)}$ & -10.4 & -24.8 & 83 &  \\ 
203860131 & 16 07 36.51 & -24 39 22.2 & 13.3 & 10.0 & -19.44$\pm$2.09 & -24.42$\pm$2.09 & 4.7$\pm$0.9$^{(1)}$ & -13.2 & -23.9 & 49 & 5.943\\ 
203866877 & 15 55 43.14 & -24 37 43.5 & 16.81 & 12.17 & -26.82$\pm$2.1 & -33.99$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -14.0 & -23.6 & 45 & 1.411\\ 
203868400 & 16 04 29.22 & -24 37 21.3 & 10.87 & 9.39 & -11.4$\pm$1.57 & -9.64$\pm$0.87 & 5.8$\pm$0.3$^{(0)}$ & -13.4 & -23.8 & 18 &  \\ 
203868608 & 16 17 18.99 & -24 37 18.7 & 15.38 & 10.76 & -7.76$\pm$2.09 & -20.08$\pm$2.09 & 9.9$\pm$1.8$^{(1)}$ & -12.5 & -24.1 & 86 & 5.66\\ 
203869829 & 16 20 38.48 & -24 37 01.6 & 13.66 & 9.6 & -4.9$\pm$2.24 & -17.92$\pm$2.23 & 9.3$\pm$1.7$^{(1)}$ & -12.3 & -24.2 & 69 &  \\ 
203876897 & 16 15 08.08 & -24 35 18.5 & 8.29 & 7.06 & -9.86$\pm$0.4 & -22.28$\pm$0.44 & 6.8$\pm$0.4$^{(0)}$ & -12.7 & -24.1 & 98 &  \\ 
203890834 & 15 56 03.73 & -24 31 54.5 &   & 11.34 & -7.4$\pm$3.9 & -20.1$\pm$3.9 & 19.9$\pm$3.7$^{(4)}$ & -14.0 & -23.6 & 37 & 0.616\\ 
203891877 & 16 28 13.71 & -24 31 39.1 &   & 13.82 & -8.2$\pm$5.0 & -24.0$\pm$5.0 & 17.4$\pm$3.2$^{(4)}$ & -11.8 & -24.3 & 58 &  \\ 
203891886 & 16 25 49.05 & -24 31 39.1 & 19.29 & 9.49 & -17.51$\pm$3.27 & -32.51$\pm$3.26 & 6.2$\pm$1.1$^{(1)}$ & -12.0 & -24.3 & 87 &  \\ 
203892828 & 15 55 53.21 & -24 31 25.2 & 15.97 & 11.86 & -11.95$\pm$2.1 & -19.69$\pm$2.1 & 4.7$\pm$0.9$^{(1)}$ & -14.0 & -23.6 & 57 & 0.555\\ 
203899018 & 16 24 43.42 & -24 29 55.5 & 15.58 & 10.5 & -12.77$\pm$2.05 & -37.26$\pm$2.05 & 9.2$\pm$1.7$^{(1)}$ & -12.0 & -24.3 & 84 &  \\ 
203904213 & 16 27 55.25 & -24 28 39.6 &   & 10.79 & -16.1$\pm$5.3 & -19.5$\pm$5.3 & 91.0$\pm$16.8$^{(4)}$ & -11.8 & -24.3 & 44 &  \\ 
203910995 & 16 17 32.24 & -24 26 59.8 & 14.81 & 10.49 & -5.93$\pm$2.09 & -30.6$\pm$2.09 & 8.4$\pm$1.5$^{(1)}$ & -12.5 & -24.1 & 89 & 1.47\\ 
203915140 & 16 07 21.60 & -24 25 58.5 & 11.26 & 8.88 & -5.66$\pm$0.98 & -14.88$\pm$0.98 & 5.0$\pm$0.9$^{(1)}$ & -13.2 & -23.9 & 17 & 3.412\\ 
203919192 & 16 23 21.83 & -24 24 58.0 & 12.01 & 8.76 & -14.78$\pm$1.17 & -23.55$\pm$1.18 & 7.9$\pm$1.5$^{(1)}$ & -12.1 & -24.2 & 96 & 1.37\\ 
203920102 & 16 04 14.74 & -24 24 43.4 & 15.85 & 11.68 & -11.38$\pm$2.09 & -26.46$\pm$2.09 & 5.3$\pm$1.0$^{(1)}$ & -13.4 & -23.8 & 86 & 1.606\\ 
203920801 & 15 57 38.80 & -24 24 33.0 & 9.67 & 8.21 & -16.99$\pm$1.06 & -26.43$\pm$0.35 & 6.8$\pm$0.3$^{(0)}$ & -13.9 & -23.7 & 98 & 0.466\\ 
203925874 & 16 17 34.56 & -24 23 16.1 & 15.8 & 11.57 & -11.75$\pm$2.09 & -26.85$\pm$2.09 & 4.7$\pm$0.9$^{(1)}$ & -12.5 & -24.1 & 64 & 6.643\\ 
203926358 & 16 21 07.88 & -24 23 08.7 & 12.64 & 9.05 & -17.21$\pm$2.23 & -11.44$\pm$2.23 & 9.6$\pm$1.8$^{(1)}$ & -12.3 & -24.2 & 25 &  \\ 
203939508 & 16 22 12.00 & -24 19 49.3 & 13.1 & 9.79 & -5.17$\pm$2.26 & -13.33$\pm$2.24 & 5.3$\pm$1.0$^{(1)}$ & -12.2 & -24.2 & 17 &  \\ 
203943710 & 16 25 00.63 & -24 18 44.3 & 16.92 & 10.73 & -4.49$\pm$2.46 & -27.64$\pm$2.46 & 13.8$\pm$2.5$^{(1)}$ & -12.0 & -24.3 & 66 &  \\ 
203945512 & 16 27 13.73 & -24 18 16.9 &   & 9.29 & -29.0$\pm$6.7 & -40.7$\pm$6.7 & 196.5$\pm$36.2$^{(4)}$ & -11.9 & -24.3 & 26 &  \\ 
203947055 & 16 25 31.98 & -24 17 52.4 & 17.17 & 11.27 & -7.71$\pm$2.63 & -22.52$\pm$2.74 & 11.0$\pm$2.0$^{(1)}$ & -12.0 & -24.3 & 88 & \\ 
203950167 & 16 23 09.23 & -24 17 05.2 & 14.02 & 8.07 & -8.07$\pm$2.23 & -25.02$\pm$2.23 & 24.7$\pm$4.5$^{(1)}$ & -12.1 & -24.2 & 42 & 7.474\\ 
203951969 & 16 47 28.54 & -24 16 36.9 & 13.26 & 9.96 & -8.92$\pm$2.21 & -26.24$\pm$2.21 & 5.1$\pm$0.9$^{(1)}$ & -10.5 & -24.7 & 81 & 9.754\\ 
203954277 & 16 28 10.21 & -24 16 01.2 & 12.29 & 7.97 & -14.94$\pm$2.25 & -23.35$\pm$2.25 & 22.6$\pm$4.2$^{(1)}$ & -11.8 & -24.3 & 51 & \\ 
204001352 & 16 49 22.20 & -24 03 47.0 &   & 12.62 & -19.6$\pm$5.0 & -34.0$\pm$5.0 & 23.1$\pm$4.3$^{(4)}$ & -10.4 & -24.7 & 21 &  \\ 
204022485 & 16 47 46.53 & -23 58 27.5 & 7.7 & 6.36 & -11.17$\pm$0.05 & -19.45$\pm$0.04 & 4.7$\pm$0.6$^{(0)}$ & -10.5 & -24.7 & 45 &  \\ 
204027147 & 16 46 24.46 & -23 57 22.7 & 13.74 & 9.98 & -7.5$\pm$7.7 & -12.1$\pm$5.0 & 5.9$\pm$1.1$^{(1)}$ & -10.6 & -24.6 & 46 &  \\ 
204043388 & 15 56 09.07 & -23 53 36.1 & 8.15 & 7.29 & -23.08$\pm$0.37 & -34.13$\pm$0.42 & 9.2$\pm$0.5$^{(0)}$ & -14.0 & -23.6 & 81 & $<$2\\ 
204060981 & 16 10 56.19 & -23 49 28.9 & 13.48 & 9.47 & -11.47$\pm$2.29 & -27.32$\pm$2.29 & 10.4$\pm$1.9$^{(1)}$ & -13.0 & -23.9 & 94 & 0.4\\ 
204077926 & 15 55 30.60 & -23 45 21.3 & 16.32 & 12.12 & -15.19$\pm$2.5 & -26.19$\pm$2.5 & 4.0$\pm$0.7$^{(1)}$ & -14.0 & -23.6 & 14 & 1.002\\ 
204079630 & 16 04 19.17 & -23 44 56.3 & 9.34 & 8.19 & -18.77$\pm$1.11 & -15.4$\pm$0.62 & 6.3$\pm$0.3$^{(0)}$ & -13.4 & -23.8 & 75 &  \\ 
204083786 & 16 16 17.26 & -23 43 56.4 & 12.27 & 9.25 & -20.53$\pm$1.97 & -16.39$\pm$1.97 & 5.3$\pm$1.0$^{(1)}$ & -12.6 & -24.0 & 31 & 3.408\\ 
204087208 & 15 59 17.85 & -23 43 05.7 &   & 11.37 & -10.7$\pm$3.8 & -19.2$\pm$3.8 & 7.2$\pm$1.3$^{(4)}$ & -13.8 & -23.6 & 91 & 0.587\\ 
204093170 & 15 56 43.73 & -23 41 39.8 &   & 12.06 & -7.7$\pm$5.1 & -19.9$\pm$5.1 & 5.2$\pm$1.0$^{(4)}$ & -13.9 & -23.6 & 64 & 0.552\\ 
204099505 & 16 17 21.18 & -23 40 08.6 & 15.9 & 11.59 & -9.53$\pm$2.11 & -23.99$\pm$2.11 & 5.2$\pm$1.0$^{(1)}$ & -12.5 & -24.0 & 84 & 2.035\\ 
204104740 & 15 56 27.62 & -23 38 52.1 & 12.84 & 9.11 & -7.89$\pm$2.28 & -22.87$\pm$2.28 & 9.9$\pm$1.8$^{(1)}$ & -13.9 & -23.6 & 89 & 5.577\\ 
204108293 & 15 59 11.36 & -23 38 00.2 & 18.27 & 13.21 & -10.37$\pm$3.55 & -27.78$\pm$3.55 & 4.5$\pm$0.8$^{(1)}$ & -13.8 & -23.6 & 47 &  \\ 
204121113 & 16 09 58.63 & -23 34 55.9 & 12.1 & 8.93 & -8.53$\pm$2.29 & -23.9$\pm$2.29 & 7.0$\pm$1.3$^{(1)}$ & -13.0 & -23.9 & 94 & 1.672\\ 
204122161 & 16 03 50.41 & -23 34 41.1 & 13.14 & 9.7 & -10.8$\pm$2.29 & -21.13$\pm$2.29 & 6.0$\pm$1.1$^{(1)}$ & -13.4 & -23.7 & 92 & 1.611\\ 
204134902 & 16 27 18.96 & -23 31 38.0 & 11.81 & 8.61 & -11.39$\pm$1.59 & -28.04$\pm$1.58 & 8.4$\pm$1.5$^{(1)}$ & -11.8 & -24.2 & 96 & 2.468\\ 
204137184 & 16 02 05.18 & -23 31 06.9 & 14.82 & 10.67 & -10.68$\pm$2.09 & -23.06$\pm$2.09 & 6.4$\pm$1.2$^{(1)}$ & -13.5 & -23.7 & 94 & 2.642\\ 
204142243 & 16 22 24.96 & -23 29 55.1 & 14.75 & 9.58 & -11.34$\pm$2.33 & -34.51$\pm$2.33 & 15.9$\pm$2.9$^{(1)}$ & -12.2 & -24.1 & 61 &  \\ 
204144407 & 16 16 56.10 & -23 29 25.3 &   & 9.02 & -8.2$\pm$1.7 & -19.4$\pm$1.7 & 12.5$\pm$2.3$^{(2)}$ & -12.5 & -24.0 & 76 & 3.992\\ 
204154736 & 16 08 23.09 & -23 26 56.2 & 12.94 & 9.59 & -8.62$\pm$2.29 & -22.5$\pm$2.29 & 5.6$\pm$1.0$^{(1)}$ & -13.1 & -23.8 & 88 & 7.35\\ 
204161056 & 16 25 42.90 & -23 25 26.6 & 13.87 & 9.2 & -14.54$\pm$3.39 & -30.58$\pm$3.39 & 11.2$\pm$2.1$^{(1)}$ & -11.9 & -24.2 & 90 &  \\ 
204161083 & 16 29 29.95 & -23 25 26.3 & 12.32 & 9.3 & -11.3$\pm$1.05 & -9.96$\pm$1.05 & 6.0$\pm$1.1$^{(1)}$ & -11.7 & -24.3 & 10 &  \\ 
204167344 & 16 01 25.04 & -23 23 57.0 & 11.07 & 8.33 & -6.81$\pm$0.94 & -11.47$\pm$1.05 & 7.1$\pm$1.3$^{(1)}$ & -13.6 & -23.7 & 17 &  \\ 
204168477 & 16 19 51.87 & -23 23 40.8 &   & 10.79 & -9.9$\pm$3.9 & -25.4$\pm$3.9 & 45.1$\pm$8.3$^{(4)}$ & -12.3 & -24.1 & 33 & 0.524\\ 
204178534 & 16 02 12.80 & -23 21 20.2 & 15.83 & 11.68 & -8.14$\pm$2.09 & -24.34$\pm$2.09 & 5.1$\pm$0.9$^{(1)}$ & -13.5 & -23.7 & 76 & 1.351\\ 
204179973 & 16 36 06.05 & -23 20 59.7 & 11.56 & 7.86 & -23.72$\pm$1.1 & -24.59$\pm$1.2 & 14.6$\pm$2.7$^{(1)}$ & -11.2 & -24.4 & 28 &  \\ 
204180473 & 16 03 45.03 & -23 20 52.9 & 14.28 & 10.51 & -12.04$\pm$2.09 & -23.98$\pm$2.09 & 5.8$\pm$1.1$^{(1)}$ & -13.4 & -23.7 & 93 & 1.912\\ 
204184435 & 16 12 52.66 & -23 19 56.0 & 11.65 & 9.04 & -9.18$\pm$1.0 & -24.62$\pm$1.11 & 4.9$\pm$0.9$^{(1)}$ & -12.8 & -23.9 & 78 & 4.286\\ 
204185325 & 16 36 27.61 & -23 19 43.8 & 12.48 & 9.03 & -1.98$\pm$2.34 & -12.65$\pm$2.34 & 8.1$\pm$1.5$^{(1)}$ & -11.2 & -24.4 & 17 &  \\ 
204185983 & 16 25 52.83 & -23 19 35.0 & 12.34 & 7.87 & -8.77$\pm$2.35 & -27.31$\pm$2.35 & 19.8$\pm$3.6$^{(1)}$ & -11.9 & -24.2 & 60 &  \\ 
204187225 & 16 14 19.59 & -23 19 18.1 & 13.76 & 10.22 & -19.44$\pm$2.11 & -13.59$\pm$2.11 & 5.4$\pm$1.0$^{(1)}$ & -12.7 & -24.0 & 23 & $<$2\\ 
204187469 & 16 25 10.51 & -23 19 14.8 & 12.24 & 7.51 & -13.58$\pm$2.35 & -32.94$\pm$2.35 & 21.6$\pm$4.0$^{(1)}$ & -12.0 & -24.2 & 44 &  \\ 
204190866 & 15 59 00.73 & -23 18 26.7 & 13.94 & 10.21 & -11.64$\pm$2.13 & -9.54$\pm$2.13 & 5.9$\pm$1.1$^{(1)}$ & -13.8 & -23.6 & 16 & 4.835\\ 
204193196 & 15 57 53.86 & -23 17 53.2 & 15.36 & 11.32 & -13.04$\pm$2.11 & -26.93$\pm$2.11 & 5.1$\pm$0.9$^{(1)}$ & -13.8 & -23.6 & 81 & 15.809\\ 
204193996 & 15 57 53.97 & -23 17 41.7 & 12.56 & 9.45 & -10.51$\pm$2.29 & -18.97$\pm$2.29 & 5.2$\pm$1.0$^{(1)}$ & -13.8 & -23.6 & 76 & 15.798\\ 
204194822 & 16 26 46.20 & -23 17 30.3 & 11.93 & 8.57 & -28.2$\pm$2.89 & -30.02$\pm$2.77 & 9.5$\pm$1.7$^{(1)}$ & -11.9 & -24.2 & 47 &  \\ 
204195987 & 16 22 44.94 & -23 17 13.4 &   & 12.25 & -16.0$\pm$5.4 & -32.2$\pm$5.4 & 29.2$\pm$5.4$^{(4)}$ & -12.1 & -24.1 & 26 &  \\ 
204206295 & 16 26 47.43 & -23 14 50.9 & 12.71 & 8.62 & -8.52$\pm$2.35 & -25.14$\pm$2.35 & 11.4$\pm$2.1$^{(1)}$ & -11.9 & -24.2 & 90 &  \\ 
204206497 & 16 16 40.37 & -23 14 48.2 & 13.53 & 9.82 & -18.9$\pm$2.1 & -17.1$\pm$1.9 & 7.1$\pm$1.3$^{(1)}$ & -12.5 & -24.0 & 78 &  \\ 
204211116 & 16 21 41.99 & -23 13 43.2 & 15.98 & 10.96 & -9.61$\pm$2.15 & -30.22$\pm$2.15 & 10.7$\pm$2.0$^{(1)}$ & -12.2 & -24.1 & 91 & 1.052\\ 
204212486 & 16 10 11.64 & -23 13 24.0 & 12.68 & 9.07 & -11.82$\pm$1.22 & -26.18$\pm$1.24 & 8.4$\pm$1.5$^{(1)}$ & -13.0 & -23.9 & 96 & 25.358\\ 
204217530 & 16 11 15.96 & -23 12 14.6 & 8.86 & 7.77 & -10.93$\pm$0.75 & -23.23$\pm$0.63 & 6.4$\pm$0.3$^{(0)}$ & -12.9 & -23.9 & 98 & \\ 
204221888 & 15 56 39.21 & -23 11 12.9 & 11.89 & 9.24 & -6.89$\pm$2.24 & -14.14$\pm$2.24 & 4.7$\pm$0.9$^{(1)}$ & -13.9 & -23.5 & 14 &  \\ 
204223197 & 16 26 36.64 & -23 10 55.6 & 13.13 & 9.21 & -12.86$\pm$2.36 & -22.23$\pm$2.36 & 9.5$\pm$1.7$^{(1)}$ & -11.9 & -24.2 & 94 &  \\ 
204226647 & 16 20 51.12 & -23 10 06.4 & 10.73 & 7.22 & -3.69$\pm$1.07 & -21.02$\pm$1.14 & 17.8$\pm$3.3$^{(1)}$ & -12.3 & -24.1 & 23 & 10.134\\ 
204227785 & 15 55 02.16 & -23 09 49.9 & 14.79 & 10.75 & -10.0$\pm$5.7 & -51.7$\pm$11.3 & 6.0$\pm$1.1$^{(1)}$ & -14.0 & -23.5 & 58 & 3.497\\ 
204230299 & 16 24 36.34 & -23 09 13.8 & 12.38 & 9.58 & -22.62$\pm$2.02 & -19.19$\pm$2.66 & 5.1$\pm$0.9$^{(1)}$ & -12.0 & -24.2 & 23 &  \\ 
204230890 & 16 03 59.13 & -23 09 05.6 & 12.93 & 9.53 & -13.85$\pm$2.24 & -29.04$\pm$2.24 & 6.5$\pm$1.2$^{(1)}$ & -13.4 & -23.7 & 95 & 6.746\\ 
204231426 & 16 25 48.99 & -23 08 58.0 & 13.84 & 10.2 & -15.27$\pm$2.15 & -31.89$\pm$2.15 & 6.1$\pm$1.1$^{(1)}$ & -11.9 & -24.2 & 89 &  \\ 
204236173 & 16 22 57.92 & -23 07 50.3 & 12.33 & 8.51 & -9.76$\pm$2.36 & -31.37$\pm$2.36 & 13.1$\pm$2.4$^{(1)}$ & -12.1 & -24.1 & 82 &  \\ 
204241221 & 16 16 53.38 & -23 06 37.7 & 8.51 & 7.34 & -7.68$\pm$0.09 & -23.64$\pm$0.05 & 6.4$\pm$0.3$^{(0)}$ & -12.5 & -24.0 & 93 & \\ 
204242152 & 16 07 23.76 & -23 06 24.0 & 13.6 & 9.85 & -11.02$\pm$2.24 & -23.44$\pm$2.24 & 7.4$\pm$1.4$^{(1)}$ & -13.2 & -23.8 & 96 & 1.572\\ 
204244466 & 16 21 56.78 & -23 05 50.6 & 13.89 & 10.19 & -13.98$\pm$2.16 & -16.02$\pm$2.14 & 5.8$\pm$1.1$^{(1)}$ & -12.2 & -24.1 & 73 & \\ 
204246759 & 16 03 33.80 & -23 05 19.1 & 11.79 & 9.05 & -11.4$\pm$2.24 & -23.06$\pm$2.24 & 5.1$\pm$0.9$^{(1)}$ & -13.4 & -23.7 & 84 & 4.419\\ 
204259310 & 16 13 09.83 & -23 02 18.4 &   & 11.76 & -17.5$\pm$5.0 & -20.6$\pm$5.0 & 6.2$\pm$1.1$^{(4)}$ & -12.8 & -23.9 & 88 & 1.33\\ 
204260042 & 16 19 50.93 & -23 02 08.2 & 16.44 & 12.14 & -16.12$\pm$2.14 & -29.48$\pm$2.14 & 4.7$\pm$0.9$^{(1)}$ & -12.3 & -24.0 & 53 & 1.335\\ 
204260173 & 16 25 25.53 & -23 02 06.2 & 12.79 & 9.32 & -25.17$\pm$2.36 & -26.63$\pm$2.36 & 7.7$\pm$1.4$^{(1)}$ & -11.9 & -24.2 & 68 &  \\ 
204260890 & 16 21 33.97 & -23 01 55.9 & 12.9 & 9.23 & -4.02$\pm$2.34 & -17.56$\pm$2.33 & 8.8$\pm$1.6$^{(1)}$ & -12.2 & -24.1 & 66 &  \\ 
204262368 & 16 01 26.53 & -23 01 34.4 & 15.22 & 11.18 & -9.35$\pm$2.05 & -24.33$\pm$2.05 & 5.0$\pm$0.9$^{(1)}$ & -13.6 & -23.6 & 76 & 1.87\\ 
204265204 & 16 23 49.47 & -23 00 54.0 & 12.42 & 9.19 & -7.82$\pm$1.77 & -13.3$\pm$1.74 & 7.2$\pm$1.3$^{(1)}$ & -12.0 & -24.1 & 50 & \\ 
204268916 & 16 24 35.20 & -23 00 02.9 & 15.03 & 10.99 & -12.49$\pm$2.15 & -28.41$\pm$2.15 & 5.9$\pm$1.1$^{(1)}$ & -12.0 & -24.1 & 93 & 1.754\\ 
204269918 & 15 56 23.40 & -22 59 49.1 & 16.17 & 11.62 & -14.66$\pm$2.05 & -27.15$\pm$2.05 & 7.5$\pm$1.4$^{(1)}$ & -13.9 & -23.5 & 96 & 0.834\\ 
204271115 & 16 02 23.57 & -22 59 33.2 & 15.32 & 11.03 & -7.79$\pm$2.05 & -27.0$\pm$2.05 & 7.6$\pm$1.4$^{(1)}$ & -13.5 & -23.7 & 93 & 1.018\\ 
204276894 & 16 34 39.22 & -22 58 14.8 & 10.91 & 5.74 & -19.77$\pm$2.35 & -16.72$\pm$2.35 & 65.9$\pm$12.1$^{(1)}$ & -11.3 & -24.3 & 15 & 38.372\\ 
204287798 & 16 20 26.09 & -22 55 42.9 & 16.48 & 11.84 & -7.74$\pm$2.14 & -26.88$\pm$2.15 & 6.6$\pm$1.2$^{(1)}$ & -12.3 & -24.0 & 94 & 0.975\\ 
204289171 & 16 23 43.33 & -22 55 23.1 & 17.6 & 12.2 & -6.13$\pm$2.78 & -15.73$\pm$2.64 & 5.5$\pm$1.0$^{(1)}$ & -12.0 & -24.1 & 50 &  \\ 
204292739 & 15 55 36.25 & -22 54 31.8 & 11.16 & 8.64 & -6.06$\pm$2.49 & -11.62$\pm$2.49 & 5.9$\pm$1.1$^{(1)}$ & -14.0 & -23.5 & 20 &  \\ 
204294596 & 16 28 07.85 & -22 54 04.5 & 12.18 & 9.22 & -6.29$\pm$1.22 & -18.24$\pm$1.22 & 6.6$\pm$1.2$^{(1)}$ & -11.7 & -24.2 & 82 &  \\ 
204295293 & 16 24 12.37 & -22 53 54.7 & 14.8 & 10.8 & -14.18$\pm$2.15 & -24.28$\pm$2.15 & 5.6$\pm$1.0$^{(1)}$ & -12.0 & -24.1 & 90 & 3.992\\ 
204296148 & 16 24 51.80 & -22 53 42.8 & 16.07 & 10.99 & -12.53$\pm$2.64 & -27.41$\pm$2.64 & 13.3$\pm$2.4$^{(1)}$ & -12.0 & -24.1 & 88 & $<$2\\ 
204299578 & 16 15 15.19 & -22 52 53.8 & 16.33 & 12.01 & -7.09$\pm$2.07 & -30.68$\pm$2.07 & 5.2$\pm$1.0$^{(1)}$ & -12.6 & -23.9 & 65 & 0.771\\ 
204303682 & 16 36 36.47 & -22 51 54.6 & 11.34 & 8.02 & -14.31$\pm$1.21 & -25.75$\pm$1.04 & 11.9$\pm$2.2$^{(1)}$ & -11.2 & -24.4 & 91 &  \\ 
204309340 & 16 35 24.48 & -22 50 32.7 &   & 14.73 & -2.1$\pm$4.2 & -10.8$\pm$4.2 & 8.2$\pm$1.5$^{(4)}$ & -11.3 & -24.3 & 25 &  \\ 
204321142 & 16 22 35.30 & -22 47 43.4 &   & 10.52 & -8.6$\pm$3.9 & -28.9$\pm$3.9 & 60.5$\pm$11.2$^{(4)}$ & -12.1 & -24.1 & 28 & 0.476\\ 
204329402 & 16 29 43.26 & -22 45 44.9 & 11.35 & 7.74 & -12.34$\pm$1.02 & -20.5$\pm$1.02 & 14.0$\pm$2.6$^{(1)}$ & -11.6 & -24.2 & 80 & \\ 
204329690 & 16 22 01.95 & -22 45 41.0 &   & 10.88 & -16.3$\pm$5.0 & -29.1$\pm$5.0 & 52.3$\pm$9.6$^{(4)}$ & -12.2 & -24.1 & 27 &  \\ 
204345402 & 16 11 47.55 & -22 41 54.9 & 15.0 & 11.08 & -8.83$\pm$2.07 & -20.58$\pm$2.07 & 4.5$\pm$0.8$^{(1)}$ & -12.8 & -23.8 & 46 & 2.792\\ 
204346718 & 16 21 16.81 & -22 41 36.7 & 16.97 & 12.22 & -10.04$\pm$2.6 & -23.35$\pm$2.6 & 6.0$\pm$1.1$^{(1)}$ & -12.2 & -24.0 & 93 & 0.643\\ 
204348630 & 16 16 02.95 & -22 41 09.1 & 14.84 & 10.77 & -15.19$\pm$2.07 & -19.19$\pm$2.07 & 6.8$\pm$1.3$^{(1)}$ & -12.6 & -23.9 & 92 & $<$2\\ 
204356847 & 16 02 40.09 & -22 39 13.4 & 15.54 & 11.38 & -10.29$\pm$2.05 & -24.25$\pm$2.05 & 5.7$\pm$1.0$^{(1)}$ & -13.5 & -23.6 & 91 & 1.291\\ 
204360645 & 16 03 22.78 & -22 38 20.6 & 15.35 & 11.17 & -15.63$\pm$2.05 & -30.74$\pm$2.05 & 6.0$\pm$1.1$^{(1)}$ & -13.4 & -23.7 & 91 & $<$2\\ 
204360807 & 16 21 57.40 & -22 38 18.2 & 14.98 & 10.13 & -3.1$\pm$2.14 & -33.93$\pm$2.14 & 15.5$\pm$2.9$^{(1)}$ & -12.2 & -24.1 & 24 & 5.027\\ 
204364130 & 16 19 54.97 & -22 37 32.3 & 16.01 & 11.46 & -15.83$\pm$2.14 & -25.88$\pm$2.14 & 8.0$\pm$1.5$^{(1)}$ & -12.3 & -24.0 & 96 & 1.269\\ 
204374147 & 16 22 34.21 & -22 35 12.4 & 12.48 & 8.54 & -13.29$\pm$2.36 & -27.02$\pm$2.36 & 13.8$\pm$2.5$^{(1)}$ & -12.1 & -24.1 & 87 & 0.624\\ 
204374716 & 16 22 30.40 & -22 35 04.3 &   & 10.82 & -15.6$\pm$3.9 & -19.3$\pm$3.9 & 49.2$\pm$9.1$^{(4)}$ & -12.1 & -24.1 & 21 & 2.043\\ 
204376071 & 16 04 10.12 & -22 34 45.4 & 15.84 & 11.55 & -10.93$\pm$2.05 & -20.36$\pm$2.05 & 6.2$\pm$1.1$^{(1)}$ & -13.4 & -23.7 & 92 & 1.626\\ 
204377731 & 16 32 32.55 & -22 34 21.4 & 13.84 & 9.83 & -5.3$\pm$2.35 & -16.57$\pm$2.35 & 7.8$\pm$1.4$^{(1)}$ & -11.4 & -24.3 & 73 & 4.466\\ 
204377821 & 16 26 39.66 & -22 34 20.1 & 15.04 & 10.49 & -16.47$\pm$2.15 & -23.04$\pm$2.15 & 9.3$\pm$1.7$^{(1)}$ & -11.8 & -24.1 & 93 & 1.351\\ 
204403575 & 16 09 50.94 & -22 28 15.6 & 11.51 & 9.32 & -12.88$\pm$1.58 & -39.24$\pm$0.88 & 6.6$\pm$0.3$^{(0)}$ & -13.0 & -23.8 & 24 &  \\ 
204408707 & 16 20 22.91 & -22 27 04.1 & 14.12 & 10.18 & -12.41$\pm$2.14 & -20.33$\pm$2.14 & 7.0$\pm$1.3$^{(1)}$ & -12.3 & -24.0 & 94 & 3.293\\ 
204416606 & 16 34 28.78 & -22 25 12.7 & 11.63 & 8.08 & -10.69$\pm$2.35 & -16.53$\pm$2.35 & 12.5$\pm$2.3$^{(1)}$ & -11.3 & -24.3 & 66 & 19.063\\ 
204417649 & 16 02 25.98 & -22 24 57.5 & 15.84 & 11.64 & -9.02$\pm$2.05 & -23.54$\pm$2.05 & 5.2$\pm$1.0$^{(1)}$ & -13.5 & -23.6 & 82 & 1.435\\ 
204419255 & 16 09 58.05 & -22 24 34.9 & 7.64 & 6.88 & -10.38$\pm$0.38 & -25.84$\pm$0.39 & 6.9$\pm$0.3$^{(0)}$ & -13.0 & -23.8 & 98 &  \\ 
204422598 & 16 22 24.22 & -22 23 48.7 & 15.71 & 11.24 & -17.64$\pm$2.15 & -27.21$\pm$2.15 & 7.1$\pm$1.3$^{(1)}$ & -12.1 & -24.0 & 94 & 1.512\\ 
204426847 & 16 14 53.33 & -22 22 49.1 & 7.37 & 7.03 & -17.08$\pm$0.04 & -22.65$\pm$0.03 & 5.5$\pm$0.4$^{(0)}$ & -12.6 & -23.9 & 10 &  \\ 
204428210 & 16 24 45.15 & -22 22 29.5 & 12.22 & 9.11 & -6.58$\pm$1.05 & -13.95$\pm$1.05 & 6.2$\pm$1.1$^{(1)}$ & -12.0 & -24.1 & 42 &  \\ 
204429168 & 16 03 06.38 & -22 22 15.9 & 11.38 & 8.67 & -16.84$\pm$2.24 & -10.86$\pm$2.24 & 6.4$\pm$1.2$^{(1)}$ & -13.4 & -23.6 & 32 &  \\ 
204434699 & 15 57 39.35 & -22 20 57.4 & 15.61 & 11.5 & -14.43$\pm$2.09 & -23.93$\pm$2.09 & 4.9$\pm$0.9$^{(1)}$ & -13.8 & -23.5 & 78 & \\ 
204435603 & 16 01 49.51 & -22 20 45.2 & 16.91 & 12.42 & -7.93$\pm$2.05 & -23.17$\pm$2.05 & 4.8$\pm$0.9$^{(1)}$ & -13.5 & -23.6 & 63 & 1.594\\ 
204435866 & 16 19 23.93 & -22 20 41.3 & 16.34 & 11.9 & -10.53$\pm$2.19 & -27.83$\pm$2.24 & 5.3$\pm$1.0$^{(1)}$ & -12.3 & -24.0 & 85 &  \\ 
204438578 & 16 01 16.80 & -22 20 02.2 & 11.23 & 8.62 & -12.34$\pm$1.03 & -11.53$\pm$0.97 & 6.4$\pm$1.2$^{(1)}$ & -13.5 & -23.6 & 38 &  \\ 
204447226 & 16 39 43.44 & -22 17 59.4 & 10.16 & 8.68 & -17.63$\pm$1.51 & -22.98$\pm$0.93 & 8.4$\pm$0.6$^{(0)}$ & -11.0 & -24.4 & 90 &  \\ 
204451363 & 15 54 39.32 & -22 17 01.5 & 14.74 & 10.7 & -12.17$\pm$2.1 & -22.4$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -14.0 & -23.4 & 94 & 2.062\\ 
204462113 & 16 24 55.33 & -22 14 28.6 & 13.98 & 10.22 & -5.8$\pm$3.4 & -27.0$\pm$2.3 & 7.4$\pm$1.4$^{(1)}$ & -11.9 & -24.1 & 93 & 5.755\\ 
204462739 & 16 16 00.81 & -22 14 18.8 & 15.35 & 10.98 & -10.46$\pm$2.07 & -27.74$\pm$2.07 & 9.3$\pm$1.7$^{(1)}$ & -12.5 & -23.9 & 95 & 1.295\\ 
204465247 & 16 11 44.91 & -22 13 41.9 & 11.0 & 8.11 & -3.62$\pm$1.05 & -15.92$\pm$1.01 & 8.5$\pm$1.6$^{(1)}$ & -12.8 & -23.8 & 38 & 7.664\\ 
204469527 & 16 24 31.29 & -22 12 39.8 & 14.69 & 10.35 & -7.74$\pm$2.16 & -18.19$\pm$2.15 & 7.8$\pm$1.4$^{(1)}$ & -12.0 & -24.1 & 87 & 4.869\\ 
204469985 & 16 41 30.94 & -22 12 33.6 & 12.75 & 9.53 & -10.52$\pm$2.32 & -16.75$\pm$2.32 & 6.0$\pm$1.1$^{(1)}$ & -10.8 & -24.4 & 80 & 39.066\\ 
204471912 & 16 21 41.26 & -22 12 05.6 & 14.0 & 9.94 & -13.72$\pm$2.33 & -27.31$\pm$2.33 & 9.4$\pm$1.7$^{(1)}$ & -12.2 & -24.0 & 95 & 0.803\\ 
204475702 & 15 58 29.63 & -22 11 12.0 & 12.12 & 8.82 & -8.5$\pm$2.24 & -23.68$\pm$2.24 & 7.5$\pm$1.4$^{(1)}$ & -13.7 & -23.5 & 94 & 40.083\\ 
204483158 & 16 10 19.90 & -22 09 25.3 & 7.01 & 6.4 & -9.27$\pm$0.05 & -24.53$\pm$0.03 & 4.6$\pm$0.5$^{(0)}$ & -12.9 & -23.8 & 24 &  \\ 
204486919 & 16 40 48.18 & -22 08 30.1 & 10.84 & 8.49 & -23.53$\pm$3.26 & -18.63$\pm$1.73 & 5.8$\pm$0.4$^{(0)}$ & -10.9 & -24.4 & 19 &  \\ 
204487447 & 16 10 30.70 & -22 08 22.9 & 16.37 & 11.76 & -6.54$\pm$2.49 & -26.88$\pm$2.49 & 6.0$\pm$1.1$^{(1)}$ & -12.9 & -23.8 & 87 &  \\ 
204488355 & 16 14 20.50 & -22 08 09.7 & 7.66 & 6.88 & -8.76$\pm$0.32 & -25.42$\pm$0.34 & 7.3$\pm$0.3$^{(0)}$ & -12.7 & -23.9 & 98 &  \\ 
204489514 & 16 03 01.62 & -22 07 52.4 & 16.27 & 11.73 & -10.59$\pm$2.45 & -23.94$\pm$2.45 & 6.7$\pm$1.2$^{(1)}$ & -13.4 & -23.6 & 95 &  \\ 
204491374 & 16 13 11.72 & -22 07 25.2 & 15.38 & 11.21 & -8.96$\pm$2.07 & -24.68$\pm$2.07 & 6.1$\pm$1.1$^{(1)}$ & -12.7 & -23.8 & 93 & 1.245\\ 
204492163 & 16 14 08.95 & -22 07 13.4 & 15.59 & 11.48 & -9.59$\pm$2.07 & -22.1$\pm$2.07 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -23.9 & 80 & 0.567\\ 
204494046 & 16 15 51.63 & -22 06 44.9 & 15.4 & 11.48 & -8.39$\pm$2.07 & -24.12$\pm$2.07 & 4.4$\pm$0.8$^{(1)}$ & -12.5 & -23.9 & 45 & 1.742\\ 
204495624 & 16 10 42.59 & -22 06 21.3 & 15.82 & 11.5 & -11.09$\pm$2.07 & -25.09$\pm$2.07 & 6.3$\pm$1.2$^{(1)}$ & -12.9 & -23.8 & 95 & 1.966\\ 
204501712 & 16 10 56.91 & -22 04 51.6 & 15.65 & 11.4 & -8.28$\pm$2.07 & -25.35$\pm$2.07 & 5.6$\pm$1.0$^{(1)}$ & -12.9 & -23.8 & 89 & 2.029\\ 
204506663 & 16 32 43.64 & -22 03 38.4 & 13.3 & 9.67 & -12.87$\pm$2.35 & -11.56$\pm$2.35 & 6.4$\pm$1.2$^{(1)}$ & -11.4 & -24.2 & 39 &  \\ 
204508969 & 15 57 41.32 & -22 03 03.3 & 9.76 & 8.1 & -31.99$\pm$1.35 & -24.02$\pm$0.42 & 9.0$\pm$0.4$^{(0)}$ & -13.8 & -23.5 & 21 &  \\ 
204512343 & 15 57 21.10 & -22 02 13.0 & 14.0 & 10.1 & -10.83$\pm$2.09 & -19.1$\pm$2.09 & 5.3$\pm$1.0$^{(1)}$ & -13.8 & -23.5 & 80 & 7.761\\ 
204520625 & 16 26 22.23 & -22 00 09.0 & 14.94 & 10.59 & -16.93$\pm$2.15 & -21.07$\pm$2.15 & 7.0$\pm$1.3$^{(1)}$ & -11.8 & -24.1 & 92 & 1.378\\ 
204524139 & 16 29 31.13 & -21 59 15.9 & 10.5 & 8.79 & -4.61$\pm$2.26 & -26.18$\pm$0.63 & 5.1$\pm$0.6$^{(0)}$ & -11.6 & -24.1 & 49 & \\ 
204530046 & 16 10 50.11 & -21 57 48.2 & 15.03 & 10.79 & -9.65$\pm$2.07 & -25.93$\pm$2.07 & 6.6$\pm$1.2$^{(1)}$ & -12.9 & -23.8 & 95 & 1.973\\ 
204544974 & 16 07 33.51 & -21 54 05.8 & 11.28 & 8.77 & -5.64$\pm$2.24 & -17.21$\pm$2.24 & 5.3$\pm$1.0$^{(1)}$ & -13.1 & -23.7 & 50 &  \\ 
204546194 & 16 23 20.93 & -21 53 47.9 & 12.5 & 8.73 & -1.24$\pm$2.36 & -16.26$\pm$2.36 & 8.9$\pm$1.6$^{(1)}$ & -12.0 & -24.0 & 33 &  \\ 
204547272 & 15 59 22.93 & -21 53 31.6 & 14.14 & 10.39 & -1.21$\pm$2.07 & -19.88$\pm$2.07 & 5.3$\pm$1.0$^{(1)}$ & -13.7 & -23.5 & 19 & 3.398\\ 
204553407 & 16 03 01.81 & -21 51 58.4 & 15.59 & 11.49 & -9.55$\pm$2.05 & -22.9$\pm$2.05 & 5.5$\pm$1.0$^{(1)}$ & -13.4 & -23.6 & 88 & 1.718\\ 
204554162 & 16 16 09.43 & -21 51 46.8 & 12.47 & 9.26 & -15.24$\pm$2.24 & -26.7$\pm$2.24 & 6.1$\pm$1.1$^{(1)}$ & -12.5 & -23.9 & 94 & 7.228\\ 
204555809 & 16 09 01.98 & -21 51 22.5 & 17.57 & 12.63 & -10.06$\pm$2.49 & -40.74$\pm$2.82 & 6.5$\pm$1.2$^{(1)}$ & -13.0 & -23.7 & 45 & 0.269\\ 
204561327 & 16 11 09.20 & -21 49 56.2 &   & 11.6 & -9.7$\pm$3.9 & -23.5$\pm$3.9 & 31.5$\pm$5.8$^{(4)}$ & -12.9 & -23.8 & 32 & 0.946\\ 
204566795 & 16 23 58.05 & -21 48 33.8 & 16.25 & 11.44 & -12.97$\pm$2.16 & -15.89$\pm$2.16 & 9.9$\pm$1.8$^{(1)}$ & -12.0 & -24.0 & 78 & 1.115\\ 
204569741 & 16 15 42.70 & -21 47 49.7 & 10.74 & 9.28 & -19.56$\pm$2.2 & -19.91$\pm$1.18 & 5.8$\pm$0.7$^{(0)}$ & -12.5 & -23.9 & 75 &  \\ 
204571451 & 16 34 06.49 & -21 47 23.5 &   & 5.99 & -5.7$\pm$5.1 & -23.9$\pm$5.1 & 794.0$\pm$146.3$^{(4)}$ & -11.3 & -24.2 & 74 &  \\ 
204575214 & 16 15 22.63 & -21 46 25.8 & 9.99 & 8.52 & -26.62$\pm$1.33 & -24.74$\pm$2.09 & 6.7$\pm$0.8$^{(0)}$ & -12.6 & -23.8 & 47 &  \\ 
204576585 & 16 28 40.75 & -21 46 05.2 & 10.29 & 8.17 & -16.72$\pm$2.19 & -30.7$\pm$0.53 & 5.9$\pm$0.5$^{(0)}$ & -11.7 & -24.1 & 70 & \\ 
204577308 & 15 56 45.52 & -21 45 54.8 & 11.88 & 9.07 & -12.1$\pm$2.24 & -9.78$\pm$2.24 & 5.4$\pm$1.0$^{(1)}$ & -13.8 & -23.4 & 15 &  \\ 
204584778 & 16 15 25.17 & -21 44 01.3 &   & 11.78 & -5.8$\pm$5.0 & -22.5$\pm$5.0 & 28.6$\pm$5.3$^{(4)}$ & -12.6 & -23.8 & 22 &  \\ 
204589989 & 16 21 40.59 & -21 42 44.0 & 11.52 & 8.82 & -3.01$\pm$1.02 & -19.96$\pm$1.01 & 6.0$\pm$1.1$^{(1)}$ & -12.1 & -24.0 & 62 & 11.111\\ 
204594663 & 16 25 22.43 & -21 41 32.9 &   & 11.63 & -11.6$\pm$5.1 & -22.4$\pm$5.1 & 31.7$\pm$5.8$^{(4)}$ & -11.9 & -24.0 & 30 & 0.922\\ 
204603210 & 16 04 35.88 & -21 39 22.2 & 13.9 & 9.86 & -24.66$\pm$2.65 & -24.25$\pm$2.34 & 9.0$\pm$1.7$^{(1)}$ & -13.3 & -23.6 & 81 & $<$2\\ 
204603511 & 16 22 10.05 & -21 39 17.3 & 8.51 & 7.65 & -9.76$\pm$0.49 & -21.81$\pm$0.53 & 7.2$\pm$0.4$^{(0)}$ & -12.1 & -24.0 & 97 & $<$2\\ 
204604402 & 15 55 17.96 & -21 39 04.0 & 15.34 & 11.12 & -14.29$\pm$2.1 & -21.18$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -13.9 & -23.4 & 92 & 3.091\\ 
204608292 & 16 09 35.75 & -21 38 05.8 & 13.73 & 9.91 & -10.64$\pm$2.24 & -21.62$\pm$2.24 & 7.0$\pm$1.3$^{(1)}$ & -13.0 & -23.7 & 95 & 4.404\\ 
204611596 & 16 16 54.57 & -21 37 15.5 & 9.91 & 8.38 & -10.56$\pm$1.34 & -24.0$\pm$0.91 & 7.6$\pm$0.5$^{(0)}$ & -12.5 & -23.9 & 97 & \\ 
204612315 & 16 01 56.47 & -21 37 03.9 & 10.6 & 8.3 & -11.97$\pm$2.59 & -23.45$\pm$0.36 & 6.9$\pm$0.6$^{(0)}$ & -13.5 & -23.5 & 98 & 2.305\\ 
204614662 & 16 25 33.83 & -21 36 28.7 & 11.27 & 7.96 & -19.79$\pm$2.36 & -13.86$\pm$2.36 & 11.4$\pm$2.1$^{(1)}$ & -11.9 & -24.0 & 29 & 7.764\\ 
204615541 & 16 20 31.18 & -21 36 15.1 & 14.47 & 10.59 & -10.98$\pm$2.14 & -18.22$\pm$2.14 & 5.8$\pm$1.1$^{(1)}$ & -12.2 & -23.9 & 86 & 2.47\\ 
204623020 & 16 25 10.35 & -21 34 23.5 & 16.02 & 11.45 & -11.28$\pm$2.64 & -19.42$\pm$2.64 & 7.4$\pm$1.4$^{(1)}$ & -11.9 & -24.0 & 93 & 0.658\\ 
204635232 & 16 22 59.44 & -21 31 18.5 & 12.63 & 8.99 & -1.46$\pm$1.99 & -33.9$\pm$3.26 & 9.4$\pm$1.7$^{(1)}$ & -12.0 & -24.0 & 48 &  \\ 
204637674 & 16 23 45.17 & -21 30 40.9 & 11.93 & 8.99 & -13.68$\pm$2.36 & -21.78$\pm$2.36 & 5.6$\pm$1.0$^{(1)}$ & -12.0 & -24.0 & 90 & 8.835\\ 
204639156 & 16 40 27.82 & -21 30 18.8 & 13.4 & 10.16 & -8.85$\pm$2.1 & -22.02$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -10.9 & -24.3 & 51 & \\ 
204651122 & 16 12 22.90 & -21 27 15.9 &   & 12.03 & -5.4$\pm$4.6 & -30.9$\pm$4.6 & 25.7$\pm$4.7$^{(4)}$ & -12.8 & -23.8 & 19 &  \\ 
204683246 & 16 22 36.01 & -21 19 01.1 & 13.45 & 9.86 & -15.74$\pm$2.36 & -26.8$\pm$2.36 & 6.1$\pm$1.1$^{(1)}$ & -12.1 & -24.0 & 93 & 8.921\\ 
204750116 & 15 55 16.73 & -21 01 36.6 & 11.44 & 9.62 & -10.44$\pm$2.09 & -20.92$\pm$0.44 & 5.6$\pm$0.6$^{(0)}$ & -13.9 & -23.4 & 89 & \\ 
204769996 & 16 09 36.08 & -20 56 25.6 &   & 11.68 & -9.3$\pm$3.6 & -29.3$\pm$3.6 & 15.9$\pm$2.9$^{(4)}$ & -12.9 & -23.7 & 68 & 1.718\\ 
204776782 & 16 15 20.83 & -20 54 37.3 &   & 11.28 & -8.2$\pm$3.6 & -36.5$\pm$3.6 & 10.9$\pm$2.0$^{(4)}$ & -12.5 & -23.8 & 74 & 1.93\\ 
204777646 & 15 58 19.07 & -20 54 24.1 & 12.22 & 9.03 & -10.22$\pm$2.2 & -24.59$\pm$2.2 & 6.5$\pm$1.2$^{(1)}$ & -13.7 & -23.4 & 95 & 7.133\\ 
204780592 & 15 58 30.39 & -20 53 36.0 & 7.21 & 6.53 & -12.64$\pm$0.25 & -23.5$\pm$0.28 & 7.2$\pm$0.4$^{(0)}$ & -13.7 & -23.4 & 98 &  \\ 
204807722 & 15 57 01.46 & -20 46 18.5 & 15.02 & 10.38 & -15.34$\pm$2.11 & -20.25$\pm$2.11 & 9.1$\pm$1.7$^{(1)}$ & -13.8 & -23.4 & 94 & 2.181\\ 
204810161 & 16 22 14.81 & -20 45 39.8 & 15.49 & 11.22 & -13.57$\pm$2.15 & -26.96$\pm$2.15 & 6.9$\pm$1.3$^{(1)}$ & -12.1 & -23.9 & 96 & $<$2\\ 
204828211 & 16 14 36.39 & -20 40 49.1 & 15.42 & 11.5 & -16.94$\pm$1.99 & -29.26$\pm$1.99 & 4.4$\pm$0.8$^{(1)}$ & -12.6 & -23.7 & 26 & 0.726\\ 
204828394 & 16 23 13.16 & -20 40 46.0 & 12.89 & 9.76 & -22.28$\pm$2.36 & -32.88$\pm$2.36 & 5.2$\pm$1.0$^{(1)}$ & -12.0 & -23.9 & 28 &  \\ 
204830256 & 16 07 57.14 & -20 40 17.4 &   & 11.65 & -8.9$\pm$3.6 & -22.9$\pm$3.6 & 30.4$\pm$5.6$^{(4)}$ & -13.0 & -23.6 & 31 &  \\ 
204840715 & 16 26 40.58 & -20 37 28.7 & 12.41 & 9.14 & -9.0$\pm$1.1 & -28.88$\pm$1.15 & 6.4$\pm$1.2$^{(1)}$ & -11.8 & -24.0 & 93 & \\ 
204852633 & 16 03 24.38 & -20 34 13.0 & 16.98 & 12.34 & -11.99$\pm$2.38 & -19.04$\pm$2.38 & 5.6$\pm$1.0$^{(1)}$ & -13.3 & -23.5 & 87 & 0.345\\ 
204853319 & 16 27 43.41 & -20 34 01.8 & 18.15 & 12.68 & -11.23$\pm$2.89 & -30.21$\pm$2.89 & 5.1$\pm$0.9$^{(1)}$ & -11.7 & -24.0 & 75 & 1.001\\ 
204857023 & 16 12 08.24 & -20 33 01.6 & 14.28 & 9.84 & -22.37$\pm$2.14 & -14.8$\pm$2.14 & 10.5$\pm$1.9$^{(1)}$ & -12.7 & -23.7 & 35 & 1.464\\ 
204862399 & 15 55 52.73 & -20 31 33.6 &   & 11.67 & -6.0$\pm$3.9 & -18.0$\pm$3.9 & 30.7$\pm$5.6$^{(4)}$ & -13.8 & -23.3 & 13 & 0.295\\ 
204862760 & 16 21 53.10 & -20 31 27.7 & 12.62 & 8.47 & -9.01$\pm$1.01 & -14.62$\pm$0.59 & 7.2$\pm$0.2$^{(0)}$ & -12.1 & -23.9 & 77 &  \\ 
204862767 & 16 18 44.87 & -20 31 27.6 & 14.48 & 10.41 & -12.85$\pm$2.05 & -25.8$\pm$2.05 & 6.3$\pm$1.2$^{(1)}$ & -12.3 & -23.8 & 95 & 1.048\\ 
204870435 & 16 08 46.05 & -20 29 20.6 & 11.38 & 8.29 & -10.81$\pm$2.14 & -11.14$\pm$2.14 & 8.1$\pm$1.5$^{(1)}$ & -13.0 & -23.6 & 44 &  \\ 
204874314 & 16 35 39.13 & -20 28 19.5 & 11.95 & 8.31 & -2.02$\pm$2.35 & -18.28$\pm$2.35 & 11.6$\pm$2.1$^{(1)}$ & -11.2 & -24.1 & 45 & 52.613\\ 
204886563 & 15 57 00.86 & -20 24 59.5 & 12.23 & 8.89 & -17.1$\pm$2.3 & -35.26$\pm$2.3 & 8.1$\pm$1.5$^{(1)}$ & -13.7 & -23.3 & 89 & 1.898\\ 
204888409 & 16 12 48.97 & -20 24 30.3 & 16.34 & 12.08 & -13.05$\pm$1.99 & -23.12$\pm$1.99 & 4.4$\pm$0.8$^{(1)}$ & -12.7 & -23.7 & 44 & 1.374\\ 
204894208 & 16 00 29.46 & -20 22 53.6 &   & 11.29 & -15.4$\pm$3.6 & -24.0$\pm$3.6 & 33.6$\pm$6.2$^{(4)}$ & -13.5 & -23.4 & 37 & 1.697\\ 
204894630 & 16 08 57.46 & -20 22 47.2 & 15.05 & 11.1 & -19.33$\pm$1.99 & -27.49$\pm$1.99 & 4.9$\pm$0.9$^{(1)}$ & -12.9 & -23.6 & 57 & 1.019\\ 
204896403 & 15 57 08.53 & -20 22 18.4 & 15.5 & 11.42 & -17.7$\pm$2.04 & -26.96$\pm$2.04 & 5.4$\pm$1.0$^{(1)}$ & -13.7 & -23.3 & 85 & 1.446\\ 
204903039 & 16 13 44.75 & -20 20 26.5 & 12.52 & 9.4 & -5.86$\pm$2.14 & -19.34$\pm$2.14 & 5.0$\pm$0.9$^{(1)}$ & -12.6 & -23.7 & 55 & 2.774\\ 
204907615 & 16 13 51.41 & -20 19 12.6 & 11.09 & 8.29 & -14.55$\pm$2.14 & -11.4$\pm$2.14 & 7.6$\pm$1.4$^{(1)}$ & -12.6 & -23.7 & 48 &  \\ 
204907707 & 16 28 34.97 & -20 19 11.2 & 14.04 & 10.5 & -3.91$\pm$2.15 & -20.34$\pm$2.15 & 4.6$\pm$0.8$^{(1)}$ & -11.6 & -24.0 & 28 & \\ 
204912203 & 16 12 26.64 & -20 17 57.4 & 12.4 & 9.27 & -4.88$\pm$2.14 & -12.48$\pm$2.14 & 5.4$\pm$1.0$^{(1)}$ & -12.7 & -23.7 & 15 &  \\ 
204912351 & 16 12 02.23 & -20 17 55.2 &   & 11.08 & -7.3$\pm$3.6 & -29.4$\pm$3.6 & 32.6$\pm$6.0$^{(4)}$ & -12.7 & -23.7 & 22 & 3.263\\ 
204914113 & 16 31 16.58 & -20 17 26.3 & 11.98 & 8.64 & -2.34$\pm$1.02 & -17.81$\pm$1.02 & 8.2$\pm$1.5$^{(1)}$ & -11.5 & -24.0 & 54 &  \\ 
204917514 & 16 15 09.49 & -20 16 28.8 & 11.39 & 8.9 & -22.18$\pm$1.0 & -29.66$\pm$1.0 & 5.5$\pm$1.0$^{(1)}$ & -12.5 & -23.7 & 51 &  \\ 
204932248 & 16 20 08.99 & -20 12 22.4 & 14.97 & 10.62 & -11.09$\pm$2.05 & -29.65$\pm$2.05 & 8.3$\pm$1.5$^{(1)}$ & -12.2 & -23.8 & 95 & 3.723\\ 
204933893 & 16 00 35.99 & -20 11 55.0 & 14.79 & 10.66 & -17.16$\pm$1.99 & -32.74$\pm$1.99 & 7.4$\pm$1.4$^{(1)}$ & -13.5 & -23.4 & 92 & 1.53\\ 
204942358 & 16 20 26.00 & -20 09 31.1 & 12.69 & 9.48 & -19.54$\pm$2.22 & -13.96$\pm$2.22 & 6.1$\pm$1.1$^{(1)}$ & -12.2 & -23.8 & 43 &  \\ 
204949414 & 16 10 42.79 & -20 07 31.0 & 11.7 & 9.11 & -3.6$\pm$2.14 & -14.96$\pm$2.14 & 5.0$\pm$0.9$^{(1)}$ & -12.8 & -23.6 & 15 &  \\ 
204951022 & 16 20 30.26 & -20 07 03.7 & 7.4 & 6.23 & -11.07$\pm$0.2 & -26.53$\pm$0.12 & 8.5$\pm$0.5$^{(0)}$ & -12.2 & -23.8 & 90 &  \\ 
204952800 & 16 10 45.26 & -20 06 34.5 &   & 10.17 & -20.6$\pm$2.7 & -21.0$\pm$2.2 & 60.8$\pm$11.2$^{(4)}$ & -12.8 & -23.6 & 18 & $<$2\\ 
204952985 & 16 39 44.75 & -20 06 30.9 & 12.33 & 9.45 & -13.3$\pm$2.32 & -30.07$\pm$2.32 & 4.9$\pm$0.9$^{(1)}$ & -10.9 & -24.2 & 64 & 1.001\\ 
204955018 & 16 07 09.55 & -20 05 56.2 & 11.2 & 8.51 & -5.82$\pm$1.04 & -12.64$\pm$1.03 & 6.7$\pm$1.2$^{(1)}$ & -13.0 & -23.5 & 28 & $<$2\\ 
204957540 & 15 58 21.07 & -20 05 13.6 & 15.05 & 11.06 & -13.77$\pm$1.99 & -19.64$\pm$1.99 & 5.1$\pm$0.9$^{(1)}$ & -13.6 & -23.3 & 80 & 2.231\\ 
204958441 & 16 53 07.98 & -20 04 59.0 & 11.57 & 8.25 & -7.78$\pm$2.28 & -9.43$\pm$2.28 & 9.4$\pm$1.7$^{(1)}$ & -18.2 & -22.7 & 14 &  \\ 
204960911 & 16 24 40.79 & -20 04 17.2 & 14.38 & 10.5 & -2.4$\pm$2.15 & -29.19$\pm$2.15 & 4.7$\pm$0.9$^{(1)}$ & -11.9 & -23.9 & 21 &  \\ 
204975077 & 16 07 44.01 & -20 00 15.3 & 11.8 & 9.4 & -9.68$\pm$1.05 & -18.36$\pm$1.04 & 4.2$\pm$0.8$^{(1)}$ & -13.0 & -23.5 & 22 & 18.95\\ 
204982668 & 16 10 43.63 & -19 58 07.1 & 11.3 & 8.34 & -16.25$\pm$2.14 & -11.21$\pm$2.14 & 7.2$\pm$1.3$^{(1)}$ & -12.8 & -23.6 & 43 &  \\ 
204982702 & 16 09 52.07 & -19 58 06.6 & 15.22 & 10.46 & -14.39$\pm$1.99 & -25.34$\pm$1.99 & 5.2$\pm$1.0$^{(1)}$ & -12.9 & -23.6 & 85 & 2.405\\ 
204983289 & 16 13 45.01 & -19 57 56.8 & 12.02 & 9.04 & -17.13$\pm$2.14 & -10.84$\pm$2.14 & 6.0$\pm$1.1$^{(1)}$ & -12.6 & -23.7 & 25 &  \\ 
204983628 & 16 12 27.05 & -19 57 50.9 & 12.06 & 9.23 & -10.98$\pm$2.14 & -11.72$\pm$2.14 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -23.6 & 21 &  \\ 
204986244 & 16 12 31.39 & -19 57 06.7 & 11.93 & 9.14 & -16.78$\pm$2.14 & -33.22$\pm$2.14 & 5.3$\pm$1.0$^{(1)}$ & -12.7 & -23.6 & 62 & $<$2\\ 
205001070 & 16 00 29.13 & -19 52 53.8 & 11.27 & 8.68 & -9.39$\pm$1.01 & -21.62$\pm$1.01 & 5.8$\pm$1.1$^{(1)}$ & -13.5 & -23.4 & 91 & 3.931\\ 
205010433 & 16 25 26.74 & -19 50 14.2 & 8.76 & 7.28 & -9.61$\pm$0.08 & -30.26$\pm$0.05 & 5.9$\pm$0.3$^{(0)}$ & -11.8 & -23.9 & 43 & \\ 
205011893 & 16 50 04.50 & -19 49 49.8 & 13.41 & 9.91 & -6.6$\pm$2.28 & -14.41$\pm$2.28 & 4.6$\pm$0.8$^{(1)}$ & -19.2 & -22.2 & 16 &  \\ 
205013031 & 16 12 40.21 & -19 49 30.2 &   & 11.29 & -9.1$\pm$3.6 & -28.1$\pm$3.6 & 19.7$\pm$3.6$^{(4)}$ & -12.7 & -23.6 & 53 & 3.621\\ 
205024586 & 16 24 15.28 & -19 46 10.3 & 13.77 & 10.04 & -11.79$\pm$2.15 & -11.47$\pm$2.15 & 5.5$\pm$1.0$^{(1)}$ & -11.9 & -23.8 & 28 &  \\ 
205026865 & 16 45 59.92 & -19 45 31.1 & 10.31 & 8.69 & -5.99$\pm$2.36 & -15.2$\pm$1.71 & 6.2$\pm$0.3$^{(0)}$ & -10.5 & -24.2 & 81 & 6.574\\ 
205037489 & 16 15 17.76 & -19 42 30.2 & 14.29 & 10.19 & -12.92$\pm$1.99 & -19.55$\pm$1.99 & 6.9$\pm$1.3$^{(1)}$ & -12.5 & -23.7 & 94 & 6.018\\ 
205039568 & 16 49 17.09 & -19 41 53.4 & 11.94 & 8.33 & -8.72$\pm$2.29 & -18.91$\pm$2.29 & 10.3$\pm$1.9$^{(1)}$ & -19.5 & -22.0 & 87 & 13.733\\ 
205047378 & 16 14 13.82 & -19 39 36.3 & 9.22 & 7.25 & -7.32$\pm$1.05 & -19.2$\pm$0.66 & 6.4$\pm$0.4$^{(0)}$ & -12.6 & -23.6 & 94 & 1.869\\ 
205048103 & 16 25 41.31 & -19 39 23.0 & 14.85 & 10.42 & -10.45$\pm$2.15 & -20.06$\pm$2.15 & 6.5$\pm$1.2$^{(1)}$ & -11.8 & -23.9 & 93 & \\ 
205049221 & 15 55 22.40 & -19 39 02.9 & 15.19 & 11.01 & -11.84$\pm$2.13 & -23.96$\pm$2.13 & 6.5$\pm$1.2$^{(1)}$ & -13.8 & -23.2 & 96 & 29.704\\ 
205049683 & 16 14 12.18 & -19 38 55.4 & 12.05 & 9.03 & -9.71$\pm$2.14 & -17.64$\pm$2.14 & 6.0$\pm$1.1$^{(1)}$ & -12.6 & -23.6 & 85 & 4.235\\ 
205059490 & 16 36 39.23 & -19 36 07.6 & 9.31 & 8.11 & -12.28$\pm$0.7 & -20.43$\pm$0.86 & 6.2$\pm$0.5$^{(0)}$ & -11.1 & -24.1 & 96 & \\ 
205061092 & 16 14 51.79 & -19 35 40.3 & 20.15 & 12.37 & -9.8$\pm$4.6 & -24.1$\pm$4.6 & 4.2$\pm$0.8$^{(1)}$ & -12.5 & -23.6 & 18 &  \\ 
205063210 & 16 07 39.16 & -19 35 04.1 & 15.66 & 11.31 & -11.26$\pm$1.99 & -26.6$\pm$1.99 & 7.1$\pm$1.3$^{(1)}$ & -13.0 & -23.5 & 96 & 2.435\\ 
205075874 & 16 38 28.57 & -19 31 26.0 & 9.86 & 8.3 & -7.93$\pm$0.71 & -20.97$\pm$0.78 & 5.1$\pm$0.9$^{(1)}$ & -11.0 & -24.1 & 81 & 0.811\\ 
205085890 & 16 47 06.31 & -19 28 26.4 & 12.09 & 9.22 & -1.83$\pm$2.28 & -15.82$\pm$2.28 & 5.5$\pm$1.0$^{(1)}$ & -20.3 & -21.7 & 34 &  \\ 
205092842 & 16 12 02.40 & -19 26 22.1 & 15.24 & 10.86 & -4.0$\pm$4.9 & -31.6$\pm$4.8 & 7.2$\pm$1.3$^{(1)}$ & -12.7 & -23.6 & 85 & 1.777\\ 
205102553 & 16 12 18.45 & -19 23 32.5 &   & 12.0 & -7.9$\pm$4.6 & -26.3$\pm$4.6 & 26.2$\pm$4.8$^{(4)}$ & -12.7 & -23.6 & 32 & 1.851\\ 
205110559 & 16 15 19.72 & -19 21 07.1 & 15.07 & 10.46 & -12.07$\pm$1.99 & -24.54$\pm$1.99 & 10.7$\pm$2.0$^{(1)}$ & -12.5 & -23.6 & 94 & 0.403\\ 
205110634 & 16 12 38.81 & -19 21 05.7 & 11.32 & 8.05 & -7.22$\pm$2.14 & -10.29$\pm$2.14 & 8.9$\pm$1.6$^{(1)}$ & -12.6 & -23.6 & 21 &  \\ 
205114690 & 16 26 35.44 & -19 19 53.4 & 12.45 & 9.26 & -13.44$\pm$2.36 & -20.68$\pm$2.36 & 6.2$\pm$1.1$^{(1)}$ & -11.7 & -23.8 & 93 & \\ 
205120406 & 16 28 37.94 & -19 18 12.3 & 10.51 & 8.5 & -6.36$\pm$1.02 & -18.1$\pm$1.01 & 6.4$\pm$1.2$^{(1)}$ & -11.6 & -23.9 & 84 & \\ 
205121036 & 16 27 50.66 & -19 18 00.4 & 12.63 & 9.31 & -18.76$\pm$2.36 & -28.92$\pm$2.36 & 6.7$\pm$1.2$^{(1)}$ & -11.6 & -23.9 & 90 & 26.981\\ 
205123115 & 16 12 59.53 & -19 17 23.6 & 12.86 & 9.02 & -7.27$\pm$2.14 & -8.72$\pm$2.14 & 7.9$\pm$1.5$^{(1)}$ & -12.6 & -23.6 & 11 &  \\ 
205129147 & 16 12 05.40 & -19 15 35.5 & 12.22 & 8.79 & -12.33$\pm$2.14 & -28.28$\pm$2.14 & 8.6$\pm$1.6$^{(1)}$ & -12.7 & -23.6 & 96 & 8.634\\ 
205142340 & 16 08 35.78 & -19 11 37.3 & 16.78 & 12.17 & -11.85$\pm$2.41 & -25.87$\pm$2.41 & 6.4$\pm$1.2$^{(1)}$ & -12.9 & -23.5 & 95 & 1.306\\ 
205146145 & 16 47 14.88 & -19 10 27.9 & 11.78 & 8.99 & -5.29$\pm$0.99 & -13.96$\pm$0.99 & 5.6$\pm$1.0$^{(1)}$ & -20.2 & -21.3 & 37 & \\ 
205149448 & 16 08 15.21 & -19 09 28.4 & 11.52 & 8.3 & -6.25$\pm$2.14 & -15.66$\pm$2.14 & 8.4$\pm$1.5$^{(1)}$ & -12.9 & -23.5 & 69 &  \\ 
205152398 & 16 10 24.69 & -19 08 34.9 & 11.88 & 8.86 & -7.1$\pm$2.14 & -10.86$\pm$2.14 & 6.3$\pm$1.2$^{(1)}$ & -12.8 & -23.5 & 25 &  \\ 
205153472 & 16 00 34.55 & -19 08 15.9 &   & 11.46 & -20.0$\pm$3.6 & -30.1$\pm$3.6 & 6.5$\pm$1.2$^{(4)}$ & -13.4 & -23.3 & 91 & 0.761\\ 
205155483 & 15 56 57.16 & -19 07 38.9 & 9.78 & 8.17 & -19.74$\pm$0.69 & -21.4$\pm$0.85 & 5.5$\pm$1.0$^{(1)}$ & -13.7 & -23.2 & 83 & 5.889\\ 
205156004 & 16 10 30.94 & -19 07 29.6 & 11.16 & 8.26 & -9.13$\pm$1.15 & -13.3$\pm$1.12 & 7.7$\pm$1.4$^{(1)}$ & -12.8 & -23.5 & 60 &  \\ 
205156547 & 16 12 12.42 & -19 07 19.2 & 15.68 & 10.96 & -7.96$\pm$1.99 & -26.55$\pm$1.99 & 9.3$\pm$1.7$^{(1)}$ & -12.7 & -23.6 & 93 & 1.801\\ 
205156961 & 16 19 54.65 & -19 07 11.5 & 14.26 & 10.7 & -11.12$\pm$2.05 & -23.88$\pm$2.05 & 4.1$\pm$0.8$^{(1)}$ & -12.2 & -23.7 & 19 & 7.941\\ 
205160565 & 16 14 20.91 & -19 06 05.2 & 13.04 & 8.15 & -13.86$\pm$2.14 & -23.9$\pm$2.14 & 17.0$\pm$3.1$^{(1)}$ & -12.5 & -23.6 & 76 & 18.989\\ 
205161474 & 16 49 33.97 & -19 05 48.1 & 13.95 & 10.44 & -10.58$\pm$2.08 & -17.89$\pm$2.08 & 4.3$\pm$0.8$^{(1)}$ & -19.4 & -21.3 & 19 & \\ 
205161643 & 16 24 08.95 & -19 05 44.6 & 13.99 & 10.4 & -21.56$\pm$2.15 & -25.22$\pm$2.15 & 5.4$\pm$1.0$^{(1)}$ & -11.9 & -23.8 & 62 & 4.379\\ 
205162306 & 15 58 20.38 & -19 05 32.6 & 15.12 & 11.0 & -13.39$\pm$1.99 & -24.1$\pm$1.99 & 5.5$\pm$1.0$^{(1)}$ & -13.6 & -23.3 & 91 & 1.954\\ 
205164304 & 16 06 31.11 & -19 04 57.6 & 17.5 & 12.72 & -7.47$\pm$2.39 & -24.84$\pm$2.39 & 5.5$\pm$1.0$^{(1)}$ & -13.0 & -23.4 & 84 & 2.3\\ 
205165393 & 16 31 28.81 & -19 04 38.0 & 14.76 & 10.68 & -15.22$\pm$2.14 & -19.02$\pm$2.14 & 5.3$\pm$1.0$^{(1)}$ & -11.4 & -23.9 & 76 & 7.558\\ 
205166435 & 16 39 01.15 & -19 04 18.5 & 13.08 & 10.15 & -4.92$\pm$2.1 & -22.06$\pm$2.1 & 4.1$\pm$0.8$^{(1)}$ & -10.9 & -24.0 & 11 &  \\ 
205168266 & 16 12 05.99 & -19 03 44.4 & 7.87 & 6.81 & -8.46$\pm$0.42 & -23.89$\pm$0.47 & 6.4$\pm$0.4$^{(0)}$ & -12.7 & -23.5 & 96 & $<$2\\ 
205172974 & 16 48 51.59 & -19 02 18.3 & 11.94 & 8.45 & -7.31$\pm$2.29 & -13.67$\pm$2.29 & 10.1$\pm$1.9$^{(1)}$ & -19.7 & -21.2 & 54 &  \\ 
205173226 & 16 31 16.21 & -19 02 13.4 & 15.29 & 11.02 & -15.1$\pm$2.14 & -33.36$\pm$2.14 & 5.0$\pm$0.9$^{(1)}$ & -11.4 & -23.9 & 46 & 15.077\\ 
205173629 & 16 02 21.47 & -19 02 05.7 & 14.42 & 10.3 & -1.49$\pm$1.98 & -22.25$\pm$1.98 & 7.4$\pm$1.4$^{(1)}$ & -13.3 & -23.3 & 56 & 9.103\\ 
205178598 & 15 58 33.27 & -19 00 36.7 & 11.63 & 9.05 & -20.16$\pm$2.14 & -20.42$\pm$2.14 & 5.2$\pm$1.0$^{(1)}$ & -13.6 & -23.3 & 68 & \\ 
205183565 & 16 33 58.45 & -18 59 03.0 & 13.78 & 9.98 & -5.11$\pm$2.35 & -10.09$\pm$2.35 & 6.0$\pm$1.1$^{(1)}$ & -11.2 & -23.9 & 13 &  \\ 
205194104 & 16 34 30.19 & -18 55 45.1 & 12.58 & 9.27 & -2.76$\pm$2.35 & -14.6$\pm$2.35 & 6.8$\pm$1.2$^{(1)}$ & -11.2 & -23.9 & 45 &  \\ 
205198363 & 16 15 33.41 & -18 54 25.0 & 16.47 & 11.27 & -11.67$\pm$2.58 & -20.53$\pm$2.47 & 10.6$\pm$1.9$^{(1)}$ & -12.4 & -23.6 & 92 & $<$2\\ 
205200173 & 16 03 28.72 & -18 53 51.7 & 14.17 & 10.12 & -11.06$\pm$1.98 & -20.85$\pm$1.98 & 7.5$\pm$1.4$^{(1)}$ & -13.2 & -23.4 & 95 & 7.531\\ 
205202444 & 15 58 13.21 & -18 53 10.1 & 14.99 & 11.11 & -17.4$\pm$1.99 & -27.25$\pm$1.99 & 4.7$\pm$0.9$^{(1)}$ & -13.6 & -23.2 & 57 & 1.521\\ 
205203719 & 16 34 38.20 & -18 52 47.8 & 13.73 & 10.13 & -5.89$\pm$2.14 & -11.29$\pm$2.14 & 5.3$\pm$1.0$^{(1)}$ & -11.2 & -23.9 & 12 &  \\ 
205209357 & 16 15 08.57 & -18 51 01.1 & 13.55 & 9.54 & -5.88$\pm$2.14 & -24.3$\pm$2.14 & 7.1$\pm$1.3$^{(1)}$ & -12.5 & -23.6 & 92 & 11.394\\ 
205210347 & 16 15 59.85 & -18 50 42.8 & 11.97 & 8.43 & -21.76$\pm$2.14 & -22.21$\pm$2.14 & 9.7$\pm$1.8$^{(1)}$ & -12.4 & -23.6 & 84 & 1.349\\ 
205225428 & 16 00 35.45 & -18 45 58.1 & 15.05 & 10.87 & -10.42$\pm$1.99 & -21.72$\pm$1.99 & 6.4$\pm$1.2$^{(1)}$ & -13.4 & -23.3 & 94 & 1.423\\ 
205225696 & 16 13 43.51 & -18 45 52.6 &   & 10.52 & -5.9$\pm$3.6 & -24.2$\pm$3.6 & 55.7$\pm$10.3$^{(4)}$ & -12.5 & -23.6 & 18 & 0.888\\ 
205232648 & 16 01 57.67 & -18 43 41.9 & 14.95 & 10.9 & -11.28$\pm$1.98 & -22.11$\pm$1.98 & 5.6$\pm$1.0$^{(1)}$ & -13.3 & -23.3 & 91 & 1.976\\ 
205258053 & 16 32 40.95 & -18 35 39.6 & 11.63 & 8.38 & -6.05$\pm$2.35 & -9.83$\pm$2.35 & 8.9$\pm$1.6$^{(1)}$ & -11.3 & -23.9 & 17 &  \\ 
205272194 & 16 18 37.59 & -18 31 06.6 &   & 11.13 & -2.3$\pm$3.6 & -19.1$\pm$3.6 & 15.0$\pm$2.8$^{(4)}$ & -12.2 & -23.6 & 34 & 0.437\\ 
205278648 & 16 27 34.79 & -18 29 02.8 & 10.84 & 8.67 & -2.82$\pm$1.2 & -35.73$\pm$1.12 & 7.4$\pm$1.4$^{(1)}$ & -11.6 & -23.8 & 41 &  \\ 
205285100 & 16 46 03.77 & -18 26 56.9 &   & 10.22 & -0.3$\pm$5.2 & -31.2$\pm$5.1 & 19.6$\pm$3.6$^{(4)}$ & -20.6 & -20.3 & 22 & 1.527\\ 
205290233 & 16 24 18.23 & -18 25 17.7 & 12.53 & 9.44 & -14.36$\pm$2.36 & -38.72$\pm$2.36 & 6.2$\pm$1.1$^{(1)}$ & -11.8 & -23.7 & 54 & 4.937\\ 
205300382 & 16 39 47.61 & -18 22 00.1 & 11.49 & 8.4 & -8.98$\pm$2.32 & -31.26$\pm$2.32 & 8.0$\pm$1.5$^{(1)}$ & -22.8 & -20.0 & 94 & 1.498\\ 
205308135 & 16 43 53.35 & -18 19 29.7 & 10.15 & 7.21 & -15.94$\pm$1.04 & -32.16$\pm$1.04 & 14.1$\pm$2.6$^{(1)}$ & -21.4 & -20.1 & 78 &  \\ 
205312747 & 16 43 08.06 & -18 17 58.8 & 11.13 & 9.09 & -17.13$\pm$2.44 & -30.47$\pm$1.36 & 6.4$\pm$1.0$^{(0)}$ & -21.6 & -20.0 & 86 &  \\ 
205345560 & 16 06 23.83 & -18 07 18.4 & 14.38 & 10.38 & -14.31$\pm$2.02 & -15.08$\pm$2.02 & 6.3$\pm$1.2$^{(1)}$ & -13.0 & -23.3 & 82 & \\ 
205373716 & 16 13 20.80 & -17 57 52.1 & 13.89 & 9.87 & -5.58$\pm$6.55 & -22.34$\pm$6.55 & 9.6$\pm$1.8$^{(1)}$ & -12.5 & -23.5 & 85 & 4.116\\ 
205373893 & 16 13 21.24 & -17 57 48.7 & 13.99 & 10.04 & -4.85$\pm$2.72 & -19.37$\pm$2.72 & 8.0$\pm$1.5$^{(1)}$ & -12.5 & -23.5 & 83 & $<$2\\ 
205387342 & 16 49 15.04 & -17 53 25.9 & 13.42 & 9.85 & -4.26$\pm$2.27 & -14.94$\pm$2.27 & 6.1$\pm$1.1$^{(1)}$ & -19.5 & -19.6 & 59 &  \\ 
205399487 & 16 20 08.56 & -17 49 18.4 & 10.79 & 8.23 & -4.1$\pm$0.99 & -20.6$\pm$1.04 & 7.3$\pm$1.3$^{(1)}$ & -12.1 & -23.6 & 83 & 14.994\\ 
205403104 & 16 20 07.59 & -17 47 59.4 & 11.5 & 8.72 & -5.46$\pm$1.03 & -19.95$\pm$1.03 & 5.7$\pm$1.1$^{(1)}$ & -12.1 & -23.6 & 79 & 2.931\\ 
205404737 & 16 12 36.30 & -17 47 23.9 & 10.89 & 7.75 & -3.05$\pm$1.0 & -20.04$\pm$1.0 & 10.7$\pm$2.0$^{(1)}$ & -12.6 & -23.4 & 55 & 20.228\\ 
205406802 & 16 06 06.46 & -17 46 39.6 & 10.64 & 8.97 & -17.34$\pm$0.85 & -16.73$\pm$0.43 & 6.8$\pm$0.3$^{(0)}$ & -13.0 & -23.3 & 93 &  \\ 
205422543 & 16 13 34.37 & -17 40 50.5 & 9.94 & 8.43 & -18.86$\pm$1.9 & -27.06$\pm$0.5 & 8.7$\pm$0.5$^{(0)}$ & -12.5 & -23.4 & 93 & 3.245\\ 
205428264 & 16 21 29.76 & -17 38 43.8 & 11.58 & 8.64 & -7.72$\pm$1.06 & -11.97$\pm$1.04 & 6.7$\pm$1.2$^{(1)}$ & -12.0 & -23.6 & 36 & 0.648\\ 
205431822 & 16 24 50.66 & -17 37 23.4 & 12.0 & 9.07 & -8.09$\pm$1.03 & -14.3$\pm$1.16 & 5.8$\pm$1.1$^{(1)}$ & -11.8 & -23.7 & 59 & 6.048\\ 
205435449 & 16 36 44.45 & -17 36 01.1 & 13.7 & 10.01 & -14.14$\pm$2.13 & -21.23$\pm$2.13 & 6.2$\pm$1.1$^{(1)}$ & -23.8 & -18.9 & 93 &  \\ 
205454164 & 16 06 39.31 & -17 28 49.9 & 14.01 & 10.28 & -3.06$\pm$2.05 & -18.44$\pm$2.05 & 5.8$\pm$1.1$^{(1)}$ & -13.0 & -23.3 & 52 & 17.649\\ 
205457507 & 16 13 15.93 & -17 27 33.5 & 12.41 & 9.28 & -9.4$\pm$1.25 & -14.04$\pm$1.25 & 5.6$\pm$1.0$^{(1)}$ & -12.5 & -23.4 & 57 & 5.82\\ 
205462610 & 16 27 52.56 & -17 25 35.2 & 14.57 & 10.83 & -13.5$\pm$2.2 & -16.77$\pm$2.2 & 4.3$\pm$0.8$^{(1)}$ & -11.6 & -23.7 & 19 & 30.93\\ 
205473114 & 16 22 02.32 & -17 21 27.7 & 11.74 & 8.87 & -3.79$\pm$1.12 & -11.78$\pm$1.16 & 5.8$\pm$1.1$^{(1)}$ & -12.0 & -23.6 & 10 &  \\ 
205473448 & 16 39 04.20 & -17 21 19.6 & 11.73 & 9.33 & -17.65$\pm$1.0 & -16.46$\pm$1.0 & 4.9$\pm$0.9$^{(1)}$ & -23.0 & -18.6 & 24 & $<$2\\ 
205477423 & 16 09 46.88 & -17 19 44.9 & 11.55 & 8.69 & -7.84$\pm$1.15 & -15.22$\pm$1.11 & 6.2$\pm$1.1$^{(1)}$ & -12.7 & -23.3 & 71 & 5.424\\ 
205483967 & 16 26 58.64 & -17 17 09.9 & 11.56 & 8.96 & -14.99$\pm$1.02 & -17.72$\pm$1.03 & 6.4$\pm$1.2$^{(1)}$ & -11.6 & -23.7 & 89 & $<$2\\ 
205495323 & 16 07 23.13 & -17 12 42.0 & 12.4 & 9.38 & -6.9$\pm$2.24 & -17.14$\pm$2.24 & 5.2$\pm$1.0$^{(1)}$ & -12.9 & -23.3 & 60 & 7.078\\ 
205499733 & 16 11 20.78 & -17 10 54.2 & 10.37 & 8.97 & -4.28$\pm$0.77 & -22.28$\pm$0.52 & 6.1$\pm$0.2$^{(0)}$ & -12.6 & -23.4 & 83 & 2.55\\ 
205512911 & 16 27 04.72 & -17 05 32.1 &   & 12.62 & -7.4$\pm$5.6 & -29.7$\pm$5.6 & 23.8$\pm$4.4$^{(4)}$ & -11.6 & -23.6 & 31 & 1.601\\ 
205516967 & 16 20 28.25 & -17 03 51.1 & 11.98 & 8.96 & -15.47$\pm$1.06 & -12.98$\pm$1.1 & 5.9$\pm$1.1$^{(1)}$ & -12.0 & -23.5 & 47 &  \\ 
205525030 & 16 33 20.37 & -17 00 35.1 & 11.01 & 9.44 & -9.32$\pm$1.03 & -20.45$\pm$0.54 & 5.0$\pm$0.3$^{(0)}$ & -25.0 & -18.0 & 37 & 1.423\\ 
205527407 & 16 26 28.50 & -16 59 37.2 & 14.28 & 9.98 & -4.15$\pm$2.42 & -15.85$\pm$2.42 & 6.7$\pm$1.2$^{(1)}$ & -11.7 & -23.6 & 67 &  \\ 
205528725 & 16 26 18.03 & -16 59 06.1 & 12.34 & 8.69 & -19.74$\pm$2.42 & -10.86$\pm$2.42 & 9.6$\pm$1.8$^{(1)}$ & -11.7 & -23.6 & 21 &  \\ 
205537196 & 16 22 43.93 & -16 55 38.4 &   & 8.97 & -27.8$\pm$1.7 & -35.0$\pm$2.1 & 7.2$\pm$1.3$^{(2)}$ & -11.9 & -23.5 & 27 &  \\ 
205549542 & 16 30 22.80 & -16 50 26.3 & 11.52 & 8.23 & -18.77$\pm$2.37 & -17.49$\pm$2.37 & 9.6$\pm$1.8$^{(1)}$ & -11.4 & -23.7 & 78 &  \\ 
205554715 & 16 24 32.22 & -16 48 12.4 & 11.89 & 8.76 & -12.12$\pm$2.42 & -11.17$\pm$2.42 & 7.5$\pm$1.4$^{(1)}$ & -11.8 & -23.6 & 55 &  \\ 
205558283 & 16 09 20.42 & -16 46 40.4 & 10.8 & 8.15 & -4.11$\pm$0.95 & -29.51$\pm$0.95 & 7.6$\pm$1.4$^{(1)}$ & -12.7 & -23.3 & 76 & 3.909\\ 
205577864 & 16 24 41.20 & -16 38 20.5 & 12.71 & 8.88 & -5.76$\pm$2.42 & -9.4$\pm$2.42 & 9.0$\pm$1.7$^{(1)}$ & -11.8 & -23.6 & 15 &  \\ 
205586449 & 16 23 52.27 & -16 34 34.6 & 12.65 & 8.88 & -9.94$\pm$2.42 & -9.79$\pm$2.42 & 8.6$\pm$1.6$^{(1)}$ & -11.8 & -23.5 & 33 &  \\ 
205596184 & 16 18 03.05 & -16 30 15.2 &   & 11.69 & -14.3$\pm$4.9 & -29.4$\pm$4.9 & 10.5$\pm$1.9$^{(4)}$ & -12.2 & -23.4 & 91 & 2.095\\ 
205626492 & 16 09 04.58 & -16 16 32.8 & 14.81 & 10.75 & -5.15$\pm$2.11 & -15.76$\pm$2.11 & 6.6$\pm$1.2$^{(1)}$ & -12.7 & -23.2 & 67 & $<$2\\ 
205627441 & 16 27 03.36 & -16 16 06.3 & 11.18 & 7.88 & -14.55$\pm$0.97 & -20.95$\pm$0.97 & 12.9$\pm$2.4$^{(1)}$ & -11.6 & -23.6 & 88 & 1.737\\ 
205636990 & 16 25 48.08 & -16 11 40.6 & 10.88 & 7.58 & -10.32$\pm$1.73 & -16.9$\pm$1.73 & 14.0$\pm$2.6$^{(1)}$ & -11.7 & -23.5 & 71 & 2.796\\ 
205655538 & 16 12 28.63 & -16 02 46.8 & 10.37 & 8.93 & -16.41$\pm$0.84 & -37.97$\pm$0.53 & 7.6$\pm$0.2$^{(0)}$ & -12.5 & -23.3 & 87 &  \\ 
205661547 & 16 26 02.81 & -15 59 54.4 & 11.99 & 9.24 & -12.51$\pm$1.14 & -23.17$\pm$1.0 & 6.0$\pm$1.1$^{(1)}$ & -11.6 & -23.5 & 95 & 38.765\\ 
205666737 & 16 21 57.83 & -15 57 22.1 & 12.13 & 9.15 & -16.07$\pm$2.42 & -20.33$\pm$2.42 & 5.4$\pm$1.0$^{(1)}$ & -11.9 & -23.4 & 84 & 2.726\\ 
205669197 & 16 33 40.19 & -15 56 07.7 & 13.78 & 10.0 & -2.88$\pm$2.15 & -12.41$\pm$2.15 & 5.4$\pm$1.0$^{(1)}$ & -24.8 & -16.6 & 14 & 5.527\\ 
205669675 & 16 32 49.80 & -15 55 53.5 & 13.47 & 9.9 & -10.48$\pm$2.37 & -8.83$\pm$2.37 & 5.6$\pm$1.0$^{(1)}$ & -25.1 & -16.5 & 14 &  \\ 
205671341 & 16 37 56.46 & -15 55 03.0 & 10.43 & 8.92 & -18.79$\pm$0.82 & -11.37$\pm$0.42 & 6.9$\pm$0.2$^{(0)}$ & -23.4 & -16.7 & 27 &  \\ 
205671733 & 16 24 12.95 & -15 54 51.6 & 10.77 & 7.94 & -8.73$\pm$1.83 & -16.96$\pm$1.83 & 9.7$\pm$1.8$^{(1)}$ & -11.8 & -23.5 & 86 & 2.717\\ 
205676247 & 16 35 16.04 & -15 52 35.9 & 10.13 & 8.48 & -11.94$\pm$1.51 & -28.97$\pm$0.76 & 5.6$\pm$0.6$^{(0)}$ & -24.3 & -16.6 & 80 & 1.031\\ 
205682396 & 16 26 28.58 & -15 49 30.3 & 13.94 & 10.32 & -12.21$\pm$2.2 & -20.23$\pm$2.2 & 4.5$\pm$0.8$^{(1)}$ & -27.3 & -16.2 & 53 & 1.772\\ 
205683283 & 16 35 02.71 & -15 49 02.3 & 14.47 & 10.64 & -14.2$\pm$2.15 & -28.45$\pm$2.15 & 4.5$\pm$0.8$^{(1)}$ & -24.4 & -16.5 & 39 & 19.042\\ 
205684752 & 16 34 30.03 & -15 48 17.7 & 16.37 & 11.61 & -12.5$\pm$2.15 & -23.0$\pm$2.15 & 4.4$\pm$0.8$^{(1)}$ & -24.6 & -16.4 & 40 & 37.37\\ 
205684783 & 16 34 09.17 & -15 48 16.9 & 13.33 & 6.57 & -17.09$\pm$2.42 & -29.42$\pm$2.42 & 81.6$\pm$15.0$^{(1)}$ & -24.7 & -16.4 & 47 & 3.309\\ 
205684985 & 16 26 37.08 & -15 48 09.8 & 12.12 & 8.8 & -4.1$\pm$2.42 & -10.85$\pm$2.42 & 8.1$\pm$1.5$^{(1)}$ & -27.3 & -16.2 & 24 &  \\ 
205708570 & 16 26 41.29 & -15 35 53.2 & 12.14 & 8.71 & -10.42$\pm$2.42 & -23.77$\pm$2.42 & 8.9$\pm$1.6$^{(1)}$ & -27.2 & -15.9 & 96 & \\ 
\enddata 
 \tablecomments{stuff} 
 \label{USAmemtab} 
 \end{deluxetable} 


==> USK_memtable.tex <==
\begin{deluxetable}{ccccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Upper Scorpius confirmed members from the literature.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$}  & \colhead{Ref}           \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)}  & \colhead{}           \\ } 
 \startdata 
202522205 & 16 13 17.38 & -29 22 19.9 & 12.39 & 8.91 & -21.4$\pm$2.4 & -25.2$\pm$2.4 & 9.1$\pm$1.7$^{(1)}$ & -13.0 & -24.4 & 88 & $<$2 & 0\\ 
202533810 & 16 15 00.60 & -29 19 34.9 & 12.98 & 9.44 & -15.2$\pm$2.4 & -23.4$\pm$2.4 & 7.8$\pm$1.4$^{(1)}$ & -12.9 & -24.4 & 95 & 5.031 & 1\\ 
202539362 & 16 09 13.64 & -29 18 15.6 & 9.02 & 8.07 & -13.0$\pm$0.1 & -14.1$\pm$0.0 & 6.8$\pm$1.5$^{(0)}$ & -13.3 & -24.3 & 59 & 0.569 & 2\\ 
202552141 & 16 19 16.09 & -29 15 12.7 & 14.18 & 10.44 & -8.0$\pm$2.1 & -21.2$\pm$2.1 & 5.9$\pm$1.1$^{(1)}$ & -12.6 & -24.5 & 87 & 1.822 & 1\\ 
202552587 & 16 22 08.59 & -29 15 06.4 & 13.01 & 9.65 & -14.1$\pm$2.3 & -24.6$\pm$2.3 & 6.1$\pm$1.1$^{(1)}$ & -12.4 & -24.6 & 93 & 1.531 & 1\\ 
202569086 & 16 18 11.07 & -29 11 12.7 & 10.14 & 8.38 & -12.6$\pm$1.9 & -21.9$\pm$0.6 & 6.5$\pm$0.5$^{(0)}$ & -12.7 & -24.5 & 97 & 1.144 & 3\\ 
202640668 & 16 24 18.61 & -28 54 47.6 & 10.82 & 8.33 & -3.9$\pm$1.0 & -14.0$\pm$1.1 & 7.1$\pm$1.3$^{(1)}$ & -12.2 & -24.6 & 23 & 0.763 & 1\\ 
202661711 & 16 23 46.98 & -28 50 02.4 & 10.53 & 8.66 & -10.0$\pm$1.6 & -19.3$\pm$1.0 & 4.7$\pm$0.9$^{(1)}$ & -12.3 & -24.6 & 52 & 1.741 & 4\\ 
202678486 & 16 31 56.68 & -28 46 12.7 & 14.49 & 10.5 & -10.4$\pm$2.1 & -19.9$\pm$2.1 & 7.1$\pm$1.3$^{(1)}$ & -11.7 & -24.8 & 92 & 7.376 & 1\\ 
202679988 & 16 35 11.89 & -28 45 52.1 & 11.91 & 8.99 & -5.9$\pm$2.3 & -19.0$\pm$2.3 & 6.0$\pm$1.1$^{(1)}$ & -11.4 & -24.8 & 77 & 2.948 & 0\\ 
202709862 & 16 12 17.24 & -28 39 08.6 & 15.26 & 11.3 & -14.3$\pm$2.1 & -25.7$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -13.1 & -24.3 & 82 &   & 1\\ 
202724025 & 16 08 56.95 & -28 35 57.4 & 13.54 & 9.63 & -13.7$\pm$2.4 & -23.6$\pm$2.4 & 9.8$\pm$1.8$^{(1)}$ & -13.3 & -24.2 & 94 & $<$2 & 1\\ 
202724532 & 16 34 38.27 & -28 35 50.5 & 13.37 & 9.77 & -10.5$\pm$2.3 & -22.3$\pm$2.3 & 6.5$\pm$1.2$^{(1)}$ & -11.5 & -24.8 & 93 & 5.073 & 1\\ 
202787821 & 16 27 27.66 & -28 21 50.4 & 13.47 & 10.02 & -11.9$\pm$2.1 & -25.9$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -12.0 & -24.6 & 92 & 4.265 & 1\\ 
202790830 & 16 27 33.21 & -28 21 09.8 & 14.07 & 10.51 & -11.7$\pm$2.1 & -24.6$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -12.0 & -24.6 & 81 & 3.893 & 1\\ 
202818196 & 16 13 58.12 & -28 15 09.5 & 7.88 & 6.98 & -13.9$\pm$0.1 & -22.5$\pm$0.0 & 5.9$\pm$0.7$^{(0)}$ & -12.9 & -24.3 & 96 & $<$2 & 2\\ 
202876718 & 16 18 16.16 & -28 02 30.2 & 7.09 & 7.04 & -11.1$\pm$0.0 & -25.2$\pm$0.0 & 7.7$\pm$0.5$^{(0)}$ & -12.6 & -24.4 & 77 &   & 2\\ 
202891090 & 16 23 04.74 & -27 59 25.4 & 13.05 & 9.56 & -6.7$\pm$2.3 & -22.0$\pm$2.3 & 6.7$\pm$1.2$^{(1)}$ & -12.3 & -24.5 & 90 & 2.661 & 1\\ 
202903160 & 16 26 27.36 & -27 56 50.8 & 11.11 & 8.19 & -8.3$\pm$1.2 & -30.5$\pm$1.2 & 9.1$\pm$1.7$^{(1)}$ & -12.0 & -24.6 & 93 & 2.091 & 0\\ 
202904813 & 16 10 26.54 & -27 56 29.4 & 12.92 & 9.57 & -9.5$\pm$2.9 & -20.5$\pm$2.9 & 6.8$\pm$1.3$^{(1)}$ & -13.2 & -24.2 & 91 & 1.222 & 0\\ 
202909059 & 16 12 18.20 & -27 55 34.9 &   &   & -10.4$\pm$0.2 & -23.9$\pm$0.1 &   & -13.0 & -24.3 &   & $<$2 & 2\\ 
202933888 & 16 14 59.18 & -27 50 22.9 & 10.74 & 8.69 & -13.1$\pm$0.8 & -20.5$\pm$0.5 & 6.9$\pm$0.2$^{(0)}$ & -12.8 & -24.3 & 97 & 4.398 & 5\\ 
202947197 & 16 13 47.82 & -27 47 33.9 & 9.13 & 8.01 & -10.6$\pm$0.9 & -20.9$\pm$0.5 & 6.5$\pm$0.3$^{(0)}$ & -12.9 & -24.3 & 97 &  & 1\\ 
202949156 & 16 22 20.93 & -27 47 09.6 & 13.2 & 9.47 & -11.2$\pm$2.3 & -32.2$\pm$2.3 & 8.9$\pm$1.6$^{(1)}$ & -12.3 & -24.5 & 93 & 6.918 & 1\\ 
202957873 & 16 09 00.52 & -27 45 19.4 & 15.42 & 11.24 & -16.8$\pm$2.2 & -28.8$\pm$2.2 & 6.7$\pm$1.2$^{(1)}$ & -13.3 & -24.2 & 94 & 0.772 & 1\\ 
202976647 & 16 26 29.91 & -27 41 20.3 & 8.45 & 7.22 & -11.8$\pm$0.1 & -24.6$\pm$0.1 & 7.6$\pm$0.3$^{(0)}$ & -12.0 & -24.6 & 98 & 2.079 & 6\\ 
203001867 & 16 23 59.02 & -27 36 03.7 & 13.38 & 9.43 & -1.7$\pm$2.4 & -29.7$\pm$2.4 & 11.8$\pm$2.2$^{(1)}$ & -12.2 & -24.5 & 53 & 5.316 & 1\\ 
203015557 & 16 11 50.69 & -27 33 09.8 & 7.93 & 7.18 & -20.2$\pm$0.1 & -34.5$\pm$0.0 & 10.0$\pm$0.4$^{(0)}$ & -13.0 & -24.2 & 100 &   & 2\\ 
203015926 & 16 11 50.63 & -27 33 04.9 & 9.54 & 7.8 & -20.2$\pm$0.2 & -34.6$\pm$0.3 & 8.7$\pm$1.6$^{(1)}$ & -13.0 & -24.2 & 86 &   & 2\\ 
203036210 & 16 29 49.91 & -27 28 50.0 & 10.66 & 8.65 & -9.9$\pm$0.9 & -23.3$\pm$0.9 & 4.9$\pm$0.9$^{(1)}$ & -11.8 & -24.6 & 77 & 3.027 & 4\\ 
203036352 & 16 10 03.94 & -27 28 48.0 & 15.11 & 11.2 & -13.2$\pm$2.1 & -18.9$\pm$2.1 & 5.0$\pm$0.9$^{(1)}$ & -13.2 & -24.2 & 67 & 0.71 & 1\\ 
203042487 & 16 25 23.27 & -27 27 31.5 & 14.61 & 10.72 & -17.3$\pm$2.1 & -25.6$\pm$2.1 & 6.4$\pm$1.2$^{(1)}$ & -12.1 & -24.5 & 91 & 1.276 & 1\\ 
203044910 & 16 30 02.76 & -27 27 00.5 & 13.39 & 9.75 & -17.3$\pm$2.4 & -17.1$\pm$2.4 & 7.2$\pm$1.3$^{(1)}$ & -11.8 & -24.6 & 76 & 7.75 & 1\\ 
203050730 & 16 31 05.79 & -27 25 46.1 & 14.47 & 10.53 & -9.3$\pm$2.1 & -22.7$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -11.7 & -24.6 & 94 & $<$2 & 1\\ 
203065387 & 16 09 51.08 & -27 22 41.9 & 17.23 & 12.45 & -9.3$\pm$2.5 & -27.4$\pm$2.5 & 7.4$\pm$1.4$^{(1)}$ & -13.2 & -24.2 & 95 & 0.543 & 7\\ 
203071614 & 16 25 55.41 & -27 21 24.3 & 13.89 & 9.98 & -10.9$\pm$2.3 & -26.8$\pm$2.3 & 9.0$\pm$1.7$^{(1)}$ & -12.1 & -24.5 & 95 & 0.463 & 1\\ 
203099159 & 16 33 35.04 & -27 15 44.9 & 14.78 & 10.95 & -13.7$\pm$2.1 & -22.2$\pm$2.1 & 4.7$\pm$0.9$^{(1)}$ & -11.5 & -24.7 & 58 & 2.099 & 1\\ 
203117371 & 16 28 46.05 & -27 11 57.5 & 14.27 & 10.4 & -13.7$\pm$2.1 & -22.5$\pm$2.3 & 5.6$\pm$1.0$^{(1)}$ & -11.8 & -24.6 & 89 & 14.151 & 1\\ 
203119637 & 16 17 55.03 & -27 11 30.4 & 13.18 & 9.9 & -12.5$\pm$2.3 & -24.9$\pm$2.3 & 5.1$\pm$0.9$^{(1)}$ & -12.6 & -24.3 & 82 & 6.279 & 1\\ 
203120347 & 16 27 12.52 & -27 11 21.9 & 8.11 & 7.19 & -13.1$\pm$0.1 & -23.6$\pm$0.1 & 9.2$\pm$0.3$^{(0)}$ & -12.0 & -24.5 & 81 &   & 6\\ 
203120753 & 16 35 45.74 & -27 11 16.6 & 13.9 & 10.28 & -11.0$\pm$2.1 & -23.1$\pm$2.1 & 5.6$\pm$1.0$^{(1)}$ & -11.4 & -24.7 & 90 & 5.312 & 1\\ 
203135082 & 16 36 52.88 & -27 08 18.6 & 9.78 & 8.1 & -7.5$\pm$1.7 & -21.2$\pm$1.3 & 6.3$\pm$0.2$^{(0)}$ & -11.3 & -24.7 & 96 & 1.605 & 3\\ 
203143409 & 16 21 59.76 & -27 06 36.6 & 15.19 & 11.26 & -7.7$\pm$2.1 & -22.2$\pm$2.0 & 4.8$\pm$0.9$^{(1)}$ & -12.3 & -24.4 & 64 & 2.066 & 1\\ 
203150950 & 16 21 55.94 & -27 05 03.5 & 15.17 & 10.76 & -2.0$\pm$2.0 & -20.3$\pm$2.0 & 11.1$\pm$2.0$^{(1)}$ & -12.3 & -24.4 & 45 & 2.485 & 1\\ 
203178795 & 16 29 56.63 & -26 59 18.4 & 14.36 & 10.44 & -13.7$\pm$2.1 & -25.1$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -11.8 & -24.6 & 95 & 1.606 & 1\\ 
203181641 & 16 34 05.85 & -26 58 44.2 & 11.64 & 8.78 & -20.0$\pm$2.3 & -22.0$\pm$2.3 & 6.3$\pm$1.2$^{(1)}$ & -11.5 & -24.7 & 77 & 1.304 & 0\\ 
203185083 & 16 34 35.14 & -26 58 03.1 & 14.71 & 10.48 & -8.0$\pm$2.1 & -17.5$\pm$2.1 & 8.5$\pm$1.6$^{(1)}$ & -11.4 & -24.7 & 81 & $<$2& 1\\ 
203189054 & 16 31 15.42 & -26 57 15.1 & 13.89 & 10.25 & -12.9$\pm$2.1 & -19.5$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -11.7 & -24.6 & 69 & 10.753 & 1\\ 
203249626 & 16 01 08.97 & -26 45 10.6 & 14.72 & 10.6 & -15.8$\pm$2.1 & -16.1$\pm$2.1 & 8.0$\pm$1.5$^{(1)}$ & -13.8 & -23.9 & 83 & 2.026 & 1\\ 
203271901 & 16 08 04.10 & -26 40 44.9 & 12.53 & 9.06 & -16.5$\pm$2.3 & -22.1$\pm$2.3 & 8.6$\pm$1.6$^{(1)}$ & -13.3 & -24.1 & 94 & 1.089 & 1\\ 
203278103 & 16 11 16.87 & -26 39 33.1 & 15.29 & 11.42 & -11.7$\pm$2.1 & -27.4$\pm$2.1 & 4.6$\pm$0.8$^{(1)}$ & -13.1 & -24.1 & 55 & 1.695 & 1\\ 
203290460 & 16 04 06.71 & -26 37 07.1 & 13.61 & 9.98 & -6.4$\pm$2.3 & -28.4$\pm$2.3 & 6.2$\pm$1.1$^{(1)}$ & -13.6 & -24.0 & 86 & 2.337 & 1\\ 
203318214 & 16 11 26.02 & -26 31 55.9 & 13.29 & 9.57 & -12.5$\pm$2.3 & -23.5$\pm$2.3 & 7.7$\pm$1.4$^{(1)}$ & -13.0 & -24.1 & 96 & 4.185 & 1\\ 
203341895 & 16 03 25.98 & -26 27 32.2 & 14.82 & 10.77 & -11.2$\pm$2.1 & -18.0$\pm$2.1 & 6.9$\pm$1.3$^{(1)}$ & -13.6 & -23.9 & 89 & 0.981 & 1\\ 
203342257 & 16 15 27.51 & -26 27 28.1 & 15.26 & 11.17 & -14.4$\pm$2.1 & -25.2$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -24.2 & 81 & 3.091 & 1\\ 
203348270 & 16 03 01.77 & -26 26 21.9 & 12.96 & 9.69 & -19.5$\pm$2.3 & -21.9$\pm$2.3 & 5.3$\pm$1.0$^{(1)}$ & -13.6 & -23.9 & 74 & 4.171 & 1\\ 
203348744 & 16 03 02.36 & -26 26 16.4 & 16.7 & 12.15 & -12.0$\pm$2.1 & -24.0$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -13.6 & -23.9 & 54 & 4.174 & 1\\ 
203361837 & 15 58 06.95 & -26 23 46.7 & 13.86 & 10.16 & -10.5$\pm$2.1 & -29.6$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -14.0 & -23.8 & 92 & 7.728 & 1\\ 
203365890 & 16 26 32.77 & -26 22 59.0 &   & 10.49 & -18.6$\pm$3.9 & -27.0$\pm$3.9 & 13.4$\pm$2.5$^{(4)}$ & -12.0 & -24.5 & 79 &  & 1\\ 
203369443 & 16 23 22.72 & -26 22 16.8 & 9.42 & 8.04 & -17.7$\pm$0.1 & -35.2$\pm$0.1 & 10.0$\pm$0.2$^{(0)}$ & -12.2 & -24.4 & 100 & $<$2 & 1\\ 
203369479 & 16 23 22.93 & -26 22 16.4 & 9.42 & 7.92 & -17.7$\pm$0.1 & -35.2$\pm$0.1 & 10.0$\pm$0.2$^{(0)}$ & -12.2 & -24.4 & 100 &  $<$2 & 1\\ 
203370081 & 16 15 36.43 & -26 22 09.2 & 14.86 & 10.24 & -13.7$\pm$2.1 & -46.3$\pm$2.1 & 15.1$\pm$2.8$^{(1)}$ & -12.7 & -24.2 & 10 & 1.91 & 1\\ 
203378869 & 16 23 57.23 & -26 20 24.6 &   & 10.24 & -8.3$\pm$2.8 & -23.0$\pm$2.1 & 11.4$\pm$2.1$^{(4)}$ & -12.2 & -24.4 & 87 & 1.136 & 1\\ 
203385048 & 16 18 16.19 & -26 19 08.1 &   & 10.94 & -4.8$\pm$5.1 & -24.6$\pm$5.1 & 48.7$\pm$9.0$^{(4)}$ & -12.5 & -24.3 & 19 & 1.078 & 7\\ 
203386139 & 16 27 09.51 & -26 18 54.9 & 14.82 & 10.76 & -12.0$\pm$2.1 & -23.7$\pm$2.1 & 6.8$\pm$1.2$^{(1)}$ & -11.9 & -24.5 & 95 & 0.909 & 1\\ 
203397761 & 15 59 01.94 & -26 16 33.0 & 15.34 & 11.26 & -16.1$\pm$2.1 & -23.7$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -13.9 & -23.8 & 94 & 28.409 & 1\\ 
203399155 & 16 23 47.17 & -26 16 15.8 & 8.83 & 7.97 & -9.8$\pm$0.1 & -20.9$\pm$0.1 & 6.3$\pm$0.3$^{(0)}$ & -12.2 & -24.4 & 92 & $<$2 & 2\\ 
203410665 & 16 25 38.48 & -26 13 54.0 & 11.37 & 7.52 & -7.0$\pm$1.1 & -23.7$\pm$1.1 & 17.7$\pm$3.3$^{(1)}$ & -12.0 & -24.4 & 60 &   & 8\\ 
203417549 & 16 21 34.71 & -26 12 26.9 & 12.41 & 8.86 & -11.4$\pm$2.2 & -23.0$\pm$2.2 & 6.6$\pm$1.2$^{(1)}$ & -12.3 & -24.3 & 95 & 3.408 & 9\\ 
203421625 & 16 25 32.74 & -26 11 38.6 & 15.1 & 10.97 & -20.0$\pm$2.1 & -28.6$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -12.0 & -24.4 & 87 & 1.703 & 1\\ 
203433962 & 16 16 17.20 & -26 09 10.2 & 12.22 & 8.72 & -13.0$\pm$2.3 & -27.9$\pm$2.3 & 8.8$\pm$1.6$^{(1)}$ & -12.7 & -24.2 & 96 & 1.966 & 1\\ 
203440253 & 16 25 28.81 & -26 07 53.9 & 13.63 & 9.85 & -13.4$\pm$2.3 & -30.0$\pm$2.3 & 6.8$\pm$1.3$^{(1)}$ & -12.0 & -24.4 & 95 & 6.812 & 1\\ 
203448860 & 16 13 06.28 & -26 06 10.7 & 14.72 & 10.85 & -9.4$\pm$2.1 & -24.2$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -12.9 & -24.1 & 89 & 3.377 & 1\\ 
203462615 & 15 59 38.07 & -26 03 23.5 & 14.29 & 10.25 & -14.5$\pm$2.2 & -26.9$\pm$2.2 & 8.9$\pm$1.6$^{(1)}$ & -13.8 & -23.8 & 96 & 9.842 & 1\\ 
203467084 & 16 23 57.90 & -26 02 29.9 & 13.4 & 9.97 & -15.2$\pm$2.2 & -19.2$\pm$2.2 & 5.0$\pm$0.9$^{(1)}$ & -12.1 & -24.4 & 63 & 1.061 & 1\\ 
203468205 & 16 08 43.41 & -26 02 16.8 & 9.93 & 7.91 & -10.7$\pm$1.5 & -25.3$\pm$1.2 & 6.6$\pm$0.5$^{(0)}$ & -13.2 & -24.0 & 98 & 2.218 & 5\\ 
203475138 & 15 59 08.65 & -26 00 54.5 & 14.57 & 10.76 & -16.4$\pm$2.1 & -22.6$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -13.9 & -23.8 & 86 & 2.12 & 1\\ 
203476597 & 16 25 57.92 & -26 00 37.4 & 11.9 & 8.53 & -6.7$\pm$2.3 & -20.2$\pm$2.3 & 8.6$\pm$1.6$^{(1)}$ & -12.0 & -24.4 & 87 & 3.227 & 1\\ 
203499175 & 16 14 41.26 & -25 56 05.3 & 13.85 & 10.06 & -9.1$\pm$2.1 & -25.9$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -12.8 & -24.2 & 94 & 3.172 & 1\\ 
203499724 & 15 59 49.89 & -25 55 58.5 & 13.23 & 9.61 & -15.9$\pm$1.9 & -26.3$\pm$1.9 & 7.7$\pm$1.4$^{(1)}$ & -13.8 & -23.8 & 96 & 0.624 & 10\\ 
203506352 & 16 25 49.25 & -25 54 37.3 & 13.0 & 9.49 & -18.3$\pm$2.3 & -24.7$\pm$2.3 & 5.6$\pm$1.0$^{(1)}$ & -12.0 & -24.4 & 81 & 2.575 & 1\\ 
203516237 & 16 16 33.45 & -25 52 36.8 & 13.34 & 9.62 & -10.7$\pm$2.3 & -28.1$\pm$2.3 & 7.0$\pm$1.3$^{(1)}$ & -12.7 & -24.2 & 95 & 4.886 & 1\\ 
203517602 & 16 22 22.31 & -25 52 20.1 & 13.55 & 9.44 & -14.8$\pm$2.2 & -23.8$\pm$2.2 & 10.2$\pm$1.9$^{(1)}$ & -12.2 & -24.3 & 93 & 1.14 & 11\\ 
203520293 & 16 16 50.63 & -25 51 46.7 & 8.21 & 7.1 & -11.9$\pm$0.1 & -23.2$\pm$0.0 & 6.6$\pm$0.3$^{(0)}$ & -12.6 & -24.2 & 99 &  $<$2 & 2\\ 
203521205 & 15 57 42.47 & -25 51 35.5 & 14.77 & 10.81 & -12.3$\pm$2.1 & -24.0$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -14.0 & -23.8 & 95 & 0.742 & 1\\ 
203538882 & 16 12 08.15 & -25 47 57.9 & 14.24 & 10.31 & -16.1$\pm$2.1 & -26.5$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -13.0 & -24.1 & 95 & 6.511 & 1\\ 
203553934 & 15 55 29.81 & -25 44 50.0 & 12.82 & 9.14 & -11.0$\pm$2.3 & -29.4$\pm$2.3 & 8.6$\pm$1.6$^{(1)}$ & -14.1 & -23.7 & 94 & 6.235 & 1\\ 
203555168 & 16 24 15.51 & -25 44 34.6 & 13.21 & 9.63 & -15.0$\pm$2.3 & -23.2$\pm$2.3 & 5.9$\pm$1.1$^{(1)}$ & -12.1 & -24.4 & 91 & 17.531 & 1\\ 
203560204 & 16 02 44.48 & -25 43 32.3 & 15.16 & 11.33 & -11.6$\pm$2.1 & -20.7$\pm$2.1 & 4.3$\pm$0.8$^{(1)}$ & -13.6 & -23.9 & 33 & 2.302 & 1\\ 
203565326 & 16 16 18.95 & -25 42 28.9 & 12.75 & 8.71 & -3.9$\pm$2.3 & -31.6$\pm$2.3 & 12.7$\pm$2.3$^{(1)}$ & -12.7 & -24.2 & 57 & 0.793 & 1\\ 
203566940 & 16 02 39.10 & -25 42 07.9 & 11.5 & 9.12 & -21.5$\pm$2.3 & -31.8$\pm$2.3 & 4.7$\pm$0.9$^{(1)}$ & -13.6 & -23.9 & 18 & 3.102 & 5\\ 
203570729 & 15 56 24.92 & -25 41 20.2 & 14.1 & 10.44 & -16.7$\pm$2.1 & -16.2$\pm$2.2 & 5.3$\pm$1.0$^{(1)}$ & -14.0 & -23.7 & 62 & 4.676 & 1\\ 
203576256 & 16 15 19.49 & -25 40 12.0 & 12.76 & 9.12 & -14.4$\pm$2.3 & -24.0$\pm$2.3 & 8.9$\pm$1.6$^{(1)}$ & -12.7 & -24.2 & 95 & 0.699 & 1\\ 
203596697 & 16 10 25.16 & -25 35 59.1 & 14.91 & 10.8 & -9.7$\pm$2.1 & -26.9$\pm$2.1 & 7.3$\pm$1.4$^{(1)}$ & -13.1 & -24.0 & 95 & 0.587 & 3\\ 
203597182 & 16 15 07.02 & -25 35 52.9 &   & 13.0 &   &   &   & -12.7 & -24.2 &   &    & 3\\ 
203598787 & 16 21 09.84 & -25 35 33.0 & 8.37 & 7.18 & -4.7$\pm$2.3 & -20.2$\pm$2.3 & 7.4$\pm$1.4$^{(1)}$ & -12.3 & -24.3 & 82 &   & 3\\ 
203626828 & 16 21 29.55 & -25 29 43.2 & 13.97 & 10.19 & -0.5$\pm$2.7 & -25.4$\pm$2.7 & 6.2$\pm$1.1$^{(1)}$ & -12.3 & -24.3 & 60 & 2.056 & 1\\ 
203628765 & 15 57 16.74 & -25 29 19.3 &   & 8.86 & -14.0$\pm$1.4 & -20.0$\pm$1.4 & 10.0$\pm$1.8$^{(2)}$ & -14.0 & -23.7 & 92 & 0.503 & 1\\ 
203637940 & 16 26 27.75 & -25 27 24.6 & 14.53 & 9.21 & -11.9$\pm$2.3 & -30.5$\pm$2.3 & 14.3$\pm$2.6$^{(1)}$ & -11.9 & -24.4 & 82 & 3.3 & 12\\ 
203640875 & 16 26 28.04 & -25 26 47.8 & 13.08 & 9.1 & -12.7$\pm$2.3 & -29.0$\pm$2.3 & 9.4$\pm$1.7$^{(1)}$ & -11.9 & -24.4 & 95 & 9.103 & 1\\ 
203641931 & 16 11 43.86 & -25 26 35.0 & 11.21 & 8.74 & -12.8$\pm$1.0 & -23.8$\pm$1.0 & 5.7$\pm$1.1$^{(1)}$ & -13.0 & -24.1 & 93 &   & 0\\ 
203642381 & 15 59 52.70 & -25 26 29.2 & 12.75 & 9.72 & -21.1$\pm$2.3 & -24.6$\pm$2.3 & 4.4$\pm$0.8$^{(1)}$ & -13.8 & -23.8 & 17 & 4.487 & 1\\ 
203649927 & 16 24 02.89 & -25 24 54.0 & 9.01 & 6.72 & -9.8$\pm$0.1 & -20.2$\pm$0.1 & 5.1$\pm$0.4$^{(0)}$ & -12.1 & -24.3 & 47 & 2.626 & 2\\ 
203652652 & 16 27 57.93 & -25 24 18.8 & 13.64 & 10.08 & -14.6$\pm$2.1 & -26.2$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -11.8 & -24.4 & 92 & 6.266 & 1\\ 
203655051 & 16 23 32.31 & -25 23 48.6 & 10.68 & 7.7 & 2.5$\pm$3.6 & -26.2$\pm$0.7 &   & -12.1 & -24.3 &   & 2.395 & 13\\ 
203655505 & 16 00 52.72 & -25 23 42.8 & 14.07 & 10.35 & -14.9$\pm$2.1 & -21.3$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -13.7 & -23.8 & 88 & 7.128 & 1\\ 
203660895 & 16 08 43.67 & -25 22 36.6 & 8.57 & 7.25 & -12.3$\pm$0.1 & -23.4$\pm$0.0 & 7.2$\pm$0.4$^{(0)}$ & -13.2 & -24.0 & 98 &   & 2\\ 
203664569 & 16 16 33.44 & -25 21 50.7 & 13.8 & 10.13 & -14.4$\pm$2.1 & -24.7$\pm$2.1 & 5.0$\pm$0.9$^{(1)}$ & -12.6 & -24.2 & 78 & & 3\\ 
203667805 & 15 55 06.25 & -25 21 10.2 & 11.49 & 8.51 & -16.1$\pm$2.3 & -22.0$\pm$2.3 & 7.5$\pm$1.4$^{(1)}$ & -14.1 & -23.7 & 95 & 3.906 & 10\\ 
203675097 & 15 55 50.98 & -25 19 39.4 & 14.54 & 10.7 & -12.1$\pm$2.1 & -24.2$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -14.1 & -23.7 & 91 & 2.869 & 1\\ 
203678376 & 16 12 55.89 & -25 18 58.1 & 14.83 & 10.78 & -13.3$\pm$2.1 & -24.3$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -12.9 & -24.1 & 95 &   & 3\\ 
203685806 & 16 21 48.53 & -25 17 26.6 & 13.73 & 9.97 & -14.0$\pm$2.2 & -20.8$\pm$2.2 & 5.9$\pm$1.1$^{(1)}$ & -12.3 & -24.3 & 90 & 3.786 & 1\\ 
203690414 & 16 01 14.00 & -25 16 28.3 & 14.28 & 10.42 & -13.2$\pm$2.1 & -21.4$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -13.7 & -23.8 & 94 & 1.817 & 1\\ 
203703016 & 16 14 52.42 & -25 13 52.5 & 14.76 & 10.45 & -16.4$\pm$2.1 & -30.5$\pm$2.1 & 8.6$\pm$1.6$^{(1)}$ & -12.7 & -24.1 & 95 & 4.855 & 1\\ 
203709312 & 15 58 53.53 & -25 12 33.5 & 12.92 & 9.65 & -25.1$\pm$2.3 & -32.8$\pm$2.3 & 5.7$\pm$1.0$^{(1)}$ & -13.9 & -23.7 & 41 & 3.7 & 10\\ 
203710077 & 15 55 48.82 & -25 12 24.0 & 10.09 & 8.29 & -14.7$\pm$1.7 & -24.1$\pm$0.5 & 7.5$\pm$0.5$^{(0)}$ & -14.1 & -23.7 & 98 & 3.733 & 10\\ 
203710387 & 16 16 30.68 & -25 12 20.2 &   & 11.91 & -11.8$\pm$5.1 & -28.0$\pm$5.1 & 27.2$\pm$5.0$^{(4)}$ & -12.6 & -24.2 & 36 & 2.555 & 3\\ 
203710635 & 15 55 48.40 & -25 12 17.3 & 13.71 & 10.0 &   & 124.2$\pm$2.2 &   & -14.1 & -23.7 &   & 3.733 & 14\\ 
203712541 & 16 01 26.64 & -25 11 54.6 & 7.67 & 6.89 & -11.6$\pm$0.1 & -25.4$\pm$0.0 & 6.0$\pm$0.4$^{(0)}$ & -13.7 & -23.8 & 100 &   & 2\\ 
203713606 & 16 26 34.96 & -25 11 40.9 & 13.47 & 9.99 & -10.2$\pm$2.3 & -27.8$\pm$2.3 & 4.9$\pm$0.9$^{(1)}$ & -11.9 & -24.4 & 76 & 4.821 & 1\\ 
203716047 & 16 10 57.92 & -25 11 10.2 & 13.82 & 9.93 & -15.0$\pm$2.3 & -27.5$\pm$2.3 & 8.1$\pm$1.5$^{(1)}$ & -13.0 & -24.0 & 96 & 0.855 & 3\\ 
203721488 & 16 09 05.31 & -25 10 00.9 & 14.91 & 10.61 & -16.7$\pm$2.1 & -28.5$\pm$2.1 & 9.3$\pm$1.7$^{(1)}$ & -13.1 & -24.0 & 95 & 0.747 & 3\\ 
203723257 & 16 03 54.05 & -25 09 39.4 & 15.41 & 11.38 & -10.3$\pm$2.1 & -32.4$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -13.5 & -23.9 & 69 & 15.645 & 1\\ 
203725791 & 16 01 29.03 & -25 09 07.0 & 14.54 & 10.08 & -16.1$\pm$2.1 & -35.2$\pm$2.1 & 11.1$\pm$2.0$^{(1)}$ & -13.7 & -23.8 & 85 & 14.983 & 1\\ 
203726323 & 16 13 48.81 & -25 09 00.7 & 17.18 & 12.51 & -4.4$\pm$2.5 & -25.7$\pm$2.5 & 4.4$\pm$0.8$^{(1)}$ & -12.8 & -24.1 & 22 & 1.022 & 15\\ 
203747590 & 16 14 53.93 & -25 04 30.5 & 15.38 & 11.25 & -11.4$\pm$2.1 & -30.0$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -12.7 & -24.1 & 85 & 1.04 & 3\\ 
203749770 & 16 27 12.74 & -25 04 01.8 & 13.32 & 9.38 & -3.4$\pm$2.3 & -27.1$\pm$2.3 & 8.0$\pm$1.5$^{(1)}$ & -11.9 & -24.4 & 86 & 2.495 & 1\\ 
203750949 & 16 16 22.94 & -25 03 46.8 & 8.37 & 7.23 & -11.9$\pm$0.1 & -21.4$\pm$0.1 & 5.2$\pm$0.4$^{(0)}$ & -12.6 & -24.1 & 76 & $<$2 & 2\\ 
203751997 & 16 27 45.23 & -25 03 32.9 & 15.53 & 11.45 & -7.5$\pm$2.1 & -26.5$\pm$2.1 & 4.9$\pm$0.9$^{(1)}$ & -11.8 & -24.4 & 69 & 2.736 & 16\\ 
203754361 & 16 11 07.44 & -25 03 01.7 & 13.44 & 9.62 & -12.9$\pm$2.3 & -22.9$\pm$2.3 & 8.6$\pm$1.6$^{(1)}$ & -13.0 & -24.0 & 95 & 2.221 & 3\\ 
203756600 & 16 10 18.88 & -25 02 32.5 & 15.43 & 11.26 & -10.8$\pm$1.8 & -23.0$\pm$0.9 & 6.6$\pm$0.3$^{(0)}$ & -13.0 & -24.0 & 98 & 18.753 & 14\\ 
203756781 & 16 10 19.19 & -25 02 30.3 & 11.26 & 8.36 & -10.8$\pm$1.8 & -23.0$\pm$0.9 & 6.6$\pm$0.3$^{(0)}$ & -13.0 & -24.0 & 98 & 18.779 & 5\\ 
203760219 & 16 13 02.35 & -25 01 46.0 & 12.9 & 9.43 & -8.7$\pm$1.4 & -21.0$\pm$1.4 & 6.6$\pm$1.2$^{(1)}$ & -12.9 & -24.1 & 92 & 2.029 & 3\\ 
203760606 & 16 13 01.88 & -25 01 41.1 & 15.64 & 11.7 & -17.0$\pm$2.7 & -33.6$\pm$2.7 & 3.6$\pm$0.7$^{(1)}$ & -12.9 & -24.1 &   & $<$2 & 3\\ 
203761347 & 16 24 21.32 & -25 01 31.5 & 8.06 & 6.19 & -10.8$\pm$0.1 & -22.4$\pm$0.1 & 6.5$\pm$0.3$^{(0)}$ & -12.1 & -24.3 & 98 &   & 2\\ 
203764923 & 16 15 06.20 & -25 00 46.1 & 18.92 & 10.07 & -16.1$\pm$12.8 & -22.7$\pm$11.3 & 7.4$\pm$1.4$^{(1)}$ & -12.7 & -24.1 & 85 & 0.841 & 1\\ 
203768482 & 16 16 54.27 & -24 59 59.6 & 15.04 & 10.83 & -10.1$\pm$2.1 & -21.7$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -12.6 & -24.1 & 94 & 1.627 & 3\\ 
203770135 & 16 24 56.53 & -24 59 38.1 & 14.98 & 11.62 & -7.4$\pm$2.0 & -4.7$\pm$2.0 &   & -12.0 & -24.3 &   &  & 16\\ 
203770366 & 16 15 05.25 & -24 59 35.1 &   & 11.48 & -7.2$\pm$4.0 & -21.7$\pm$4.0 & 34.1$\pm$6.3$^{(4)}$ & -12.7 & -24.1 & 22 & 1.814 & 17\\ 
203770559 & 16 25 02.12 & -24 59 32.4 &   & 9.22 & 2.9$\pm$4.8 & -14.9$\pm$11.0 &   & -12.0 & -24.3 &   & 12.422 & 16\\ 
203770673 & 16 14 59.29 & -24 59 30.8 & 15.28 & 11.09 & -8.6$\pm$2.1 & -31.2$\pm$2.1 & 5.7$\pm$1.0$^{(1)}$ & -12.7 & -24.1 & 83 & 2.29 & 3\\ 
203771564 & 16 16 25.17 & -24 59 19.5 & 7.85 & 7.03 & -12.1$\pm$0.1 & -21.9$\pm$0.0 & 6.3$\pm$0.3$^{(0)}$ & -12.6 & -24.1 & 97 & $<$2 & 2\\ 
203774126 & 16 29 54.60 & -24 58 46.1 & 7.82 & 7.31 & -14.8$\pm$0.0 & -25.4$\pm$0.0 &   & -11.7 & -24.4 &   &   & 12\\ 
203775036 & 16 12 34.59 & -24 58 34.2 &   & 11.04 & -12.9$\pm$4.0 & -20.9$\pm$4.0 & 4.5$\pm$0.8$^{(4)}$ & -12.9 & -24.0 & 35 & 0.749 & 17\\ 
203777800 & 16 13 56.63 & -24 57 56.8 & 14.05 & 10.15 & -14.6$\pm$2.1 & -26.4$\pm$2.1 & 7.0$\pm$1.3$^{(1)}$ & -12.8 & -24.1 & 96 & 2.278 & 1\\ 
203779568 & 16 28 19.22 & -24 57 34.1 & 14.7 & 9.93 & -5.2$\pm$2.3 & -20.9$\pm$2.3 & 11.8$\pm$2.2$^{(1)}$ & -11.8 & -24.4 & 74 & 12.038 & 16\\ 
203781195 & 16 27 48.00 & -24 57 13.4 &   & 12.12 &   & 150.0$\pm$8.1 &   & -11.8 & -24.4 &   & 0.414 & 18\\ 
203782748 & 16 29 36.25 & -24 56 52.8 & 17.04 & 12.49 & 4.9$\pm$2.4 & -29.7$\pm$2.2 &   & -11.7 & -24.4 &   &  & 17\\ 
203783190 & 16 24 06.34 & -24 56 47.0 & 11.93 & 8.28 & -16.1$\pm$2.2 & -23.1$\pm$2.2 & 10.4$\pm$1.9$^{(1)}$ & -12.1 & -24.3 & 91 & 0.818 & 13\\ 
203785905 & 16 28 13.86 & -24 56 11.3 & 15.23 & 9.7 & -7.8$\pm$2.3 & -23.2$\pm$2.3 & 14.1$\pm$2.6$^{(1)}$ & -11.8 & -24.4 & 78 & 8.755 & 16\\ 
203786695 & 16 24 59.74 & -24 56 00.8 &   & 9.44 & 0.9$\pm$5.5 & -18.3$\pm$5.5 &   & -12.0 & -24.3 &   & 22.028 & 16\\ 
203787831 & 16 25 14.31 & -24 55 45.0 & 16.38 & 10.92 & 3.8$\pm$2.0 & -5.3$\pm$2.1 &   & -12.0 & -24.3 &   & 4.865 & 13\\ 
203788687 & 16 08 05.22 & -24 55 33.2 & 8.99 & 7.43 & -14.2$\pm$1.0 & -24.0$\pm$0.6 & 6.7$\pm$0.2$^{(0)}$ & -13.2 & -23.9 & 98 & 0.891 & 4\\ 
203788910 & 16 29 33.97 & -24 55 30.4 & 11.56 & 8.53 & -15.4$\pm$2.3 & -22.4$\pm$2.3 & 7.8$\pm$1.4$^{(1)}$ & -11.7 & -24.4 & 94 & 2.267 & 16\\ 
203791768 & 16 27 18.35 & -24 54 53.5 & 14.48 & 10.06 & -6.3$\pm$2.1 & -23.1$\pm$2.1 & 4.6$\pm$0.8$^{(1)}$ & -11.9 & -24.4 & 47 & 2.853 & 19\\ 
203793391 & 16 27 28.73 & -24 54 31.8 & 15.63 & 11.69 & -14.9$\pm$2.1 & -27.6$\pm$2.1 & 4.0$\pm$0.7$^{(1)}$ & -11.9 & -24.4 & 9 & 0.881 & 16\\ 
203793637 & 16 14 12.59 & -24 54 28.8 & 13.17 & 9.89 & -13.3$\pm$2.3 & -20.2$\pm$2.3 & 4.8$\pm$0.9$^{(1)}$ & -12.8 & -24.1 & 65 & 7.997 & 1\\ 
203795359 & 16 28 29.92 & -24 54 06.2 & 20.39 & 14.0 &   &   &   & -11.8 & -24.4 &   &  & 20\\ 
203797163 & 16 28 00.12 & -24 53 42.3 &   & 9.65 & 6.3$\pm$2.9 & -11.4$\pm$3.1 &   & -11.8 & -24.4 &   & 14.796 & 16\\ 
203798606 & 16 28 03.36 & -24 53 23.7 &   & 10.49 & -2.1$\pm$3.9 & -29.9$\pm$3.9 & 60.6$\pm$11.2$^{(4)}$ & -11.8 & -24.4 & 11 & 2.302 & 16\\ 
203799762 & 16 14 03.80 & -24 53 08.9 & 13.46 & 10.02 & -11.1$\pm$2.1 & -24.9$\pm$2.1 & 4.9$\pm$0.9$^{(1)}$ & -12.8 & -24.1 & 79 & 6.704 & 1\\ 
203801323 & 16 25 58.93 & -24 52 48.4 &   & 10.24 & -2.5$\pm$4.0 & -27.8$\pm$4.0 & 68.3$\pm$12.6$^{(4)}$ & -12.0 & -24.3 & 24 & 1.255 & 16\\ 
203802752 & 16 29 34.41 & -24 52 29.3 & 10.34 & 8.88 & -36.4$\pm$2.8 &   &   & -11.7 & -24.4 &   &  & 16\\ 
203803109 & 16 26 43.50 & -24 52 24.8 & 15.56 & 10.37 & -4.0$\pm$2.1 & 2.1$\pm$2.1 &   & -11.9 & -24.3 &   &  & 16\\ 
203806417 & 16 29 03.93 & -24 51 41.4 &   & 10.74 & -18.7$\pm$5.0 & -25.4$\pm$5.0 & 52.7$\pm$9.7$^{(4)}$ & -11.8 & -24.4 & 18 & 8.092 & 16\\ 
203806628 & 16 27 15.11 & -24 51 38.8 & 13.57 & 9.39 & 8.6$\pm$2.5 & -31.0$\pm$2.3 &   & -11.9 & -24.3 &   & 2.607 & 19\\ 
203806838 & 16 27 36.61 & -24 51 36.1 &   & 14.95 &   &   &   & -11.9 & -24.4 &   &  & 20\\ 
203807051 & 16 27 14.50 & -24 51 33.6 & 14.6 & 10.38 & -7.9$\pm$2.1 & -22.0$\pm$2.1 & 7.7$\pm$1.4$^{(1)}$ & -11.9 & -24.3 & 93 & 2.607 & 19\\ 
203807162 & 16 25 49.65 & -24 51 32.0 & 11.98 & 8.78 & -10.1$\pm$2.3 & -26.2$\pm$2.3 & 7.0$\pm$1.3$^{(1)}$ & -12.0 & -24.3 & 96 & 11.228 & 16\\ 
203809317 & 16 17 29.95 & -24 51 03.2 & 14.03 & 9.79 & -3.9$\pm$2.3 & -24.4$\pm$2.3 & 9.6$\pm$1.8$^{(1)}$ & -12.5 & -24.1 & 80 & 6.474 & 1\\ 
203809634 & 16 17 26.15 & -24 50 59.2 & 13.97 & 9.85 & -11.6$\pm$2.3 & -22.5$\pm$2.3 & 9.0$\pm$1.7$^{(1)}$ & -12.5 & -24.1 & 95 & 2.968 & 1\\ 
203810647 & 16 28 12.54 & -24 50 45.3 & 15.25 & 10.38 & -29.5$\pm$2.3 & -17.3$\pm$2.3 & 7.1$\pm$1.3$^{(1)}$ & -11.8 & -24.4 & 3 &   & 16\\ 
203810698 & 16 28 12.28 & -24 50 44.6 & 15.25 & 9.56 & -29.5$\pm$2.3 & -17.3$\pm$2.3 & 23.5$\pm$4.3$^{(1)}$ & -11.8 & -24.4 &   & 3.992 & 16\\ 
203812608 & 16 22 24.42 & -24 50 18.8 &   & 7.73 & -3.1$\pm$5.5 & -8.0$\pm$5.5 & 324.6$\pm$59.8$^{(4)}$ & -12.2 & -24.2 & 2 &  & 21\\ 
203814494 & 15 58 34.87 & -24 49 53.4 &   & 5.65 & -12.3$\pm$0.3 & -24.7$\pm$0.2 & 5.9$\pm$0.2$^{(0)}$ & -13.9 & -23.7 & 92 & $<$2 & 2\\ 
203815783 & 16 08 58.71 & -24 49 36.3 & 15.34 & 11.41 & -10.9$\pm$2.1 & -24.5$\pm$2.1 & 4.6$\pm$0.8$^{(1)}$ & -13.1 & -24.0 & 61 & 1.562 & 17\\ 
203820868 & 16 28 22.96 & -24 48 28.9 &   & 10.95 & -13.5$\pm$5.3 & -13.1$\pm$5.3 & 63.4$\pm$11.7$^{(4)}$ & -11.8 & -24.4 & 9 & 1.45 & 16\\ 
203821589 & 16 27 59.97 & -24 48 19.3 &   & 9.27 & -1.1$\pm$5.4 & -30.7$\pm$5.4 & 122.8$\pm$22.6$^{(4)}$ & -11.8 & -24.4 & 52 & 0.668 & 19\\ 
203822485 & 16 27 22.96 & -24 48 07.1 & 14.4 & 9.39 & -6.4$\pm$2.3 & -30.3$\pm$2.3 & 14.5$\pm$2.7$^{(1)}$ & -11.9 & -24.3 & 70 & & 19\\ 
203822946 & 16 25 18.91 & -24 48 00.7 &   & 10.32 & -18.6$\pm$5.2 & -19.8$\pm$5.2 & 83.0$\pm$15.3$^{(4)}$ & -12.0 & -24.3 & 30 & 0.581 & 16\\ 
203824153 & 16 28 54.07 & -24 47 44.2 &   & 8.9 & -14.6$\pm$6.8 & -16.4$\pm$6.7 & 166.0$\pm$30.6$^{(4)}$ & -11.8 & -24.4 & 53 & 24.167 & 19\\ 
203824768 & 16 25 50.56 & -24 47 36.0 & 14.66 & 9.12 & -10.8$\pm$2.3 & -20.2$\pm$2.3 & 20.1$\pm$3.7$^{(1)}$ & -12.0 & -24.3 & 51 & 7.044 & 16\\ 
203831587 & 16 25 10.93 & -24 46 03.8 &   & 11.51 & 11.6$\pm$5.6 & -80.7$\pm$5.6 &   & -12.0 & -24.3 &   & 1.934 & 16\\ 
203833873 & 16 26 58.43 & -24 45 31.8 & 14.45 & 7.55 & -9.4$\pm$8.8 & -3.4$\pm$8.8 & 35.9$\pm$6.6$^{(1)}$ & -11.9 & -24.3 & 2 & 3.108 & 16\\ 
203833980 & 16 08 36.48 & -24 45 30.3 & 14.39 & 10.73 & -21.7$\pm$2.1 & -28.5$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -13.2 & -23.9 & 47 & 2.821 & 17\\ 
203834337 & 16 01 51.49 & -24 45 25.0 & 11.45 & 8.48 & -13.1$\pm$2.3 & -24.0$\pm$2.3 & 7.3$\pm$1.3$^{(1)}$ & -13.6 & -23.8 & 96 & 4.65 & 10\\ 
203837143 & 16 09 49.55 & -24 44 46.9 & 13.62 & 10.07 & -9.9$\pm$2.1 & -23.9$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -13.1 & -24.0 & 89 & 8.921 & 1\\ 
203837701 & 16 26 21.90 & -24 44 39.8 & 16.93 & 10.86 & -9.1$\pm$2.8 & -21.5$\pm$2.8 & 18.4$\pm$3.4$^{(1)}$ & -11.9 & -24.3 & 58 & 2.62 & 16\\ 
203837965 & 16 15 55.08 & -24 44 36.5 &   & 12.28 & -19.2$\pm$5.5 & -15.3$\pm$5.5 & 24.1$\pm$4.4$^{(4)}$ & -12.6 & -24.1 & 15 & 2.012 & 18\\ 
203838456 & 16 26 47.05 & -24 44 29.9 &   & 10.56 & -14.4$\pm$5.3 & -32.4$\pm$5.3 & 77.5$\pm$14.3$^{(4)}$ & -11.9 & -24.3 & 39 & 3.504 & 16\\ 
203839698 & 15 57 47.57 & -24 44 12.2 & 16.19 & 12.05 & -15.0$\pm$2.1 & -22.3$\pm$2.1 & 4.0$\pm$0.7$^{(1)}$ & -13.9 & -23.7 & 14 & 0.967 & 17\\ 
203840786 & 16 16 13.29 & -24 43 57.2 & 13.84 & 9.71 & -8.6$\pm$2.4 & -18.6$\pm$2.4 & 8.9$\pm$1.6$^{(1)}$ & -12.6 & -24.1 & 87 & 2.388 & 3\\ 
203842174 & 16 09 30.34 & -24 43 37.8 & 13.6 & 9.5 & -14.1$\pm$2.3 & -22.1$\pm$2.3 & 10.6$\pm$2.0$^{(1)}$ & -13.1 & -24.0 & 93 & 2.43 & 3\\ 
203842665 & 16 13 38.40 & -24 43 31.2 & 14.29 & 10.35 & -14.7$\pm$2.1 & -25.2$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -12.8 & -24.1 & 95 & 1.295 & 1\\ 
203843009 & 16 07 55.67 & -24 43 26.8 & 17.26 & 12.71 & -12.6$\pm$2.5 & -22.5$\pm$2.5 & 3.5$\pm$0.6$^{(1)}$ & -13.2 & -23.9 &   & & 17\\ 
203843841 & 16 27 39.83 & -24 43 15.1 &   & 8.99 &   &   &   & -11.8 & -24.3 &   & 2.268 & 22\\ 
203843900 & 16 26 44.33 & -24 43 14.0 &   & 9.57 & 10.0$\pm$4.4 & -23.8$\pm$4.3 &   & -11.9 & -24.3 &   & 0.766 & 19\\ 
203843911 & 16 26 23.70 & -24 43 13.8 & 12.6 & 7.85 & 4.2$\pm$2.3 & -35.4$\pm$2.3 &   & -11.9 & -24.3 &   & 8.903 & 19\\ 
203844249 & 16 25 26.87 & -24 43 09.0 & 12.48 & 8.66 & 0.2$\pm$2.3 & -24.9$\pm$2.3 &   & -12.0 & -24.3 &   & 2.637 & 16\\ 
203844856 & 16 27 04.52 & -24 42 59.7 & 16.35 & 9.84 & -7.7$\pm$2.3 & -26.1$\pm$2.3 & 20.2$\pm$3.7$^{(1)}$ & -11.9 & -24.3 & 55 & 3.538 & 16\\ 
203848252 & 16 27 04.56 & -24 42 14.0 & 17.11 & 9.81 & 0.0$\pm$3.1 & -26.5$\pm$3.1 &   & -11.9 & -24.3 &   & 14.43 & 16\\ 
203849021 & 16 26 48.11 & -24 42 03.3 &   & 10.66 & -13.0$\pm$5.0 & -25.8$\pm$5.0 & 74.8$\pm$13.8$^{(4)}$ & -11.9 & -24.3 & 52 & 3.934 & 16\\ 
203849738 & 16 09 52.88 & -24 41 53.5 &   & 10.93 & -17.4$\pm$4.0 & -24.8$\pm$4.0 & 9.4$\pm$1.7$^{(4)}$ & -13.1 & -24.0 & 93 & 0.31 & 1\\ 
203850058 & 16 27 06.60 & -24 41 48.8 & 16.7 & 10.77 & -4.0$\pm$2.5 & -24.0$\pm$2.5 & 16.0$\pm$2.9$^{(1)}$ & -11.9 & -24.3 & 50 & 2.855 & 19\\ 
203850425 & 16 27 21.47 & -24 41 43.1 &   & 8.48 &   &   &   & -11.9 & -24.3 &   & 3.904 & 22\\ 
203850605 & 16 27 19.49 & -24 41 40.4 & 11.97 & 8.41 & -7.9$\pm$2.3 & -26.7$\pm$2.3 & 11.1$\pm$2.0$^{(1)}$ & -11.9 & -24.3 & 90 & 3.506 & 19\\ 
203851147 & 16 07 58.77 & -24 41 31.9 & 13.94 & 9.83 & -3.0$\pm$2.3 & -24.9$\pm$2.3 & 11.1$\pm$2.1$^{(1)}$ & -13.2 & -23.9 & 61 & 5.345 & 3\\ 
203851860 & 16 29 44.29 & -24 41 21.8 & 13.44 & 9.14 & -16.1$\pm$2.3 & -23.1$\pm$2.3 & 18.3$\pm$3.4$^{(1)}$ & -11.7 & -24.4 & 60 & 3.519 & 21\\ 
203851946 & 16 11 17.44 & -24 41 20.4 & 14.26 & 10.44 & -11.0$\pm$2.1 & -26.7$\pm$2.1 & 6.1$\pm$1.1$^{(1)}$ & -13.0 & -24.0 & 94 & 1.914 & 1\\ 
203852282 & 16 27 33.11 & -24 41 15.3 &   & 7.81 & -9.8$\pm$6.7 & -29.3$\pm$6.7 & 388.7$\pm$71.6$^{(4)}$ & -11.8 & -24.3 & 82 &  & 23\\ 
203853244 & 16 01 47.70 & -24 41 01.1 & 17.38 & 13.01 & -9.8$\pm$2.5 & -25.1$\pm$2.5 & 3.8$\pm$0.7$^{(1)}$ & -13.6 & -23.8 & 6 & 0.649 & 18\\ 
203853992 & 16 27 52.08 & -24 40 50.3 & 14.11 & 8.13 & -3.0$\pm$2.3 & -24.0$\pm$2.3 & 43.4$\pm$8.0$^{(1)}$ & -11.8 & -24.3 & 14 & 1.551 & 19\\ 
203854810 & 16 00 52.84 & -24 40 38.4 & 14.11 &   & -10.4$\pm$2.1 & -35.7$\pm$2.1 &   & -13.7 & -23.8 &   &   & 3\\ 
203856244 & 16 26 41.22 & -24 40 17.7 &   & 9.27 & -21.8$\pm$7.6 & -28.3$\pm$7.8 & 119.8$\pm$22.1$^{(4)}$ & -11.9 & -24.3 & 50 & 4.07 & 19\\ 
203857149 & 16 24 48.03 & -24 40 05.1 &   & 11.36 & -86.3$\pm$5.3 &   &   & -12.0 & -24.3 &   & 5.405 & 16\\ 
203857404 & 16 27 57.83 & -24 40 01.8 &   & 9.87 & 109.4$\pm$8.1 & 97.2$\pm$8.1 &   & -11.8 & -24.3 &   & 0.77 & 22\\ 
203860070 & 16 27 26.49 & -24 39 23.1 &   & 9.95 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203860592 & 16 27 39.43 & -24 39 15.5 &   & 8.46 & -1.5$\pm$5.4 & -34.5$\pm$5.4 & 271.9$\pm$50.1$^{(4)}$ & -11.8 & -24.3 & 65 & 6.227 & 19\\ 
203860653 & 16 25 50.52 & -24 39 14.8 & 13.47 & 8.33 & 2.7$\pm$2.3 & -20.8$\pm$2.3 &   & -12.0 & -24.3 &   & 3.556 & 16\\ 
203861461 & 16 26 37.81 & -24 39 03.2 & 20.04 & 12.85 &   &   &   & -11.9 & -24.3 &   &  & 20\\ 
203862309 & 16 27 42.70 & -24 38 50.6 & 18.8 & 10.54 & -4.4$\pm$3.9 & -27.1$\pm$3.9 & 7.8$\pm$1.4$^{(1)}$ & -11.8 & -24.3 & 90 & 4.346 & 19\\ 
203863066 & 16 27 38.63 & -24 38 39.2 & 18.99 & 11.08 &   &   &   & -11.8 & -24.3 &   & 4.107 & 24\\ 
203863067 & 16 17 30.32 & -24 38 39.2 & 13.53 & 9.73 & -11.0$\pm$2.3 & -25.6$\pm$2.3 & 6.7$\pm$1.2$^{(1)}$ & -12.5 & -24.1 & 95 & 6.072 & 1\\ 
203863479 & 16 27 35.26 & -24 38 33.4 &   & 9.67 & -5.2$\pm$6.7 & -30.8$\pm$6.7 & 106.1$\pm$19.6$^{(4)}$ & -11.8 & -24.3 & 48 & 1.627 & 19\\ 
203863529 & 16 02 14.90 & -24 38 32.6 &   & 11.15 & -17.9$\pm$4.0 & -31.1$\pm$4.0 & 6.2$\pm$1.1$^{(4)}$ & -13.6 & -23.8 & 90 & 0.254 & 1\\ 
203863576 & 16 23 54.71 & -24 38 32.0 & 17.56 & 11.92 & 1.7$\pm$2.5 & -21.7$\pm$2.5 &   & -12.1 & -24.3 &   & 1.765 & 18\\ 
203864032 & 16 26 48.98 & -24 38 25.2 & 19.18 &   & -6.0$\pm$3.1 & -17.7$\pm$3.1 &   & -11.9 & -24.3 &   &   & 16\\ 
203867167 & 16 25 47.68 & -24 37 39.5 & 15.61 & 10.38 & -6.7$\pm$2.1 & -22.5$\pm$2.1 & 13.0$\pm$2.4$^{(1)}$ & -12.0 & -24.3 & 78 & 3.169 & 13\\ 
203867961 & 16 26 19.52 & -24 37 27.4 & 14.62 & 10.1 & -2.9$\pm$2.1 & -22.7$\pm$2.1 & 12.0$\pm$2.2$^{(1)}$ & -11.9 & -24.3 & 61 & 3.25 & 16\\ 
203867975 & 16 27 02.34 & -24 37 27.2 &   & 8.06 &   &   &   & -11.9 & -24.3 &   &  & 22\\ 
203868595 & 16 27 09.43 & -24 37 18.8 &   & 7.14 &   &   &   & -11.9 & -24.3 &   & 2.207 & 25\\ 
203870022 & 16 27 38.32 & -24 36 58.6 & 17.17 & 8.27 & -7.5$\pm$3.1 & -25.9$\pm$3.1 & 16.5$\pm$3.0$^{(1)}$ & -11.8 & -24.3 & 68 & 12.561 & 19\\ 
203870058 & 16 28 16.51 & -24 36 58.0 &   & 9.32 & -11.6$\pm$5.4 & -16.3$\pm$5.4 & 155.0$\pm$28.6$^{(4)}$ & -11.8 & -24.3 & 52 & 2.891 & 19\\ 
203871153 & 16 23 12.59 & -24 36 41.7 & 13.94 & 8.57 & -3.0$\pm$2.2 & -7.3$\pm$2.2 & 23.3$\pm$4.3$^{(1)}$ & -12.1 & -24.2 &   & 48.424 & 21\\ 
203873262 & 16 21 15.65 & -24 36 11.9 & 15.08 & 11.59 & -28.7$\pm$2.1 & -21.5$\pm$2.1 & 3.0$\pm$0.6$^{(1)}$ & -12.3 & -24.2 &   & 4.852 & 17\\ 
203873374 & 16 29 35.09 & -24 36 10.4 &   & 9.68 & -7.3$\pm$5.4 & -11.6$\pm$5.4 & 104.0$\pm$19.2$^{(4)}$ & -11.7 & -24.4 & 9 & 2.063 & 21\\ 
203874287 & 16 26 59.05 & -24 35 56.9 &   & 11.82 &   &   &   & -11.9 & -24.3 &   &  & 22\\ 
203875175 & 16 28 24.80 & -24 35 43.4 &   & 11.3 & -16.6$\pm$3.9 & -33.5$\pm$3.9 & 41.0$\pm$7.6$^{(4)}$ & -11.8 & -24.4 & 18 & 1.911 & 19\\ 
203876392 & 16 13 10.00 & -24 35 25.6 & 14.97 & 10.96 & -9.9$\pm$2.1 & -27.7$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -12.8 & -24.0 & 91 & 1.902 & 1\\ 
203877533 & 16 24 39.70 & -24 35 09.2 & 17.24 & 10.29 & -6.5$\pm$2.7 & -21.0$\pm$2.7 & 16.0$\pm$2.9$^{(1)}$ & -12.0 & -24.3 & 58 & 1.627 & 16\\ 
203878369 & 16 10 09.88 & -24 34 56.7 & 6.66 & 6.55 & -19.8$\pm$0.0 & -34.2$\pm$0.0 & 9.3$\pm$0.5$^{(0)}$ & -13.0 & -24.0 & 100 &   & 2\\ 
203878861 & 16 27 12.13 & -24 34 49.1 &   & 11.49 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203878912 & 16 26 44.20 & -24 34 48.3 &   & 11.6 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203881218 & 16 13 44.91 & -24 34 14.5 & 13.97 & 10.26 & -12.1$\pm$2.1 & -25.4$\pm$2.1 & 5.6$\pm$1.0$^{(1)}$ & -12.8 & -24.0 & 92 & 5.398 & 1\\ 
203881373 & 16 26 09.33 & -24 34 12.2 & 10.8 & 6.5 & -7.7$\pm$1.1 & -26.1$\pm$1.1 & 38.8$\pm$7.2$^{(1)}$ & -11.9 & -24.3 & 27 & 0.275 & 16\\ 
203881640 & 16 27 09.10 & -24 34 08.1 & 19.15 & 8.91 &   &   &   & -11.9 & -24.3 &   & 2.413 & 22\\ 
203881856 & 16 25 32.42 & -24 34 05.1 & 19.65 & 13.36 &   &   &   & -12.0 & -24.3 &   &   & 20\\ 
203884472 & 16 16 51.30 & -24 33 27.7 & 9.74 & 7.65 & -13.5$\pm$1.0 & -21.8$\pm$0.6 & 6.7$\pm$0.3$^{(0)}$ & -12.6 & -24.1 & 98 & 1.417 & 1\\ 
203887087 & 16 28 13.79 & -24 32 49.4 &   & 10.1 & -21.6$\pm$5.3 & -35.1$\pm$5.3 & 125.3$\pm$23.1$^{(4)}$ & -11.8 & -24.3 & 49 & 6.741 & 16\\ 
203887643 & 16 26 51.28 & -24 32 42.0 & 19.94 & 13.89 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203888182 & 16 27 30.51 & -24 32 34.4 & 15.53 & 12.24 & 83.7$\pm$2.1 & -43.1$\pm$2.1 &   & -11.8 & -24.3 &   &  & 19\\ 
203889938 & 16 07 26.25 & -24 32 08.0 & 13.79 & 9.88 & -11.7$\pm$2.3 & -26.5$\pm$2.3 & 7.0$\pm$1.3$^{(1)}$ & -13.2 & -23.9 & 96 & 2.975 & 3\\ 
203891751 & 16 27 46.29 & -24 31 41.2 & 19.54 & 11.32 &   &   &   & -11.8 & -24.3 &   & & 24\\ 
203891936 & 16 20 44.69 & -24 31 38.4 & 11.57 & 8.53 & -4.3$\pm$2.2 & -20.4$\pm$2.2 & 8.6$\pm$1.6$^{(1)}$ & -12.3 & -24.2 & 80 & $<$2 & 0\\ 
203892022 & 16 12 13.69 & -24 31 36.9 & 13.81 & 10.11 & -14.8$\pm$2.1 & -26.5$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -12.9 & -24.0 & 94 & 17.296 & 1\\ 
203892903 & 16 22 45.41 & -24 31 24.1 & 14.02 & 9.06 & 4.8$\pm$2.2 & -30.9$\pm$2.2 &   & -12.2 & -24.2 &   &  & 21\\ 
203893268 & 16 09 45.22 & -24 31 18.6 & 12.25 & 9.14 & -14.3$\pm$2.3 & -28.5$\pm$2.3 & 6.2$\pm$1.1$^{(1)}$ & -13.1 & -23.9 & 94 & 6.376 & 3\\ 
203893434 & 16 27 27.38 & -24 31 16.6 & 18.91 & 9.32 & -18.9$\pm$21.4 &   &   & -11.8 & -24.3 &   & & 22\\ 
203893891 & 16 28 56.95 & -24 31 09.7 & 20.29 & 10.91 & -23.2$\pm$5.0 & -22.2$\pm$5.0 & 3.9$\pm$0.7$^{(1)}$ & -11.7 & -24.4 & 2 & 3.945 & 16\\ 
203894955 & 16 16 02.92 & -24 30 54.8 & 12.79 & 8.96 & -3.1$\pm$2.3 & -20.8$\pm$2.3 & 9.9$\pm$1.8$^{(1)}$ & -12.6 & -24.1 & 65 & 4.435 & 3\\ 
203895004 & 16 16 12.93 & -24 30 54.2 & 14.45 & 10.0 & -10.8$\pm$2.1 & -24.5$\pm$2.1 & 10.7$\pm$2.0$^{(1)}$ & -12.6 & -24.1 & 93 & 2.657 & 3\\ 
203895244 & 16 00 43.10 & -24 30 50.5 & 14.8 & 10.77 & -10.9$\pm$2.1 & -25.7$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -13.7 & -23.7 & 95 & 0.531 & 1\\ 
203895738 & 16 27 38.13 & -24 30 42.9 & 18.49 & 9.66 &   &   &   & -11.8 & -24.3 &   & & 22\\ 
203895983 & 16 04 18.94 & -24 30 39.3 & 12.53 & 8.85 & -11.7$\pm$2.3 & -24.8$\pm$2.3 & 8.7$\pm$1.6$^{(1)}$ & -13.4 & -23.8 & 96 & 2.449 & 1\\ 
203896277 & 16 27 37.19 & -24 30 35.0 &   & 7.58 & -9.6$\pm$6.7 & -31.7$\pm$6.7 & 430.9$\pm$79.4$^{(4)}$ & -11.8 & -24.3 & 82 &  & 16\\ 
203896485 & 16 25 57.53 & -24 30 32.2 & 14.12 & 8.32 & -0.2$\pm$2.3 & -23.5$\pm$2.3 & 32.7$\pm$6.0$^{(1)}$ & -12.0 & -24.3 & 5 & 5.963 & 19\\ 
203897325 & 16 20 34.56 & -24 30 20.5 &   & 12.54 &   &   &   & -12.3 & -24.2 &   &  & 3\\ 
203897643 & 16 08 47.42 & -24 30 15.6 & 14.93 & 10.77 & -13.9$\pm$2.1 & -20.8$\pm$2.1 & 7.5$\pm$1.4$^{(1)}$ & -13.1 & -23.9 & 95 & 1.504 & 3\\ 
203897692 & 16 25 56.10 & -24 30 14.9 &   & 9.76 & -2.9$\pm$6.7 & -27.0$\pm$6.7 & 107.5$\pm$19.8$^{(4)}$ & -12.0 & -24.3 & 54 & 0.501 & 19\\ 
203898731 & 16 08 45.65 & -24 29 59.9 & 15.2 & 11.24 & -11.0$\pm$2.1 & -21.2$\pm$2.1 & 4.8$\pm$0.9$^{(1)}$ & -13.1 & -23.9 & 69 & 1.783 & 3\\ 
203899767 & 16 26 01.61 & -24 29 45.0 &   & 9.63 & -2.2$\pm$6.8 & -27.3$\pm$6.8 & 140.1$\pm$25.8$^{(4)}$ & -11.9 & -24.3 & 63 & 37.568 & 16\\ 
203899786 & 16 25 24.36 & -24 29 44.8 & 13.53 & 9.45 & -1.2$\pm$2.3 & -32.3$\pm$2.3 & 7.5$\pm$1.4$^{(1)}$ & -12.0 & -24.3 & 63 & 5.926 & 19\\ 
203901938 & 16 27 10.04 & -24 29 13.3 &   & 14.11 &   &   &   & -11.9 & -24.3 &   & 0.919 & 20\\ 
203902450 & 16 27 18.49 & -24 29 05.9 &   & 9.68 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203902784 & 16 27 40.84 & -24 29 00.7 &   & 13.1 &   &   &   & -11.8 & -24.3 &   & 20.863 & 20\\ 
203904156 & 16 14 19.74 & -24 28 40.5 & 17.61 & 12.76 & -8.5$\pm$2.8 & -19.7$\pm$2.8 & 5.4$\pm$1.0$^{(1)}$ & -12.7 & -24.0 & 79 & 0.346 & 18\\ 
203904426 & 16 27 05.98 & -24 28 36.3 &   & 12.97 &   &   &   & -11.9 & -24.3 &   & 1.369 & 22\\ 
203904453 & 16 28 18.09 & -24 28 35.8 & 16.95 & 11.3 & -7.7$\pm$2.5 & -30.2$\pm$2.5 & 13.9$\pm$2.6$^{(1)}$ & -11.8 & -24.3 & 77 & 0.796 & 17\\ 
203904870 & 16 27 04.11 & -24 28 29.9 &   & 10.86 &   &   &   & -11.9 & -24.3 &   & 0.49 & 22\\ 
203905625 & 16 28 45.27 & -24 28 19.0 & 11.92 & 8.0 & -12.9$\pm$2.3 & -25.4$\pm$2.3 & 14.2$\pm$2.6$^{(1)}$ & -11.8 & -24.3 & 85 & 8.408 & 16\\ 
203905980 & 16 28 47.04 & -24 28 13.8 & 17.18 & 11.95 & -9.1$\pm$2.5 & -25.2$\pm$2.5 & 8.2$\pm$1.5$^{(1)}$ & -11.8 & -24.3 & 95 & 1.896 & 17\\ 
203906801 & 16 12 57.23 & -24 28 01.3 & 16.29 & 11.95 & -8.1$\pm$2.1 & -12.1$\pm$2.1 & 4.9$\pm$0.9$^{(1)}$ & -12.8 & -24.0 & 10 & 0.763 & 17\\ 
203907143 & 16 25 24.32 & -24 27 56.6 & 7.39 &   & -3.0$\pm$0.1 & -25.7$\pm$0.0 &   & -12.0 & -24.3 &   &   & 16\\ 
203907608 & 16 29 02.87 & -24 27 49.5 &   &   & -14.7$\pm$7.1 & -32.3$\pm$7.6 &   & -11.7 & -24.4 &   &   & 16\\ 
203908052 & 16 27 30.18 & -24 27 43.4 &   & 9.02 &   &   &   & -11.8 & -24.3 &   & 17.835 & 22\\ 
203908611 & 16 24 15.87 & -24 27 35.6 & 14.06 & 9.23 & 0.8$\pm$2.2 & -22.8$\pm$2.2 &   & -12.1 & -24.3 &   & 2.302 & 13\\ 
203909577 & 16 27 28.45 & -24 27 21.0 &   & 10.1 &   &   &   & -11.8 & -24.3 &   &   & 22\\ 
203910454 & 16 14 14.84 & -24 27 08.1 & 16.1 & 11.48 & 2.1$\pm$2.1 & -33.9$\pm$2.1 &   & -12.8 & -24.0 &   & 1.189 & 17\\ 
203911473 & 16 25 19.25 & -24 26 52.7 & 9.64 & 7.8 & -20.0$\pm$1.8 & -26.1$\pm$1.7 & 6.8$\pm$0.8$^{(0)}$ & -12.0 & -24.3 & 90 & 2.618 & 16\\ 
203912136 & 16 11 03.61 & -24 26 42.9 & 19.17 & 13.7 &   &   &   & -13.0 & -24.0 &   &  & 7\\ 
203912192 & 16 26 27.81 & -24 26 41.8 & 19.17 & 12.09 & 230.4$\pm$7.3 &   &   & -11.9 & -24.3 &   & 1.593 & 19\\ 
203912637 & 16 26 32.53 & -24 26 35.4 &   & 13.2 &   &   &   & -11.9 & -24.3 &   & 14.551 & 22\\ 
203912674 & 16 25 39.58 & -24 26 34.9 & 17.43 & 8.95 & -5.3$\pm$2.8 & -22.9$\pm$2.8 & 14.7$\pm$2.7$^{(1)}$ & -12.0 & -24.3 & 64 & 30.587 & 16\\ 
203912855 & 16 28 48.70 & -24 26 31.8 &   & 13.1 &   &   &   & -11.8 & -24.3 &   &  & 20\\ 
203913100 & 16 09 05.12 & -24 26 28.3 & 14.8 & 10.98 & -12.1$\pm$2.1 & -23.3$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -13.1 & -23.9 & 54 & 2.119 & 17\\ 
203913635 & 16 26 54.44 & -24 26 20.7 &   & 10.01 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203913804 & 16 27 55.56 & -24 26 18.0 & 12.91 & 8.9 & -13.2$\pm$2.3 & -27.7$\pm$2.3 & 9.8$\pm$1.8$^{(1)}$ & -11.8 & -24.3 & 95 & 23.497 & 19\\ 
203914036 & 16 21 24.88 & -24 26 14.5 & 16.63 & 11.42 & -8.0$\pm$2.5 & -18.2$\pm$2.5 & 8.0$\pm$1.5$^{(1)}$ & -12.3 & -24.2 & 86 & 2.279 & 17\\ 
203914316 & 16 26 18.82 & -24 26 10.5 &   & 12.14 &   &   &   & -11.9 & -24.3 &   &  & 24\\ 
203914960 & 16 26 21.53 & -24 26 01.0 & 17.22 & 10.92 & -11.1$\pm$2.8 & -21.5$\pm$2.8 & 16.1$\pm$3.0$^{(1)}$ & -11.9 & -24.3 & 71 & 2.499 & 16\\ 
203915424 & 16 27 26.58 & -24 25 54.4 & 17.0 & 11.84 & -9.5$\pm$2.1 & -26.9$\pm$2.1 & 9.9$\pm$1.8$^{(1)}$ & -11.8 & -24.3 & 94 & 2.883 & 19\\ 
203915538 & 16 21 19.21 & -24 25 52.6 &   & 10.67 & -14.6$\pm$3.9 & -28.2$\pm$3.9 & 63.0$\pm$11.6$^{(4)}$ & -12.3 & -24.2 & 46 & 1.319 & 17\\ 
203915766 & 16 20 41.45 & -24 25 49.2 & 18.78 & 12.9 & -19.6$\pm$4.0 & -17.1$\pm$4.0 & 7.0$\pm$1.3$^{(1)}$ & -12.3 & -24.2 & 79 &  & 7\\ 
203916376 & 16 27 49.85 & -24 25 40.2 & 13.31 & 7.3 & -8.0$\pm$2.3 & -25.8$\pm$2.3 & 44.3$\pm$8.2$^{(1)}$ & -11.8 & -24.3 & 33 & 0.472 & 19\\ 
203917082 & 16 26 31.36 & -24 25 30.2 &   & 11.72 &   &   &   & -11.9 & -24.3 &   & & 19\\ 
203917770 & 16 13 45.50 & -24 25 19.5 & 6.42 & 6.08 & -9.5$\pm$0.0 & -19.2$\pm$0.0 & 6.2$\pm$0.6$^{(0)}$ & -12.8 & -24.0 & 89 & $<$2 & 2\\ 
203918961 & 16 20 13.18 & -24 25 01.4 & 16.82 & 12.86 & -1.3$\pm$2.1 & -6.7$\pm$2.1 & 2.4$\pm$0.4$^{(1)}$ & -12.3 & -24.2 &   &  & 17\\ 
203919315 & 16 27 30.84 & -24 24 56.0 & 17.69 & 10.07 & -5.0$\pm$2.7 & -17.8$\pm$2.7 & 13.0$\pm$2.4$^{(1)}$ & -11.8 & -24.3 & 51 & 17.796 & 19\\ 
203919797 & 16 26 24.04 & -24 24 48.1 & 16.65 & 7.32 & -6.4$\pm$3.1 & -25.0$\pm$3.1 & 21.0$\pm$3.9$^{(1)}$ & -11.9 & -24.3 & 44 & 4.791 & 16\\ 
203920000 & 16 26 25.28 & -24 24 45.0 &   & 11.07 &   &   &   & -11.9 & -24.3 &   & 4.788 & 22\\ 
203920354 & 16 26 23.58 & -24 24 39.5 &   & 10.22 &   &   &   & -11.9 & -24.3 &   & 4.791 & 22\\ 
203920452 & 16 15 53.27 & -24 24 38.0 & 14.3 & 10.35 & -10.8$\pm$2.1 & -24.1$\pm$2.1 & 6.1$\pm$1.1$^{(1)}$ & -12.6 & -24.1 & 94 & 6.937 & 3\\ 
203922515 & 16 26 22.27 & -24 24 07.1 &   & 13.94 &   &   &   & -11.9 & -24.3 &   &   & 24\\ 
203923457 & 16 26 22.19 & -24 23 52.4 &   & 12.22 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203924150 & 16 27 11.68 & -24 23 42.0 &   & 10.11 &   &   &   & -11.9 & -24.3 &   & & 22\\ 
203924493 & 16 26 03.40 & -24 23 36.7 &   &   & -8.9$\pm$5.5 & -22.9$\pm$5.5 &   & -11.9 & -24.3 &   &   & 21\\ 
203924502 & 16 26 03.03 & -24 23 36.6 & 11.97 & 6.23 & -17.9$\pm$2.3 & -13.4$\pm$2.3 & 82.9$\pm$15.3$^{(1)}$ & -11.9 & -24.3 & 8 & 3.465 & 21\\ 
203925053 & 16 26 34.17 & -24 23 28.3 & 13.97 & 6.32 & 0.0$\pm$2.3 & -28.9$\pm$2.3 &   & -11.9 & -24.3 &   & 6.214 & 16\\ 
203925433 & 16 26 38.80 & -24 23 22.7 &   & 11.56 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203925751 & 16 28 20.04 & -24 23 17.8 &   & 10.62 & -13.1$\pm$5.0 & -18.0$\pm$5.0 & 83.1$\pm$15.3$^{(4)}$ & -11.8 & -24.3 & 34 & 1.814 & 19\\ 
203926424 & 16 26 45.03 & -24 23 07.7 & 20.06 & 8.95 &   &   &   & -11.9 & -24.3 &   & 4.165 & 22\\ 
203926667 & 16 26 21.38 & -24 23 04.1 &   &   &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203926890 & 16 26 37.79 & -24 23 00.7 &   & 11.11 &   &   &   & -11.9 & -24.3 &   & 25.876 & 22\\ 
203927020 & 16 22 36.73 & -24 22 58.7 & 8.42 & 7.16 & -4.6$\pm$0.2 & -27.1$\pm$0.1 & 8.2$\pm$0.9$^{(0)}$ & -12.2 & -24.2 & 87 & $<$2 & 2\\ 
203927115 & 16 26 30.47 & -24 22 57.1 &   & 9.98 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203927391 & 16 26 22.39 & -24 22 52.9 &   & 9.96 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203927435 & 16 28 43.04 & -24 22 52.3 &   & 10.14 & -14.6$\pm$5.0 & -23.8$\pm$5.0 & 84.1$\pm$15.5$^{(4)}$ & -11.8 & -24.3 & 55 & $<$2 & 16\\ 
203927902 & 16 28 32.67 & -24 22 45.0 & 12.44 & 6.85 & -13.7$\pm$2.3 & -25.5$\pm$2.3 & 51.4$\pm$9.5$^{(1)}$ & -11.8 & -24.3 & 39 & 0.692 & 19\\ 
203928175 & 16 28 23.32 & -24 22 41.0 & 16.14 & 8.62 & -8.1$\pm$2.3 & -23.5$\pm$2.3 & 22.1$\pm$4.1$^{(1)}$ & -11.8 & -24.3 & 47 & 4.376 & 16\\ 
203928675 & 16 26 39.92 & -24 22 33.4 &   & 13.5 &   &   &   & -11.9 & -24.3 &   & 21.74 & 20\\ 
203928921 & 16 26 54.97 & -24 22 29.7 &   & 10.16 &   &   &   & -11.9 & -24.3 &   & 19.663 & 22\\ 
203929332 & 16 26 16.84 & -24 22 23.2 &   & 8.2 & -8.6$\pm$6.6 & -25.8$\pm$6.6 & 324.0$\pm$59.7$^{(4)}$ & -11.9 & -24.3 & 78 & 3.575 & 16\\ 
203929472 & 16 24 46.80 & -24 22 21.1 &   & 7.97 & -1.3$\pm$5.5 & -0.4$\pm$5.5 & 358.6$\pm$66.1$^{(4)}$ & -12.0 & -24.3 &   &  & 16\\ 
203930599 & 16 27 40.27 & -24 22 04.1 & 10.89 & 7.21 & 0.6$\pm$1.1 & -27.1$\pm$1.1 &   & -11.8 & -24.3 &   &  & 19\\ 
203931209 & 16 28 21.51 & -24 21 54.9 &   & 10.18 & -7.2$\pm$5.3 & -21.3$\pm$5.3 & 98.6$\pm$18.2$^{(4)}$ & -11.8 & -24.3 & 58 & 6.681 & 19\\ 
203931628 & 16 22 19.91 & -24 21 48.2 & 8.98 & 7.1 & -3.1$\pm$0.5 & -19.7$\pm$0.6 & 4.8$\pm$1.7$^{(0)}$ & -12.2 & -24.2 & 32 &  & 2\\ 
203933268 & 16 25 59.65 & -24 21 22.3 &   & 9.53 & -2.0$\pm$5.5 & -29.7$\pm$5.5 & 86.8$\pm$16.0$^{(4)}$ & -11.9 & -24.3 & 32 & 2.39 & 16\\ 
203934572 & 16 17 27.70 & -24 21 02.6 & 14.59 & 10.3 & -6.2$\pm$2.1 & -27.0$\pm$2.1 & 9.2$\pm$1.7$^{(1)}$ & -12.5 & -24.1 & 90 & 1.111 & 1\\ 
203934728 & 16 26 23.37 & -24 20 60.0 & 12.73 & 6.57 & -0.7$\pm$2.3 & -25.8$\pm$2.3 & 49.1$\pm$9.0$^{(1)}$ & -11.9 & -24.3 & 7 & 5.873 & 19\\ 
203935066 & 16 26 10.33 & -24 20 54.8 &   & 8.48 &   &   &   & -11.9 & -24.3 &   & 27.551 & 22\\ 
203935537 & 16 25 56.17 & -24 20 48.5 & 11.7 & 7.52 & -3.0$\pm$2.3 & -26.1$\pm$2.3 & 12.6$\pm$2.3$^{(1)}$ & -11.9 & -24.3 & 63 &  & 19\\ 
203936815 & 16 26 42.86 & -24 20 29.9 &   & 7.88 & -5.4$\pm$6.7 & -29.1$\pm$6.7 & 376.0$\pm$69.3$^{(4)}$ & -11.9 & -24.3 & 77 & 8.94 & 16\\ 
203937317 & 16 26 17.08 & -24 20 22.0 & 12.77 & 8.06 & -1.9$\pm$2.3 & -28.1$\pm$2.3 & 17.1$\pm$3.2$^{(1)}$ & -11.9 & -24.3 & 26 & 29.252 & 19\\ 
203937768 & 16 15 11.16 & -24 20 15.3 & 17.92 & 13.17 & -6.9$\pm$2.9 & -16.1$\pm$2.9 & 4.0$\pm$0.7$^{(1)}$ & -12.7 & -24.1 & 2 &   & 18\\ 
203938167 & 16 15 12.39 & -24 20 09.1 &   & 12.13 & -12.2$\pm$4.0 & -30.1$\pm$4.0 & 6.3$\pm$1.2$^{(4)}$ & -12.7 & -24.1 & 92 & 1.615 & 14\\ 
203938591 & 16 26 49.23 & -24 20 02.9 &   & 8.69 & 10.0$\pm$12.0 & 150.0$\pm$55.0 &   & -11.9 & -24.3 &   &  & 22\\ 
203938834 & 16 25 32.24 & -24 19 59.0 & 16.93 & 10.49 & 9.0$\pm$2.5 & 1.5$\pm$2.5 &   & -12.0 & -24.3 &   &  & 16\\ 
203941210 & 16 27 26.22 & -24 19 23.0 &   & 12.93 &   &   &   & -11.8 & -24.3 &   &   & 20\\ 
203941277 & 16 26 15.81 & -24 19 22.1 &   & 10.03 &   &   &   & -11.9 & -24.3 &   &   & 22\\ 
203941468 & 16 27 10.31 & -24 19 18.9 & 16.87 & 9.47 & 564.9$\pm$11.3 &   &   & -11.9 & -24.3 &   &   & 16\\ 
203941868 & 16 27 10.26 & -24 19 12.6 & 12.42 & 6.72 & -4.5$\pm$2.3 & -28.9$\pm$2.3 & 49.1$\pm$9.1$^{(1)}$ & -11.9 & -24.3 & 14 & 2.049 & 16\\ 
203942275 & 16 26 29.67 & -24 19 05.5 &   & 11.17 &   &   &   & -11.9 & -24.3 &   & 0.593 & 22\\ 
203942620 & 16 26 36.82 & -24 19 00.2 & 20.08 & 14.76 &   &   &   & -11.9 & -24.3 &   & 14.141 & 20\\ 
203946777 & 16 27 22.91 & -24 17 57.4 & 20.05 & 9.45 &   &   &   & -11.8 & -24.3 &   & 5.394 & 22\\ 
203946909 & 16 27 37.42 & -24 17 54.9 & 19.68 & 11.95 &   &   &   & -11.8 & -24.3 &   & 2.107 & 24\\ 
203947305 & 16 24 41.05 & -24 17 48.8 & 16.46 & 8.98 & 0.9$\pm$2.8 & -10.3$\pm$2.8 &   & -12.0 & -24.3 &   & 34.966 & 16\\ 
203947410 & 16 26 03.30 & -24 17 47.1 & 14.25 & 9.11 & -6.4$\pm$2.3 & -31.7$\pm$2.3 & 18.1$\pm$3.3$^{(1)}$ & -11.9 & -24.3 & 44 & 5.683 & 16\\ 
203952180 & 16 26 43.76 & -24 16 33.3 & 19.14 & 9.6 &   &   &   & -11.9 & -24.3 &   & 1.772 & 22\\ 
203953466 & 16 26 24.07 & -24 16 13.5 &   & 6.68 & -14.4$\pm$6.6 & -35.3$\pm$6.6 & 651.3$\pm$120.0$^{(4)}$ & -11.9 & -24.3 & 83 & 6.741 & 19\\ 
203954364 & 16 26 37.13 & -24 15 59.9 & 17.02 & 10.76 & -5.0$\pm$2.5 & -31.8$\pm$2.5 & 17.7$\pm$3.3$^{(1)}$ & -11.9 & -24.3 & 38 & 1.78 & 16\\ 
203954898 & 16 26 36.83 & -24 15 51.9 & 17.23 & 9.59 & -8.3$\pm$2.8 & -29.9$\pm$2.8 & 16.1$\pm$3.0$^{(1)}$ & -11.9 & -24.3 & 68 &  & 16\\ 
203955457 & 16 25 36.74 & -24 15 42.9 & 14.62 & 8.38 & 1.6$\pm$2.3 & -26.9$\pm$2.3 &   & -12.0 & -24.3 &   & 28.135 & 16\\ 
203955624 & 16 25 24.29 & -24 15 40.1 &   & 10.93 & -10.9$\pm$5.1 & -33.5$\pm$5.1 & 47.2$\pm$8.7$^{(4)}$ & -12.0 & -24.3 & 20 & 0.424 & 16\\ 
203956650 & 16 28 32.56 & -24 15 24.2 &   & 9.84 & -14.1$\pm$19.2 & -10.6$\pm$19.2 & 145.3$\pm$26.8$^{(4)}$ & -11.8 & -24.3 & 25 & 0.675 & 19\\ 
203960268 & 16 26 25.68 & -24 14 27.8 &   & 11.5 & -14.9$\pm$4.9 & -36.6$\pm$4.9 & 41.3$\pm$7.6$^{(4)}$ & -11.9 & -24.3 & 14 & 1.959 & 16\\ 
203962241 & 16 29 23.39 & -24 13 56.9 &   & 7.02 & -22.1$\pm$6.7 & -5.8$\pm$6.7 & 558.2$\pm$102.8$^{(4)}$ & -11.7 & -24.3 & 11 & 24.13 & 21\\ 
203962559 & 16 26 50.48 & -24 13 52.3 &   & 10.8 & -10.7$\pm$5.0 & -32.4$\pm$5.0 & 57.5$\pm$10.6$^{(4)}$ & -11.9 & -24.3 & 27 & 1.541 & 16\\ 
203962599 & 16 26 56.77 & -24 13 51.6 & 17.79 & 9.25 & -16.2$\pm$3.1 & -23.5$\pm$3.1 & 12.4$\pm$2.3$^{(1)}$ & -11.9 & -24.3 & 86 & 5.227 & 16\\ 
203969672 & 16 27 09.07 & -24 12 00.8 &   & 9.8 & -4.2$\pm$6.7 & -21.1$\pm$6.7 & 155.2$\pm$28.6$^{(4)}$ & -11.9 & -24.3 & 58 & 4.865 & 16\\ 
203969721 & 16 26 46.41 & -24 12 00.0 & 13.66 & 7.49 & -6.1$\pm$2.3 & -26.6$\pm$2.3 & 44.2$\pm$8.1$^{(1)}$ & -11.9 & -24.3 & 24 & 3.358 & 19\\ 
203971352 & 16 28 12.72 & -24 11 35.6 &   & 11.09 & -0.6$\pm$5.3 & -43.4$\pm$5.3 & 85.8$\pm$15.8$^{(4)}$ & -11.8 & -24.3 &   & 2.43 & 24\\ 
203972079 & 16 24 57.29 & -24 11 24.1 &   & 9.23 & -9.0$\pm$5.5 & -31.4$\pm$5.5 & 136.9$\pm$25.2$^{(4)}$ & -12.0 & -24.2 & 71 & 6.358 & 19\\ 
203972954 & 16 26 43.14 & -24 11 10.4 & 14.54 & 9.68 & -10.2$\pm$2.3 & -28.4$\pm$2.3 & 11.3$\pm$2.1$^{(1)}$ & -11.9 & -24.3 & 91 & 13.107 & 19\\ 
203975467 & 16 27 11.88 & -24 10 31.3 &   & 9.64 & -7.6$\pm$6.7 & -12.9$\pm$6.7 & 153.2$\pm$28.2$^{(4)}$ & -11.9 & -24.3 & 28 & 8.42 & 16\\ 
203979309 & 16 27 04.06 & -24 09 31.8 &   & 10.09 & -2.7$\pm$3.9 & -32.0$\pm$3.9 & 83.4$\pm$15.4$^{(4)}$ & -11.9 & -24.3 & 17 & 4.605 & 16\\ 
203979314 & 16 28 24.30 & -24 09 31.7 &   & 9.83 & -8.5$\pm$6.7 & -20.3$\pm$6.7 & 114.5$\pm$21.1$^{(4)}$ & -11.8 & -24.3 & 57 & 10.421 & 16\\ 
203981774 & 16 26 20.99 & -24 08 52.5 & 14.39 & 9.5 & -8.2$\pm$2.3 & -35.3$\pm$2.3 & 15.2$\pm$2.8$^{(1)}$ & -11.9 & -24.3 & 54 & 0.824 & 16\\ 
203987773 & 16 26 18.80 & -24 07 19.6 &   & 9.35 & 7.0$\pm$5.2 & -43.5$\pm$5.2 &   & -11.9 & -24.3 &   & 6.38 & 16\\ 
203988827 & 16 27 06.55 & -24 07 03.2 &   & 10.76 & -2.6$\pm$5.3 & -30.1$\pm$5.3 & 67.4$\pm$12.4$^{(4)}$ & -11.9 & -24.3 & 17 & 4.235 & 19\\ 
203991803 & 16 28 10.99 & -24 06 17.8 &   & 10.06 & -19.3$\pm$5.0 & -21.0$\pm$5.0 & 85.2$\pm$15.7$^{(4)}$ & -11.8 & -24.3 & 41 & 1.533 & 19\\ 
203993703 & 16 28 32.17 & -24 05 48.3 & 16.81 & 10.21 & -6.5$\pm$2.5 & -28.6$\pm$2.5 & 19.4$\pm$3.6$^{(1)}$ & -11.8 & -24.3 & 49 & 1.489 & 16\\ 
203995761 & 16 28 16.73 & -24 05 14.3 &   & 8.86 & -13.9$\pm$6.7 & -13.7$\pm$6.7 & 206.2$\pm$38.0$^{(4)}$ & -11.8 & -24.3 & 42 & 5.159 & 16\\ 
204040060 & 15 57 25.74 & -23 54 22.3 & 12.94 & 9.09 & -18.0$\pm$2.3 & -31.0$\pm$2.3 & 11.2$\pm$2.1$^{(1)}$ & -13.9 & -23.6 & 91 & 7.248 & 26\\ 
204041137 & 15 56 12.17 & -23 54 07.7 & 14.19 & 10.23 & -20.7$\pm$2.1 & -31.4$\pm$2.1 & 8.2$\pm$1.5$^{(1)}$ & -14.0 & -23.6 & 92 & 0.42 & 1\\ 
204054129 & 16 01 49.56 & -23 51 08.2 & 16.19 & 11.93 & -3.9$\pm$2.1 & -23.4$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -13.6 & -23.7 & 21 & 0.527 & 27\\ 
204054556 & 16 08 10.50 & -23 51 02.4 & 9.01 & 7.83 & -9.8$\pm$0.1 & -20.6$\pm$0.1 & 6.3$\pm$0.3$^{(0)}$ & -13.1 & -23.9 & 99 & $<$2 & 6\\ 
204059992 & 16 10 01.85 & -23 49 43.5 & 14.14 & 10.13 & -12.0$\pm$2.1 & -25.7$\pm$2.1 & 8.6$\pm$1.6$^{(1)}$ & -13.0 & -23.9 & 96 & 1.434 & 28\\ 
204063024 & 16 03 31.82 & -23 48 58.3 & 13.14 & 9.73 & -10.0$\pm$2.3 & -20.1$\pm$2.3 & 5.7$\pm$1.0$^{(1)}$ & -13.5 & -23.8 & 86 & 9.212 & 3\\ 
204065688 & 15 56 29.42 & -23 48 19.8 & 11.93 & 8.74 & -13.0$\pm$4.5 & -41.3$\pm$1.1 & 7.8$\pm$1.4$^{(1)}$ & -14.0 & -23.6 & 58 & 8.013 & 26\\ 
204066097 & 15 58 35.98 & -23 48 13.7 &   & 12.08 & -10.3$\pm$5.0 & -21.7$\pm$5.0 & 3.3$\pm$0.6$^{(4)}$ & -13.8 & -23.6 &   & 0.359 & 27\\ 
204066898 & 15 58 36.21 & -23 48 02.0 & 14.02 & 10.19 & -14.9$\pm$2.1 & -24.3$\pm$2.1 & 7.1$\pm$1.3$^{(1)}$ & -13.8 & -23.6 & 96 & 0.359 & 14\\ 
204072696 & 16 04 04.54 & -23 46 37.8 & 14.75 & 10.73 & -9.2$\pm$2.1 & -25.5$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -13.4 & -23.8 & 91 & 3.767 & 17\\ 
204074274 & 16 11 37.62 & -23 46 14.7 & 15.31 & 11.21 & -8.5$\pm$2.1 & -24.3$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -12.9 & -23.9 & 85 & 1.803 & 28\\ 
204076987 & 16 15 09.28 & -23 45 35.0 & 9.34 & 8.03 & -8.0$\pm$0.1 & -23.7$\pm$0.1 & 6.5$\pm$0.3$^{(0)}$ & -12.7 & -24.0 & 95 & $<$2 & 2\\ 
204078097 & 16 09 58.52 & -23 45 18.6 &   & 11.62 & -10.4$\pm$5.0 & -21.1$\pm$5.0 & 30.7$\pm$5.7$^{(4)}$ & -13.0 & -23.9 & 28 & 1.41 & 7\\ 
204078986 & 16 08 07.45 & -23 45 05.6 & 18.35 & 13.34 & -24.9$\pm$2.8 & -13.0$\pm$2.8 & 4.8$\pm$0.9$^{(1)}$ & -13.1 & -23.9 & 3 & 1.553 & 28\\ 
204079030 & 16 15 08.92 & -23 45 04.8 & 15.37 & 11.34 & -10.1$\pm$2.1 & -26.3$\pm$2.1 & 5.0$\pm$0.9$^{(1)}$ & -12.7 & -24.0 & 80 & 2.829 & 28\\ 
204084492 & 15 57 12.79 & -23 43 46.6 & 17.13 & 12.59 & -7.6$\pm$2.5 & -29.9$\pm$2.5 & 5.4$\pm$1.0$^{(1)}$ & -13.9 & -23.6 & 73 & 1.142 & 27\\ 
204086598 & 16 00 44.65 & -23 43 14.7 & 14.58 & 10.22 & -25.2$\pm$2.1 & -36.3$\pm$2.1 & 12.6$\pm$2.3$^{(1)}$ & -13.7 & -23.7 & 54 & 1.705 & 10\\ 
204086791 & 16 09 29.39 & -23 43 12.1 & 18.23 & 13.22 & -2.5$\pm$7.3 & -6.2$\pm$7.3 & 5.8$\pm$1.1$^{(1)}$ & -13.0 & -23.9 & 18 & 0.526 & 28\\ 
204093677 & 16 09 16.90 & -23 41 32.5 & 15.2 & 10.97 & -12.8$\pm$2.1 & -21.0$\pm$2.1 & 7.2$\pm$1.3$^{(1)}$ & -13.1 & -23.9 & 95 & 0.363 & 28\\ 
204094503 & 16 08 48.37 & -23 41 20.9 & 15.9 & 11.59 & -4.7$\pm$2.9 & -23.4$\pm$2.9 & 5.5$\pm$1.0$^{(1)}$ & -13.1 & -23.9 & 73 & 1.653 & 28\\ 
204095429 & 16 08 43.72 & -23 41 07.5 & 5.88 & 5.71 & -10.3$\pm$0.0 & -25.5$\pm$0.0 & 5.7$\pm$0.6$^{(0)}$ & -13.1 & -23.9 & 95 &   & 2\\ 
204096760 & 16 00 07.05 & -23 40 48.7 &   & 10.61 & -10.9$\pm$3.9 & -29.7$\pm$3.9 & 8.8$\pm$1.6$^{(4)}$ & -13.7 & -23.7 & 94 & 0.526 & 1\\ 
204097242 & 15 58 06.40 & -23 40 41.9 & 14.58 & 10.65 & -12.2$\pm$2.1 & -23.2$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -13.8 & -23.6 & 93 & 2.529 & 1\\ 
204099713 & 16 11 26.30 & -23 40 06.0 & 16.99 & 12.47 & 2.2$\pm$2.6 & -22.3$\pm$2.5 &   & -12.9 & -23.9 &   & 1.798 & 17\\ 
204099739 & 16 08 39.09 & -23 40 05.7 & 12.91 & 9.15 & -7.0$\pm$2.3 & -23.3$\pm$2.3 & 10.0$\pm$1.8$^{(1)}$ & -13.1 & -23.9 & 88 & 0.716 & 3\\ 
204100531 & 16 09 07.76 & -23 39 54.5 &   & 11.13 & -5.1$\pm$3.9 & -28.1$\pm$3.9 & 7.1$\pm$1.3$^{(4)}$ & -13.1 & -23.9 & 89 & 1.255 & 17\\ 
204101029 & 16 16 17.94 & -23 39 47.6 & 10.23 & 8.1 & -8.5$\pm$1.4 & -22.4$\pm$0.4 & 7.4$\pm$0.3$^{(0)}$ & -12.6 & -24.0 & 96 & 2.639 & 5\\ 
204103213 & 16 14 21.44 & -23 39 14.7 &   & 14.0 &   &   &   & -12.7 & -24.0 &   &  & 28\\ 
204104882 & 15 57 19.99 & -23 38 50.0 & 11.92 & 8.88 & -30.2$\pm$2.3 & -36.8$\pm$2.3 & 7.0$\pm$1.3$^{(1)}$ & -13.9 & -23.6 & 21 & 6.188 & 26\\ 
204105333 & 16 00 49.72 & -23 38 43.1 & 13.27 & 9.74 & -15.7$\pm$2.3 & -27.2$\pm$2.3 & 6.3$\pm$1.2$^{(1)}$ & -13.6 & -23.7 & 94 & 10.071 & 1\\ 
204105498 & 16 12 46.92 & -23 38 40.8 &   & 12.62 & -3.7$\pm$5.0 & -22.1$\pm$5.0 & 19.7$\pm$3.6$^{(4)}$ & -12.8 & -23.9 & 29 & 0.284 & 18\\ 
204107757 & 15 56 01.04 & -23 38 08.1 & 17.6 & 12.81 & -18.5$\pm$2.8 & -28.7$\pm$2.8 & 5.1$\pm$0.9$^{(1)}$ & -14.0 & -23.6 & 71 & 1.506 & 27\\ 
204115917 & 15 56 20.61 & -23 36 10.0 & 14.1 & 10.32 & -9.7$\pm$2.1 & -14.6$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -14.0 & -23.6 & 67 & 2.388 & 1\\ 
204117263 & 16 11 02.12 & -23 35 50.5 & 15.11 & 10.95 & -8.0$\pm$2.1 & -29.1$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -12.9 & -23.9 & 92 & 0.642 & 28\\ 
204118782 & 16 08 23.04 & -23 35 29.5 & 13.64 & 9.94 & -8.9$\pm$2.3 & -24.0$\pm$2.3 & 6.6$\pm$1.2$^{(1)}$ & -13.1 & -23.8 & 94 & 3.241 & 28\\ 
204119181 & 16 03 40.31 & -23 35 23.6 & 15.27 & 11.32 & -9.0$\pm$2.1 & -23.0$\pm$2.1 & 4.6$\pm$0.9$^{(1)}$ & -13.4 & -23.7 & 57 & 2.687 & 17\\ 
204120066 & 16 08 30.49 & -23 35 11.0 & 19.3 & 13.81 &   &   &   & -13.1 & -23.8 &   &  & 28\\ 
204121833 & 16 00 30.24 & -23 34 45.7 & 16.37 & 11.84 & -14.9$\pm$2.1 & -22.6$\pm$2.1 & 7.0$\pm$1.3$^{(1)}$ & -13.7 & -23.7 & 96 & 0.448 & 27\\ 
204123651 & 15 58 28.56 & -23 34 19.2 & 14.28 & 10.42 & -11.5$\pm$2.1 & -23.2$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -13.8 & -23.6 & 93 & 2.393 & 1\\ 
204124762 & 16 26 06.26 & -23 34 03.1 &   & 11.75 & -30.6$\pm$14.5 & 5.5$\pm$14.5 &   & -11.9 & -24.2 &   & 2.052 & 17\\ 
204125373 & 16 15 20.10 & -23 33 54.5 &   & 11.93 & -3.6$\pm$2.2 & -34.1$\pm$2.2 & 27.1$\pm$5.0$^{(4)}$ & -12.6 & -24.0 & 6 & 3.82 & 28\\ 
204126288 & 16 16 45.39 & -23 33 41.4 &   & 12.82 & -16.7$\pm$5.0 & -39.4$\pm$5.0 & 4.6$\pm$0.8$^{(4)}$ & -12.5 & -24.0 & 18 & 0.211 & 17\\ 
204127977 & 16 11 04.80 & -23 33 16.6 & 12.93 & 9.66 & -4.5$\pm$2.3 & -14.9$\pm$2.3 & 5.6$\pm$1.0$^{(1)}$ & -12.9 & -23.9 & 33 & 4.879 & 1\\ 
204128422 & 16 22 53.29 & -23 33 10.2 & 14.39 & 9.39 & -8.3$\pm$2.3 & -28.4$\pm$2.2 & 13.3$\pm$2.4$^{(1)}$ & -12.1 & -24.2 & 83 & 1.245 & 13\\ 
204129511 & 16 25 35.05 & -23 32 55.1 & 12.89 & 8.91 & 0.6$\pm$2.4 & -28.4$\pm$2.4 &   & -11.9 & -24.2 &   & 7.798 & 1\\ 
204129971 & 16 21 28.69 & -23 32 48.9 & 14.84 & 9.6 & -4.1$\pm$6.1 & -39.9$\pm$7.1 & 13.1$\pm$2.4$^{(1)}$ & -12.2 & -24.1 & 45 &  & 13\\ 
204130665 & 16 21 28.81 & -23 32 39.0 & 10.96 & 7.17 & -7.8$\pm$1.1 & -23.8$\pm$1.0 & 21.4$\pm$4.0$^{(1)}$ & -12.2 & -24.1 & 52 &  & 13\\ 
204133691 & 16 10 20.88 & -23 31 55.7 &   & 11.05 & 3.5$\pm$7.0 & -13.2$\pm$7.0 &   & -13.0 & -23.9 &   & 0.811 & 28\\ 
204134887 & 15 57 48.80 & -23 31 38.3 & 6.76 & 6.67 & -8.0$\pm$0.0 & -17.4$\pm$0.0 & 5.2$\pm$0.6$^{(0)}$ & -13.8 & -23.6 & 24 & $<$2 & 2\\ 
204139015 & 16 23 55.09 & -23 30 40.0 & 14.18 & 10.07 & -9.3$\pm$2.1 & -27.3$\pm$2.1 & 7.5$\pm$1.4$^{(1)}$ & -12.1 & -24.2 & 96 & 2.853 & 1\\ 
204139016 & 16 23 55.80 & -23 30 40.0 & 15.08 & 10.75 & -5.9$\pm$2.3 & -29.2$\pm$2.2 & 7.4$\pm$1.4$^{(1)}$ & -12.1 & -24.2 & 91 & 2.853 & 1\\ 
204141928 & 16 00 23.24 & -23 29 59.5 & 18.99 & 13.31 & 396.2$\pm$7.7 & 113.1$\pm$7.7 &   & -13.7 & -23.7 &   & 31.782 & 3\\ 
204142789 & 15 56 54.98 & -23 29 47.8 & 13.97 & 10.28 & -21.0$\pm$2.1 & -32.8$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -13.9 & -23.6 & 72 & 4.528 & 26\\ 
204143627 & 16 15 59.25 & -23 29 36.3 & 15.42 & 11.31 & -10.1$\pm$2.1 & -25.5$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -12.6 & -24.0 & 88 & 1.123 & 28\\ 
204147295 & 16 14 57.50 & -23 28 42.8 & 14.69 & 10.82 & -11.8$\pm$2.1 & -21.6$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -12.7 & -24.0 & 85 & 2.747 & 28\\ 
204147776 & 15 58 12.71 & -23 28 36.5 & 10.0 & 8.02 & -14.1$\pm$1.4 & -24.0$\pm$0.4 & 6.6$\pm$0.6$^{(0)}$ & -13.8 & -23.6 & 98 & 1.72 & 10\\ 
204149252 & 16 13 34.77 & -23 28 15.6 & 16.91 & 12.5 & -8.0$\pm$2.5 & -20.2$\pm$2.5 & 4.0$\pm$0.7$^{(1)}$ & -12.8 & -24.0 & 7 & 0.995 & 28\\ 
204150518 & 16 17 16.49 & -23 27 57.1 & 14.19 & 10.24 & -15.3$\pm$2.1 & -27.1$\pm$2.1 & 6.9$\pm$1.3$^{(1)}$ & -12.5 & -24.0 & 96 & 5.169 & 1\\ 
204151925 & 16 25 24.28 & -23 27 36.8 & 6.59 & 5.43 & -4.6$\pm$0.3 & -21.2$\pm$0.2 & 8.0$\pm$0.8$^{(0)}$ & -12.0 & -24.2 & 81 & $<$2 & 2\\ 
204152030 & 16 13 36.48 & -23 27 35.3 &   & 11.22 & -14.1$\pm$3.9 & -24.5$\pm$3.9 & 14.4$\pm$2.7$^{(4)}$ & -12.8 & -24.0 & 81 & 1.803 & 28\\ 
204152441 & 16 13 36.89 & -23 27 29.8 & 14.81 & 10.91 & -13.3$\pm$2.2 & -22.6$\pm$2.2 & 5.0$\pm$0.9$^{(1)}$ & -12.8 & -24.0 & 79 & 1.803 & 28\\ 
204153041 & 16 16 33.44 & -23 27 21.1 &   & 11.34 & -11.6$\pm$3.9 & -24.5$\pm$3.9 & 11.3$\pm$2.1$^{(4)}$ & -12.6 & -24.0 & 90 & 0.757 & 28\\ 
204154149 & 16 16 11.74 & -23 27 05.2 & 14.95 & 11.0 & -13.0$\pm$2.1 & -26.5$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -12.6 & -24.0 & 87 & 1.887 & 28\\ 
204156256 & 16 22 59.81 & -23 26 34.9 & 13.61 & 8.95 & -10.7$\pm$2.3 & -33.8$\pm$2.3 & 13.1$\pm$2.4$^{(1)}$ & -12.1 & -24.1 & 78 & 12.259 & 13\\ 
204156820 & 16 13 36.45 & -23 26 27.0 & 13.39 & 9.31 & -16.3$\pm$2.3 & -20.5$\pm$2.3 & 11.9$\pm$2.2$^{(1)}$ & -12.8 & -23.9 & 85 & 2.615 & 1\\ 
204159842 & 16 22 47.22 & -23 25 44.8 & 14.89 & 9.64 & -5.6$\pm$2.3 & -29.1$\pm$2.3 & 16.6$\pm$3.1$^{(1)}$ & -12.1 & -24.1 & 53 & 10.738 & 13\\ 
204160652 & 16 22 46.80 & -23 25 32.8 & 14.02 & 8.23 & -21.9$\pm$2.3 & -31.4$\pm$2.3 & 51.3$\pm$9.4$^{(1)}$ & -12.1 & -24.1 & 11 & 10.731 & 13\\ 
204162631 & 16 15 59.87 & -23 25 04.5 & 11.45 &   & -8.1$\pm$1.1 & -25.1$\pm$1.0 &   & -12.6 & -24.0 &   & $<$2 & 1\\ 
204162886 & 16 17 21.63 & -23 25 00.4 & 14.66 & 10.8 & -10.5$\pm$2.1 & -26.4$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -12.5 & -24.0 & 87 & 6.76 & 1\\ 
204165788 & 16 25 35.08 & -23 24 18.8 & 7.06 & 5.78 & -7.9$\pm$0.0 & -24.7$\pm$0.0 & 7.2$\pm$0.3$^{(0)}$ & -11.9 & -24.2 & 97 & $<$2 & 2\\ 
204172667 & 16 15 11.05 & -23 22 42.6 & 13.26 & 9.84 & -7.7$\pm$2.3 & -27.9$\pm$2.3 & 5.4$\pm$1.0$^{(1)}$ & -12.6 & -24.0 & 82 & 1.271 & 1\\ 
204172838 & 16 09 02.02 & -23 22 40.2 & 13.83 & 10.11 & -8.8$\pm$2.1 & -25.9$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -13.1 & -23.8 & 93 & 4.563 & 28\\ 
204174563 & 15 55 17.04 & -23 22 16.6 & 13.27 & 9.33 & -22.2$\pm$2.0 & -32.0$\pm$1.9 & 11.0$\pm$2.0$^{(1)}$ & -14.0 & -23.5 & 84 & $<$2 & 26\\ 
204175249 & 15 55 18.76 & -23 22 07.3 & 13.92 & 9.77 & -47.9$\pm$3.4 & -60.6$\pm$3.0 &   & -14.0 & -23.5 &   & 38.371 & 26\\ 
204175508 & 15 55 17.59 & -23 22 03.8 & 8.4 & 7.39 & -18.6$\pm$0.1 & -28.0$\pm$0.0 & 8.2$\pm$0.3$^{(0)}$ & -14.0 & -23.5 & 98 &   & 2\\ 
204175516 & 16 25 16.90 & -23 22 03.6 & 12.89 & 9.02 & -9.5$\pm$2.4 & -32.1$\pm$2.4 & 9.0$\pm$1.7$^{(1)}$ & -12.0 & -24.2 & 93 & 6.817 & 1\\ 
204176565 & 16 22 18.53 & -23 21 48.2 & 12.03 & 8.11 & -8.9$\pm$1.2 & -24.4$\pm$1.0 & 10.4$\pm$1.9$^{(1)}$ & -12.2 & -24.1 & 93 & 8.194 & 21\\ 
204176771 & 16 25 02.38 & -23 21 45.1 & 13.4 & 9.29 & -10.2$\pm$2.4 & -27.5$\pm$2.4 & 9.7$\pm$1.8$^{(1)}$ & -12.0 & -24.2 & 94 & 0.721 & 1\\ 
204177257 & 16 14 38.11 & -23 21 38.1 & 18.23 &   & -13.8$\pm$2.7 & -11.1$\pm$2.7 &   & -12.7 & -24.0 &   &   & 28\\ 
204177311 & 16 14 38.47 & -23 21 37.4 & 14.24 & 10.59 & 0.7$\pm$6.5 & -27.1$\pm$11.4 &   & -12.7 & -24.0 &   & 5.783 & 28\\ 
204179058 & 15 57 34.31 & -23 21 12.3 & 12.51 & 8.99 & -13.8$\pm$2.3 & -22.6$\pm$2.3 & 9.0$\pm$1.7$^{(1)}$ & -13.9 & -23.6 & 95 & 1.494 & 1\\ 
204179868 & 16 07 14.78 & -23 21 01.1 & 19.82 & 15.13 & 4.6$\pm$2.9 & -6.7$\pm$2.9 &   & -13.2 & -23.8 &   & 1.962 & 29\\ 
204181799 & 16 13 54.35 & -23 20 34.2 & 14.05 & 10.06 & 77.4$\pm$17.0 & 89.9$\pm$17.0 &   & -12.7 & -23.9 &   &  & 28\\ 
204182919 & 16 02 35.88 & -23 20 17.1 & 14.09 & 10.2 & -7.9$\pm$2.1 & -21.9$\pm$2.1 & 7.1$\pm$1.3$^{(1)}$ & -13.5 & -23.7 & 92 & 6.704 & 1\\ 
204185181 & 16 12 55.34 & -23 19 45.7 & 8.99 & 7.29 & -9.5$\pm$0.1 & -23.9$\pm$0.1 & 6.6$\pm$0.2$^{(0)}$ & -12.8 & -23.9 & 99 & 5.144 & 2\\ 
204187094 & 16 11 19.09 & -23 19 20.1 &   & 10.7 & -6.0$\pm$3.2 & -12.1$\pm$3.9 & 41.4$\pm$7.6$^{(4)}$ & -12.9 & -23.9 & 3 & 7.831 & 28\\ 
204189121 & 15 55 08.52 & -23 18 51.1 & 13.78 & 9.9 & -16.0$\pm$2.3 & -18.0$\pm$2.3 & 7.3$\pm$1.3$^{(1)}$ & -14.0 & -23.5 & 92 & 5.213 & 1\\ 
204189554 & 16 15 12.41 & -23 18 45.4 & 12.98 & 9.7 & -8.5$\pm$2.3 & -24.9$\pm$2.3 & 5.1$\pm$0.9$^{(1)}$ & -12.6 & -24.0 & 80 & 13.926 & 1\\ 
204190916 & 16 04 43.04 & -23 18 25.9 & 17.57 & 12.86 & 179.4$\pm$7.3 & 3.7$\pm$7.3 &   & -13.4 & -23.7 &   & 0.208 & 18\\ 
204195050 & 16 23 51.56 & -23 17 27.0 & 17.74 & 12.42 & -12.4$\pm$2.7 & -24.9$\pm$2.7 & 9.0$\pm$1.7$^{(1)}$ & -12.1 & -24.1 & 95 & 1.957 & 18\\ 
204197234 & 16 32 42.22 & -23 16 56.2 &   & 10.87 & -27.2$\pm$4.0 & -41.2$\pm$4.0 & 10.4$\pm$1.9$^{(4)}$ & -11.5 & -24.3 & 31 & 0.667 & 17\\ 
204199333 & 16 16 11.84 & -23 16 26.8 &   & 11.88 & -21.5$\pm$3.9 & -27.3$\pm$3.9 & 4.9$\pm$0.9$^{(4)}$ & -12.6 & -24.0 & 46 & 0.837 & 28\\ 
204201027 & 16 20 25.24 & -23 16 03.3 & 18.36 & 13.23 & 14.3$\pm$10.5 & 88.7$\pm$10.5 &   & -12.3 & -24.1 &   & 1.023 & 18\\ 
204202443 & 16 15 28.19 & -23 15 43.9 & 16.41 & 12.34 & -14.3$\pm$2.5 & -36.9$\pm$2.5 & 3.5$\pm$0.7$^{(1)}$ & -12.6 & -24.0 &   & $<$2 & 28\\ 
204202811 & 16 16 41.62 & -23 15 39.1 & 14.97 & 11.04 & -16.7$\pm$2.1 & -30.3$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -12.5 & -24.0 & 76 & 1.25 & 28\\ 
204204414 & 16 15 36.48 & -23 15 17.5 &   & 13.1 & -16.3$\pm$5.0 & -20.1$\pm$5.0 & 1.9$\pm$0.3$^{(4)}$ & -12.6 & -24.0 &   & 0.622 & 28\\ 
204204469 & 16 10 30.15 & -23 15 16.7 &   & 13.26 &   &   &   & -13.0 & -23.9 &   &  & 28\\ 
204204545 & 16 13 12.17 & -23 15 15.6 & 14.77 & 10.84 & -11.8$\pm$2.1 & -23.9$\pm$2.1 & 5.7$\pm$1.1$^{(1)}$ & -12.8 & -23.9 & 92 & 1.798 & 28\\ 
204204606 & 16 15 54.87 & -23 15 14.7 & 14.2 & 10.33 & -9.5$\pm$2.2 & -21.9$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -12.6 & -24.0 & 94 & 1.149 & 28\\ 
204204888 & 16 08 28.47 & -23 15 10.3 &   & 14.2 &   &   &   & -13.1 & -23.8 &   &   & 29\\ 
204210528 & 16 13 10.83 & -23 13 51.4 &   & 11.61 & -17.3$\pm$3.9 & -26.8$\pm$3.9 & 14.8$\pm$2.7$^{(4)}$ & -12.8 & -23.9 & 78 & 0.986 & 28\\ 
204210698 & 16 22 15.76 & -23 13 49.1 & 17.37 & 12.8 & -20.4$\pm$2.6 & -50.1$\pm$2.6 &   & -12.2 & -24.1 &   & 0.282 & 17\\ 
204217309 & 16 10 23.45 & -23 12 17.7 & 14.22 & 10.16 & -10.6$\pm$2.1 & -33.7$\pm$2.1 & 7.9$\pm$1.5$^{(1)}$ & -13.0 & -23.9 & 90 & $<$2 & 28\\ 
204217770 & 16 21 28.45 & -23 12 11.2 & 12.6 & 8.74 & -10.0$\pm$2.4 & -29.6$\pm$2.4 & 9.7$\pm$1.8$^{(1)}$ & -12.2 & -24.1 & 94 & 2.927 & 13\\ 
204220275 & 16 11 40.40 & -23 11 34.8 & 16.51 & 11.62 & -10.2$\pm$2.5 & -26.7$\pm$2.5 & 10.3$\pm$1.9$^{(1)}$ & -12.9 & -23.9 & 93 & 1.332 & 28\\ 
204222295 & 16 13 29.29 & -23 11 07.6 & 11.06 & 8.49 & -10.3$\pm$1.0 & -25.9$\pm$1.2 & 6.2$\pm$1.1$^{(1)}$ & -12.8 & -23.9 & 95 & 3.095 & 5\\ 
204222666 & 15 56 47.85 & -23 11 02.7 & 7.71 & 7.18 & -12.6$\pm$0.1 & -24.2$\pm$0.0 & 6.6$\pm$0.3$^{(0)}$ & -13.9 & -23.6 & 99 &   & 2\\ 
204226548 & 15 58 29.81 & -23 10 07.7 & 15.4 & 11.3 & -13.9$\pm$2.1 & -25.4$\pm$2.1 & 5.0$\pm$0.9$^{(1)}$ & -13.8 & -23.6 & 82 & 13.016 & 30\\ 
204230492 & 16 10 54.29 & -23 09 10.9 & 18.31 & 12.12 & 5.5$\pm$5.0 & -14.6$\pm$5.0 &   & -12.9 & -23.9 &   & 0.351 & 28\\ 
204232199 & 16 23 34.60 & -23 08 46.8 &   & 6.91 & 4.0$\pm$7.0 & 10.0$\pm$2.0 &   & -12.1 & -24.1 &   & & 21\\ 
204233911 & 16 12 43.72 & -23 08 23.0 & 15.07 & 10.92 & -2.8$\pm$2.1 & -28.3$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -12.8 & -23.9 & 72 & 1.739 & 28\\ 
204234295 & 15 55 32.44 & -23 08 17.2 & 16.08 & 12.48 & 20.9$\pm$2.1 & 4.1$\pm$2.1 &   & -14.0 & -23.5 &   & 18.454 & 30\\ 
204235325 & 16 14 52.70 & -23 08 02.7 & 13.57 & 9.6 & -19.4$\pm$2.2 & -27.1$\pm$2.2 & 10.0$\pm$1.8$^{(1)}$ & -12.7 & -24.0 & 92 & 23.717 & 1\\ 
204239132 & 16 22 51.78 & -23 07 07.5 & 7.71 & 6.62 & -11.7$\pm$1.2 & -25.2$\pm$1.1 & 7.6$\pm$1.1$^{(0)}$ & -12.1 & -24.1 & 97 &   & 2\\ 
204239143 & 16 11 38.37 & -23 07 07.3 & 17.5 & 12.78 & -12.0$\pm$2.5 & -31.4$\pm$2.5 & 4.9$\pm$0.9$^{(1)}$ & -12.9 & -23.9 & 63 & 0.72 & 28\\ 
204241103 & 16 01 19.16 & -23 06 39.4 &   & 12.67 & -5.5$\pm$5.0 & -26.3$\pm$5.0 & 2.6$\pm$0.5$^{(4)}$ & -13.6 & -23.6 &   & 0.572 & 27\\ 
204242194 & 16 10 25.36 & -23 06 23.4 &   & 7.24 & -17.7$\pm$0.9 & -31.0$\pm$0.6 & 9.1$\pm$0.8$^{(0)}$ & -13.0 & -23.9 & 93 &   & 2\\ 
204245509 & 16 14 11.08 & -23 05 36.2 & 10.07 & 7.46 & -10.1$\pm$1.4 & -26.8$\pm$1.4 & 10.3$\pm$1.9$^{(1)}$ & -12.7 & -23.9 & 94 &  & 5\\ 
204245943 & 16 12 45.07 & -23 05 30.3 & 17.06 & 12.46 & -9.0$\pm$2.5 & -22.6$\pm$2.5 & 5.0$\pm$0.9$^{(1)}$ & -12.8 & -23.9 & 74 & 0.755 & 17\\ 
204247416 & 15 57 50.03 & -23 05 09.5 & 12.35 & 9.27 & -13.9$\pm$2.2 & -25.6$\pm$2.2 & 5.7$\pm$1.0$^{(1)}$ & -13.8 & -23.6 & 92 & 7.848 & 10\\ 
204247509 & 15 59 25.92 & -23 05 08.2 &   & 11.57 & -11.7$\pm$3.9 & -29.3$\pm$3.9 & 12.3$\pm$2.3$^{(4)}$ & -13.7 & -23.6 & 87 & 0.62 & 27\\ 
204247811 & 16 13 12.12 & -23 05 03.2 & 18.65 & 13.01 &   &   &   & -12.8 & -23.9 &   & 1.155 & 18\\ 
204248645 & 16 02 45.75 & -23 04 50.9 & 15.86 & 11.5 & -19.7$\pm$2.1 & -34.2$\pm$2.1 & 6.4$\pm$1.2$^{(1)}$ & -13.5 & -23.7 & 81 & 0.262 & 27\\ 
204248842 & 15 57 03.69 & -23 04 48.3 & 14.29 & 10.21 & -12.3$\pm$2.1 & -22.4$\pm$2.1 & 8.8$\pm$1.6$^{(1)}$ & -13.9 & -23.5 & 95 & 0.83 & 1\\ 
204249804 & 15 58 58.21 & -23 04 35.2 & 13.39 & 9.88 & -12.9$\pm$2.2 & -25.1$\pm$2.2 & 5.8$\pm$1.1$^{(1)}$ & -13.7 & -23.6 & 93 & 3.904 & 1\\ 
204250417 & 16 15 13.61 & -23 04 26.1 & 18.75 & 13.92 & -13.5$\pm$3.3 & -29.6$\pm$3.3 & 4.0$\pm$0.7$^{(1)}$ & -12.6 & -24.0 & 8 & 1.344 & 17\\ 
204251947 & 16 11 56.33 & -23 04 04.6 & 12.48 &   & -16.8$\pm$2.2 & -15.0$\pm$2.2 &   & -12.9 & -23.9 &   &   & 5\\ 
204258708 & 16 02 09.56 & -23 02 27.7 & 16.02 & 11.83 & -10.2$\pm$2.1 & -24.8$\pm$2.1 & 4.7$\pm$0.9$^{(1)}$ & -13.5 & -23.7 & 67 & 0.484 & 27\\ 
204262828 & 16 13 42.65 & -23 01 27.9 & 17.49 & 12.79 & -12.4$\pm$3.3 & -24.7$\pm$3.3 & 5.2$\pm$1.0$^{(1)}$ & -12.7 & -23.9 & 83 &  & 28\\ 
204264641 & 16 14 02.12 & -23 01 02.2 & 11.01 & 8.61 & -10.2$\pm$1.0 & -22.0$\pm$1.0 & 5.6$\pm$1.0$^{(1)}$ & -12.7 & -23.9 & 91 & 2.991 & 5\\ 
204264833 & 16 23 07.78 & -23 00 59.6 & 11.22 & 8.18 & -15.1$\pm$1.6 & -26.4$\pm$1.6 & 9.6$\pm$1.8$^{(1)}$ & -12.1 & -24.1 & 95 & 4.084 & 5\\ 
204270520 & 16 00 26.31 & -22 59 41.3 &   & 11.34 & -8.4$\pm$5.0 & -30.0$\pm$5.0 & 6.1$\pm$1.1$^{(4)}$ & -13.6 & -23.6 & 87 & 0.512 & 27\\ 
204273100 & 16 08 02.18 & -22 59 05.8 & 15.58 & 11.26 & -10.9$\pm$2.1 & -23.4$\pm$2.1 & 7.0$\pm$1.3$^{(1)}$ & -13.1 & -23.8 & 96 & 0.512 & 28\\ 
204274536 & 16 23 32.84 & -22 58 46.9 &   & 10.29 & -17.4$\pm$3.9 & -27.0$\pm$3.9 & 63.2$\pm$11.6$^{(4)}$ & -12.1 & -24.1 & 32 & 5.126 & 21\\ 
204274743 & 15 57 29.86 & -22 58 43.8 & 15.38 & 11.19 & -14.3$\pm$2.1 & -18.3$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -13.8 & -23.6 & 89 & 1.769 & 30\\ 
204274993 & 15 56 55.46 & -22 58 40.4 & 12.81 & 9.43 & -10.8$\pm$2.2 & -25.5$\pm$2.2 & 6.2$\pm$1.1$^{(1)}$ & -13.9 & -23.5 & 94 & 8.183 & 1\\ 
204277211 & 16 01 40.87 & -22 58 10.6 & 15.11 & 9.85 & -12.1$\pm$2.2 & -31.0$\pm$2.2 & 22.5$\pm$4.1$^{(1)}$ & -13.6 & -23.6 & 43 & 2.561 & 30\\ 
204277248 & 16 26 19.98 & -22 58 10.0 & 14.51 & 10.54 & -7.9$\pm$2.2 & -26.6$\pm$2.2 & 6.1$\pm$1.1$^{(1)}$ & -11.9 & -24.2 & 92 & 3.091 & 1\\ 
204278916 & 16 02 07.58 & -22 57 46.9 & 13.49 & 9.86 & -14.8$\pm$2.2 & -23.9$\pm$2.2 & 5.9$\pm$1.1$^{(1)}$ & -13.5 & -23.7 & 94 & 3.636 & 30\\ 
204279000 & 16 20 32.46 & -22 57 45.5 & 14.02 & 9.77 & -15.2$\pm$2.3 & -25.3$\pm$2.3 & 9.6$\pm$1.8$^{(1)}$ & -12.3 & -24.1 & 95 & 4.401 & 1\\ 
204279085 & 16 13 02.72 & -22 57 44.5 & 11.19 & 8.45 & -9.5$\pm$1.0 & -25.5$\pm$1.0 & 6.7$\pm$1.2$^{(1)}$ & -12.8 & -23.9 & 95 & 2.088 & 5\\ 
204281210 & 15 58 36.92 & -22 57 15.3 & 9.83 & 7.05 & -11.5$\pm$1.4 & -21.2$\pm$0.6 & 6.0$\pm$0.4$^{(0)}$ & -13.8 & -23.6 & 95 & 2.446 & 31\\ 
204281213 & 15 58 36.91 & -22 57 15.2 & 9.83 &   & -11.5$\pm$1.4 & -21.2$\pm$0.6 &   & -13.8 & -23.6 &   &   & 31\\ 
204282380 & 15 56 29.54 & -22 56 58.2 & 14.25 & 10.39 & -2.1$\pm$2.0 & -26.0$\pm$2.0 & 6.0$\pm$1.1$^{(1)}$ & -13.9 & -23.5 & 51 & 3.0 & 30\\ 
204282976 & 16 02 58.55 & -22 56 49.6 & 13.68 & 10.11 & -8.0$\pm$2.1 & -24.1$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -13.5 & -23.7 & 83 & 1.865 & 30\\ 
204284515 & 16 00 19.44 & -22 56 28.8 & 18.71 & 13.48 &   &   &   & -13.6 & -23.6 &   & 0.928 & 27\\ 
204288433 & 16 09 46.34 & -22 55 33.5 & 15.17 & 11.03 & -3.7$\pm$2.1 & -23.7$\pm$2.1 & 6.2$\pm$1.2$^{(1)}$ & -13.0 & -23.8 & 78 & 1.816 & 28\\ 
204290833 & 16 02 08.45 & -22 54 59.1 & 12.96 & 9.55 & -10.8$\pm$2.2 & -22.0$\pm$2.2 & 6.0$\pm$1.1$^{(1)}$ & -13.5 & -23.7 & 93 & 6.192 & 1\\ 
204290918 & 16 21 18.48 & -22 54 57.8 & 14.94 & 10.15 & -9.8$\pm$2.2 & -23.1$\pm$2.1 & 11.5$\pm$2.1$^{(1)}$ & -12.2 & -24.1 & 90 & 2.536 & 21\\ 
204292655 & 16 11 45.30 & -22 54 32.9 &   & 11.81 & 9.2$\pm$3.9 & -29.1$\pm$3.9 &   & -12.9 & -23.9 &   & 1.558 & 3\\ 
204296346 & 16 20 50.96 & -22 53 40.0 & 13.57 & 9.8 & -13.2$\pm$2.4 & -21.2$\pm$2.3 & 6.4$\pm$1.2$^{(1)}$ & -12.2 & -24.1 & 94 & 8.234 & 1\\ 
204296945 & 16 11 23.99 & -22 53 32.6 & 14.36 & 10.65 & -10.9$\pm$2.1 & -21.3$\pm$2.1 & 4.8$\pm$0.9$^{(1)}$ & -12.9 & -23.9 & 71 & 11.922 & 28\\ 
204303402 & 16 17 13.81 & -22 51 58.5 & 14.83 & 10.86 & -11.6$\pm$2.5 & -25.4$\pm$2.5 & 5.8$\pm$1.1$^{(1)}$ & -12.5 & -24.0 & 93 & 1.572 & 1\\ 
204305663 & 15 59 30.21 & -22 51 26.4 & 16.66 & 12.43 & 47.9$\pm$2.5 & -29.3$\pm$2.5 &   & -13.7 & -23.6 &   &  & 30\\ 
204315134 & 16 00 54.46 & -22 49 09.0 & 14.5 & 10.93 &   & -52.0$\pm$2.1 &   & -13.6 & -23.6 &   & 47.607 & 30\\ 
204317053 & 16 02 41.43 & -22 48 41.9 & 16.64 & 12.0 & -8.1$\pm$2.1 & -30.9$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -13.5 & -23.7 & 86 & 1.593 & 17\\ 
204317321 & 16 01 29.84 & -22 48 38.5 & 14.8 & 10.49 & -9.4$\pm$2.1 & -19.8$\pm$2.1 & 9.3$\pm$1.7$^{(1)}$ & -13.6 & -23.6 & 90 & 1.931 & 30\\ 
204321428 & 16 08 14.00 & -22 47 39.3 & 14.71 & 10.73 & -11.2$\pm$2.1 & -26.1$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -13.1 & -23.8 & 93 & 1.543 & 28\\ 
204321959 & 16 20 06.86 & -22 47 32.1 & 14.97 & 10.79 & -11.0$\pm$2.1 & -18.9$\pm$2.1 & 7.1$\pm$1.3$^{(1)}$ & -12.3 & -24.0 & 92 & 0.781 & 1\\ 
204322706 & 16 02 55.13 & -22 47 20.8 & 14.48 & 10.57 & -9.6$\pm$2.1 & -25.6$\pm$2.1 & 5.9$\pm$1.1$^{(1)}$ & -13.5 & -23.7 & 92 & 3.099 & 3\\ 
204324196 & 16 08 46.06 & -22 46 59.3 & 14.74 & 10.88 & -9.0$\pm$2.1 & -20.7$\pm$2.1 & 4.8$\pm$0.9$^{(1)}$ & -13.1 & -23.8 & 63 & 3.132 & 28\\ 
204324250 & 15 58 48.44 & -22 46 58.5 & 14.34 & 11.33 &   &   &   & -13.7 & -23.6 &   &  & 30\\ 
204328391 & 16 09 09.39 & -22 45 59.0 & 14.31 & 10.53 & -12.5$\pm$2.1 & -22.6$\pm$2.1 & 5.2$\pm$1.0$^{(1)}$ & -13.0 & -23.8 & 86 & 5.42 & 28\\ 
204328600 & 16 03 35.50 & -22 45 56.2 & 10.52 & 8.36 & -12.9$\pm$1.7 & -24.2$\pm$0.3 & 6.9$\pm$0.3$^{(0)}$ & -13.4 & -23.7 & 98 & 2.424 & 10\\ 
204330772 & 15 57 37.18 & -22 45 25.2 & 16.16 & 12.56 & -16.3$\pm$2.5 & -13.6$\pm$2.5 &   & -13.8 & -23.5 &   & 24.473 & 30\\ 
204330803 & 16 03 46.95 & -22 45 24.8 & 12.74 & 9.1 & -11.5$\pm$2.2 & -23.8$\pm$2.2 & 9.0$\pm$1.7$^{(1)}$ & -13.4 & -23.7 & 95 & 13.052 & 1\\ 
204330922 & 16 27 39.54 & -22 45 23.1 & 11.05 & 8.08 & -5.9$\pm$1.0 & -23.9$\pm$0.7 & 7.7$\pm$0.3$^{(0)}$ & -11.8 & -24.2 & 94 & 4.182 & 5\\ 
204332672 & 16 14 13.51 & -22 44 57.8 & 15.51 & 11.42 & -9.4$\pm$2.1 & -22.7$\pm$2.1 & 5.0$\pm$0.9$^{(1)}$ & -12.7 & -23.9 & 78 & 2.635 & 17\\ 
204337881 & 16 16 09.47 & -22 43 43.8 & 14.16 & 10.51 & -12.1$\pm$2.1 & -20.1$\pm$2.1 & 4.9$\pm$0.9$^{(1)}$ & -12.6 & -23.9 & 70 & 9.459 & 1\\ 
204341806 & 16 07 37.99 & -22 42 46.8 &   &   &   &   &   & -13.1 & -23.8 &   &   & 29\\ 
204342099 & 16 15 34.57 & -22 42 42.5 & 12.07 & 7.91 & -15.2$\pm$2.2 & -31.1$\pm$2.2 & 12.8$\pm$2.4$^{(1)}$ & -12.6 & -23.9 & 86 & 8.114 & 5\\ 
204342846 & 16 01 32.95 & -22 42 31.6 & 14.56 & 11.31 & -11.8$\pm$2.1 & -5.8$\pm$2.1 & 2.5$\pm$0.5$^{(1)}$ & -13.5 & -23.6 &   & 42.601 & 30\\ 
204344180 & 16 14 32.87 & -22 42 13.3 & 18.22 & 13.24 & -10.3$\pm$3.3 & -22.4$\pm$3.3 & 5.5$\pm$1.0$^{(1)}$ & -12.7 & -23.9 & 87 & 1.817 & 17\\ 
204346960 & 16 19 51.44 & -22 41 33.3 & 18.63 & 13.43 & -10.8$\pm$3.9 & -17.3$\pm$3.9 & 5.5$\pm$1.0$^{(1)}$ & -12.3 & -24.0 & 75 & 6.808 & 3\\ 
204347304 & 16 02 10.45 & -22 41 28.3 & 10.76 & 8.06 & -17.5$\pm$1.0 & -33.6$\pm$1.1 & 8.5$\pm$1.6$^{(1)}$ & -13.5 & -23.6 & 92 & 3.514 & 26\\ 
204347422 & 16 19 51.41 & -22 41 26.7 & 16.91 & 12.18 & -9.2$\pm$2.1 & -21.1$\pm$2.2 & 6.4$\pm$1.2$^{(1)}$ & -12.3 & -24.0 & 93 & 6.846 & 3\\ 
204348206 & 16 02 13.56 & -22 41 15.2 & 7.32 & 6.97 & -12.5$\pm$0.0 & -23.1$\pm$0.0 & 6.3$\pm$0.3$^{(0)}$ & -13.5 & -23.6 & 99 & $<$2 & 2\\ 
204350593 & 16 00 41.35 & -22 40 41.6 & 13.49 & 9.64 & -8.4$\pm$2.2 & -28.0$\pm$2.2 & 8.7$\pm$1.6$^{(1)}$ & -13.6 & -23.6 & 93 & 3.154 & 3\\ 
204350686 & 16 01 25.64 & -22 40 40.3 & 11.14 & 8.52 & -12.1$\pm$1.4 & -23.5$\pm$0.6 & 7.1$\pm$0.3$^{(0)}$ & -13.6 & -23.6 & 98 & 2.395 & 26\\ 
204350687 & 16 01 25.62 & -22 40 40.3 & 11.14 &   & -12.1$\pm$1.4 & -23.5$\pm$0.6 &   & -13.6 & -23.6 &   &   & 26\\ 
204350917 & 16 15 38.67 & -22 40 37.1 & 16.09 & 11.69 & 6.4$\pm$2.6 & -20.2$\pm$2.6 &   & -12.6 & -23.9 &   & $<$2 & 28\\ 
204350926 & 16 01 58.94 & -22 40 37.0 & 14.28 & 10.43 & -18.6$\pm$2.1 & -27.3$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -13.5 & -23.6 & 93 & 0.73 & 30\\ 
204351607 & 15 56 25.63 & -22 40 27.2 & 14.28 & 10.37 & -14.9$\pm$2.0 & -24.5$\pm$2.0 & 6.4$\pm$1.2$^{(1)}$ & -13.9 & -23.5 & 96 & 1.386 & 30\\ 
204353205 & 16 21 15.84 & -22 40 04.6 & 13.69 & 9.75 & -10.7$\pm$2.3 & -25.3$\pm$2.3 & 7.7$\pm$1.4$^{(1)}$ & -12.2 & -24.0 & 96 & 6.039 & 1\\ 
204354278 & 16 10 47.14 & -22 39 49.3 & 19.98 & 14.02 &   &   &   & -12.9 & -23.8 &   & 16.704 & 28\\ 
204355491 & 16 24 51.37 & -22 39 32.5 & 9.26 & 7.08 & -10.9$\pm$1.4 & -27.1$\pm$0.6 & 7.1$\pm$0.4$^{(0)}$ & -12.0 & -24.1 & 98 & $<$2 & 5\\ 
204355829 & 16 15 27.43 & -22 39 27.6 & 14.26 & 10.49 & -10.3$\pm$2.1 & -23.2$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -12.6 & -23.9 & 90 & 1.722 & 28\\ 
204357531 & 16 07 27.82 & -22 39 04.1 &   & 15.42 &   &   &   & -13.1 & -23.8 &   &   & 29\\ 
204364515 & 16 01 21.56 & -22 37 26.5 & 14.36 & 10.05 & -13.7$\pm$2.1 & -27.6$\pm$2.1 & 11.6$\pm$2.1$^{(1)}$ & -13.6 & -23.6 & 92 & 3.091 & 30\\ 
204365837 & 16 11 31.81 & -22 37 08.2 & 16.25 & 11.85 & -7.8$\pm$2.1 & -22.0$\pm$2.1 & 5.9$\pm$1.1$^{(1)}$ & -12.9 & -23.8 & 89 & 1.743 & 28\\ 
204365840 & 16 32 01.36 & -22 37 08.2 &   & 12.27 & -25.6$\pm$5.5 & -16.5$\pm$5.5 & 32.7$\pm$6.0$^{(4)}$ & -11.5 & -24.2 & 3 & $<$2 & 3\\ 
204367097 & 16 00 17.30 & -22 36 50.4 & 13.89 & 9.94 & 27.1$\pm$7.8 & -22.4$\pm$7.8 &   & -13.6 & -23.6 &   & 18.695 & 3\\ 
204367110 & 15 59 12.45 & -22 36 50.2 & 16.17 & 11.79 & -16.7$\pm$2.1 & -26.5$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -13.7 & -23.6 & 92 & 0.944 & 30\\ 
204367193 & 16 11 54.39 & -22 36 49.2 & 18.08 & 13.3 & -15.9$\pm$2.5 & -21.4$\pm$2.5 & 4.5$\pm$0.8$^{(1)}$ & -12.8 & -23.8 & 43 & 0.483 & 28\\ 
204369652 & 16 02 02.85 & -22 36 14.1 & 15.32 &   & -30.9$\pm$2.1 & -32.7$\pm$2.1 &   & -13.5 & -23.6 &   &   & 30\\ 
204371512 & 16 08 47.44 & -22 35 47.8 &   & 14.5 &   &   &   & -13.0 & -23.8 &   & 0.736 & 29\\ 
204372172 & 16 20 50.23 & -22 35 38.8 & 8.86 & 7.78 & -10.3$\pm$0.2 & -19.9$\pm$0.1 & 7.2$\pm$1.8$^{(0)}$ & -12.2 & -24.0 & 90 &  & 2\\ 
204376053 & 16 03 14.88 & -22 34 45.6 & 15.03 & 10.7 & -10.8$\pm$2.1 & -28.3$\pm$2.1 & 8.9$\pm$1.6$^{(1)}$ & -13.4 & -23.7 & 95 & 2.03 & 1\\ 
204382154 & 16 13 40.27 & -22 33 19.3 &   & 12.57 & -37.9$\pm$5.0 & -64.5$\pm$5.0 &   & -12.7 & -23.9 &   & 1.718 & 3\\ 
204382615 & 16 26 20.16 & -22 33 12.7 & 14.41 & 10.41 & -9.4$\pm$2.1 & -29.1$\pm$2.1 & 6.4$\pm$1.2$^{(1)}$ & -11.9 & -24.1 & 93 & 23.162 & 1\\ 
204383288 & 16 26 19.98 & -22 33 02.5 & 13.49 & 9.82 & -15.6$\pm$2.4 & -20.7$\pm$2.4 & 6.5$\pm$1.2$^{(1)}$ & -11.9 & -24.1 & 92 & 23.178 & 1\\ 
204385932 & 16 08 18.44 & -22 32 24.8 &   & 14.78 &   &   &   & -13.1 & -23.8 &   & 35.904 & 28\\ 
204387835 & 16 00 15.67 & -22 31 58.1 & 14.27 & 10.44 & -9.7$\pm$2.2 & -26.5$\pm$2.2 & 6.3$\pm$1.2$^{(1)}$ & -13.6 & -23.6 & 93 & 2.38 & 3\\ 
204388140 & 16 09 39.68 & -22 31 53.9 & 14.73 & 10.74 & -8.9$\pm$2.1 & -25.3$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -13.0 & -23.8 & 93 & 3.728 & 28\\ 
204392438 & 16 10 26.49 & -22 30 53.4 & 14.53 & 10.47 & -6.6$\pm$2.1 & -25.8$\pm$2.1 & 6.9$\pm$1.3$^{(1)}$ & -12.9 & -23.8 & 92 & 0.925 & 28\\ 
204393705 & 16 13 26.66 & -22 30 34.8 & 17.39 & 12.58 & -3.0$\pm$2.7 & -29.0$\pm$2.6 & 6.2$\pm$1.1$^{(1)}$ & -12.7 & -23.9 & 72 & 1.532 & 28\\ 
204395172 & 16 00 04.13 & -22 30 14.1 & 15.63 & 12.03 &   & 29.7$\pm$2.2 &   & -13.6 & -23.6 &   &  & 30\\ 
204395393 & 16 00 18.43 & -22 30 11.4 & 14.67 & 10.41 & -12.7$\pm$2.1 & -21.4$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -13.6 & -23.6 & 95 & 19.8 & 30\\ 
204396010 & 16 25 43.22 & -22 30 02.6 & 16.47 & 12.09 & -13.8$\pm$2.6 & -31.7$\pm$2.6 & 5.3$\pm$1.0$^{(1)}$ & -11.9 & -24.1 & 75 & 1.56 & 18\\ 
204397408 & 16 08 10.82 & -22 29 42.8 & 16.1 & 11.68 & -6.8$\pm$2.1 & -25.8$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -13.1 & -23.8 & 92 & 1.645 & 17\\ 
204398735 & 16 01 42.54 & -22 29 24.0 & 13.48 & 10.22 & -62.5$\pm$2.2 & -68.8$\pm$2.2 &   & -13.5 & -23.6 &   & 38.024 & 30\\ 
204398857 & 16 09 31.65 & -22 29 22.4 & 12.85 & 9.15 & -13.0$\pm$2.3 & -20.6$\pm$2.2 & 9.2$\pm$1.7$^{(1)}$ & -13.0 & -23.8 & 94 & 12.889 & 1\\ 
204399028 & 15 57 46.62 & -22 29 20.2 & 14.28 & 10.46 & -14.5$\pm$2.1 & -23.5$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -13.8 & -23.5 & 94 & 3.863 & 30\\ 
204399319 & 16 13 20.55 & -22 29 15.9 & 13.72 & 10.24 & -8.0$\pm$2.1 & -19.9$\pm$2.1 & 5.1$\pm$0.9$^{(1)}$ & -12.7 & -23.9 & 71 & 3.909 & 1\\ 
204399436 & 16 00 43.18 & -22 29 14.3 & 19.45 & 14.3 &   &   &   & -13.6 & -23.6 &   & & 3\\ 
204399980 & 16 13 11.59 & -22 29 06.7 & 8.67 & 6.69 & -8.5$\pm$0.1 & -23.5$\pm$0.1 & 6.7$\pm$0.2$^{(0)}$ & -12.7 & -23.9 & 97 & 16.53 & 2\\ 
204401119 & 16 11 07.38 & -22 28 50.1 &   & 11.33 & -6.1$\pm$3.9 & -35.2$\pm$3.9 & 18.8$\pm$3.5$^{(4)}$ & -12.9 & -23.8 & 24 & 1.79 & 17\\ 
204402572 & 16 19 33.96 & -22 28 29.4 & 11.0 & 8.51 & -9.6$\pm$1.0 & -26.5$\pm$1.0 & 6.6$\pm$1.2$^{(1)}$ & -12.3 & -24.0 & 95 & 4.031 & 5\\ 
204404080 & 16 12 39.55 & -22 28 08.2 & 14.27 & 10.42 & -13.4$\pm$2.1 & -24.3$\pm$2.1 & 6.1$\pm$1.1$^{(1)}$ & -12.8 & -23.8 & 94 & 1.962 & 28\\ 
204406748 & 16 01 05.19 & -22 27 31.2 & 12.39 & 8.75 & -9.5$\pm$2.2 & -27.8$\pm$2.2 & 10.6$\pm$2.0$^{(1)}$ & -13.6 & -23.6 & 91 & 17.248 & 26\\ 
204408619 & 16 14 41.20 & -22 27 05.4 & 14.79 & 10.87 & -11.1$\pm$2.1 & -26.3$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -12.6 & -23.9 & 90 & 2.631 & 28\\ 
204409463 & 16 12 55.28 & -22 26 54.2 &   & 11.39 & -8.7$\pm$3.9 & -44.6$\pm$3.9 & 12.5$\pm$2.3$^{(4)}$ & -12.8 & -23.9 & 22 & 1.756 & 28\\ 
204412942 & 15 57 42.50 & -22 26 05.5 & 15.24 & 11.42 & -17.1$\pm$2.1 & -27.5$\pm$2.1 & 4.1$\pm$0.8$^{(1)}$ & -13.8 & -23.5 & 14 & 1.445 & 30\\ 
204413519 & 16 08 40.59 & -22 25 57.1 & 17.05 & 13.22 & -43.0$\pm$2.5 & -11.1$\pm$2.5 &   & -13.0 & -23.8 &   & 18.429 & 17\\ 
204413641 & 15 56 24.77 & -22 25 55.3 & 14.97 & 10.79 & -13.3$\pm$2.0 & -23.2$\pm$2.0 & 6.8$\pm$1.3$^{(1)}$ & -13.9 & -23.5 & 96 & 1.969 & 30\\ 
204414610 & 16 17 06.07 & -22 25 41.2 & 15.27 & 11.24 & -9.2$\pm$2.1 & -21.9$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -12.5 & -23.9 & 86 & 3.651 & 1\\ 
204417450 & 16 08 08.47 & -22 25 00.1 & 14.43 & 10.78 & -11.3$\pm$2.1 & -23.4$\pm$2.1 & 4.6$\pm$0.8$^{(1)}$ & -13.1 & -23.7 & 63 & 9.199 & 28\\ 
204418005 & 16 09 04.52 & -22 24 52.4 &   & 11.99 & -7.0$\pm$5.0 & -30.6$\pm$5.0 & 26.1$\pm$4.8$^{(4)}$ & -13.0 & -23.8 & 24 & 2.181 & 17\\ 
204418342 & 16 19 48.77 & -22 24 47.5 & 14.93 & 10.83 & -22.7$\pm$2.2 & -30.4$\pm$2.1 & 7.7$\pm$1.4$^{(1)}$ & -12.3 & -24.0 & 83 & 0.476 & 1\\ 
204421329 & 16 00 07.14 & -22 24 06.6 & 16.41 & 12.54 & -26.1$\pm$2.1 & -7.0$\pm$2.1 & 2.3$\pm$0.4$^{(1)}$ & -13.6 & -23.6 &   & 0.696 & 30\\ 
204422391 & 15 57 44.91 & -22 23 51.6 &   & 10.77 & 2.0$\pm$1.6 & 15.4$\pm$1.7 &   & -13.8 & -23.5 &   & 40.047 & 30\\ 
204426231 & 16 07 45.22 & -22 22 57.4 & 15.81 & 11.52 & 0.3$\pm$2.1 & -25.3$\pm$2.1 &   & -13.1 & -23.7 &   & 2.252 & 28\\ 
204428324 & 16 01 10.37 & -22 22 27.6 & 13.82 & 9.76 & -11.8$\pm$2.2 & -24.6$\pm$2.2 & 10.1$\pm$1.9$^{(1)}$ & -13.6 & -23.6 & 94 & 0.325 & 30\\ 
204428864 & 16 08 15.67 & -22 22 20.1 & 13.52 & 9.95 & -7.2$\pm$2.2 & -21.9$\pm$2.2 & 6.4$\pm$1.2$^{(1)}$ & -13.1 & -23.7 & 90 & 18.022 & 28\\ 
204429883 & 16 09 20.64 & -22 22 05.7 & 13.92 & 9.5 & -8.5$\pm$2.3 & -18.2$\pm$2.2 & 16.4$\pm$3.0$^{(1)}$ & -13.0 & -23.8 & 51 & $<$2 & 1\\ 
204432860 & 16 02 00.39 & -22 21 23.9 & 12.37 & 8.84 & -11.0$\pm$2.2 & -25.0$\pm$2.2 & 9.2$\pm$1.7$^{(1)}$ & -13.5 & -23.6 & 95 & 2.875 & 1\\ 
204434363 & 16 07 50.40 & -22 21 02.2 &   & 11.34 & -8.0$\pm$3.9 & -28.0$\pm$3.9 & 34.9$\pm$6.4$^{(4)}$ & -13.1 & -23.7 & 24 & 1.596 & 28\\ 
204436170 & 15 59 59.95 & -22 20 36.8 & 12.08 & 8.63 & -12.7$\pm$1.2 & -23.4$\pm$1.2 & 9.3$\pm$1.7$^{(1)}$ & -13.6 & -23.6 & 96 & 0.862 & 1\\ 
204437393 & 16 02 23.67 & -22 20 19.4 & 13.42 & 9.62 & -8.6$\pm$2.2 & -23.5$\pm$2.2 & 8.3$\pm$1.5$^{(1)}$ & -13.5 & -23.6 & 94 & 1.499 & 3\\ 
204439731 & 16 13 40.80 & -22 19 46.0 &   & 13.67 &   &   &   & -12.7 & -23.9 &   & 1.336 & 28\\ 
204439854 & 16 11 34.70 & -22 19 44.2 & 16.87 & 12.33 & 19.0$\pm$10.4 & 21.9$\pm$10.4 &   & -12.8 & -23.8 &   & 0.597 & 28\\ 
204440160 & 16 11 34.95 & -22 19 40.0 & 18.29 &   & -3.0$\pm$2.1 & -0.2$\pm$2.1 &   & -12.8 & -23.8 &   &   & 28\\ 
204440603 & 16 14 23.13 & -22 19 33.8 & 15.23 & 10.8 & -8.7$\pm$2.1 & -24.9$\pm$2.1 & 9.0$\pm$1.7$^{(1)}$ & -12.7 & -23.9 & 94 &   & 28\\ 
204442667 & 15 57 28.49 & -22 19 05.1 & 15.88 & 11.6 & -12.4$\pm$2.1 & -24.6$\pm$2.1 & 5.9$\pm$1.1$^{(1)}$ & -13.8 & -23.5 & 94 & 1.318 & 30\\ 
204446383 & 16 00 17.33 & -22 18 11.1 & 16.02 & 12.26 &   &   &   & -13.6 & -23.6 &   & 33.139 & 30\\ 
204446677 & 16 08 05.55 & -22 18 07.0 & 13.49 & 9.85 & -4.6$\pm$2.2 & -24.4$\pm$2.2 & 6.8$\pm$1.2$^{(1)}$ & -13.1 & -23.7 & 85 & 5.605 & 28\\ 
204447221 & 16 09 41.00 & -22 17 59.5 & 11.61 & 8.44 & -10.0$\pm$1.0 & -23.7$\pm$1.1 & 7.6$\pm$1.4$^{(1)}$ & -13.0 & -23.8 & 96 & 9.72 & 5\\ 
204448136 & 16 09 08.84 & -22 17 46.7 & 16.24 & 12.07 & -16.1$\pm$2.1 & -34.3$\pm$2.1 & 4.4$\pm$0.8$^{(1)}$ & -13.0 & -23.8 & 9 & 24.868 & 17\\ 
204449165 & 16 14 07.34 & -22 17 32.2 & 12.68 & 9.1 & -9.7$\pm$2.2 & -22.2$\pm$2.2 & 8.4$\pm$1.5$^{(1)}$ & -12.7 & -23.9 & 95 & 0.617 & 1\\ 
204449274 & 16 22 21.60 & -22 17 30.7 &   & 12.62 & -18.1$\pm$3.9 & -21.6$\pm$3.9 & 20.7$\pm$3.8$^{(4)}$ & -12.1 & -24.0 & 44 & 1.549 & 18\\ 
204449800 & 16 14 10.12 & -22 17 23.5 & 14.35 & 9.81 & -4.6$\pm$2.2 & -16.7$\pm$2.2 & 16.5$\pm$3.0$^{(1)}$ & -12.7 & -23.9 & 21 & 2.447 & 1\\ 
204450240 & 16 11 17.12 & -22 17 17.4 & 18.36 & 13.25 & -87.8$\pm$8.2 &   &   & -12.9 & -23.8 &   &  & 18\\ 
204451272 & 16 08 22.29 & -22 17 02.9 & 16.48 & 12.03 & -14.6$\pm$2.1 & -24.2$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -13.1 & -23.7 & 89 & 0.973 & 28\\ 
204454456 & 16 19 43.09 & -22 16 17.6 & 15.25 & 11.3 & -17.7$\pm$2.1 & -22.7$\pm$2.1 & 4.9$\pm$0.9$^{(1)}$ & -12.3 & -24.0 & 62 & 3.187 & 1\\ 
204458208 & 16 01 06.05 & -22 15 24.5 & 15.4 & 11.38 & -9.5$\pm$2.1 & -25.0$\pm$2.1 & 5.2$\pm$1.0$^{(1)}$ & -13.6 & -23.6 & 83 & 1.758 & 30\\ 
204458254 & 15 57 29.20 & -22 15 23.7 & 16.54 & 12.56 & -37.9$\pm$2.2 & -10.5$\pm$2.2 &   & -13.8 & -23.5 &   & 1.189 & 30\\ 
204459941 & 16 13 43.66 & -22 14 59.5 & 12.3 & 9.11 & -8.6$\pm$2.2 & -17.3$\pm$2.2 & 6.2$\pm$1.2$^{(1)}$ & -12.7 & -23.9 & 83 & 4.663 & 0\\ 
204460283 & 16 25 29.70 & -22 14 54.4 & 16.97 & 12.11 & -8.4$\pm$2.6 & -20.5$\pm$2.6 & 7.0$\pm$1.3$^{(1)}$ & -11.9 & -24.1 & 92 & 1.396 & 18\\ 
204464537 & 16 26 56.20 & -22 13 51.9 &   & 12.41 & -13.1$\pm$5.1 & -37.4$\pm$5.1 & 22.1$\pm$4.1$^{(4)}$ & -11.8 & -24.1 & 24 & 0.284 & 18\\ 
204464828 & 16 10 28.88 & -22 13 47.9 & 9.25 & 7.23 & -10.5$\pm$0.1 & -24.5$\pm$0.1 & 6.5$\pm$0.4$^{(0)}$ & -12.9 & -23.8 & 99 & 2.275 & 6\\ 
204465961 & 16 12 46.81 & -22 13 31.7 & 10.66 & 8.03 & -7.5$\pm$1.5 & -24.5$\pm$0.8 & 7.4$\pm$0.3$^{(0)}$ & -12.8 & -23.8 & 96 & 10.553 & 0\\ 
204467584 & 16 11 17.07 & -22 13 08.7 & 14.86 & 10.58 & -11.7$\pm$2.1 & -25.6$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -12.9 & -23.8 & 96 & 2.072 & 28\\ 
204468718 & 16 19 48.37 & -22 12 51.8 & 13.96 & 10.32 & -14.4$\pm$2.1 & -25.6$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -12.3 & -24.0 & 88 & 15.268 & 1\\ 
204468732 & 16 10 49.96 & -22 12 51.6 & 16.39 & 11.73 & -11.7$\pm$2.5 & -23.9$\pm$2.5 & 7.0$\pm$1.3$^{(1)}$ & -12.9 & -23.8 & 96 & 0.77 & 7\\ 
204468888 & 16 13 18.58 & -22 12 49.0 & 9.97 & 7.43 & -9.8$\pm$2.6 & -19.6$\pm$1.3 & 5.9$\pm$0.8$^{(0)}$ & -12.7 & -23.8 & 90 & 5.864 & 5\\ 
204469637 & 16 20 06.16 & -22 12 38.5 & 14.52 & 10.65 & -13.3$\pm$2.1 & -26.4$\pm$2.1 & 5.7$\pm$1.0$^{(1)}$ & -12.3 & -24.0 & 92 & 4.913 & 1\\ 
204472125 & 16 09 56.96 & -22 12 02.7 & 17.22 & 12.66 & -4.1$\pm$2.5 & -20.8$\pm$2.5 & 4.8$\pm$0.9$^{(1)}$ & -13.0 & -23.8 & 34 & 0.815 & 17\\ 
204476372 & 16 07 23.82 & -22 11 01.9 & 19.76 & 14.09 & -24.6$\pm$3.8 & -21.0$\pm$3.6 & 4.9$\pm$0.9$^{(1)}$ & -13.1 & -23.7 & 26 & 0.572 & 28\\ 
204477741 & 15 59 18.39 & -22 10 43.0 & 14.19 & 10.07 & -11.5$\pm$2.1 & -23.1$\pm$2.1 & 9.3$\pm$1.7$^{(1)}$ & -13.7 & -23.5 & 95 & 0.822 & 30\\ 
204478864 & 16 11 37.85 & -22 10 27.4 & 13.97 & 10.13 & -8.0$\pm$2.1 & -24.2$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -12.8 & -23.8 & 93 & 1.103 & 28\\ 
204483334 & 16 00 28.45 & -22 09 22.9 & 16.72 & 12.52 & -55.8$\pm$2.1 & -27.5$\pm$2.1 &   & -13.6 & -23.6 &   &  & 30\\ 
204484164 & 16 10 26.25 & -22 09 10.6 & 13.0 & 9.02 & -8.4$\pm$2.2 & -27.0$\pm$2.2 & 11.6$\pm$2.1$^{(1)}$ & -12.9 & -23.8 & 88 & $<$2& 1\\ 
204492384 & 16 15 10.45 & -22 07 10.0 & 9.99 & 8.54 & -9.7$\pm$0.1 & -20.1$\pm$0.1 & 6.0$\pm$0.3$^{(0)}$ & -12.6 & -23.9 & 93 & 0.878 & 2\\ 
204494633 & 16 07 00.52 & -22 06 36.2 & 14.23 & 10.44 & -10.5$\pm$2.1 & -21.3$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -13.1 & -23.7 & 92 & 2.511 & 3\\ 
204494885 & 16 21 21.15 & -22 06 32.3 & 8.47 & 7.37 & -18.8$\pm$0.2 & -17.9$\pm$0.1 & 6.9$\pm$1.2$^{(0)}$ & -12.2 & -24.0 & 80 &  & 2\\ 
204496657 & 15 57 06.42 & -22 06 06.1 & 15.53 & 11.29 & -14.7$\pm$2.1 & -19.5$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -13.8 & -23.5 & 51 & 0.899 & 30\\ 
204499729 & 16 16 32.27 & -22 05 20.1 &   & 12.71 & -15.7$\pm$5.0 & -20.4$\pm$5.0 & 18.8$\pm$3.5$^{(4)}$ & -12.5 & -23.9 & 52 & 1.512 & 7\\ 
204506777 & 16 07 17.79 & -22 03 36.6 & 8.45 & 7.05 & -10.8$\pm$0.1 & -24.6$\pm$0.1 & 7.5$\pm$0.3$^{(0)}$ & -13.1 & -23.7 & 97 & $<$2 & 6\\ 
204507317 & 16 08 50.36 & -22 03 28.7 & 14.81 & 10.83 & -9.1$\pm$2.1 & -22.7$\pm$2.1 & 5.3$\pm$1.0$^{(1)}$ & -13.0 & -23.7 & 85 & 3.868 & 28\\ 
204508462 & 16 19 47.12 & -22 03 11.2 & 14.6 & 10.54 & -11.1$\pm$2.1 & -26.3$\pm$2.1 & 7.3$\pm$1.3$^{(1)}$ & -12.3 & -24.0 & 96 & 0.786 & 1\\ 
204514546 & 15 56 40.02 & -22 01 40.0 & 8.62 & 6.08 & -13.2$\pm$0.6 & -22.7$\pm$0.4 & 6.7$\pm$0.2$^{(0)}$ & -13.8 & -23.5 & 98 & 37.534 & 32\\ 
204514548 & 15 56 40.02 & -22 01 40.0 & 8.62 &   & -13.2$\pm$0.6 & -22.7$\pm$0.4 &   & -13.8 & -23.5 &   &   & 32\\ 
204516435 & 16 34 28.50 & -22 01 11.9 &   & 12.1 & -6.8$\pm$5.2 & -28.6$\pm$5.2 & 27.3$\pm$5.0$^{(4)}$ & -11.3 & -24.2 & 29 & 0.583 & 15\\ 
204517282 & 16 09 29.71 & -22 00 58.0 & 13.21 & 9.57 & -8.4$\pm$2.2 & -25.5$\pm$2.2 & 7.0$\pm$1.3$^{(1)}$ & -13.0 & -23.7 & 94 & 2.933 & 1\\ 
204517888 & 16 02 32.27 & -22 00 48.7 &   & 12.34 & 0.7$\pm$5.1 & -22.0$\pm$5.1 &   & -13.4 & -23.6 &   &  & 3\\ 
204518032 & 16 09 39.70 & -22 00 46.6 & 12.76 & 9.3 & -8.7$\pm$2.2 & -25.4$\pm$2.2 & 6.9$\pm$1.3$^{(1)}$ & -13.0 & -23.7 & 95 & 6.547 & 1\\ 
204518814 & 16 02 34.19 & -22 00 35.5 &   & 11.75 & -7.1$\pm$5.1 & -23.3$\pm$5.1 & 29.5$\pm$5.4$^{(4)}$ & -13.4 & -23.6 & 23 &  & 3\\ 
204519031 & 16 00 40.55 & -22 00 32.2 & 10.7 & 8.44 & -5.9$\pm$1.8 & -22.1$\pm$0.3 & 8.0$\pm$0.5$^{(0)}$ & -13.6 & -23.6 & 83 & 2.723 & 10\\ 
204519555 & 16 02 24.61 & -22 00 24.8 & 12.68 & 9.38 & -9.4$\pm$2.2 & -22.3$\pm$2.2 & 6.1$\pm$1.1$^{(1)}$ & -13.5 & -23.6 & 92 & 0.895 & 3\\ 
204520585 & 16 26 41.20 & -22 00 09.6 & 13.11 & 9.34 & -12.1$\pm$1.1 & -22.4$\pm$1.1 & 8.2$\pm$1.5$^{(1)}$ & -11.8 & -24.1 & 96 & 19.404 & 1\\ 
204522817 & 16 12 28.95 & -21 59 35.8 &   & 15.0 &   &   &   & -12.8 & -23.8 &   & 1.103 & 29\\ 
204524752 & 16 23 17.41 & -21 59 07.0 & 14.28 & 10.16 & -11.2$\pm$2.2 & -24.2$\pm$2.2 & 7.9$\pm$1.5$^{(1)}$ & -12.0 & -24.0 & 96 & 2.96 & 1\\ 
204525772 & 16 13 38.35 & -21 58 52.0 & 15.05 & 11.0 & -9.1$\pm$2.1 & -20.8$\pm$2.1 & 5.8$\pm$1.1$^{(1)}$ & -12.7 & -23.8 & 89 & 1.547 & 1\\ 
204525799 & 16 26 38.63 & -21 58 51.6 & 14.95 & 10.73 & -16.5$\pm$2.2 & -24.6$\pm$2.2 & 6.5$\pm$1.2$^{(1)}$ & -11.8 & -24.1 & 93 & 2.012 & 15\\ 
204525956 & 16 01 55.46 & -21 58 49.4 & 7.17 & 6.9 & -12.1$\pm$0.0 & -24.1$\pm$0.0 & 7.1$\pm$0.5$^{(0)}$ & -13.5 & -23.6 & 100 &   & 2\\ 
204533053 & 16 00 12.17 & -21 57 03.3 & 14.15 & 10.34 & -11.2$\pm$2.1 & -24.4$\pm$2.1 & 6.1$\pm$1.1$^{(1)}$ & -13.6 & -23.5 & 94 & 2.847 & 1\\ 
204538466 & 16 09 59.91 & -21 55 42.5 & 18.06 & 13.31 & -11.6$\pm$3.3 & -23.2$\pm$3.3 & 4.2$\pm$0.8$^{(1)}$ & -12.9 & -23.7 & 22 & 0.874 & 18\\ 
204538777 & 16 03 26.25 & -21 55 37.9 & 15.96 & 11.6 & -12.0$\pm$2.1 & -21.3$\pm$2.1 & 5.4$\pm$1.0$^{(1)}$ & -13.4 & -23.6 & 88 &  $<$2& 3\\ 
204542962 & 16 19 50.69 & -21 54 35.5 & 11.41 & 8.2 & -5.5$\pm$1.2 & -21.5$\pm$1.1 & 9.9$\pm$1.8$^{(1)}$ & -12.3 & -23.9 & 83 & 1.271 & 0\\ 
204543498 & 16 16 59.83 & -21 54 27.3 & 14.46 & 10.64 & -14.5$\pm$2.1 & -26.4$\pm$2.1 & 5.5$\pm$1.0$^{(1)}$ & -12.5 & -23.9 & 90 & 1.939 & 1\\ 
204544020 & 16 25 48.09 & -21 54 19.5 & 15.15 & 11.15 & -18.7$\pm$2.2 & -24.8$\pm$2.2 & 5.2$\pm$1.0$^{(1)}$ & -11.9 & -24.1 & 71 & 1.849 & 1\\ 
204548337 & 16 03 27.88 & -21 53 15.5 & 13.26 & 9.86 & -11.2$\pm$2.2 & -18.7$\pm$2.2 & 5.2$\pm$1.0$^{(1)}$ & -13.4 & -23.6 & 76 & 5.573 & 3\\ 
204551703 & 16 10 01.29 & -21 52 24.4 &   & 11.71 & -14.5$\pm$3.9 & -25.4$\pm$3.9 & 2.5$\pm$0.5$^{(4)}$ & -12.9 & -23.7 &   & 1.681 & 17\\ 
204553379 & 15 58 23.37 & -21 51 58.8 &   & 11.28 & -18.9$\pm$3.9 & -22.0$\pm$3.9 & 9.6$\pm$1.8$^{(4)}$ & -13.7 & -23.5 & 92 & 1.847 & 17\\ 
204559470 & 16 33 38.83 & -21 50 26.3 & 12.86 & 8.87 & -3.2$\pm$2.4 & -22.1$\pm$2.4 & 11.2$\pm$2.1$^{(1)}$ & -11.3 & -24.2 & 72 & 3.621 & 1\\ 
204559599 & 16 20 24.98 & -21 50 24.0 & 13.53 & 9.88 & -18.3$\pm$2.3 & -26.1$\pm$2.3 & 6.3$\pm$1.2$^{(1)}$ & -12.2 & -24.0 & 91 & 5.66 & 1\\ 
204562176 & 15 55 02.13 & -21 49 43.5 & 11.68 & 8.64 & -14.5$\pm$2.3 & -18.1$\pm$2.3 & 7.2$\pm$1.3$^{(1)}$ & -13.9 & -23.4 & 93 & 4.11 & 1\\ 
204565769 & 16 08 56.29 & -21 48 49.0 & 13.2 & 9.64 & -11.5$\pm$2.2 & -21.9$\pm$2.2 & 7.0$\pm$1.3$^{(1)}$ & -13.0 & -23.7 & 95 & 9.485 & 1\\ 
204565982 & 16 27 09.42 & -21 48 45.7 & 16.66 & 11.71 & -13.2$\pm$2.6 & -26.3$\pm$2.6 & 7.1$\pm$1.3$^{(1)}$ & -11.8 & -24.1 & 96 & 1.555 & 17\\ 
204566199 & 16 07 40.06 & -21 48 42.7 & 12.82 & 9.67 & -15.7$\pm$2.2 & -19.6$\pm$2.2 & 4.8$\pm$0.9$^{(1)}$ & -13.1 & -23.7 & 62 & 6.607 & 1\\ 
204566404 & 16 35 48.37 & -21 48 39.7 & 12.12 & 8.48 & -3.7$\pm$1.7 & -18.0$\pm$7.2 & 11.2$\pm$2.1$^{(1)}$ & -11.2 & -24.2 & 75 & 1.742 & 5\\ 
204569229 & 16 19 45.38 & -21 47 57.8 & 12.39 & 9.08 & -15.1$\pm$2.3 & -23.0$\pm$2.3 & 7.5$\pm$1.4$^{(1)}$ & -12.3 & -23.9 & 95 & 1.264 & 1\\ 
204570302 & 16 28 52.80 & -21 47 40.9 & 14.87 & 10.85 & -14.2$\pm$2.2 & -23.8$\pm$2.2 & 5.4$\pm$1.0$^{(1)}$ & -11.7 & -24.1 & 87 & 3.033 & 15\\ 
204578601 & 16 19 39.76 & -21 45 35.0 & 18.7 & 12.12 & -39.3$\pm$5.0 & 24.3$\pm$5.0 &   & -12.3 & -23.9 &   & 1.715 & 7\\ 
204583750 & 16 07 26.42 & -21 44 16.9 &   & 13.68 & -19.9$\pm$5.3 & -23.1$\pm$5.3 & 6.2$\pm$1.1$^{(4)}$ & -13.1 & -23.7 & 88 & 1.537 & 17\\ 
204584635 & 16 11 05.67 & -21 44 03.4 & 13.14 & 9.24 & -10.9$\pm$2.2 & -23.1$\pm$2.2 & 9.9$\pm$1.8$^{(1)}$ & -12.9 & -23.8 & 94 & 6.713 & 1\\ 
204591415 & 16 22 44.07 & -21 42 22.2 & 13.85 & 9.85 & -12.3$\pm$2.4 & -26.1$\pm$2.4 & 8.4$\pm$1.5$^{(1)}$ & -12.1 & -24.0 & 96 & 14.869 & 1\\ 
204594600 & 15 58 48.13 & -21 41 33.9 & 17.02 & 12.52 & -15.5$\pm$2.1 & -30.7$\pm$2.1 & 4.8$\pm$0.9$^{(1)}$ & -13.7 & -23.5 & 54 &  $<$2 & 17\\ 
204595607 & 16 25 24.11 & -21 41 18.7 & 8.99 & 7.71 & -5.6$\pm$0.1 & -22.9$\pm$0.1 & 7.4$\pm$0.3$^{(0)}$ & -11.9 & -24.0 & 96 & $<$2 & 2\\ 
204598375 & 16 22 08.94 & -21 40 37.2 & 14.5 & 10.6 & -13.0$\pm$2.1 & -22.1$\pm$2.1 & 6.0$\pm$1.1$^{(1)}$ & -12.1 & -24.0 & 93 & 4.13 & 1\\ 
204598458 & 16 19 48.86 & -21 40 36.0 & 14.64 & 10.81 & -14.5$\pm$2.1 & -25.6$\pm$2.1 & 5.2$\pm$1.0$^{(1)}$ & -12.3 & -23.9 & 84 & 1.542 & 1\\ 
204599787 & 16 03 51.75 & -21 40 15.5 &   & 10.55 & -15.7$\pm$4.0 & -22.7$\pm$4.0 & 25.3$\pm$4.7$^{(4)}$ & -13.3 & -23.6 & 44 & 0.819 & 1\\ 
204602441 & 16 09 21.37 & -21 39 34.3 &   & 11.03 & -16.6$\pm$3.9 & -34.3$\pm$3.9 & 9.3$\pm$1.7$^{(4)}$ & -13.0 & -23.7 & 90 & $<$2 & 17\\ 
204602579 & 16 14 49.89 & -21 39 32.2 & 13.81 & 10.11 & -9.2$\pm$2.1 & -26.7$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -12.6 & -23.8 & 93 & 4.982 & 1\\ 
204607034 & 16 02 41.52 & -21 38 24.6 & 15.51 & 11.18 & -12.1$\pm$2.1 & -25.1$\pm$2.1 & 5.6$\pm$1.0$^{(1)}$ & -13.4 & -23.6 & 92 &  & 3\\ 
204608015 & 16 19 02.15 & -21 38 09.8 & 14.26 & 10.4 & -12.4$\pm$2.1 & -25.4$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -12.3 & -23.9 & 96 & 8.841 & 1\\ 
204608050 & 16 22 54.78 & -21 38 09.3 & 13.79 & 10.07 & -20.2$\pm$2.2 & -26.9$\pm$2.2 & 6.2$\pm$1.1$^{(1)}$ & -12.1 & -24.0 & 85 & 2.037 & 1\\ 
204608421 & 16 27 25.53 & -21 38 03.7 & 15.59 & 11.26 & -11.4$\pm$2.2 & -25.3$\pm$2.2 & 6.0$\pm$1.1$^{(1)}$ & -11.8 & -24.1 & 94 & 1.833 & 15\\ 
204611221 & 16 26 19.64 & -21 37 20.8 & 13.09 & 9.42 & -11.6$\pm$2.4 & -29.8$\pm$2.4 & 7.7$\pm$1.4$^{(1)}$ & -11.8 & -24.1 & 96 & 20.162 & 1\\ 
204614722 & 16 09 52.17 & -21 36 27.7 &   & 11.57 & -6.6$\pm$5.0 & -24.8$\pm$5.0 & 27.7$\pm$5.1$^{(4)}$ & -12.9 & -23.7 & 26 & 0.701 & 17\\ 
204615647 & 16 13 21.91 & -21 36 13.7 & 13.81 & 9.98 & -8.5$\pm$2.2 & -25.7$\pm$2.2 & 6.7$\pm$1.2$^{(1)}$ & -12.7 & -23.8 & 94 & 7.755 & 1\\ 
204624141 & 16 24 09.44 & -21 34 07.3 & 14.52 & 10.45 & -12.2$\pm$2.2 & -21.2$\pm$2.2 & 6.5$\pm$1.2$^{(1)}$ & -12.0 & -24.0 & 94 & 2.8 & 1\\ 
204630212 & 16 02 31.85 & -21 32 34.0 & 16.18 & 11.8 & 19.6$\pm$2.1 & -22.7$\pm$2.1 &   & -13.4 & -23.6 &   & 1.669 & 3\\ 
204630363 & 16 10 05.02 & -21 32 31.9 & 12.31 & 8.95 & -14.3$\pm$2.2 & -23.5$\pm$2.2 & 6.3$\pm$1.2$^{(1)}$ & -12.9 & -23.7 & 95 & 6.657 & 1\\ 
204634894 & 16 08 20.77 & -21 31 23.4 & 14.84 & 10.83 & -15.0$\pm$2.0 & -23.8$\pm$2.0 & 6.3$\pm$1.2$^{(1)}$ & -13.0 & -23.7 & 95 & 1.968 & 1\\ 
204637622 & 16 04 20.98 & -21 30 41.7 & 13.38 & 9.43 & -15.1$\pm$2.1 & -23.4$\pm$2.1 & 9.8$\pm$1.8$^{(1)}$ & -13.3 & -23.6 & 95 & 1.387 & 10\\ 
204638251 & 16 20 28.13 & -21 30 32.5 & 8.47 & 7.5 & -12.7$\pm$0.1 & -25.8$\pm$0.0 & 8.2$\pm$0.8$^{(0)}$ & -12.2 & -23.9 & 100 &  & 2\\ 
204638512 & 16 04 21.65 & -21 30 28.5 & 11.77 & 8.51 & -10.6$\pm$1.0 & -27.1$\pm$1.0 & 4.9$\pm$0.9$^{(1)}$ & -13.3 & -23.6 & 73 & 4.975 & 10\\ 
204643047 & 16 08 04.22 & -21 29 19.6 & 13.47 & 9.82 & -7.7$\pm$2.1 & -27.3$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -13.0 & -23.7 & 92 & 3.275 & 3\\ 
204644117 & 16 21 29.62 & -21 29 03.8 & 15.5 & 11.22 & -7.0$\pm$2.1 & -22.6$\pm$2.1 & 7.1$\pm$1.3$^{(1)}$ & -12.1 & -23.9 & 93 & 0.574 & 1\\ 
204649301 & 16 10 06.08 & -21 27 44.0 & 19.42 & 13.77 &   &   &   & -12.9 & -23.7 &   & 27.207 & 7\\ 
204651589 & 16 22 06.58 & -21 27 08.9 & 14.12 & 10.13 & -14.7$\pm$2.1 & -25.3$\pm$2.1 & 7.9$\pm$1.4$^{(1)}$ & -12.1 & -24.0 & 96 & 6.808 & 1\\ 
204655153 & 16 10 54.99 & -21 26 13.9 &   & 11.78 & -7.2$\pm$3.8 & -21.0$\pm$3.8 & 20.9$\pm$3.8$^{(4)}$ & -12.9 & -23.7 & 39 & 0.52 & 17\\ 
204655550 & 16 20 27.24 & -21 26 06.9 & 12.62 & 9.19 & -10.3$\pm$2.2 & -28.2$\pm$2.2 & 7.6$\pm$1.4$^{(1)}$ & -12.2 & -23.9 & 96 & 6.089 & 1\\ 
204662993 & 16 19 29.24 & -21 24 13.3 & 8.93 & 7.8 & -11.5$\pm$0.1 & -25.8$\pm$0.1 & 8.2$\pm$1.0$^{(0)}$ & -12.3 & -23.9 & 96 & $<$2 & 6\\ 
204666965 & 16 20 36.41 & -21 23 12.0 & 14.06 & 10.02 & -12.8$\pm$2.1 & -25.9$\pm$2.1 & 9.4$\pm$1.7$^{(1)}$ & -12.2 & -23.9 & 96 & 13.994 & 1\\ 
204671953 & 16 22 05.88 & -21 21 55.6 & 13.53 & 9.96 & -13.9$\pm$2.4 & -30.4$\pm$2.4 & 5.8$\pm$1.1$^{(1)}$ & -12.1 & -23.9 & 89 & 3.41 & 1\\ 
204730095 & 15 56 04.97 & -21 06 46.1 & 18.18 & 12.98 & -13.0$\pm$2.7 & -13.5$\pm$2.7 & 6.2$\pm$1.1$^{(1)}$ & -13.8 & -23.4 & 70 & 0.26 & 7\\ 
204756726 & 16 09 30.19 & -20 59 53.6 & 17.76 & 12.98 & -11.5$\pm$2.4 & -21.4$\pm$2.4 & 4.9$\pm$0.9$^{(1)}$ & -12.9 & -23.7 & 73 & 1.593 & 18\\ 
204757338 & 16 07 27.46 & -20 59 44.2 &   & 10.22 & -6.6$\pm$3.3 & -23.1$\pm$3.3 & 58.6$\pm$10.8$^{(4)}$ & -13.1 & -23.6 & 34 & 2.3 & 3\\ 
204760247 & 15 57 40.46 & -20 58 59.1 & 5.87 & 5.73 & -9.7$\pm$0.0 & -21.7$\pm$0.0 & 6.3$\pm$0.9$^{(0)}$ & -13.7 & -23.4 & 100 &   & 2\\ 
204769599 & 16 00 26.70 & -20 56 31.6 & 16.95 & 12.51 & -7.9$\pm$2.4 & -17.0$\pm$2.4 & 4.6$\pm$0.8$^{(1)}$ & -13.5 & -23.5 & 27 & 1.64 & 27\\ 
204782414 & 15 55 39.28 & -20 53 07.3 & 14.6 & 10.62 & -8.5$\pm$2.1 & -24.5$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -13.9 & -23.3 & 93 & 1.01 & 1\\ 
204783273 & 16 09 37.07 & -20 52 53.0 &   & 11.98 & -2.5$\pm$3.6 & -37.7$\pm$3.6 & 2.6$\pm$0.5$^{(4)}$ & -12.9 & -23.7 &   & 1.11 & 17\\ 
204787127 & 16 07 14.45 & -20 51 51.9 & 13.27 & 9.63 & -12.7$\pm$1.6 & -27.7$\pm$1.7 & 6.8$\pm$1.3$^{(1)}$ & -13.1 & -23.6 & 96 & 7.427 & 3\\ 
204787516 & 15 57 23.91 & -20 51 45.4 & 13.54 & 9.8 & -11.8$\pm$2.2 & -28.7$\pm$2.2 & 6.8$\pm$1.3$^{(1)}$ & -13.7 & -23.4 & 95 & 0.487 & 1\\ 
204791347 & 16 02 04.30 & -20 50 42.6 & 16.58 & 11.83 & -8.0$\pm$2.4 & -21.6$\pm$2.4 & 8.0$\pm$1.5$^{(1)}$ & -13.4 & -23.5 & 92 & 15.809 & 27\\ 
204794876 & 16 01 47.44 & -20 49 45.8 & 12.05 & 8.61 & -14.1$\pm$2.1 & -22.7$\pm$2.1 & 9.6$\pm$1.8$^{(1)}$ & -13.4 & -23.5 & 95 & 2.154 & 10\\ 
204801261 & 16 08 15.61 & -20 48 02.2 & 13.74 & 9.86 & -10.3$\pm$2.1 & -20.7$\pm$2.1 & 7.6$\pm$1.4$^{(1)}$ & -13.0 & -23.6 & 94 & 0.55 & 3\\ 
204803505 & 16 12 11.86 & -20 47 26.7 & 17.56 & 12.61 & -6.6$\pm$2.4 & -25.9$\pm$2.4 & 6.5$\pm$1.2$^{(1)}$ & -12.7 & -23.7 & 91 & 4.37 & 18\\ 
204810792 & 16 08 35.14 & -20 45 29.7 & 8.18 & 6.68 & -9.9$\pm$0.1 & -23.1$\pm$0.1 & 6.0$\pm$0.4$^{(0)}$ & -13.0 & -23.6 & 97 & & 2\\ 
204811478 & 15 55 56.01 & -20 45 18.7 &   & 12.15 & -17.9$\pm$4.8 & -24.9$\pm$4.8 & 36.4$\pm$6.7$^{(4)}$ & -13.8 & -23.3 & 30 & 1.696 & 7\\ 
204812713 & 16 13 09.79 & -20 44 59.0 & 13.91 & 9.86 & -7.3$\pm$2.1 & -16.4$\pm$2.1 & 8.5$\pm$1.6$^{(1)}$ & -12.7 & -23.7 & 77 & 0.924 & 1\\ 
204813678 & 16 07 16.07 & -20 44 43.8 & 14.53 & 10.37 & -10.2$\pm$2.0 & -23.4$\pm$2.0 & 7.5$\pm$1.4$^{(1)}$ & -13.1 & -23.6 & 96 & 2.315 & 30\\ 
204813829 & 16 13 32.79 & -20 44 41.4 & 13.92 & 10.13 & -11.2$\pm$2.0 & -25.0$\pm$2.0 & 6.3$\pm$1.2$^{(1)}$ & -12.6 & -23.7 & 95 & 1.708 & 1\\ 
204817605 & 16 12 05.05 & -20 43 40.5 & 12.79 & 9.06 & -10.4$\pm$2.1 & -23.6$\pm$2.1 & 9.2$\pm$1.7$^{(1)}$ & -12.7 & -23.7 & 95 & 9.328 & 1\\ 
204819202 & 15 55 41.41 & -20 43 15.1 & 13.34 & 9.45 & -13.3$\pm$2.3 & -20.6$\pm$2.3 & 8.8$\pm$1.6$^{(1)}$ & -13.8 & -23.3 & 95 & 1.028 & 1\\ 
204819492 & 16 07 00.10 & -20 43 10.2 & 14.97 & 10.82 & -24.0$\pm$2.0 & -27.8$\pm$2.0 & 6.0$\pm$1.1$^{(1)}$ & -13.1 & -23.6 & 68 & 2.078 & 3\\ 
204819556 & 16 21 54.67 & -20 43 09.1 & 11.73 & 9.15 & -18.7$\pm$1.0 & -30.3$\pm$1.0 & 4.5$\pm$0.8$^{(1)}$ & -12.1 & -23.9 & 15 & 7.584 & 1\\ 
204819661 & 16 07 03.73 & -20 43 07.4 & 13.14 & 9.53 & -9.1$\pm$2.1 & -26.6$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -13.1 & -23.6 & 93 & 10.248 & 10\\ 
204823656 & 16 14 05.15 & -20 42 01.7 & 18.55 & 13.38 & 0.8$\pm$2.0 & -11.6$\pm$2.0 &   & -12.6 & -23.7 &   & 1.42 & 3\\ 
204824257 & 16 16 08.55 & -20 41 51.5 & 14.67 & 10.71 & -10.1$\pm$2.0 & -26.4$\pm$2.0 & 5.8$\pm$1.1$^{(1)}$ & -12.5 & -23.8 & 92 & 3.069 & 1\\ 
204824603 & 16 09 31.10 & -20 41 46.0 & 14.42 & 10.14 & -12.8$\pm$2.0 & -23.2$\pm$2.0 & 10.5$\pm$1.9$^{(1)}$ & -12.9 & -23.6 & 94 & 3.097 & 1\\ 
204829482 & 16 08 00.52 & -20 40 28.9 &   & 11.33 & -9.8$\pm$3.6 & -22.6$\pm$3.6 & 28.2$\pm$5.2$^{(4)}$ & -13.0 & -23.6 & 36 & 1.949 & 30\\ 
204830786 & 16 07 57.96 & -20 40 08.7 & 14.17 & 7.81 & -8.5$\pm$2.1 & -35.0$\pm$2.1 & 8.9$\pm$1.6$^{(1)}$ & -13.0 & -23.6 & 81 & 6.709 & 14\\ 
204832041 & 16 07 58.51 & -20 39 48.6 & 17.32 & 12.58 & -18.0$\pm$2.4 & -23.1$\pm$2.4 & 5.6$\pm$1.0$^{(1)}$ & -13.0 & -23.6 & 87 & 0.582 & 18\\ 
204832936 & 15 56 42.45 & -20 39 34.2 & 14.26 & 10.28 & -13.2$\pm$2.1 & -25.2$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -13.8 & -23.4 & 96 & 4.259 & 1\\ 
204836433 & 15 57 24.55 & -20 38 38.2 & 13.65 & 9.99 & -9.3$\pm$2.2 & -24.5$\pm$2.2 & 5.6$\pm$1.0$^{(1)}$ & -13.7 & -23.4 & 89 & 8.64 & 1\\ 
204838119 & 16 08 15.35 & -20 38 11.2 & 14.68 & 10.68 & -11.4$\pm$2.0 & -22.4$\pm$2.0 & 5.8$\pm$1.1$^{(1)}$ & -13.0 & -23.6 & 93 & 3.981 & 30\\ 
204841911 & 16 10 39.79 & -20 37 09.5 & 13.99 & 9.95 & -10.3$\pm$2.1 & -21.8$\pm$2.1 & 7.3$\pm$1.3$^{(1)}$ & -12.8 & -23.7 & 95 & 3.59 & 1\\ 
204844509 & 16 07 03.56 & -20 36 26.5 &   & 8.1 & -13.2$\pm$1.1 & -21.9$\pm$1.1 & 14.3$\pm$2.6$^{(2)}$ & -13.1 & -23.6 & 86 & 1.714 & 10\\ 
204845955 & 16 07 44.49 & -20 36 02.9 & 13.1 & 9.08 & -9.8$\pm$2.1 & -22.1$\pm$2.1 & 12.8$\pm$2.4$^{(1)}$ & -13.0 & -23.6 & 85 & 2.534 & 30\\ 
204851310 & 16 12 35.32 & -20 34 34.0 & 12.86 & 9.3 & -12.7$\pm$2.1 & -45.1$\pm$2.1 & 7.6$\pm$1.4$^{(1)}$ & -12.7 & -23.7 & 21 & 3.895 & 1\\ 
204852312 & 16 08 54.08 & -20 34 18.1 & 14.27 & 10.0 & -13.3$\pm$2.0 & -21.0$\pm$2.0 & 10.3$\pm$1.9$^{(1)}$ & -12.9 & -23.6 & 93 & 0.458 & 30\\ 
204854345 & 16 08 56.73 & -20 33 45.9 & 11.49 & 8.62 & -8.0$\pm$2.1 & -20.1$\pm$2.1 & 6.7$\pm$1.2$^{(1)}$ & -12.9 & -23.6 & 91 & 5.312 & 5\\ 
204856535 & 16 07 00.15 & -20 33 09.3 & 13.87 & 9.94 & -11.3$\pm$2.1 & -22.0$\pm$2.1 & 6.1$\pm$1.1$^{(1)}$ & -13.1 & -23.6 & 94 & 1.648 & 30\\ 
204856827 & 16 06 59.37 & -20 33 04.8 & 13.55 & 9.54 & -14.0$\pm$2.1 & -18.0$\pm$2.1 & 9.7$\pm$1.8$^{(1)}$ & -13.1 & -23.6 & 90 & 1.648 & 14\\ 
204862109 & 16 03 54.97 & -20 31 38.6 & 12.1 & 8.62 & -7.8$\pm$2.1 & -32.0$\pm$2.1 & 9.7$\pm$1.8$^{(1)}$ & -13.3 & -23.5 & 85 & 1.728 & 10\\ 
204864076 & 16 03 57.67 & -20 31 05.6 & 11.93 & 8.37 & -12.1$\pm$1.0 & -22.0$\pm$1.0 & 8.4$\pm$1.5$^{(1)}$ & -13.3 & -23.5 & 96 & 3.882 & 10\\ 
204864711 & 16 07 45.76 & -20 30 55.9 & 16.6 & 12.75 & -88.8$\pm$2.0 & -31.7$\pm$2.0 &   & -13.0 & -23.6 &   &  & 30\\ 
204870258 & 15 59 44.28 & -20 29 23.4 & 14.72 & 10.4 & -12.1$\pm$2.0 & -25.8$\pm$2.0 & 7.9$\pm$1.5$^{(1)}$ & -13.6 & -23.4 & 97 & 24.0 & 1\\ 
204870669 & 16 10 35.25 & -20 29 16.9 & 16.25 & 11.71 & -8.9$\pm$2.4 & -25.9$\pm$2.4 & 7.0$\pm$1.3$^{(1)}$ & -12.8 & -23.6 & 95 & 1.384 & 17\\ 
204871202 & 16 09 00.72 & -20 29 08.7 & 18.53 & 12.17 & -10.5$\pm$3.9 & -22.6$\pm$3.9 & 8.8$\pm$1.6$^{(1)}$ & -12.9 & -23.6 & 94 & 1.638 & 3\\ 
204871862 & 16 07 01.70 & -20 28 58.0 &   & 12.32 & -13.9$\pm$4.6 & -18.1$\pm$4.6 & 25.5$\pm$4.7$^{(4)}$ & -13.1 & -23.6 & 32 & 37.542 & 3\\ 
204876697 & 16 08 01.41 & -20 27 41.7 & 12.76 & 9.29 & -11.6$\pm$2.1 & -22.8$\pm$2.1 & 6.9$\pm$1.3$^{(1)}$ & -13.0 & -23.6 & 96 & 9.25 & 30\\ 
204878461 & 16 07 35.56 & -20 27 13.5 &   & 11.96 & -6.0$\pm$4.6 & -26.8$\pm$4.6 & 7.5$\pm$1.4$^{(4)}$ & -13.0 & -23.6 & 91 & 1.826 & 30\\ 
204878974 & 16 00 31.35 & -20 27 05.1 & 12.42 & 8.83 & -11.0$\pm$2.1 & -21.9$\pm$2.1 & 10.2$\pm$1.9$^{(1)}$ & -13.5 & -23.4 & 93 & 3.093 & 10\\ 
204882444 & 15 55 05.13 & -20 26 07.8 & 13.63 & 9.74 & -14.5$\pm$2.4 & -24.0$\pm$2.4 & 7.7$\pm$1.4$^{(1)}$ & -13.9 & -23.3 & 97 & 0.383 & 1\\ 
204884822 & 16 35 06.26 & -20 25 28.3 & 13.57 & 9.55 & -3.6$\pm$2.4 & -30.6$\pm$2.4 & 10.1$\pm$1.9$^{(1)}$ & -11.2 & -24.1 & 81 & 0.799 & 1\\ 
204894575 & 16 02 53.96 & -20 22 48.0 &   & 8.19 & -8.5$\pm$1.3 & -21.7$\pm$1.2 & 15.4$\pm$2.8$^{(2)}$ & -13.3 & -23.5 & 72 & 1.954 & 10\\ 
204895410 & 16 08 02.38 & -20 22 33.9 & 14.93 & 10.62 & -14.5$\pm$2.0 & -32.6$\pm$2.0 & 9.2$\pm$1.7$^{(1)}$ & -13.0 & -23.6 & 93 & 2.11 & 30\\ 
204895521 & 16 06 47.51 & -20 22 32.2 & 13.65 & 9.87 & -10.2$\pm$2.1 & -17.6$\pm$2.1 & 6.8$\pm$1.3$^{(1)}$ & -13.1 & -23.6 & 89 & 4.892 & 30\\ 
204897050 & 16 01 40.98 & -20 22 08.0 &   & 10.86 & -9.9$\pm$3.7 & -22.8$\pm$3.7 & 44.4$\pm$8.2$^{(4)}$ & -13.4 & -23.4 & 31 & 0.264 & 27\\ 
204898840 & 15 58 15.73 & -20 21 36.8 & 15.14 & 11.06 & -16.4$\pm$2.0 & -26.6$\pm$2.0 & 6.1$\pm$1.1$^{(1)}$ & -13.7 & -23.4 & 94 & 0.447 & 1\\ 
204901273 & 16 07 19.72 & -20 20 55.6 & 14.8 & 10.72 & -8.4$\pm$2.0 & -20.9$\pm$2.0 & 6.2$\pm$1.1$^{(1)}$ & -13.0 & -23.6 & 91 & 4.92 & 30\\ 
204906020 & 16 07 02.12 & -20 19 38.8 & 16.33 & 11.4 & 12.1$\pm$2.0 & -16.0$\pm$2.0 &   & -13.1 & -23.6 &   & 1.54 & 30\\ 
204907231 & 16 11 13.96 & -20 19 18.9 & 14.58 & 10.41 & -10.4$\pm$2.0 & -21.2$\pm$2.0 & 7.7$\pm$1.4$^{(1)}$ & -12.8 & -23.6 & 95 & 7.82 & 1\\ 
204908189 & 16 11 13.31 & -20 19 03.0 & 13.85 & 9.56 & -11.1$\pm$2.1 & -21.3$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -12.8 & -23.6 & 94 &   & 3\\ 
204909952 & 16 07 27.54 & -20 18 34.4 &   & 11.44 & -8.0$\pm$3.0 & -15.0$\pm$3.0 & 13.7$\pm$2.5$^{(3)}$ & -13.0 & -23.6 & 45 & $<$2 & 30\\ 
204914881 & 16 14 52.59 & -20 17 13.3 & 19.8 & 14.06 &   &   &   & -12.5 & -23.7 &   &  & 7\\ 
204918279 & 15 56 25.11 & -20 16 15.8 &   & 9.86 & -13.4$\pm$4.0 & -22.5$\pm$4.4 & 18.6$\pm$3.4$^{(4)}$ & -13.8 & -23.3 & 64 & 0.459 & 1\\ 
204919503 & 16 07 04.74 & -20 15 55.7 & 15.65 & 11.46 & -10.8$\pm$2.0 & -25.8$\pm$2.0 & 5.1$\pm$0.9$^{(1)}$ & -13.1 & -23.5 & 82 & 3.117 & 30\\ 
204920926 & 16 03 43.35 & -20 15 31.5 & 13.34 & 9.72 & -11.6$\pm$2.1 & -21.5$\pm$2.1 & 6.4$\pm$1.2$^{(1)}$ & -13.3 & -23.5 & 95 & 5.609 & 30\\ 
204926239 & 16 14 40.16 & -20 14 03.0 & 8.83 & 7.07 & -17.4$\pm$0.2 & -27.7$\pm$0.1 & 6.6$\pm$0.2$^{(0)}$ & -12.5 & -23.7 & 90 & & 2\\ 
204931558 & 15 57 51.95 & -20 12 33.9 & 16.42 & 12.08 & -25.9$\pm$2.4 & -28.2$\pm$2.4 & 5.7$\pm$1.1$^{(1)}$ & -13.7 & -23.3 & 51 & 0.509 & 27\\ 
204932100 & 16 08 25.11 & -20 12 24.6 & 13.47 & 9.87 & -9.9$\pm$2.1 & -20.3$\pm$2.1 & 5.9$\pm$1.1$^{(1)}$ & -13.0 & -23.6 & 91 & 18.352 & 30\\ 
204932990 & 16 11 50.93 & -20 12 09.9 & 14.47 & 10.4 & -11.0$\pm$2.0 & -21.3$\pm$2.0 & 6.7$\pm$1.2$^{(1)}$ & -12.7 & -23.6 & 95 & 2.315 & 3\\ 
204933717 & 16 07 22.40 & -20 11 58.2 &   & 11.59 & -6.0$\pm$3.0 & -27.0$\pm$3.0 & 10.5$\pm$1.9$^{(3)}$ & -13.0 & -23.5 & 85 & 1.553 & 30\\ 
204939243 & 16 15 32.20 & -20 10 23.7 & 13.22 & 8.91 & -13.4$\pm$2.1 & -30.3$\pm$2.1 & 12.8$\pm$2.4$^{(1)}$ & -12.5 & -23.7 & 88 & 2.915 & 1\\ 
204940701 & 16 12 27.38 & -20 09 59.7 & 16.63 & 11.54 & -5.6$\pm$2.2 & -4.3$\pm$2.2 & 13.2$\pm$2.4$^{(1)}$ & -12.7 & -23.6 &   & $<$2 & 3\\ 
204942552 & 16 09 08.42 & -20 09 27.6 & 13.81 &   & -22.5$\pm$2.1 & -5.0$\pm$2.1 &   & -12.9 & -23.6 &   &   & 30\\ 
204947015 & 16 01 58.22 & -20 08 12.0 & 10.01 & 7.67 & -9.0$\pm$1.0 & -23.0$\pm$0.6 & 6.5$\pm$0.3$^{(0)}$ & -13.4 & -23.4 & 97 & 1.774 & 10\\ 
204948308 & 16 02 10.96 & -20 07 49.6 & 15.62 & 11.42 & -9.1$\pm$2.0 & -23.2$\pm$2.0 & 5.5$\pm$1.0$^{(1)}$ & -13.4 & -23.4 & 88 & 0.94 & 30\\ 
204949180 & 16 09 18.37 & -20 07 34.9 & 17.69 & 12.02 & 45.4$\pm$4.6 & -18.7$\pm$4.6 &   & -12.9 & -23.6 &   & 18.95 & 17\\ 
204949182 & 16 09 18.15 & -20 07 34.9 & 17.69 &   & 45.4$\pm$4.6 & -18.7$\pm$4.6 &   & -12.9 & -23.6 &   &   & 17\\ 
204951731 & 16 20 30.56 & -20 06 52.0 & 8.25 & 7.09 & -12.3$\pm$0.2 & -25.2$\pm$0.1 & 8.1$\pm$0.3$^{(0)}$ & -12.2 & -23.8 & 98 &   & 2\\ 
204954915 & 16 03 41.88 & -20 05 57.7 & 13.12 & 9.49 & -13.3$\pm$2.1 & -24.7$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -13.3 & -23.5 & 97 & 4.627 & 30\\ 
204956337 & 16 20 21.64 & -20 05 34.8 &   & 10.96 & -17.6$\pm$4.7 & -18.4$\pm$4.7 & 42.7$\pm$7.9$^{(4)}$ & -12.2 & -23.8 & 15 & 7.804 & 1\\ 
204959839 & 16 15 50.52 & -20 04 35.3 & 8.02 & 7.27 & -19.1$\pm$0.1 & -29.4$\pm$0.0 & 9.7$\pm$1.0$^{(0)}$ & -12.5 & -23.7 & 87 & $<$2 & 2\\ 
204960156 & 16 14 33.64 & -20 04 29.9 & 14.11 & 10.04 & -9.1$\pm$2.0 & -26.7$\pm$2.0 & 7.8$\pm$1.4$^{(1)}$ & -12.5 & -23.7 & 95 & 2.101 & 1\\ 
204963464 & 15 56 34.26 & -20 03 33.3 & 15.1 & 10.87 & -12.1$\pm$2.1 & -21.9$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -13.8 & -23.3 & 96 & 0.369 & 1\\ 
204964091 & 16 20 05.49 & -20 03 23.0 & 7.3 & 6.68 & -11.6$\pm$0.1 & -24.7$\pm$0.0 & 7.8$\pm$0.3$^{(0)}$ & -12.2 & -23.8 & 99 &   & 2\\ 
204966512 & 16 20 03.98 & -20 02 41.5 & 7.98 & 7.09 & -11.3$\pm$0.2 & -26.3$\pm$0.2 & 5.8$\pm$1.1$^{(0)}$ & -12.2 & -23.8 & 94 &   & 2\\ 
204966558 & 16 02 26.14 & -20 02 40.7 & 15.11 & 10.99 & -14.7$\pm$2.0 & -6.5$\pm$2.0 & 6.5$\pm$1.2$^{(1)}$ & -13.4 & -23.4 & 4 & 2.169 & 30\\ 
204970885 & 16 06 39.90 & -20 01 28.2 & 13.92 & 10.08 & -10.1$\pm$2.0 & -21.3$\pm$2.0 & 6.6$\pm$1.2$^{(1)}$ & -13.1 & -23.5 & 94 & 6.913 & 26\\ 
204986988 & 16 02 22.48 & -19 56 54.0 & 14.65 & 10.66 & -11.1$\pm$2.0 & -25.6$\pm$2.0 & 6.0$\pm$1.1$^{(1)}$ & -13.4 & -23.4 & 94 & 1.675 & 30\\ 
204987267 & 16 02 22.35 & -19 56 49.2 & 18.36 & 14.44 & -4.5$\pm$3.7 & 12.3$\pm$3.9 &   & -13.4 & -23.4 &   & $<$2 & 30\\ 
204990278 & 16 24 11.78 & -19 55 58.3 & 13.95 & 9.95 & -20.2$\pm$2.4 & -26.2$\pm$2.4 & 7.4$\pm$1.4$^{(1)}$ & -11.9 & -23.9 & 91 & 3.82 & 1\\ 
204993463 & 16 03 29.41 & -19 55 03.6 & 15.09 & 11.03 & -11.2$\pm$2.0 & -19.1$\pm$2.0 & 5.6$\pm$1.0$^{(1)}$ & -13.3 & -23.4 & 87 & 1.106 & 30\\ 
205000676 & 16 22 09.61 & -19 53 00.7 & 13.39 & 8.9 & -8.1$\pm$2.4 & -29.6$\pm$2.4 & 16.4$\pm$3.0$^{(1)}$ & -12.0 & -23.8 & 66 & 3.187 & 3\\ 
205002311 & 16 47 47.34 & -19 52 31.9 & 8.89 & 7.8 & -16.1$\pm$0.1 & -27.7$\pm$0.1 & 8.9$\pm$0.3$^{(0)}$ & -10.4 & -24.3 & 98 & 1.147 & 6\\ 
205002988 & 16 01 59.77 & -19 52 20.3 & 17.81 & 11.51 & -21.3$\pm$4.7 & -47.7$\pm$4.7 & 12.3$\pm$2.3$^{(1)}$ & -13.4 & -23.4 & 19 & 0.562 & 30\\ 
205005589 & 16 10 14.46 & -19 51 37.6 & 14.18 & 10.23 & -10.8$\pm$2.0 & -22.9$\pm$2.0 & 7.1$\pm$1.3$^{(1)}$ & -12.8 & -23.6 & 96 & 5.116 & 1\\ 
205007364 & 16 22 43.60 & -19 51 06.5 & 15.84 & 12.74 & -8.6$\pm$2.2 & -8.4$\pm$2.2 &   & -12.0 & -23.8 &   & $<$2 & 18\\ 
205007401 & 16 22 43.85 & -19 51 05.8 & 16.9 & 11.16 & -8.6$\pm$2.2 & -8.4$\pm$2.2 & 18.7$\pm$3.4$^{(1)}$ & -12.0 & -23.8 & 1 & 1.381 & 18\\ 
205008763 & 15 57 02.34 & -19 50 42.2 & 10.97 & 8.37 & -14.3$\pm$1.0 & -24.9$\pm$1.0 & 6.9$\pm$1.3$^{(1)}$ & -13.7 & -23.3 & 97 & 2.538 & 5\\ 
205010817 & 15 56 47.69 & -19 50 07.6 & 12.44 & 8.95 & -10.0$\pm$2.3 & -21.0$\pm$2.3 & 8.8$\pm$1.6$^{(1)}$ & -13.7 & -23.3 & 93 & 2.637 & 1\\ 
205012599 & 16 12 41.24 & -19 49 38.0 & 12.52 & 8.9 & -13.7$\pm$2.1 & -26.3$\pm$2.1 & 9.4$\pm$1.7$^{(1)}$ & -12.7 & -23.6 & 96 & 3.626 & 3\\ 
205014939 & 16 04 07.76 & -19 48 57.8 & 16.24 & 12.41 & -44.2$\pm$2.0 & -19.8$\pm$2.0 &   & -13.2 & -23.4 &   & 0.545 & 30\\ 
205019241 & 16 11 49.20 & -19 47 43.2 & 15.15 & 10.82 & -11.3$\pm$2.0 & -24.7$\pm$2.0 & 8.0$\pm$1.5$^{(1)}$ & -12.7 & -23.6 & 96 & 0.92 & 3\\ 
205020984 & 16 08 04.32 & -19 47 12.6 & 13.78 & 10.57 & -4.5$\pm$2.0 & -4.7$\pm$2.0 & 2.9$\pm$0.5$^{(1)}$ & -13.0 & -23.5 &   & 3.912 & 30\\ 
205024407 & 15 58 36.20 & -19 46 13.5 & 14.64 & 10.72 & -13.7$\pm$2.0 & -23.9$\pm$2.0 & 5.6$\pm$1.0$^{(1)}$ & -13.6 & -23.3 & 92 & 3.002 & 1\\ 
205024957 & 16 10 11.01 & -19 46 04.1 & 15.58 & 11.38 & -17.0$\pm$2.0 & -23.8$\pm$2.0 & 5.6$\pm$1.0$^{(1)}$ & -12.8 & -23.6 & 89 & $<$2 & 30\\ 
205024963 & 16 02 45.49 & -19 46 03.9 & 15.81 & 12.04 & 7.4$\pm$2.0 & 3.7$\pm$2.0 &   & -13.3 & -23.4 &   & 17.14 & 30\\ 
205025028 & 16 04 00.24 & -19 46 02.9 & 7.77 & 7.24 & -10.1$\pm$0.1 & -21.6$\pm$0.0 & 6.1$\pm$0.3$^{(0)}$ & -13.2 & -23.4 & 98 &   & 2\\ 
205026365 & 16 10 10.41 & -19 45 39.8 & 14.34 & 10.41 & -16.5$\pm$2.0 & -21.7$\pm$2.0 & 6.6$\pm$1.2$^{(1)}$ & -12.8 & -23.6 & 94 & 2.028 & 30\\ 
205030030 & 16 03 25.62 & -19 44 38.5 & 14.95 & 11.48 & -66.1$\pm$3.8 & 24.3$\pm$3.8 &   & -13.3 & -23.4 &   & 52.469 & 30\\ 
205030103 & 15 59 50.51 & -19 44 37.3 & 14.31 & 10.17 & -12.0$\pm$2.0 & -23.1$\pm$2.0 & 8.7$\pm$1.6$^{(1)}$ & -13.5 & -23.3 & 96 & 31.539 & 27\\ 
205034152 & 16 09 13.39 & -19 43 28.1 & 14.5 & 10.6 & -8.5$\pm$2.0 & -22.0$\pm$2.0 & 5.8$\pm$1.1$^{(1)}$ & -12.9 & -23.5 & 90 & 3.621 & 30\\ 
205034491 & 16 11 56.26 & -19 43 22.9 & 13.79 & 9.81 & -13.6$\pm$2.1 & -25.3$\pm$2.1 & 8.6$\pm$1.6$^{(1)}$ & -12.7 & -23.6 & 96 & 5.914 & 30\\ 
205037578 & 16 04 17.40 & -19 42 28.8 & 14.53 & 10.42 & 0.9$\pm$2.4 & 11.7$\pm$2.6 &   & -13.2 & -23.4 &   & 1.728 & 3\\ 
205038557 & 16 03 57.93 & -19 42 10.9 & 14.1 & 10.32 & -11.4$\pm$2.0 & -23.1$\pm$2.0 & 5.4$\pm$1.0$^{(1)}$ & -13.2 & -23.4 & 89 & 3.831 & 30\\ 
205040772 & 16 10 21.53 & -19 41 31.9 & 14.03 & 9.86 & -4.0$\pm$2.1 & -3.4$\pm$2.1 & 10.9$\pm$2.0$^{(1)}$ & -12.8 & -23.6 &   & 1.12 & 30\\ 
205041327 & 16 03 50.46 & -19 41 21.6 & 14.63 & 10.59 & -9.7$\pm$2.0 & -20.2$\pm$2.0 & 6.6$\pm$1.2$^{(1)}$ & -13.2 & -23.4 & 93 & 2.962 & 30\\ 
205046529 & 16 10 26.39 & -19 39 51.1 & 15.33 & 10.4 & -6.7$\pm$2.0 & -9.8$\pm$2.0 & 21.6$\pm$4.0$^{(1)}$ & -12.8 & -23.6 & 1 & 2.562 & 30\\ 
205046848 & 16 09 03.97 & -19 39 45.6 & 14.37 & 10.37 & -9.0$\pm$2.0 & -33.1$\pm$2.0 & 7.2$\pm$1.3$^{(1)}$ & -12.9 & -23.5 & 87 & 4.472 & 30\\ 
205047099 & 16 09 03.96 & -19 39 41.5 & 18.34 &   & -9.0$\pm$2.0 & -33.1$\pm$2.0 &   & -12.9 & -23.5 &   &   & 30\\ 
205051240 & 16 14 07.93 & -19 38 29.1 & 11.08 & 7.72 & -8.1$\pm$1.0 & -18.1$\pm$1.0 & 7.9$\pm$1.5$^{(1)}$ & -12.6 & -23.6 & 88 & 5.319 & 8\\ 
205054287 & 16 09 46.45 & -19 37 36.1 & 13.28 & 9.63 & -10.3$\pm$2.1 & -23.5$\pm$2.1 & 6.8$\pm$1.3$^{(1)}$ & -12.8 & -23.5 & 96 & 4.156 & 30\\ 
205054397 & 16 10 52.41 & -19 37 34.4 & 14.89 & 10.73 & -10.1$\pm$2.0 & -24.4$\pm$2.0 & 7.1$\pm$1.3$^{(1)}$ & -12.8 & -23.6 & 96 & 1.81 & 30\\ 
205055104 & 16 01 22.33 & -19 37 22.3 & 13.21 & 9.56 & -15.0$\pm$2.1 & -24.4$\pm$2.1 & 6.9$\pm$1.3$^{(1)}$ & -13.4 & -23.4 & 96 & 8.103 & 1\\ 
205056060 & 16 09 15.81 & -19 37 06.3 & 15.52 & 11.46 & -6.9$\pm$2.0 & -22.7$\pm$2.0 & 5.0$\pm$0.9$^{(1)}$ & -12.9 & -23.5 & 69 & 1.722 & 30\\ 
205060410 & 16 08 23.87 & -19 35 51.9 & 12.85 & 9.25 & -2.3$\pm$2.1 & -26.1$\pm$2.1 & 8.5$\pm$1.6$^{(1)}$ & -12.9 & -23.5 & 71 & 17.997 & 30\\ 
205064383 & 16 12 21.83 & -19 34 44.6 & 7.6 & 7.07 & -9.1$\pm$0.1 & -24.1$\pm$0.1 & 6.5$\pm$0.4$^{(0)}$ & -12.7 & -23.6 & 97 &   & 2\\ 
205066998 & 16 09 04.05 & -19 34 00.1 & 15.66 & 10.88 & -19.8$\pm$2.0 & -7.2$\pm$2.0 & 13.0$\pm$2.4$^{(1)}$ & -12.9 & -23.5 & 1 & 3.095 & 30\\ 
205068630 & 16 11 10.96 & -19 33 32.1 & 15.57 & 11.24 & 0.5$\pm$2.0 & -28.5$\pm$2.0 &   & -12.8 & -23.6 &   &   & 30\\ 
205072354 & 16 12 10.44 & -19 32 27.6 & 15.73 & 11.24 & -7.2$\pm$2.4 & -22.5$\pm$2.4 & 8.0$\pm$1.5$^{(1)}$ & -12.7 & -23.6 & 93 & 0.772 & 17\\ 
205078547 & 16 02 45.45 & -19 30 37.8 &   & 11.14 & -10.8$\pm$3.7 & -22.8$\pm$3.7 & 22.5$\pm$4.1$^{(4)}$ & -13.3 & -23.4 & 49 & 0.786 & 30\\ 
205080089 & 16 12 44.10 & -19 30 10.3 & 7.56 & 6.94 & -6.6$\pm$0.1 & -24.7$\pm$0.0 & 6.9$\pm$0.3$^{(0)}$ & -12.6 & -23.6 & 100 &   & 2\\ 
205080360 & 16 08 22.34 & -19 30 05.3 & 12.62 & 9.06 & -17.2$\pm$2.1 & -27.0$\pm$2.1 & 8.7$\pm$1.6$^{(1)}$ & -12.9 & -23.5 & 96 & 2.382 & 30\\ 
205080616 & 16 08 23.24 & -19 30 01.0 & 12.94 & 9.47 & -11.1$\pm$2.1 & -23.1$\pm$2.1 & 5.6$\pm$1.0$^{(1)}$ & -12.9 & -23.5 & 91 & 2.383 & 30\\ 
205082248 & 16 13 03.07 & -19 29 31.9 &   & 12.36 & -23.6$\pm$4.6 & -40.1$\pm$4.6 & 23.1$\pm$4.2$^{(4)}$ & -12.6 & -23.6 & 8 & $<$2 & 17\\ 
205086621 & 16 11 45.34 & -19 28 13.2 & 16.51 & 11.81 & -12.2$\pm$2.6 & -21.5$\pm$2.6 & 7.0$\pm$1.3$^{(1)}$ & -12.7 & -23.6 & 95 & 1.742 & 3\\ 
205087347 & 16 00 49.89 & -19 28 00.4 & 13.49 & 9.69 & -9.5$\pm$2.1 & -21.5$\pm$2.1 & 8.0$\pm$1.5$^{(1)}$ & -13.4 & -23.3 & 94 & 9.747 & 1\\ 
205087483 & 16 08 01.56 & -19 27 57.9 & 14.22 & 9.69 & -14.8$\pm$2.1 & -15.5$\pm$2.1 & 16.6$\pm$3.1$^{(1)}$ & -13.0 & -23.5 & 44 & $<$2 & 30\\ 
205088645 & 16 11 12.38 & -19 27 37.4 & 16.38 & 11.67 & -10.4$\pm$2.4 & -26.8$\pm$2.4 & 7.1$\pm$1.3$^{(1)}$ & -12.7 & -23.6 & 96 & & 30\\ 
205088828 & 16 07 08.73 & -19 27 34.2 & 15.2 & 11.17 & -13.2$\pm$2.0 & -24.2$\pm$2.0 & 4.9$\pm$0.9$^{(1)}$ & -13.0 & -23.5 & 77 & 1.661 & 30\\ 
205089268 & 16 09 20.89 & -19 27 25.9 & 8.03 & 7.48 & -8.1$\pm$0.1 & -23.2$\pm$0.0 & 6.8$\pm$0.4$^{(0)}$ & -12.9 & -23.5 & 96 &   & 2\\ 
205089832 & 16 07 07.68 & -19 27 16.2 & 13.52 & 9.8 & -16.7$\pm$2.1 & -30.3$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -13.0 & -23.5 & 95 & 8.188 & 30\\ 
205091385 & 16 13 43.89 & -19 26 48.5 & 13.19 & 8.9 & -10.2$\pm$2.1 & -31.7$\pm$2.1 & 16.1$\pm$3.0$^{(1)}$ & -12.6 & -23.6 & 65 & 1.31 & 13\\ 
205092303 & 16 09 20.55 & -19 26 31.9 & 16.63 & 12.08 & -11.9$\pm$2.4 & -24.8$\pm$2.4 & 4.1$\pm$0.8$^{(1)}$ & -12.9 & -23.5 & 21 & 1.72 & 3\\ 
205097367 & 16 09 26.70 & -19 25 02.5 & 14.61 & 11.08 &   & 6.1$\pm$2.0 &   & -12.9 & -23.5 &   & 47.566 & 30\\ 
205097920 & 16 13 28.09 & -19 24 52.4 & 16.66 & 11.91 & -13.3$\pm$2.4 & -27.8$\pm$2.4 & 7.7$\pm$1.4$^{(1)}$ & -12.6 & -23.6 & 96 & 1.514 & 30\\ 
205099884 & 16 12 41.19 & -19 24 18.3 & 12.59 & 8.77 & -8.3$\pm$2.3 & -20.1$\pm$2.2 & 11.2$\pm$2.1$^{(1)}$ & -12.6 & -23.6 & 85 & 4.145 & 13\\ 
205106221 & 16 10 43.92 & -19 22 25.8 & 13.75 & 9.93 & -9.2$\pm$2.2 & -24.9$\pm$2.2 & 6.4$\pm$1.2$^{(1)}$ & -12.8 & -23.5 & 94 & 5.439 & 30\\ 
205110000 & 16 15 44.17 & -19 21 17.3 & 12.75 & 8.4 & -12.9$\pm$2.1 & -25.3$\pm$2.1 & 10.9$\pm$2.0$^{(1)}$ & -12.4 & -23.6 & 94 &  & 3\\ 
205115701 & 16 10 05.42 & -19 19 36.3 & 18.32 & 12.7 & -8.9$\pm$2.6 & -27.8$\pm$2.6 & 6.2$\pm$1.1$^{(1)}$ & -12.8 & -23.5 & 92 & 2.552 & 7\\ 
205117205 & 16 10 14.74 & -19 19 09.4 & 13.93 & 10.03 & -12.6$\pm$2.0 & -24.7$\pm$2.0 & 6.7$\pm$1.2$^{(1)}$ & -12.8 & -23.5 & 96 & 6.292 & 30\\ 
205121714 & 16 07 39.40 & -19 17 47.2 & 13.52 & 9.8 & -12.7$\pm$2.1 & -23.7$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -13.0 & -23.5 & 95 & 9.103 & 30\\ 
205122602 & 16 02 36.24 & -19 17 32.3 & 16.49 & 12.43 & -32.0$\pm$2.0 & -27.8$\pm$2.0 & 2.6$\pm$0.5$^{(1)}$ & -13.3 & -23.4 &   & 25.589 & 30\\ 
205124381 & 16 15 39.14 & -19 17 00.6 &   & 10.43 & -28.9$\pm$3.8 & -9.6$\pm$3.6 & 60.8$\pm$11.2$^{(4)}$ & -12.4 & -23.6 &   & 1.396 & 17\\ 
205124839 & 16 10 39.57 & -19 16 52.4 & 14.33 & 10.27 & -14.8$\pm$2.0 & -20.6$\pm$2.0 & 7.2$\pm$1.3$^{(1)}$ & -12.8 & -23.5 & 95 & 4.708 & 30\\ 
205128625 & 15 58 18.84 & -19 15 44.9 & 13.91 & 10.13 & -9.7$\pm$2.0 & -19.4$\pm$2.0 & 6.0$\pm$1.1$^{(1)}$ & -13.6 & -23.3 & 90 & 13.752 & 1\\ 
205130041 & 16 12 05.33 & -19 15 19.8 & 12.57 & 8.86 & -12.4$\pm$2.1 & 1.7$\pm$2.1 &   & -12.7 & -23.6 &   & 17.686 & 13\\ 
205133963 & 16 10 24.74 & -19 14 07.4 & 14.43 & 10.33 & -9.4$\pm$2.0 & -20.0$\pm$2.0 & 7.0$\pm$1.3$^{(1)}$ & -12.8 & -23.5 & 93 & 1.577 & 30\\ 
205137295 & 16 10 32.33 & -19 13 08.6 & 18.44 & 12.73 &   &   &   & -12.8 & -23.5 &   & 12.259 & 14\\ 
205137430 & 16 10 31.95 & -19 13 06.1 & 12.5 & 8.99 & -13.8$\pm$2.1 & -24.2$\pm$2.1 & 7.9$\pm$1.5$^{(1)}$ & -12.8 & -23.5 & 97 & 12.259 & 30\\ 
205142483 & 16 07 03.94 & -19 11 34.0 & 12.96 & 9.22 & -11.4$\pm$2.1 & -27.8$\pm$2.1 & 8.9$\pm$1.6$^{(1)}$ & -13.0 & -23.5 & 95 & 6.648 & 10\\ 
205142641 & 16 08 23.57 & -19 11 31.6 & 13.84 & 9.93 & -12.7$\pm$2.1 & -25.8$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -12.9 & -23.5 & 97 & 6.345 & 30\\ 
205143329 & 16 15 47.33 & -19 11 18.5 & 13.82 & 9.68 & -12.7$\pm$2.1 & -25.1$\pm$2.1 & 8.6$\pm$1.6$^{(1)}$ & -12.4 & -23.6 & 96 & 5.432 & 1\\ 
205145188 & 16 10 28.20 & -19 10 44.5 & 16.39 & 11.79 & -11.6$\pm$2.4 & -25.4$\pm$2.4 & 5.9$\pm$1.1$^{(1)}$ & -12.8 & -23.5 & 94 & 0.875 & 30\\ 
205150770 & 16 12 20.93 & -19 09 04.1 & 13.54 & 9.6 & -8.3$\pm$2.1 & -21.2$\pm$2.1 & 8.1$\pm$1.5$^{(1)}$ & -12.7 & -23.6 & 93 & 0.755 & 26\\ 
205151387 & 16 09 00.76 & -19 08 52.7 & 12.73 & 9.15 & -5.9$\pm$2.1 & -23.7$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -12.9 & -23.5 & 91 & 9.953 & 30\\ 
205152244 & 16 09 00.04 & -19 08 37.6 & 15.21 & 10.96 & -10.6$\pm$2.0 & -27.1$\pm$2.0 & 6.7$\pm$1.2$^{(1)}$ & -12.9 & -23.5 & 95 & 1.814 & 30\\ 
205152548 & 16 08 14.75 & -19 08 32.5 & 10.88 & 8.43 & -8.5$\pm$0.9 & -27.6$\pm$0.6 & 7.0$\pm$0.3$^{(0)}$ & -12.9 & -23.5 & 97 & 10.436 & 5\\ 
205154017 & 16 06 43.86 & -19 08 05.6 & 12.44 & 9.19 & -8.6$\pm$2.1 & -22.1$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -13.0 & -23.4 & 93 & 7.024 & 1\\ 
205155253 & 16 11 46.13 & -19 07 43.0 & 15.76 & 11.15 & -8.2$\pm$2.0 & -23.1$\pm$2.0 & 7.9$\pm$1.4$^{(1)}$ & -12.7 & -23.5 & 95 & 1.786 & 30\\ 
205157766 & 16 11 59.23 & -19 06 56.3 & 14.45 & 8.34 & -8.4$\pm$2.1 & -19.6$\pm$2.1 & 57.6$\pm$10.6$^{(1)}$ & -12.7 & -23.5 & 41 &   & 26\\ 
205157836 & 16 09 54.42 & -19 06 55.0 & 13.24 & 9.6 & -14.8$\pm$2.1 & -22.7$\pm$2.1 & 6.6$\pm$1.2$^{(1)}$ & -12.8 & -23.5 & 95 & 16.634 & 30\\ 
205157937 & 16 11 59.27 & -19 06 53.4 & 11.05 & 8.09 & -8.4$\pm$2.1 & -19.6$\pm$2.1 & 9.1$\pm$1.7$^{(1)}$ & -12.7 & -23.5 & 90 & 3.692 & 26\\ 
205158239 & 16 14 20.30 & -19 06 48.2 & 14.04 & 7.81 & -8.4$\pm$2.1 & -25.7$\pm$2.1 & 27.4$\pm$5.1$^{(1)}$ & -12.5 & -23.6 & 37 & 4.771 & 30\\ 
205164400 & 16 09 33.79 & -19 04 56.2 & 13.58 & 9.85 & -13.5$\pm$2.1 & -25.0$\pm$2.1 & 6.3$\pm$1.2$^{(1)}$ & -12.8 & -23.5 & 95 & 13.496 & 30\\ 
205164832 & 16 08 10.83 & -19 04 47.9 & 11.15 & 8.47 & -8.7$\pm$1.1 & -23.9$\pm$1.0 & 7.5$\pm$0.3$^{(0)}$ & -12.9 & -23.5 & 97 & 3.054 & 0\\ 
205164892 & 16 10 28.57 & -19 04 46.9 & 12.55 & 8.71 & -10.6$\pm$2.2 & -26.7$\pm$2.1 & 11.3$\pm$2.1$^{(1)}$ & -12.8 & -23.5 & 92 & 6.681 & 26\\ 
205164999 & 16 13 02.35 & -19 04 45.1 &   & 12.72 & -30.9$\pm$4.9 & -17.2$\pm$4.9 & 21.7$\pm$4.0$^{(4)}$ & -12.6 & -23.6 & 3 & 1.958 & 3\\ 
205165965 & 16 13 09.97 & -19 04 26.9 & 15.0 & 10.58 & -8.2$\pm$2.0 & -27.1$\pm$2.0 & 7.6$\pm$1.4$^{(1)}$ & -12.6 & -23.6 & 94 & 6.86 & 13\\ 
205166677 & 16 13 10.24 & -19 04 13.1 & 13.83 & 9.65 & -6.0$\pm$2.1 & -24.6$\pm$2.1 & 11.9$\pm$2.2$^{(1)}$ & -12.6 & -23.6 & 81 & 6.865 & 13\\ 
205167008 & 16 10 21.74 & -19 04 06.6 & 13.41 & 9.62 & -16.1$\pm$2.1 & -32.9$\pm$2.1 & 7.4$\pm$1.4$^{(1)}$ & -12.8 & -23.5 & 92 & 4.139 & 26\\ 
205167265 & 16 10 21.78 & -19 04 02.2 & 16.83 & 11.92 & -16.1$\pm$2.1 & -32.9$\pm$2.1 & 8.7$\pm$1.6$^{(1)}$ & -12.8 & -23.5 & 93 & 4.139 & 14\\ 
205167772 & 16 12 47.27 & -19 03 53.2 &   & 11.75 & -4.3$\pm$3.6 & -27.1$\pm$3.6 & 30.3$\pm$5.6$^{(4)}$ & -12.6 & -23.6 & 15 & 1.188 & 30\\ 
205177336 & 16 08 18.36 & -19 00 59.4 & 14.31 & 10.22 & -4.8$\pm$2.3 & -22.5$\pm$2.3 & 8.0$\pm$1.5$^{(1)}$ & -12.9 & -23.5 & 86 & 3.245 & 30\\ 
205177770 & 16 08 43.10 & -19 00 51.9 & 14.39 & 10.27 & -12.6$\pm$2.0 & -22.7$\pm$2.0 & 8.5$\pm$1.6$^{(1)}$ & -12.9 & -23.5 & 96 & 0.935 & 30\\ 
205179845 & 16 14 33.67 & -19 00 13.5 & 13.41 & 8.26 & -9.0$\pm$2.1 & -23.0$\pm$2.1 & 17.7$\pm$3.3$^{(1)}$ & -12.5 & -23.6 & 66 & 2.6 & 30\\ 
205181377 & 16 09 02.60 & -18 59 44.0 & 7.72 & 7.01 & -7.3$\pm$0.0 & -24.0$\pm$0.0 & 7.7$\pm$0.3$^{(0)}$ & -12.9 & -23.5 & 84 &   & 2\\ 
205182200 & 16 12 39.17 & -18 59 28.5 & 12.84 & 9.11 & -12.0$\pm$2.1 & -20.0$\pm$2.1 & 7.6$\pm$1.4$^{(1)}$ & -12.6 & -23.5 & 95 & 1.519 & 13\\ 
205182220 & 16 12 40.51 & -18 59 28.2 & 10.29 & 7.49 & -9.9$\pm$0.8 & -21.7$\pm$0.5 & 7.6$\pm$0.2$^{(0)}$ & -12.6 & -23.5 & 96 & 1.519 & 26\\ 
205185617 & 16 14 37.51 & -18 58 24.3 & 15.43 & 11.87 & -23.3$\pm$2.0 & -44.8$\pm$2.0 &   & -12.5 & -23.6 &   & 2.026 & 30\\ 
205188906 & 16 14 28.93 & -18 57 22.5 & 13.27 & 9.47 & -8.3$\pm$2.1 & -25.1$\pm$2.1 & 8.8$\pm$1.6$^{(1)}$ & -12.5 & -23.6 & 94 & 16.588 & 13\\ 
205192701 & 16 08 41.71 & -18 56 10.8 &   & 11.21 & -5.0$\pm$3.0 & -21.0$\pm$3.0 & 15.2$\pm$2.8$^{(3)}$ & -12.9 & -23.5 & 52 & 1.571 & 30\\ 
205195402 & 16 07 26.81 & -18 55 21.0 & 14.97 &   & 1.1$\pm$2.6 & 1.2$\pm$2.2 &   & -13.0 & -23.4 &   & $<$2 & 30\\ 
205199316 & 16 03 38.30 & -18 54 07.7 & 13.29 & 9.54 & -9.6$\pm$2.1 & -18.9$\pm$2.1 & 7.3$\pm$1.3$^{(1)}$ & -13.2 & -23.4 & 92 & 0.773 & 1\\ 
205203376 & 16 09 29.20 & -18 52 53.7 & 11.74 & 8.38 & -9.0$\pm$2.2 & -20.9$\pm$2.1 & 8.6$\pm$1.6$^{(1)}$ & -12.8 & -23.5 & 93 & 12.055 & 0\\ 
205207894 & 16 03 39.22 & -18 51 29.3 & 19.08 & 10.2 & -10.0$\pm$2.0 & -21.0$\pm$2.0 & 6.9$\pm$1.3$^{(1)}$ & -13.2 & -23.4 & 94 & 10.501 & 1\\ 
205208701 & 16 06 42.66 & -18 51 14.0 &   & 13.18 & 310.7$\pm$7.4 & 183.2$\pm$7.4 &   & -13.0 & -23.4 &   & 0.907 & 3\\ 
205216176 & 16 09 50.60 & -18 48 52.1 &   & 13.01 &   &   &   & -12.8 & -23.5 &   & 0.42 & 3\\ 
205217412 & 16 13 58.15 & -18 48 29.0 & 13.48 & 9.88 & -5.8$\pm$2.1 & -23.3$\pm$2.1 & 6.2$\pm$1.1$^{(1)}$ & -12.5 & -23.6 & 88 & 2.078 & 30\\ 
205218826 & 16 09 36.54 & -18 48 00.9 & 14.84 & 10.28 & -9.0$\pm$2.2 & -28.4$\pm$2.0 & 8.8$\pm$1.6$^{(1)}$ & -12.8 & -23.5 & 94 & 1.732 & 30\\ 
205228053 & 16 03 37.78 & -18 45 08.4 & 13.59 & 9.81 & -11.5$\pm$2.1 & -20.3$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -13.2 & -23.3 & 94 & 7.664 & 1\\ 
205232450 & 16 01 59.87 & -18 43 45.6 & 14.08 & 10.18 & -11.5$\pm$2.0 & -23.0$\pm$2.0 & 6.4$\pm$1.2$^{(1)}$ & -13.3 & -23.3 & 95 & 15.236 & 1\\ 
205238942 & 16 06 47.94 & -18 41 43.8 & 11.89 & 8.98 & -9.6$\pm$2.1 & -17.2$\pm$2.1 & 5.7$\pm$1.0$^{(1)}$ & -13.0 & -23.4 & 81 & 9.322 & 1\\ 
205241182 & 16 10 46.36 & -18 40 59.9 &   & 11.27 & -13.0$\pm$4.6 & -30.2$\pm$4.6 & 46.3$\pm$8.5$^{(4)}$ & -12.7 & -23.5 & 26 & 2.139 & 30\\ 
205247191 & 16 10 30.08 & -18 39 06.5 & 15.29 & 10.55 & -8.9$\pm$2.0 & -26.1$\pm$2.0 & 11.4$\pm$2.1$^{(1)}$ & -12.8 & -23.5 & 90 & 3.906 & 30\\ 
205249328 & 16 11 31.35 & -18 38 26.0 & 12.38 & 5.78 & 5.7$\pm$1.2 & -15.2$\pm$1.1 &   & -12.7 & -23.5 &   & 5.775 & 8\\ 
205260089 & 16 13 47.50 & -18 35 00.5 & 14.31 & 9.91 & -6.6$\pm$2.1 & -51.0$\pm$2.4 &   & -12.5 & -23.5 &   & 7.448 & 30\\ 
205327575 & 16 38 28.65 & -18 13 13.7 & 6.61 & 5.69 & -14.0$\pm$0.0 & -20.3$\pm$0.0 & 6.7$\pm$0.6$^{(0)}$ & -10.9 & -23.9 & 95 &   & 2\\ 
205355375 & 16 11 18.21 & -18 03 58.6 &   & 11.76 & -8.6$\pm$4.9 & -27.7$\pm$4.9 & 2.4$\pm$0.4$^{(4)}$ & -12.7 & -23.4 &   & 1.157 & 30\\ 
205358744 & 16 08 36.59 & -18 02 49.7 & 16.72 & 11.75 & -11.6$\pm$2.7 & -26.0$\pm$2.7 & 10.1$\pm$1.9$^{(1)}$ & -12.9 & -23.4 & 95 & 1.336 & 17\\ 
205359167 & 16 08 31.38 & -18 02 41.5 & 12.09 & 8.9 & -12.5$\pm$2.2 & -21.6$\pm$2.2 & 6.9$\pm$1.3$^{(1)}$ & -12.9 & -23.4 & 96 & 9.322 & 5\\ 
205364526 & 16 12 48.93 & -18 00 52.5 & 14.33 & 10.36 & -7.1$\pm$2.1 & -20.4$\pm$2.1 & 6.8$\pm$1.2$^{(1)}$ & -12.6 & -23.5 & 91 &   & 30\\ 
205366676 & 16 09 59.34 & -18 00 09.1 & 14.41 & 10.34 & -11.4$\pm$2.1 & -24.7$\pm$2.1 & 7.9$\pm$1.5$^{(1)}$ & -12.8 & -23.4 & 97 & 3.687 & 30\\ 
205374937 & 16 11 18.13 & -17 57 28.8 & 13.46 & 9.33 & -5.1$\pm$2.2 & -23.4$\pm$2.2 & 12.4$\pm$2.3$^{(1)}$ & -12.7 & -23.4 & 73 & 0.272 & 30\\ 
205375290 & 16 11 15.34 & -17 57 21.4 & 12.75 & 9.2 & -6.4$\pm$2.2 & -24.2$\pm$2.2 & 7.5$\pm$1.4$^{(1)}$ & -12.7 & -23.4 & 92 & 6.034 & 30\\ 
205378839 & 16 07 14.93 & -17 56 09.7 & 7.77 & 7.4 & -8.2$\pm$0.1 & -21.7$\pm$0.1 &   & -12.9 & -23.3 &   &   & 2\\ 
205383125 & 16 09 53.62 & -17 54 47.4 & 15.98 & 11.53 & -5.3$\pm$2.1 & -20.7$\pm$2.1 & 6.5$\pm$1.2$^{(1)}$ & -12.8 & -23.4 & 85 & 18.859 & 30\\ 
205412155 & 16 24 25.99 & -17 44 42.9 & 9.43 & 8.06 & -2.7$\pm$0.1 & -9.1$\pm$0.1 & 5.8$\pm$0.3$^{(0)}$ & -11.8 & -23.7 &   &  & 2\\ 
205431266 & 16 13 25.77 & -17 37 35.6 & 15.34 & 11.4 & -7.0$\pm$2.1 & -27.9$\pm$2.1 & 4.5$\pm$0.8$^{(1)}$ & -12.5 & -23.4 & 33 & 0.395 & 17\\ 
205480850 & 16 07 51.37 & -17 18 23.2 & 13.73 & 10.04 & -8.5$\pm$2.0 & -21.4$\pm$2.0 & 6.4$\pm$1.2$^{(1)}$ & -12.9 & -23.3 & 93 & 6.248 & 1\\ 
205483258 & 16 23 24.55 & -17 17 27.1 & 13.24 & 9.65 & -16.9$\pm$2.4 & -27.7$\pm$2.4 & 7.0$\pm$1.3$^{(1)}$ & -11.9 & -23.6 & 95 & 5.66 & 1\\ 
205516909 & 16 13 07.63 & -17 03 52.5 &   & 12.72 & 46.7$\pm$15.4 & 8.0$\pm$15.4 &   & -12.5 & -23.4 &   &  & 17\\ 
205517382 & 16 32 24.32 & -17 03 40.1 & 11.41 & 7.96 & 0.3$\pm$2.4 & -24.2$\pm$2.4 &   & -11.3 & -23.7 &   & 3.358 & 0\\ 
205519771 & 16 07 14.02 & -17 02 42.7 & 14.63 & 10.75 & -9.0$\pm$2.0 & -21.7$\pm$2.0 & 5.1$\pm$0.9$^{(1)}$ & -12.9 & -23.3 & 81 & 4.951 & 1\\ 
205529382 & 16 25 28.60 & -16 58 50.9 & 17.82 & 12.62 & -9.2$\pm$2.9 & -19.5$\pm$2.9 & 8.2$\pm$1.5$^{(1)}$ & -11.7 & -23.6 & 93 & 0.887 & 18\\ 
205629892 & 16 29 39.35 & -16 14 57.2 & 15.04 & 11.19 & -36.2$\pm$2.2 & -11.7$\pm$2.2 &   & -26.2 & -16.9 &   & 4.614 & 17\\ 
205634171 & 16 32 35.87 & -16 12 57.8 & 13.3 & 9.56 & -7.7$\pm$2.4 & -7.1$\pm$2.4 & 6.3$\pm$1.2$^{(1)}$ & -25.2 & -16.9 & 6 & 45.748 & 1\\ 
210282513 & 16 12 27.65 & -21 56 40.7 &   &   &   &   &   & -12.8 & -23.8 &   &   & 28\\ 
210282514 & 16 26 19.41 & -24 27 43.9 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282515 & 16 27 46.54 & -24 05 59.2 &   &   &   &   &   & -11.8 & -24.3 &   &   & 20\\ 
210282516 & 16 26 03.28 & -24 30 25.9 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282517 & 16 28 10.45 & -24 24 20.1 &   &   &   &   &   & -11.8 & -24.3 &   &   & 20\\ 
210282521 & 15 59 14.52 & -26 06 18.2 & 11.84 &   & -15.8$\pm$1.0 & -24.4$\pm$1.0 &   & -13.9 & -23.8 &   & $<$2 & 10\\ 
210282525 & 16 12 33.53 & -25 43 28.1 & 14.6 &   & 1.0$\pm$2.1 & -14.3$\pm$2.1 &   & -12.9 & -24.1 &   &   & 1\\ 
210282528 & 16 33 34.97 & -18 32 54.0 & 14.22 &   & -2.2$\pm$2.1 & -26.3$\pm$2.1 &   & -11.2 & -23.9 &   &   & 1\\ 
210282534 & 16 26 58.51 & -24 45 36.9 & 13.94 &   & -12.8$\pm$3.1 & -26.7$\pm$3.0 &   & -11.9 & -24.3 &   &   & 16\\ 
210282539 & 16 08 43.00 & -22 45 16.0 & 20.26 &   &   &   &   & -13.1 & -23.8 &   &   & 29\\ 
210282540 & 16 09 18.00 & -22 29 24.0 &   &   &   &   &   & -13.0 & -23.8 &   &   & 29\\ 
210282541 & 16 26 03.00 & -24 30 26.0 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282542 & 16 26 18.00 & -24 29 51.0 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282543 & 16 26 19.00 & -24 27 44.0 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282550 & 16 27 14.00 & -24 31 32.0 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282551 & 16 27 25.00 & -24 37 29.0 &   &   &   &   &   & -11.9 & -24.3 &   &   & 20\\ 
210282554 & 16 27 47.00 & -24 46 46.0 &   &   &   &   &   & -11.8 & -24.4 &   &   & 20\\ 
210282557 & 16 28 10.00 & -24 24 20.0 &   &   &   &   &   & -11.8 & -24.3 &   &   & 20\\ 
\enddata 
 \tablecomments{ (0)  Pecaut \& Mamajek (2016), (1)  Rizzuto et al. (2015), (2)  Rizzuto et al. (2011), (3)  Luhman \& Mamajek (2012), (4)  Aarnio et al. (2008), (5)  Preibisch et al. (1998), (6)  Chen et al. (2011), (7)  Martin et al. (2004), (8)  Gregorio-Hetem et al. (1992), (9)  Meyer et al. ((1993), (10)  Kunkel (1999), (11)  Martin (1998), (12)  Bouvier \& Appenzeller (1992), (13)  Martin et al. (1998), (14)  Kraus \& Hillenbrand (2009), (15)  Lodieu et al. (2006), (16)  Erickson et al. (2011), (17)  Slesnick et al. (2008), (18)  Slesnick et al. (2006), (19)  Wilking et al. (2005), (20)  Alves de Oliveira (2010), (21)  Cieza et al. (2010), (22)  Luhman \& Rieke (1999), (23)  Doppmann et al. (2003), (24)  Natta et al. (2002), (25)  Elias et al. (1978), (26)  Walter et al. (1994), (27)  Ardila et al. (2000), (28)  Lodieu et al. (2011), (29)  Lodieu et al. (2008), (30)  Preibisch et al. (2002), (31)  Herbig \& Bell (1988), (32)  Vieira et al. (2003).
} 
 \label{USKmemtab} 
 \end{deluxetable} 


==> shortmemtab.tex <==
\begin{deluxetable*}{cccccccccccc} 
\tabletypesize{\scriptsize} 
 \tablecaption{Candidate members in the young clusters and associations observed by \emph{K2}.} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{$\pi$}  & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} \\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} \\ } 
 \startdata 
\multicolumn{12}{l}{\bf Hyades Candidate Members} \\
210317378 & 03 52 34.34 & +11 15 38.8 & 12.42 & 9.01 & 179.36$\pm$1.64 & -5.5$\pm$1.64 & 29.7$\pm$4.1$^{(1)}$ & 136.6 & -1.9 & 89 &  \\ 
210359769 & 03 55 01.44 & +12 29 08.1 & 9.68 & 7.57 & 131.22$\pm$0.17 & -10.25$\pm$0.08 & 21.8$\pm$0.2$^{(0)}$ & 136.8 & -5.6 & 100 &  \\ 
210365286 & 03 58 14.38 & +12 37 40.9 & 14.87 & 10.99 & 129.36$\pm$2.16 & -12.5$\pm$2.16 & 24.9$\pm$3.4$^{(1)}$ & 132.8 & -6.3 & 99 & 0.8686\\ 
\enddata 
 \tablecomments{Membership information for all the cluster candidates with probabilities of membership $>$10\% and all spectroscopically confirmed members of Upper Scorpius. The complete table is available online. G-band magnitudes are taken from Gaia DR1 \citep{gaiadr1}, and K-band magnitudes from 2MASS \citep{2mass}. Proper motions are taken in order of availability from the Tycho-Gaia Astrometric Solution \citep{gaiadr1}, \emph{Hipparcos} \citep{perrymantycho, leeuwen07}, UCAC4 \citep{ucac4} and PPMXL \citep{ppmxl}. We indicated the source of the parallax measurement, with (0) indicating a true measurement from either TGAS or \emph{Hipparcos}, and larger numbers indicating photometric distances based on the cluster sequences: (1) (G,G-J) photometry, (2) - (r,r-J) photometry, (3) (V,V-K) photometry, (4) (K, J-K) photometry. We also list the expected proper motions if the candidate shares the model space velocity vector of the cluster model. Finally, rotation period measurements from Covey et al., (private communication) for Upper Scorpius, \citet{rebull16_plei} for Pleiades, \citet{douglas16} for Hyades, and \citet{douglas17} for Praesepe candidates are listed if available in the literature. Candidates not considered in these studies were visually inspected for rotation periods smaller that 2\,days, which would impact the choice of detrending window. These objects are marked as ``$<$2'' in the table.}
 \label{shortmemtab} 
 \end{deluxetable*} 


==> testtable.tex <==
\begin{deluxetable}{cccccccccccccc} 
\tabletypesize{\scriptsize} 
\onecolumngrid 
 \tablecaption{Stuff} 
\tablehead{ \colhead{EPIC} & \colhead{R.A.}    & \colhead{Decl.}   & \colhead{G}     & \colhead{K}    & \colhead{PMRA}     & \colhead{PMDE}    & \colhead{PLX}   & \colhead{P$_{s}$} & \colhead{PMRA$_c$} & \colhead{PMDE$_c$} & \colhead{P$_{m}$} & \colhead{P$_R$} &\colhead{Ref}\\ 
 \colhead{}     & \colhead{(J2000)} & \colhead{(J2000)} & \colhead{(mag)} & \colhead{(mag)}& \colhead{(mas/yr)} & \colhead{(mas/yr)} & \colhead{(mas)} & \colhead{}            & \colhead{(mas/yr)} & \colhead{(mas/yr)}  &  \colhead{(\%)}    & \colhead{(days)} &\colhead{}\\ 
 } 
\startdata 
202522205 & 16 13 17.38 & -29 22 19.9 & 12.39 & 8.91 & -21.36$\pm$2.37 & -25.25$\pm$2.36 & 9.08$\pm$1.67 & 1 & -13.02 & -24.38 & 88 & $<$2 &  (Pecaut \& Mamajek 2016)\\ 
\enddata 
\tablecomments{stuff} 
\label{USKmemtab} 
\end{deluxetable} 

